Matching Anonymized and Obfuscated Time Series to Users' Profiles

Many popular applications use traces of user data to offer various services to their users. However, even if user data is anonymized and obfuscated, a user's privacy can be compromised through the use of statistical matching techniques that match a user trace to prior user behavior. In this work, we derive the theoretical bounds on the privacy of users in such a scenario. We build on our recent study in the area of location privacy, in which we introduced formal notions of location privacy for anonymization-based location privacy-protection mechanisms. Here we derive the fundamental limits of user privacy when both anonymization and obfuscation-based protection mechanisms are applied to users' time series of data. We investigate the impact of such mechanisms on the trade-off between privacy protection and user utility. We first study achievability results for the case where the time-series of users are governed by an i.i.d. process. The converse results are proved both for the i.i.d. case as well as the more general Markov chain model. We demonstrate that as the number of users in the network grows, the obfuscation-anonymization plane can be divided into two regions: in the first region, all users have perfect privacy; and, in the second region, no user has privacy.

==> Revised paper/conclusion.tex <==
\section{Discussion}
\label{discussion}
\subsection{Markov Chain Model}
\label{markov}
As opposed to the i.i.d.\ case, we see from Section \ref{sec:perfect-MC} that if we do not limit $m=m(n)$, the assumed obfuscation method will not be sufficient to achieve perfect privacy. There are a few natural questions here. First, for a given noise level, what would be the maximum $m(n)$ that could guarantee perfect privacy in this model? The more interesting question is, how can we possibly modify the obfuscation technique to make it more suitable for the Markov chain model? A natural solution seems to be re-generating the obfuscation random variables $R_u$ periodically. This will keep the adversary from easily estimating them by observing a long sequence of data at a small increase in complexity. In fact, this will make the obfuscation much more \emph{robust} to modeling uncertainties and errors. It is worth noting, however, that this change would not affect the other results in the paper. That is, even if the obfuscation random variables are re-generated frequently, it is relatively easy to check that all the previous theorems in the paper remain valid. However, the increase in robustness to modeling errors will definitely be a significant advantage. Thus, the question is how often should the random variable $R_u$ be re-generated to strike a good balance between complexity and privacy? These are all interesting questions for future research.


\subsection{Obfuscating the Samples of Users' Data Using Continuous Noise}
Here we argue that for the setting of this paper, continuous noise such as that drawn from a Gaussian distribution is not a good option to obfuscate the sample of users' data drawn from a finite alphabet when we want to achieve perfect privacy. For a better understanding, let's consider a simple example.
\begin{example}
Consider the scenario where the users' datasets are governed by an i.i.d.\ model and the number of possible values for each sample of the users' data ($r$) is equal to 2 (two-states model). Note that the data sequence for user $u$ is a Bernoulli random variable with parameter $p_u$.

Assume that the actual sample of the data of user $u$ at time $k$ ($X_u(k)$) is obfuscated using noise drawn from a Gaussian distribution ($S_u(k)$), and $Z_u(k)$ is the obfuscated version of $X_u(k)$.  That is, we can write
\[Z_u(k)=X_u(k)+S_u(k); \ \ \ \ \  S_u(k) \sim N\left(0, R_u\right), \]
where $R_u$ is chosen from some distribution. For simplicity, we can consider $R_u\sim N\left(0, a^2_n\right)$ where $a_n$ is the noise level.

We also apply anonymization to $Z_u(k)$, and, as before, $Y_u(k)$ is the reported sample of the data of user $u$ at time $k$ after applying anonymization.  Per Section \ref{sec:framework}, anonymization is modeled by a random permutation $\Pi(u)$ on the set of $n$ users.

Now, the question is as follows: Is it possible to achieve perfect privacy independent of the number of adversary's observation ($m$) while using this continuous noise ($S_u(k)$) to obfuscate the sample of users' data?

Note that the density function of the reported sample of the data of user $u$ after applying obfuscation is
\begin{align}
%\nonumber
\no f_{Z_u}(z)&= p_u f_{S_u(k)}(z-1)+(1-p_u) f_{S_u(k)}(z) \\
\nonumber &= p_u \frac{1}{\sqrt{2\pi}R_u}e^{-\frac{(z-1)^2}{2R_u}}+(1-p_u)\frac{1}{\sqrt{2\pi}R_u}e^{-\frac{z^2}{2R_u}}.\ \
\end{align}
In this case, when the adversary's number of observations is large, the adversary can estimate the values of $P_u$ and $R_u$ for each user with an arbitrarily small error probability. As a result, the adversary can de-anonymize the data and then recover $X_u(k)$. The conclusion here is that a continuous noise distribution gives too much information to the adversary when used for obfuscation of finite alphabet data. A method to remedy this issue is to regenerate the random variables $R_u$ frequently (similar to our previous discussion for Markov chains). Understanding the optimal frequency of such a regeneration and detailed analysis in this case is an interesting future research direction.
\end{example}

%As a result, when we have finite alphabet possibilities for the sample of users' data and use continous noise to obfuscate the sample of users' data, the adversary has too much information to recover the sample of users' data. Thus it is not a good option to achieve perfect privacy.


\subsection{Relation to Differential Privacy}
Differential privacy is mainly used when there is a statistical database of users' sensitive information, and the goal is to protect an individual's data while publishing aggregate information about the database \cite{ lee2012differential, bordenabe2014optimal, chatzikokolakis2015geo, nguyen2013differential, machanavajjhala2008privacy, kousha2}. The goal of differential privacy is publishing aggregate queries with low sensitivity, which means the effect of changes in a single individual on the outcome of the aggregated information is negligible.

In \cite{geo2013} three different approaches for differential privacy are presented. The one that best matches our setting is stated as
\begin{align*}
\frac{P(X_1(k)=x_1|\textbf{Y})}{P(X_1(k)=x_2|\textbf{Y})} \leq e^{\epsilon_r}\frac{P(X_1(k)=x_1)}{P(X_1(k)=x_2)},
\end{align*}
where $\textbf{Y}$ is the set of reported datasets.
It means $\textbf{Y}$ has a limited effect on the probabilities assigned by the attacker. In differential privacy, user $1$ has strongest differential privacy when $\epsilon_r=0$.

In Lemma \ref{lem4}, we proved that if user $1$ has perfect privacy, this implies that asymptotically (for large enough $n$)
\begin{align}\label{eq1}
P\left(X_1(k)=x_1 \big{|} \textbf{Y}\right)\rightarrow P\left(X_1(k)=x_1\right).
\end{align}
\begin{align}\label{eq2}
P\left(X_1(k)=x_2 \big{|} \textbf{Y}\right)\rightarrow P\left(X_1(k)=x_2\right).
\end{align}

As a result, by using (\ref{eq1}) and (\ref{eq2}), we can conclude that if we satisfy the perfect privacy condition given in this paper, we also satisfy differential privacy with $\epsilon_r=0$, i.e., the strongest case of differential privacy.




\section{Conclusions}
In this paper, we have considered both obfuscation and anonymization techniques to achieve privacy.  The privacy level of the users depends on both $m(n)$ (number of observations per user by the adversary for a fixed anonymization mapping) and $a_n$ (noise level). That is, larger $m(n)$ and smaller $a_n$ indicate weaker privacy.  We characterized the limits of privacy in the entire $m(n)-a_n$ plane for the i.i.d.\ case; that is, we obtained the exact values of the thresholds for $m(n)$ and $a_n$ required for privacy to be maintained.  We showed that if $m(n)$ is fewer than $O\left(n^{\frac{2}{r-1}}\right)$, or $a_n$ is larger than $\Omega\left(n^{-\frac{1}{r-1}}\right)$, users have perfect privacy. On the other hand, if neither of these two conditions is satisfied, users have no privacy. For the case where the users' patterns are modeled by Markov chains, we obtained a no-privacy region in the $m(n)-a_n$ plane.

Future research in this area needs to characterize the exact privacy/no-privacy regions when user data sequences obey Markov models. It is also important to consider different ways to obfuscate users' data sets and study the utility-privacy trade-offs for different types of obfuscation techniques.


==> Revised paper/framework-1.tex <==
\section{Framework}
\label{sec:framework}
In this paper, we adopt a similar framework to that employed in~\cite{tifs2016,ciss2017}.  The general set up is provided here, and the refinement to the precise models for this paper will be presented in the following sections.  We assume a system with $n$ users with $X_u(k)$ denoting a sample of the data of user $u$ at time $k$, which we would like to protect from an interested adversary $\mathcal{A}$. We consider a strong adversary $\mathcal{A}$ that has complete statistical knowledge of the users' data patterns based on the previous observations or other resources. In order to secure data privacy of users, both obfuscation and anonymization techniques are used as shown in Figure \ref{fig:xyz}. In Figure \ref{fig:xyz}, $Z_u(k)$ shows the (reported) sample of the data of user $u$ at time $k$ after applying obfuscation, and $Y_u(k)$ shows the (reported) sample of the data of user $u$ at time $k$ after applying anonymization. The adversary observes only $Y_u(k)$, $k=1,2,\cdots, m(n)$, where $m(n)$ is the number of observations of each user before the identities are permuted. The adversary then tries to estimate $X_u(k)$ by using those observations.
\begin{figure}[h]
	\centering
	\includegraphics[width = 0.75\linewidth]{fig/xyz}
	\caption{Applying obfuscation and anonymization techniques to users' data samples.}
	\label{fig:xyz}
\end{figure}

Let $\textbf{X}_u$ be the $m(n) \times 1$ vector containing the sample of the data of user $u$, and $\textbf{X}$ be the $m(n) \times n$ matrix with $u^{th}$ column equal to $\textbf{X}_u$;
\[\textbf{X}_u = \begin{bmatrix}
X_u(1) \\ X_u(2) \\ \vdots \\X_u(m) \end{bmatrix} , \ \ \  \textbf{X} =\left[\textbf{X}_{1}, \textbf{X}_{2}, \cdots,  \textbf{X}_{n}\right].
\]


\textit{Data Samples Model:}
We assume there are $r \geq 2$ possible values ($0,1, \cdots, r-1$) for each sample of the users' data. In the first part of the paper (perfect privacy analysis), we assume an i.i.d.\ model as motivated in Section \ref{intro}. In the second part of the paper (converse results: no privacy region), the users' datasets are governed by irreducible and aperiodic Markov chains. At any time, $X_u(k)$ is equal to a value in $\left\{0,1, \cdots, r-1 \right\}$ according to a user-specific probability distribution. The collection of user distributions, which satisfy some mild regularity conditions discussed below, is known to the adversary $\mathcal{A}$, and he/she employs such to distinguish different users based on statistical matching of those user distributions to traces of user activity of length $m(n)$.%In any case, any dependency can only favor the adversary, so our results provide lower bounds on the achievable privacy in those settings, which would be desirable if the dependency is poorly understood.  Second, understanding the i.i.d.\ case can be considered the first step toward understanding the more complicated case where there is a dependency, as was done for anonymization-only LPPMs in \cite{tifs2016} to consider perfect privacy when users' data pattern are governed by Markov chains. In the second part of the paper, in addition to the above model, we consider the case where users' data patterns are modeled by Markov chains as discussed in Section \ref{subsec:markov}.%





\textit{Obfuscation Model:} The first step in obtaining privacy is to apply the obfuscation operation in order to perturb the users' data samples. In this paper, we assume that each user has only limited knowledge of the characteristics of the overall population and thus we employ a simple distributed method in which the samples of the data of each user are reported with error with a certain probability, where that probability itself is generated randomly for each user. In other words, the obfuscated data is obtained by passing the users' data through an $r$-ary symmetric channel with a random error probability. More precisely, let $\textbf{Z}_u$ be the vector which contains
%$m$ number of
the obfuscated versions of user $u$'s data samples, and $\textbf{Z}$ is the collection of $\textbf{Z}_u$ for all users,
\[\textbf{Z}_u = \begin{bmatrix}
Z_u(1) \\ Z_u(2) \\ \vdots \\Z_u(m) \end{bmatrix} , \ \ \  \textbf{Z} =\left[ \textbf{Z}_{1}, \textbf{Z}_{2}, \cdots,  \textbf{Z}_{n}\right].
\]
To create a noisy version of data samples, for each user $u$, we independently generate a random variable $R_u$ that is uniformly distributed between $0$ and $a_n$, where $a_n \in (0,1]$. The value of $R_u$ gives the probability that a user's data sample is changed to a different data sample by obfuscation, and $a_n$ is termed the ``noise level'' of the system. For the case of $r=2$ where there are two states for users' data (state $0$ and state $1$), the obfuscated data is obtained by passing users' data through a Binary Symmetric Channel (BSC) with a small error probability~\cite{randomizedresponse}. Thus, we can write
\[
{Z}_{u}(k)=\begin{cases}
{X}_{u}(k), & \textrm{with probability } 1-R_u.\\
1-{X}_{u}(k),& \textrm{with probability } R_u.
\end{cases}
\]
When $r>2$, for $l \in \{0,1,\cdots, r-1\}$:
\[
P({Z}_{u}(k)=l| X_{u}(k)=i) =\begin{cases}
1-R_u, & \textrm{for } l=i.\\
\frac{R_u}{r-1}, & \textrm{for } l \neq i.
\end{cases}
\]
Note that the effect of the obfuscation is to alter the probability distribution function of each user across the $r$ possibilities in a way that is unknown to the adversary, since it is independent of all past activity of the user, and hence the obfuscation inhibits user identification. For each user, $R_u$ is generated once and is kept constant for the collection of samples of length $m(n)$, thus, providing a very low-weight obfuscation algorithm. We will discuss the extension to the case where $R_u$ is regenerated independently over time in Section \ref{sec:perfect-MC}. There, we will also provide a discussion about obfuscation using continuous noise distributions (e.g., Gaussian noise).

\textit{Anonymization Model:} Anonymization is modeled by a random permutation $\Pi$ on the set of $n$ users. The user $u$ is assigned the pseudonym $\Pi(u)$. $\textbf{Y}$ is the anonymized version of $\textbf{Z}$; thus,
\begin{align}
\no \textbf{Y} &=\textrm{Perm}\left(\textbf{Z}_{1}, \textbf{Z}_{2}, \cdots,  \textbf{Z}_{n}; \Pi \right) \\
\nonumber &=\left[ \textbf{Z}_{\Pi^{-1}(1)}, \textbf{Z}_{\Pi^{-1}(2)}, \cdots,  \textbf{Z}_{\Pi^{-1}(n)}\right ] \\
\nonumber &=\left[ \textbf{Y}_{1}, \textbf{Y}_{2}, \cdots, \textbf{Y}_{n}\right], \ \
\end{align}
where $\textrm{Perm}( \ . \ , \Pi)$ is permutation operation with permutation function $\Pi$. As a result, $\textbf{Y}_{u} = \textbf{Z}_{\Pi^{-1}(u)}$ and $\textbf{Y}_{\Pi(u)} = \textbf{Z}_{u}$.

\textit{Adversary Model:} We protect against the strongest reasonable adversary. Through past observations or some other sources, the adversary is assumed to have complete statistical knowledge of the users' patterns; in other words, he/she knows the probability distribution for each user on the set of data samples $\{0,1,\ldots,r-1\}$. As discussed in the model for the data samples, the parameters $\textbf{p}_u$, $u=1, 2, \cdots, n$ are drawn independently from a continuous density function, $f_\textbf{P}(\textbf{p}_u)$, which has support on a subset of a defined hypercube. The density $f_\textbf{P}(\textbf{p}_u)$ might be unknown to the adversary, as all that is assumed here is that such a density exists, and it will be evident from our results that knowing or not knowing $f_\textbf{P}(\textbf{p}_u)$ does not change the results asymptotically. Specifically, from the results of Section \ref{perfectsec}, we conclude that user $u$ has perfect privacy even if the adversary knows $f_\textbf{P}(\textbf{p}_u)$. In addition, in Section \ref{converse}, it is shown that the adversary can recover the true data of user $u$ at time $k$ without using the specific density function of $f_\textbf{P}(\textbf{p}_u)$, and as result, users have no privacy even if the adversary does not know $f_\textbf{P}(\textbf{p}_u)$.

The adversary also knows the value of $a_n$ as it is a design parameter. However, the adversary does not know the realization of the random permutation $\Pi$ or the realizations of the random variables $R_u$, as these are independent of the past behavior of the users. It is critical to note that we assume the adversary does not have any auxiliary information or side information about users' data.


In \cite{tifs2016}, perfect privacy is defined as follows:
\begin{define}
User $u$ has \emph{perfect privacy} at time $k$, if and only if
\begin{align}%\label{}
\no  \forall k\in \mathbb{N}, \ \ \ \lim\limits_{n\rightarrow \infty} I \left(X_u(k);{\textbf{Y}}\right) =0,
\end{align}
where $I(X;Y)$ denotes the mutual information between random variables (vectors) $X$ and $Y$.
\end{define}

\noindent In this paper, we also consider the situation in which there is no privacy. 

\begin{define}
For an algorithm for the adversary that tries to estimate the actual sample of data of user $u$ at time $k$, define
\[P_e(u,k)\triangleq P\left(\widetilde{X_u(k)} \neq X_u(k)\right),\]
where $X_u(k)$ is the actual sample of the data of user $u$ at time $k$, $\widetilde{X_u(k)}$ is the adversary's estimated sample of the data of user $u$ at time $k$, and $P_e(u,k)$ is the error probability. Now, define ${\cal E}$ as the set of all possible adversary's estimators; then, user $u$ has \emph{no privacy} at time $k$, if and only if for large enough $n$,
\[
\forall k\in \mathbb{N}, \ \ \ P^{*}_e(u,k)\triangleq \inf_{\cal E} {P\left(\widetilde{X_u(k)} \neq X_u(k)\right)} \rightarrow 0.
\]
Hence, a user has no privacy if there exists an algorithm for the adversary to estimate $X_u(k)$ with diminishing error probability as $n$ goes to infinity.
\end{define}

\textbf{\textit{Discussion:}} Both of the privacy definitions given above (perfect privacy and no privacy) are asymptotic in the number of users $(n \to \infty)$, which allows us to find clean analytical results for the fundamental limits. Moreover, in many IoT applications, such as ride sharing and dining recommendation applications, the number of users is large. %And finally, we show in the simulation section that our results provide good predictions for the behavior observed when there is a finite number of users in the system. 

\textbf{\textit{Notation:}} Note that the sample of data of user $u$ at time $k$ after applying obfuscation $\left(Z_u(k)\right)$ and the sample of data of user $u$ at time $k$ after applying anonymization $\left(Y_u(k)\right)$ depend on the number of users in the network $(n)$, while the actual sample of data of user $u$ at time $k$ is independent of the number of users $(n)$.  Despite the dependency in the former cases, we omit this subscript $(n)$ on $\left(Z_u^{(n)}(k), Y_u^{(n)}(k) \right)$ to avoid confusion and make the notation consistent.

\textbf{\textit{Notation:}} Throughout the paper, $X_n \xrightarrow{d} X$ denotes convergence in distribution. Also, We use $P\left(X=x\bigg{|} Y=y\right)$ for the conditional probability of $X=x$ given $Y=y$. When we write $P\left(X=x \bigg{|}Y\right)$, we are referring to a random variable that is defined as a function of $Y$.


\section{Perfect Privacy Analysis: I.I.D.\ Case}
\label{perfectsec}

\subsection{Two-States Model}

We first consider the two-states case $(r=2)$ which captures the salient aspects of the problem. For the two-states case, the sample of the data of user $u$ at any time is a Bernoulli random variable with parameter $p_u$, which is the probability of user $u$ having data sample $1$. Thus,
\[X_u(k) \sim Bernoulli \left(p_u\right).\]
Per Section \ref{sec:framework}, the parameters $p_u$, $u=1, 2, \cdots, n$ are drawn independently from a continuous density function, $f_P(p_u)$, on the $(0,1)$ interval. We assume there are $\delta_1, \delta_2>0$ such that:\footnote{The condition $\delta_1<f_P(p_u) <\delta_2$ is not actually necessary for the results and can be relaxed; however, we keep it here to avoid unnecessary technicalities.}
\begin{equation}
\no\begin{cases}
    \delta_1<f_P(p_u) <\delta_2, & p_u \in (0,1).\\
    f_P(p_u)=0, &  p _u\notin (0,1).
\end{cases}
\end{equation}

The adversary knows the values of $p_u$, $u=1, 2, \cdots, n$ and uses this knowledge to identify users. We will use capital letters (i.e., $P_u$) when we are referring to the random variable, and use lower case (i.e., $p_u$) to refer to the realization of $P_u$.

In addition, since the user data $\left(X_u(k)\right)$ are i.i.d.\ and have a Bernoulli distribution, the obfuscated data $\left(Z_u(k)\right)$ are also i.i.d.\ with  a Bernoulli distribution. Specifically,
\[Z_u(k) \sim Bernoulli\left(Q_u\right),\]
where
\begin{align}
\no {Q}_u &=P_u(1-R_u)+(1-P_u)R_u  \\
\nonumber &= P_u+\left(1-2P_u\right)R_u,\ \
\end{align}
and recall that $R_u$ is the probability that user $u$'s data sample is altered at any time. For convenience, define a vector where element $Q_u$ is the probability that an obfuscated data sample of user $u$ is equal to one, and
\[\textbf{Q} =\left[{Q}_{1},{Q}_{2}, \cdots,{Q}_{n}\right].\]
Thus, a vector containing the permutation of those probabilities after anonymization is given by:
\begin{align}
\no \textbf{V} &=\textrm{Perm}\left({Q}_{1}, {Q}_{2}, \cdots,  {Q}_{n}; \Pi \right) \\
\nonumber &=\left[ {Q}_{\Pi^{-1}(1)}, {Q}_{\Pi^{-1}(2)}, \cdots, {Q}_{\Pi^{-1}(n)}\right ] \\
\nonumber &=\left[{V}_{1}, {V}_{2}, \cdots, {V}_{n}\right ] ,\ \
\end{align}
where ${V}_{u} = {Q}_{\Pi^{-1}(u)}$ and  ${V}_{\Pi(u)} = {Q}_{u}$. As a result, for $u=1,2,..., n$, the distribution of the data symbols for the user with pseudonym $u$ is given by:
\[ Y_u(k) \sim Bernoulli \left(V_u\right) \sim Bernoulli\left(Q_{\Pi^{-1}(u)}\right)  .\]

The following theorem states that if $a_n$ is significantly larger than $\frac{1}{n}$ in this two-states model, then all users have perfect privacy independent of the value of $m(n)$.
\begin{thm}\label{two_state_thm}
 For the above two-states model, if $\textbf{Z}$ is the obfuscated version of $\textbf{X}$, and $\textbf{Y}$ is the anonymized version of $\textbf{Z}$  as defined above, and
\begin{itemize}
	\item $m=m(n)$ is arbitrary;
	\item $R_u \sim Uniform [0, a_n]$, where $a_n \triangleq c'n^{-\left(1-\beta\right)}$ for any $c'>0$ and $0<\beta<1$;
\end{itemize}
then, user 1 has perfect privacy. That is,
\begin{align}%\label{}
\no  \forall k\in \mathbb{N}, \ \ \ \lim\limits_{n\rightarrow \infty} I \left(X_1(k);{\textbf{Y}}\right) =0.
\end{align}
\end{thm}

The proof of Theorem \ref{two_state_thm} will be provided for the case $0\leq p_1<\frac{1}{2}$, as the proof for the case $\frac{1}{2}\leq p_1\leq1$ is analogous and is thus omitted.
\\

\noindent \textbf{Intuition behind the Proof of Theorem \ref{two_state_thm}:} 

Since $m(n)$ is arbitrary, the adversary is able to estimate very accurately (in the limit, perfectly) the distribution from which each data sequence $\textbf{Y}_u$, $u= 1, 2, \cdots, n$ is drawn; that is, the adversary is able to accurately estimate the probability $V_u$, $u= 1, 2, \cdots, n$. Clearly, if there were no obfuscation for each user $u$, the adversary would then simply look for the $j$ such that $p_j$ is very close to $V_u$ and set $\widetilde{X_j(k)}=Y_u(k)$, resulting in no privacy for any user.

We want to make certain that the adversary obtains no information about $X_1(k)$, the sample of data of user $1$ at time $k$. To do such, we will establish that there are a large number of users whom have a probability $p_u$ that when obfuscated could have resulted in a probability consistent with $p_1$. Consider asking whether another probability $p_2$ is sufficiently close enough to be confused with $p_1$ after obfuscation; in particular, we will look for $p_2$ such that, even if the adversary is given the obfuscated probabilities $V_{\Pi(1)}$ and $V_{\Pi(2)}$, he/she cannot associate these probabilities with $p_1$ and $p_2$. This requires that the distributions $Q_{1}$ and $Q_{2}$ of the obfuscated data of user $1$ and user $2$ have significant overlap; we explore this next.

Recall that $Q_u=P_u+ (1-2P_u)R_u$, and $R_u\sim Uniform [0, a_n]$. Thus, we know $Q_u {|} P_u=p_u$ has a uniform distribution with length $(1-2p_u)a_n$. Specifically,
\[Q_u\bigg{|}P_u=p_u \sim Uniform \left[p_u,p_u+(1-2p_u)a_n\right].\]
Figure \ref{fig:piqi_a} shows the distribution of $Q_u$ given $P_u=p_u$.

\begin{figure}[h]
	\centering
	\includegraphics[width = 0.8\linewidth]{fig/piqi_a}
	\caption{Distribution of $Q_u$ given $P_u=p_u$.}
	\label{fig:piqi_a}
\end{figure}

Consider two cases: In the first case, the support of the distributions $Q_1\big{|} P_1=p_1$ and $Q_2\big{|} P_2=p_2$ are small relative to the difference between $p_1$ and $p_2$ (Figure \ref{fig:case1}); in this case, given the probabilities $V_{\Pi(1)}$ and $V_{\Pi(2)}$ of the anonymized data sequences, the adversary can associate those with $p_1$ and $p_2$ without error. In the second case, the support of the distributions $Q_1\big{|} P_1=p_1$ and $Q_2\big{|} P_2=p_2$ is large relative to the difference between $p_1$ and $p_2$ (Figure \ref{fig:case2}), so it is difficult for the adversary to associate the probabilities $V_{\Pi(1)}$ and $V_{\Pi(2)}$ of the anonymized data sequences with $p_1$ and $p_2$. In particular, if $V_{\Pi(1)}$ and $V_{\Pi(2)}$ fall into the overlap of the support of $Q_1$ and $Q_2$, we will show the adversary can only guess randomly how to de-anonymize the data. Thus, if the ratio of the support of the distributions to $\big{|}p_1-p_2\big{|}$ goes to infinity, the adversary's posterior probability for each user converges to $\frac{1}{2}$, thus, implying no information leakage on the user identities. More generally, if we can guarantee that there will be a large set of users with $p_u$'s very close to $p_1$ compared to the support of $Q_1\big{|} P_1=p_1$, we will be able to obtain perfect privacy as demonstrated rigorously below.

\begin{figure}[h]
	\centering
	\includegraphics[width = 0.8\linewidth]{fig/case1}
	\caption{Case 1: The support of the distributions is small relative to the difference between $p_1$ and $p_2$.}
	\label{fig:case1}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[width = 0.8\linewidth]{fig/case2}
	\caption{Case 2: The support of the distributions is large relative to the difference between $p_1$ and $p_2$.}
	\label{fig:case2}
\end{figure}

Given this intuition, the formal proof proceeds as follows. Given $p_1$, we define a set $J^{(n)}$ of users whose parameter $p_u$ of their data distributions is sufficiently close to $p_1$ (Figure \ref{fig:case2}; case 2), so that it is likely that $Q_1$ and $Q_u$ cannot be readily associated with $p_1$ and $p_u$.

The purpose of Lemmas \ref{lemOnePointFive}, \ref{lem2}, and \ref{lem3} is to show that, from the adversary's perspective, the users in set $J^{(n)}$ are indistinguishable. More specifically, the goal is to show that the obfuscated data corresponding to each of these users could have been generated by any other users in $J^{(n)}$ in an equally likely manner. To show this, Lemma \ref{lemOnePointFive} employs the fact that, if the observed values of $N$ uniformly distributed random variables ($N$ is size of set $J^{(n)}$) are within the intersection of their ranges, it is impossible to infer any information about the matching between the observed values and the distributions. That is, all possible $N!$ matchings are equally likely. Lemmas \ref{lem2} and \ref{lem3} leverage Lemma \ref{lemOnePointFive} to show that even if the adversary is given a set that includes all of the pseudonyms of the users in set $J^{(n)}$  (i.e., $\Pi(J^{(n)})\overset{\Delta}{=} \left\{\Pi^{-1}(u) \in J^{(n)}\right\}$) he/she still will not be able to infer any information about the matching of each specific user in set $J^{(n)}$ and his pseudonym. Then Lemma \ref{lem4} uses the above fact to show that the mutual information between the data set of user $1$ at time $k$ and the observed data sets of the adversary converges to zero for large enough $n$.

%Remember that the adversary does not know the realization of the random permutation $\Pi$ as well as the realizations of random variables  $R_u^{(n)}$. Therefore, the adversary does not know the realizations of random variables ${V}_{u}^{(n)}$ defined above.
%Then by using lemma \ref{lem2}, \ref{lem3}, and \ref{lem4} we try to prove that the the mutual information between data set of user $1$ at time $k$ and the observed data sets by the adversary will  go to zero for large enough $n$.

\noindent \textbf{Proof of Theorem \ref{two_state_thm}:}

\begin{proof}
Note, per Lemma~\ref{lemx} of Appendix \ref{sec:app_a}, it is sufficient to establish the results on a sequence of sets with high probability. That is, we can condition on high-probability events.

Now, define the critical set $J^{(n)}$ with size $N^{(n)}=\big{|}J^{(n)}\big{|}$ for $0\leq p_1<\frac{1}{2}$ as follows:
\[J^{(n)}=
\left\{  u \in \{1, 2, \dots, n\}: p_1 \leq P_u\leq p_1+\epsilon_n;  p_1+\epsilon_n\leq Q_u\leq p_1+(1-2p_1)a_n\right\},
\]
where $\epsilon_n \triangleq \frac{1}{n^{1-\frac{\beta}{2}}}$, $a_n= c'n^{-\left(1-\beta\right)}$ ,and $\beta$ is defined in the statement of Theorem \ref{two_state_thm}.


Note for large enough $n$, if $0\leq p_1<\frac{1}{2}$, we have $0\leq p_u<\frac{1}{2}$. As a result,
\[Q_u\bigg{|}P_u=p_u \sim Uniform \left(p_u,p_u+(1-2p_u)a_n\right).\]
We can prove that with high probability, $1 \in J^{(n)}$ for large enough $n$, as follows. First, Note that
\[Q_1\bigg{|}P_1=p_1 \sim Uniform \left(p_1,p_1+(1-2p_1)a_n\right).\]
Now, according to Figure \ref{fig:piqi_c},
	\begin{align}
	\no P\left(1 \in J^{(n)} \right) &= 1- \frac{\epsilon_n}{ \left(1-2p_1 \right)a_n}\\
	\nonumber &= 1- \frac{1}{ \left(1-2p_1 \right)c'n^{\frac{\beta}{2}}}, \ \
	\end{align}
thus, for any $c'>0$ and large enough $n$,
\begin{align}
	\no P\left(1 \in J^{(n)} \right) \to 1.
\end{align}
\begin{figure}[h]
	\centering
	\includegraphics[width = 0.8\linewidth]{fig/piqi_b}
	\caption{Range of $P_u$ and $Q_u$ for elements of set $J^{(n)}$ and probability density function of $Q_u\bigg{|}P_u=p_u$.}
	\label{fig:piqi_b}
\end{figure}

\begin{figure}[h]
	\centering
	\includegraphics[width = 0.8\linewidth]{fig/piqi_c}
	\caption{Range of $P_u$ and $Q_u$ for elements of set $J^{(n)}$ and probability density function of $Q_1\bigg{|}P_1=p_1$.}
	\label{fig:piqi_c}
\end{figure}




Now in the second step, we define the probability $W_j^{(n)}$ for any $j \in \Pi(J^{(n)})=\{\Pi(u): u \in J^{(n)} \}$ as
\[W_j^{(n)}= P\left(\Pi(1)=j \bigg{|} \textbf{V}, \Pi (J^{(n)})\right).\]
$W_j^{(n)}$ is the conditional probability that $\Pi(1)=j$ after perfectly observing the values of the permuted version of obfuscated probabilities ($\textbf{V}$) and set including all of the pseudonyms of the users in set $J^{(n)}$ $\left(\Pi(J^{(n)})\right)$. Since $\textbf{V}$ and $\Pi (J^{(n)})$ are random, $W_j^{(n)}$ is a random variable. However, we will prove shortly that in fact $W_j^{(n)}=\frac{1}{N^{(n)}}$, for all $j \in \Pi (J^{(n)})$.

Note: Since we are looking from the adversary's point of view, the assumption is that all the values of $P_u$, $u \in \{1,2,\cdots,n\}$ are known, so all of the probabilities are conditioned on the values of $P_1=p_1, P_2=p_2, \cdots, P_n=p_n$. Thus, to be accurate, we should write
\[W_j^{(n)}= P\left(\Pi(1)=j \bigg{|} \textbf{V}, \Pi (J^{(n)}), P_1, P_2, \cdots, P_n\right).\]
Nevertheless, for simplicity of notation, we often omit the conditioning on $P_1, P_2, \cdots, P_n$.

First, we need a lemma from elementary probability.

\begin{lem}
	\label{lemOnePointFive}
	Let $N$ be a positive integer, and let $a_1, a_2, \cdots, a_N$ and $b_1, b_2, \cdots, b_N$ be real numbers such that $a_u \leq b_u$ for all $u$. Assume that $X_1, X_2, \cdots, X_N$ are independent random variables such that
\[X_u \sim Uniform [a_u,b_u]. \]
Let also $\gamma_1, \gamma_2, \cdots, \gamma_N$ be distinct real numbers such that
\[ \gamma_j \in \bigcap_{u=1}^{N} [a_u, b_u] \ \ \textrm{for all }j \in \{1,2,..,N\}.\]
Suppose that we know the event $E$ has occurred, meaning that the observed values of $X_u$'s are equal to the set of $\gamma_j$'s (but with unknown ordering), i.e.,
\[E \ \ \equiv \ \ \{X_1, X_2, \cdots, X_N\}= \{ \gamma_1, \gamma_2, \cdots, \gamma_N \},\] then
\[P\left(X_1=\gamma_j |E\right)=\frac{1}{N}. \]
\end{lem}

\begin{proof}
Lemma \ref{lemOnePointFive} is proved in Appendix \ref{sec:app_b}.
\end{proof}


%We now state a slightly modified version of Lemma \ref{lemOnePointFive} that is suitable for our purpose. The difference here is that $N$  is a random variable rather than a fixed integer (so are $a_i, b_i$).

%\begin{lem}
	%\label{lemOnePointSix}
	%Let $N$ be a positive integer-valued random variable, and let $A_1, A_2, \cdots$ and $B_1, B_2, \cdots$ be a sequence of real-valued random variables such that $A_i \leq B_i$ for all $i$, almost surely. Assume that $X_1, X_2, \cdots$ are independent random variables such that for all $n' \in \mathbb{N}$, given $N=n'$, $A_i=a_i$ and $B_i=b_i$ for all $i$,
%\[X_i \sim Uniform [a_i,b_i]. \]
%Let also $\gamma_1, \gamma_2, \cdots$ be distinct real numbers such that for all $n' \in \mathbb{N}$
%\[ \gamma_j \in \bigcap_{i=1}^{n'} [A_i, B_i] \ \ \textrm{for all }j \in \{1,2,..,n'\} \]
%Let $E$ be the event that the observed values of $X_i$'s is equal to the set of $\gamma_j$'s (but with unknown ordering), i.e.,
%\[E \ \ \equiv \ \ \{X_1, X_2, \cdots, X_N\}= \{ \gamma_1, \gamma_2, \cdots, \gamma_N \}. \]
%Then
%\[P\left(X_1=\gamma_j |E, A_i, B_i, i=1,2\cdots, N \right)=\frac{1}{N}. \]
%\end{lem}
%\begin{proof}
%Lemma \ref{lemOnePointSix} follows directly from Lemma \ref{lemOnePointFive}. In particular, assuming $N=n'$ is observed, and given $A_i=a_i$ and $B_i=b_i$, we can apply Lemma \ref{lemOnePointFive} to write
%\[P\left(X_1=\gamma_j |E,  A_i=a_i, B_i=b_i, i=1,2\cdots, N\right)=\frac{1}{n'}. \]
%Treating $N$, $A_i$, and $B_i$ as random variables,  we can write
%\[P\left(X_1=\gamma_j |E, A_i, B_i, i=1,2\cdots, N \right)=\frac{1}{N}. \]
%\end{proof}

Using the above lemma, we can state our desired result for $W_j^{(n)}$.

\begin{lem}
	\label{lem2}
	For all $j \in \Pi (J^{(n)})$, $W_j^{(n)}=\frac{1}{N^{(n)}}.$
\end{lem}
\begin{proof}
	
%We have
%	\begin{align}
%	\no P\left(\Pi^{(n)}(1)=j \bigg{|} \Pi (J^{(n)})\right)&= \frac{P\left(\Pi^{(n)}(1)=j \bigg{|} \Pi (J^{(n)})\right)}{P\left(\Pi (J^{(n)}\right)} \\
%	\nonumber &=\frac{\left(N^{(n)}-1\right)!}{\left(N^{(n)}\right)!}\\
%		\nonumber &=\frac{1}{N^{(n)}}.\ \
%	\end{align}

We argue that the setting of this lemma is essentially equivalent to the assumptions in Lemma \ref{lemOnePointFive}. First, remember that
\[W_j^{(n)}= P\left(\Pi(1)=j \bigg{|} \textbf{V}, \Pi (J^{(n)})\right).\]

Note that ${Q}_u= P_u+(1-2P_u)R_u$, and since $R_u$ is uniformly distributed, ${Q}_u$ conditioned on $P_u$ is also uniformly distributed in the appropriate intervals. Moreover, since ${V}_{u} = {Q}_{\Pi^{-1}(u)}$, we conclude ${V}_{u}$ is also uniformly distributed. So, looking at the definition of $W_j^{(n)}$, we can say the following: given the values of the uniformly distributed random variables ${Q}_u$, we would like to know which one of the values in  $\textbf{V}$ is the actual value of ${Q}_1={V}_{\Pi(1)}$, i.e., is $\Pi(1)=j$? This is equivalent to the setting of Lemma \ref{lemOnePointFive} as described further below. 

Note that since $1 \in J^{(n)}$, $\Pi(1) \in \Pi (J^{(n)})$. Therefore, when searching for the value of $\Pi(1)$, it is sufficient to look inside set $\Pi (J^{(n)})$. Therefore, instead of looking among all the values of ${V}_{j}$, it is sufficient to look at ${V}_{j}$ for $j \in  \Pi (J^{(n)})$. Let's show these values by $\textbf{V}_{\Pi} =\{v_1, v_2, \cdots, v_{N^{(n)}} \}$, so,
\[W_j^{(n)}= P\left(\Pi(1)=j \bigg{|} \textbf{V}_{\Pi}, \Pi (J^{(n)})\right).\]

Thus, we have the following scenario: $Q_u, u \in  J^{(n)}$ are independent random variables, and
\[Q_u\big{|} P_u=p_u \sim Uniform [p_u, p_u+(1-2p_u)a_n]. \]
Also, $v_1, v_2, \cdots, v_{N^{(n)}}$ are the observed values of $Q_u$ with unknown ordering (unknown mapping $\Pi$). We also know from the definition of set $J^{(n)}$ that
\[P_u \leq p_1+\epsilon_n \leq Q_u,\]
\[Q_u \leq p_1(1-2a_n)+an \leq P_u(1-2a_n)+a_n,\]
so, we can conclude
\[ v_j \in \bigcap_{u=1}^{N^{(n)}} [p_u, p_u+(1-2p_u)a_n] \ \ \textrm{for all }j \in \{1,2,..,N^{(n)}\}. \]
We know the event $E$ has occurred, meaning that the observed values of $Q_u$'s are equal to set of $v_j$'s (but with unknown ordering), i.e.,
\[E \ \ \equiv \ \ \{Q_u, u \in  J^{(n)}\}= \{ v_1, v_2, \cdots, v_{N^{(n)}} \}. \]
Then, according to Lemma \ref{lemOnePointFive},
\[P\left(Q_1=v_j |E, P_1, P_2, \cdots, P_n \right)=\frac{1}{N^{(n)}}. \]
Note that there is a subtle difference between this lemma and Lemma \ref{lemOnePointFive}. Here $N^{(n)}$ is a random variable while $N$ is a fixed number in Lemma \ref{lemOnePointFive}. Nevertheless, since the assertion holds for every fixed $N$, it also holds for the case where $N$ is a random variable. Now, note that
\begin{align*}
P\left(Q_1=v_j |E, P_1, P_2, \cdots, P_n \right) &= P\left(\Pi(1)=j \bigg{|} E, P_1, P_2, \cdots, P_n \right)\\
&=P\left(\Pi(1)=j \bigg{|} \textbf{V}_{\Pi}, \Pi (J^{(n)}), P_1, P_2, \cdots, P_n \right)\\
&=W_j^{(n)}.
\end{align*}
Thus, we can conclude
		\[W_j^{(n)}=\frac{1}{N^{(n)}}.\]
\end{proof}	
%It is worth noting that the above lemma in fact implies that  that given $\Pi (J^{(n)})$, $\Pi (1)$ and $V^{(n)}$ are independent. Specifically,
%\[P\left(\Pi^{(n)}(1)=j \bigg{|} V^{(n)}, \Pi (J^{(n)})\right)= P\left(\Pi^{(n)}(1)=j \bigg{|} \Pi (J^{(n)})\right).\]
%
%
In the third step, we define $\widetilde{W_j^{(n)}}$ for any $j \in \Pi (J^{(n)})$ as
\[\widetilde{W_j^{(n)}} = P\left(\Pi(1)=j \bigg{|} \textbf{Y}, \Pi (J^{(n)})\right).\]

$\widetilde{W_j^{(n)}}$ is the conditional probability that $\Pi(1)=j$ after observing the values of the anonymized version of the obfuscated samples of the users' data ($\textbf{Y}$) and the aggregate set including all the pseudonyms of the users in set $J^{(n)}$ (i.e., $\Pi(J^{(n)})\overset{\Delta}{=} \left\{\Pi^{-1}(j) \in J^{(n)}\right\}$). Since $\textbf{Y}$ and $\Pi (J^{(n)})$ are random, $\widetilde{W_j^{(n)}} $ is a random variable. Now, in the following lemma, we will prove $\widetilde{W_j^{(n)}} =\frac{1}{N^{(n)}}$, for all $j \in \Pi (J^{(n)})$ by using Lemma \ref{lem3}.

Note in the following lemma, we want to show that even if the adversary is given a set including all of the pseudonyms of the users in set $J^{(n)}$, he/she cannot match each specific user in set $J^{(n)}$ and his pseudonym.

\begin{lem}
	\label{lem3}
	For all $j \in \Pi (J^{(n)})$, $\widetilde{W_j^{(n)}}=\frac{1}{N^{(n)}}.$
\end{lem}

\begin{proof}
%	Consider random variable $\Pi$  while
%	\[Range(\Pi)=\{1, 2, \cdots ,N\}.\]
First, note that

%\begin{multline*}
%\widetilde{W_j^{(n)}} = \sum_{\text{for all v}} P\left(\Pi^{(n)}(1)=j \bigg{|} Y^{(n)}, \Pi \left(J^{(n)}\right), V^{(n)}=v\right)\cdot \\
%P\left(V^{(n)}=v \bigg{|} Y^{(n)}, \Pi \left(J^{(n)}\right)\right)
%\end{multline*}

\begin{align*}
\widetilde{W_j^{(n)}} = \sum_{\text{for all v}} P\left(\Pi(1)=j \bigg{|} \textbf{Y}, \Pi \left(J^{(n)}\right), \textbf{V}=\textbf{v}\right) P\left(\textbf{V}=\textbf{v} \bigg{|} \textbf{Y}, \Pi \left(J^{(n)}\right)\right).
\end{align*}

Also, we note that given $\textbf{V}$, $\Pi(J^{(n)})$, and $\textbf{Y}$ are independent. Intuitively, this is because when observing $\textbf{Y}$, any information regarding $\Pi(J^{(n)})$ is leaked through estimating $\textbf{V}$. This can be rigorously proved similar to the proof of Lemma 1 in \cite{tifs2016}. We can state this fact as
\[
	P\left(Y_u(k)\  \bigg{ | }  \ {V}_u=v_u, \Pi(J^{(n)}) \right)  = P\left(Y_u(k)\  \bigg{ | } \ {V}_u=v_u\right)=v_u.
\]
The right and left hand side are given by $Bernoulli (v_u)$ distributions.

As a result,
\[
\widetilde{W_j^{(n)}} = \sum_{\text{for all \textbf{v}}} P\left(\Pi(1)=j \bigg{|} \Pi (J^{(n)}), \textbf{V}=\textbf{v}\right) P\left(\textbf{V}=\textbf{v} \bigg{|} \textbf{Y}, \Pi \left(J^{(n)}\right)\right).
\]
Note $W_j^{(n)}=P\left(\Pi(1)=j \bigg{|} \Pi (J^{(n)}), \textbf{V}\right)$, so
\begin{align}
\no \widetilde{W_j^{(n)}} &= \sum_{\text{for all \textbf{v}}}W_j^{(n)}  P\left(\textbf{V}=\textbf{v} \bigg{|} \textbf{Y}, \Pi \left(J^{(n)}\right) \right) \\
\nonumber &= \frac{1}{N^{(n)}}\sum_{\text{for all \textbf{v}}} P\left(\textbf{V}=\textbf{v}\bigg{|} \textbf{Y}, \Pi \left(J^{(n)}\right)\right) \\
\nonumber &= \frac {1}{N^{(n)}}.\ \
\end{align}
\end{proof}

To show that no information is leaked, we need to show that the size of set $J^{(n)}$ goes to infinity. This is established in Lemma \ref{lem1}.

\begin{lem}
	\label{lem1}
	If $N^{(n)} \triangleq |J^{(n)}| $, then $N^{(n)} \rightarrow \infty$ with high probability as $n \rightarrow \infty$.  More specifically, there exists $\lambda>0$ such that
\[
	P\left(N^{(n)} > \frac{\lambda}{2}n^{\frac{\beta}{2}}\right) \rightarrow 1.
	\]
\end{lem}

\begin{proof}
Lemma \ref{lem1} is proved in Appendix \ref{sec:app_c}.
\end{proof}

In the final step, we define $\widehat{W_j^{(n)}}$ for any $j \in \Pi (J^{(n)})$ as
\[\widehat{W_j^{(n)}}=P\left(X_1(k)=1 \bigg{|} \textbf{Y}, \Pi (J^{(n)})\right).\]
$\widehat{W_j^{(n)}}$ is the conditional probability that $X_1(k)=1$ after observing the values of the anonymized version of the obfuscated samples of the users' data ($\textbf{Y}$) and the aggregate set including all of the pseudonyms of the users in set $J^{(n)}$ ($\Pi (J^{(n)})$). $\widehat{W_j^{(n)}} $ is a random variable because $\textbf{Y}$ and $\Pi (J^{(n)})$ are random. Now, in the following lemma, we will prove $\widehat{W_j^{(n)}}$ converges in distribution to $p_1$.

Note that this is the probability from the adversary's point of view. That is, given that the adversary has observed $\textbf{Y}$ as well as the extra information $ \Pi (J^{(n)})$, what can he/she infer about $X_1(k)$?
\begin{lem}
	\label{lem4}
	For all $j \in \Pi (J^{(n)})$, $\widehat{W_j^{(n)}} \xrightarrow{d} p_1.$
\end{lem}

\begin{proof}
We know
\begin{align*}
\widehat{W_j^{(n)}}= \sum_{j \in \Pi(J^{(n)})} P\left(X_1(k)=1 \bigg{|} \Pi(1)=j, \textbf{Y}, \Pi (J^{(n)})\right) P\left(\Pi(1)=j \bigg{|} \textbf{Y}, \Pi (J^{(n)})\right),
\end{align*}
and according to the definition $\widetilde{W_j^{(n)}}=P \left(\Pi(1)=j \bigg{|} \textbf{Y}, \Pi (J^{(n)})\right)$, we have
	\begin{align}
	\no \widehat{W_j^{(n)}} &= \sum_{j \in \Pi(J^{(n)})} P\left(X_1(k)=1 \bigg{|} \Pi(1)=j, \textbf{Y}, \Pi (J^{(n)})\right) \widetilde{W_j^{(n)}}\\
	\nonumber &= \frac{1}{N^{(n)}} \sum_{j \in \Pi(J^{(n)})} P\left(X_1(k)=1 \bigg{|} \Pi(1)=j, \textbf{Y}, \Pi (J^{(n)})\right).
	\end{align}
We now claim that
\[
 P\left(X_1(k)=1 \bigg{|} \Pi(1)=j, \textbf{Y}, \Pi (J^{(n)})\right)=p_1+o(1).
\]
The reasoning goes as follows. Given $\Pi(1)=j$ and knowing $\textbf{Y}$, we know that

\[
Y_{\Pi(1)}(k)={Z}_{1}(k)=\begin{cases}
{X}_{1}(k), & \textrm{with probability } 1-R_1.\\
1-{X}_{1}(k), & \textrm{with probability } R_1.
\end{cases}
\]

Thus, given $Y_{j}(k)=1$, Bayes' rule yields:
\begin{align*}
 P\left(X_1(k)=1 \bigg{|} \Pi(1)=j, \textbf{Y}, \Pi (J^{(n)})\right)&= \left(1- R_1 \right) \frac{P(X_1(k)=1)}{P(Y_{\Pi(1)}(k)=1)}\\
 &=\left(1-R_1 \right) \frac{p_1}{p_1 (1- R_1)+(1-p_1)R_1}\\
 &=1-o(1),
\end{align*}
and similarly, given $Y_{j}(k)=0$,
\begin{align*}
P\left(X_1(k)=1 \bigg{|} \Pi(1)=j, \textbf{Y}, \Pi (J^{(n)})\right)&= R_1 \frac{P(X_1(k)=1)}{P(Y_{\Pi(1)}(k)=0)}\\
&=R_1 \frac{p_1}{p_1 (1- R_1)+(1-p_1)R_1}\\
&=o(1).
\end{align*}
Note that by the independence assumption, the above probabilities do not depend on the other values of $Y_{u}(k)$ (as we are conditioning on $\Pi(1)=j$ ).
Thus, we can write
\begin{align}
	\no \widehat{W_j^{(n)}} &= \frac{1}{N^{(n)}} \sum_{j \in \Pi(J^{(n)})} P\left(X_1(k)=1 \bigg{|} \Pi(1)=j, \textbf{Y}, \Pi (J^{(n)})\right)\\
\no &=\frac{1}{N^{(n)}} \sum_{j \in \Pi(J^{(n)}), Y_{j}(k)=1}  (1-o(1)) + \frac{1}{N^{(n)}} \sum_{j \in \Pi(J^{(n)}), Y_{j}(k)=0}  o(1).
\end{align}
First, note that since $\abs*{\left\{j \in \Pi(J^{(n)}), Y_{j}(k)=0\right\}} \leq N^{(n)}$, the second term above converges to zero, thus,
\begin{align}
	\no \widehat{W_j^{(n)}}  \rightarrow \frac{\abs*{\left\{ j \in \Pi(J^{(n)}), Y_{\Pi(1)}(k)=1\right\} }}{N^{(n)}}.
\end{align}
Since for all $j \in \Pi(J^{(n)})$, $ Y_{j}(k)  \sim Bernoulli \left(p_1+o(1)\right)$, by a simple application of Chebyshev's inequality, we can conclude $\widehat{W_j^{(n)}}\rightarrow p_1$. Appendix \ref{sec:app_d} provides the detail.
\end{proof}	

As a result,
\begin{align*}
X_1(k) {|} \textbf{Y}, \Pi (J^{(n)})\rightarrow \textit{Bernoulli} (p_1),
\end{align*}
thus,
\[H\left(X_1(k) \bigg{|} \textbf{Y}, \Pi (J^{(n)})\right)\rightarrow H\left(X_1(k)\right).\]
Since conditioning reduces entropy,
\[H\left(X_1(k) \bigg{|} \textbf{Y}, \Pi (J^{(n)})\right)\leq H\left(X_1(k) \bigg{|} \textbf{Y}\right),\]
and as a result,
\[\lim_{n \rightarrow \infty}   H\left(X_1(k)\right)-H\left(X_1(k) \bigg{|} \textbf{Y}\right) \leq 0,\]
and 
\[\lim_{n \rightarrow \infty}   I\left(X_1(k);\textbf{Y}\right)\leq 0.\]
By knowing that $I\left(X_1(k);\textbf{Y}\right)$ cannot take any negative value, we can conclude that
\[I\left(X_1(k);\textbf{Y}\right)\rightarrow 0.\]
\end{proof}

\subsection{Extension to $r$-States}
Now, assume users' data samples can have $r$ possibilities $\left(0, 1, \cdots, r-1\right)$, and $p_u(i)$ shows the probability of user $u$ having data sample $i$. We define the vector $\textbf{p}_u$ and the matrix $\textbf{p}$ as
\[\textbf{p}_u= \begin{bmatrix}
p_u(1) \\ p_u(2) \\ \vdots \\p_u(r-1) \end{bmatrix} , \ \ \  \textbf{p} =\left[ \textbf{p}_{1}, \textbf{p}_{2}, \cdots,  \textbf{p}_{n}\right].
\]
We assume $p_u(i)$'s are drawn independently from some continuous density function, $f_\textbf{P}(\textbf{p}_u)$, which has support on a subset of the $(0,1)^{r-1}$ hypercube (Note that the $p_u(i)$'s sum to one, so one of them can be considered as the dependent value and the dimension is $r-1$). In particular, define the range of the distribution as
\begin{align}
\no  \mathcal{R}_{\textbf{p}} &= \{ (x_1,x_2,  \cdots, x_{r-1}) \in (0,1)^{r-1}:  x_i > 0 , x_1+x_2+\cdots+x_{r-1} < 1,\ i=1, 2, \cdots, r-1\}.
\end{align}
Figure~\ref{fig:rp} shows the range $\mathcal{R}_{\textbf{p}}$ for the case where $r=3$.
\begin{figure}[h]
	\centering
	\includegraphics[width = 0.5\linewidth]{fig/rp}
	\caption{$\mathcal{R}_{\textbf{p}}$ for case $r=3$.}
	\label{fig:rp}
\end{figure}


Then, we assume there are $\delta_1, \delta_2>0$ such that:
\begin{equation}
\begin{cases}
\no    \delta_1<f_{\textbf{P}}(\mathbf{p}_u) <\delta_2, & \textbf{p}_u \in \mathcal{R}_{\textbf{p}}.\\
    f_{\textbf{P}}(\mathbf{p}_u)=0, &  \textbf{p}_u \notin \mathcal{R}_{\textbf{p}}.
\end{cases}
\end{equation}

The obfuscation is similar to the two-states case. Specifically, for $l \in \{0,1,\cdots, r-1\}$, we can write
\[
P({Z}_{u}(k)=l| X_{u}(k)=i) =\begin{cases}
1-R_u, & \textrm{for } l=i.\\
\frac{R_u}{r-1}, & \textrm{for } l \neq i.
\end{cases}
\]



%


\begin{thm}\label{r_state_thm}
For the above $r$-states model, if $\textbf{Z}$ is the obfuscated version of $\textbf{X}$, and $\textbf{Y}$ is the anonymized version of $\textbf{Z}$ as defined previously, and
\begin{itemize}
	 \item $m=m(n)$ is arbitrary;
	\item $R_u \sim Uniform [0, a_n]$, where $a_n \triangleq c'n^{-\left(\frac{1}{r-1}-\beta\right)}$ for any $c'>0$ and $0<\beta<\frac{1}{r-1}$;
\end{itemize}
then, user 1 has perfect privacy. That is,
\begin{align}%\label{}
\no  \forall k\in \mathbb{N}, \ \ \ \lim\limits_{n\rightarrow \infty} I \left(X_1(k);{\textbf{Y}}\right) =0.
\end{align}\end{thm}

The proof of Theorem \ref{r_state_thm} is similar to the proof of Theorem \ref{two_state_thm}. The major difference is that instead of the random variables $P_u, Q_u, V_u$, we need to consider the random vectors $\textbf{P}_u, \textbf{Q}_u, \textbf{V}_u$.  Similarly, for user $u$, we define the vector $\textbf{Q}_u$ as
\[\textbf{Q}_u= \begin{bmatrix}
Q_u(1) \\ Q_u(2) \\ \vdots \\Q_u(r-1) \end{bmatrix}.
\]

In the $r$-states case,
\begin{align}
\no {Q}_u(i) &=P_u(i)\bigg(1-R_u(i) \bigg)+\bigg(1-P_u(i)\bigg)\frac{R_u}{r-1}  \\
\nonumber &= P_u+\bigg(1-r P_u\bigg)\frac{R_u}{r-1}.\ \
\end{align}
%Note that we have dropped the superscript $n$ for simplicity of notation (we need to write $Q_u^{(n)}(1)$ instead of $Q_u(1)$).
We also need to define the critical set $J^{(n)}$.  First, for $i=0,1, \cdots, r-1$, define set $J_i^{(n)}$ as follows. If $0\leq p_1(i)<\frac{1}{r}$, then,
\begin{align*}
&J_i^{(n)}= \\
&\left\{u \in \{1, 2, \dots, n\}: p_1(i) \leq P_u(i)\leq p_1(i)+\epsilon_n; p_1(i)+\epsilon_n\leq Q_u(i)\leq p_1(i)+(1-r p_1(i))\frac{a_n}{r-1}\right\},
\end{align*}
where $\epsilon_n \triangleq \frac{1}{n^{\frac{1}{r-1}-\frac{\beta}{2}}}$,  $a_n = c'n^{-\left(\frac{1}{r-1}-\beta\right)}$, and $\beta$ is defined in the statement of Theorem \ref{r_state_thm}.

We then define the critical set $J^{(n)}$ as:
\[
J^{(n)}=\bigcap_{l=0}^{r-1} J_i^{(n)}.
\]
We can then repeat the same arguments in the proof of Theorem \ref{two_state_thm} to complete the proof.

%\[J_i^{(n)}=
%\left\{  u \in \{1, 2, \dots, n\}: p_1(i) \leq P_u(i)\leq p_1(1)+\epsilon_n;  p_1(1)+\epsilon_n\leq Q_u(i)\leq p_1(1)+(1-2p_1(1)).a_n\right\}, \ \   \text{for}\ \ 0\leq p_1(1)<\frac{1}{2}\\
%\left\{  u \in \{1, 2, \dots, n\}: p_1(i)-\epsilon_n \leq P_u(i)\leq p_1(1); p_1(1)+(1-2p_1(1)).a_n\leq Q_u(i)\leq p_1-\epsilon_n\right\}, \ \  \text{for}\ \ \frac{1}{2}\leq p_1\leq1
%\end{cases}\]




\section{Converse Results: No Privacy Region}
\label{converse}

In this section, we prove that if the number of observations by the adversary is larger than its critical value and the noise level is less than its critical value, then the adversary can find an algorithm to successfully estimate users' data samples with arbitrarily small error probability. Combined with the results of the previous section, this implies that asymptotically (as $n \rightarrow \infty$), privacy can be achieved \emph{if and only if} at least one of  the two techniques (obfuscation or anonymization) are used above their thresholds. This statement needs a clarification as follows:  Looking at the results of \cite{tifs2016}, we notice that anonymization alone can provide perfect privacy if $m(n)$ is below its threshold. On the other hand, the threshold for obfuscation requires some anonymization: In particular, the identities of the users must be permuted once to prevent the adversary from readily identifying the users.



%is valid when both anonymization and obfuscation are simultaneously used as presented above (Figure \ref{fig:xyz}). In other words, if only obfuscation is used, then clearly the limit that we obtained above for $a_n$ is not nearly enough for privacy as it approaches zero as $n$ goes to infinity.

\subsection{Two-States Model}
Again, we start with the i.i.d.\ two-states model. The data sample of user $u$ at any time is a Bernoulli random variable with parameter $p_u$.

As before, we assume that $p_u$'s are drawn independently from some continuous density function, $f_P(p_u)$, on the $(0,1)$ interval. Specifically, there are $\delta_1, \delta_2>0$ such that:%\footnote{The condition $\delta_1<f_P(p_u) <\delta_2$ is not actually necessary for the results and can be relaxed; however, we keep it here to avoid unnecessary technicalities.}:
\begin{equation}
\no\begin{cases}
    \delta_1<f_P(p_u) <\delta_2, & p_u \in (0,1).\\
    f_P(p_u)=0, &  p _u\notin (0,1).
\end{cases}
\end{equation}

\begin{thm}\label{two_state_thm_converse}
For the above two-states mode, if $\textbf{Z}$ is the obfuscated version of $\textbf{X}$, and $\textbf{Y}$ is the anonymized version of $\textbf{Z}$ as defined, and
\begin{itemize}
	\item $m =cn^{2 +  \alpha}$ for any $c>0$ and $\alpha>0$;
	\item $R_u \sim Uniform [0, a_n]$, where $a_n \triangleq c'n^{-\left(1+\beta\right)}$ for any $c'>0$ and $\beta>\frac{\alpha}{4}$;
\end{itemize}
then, user $1$ has no privacy as $n$ goes to infinity.
\end{thm}

Since this is a converse result, we give an explicit detector at the adversary and show that it can be used by the adversary to recover the true data of user $1$.

\begin{proof}
The adversary first inverts the anonymization mapping $\Pi$ to obtain $Z_1(k)$, and then estimates the value of $X_1(k)$ from that. To invert the anonymization, the adversary calculates the empirical probability that each string is in state $1$ and then assigns the string with the empirical probability closest to $p_1$ to user 1.

\begin{figure}
	\centering
	\includegraphics[width=.8\linewidth]{fig/converse.jpg}
	\centering
	\caption{$p_1$, sets $B^{(n)}$ and $C^{(n)}$ for case $r=2$.}
	\label{fig:converse}
\end{figure}


Formally, for $u=1, 2, \cdots, n$, the adversary computes $\overline{Y_u}$, the empirical probability of user $u$ being in state $1$, as follows:
\[
\overline{Y_u}=\frac{Y_u(1)+Y_u(2)+ \cdots +Y_u(m)}{m},
\]
thus,
\[
\overline{Y_{\Pi(u)}}=\frac{Z_u(1)+Z_u(2)+ \cdots +Z_u(m)}{m}.
\]

As shown in Figure \ref{fig:converse}, define
\[B^{(n)}\triangleq \left\{x \in (0,1); p_1-\Delta_n \leq x \leq p_1+\Delta_n\right\},\]
where $\Delta_n = \frac{1}{n^{1+\frac{\alpha}{4}}}$ and $\alpha $ is defined in the statement of Theorem \ref{two_state_thm_converse}. We claim that for $m =cn^{2 +  \alpha}$, $a_n=c'n^{-(1 +  \beta)}$, and large enough $n$,
\begin{enumerate}
\item $P\left( \overline{Y_{\Pi(1) }}\in B^{(n)}\right) \rightarrow 1.$
\item $P\left( \bigcup\limits_{u=2}^{n} \left(\overline{Y_{\Pi(u)}}\in B^{(n)}\right)\right) \rightarrow 0.$
\end{enumerate}
As a result, the adversary can identify $\Pi(1)$ by examining  $\overline{Y_u}$'s and assigning the one in $B^{(n)}$ to user $1$. Note that $\overline{Y_{\Pi(u) }} \in B^{(n)}$ is a set (event) in the underlying probability space and can be written as $\left\{\omega \in \Omega: \overline{Y_{\Pi(u) }}(\omega) \in B^{(n)}\right\}$.

First, we show that as $n$ goes to infinity,
\[P\left( \overline{Y_{\Pi(1) }}\in B^{(n)}\right) \rightarrow 1.\]
We can write
\begin{align}
\no P\left(\overline{Y_{\Pi(1)}} \in B^{(n)}\right) &= P\left(\frac{\sum\limits_{k=1}^{m}Z_1(k)}{m} \in  B^{(n)} \right)\\
\nonumber &= P\left(p_1-\Delta_n \leq\frac{\sum\limits_{k=1}^{m}Z_1(k)}{m}\leq p_1+\Delta_n \right)\\
\nonumber &= P\left(mp_1-m\Delta_n-mQ_1\leq \sum\limits_{k=1}^{m}Z_1(k)-mQ_1\leq  mp_1+m\Delta_n-mQ_1 \right).\ \
\end{align}
%Note as n becomes large, $a_n\ll \Delta_n$, as a result,
%\[P\left(\overline{Y_{\Pi(1)}^{(n)}} \in B^{(n)}\right)=P\left(\abs*{\sum\limits_{i=1}^{m}Z_1^{(n)}(i)-mQ_1^{(n)}}< m\Delta_n \right).\]
Note that for any $u \in \{1,2,\cdots, n \}$, we have
\begin{align}
\no |p_u-{Q}_u| &=|1-2p_u|R_u \\
\no & \leq R_u \leq a_n,
\end{align}
so, we can conclude
\begin{align}
\no P\left(\overline{Y_{\Pi(1)}} \in B^{(n)}\right) &= P\left(mp_1-m\Delta_n-mQ_1\leq \sum\limits_{k=1}^{m}Z_1(k)-mQ_1 \leq mp_1+m\Delta_n-mQ_1 \right)\\
\nonumber  &\geq P\left(-m\Delta_n+m a_n\leq \sum\limits_{k=1}^{m}Z_1(k)-mQ_1\leq -ma_n+m\Delta_n \right)\\
\nonumber &= P\left(\abs*{\sum\limits_{k=1}^{m}Z_1(k)-mQ_1}\leq m (\Delta_n-a_n) \right).\ \
\end{align}
Since $a_n \rightarrow 0$, for $p_1 \in (0,1)$ and large enough $n$, we can say $p_1+a_n < 2 p_1$. From Chernoff bound, for any $c,c',\alpha>0$ and $\beta>\frac{\alpha}{4}$,
\begin{align}
%\nonumber
\no P\left(\abs*{\sum\limits_{k=1}^{m}Z_1(k)-mQ_1}\leq m (\Delta_n-a_n) \right) &\geq 1-2e^{-\frac{m(\Delta_n-a_n)^2}{3Q_1}} \\
\nonumber &\geq 1-2e^{-\frac{1}{3(p_1+a_n)}cn^{2+\alpha}\left(\frac{1}{n^{1+\frac{\alpha}{4}}}- \frac{c'}{n^{1 +  \beta}}\right)^2}\\
%\nonumber &\geq 1-2e^{-\frac{c}{3c'(1-2p_1)}n^{1+\frac{3\alpha}{2}}}\\
\nonumber &\geq 1-2e^{-\frac{c''}{6 p_1}n^{\frac{\alpha}{2}}}\rightarrow 1. \ \
\end{align}
As a result, as $n$ becomes large,
\[P\left(\overline{Y_{\Pi(1)}} \in B^{(n)}\right) \rightarrow 1.\]

Now, we need to show that as $n$ goes to infinity,
\[P\left( \bigcup\limits_{u=2}^{n} \left(\overline{Y_{\Pi(u)}}\in B^{(n)}\right)\right) \rightarrow 0.\]
First, we define
\[
C^{(n)}=\left\{x\in (0,1); p_1-2\Delta_n \leq x \leq p_1+2\Delta_n\right\}
,\]
and claim as $n$ goes to infinity,
\[P\left(\bigcup\limits_{u=2}^n \left(P_u \in C^{(n)}\right) \right)\rightarrow 0. \]

Note
\[4\Delta_n\delta_1< P\left( P_u\in C^{(n)}\right) < 4 \Delta_n\delta_2,\]
and according to the union bound, for large enough $n$,
\begin{align}
\no P\left( \bigcup\limits_{u=2}^n \left(P_u \in C^{(n)}\right) \right) &\leq \sum\limits_{u=2}^n P\left( P_u \in C^{(n)}\right) \\
\nonumber &\leq 4n \Delta_n \delta_2\\
\nonumber &= 4n \frac{1}{n^{1+{\frac{\alpha}{4}}}} \delta_2\\
\nonumber &= 4n^{-\frac{\alpha}{4}}\delta_2 \rightarrow 0. \ \
%\nonumber &\leq 4n^{-\frac{\alpha}{4}}\delta_2 \rightarrow 0. \ \
\end{align}
As a result, we can conclude that all $p_u$'s are outside of $C^{(n)}$ for $u \in \left\{2,3, \cdots, n\right\}$ with high probability.

Now, we claim that given all $p_u$'s are outside of $C^{(n)}$, $P\left(\overline{Y_{\Pi (u)}} \in B^{(n)}\right)$ is small. Remember that for any $u \in \{1,2,\cdots, n \}$, we have
\begin{align}
\no |p_u-{Q}_u| \leq a_n.
\end{align}
Now, noting the definitions of sets $B^{(n)}$ and $C^{(n)}$, we can write for $u \in \left\{2,3,  \cdots , n\right\}$,
\begin{align}
\nonumber
\no P\left(\overline{Y_{\Pi(u)}} \in B^{(n)}\right) &\leq P\left(\abs*{\overline{Y_{\Pi(u)}}-Q_u}\geq  (\Delta_n-a_n) \right)\\
%\nonumber &\hspace{-0.2 in}\leq  P\left(\frac{\sum\limits_{i=1}^{m}Z_j^{(n)}(i)}{m}<p_j-\Delta_n ,\frac{\sum\limits_{i=1}^{m}Z_j^{(n)}(i)}{m}>p_j+\Delta_n \right)\\
%\nonumber &\hspace{-0.2 in}\leq P\left(\sum\limits_{i=1}^{m}Z_j^{(n)}(i)-mQ_j^{(n)}<mp_j-m\Delta_n-mQ_j^{(n)}, \sum\limits_{i=1}^{m}Z_j^{(n)}(i)-mQ_j^{(n)}> mp_j+m\Delta_n-mQ_j^{(n)} \right)\\
%\nonumber &\hspace{-0.2 in}\leq P\left(\sum\limits_{i=1}^{m}Z_j^{(n)}(i)-mQ_j^{(n)}<ma_n-m\Delta_n, \sum\limits_{i=1}^{m}Z_j^{(n)}(i)-mQ_j^{(n)}>-ma_n+m\Delta_n \right)\\
\nonumber &= P\left(\abs*{\sum\limits_{k=1}^{m}Z_u(k)-mQ_u}> m(\Delta_n-a_n) \right).\ \
\end{align}
%We also know that as n becomes large, $a_n\ll \Delta_n$, as a result,
%\[P\left(\overline{Y_{\Pi(j)}^{(n)}} \in B^{(n)}\right)\leq P\left(\abs*{\sum\limits_{i=1}^{m}Z_j^{(n)}(i)-mQ_j^{(n)}}> m\Delta_n \right).\]
According to the Chernoff bound, for any $c,c',\alpha>0$ and $\beta>\frac{\alpha}{4}$,
\begin{align}
%\nonumber
\no P\left(\abs*{\sum\limits_{k=1}^{m}Z_u(k)-mQ_u}> m(\Delta_n-a_n) \right) &\leq 2e^{-\frac{m(\Delta_n-a_n)^2}{3Q_1}} \\
\nonumber &\leq 2e^{-\frac{1}{3(p_1+a_n)}cn^{2+\alpha}\left(\frac{1}{n^{1+\frac{\alpha}{4}}}- \frac{c'}{n^{1 +  \beta}}\right)^2}\\
%\nonumber &\leq 2e^{-\frac{c}{3c'(1-2p_1)}n^{1+\frac{3\alpha}{2}}}\\
\nonumber &\leq 2e^{-\frac{c''}{6 p_1}n^{\frac{\alpha}{2}}}. \ \
\end{align}
Now, by using a union bound, we have
\begin{align}
\no P\left( \bigcup\limits_{u=2}^n \left(\overline{Y_{\Pi(u)}}\in B^{(n)}\right)\right)&\leq \sum\limits_{u=2}^{n}P\left(\overline{Y_{\Pi(u)}}\in B^{(n)}\right)\\
\nonumber &\leq n\left(2e^{-\frac{c''}{6 p_1}n^{\frac{\alpha}{2}}}\right),\ \
\end{align}
and thus, as $n$ goes to infinity,
\[P\left( \bigcup\limits_{u=2}^n \left(\overline{Y_{\Pi(u)}}\in B^{(n)}\right)\right) \rightarrow 0.\]

So, the adversary can successfully recover $Z_1(k)$. Since $Z_{1}(k)=X_1(k)$ with probability $1-R_1=1-o(1)$, the adversary can recover $X_{1}(k)$ with vanishing error probability for large enough $n$.
\end{proof}

\subsection{Extension to $r$-States}
Now, assume users' data samples can have $r$ possibilities $\left(0, 1, \cdots, r-1\right)$, and $p_u(i)$ shows the probability of user $u$ having data sample $i$. We define the vector $\textbf{p}_u$ and the matrix $\textbf{p}$ as
\[\textbf{p}_u= \begin{bmatrix}
p_u(1) \\ p_u(2) \\ \vdots \\p_u(r-1) \end{bmatrix} , \ \ \  \textbf{p} =\left[ \textbf{p}_{1}, \textbf{p}_{2}, \cdots,  \textbf{p}_{n}\right].
\]
We also assume $\textbf{p}_u$'s are drawn independently from some continuous density function, $f_P(\textbf{p}_u)$, which has support on a subset of the $(0,1)^{r-1}$ hypercube. In particular, define the range of distribution as
\begin{align}
\no  \mathcal{R}_{\textbf{p}} &= \left\{ (x_1, x_2, \cdots, x_{r-1}) \in (0,1)^{r-1}: x_i > 0 , x_1+ x_2+\cdots+ x_{r-1} < 1,\ \ i=1, 2,\cdots, r-1\right\}.
\end{align}
Then, we assume there are $\delta_1, \delta_2>0$ such that:
\begin{equation}
\begin{cases}
\no    \delta_1<f_{\textbf{P}}(\mathbf{p}_u) <\delta_2, & \textbf{p}_u \in \mathcal{R}_{\textbf{p}}.\\
    f_{\textbf{P}}(\mathbf{p}_u)=0, &  \textbf{p}_u \notin \mathcal{R}_{\textbf{p}}.
\end{cases}
\end{equation}

\begin{thm}\label{r_state_thm_converse}
For the above $r$-states mode, if $\textbf{Z}$ is the obfuscated version of $\textbf{X}$, and $\textbf{Y}$ is the anonymized version of $\textbf{Z}$ as defined, and
\begin{itemize}
	\item $m =cn^{\frac{2}{r-1} +  \alpha}$ for any $c>0$ and $0<\alpha<1$;
	\item $R_u \sim Uniform [0, a_n]$, where $a_n \triangleq c'n^{-\left(\frac{1}{r-1}+\beta\right)}$ for any $c'>0$ and $\beta>\frac{\alpha}{4}$;
\end{itemize}
then, user $1$ has no privacy as $n$ goes to infinity. 
\end{thm}


The proof of Theorem \ref{r_state_thm_converse} is similar to the proof of Theorem \ref{two_state_thm_converse}, so we just provide the general idea. We similarly define the empirical probability that the user with pseudonym $u$ has data sample $i$ $\left(\overline{{Y}_{u}}(i)\right)$ as follows:

\[
\overline{Y_u}(i)=\frac{\abs {\left\{k \in \{1, 2, \cdots, m\}:Y_u(k)=i\right\}}}{m},
\]
thus,
\[
\overline{Y_{\Pi(u)}}(i)=\frac{\abs {\left\{k \in \{1, 2, \cdots, m\}:Y_u(k)=i\right\}}}{m}.
\]

The difference is that now for each $u \in \{1,2,\cdots, n \}$, $\overline{\textbf{Y}_{u}}$ is a vector of size $r-1$. In other words,
\[\overline{\textbf{Y}_{u}}=\begin{bmatrix}
\overline{Y_u}(1) \\ \overline{Y_u}(2) \\ \vdots \\\overline{Y_u}(r-1) \end{bmatrix}.\]


\begin{figure}
  \centering
  \includegraphics[width=.5\linewidth, height=0.5 \linewidth]{fig/R.jpg}
  \centering
  \caption{$\textbf{p}_1$, sets $B'^{(n)}$ and $C'^{(n)}$ in $\mathcal{R}_\textbf{p}$ for case $r=3$.}
  \label{fig:rpp}
\end{figure}

Define sets $B'^{(n)}$ and $C'^{(n)}$ as
\begin{align}
 \no B'^{(n)}\triangleq & \left\{(x_1,x_2, \cdots ,x_{r-1}) \in \mathcal{R}_{\textbf{p}}: p_1(i)-\Delta'_n \leq x_i \leq p_1(i)+\Delta'_n,\ i=1,2, \cdots, r-1\right\},
\end{align}
\begin{align}
\no C'^{(n)}\triangleq &\left\{(x_1,x_2, \cdots ,x_{r-1}) \in \mathcal{R}_{\textbf{p}}: p_1(i)-2 \Delta'_n \leq x_i \leq p_1(i)+2 \Delta'_n,\ i=1,2, \cdots ,r-1\right\},
\end{align}
where $\Delta'_n = \frac{1}{n^{\frac{1}{r-1}+\frac{\alpha}{4}}}.$ Figure \ref{fig:rpp} shows $\textbf{p}_1$ and sets  $B'^{(n)}$ and $C'^{(n)}$ for the case $r=3.$

We claim for $m =cn^{\frac{2}{r-1} +  \alpha}$ and large enough $n$,
\begin{enumerate}
\item $P\left( \overline{\textbf{Y}_{\Pi(1) }}\in B'^{(n)}\right) \rightarrow 1$.
\item $P\left( \bigcup\limits_{u=2}^{n} \left(\overline{\textbf{Y}_{\Pi(u)}}\in B'^{(n)}\right)\right) \rightarrow 0.$
\end{enumerate}
The proof follows that for the two-states case. Thus, the adversary can de-anonymize the data and then recover $X_1(k)$ with vanishing error probability in the $r$-states model.



\subsection{Markov Chain Model} 
\label{subsec:markov}

So far, we have assumed users' data samples can have $r$ possibilities $\left(0, 1, \cdots, r-1\right)$ and users' pattern are i.i.d.\ . Here we model users' pattern using Markov chains to capture the dependency of the users' pattern over time. Again, we assume there are $r$ possibilities (the number of states in the Markov chains). Let $E$ be the set of edges. More specifically, $(i, l) \in E$ if there exists an edge from $i$ to $l$ with probability $ p(i,l)>0 $. What distinguishes different users is their transition probabilities $p_u(i,l)$ (the probability that user $u$ jumps from state $i$ to state $l$). The adversary knows the transition probabilities of all users. The model for obfuscation and anonymization is exactly the same as before.

We show that the adversary will be able to estimate the data samples of the users with low error probability if $m(n)$ and $a_n$ are in the appropriate range. The key idea is that the adversary can focus on a subset of the transition probabilities that are sufficient for recovering the entire transition probability matrix. By estimating those transition probabilities from the observed data and matching with the known transition probabilities of the users, the adversary will be able to first de-anonymize the data, and then estimate the actual samples of users' data. In particular, note that for each state $i$, we must have
\[\sum\limits_{l=1}^{r} p_u(i,l)=1,   \  \  \textrm{ for each }u \in \{1,2,\cdots, n \}, \]
so, the Markov chain of user $u$ is completely determined by a subset of size $d=|E|-r$ of transition probabilities. We define the vector $\textbf{p}_u$ and the matrix $\textbf{p}$ as
\[\textbf{p}_u= \begin{bmatrix}
p_u(1) \\ p_u(2) \\ \vdots \\p_u(|E|-r) \end{bmatrix} , \ \ \  \textbf{p} =\left[ \textbf{p}_{1}, \textbf{p}_{2}, \cdots,  \textbf{p}_{n}\right].
\]


We also consider $\textbf{p}_u$'s are drawn independently from some continuous density function, $f_P(\textbf{p}_u)$, which has support on a subset of the $(0,1)^{|E|-r}$ hypercube. Let $\mathcal{R}_{\textbf{p}} \subset \mathbb{R}^{d}$ be the range of acceptable values for $\textbf{p}_{u}$, so we have
\begin{align}
\no  \mathcal{R}_{\textbf{P}} &= \left\{ (x_1,x_2 \cdots, x_{d}) \in (0,1)^{d}: x_i > 0 , x_1+x_2+\cdots+x_{d} < 1,\ \ i=1,2,\cdots, d\right\}.
\end{align}
As before, we assume there are $ \delta_1, \delta_2 >0$, such that:
\begin{equation}
\begin{cases}
\no    \delta_1<f_{\textbf{P}}(\textbf{p}_u) <\delta_2, & \textbf{p}_u \in \mathcal{R}_{\textbf{p}}.\\
    f_{\textbf{P}}(\textbf{p}_u)=0, &  \textbf{p}_u \notin \mathcal{R}_{\textbf{p}}.
\end{cases}
\end{equation}

Using the above observations, we can establish the following theorem.


\begin{thm}\label{markov_thm}
For an irreducible, aperiodic Markov chain with $r$ states and $|E|$ edges as defined above, if $\textbf{Z}$ is the obfuscated version of $\textbf{X}$, and $\textbf{Y}$ is the anonymized version of $\textbf{Z}$, and
\begin{itemize}
 \item $m =cn^{\frac{2}{|E|-r} +  \alpha}$ for any $c>0$ and $\alpha>0$;
\item $R_u \sim Uniform [0, a_n]$, where $a_n \triangleq c'n^{-\left(\frac{1}{|E|-r}+\beta \right)}$ for any $c'>0$ and $\beta>\frac{\alpha}{4}$;
\end{itemize}
then, the adversary can successfully identify the data of user $1$ as $n$ goes to infinity. 
\end{thm}
The proof has a lot of similarity to the i.i.d.\ case, so we provide a sketch, mainly focusing on the differences. We argue as follows. If the total number of observations per user is $m=m(n)$, then define $M_i(u)$ to be the total number of visits by user $u$ to state $i$, for $i=0, 1, \cdots, r-1$. Since the Markov chain is irreducible and aperiodic, and $m(n) \rightarrow \infty$, all $\frac{M_i(u)}{m(n)}$ converge to their stationary values. Now conditioned on $M_i(u)=m_i(u)$, the transitions from state $i$ to state $l$ for user $u$ follow a multinomial distribution with probabilities $p_u(i,l)$.

Given the above, the setting is now very similar to the i.i.d.\ case. Each user is uniquely characterized by a vector $\textbf{p}_u$ of size $|E|-r$. We define sets $B^{''(n)}$ and $C^{''(n)}$ as
\[
 B^{''(n)}\triangleq \{(x_1, x_2, \cdots ,x_{d}) \in \mathcal{R}_{\textbf{p}}: p_1(i)-\Delta''_n \leq x_i \leq p_1(i)+\Delta''_n, i=1,2 , \cdots ,d\},
\]
\[
 C^{''(n)}\triangleq \{(x_1, x_2, \cdots ,x_{d}) \in \mathcal{R}_{\textbf{p}}:
  p_1(i)-2 \Delta''_n < x_i < p_1(i)+2 \Delta''_n, i=1,2, \cdots, d\},
\]
where $\Delta''_n= \frac{1}{n^{\frac{1}{|E|-r}+\frac{\alpha}{4}}}$, and $d= |E|-r$. Then, we can show that for the stated values of $m(n)$ and $a_n$, as $n$ becomes large:
\begin{enumerate}
\item $P\left( \overline{\textbf{Y}_{\Pi(1) }}\in B^{''(n)}\right) \rightarrow 1$,
\item $P\left( \bigcup\limits_{u=2}^{n} \left(\overline{\textbf{Y}_{\Pi(u)}}\in B{''}^{(n)}\right)\right) \rightarrow 0$,
\end{enumerate}
which means that the adversary can estimate the data of user $1$ with vanishing error probability. The proof is very similar to the proof of the i.i.d.\ case; however, there are two differences that need to be addressed:

First, the probability of observing an erroneous observation is not exactly given by $R_u$. In fact, a transition is distorted if at least one of its nodes is distorted. So, if the actual transition is from state $i$ to state $l$, then the probability of an erroneous observation is equal to
\begin{align}
	\no R'_u&=R_u+R_u-R_uR_u =R_u(2-R_u).
\end{align}


Nevertheless, here the order only matters, and the above expression is still in the order of $a_n =O \left( n^{-\left(\frac{1}{|E|-r}+\beta \right)} \right)$.

The second difference is more subtle. As opposed to the i.i.d.\ case, the error probabilities are not completely independent. In particular, if $X_u(k)$ is reported in error, then both the transition to that state and from that state are reported in error. This means that there is a dependency between errors of adjacent transitions. We can address this issue in the following way:  The adversary makes his decision only based on a subset of the observations. More specifically, the adversary looks at only odd-numbered transitions: First, third, fifth, etc., and ignores the even-numbered transitions.  In this way, the number of observations is effectively reduced from $m$ to $\frac{m}{2}$ which again does not impact the order of the result (recall that the Markov chain is aperiodic). However, the adversary now has access to observations with independent errors.



\section{Perfect Privacy Analysis: Markov Chain Model}\label{sec:perfect-MC}
So far, we have provided both achievability and converse results for the i.i.d.\ case. However, we have only provided the converse results for the Markov chain case. Here, we investigate achievability for Markov chain models. It turns out that for this case, the assumed obfuscation technique is not sufficient to achieve a reasonable level of privacy. Loosely speaking, we can state that if the adversary can make enough observations, then he can break the anonymity. The culprit is the fact that the sequence observed by the adversary is no longer modeled by a Markov chain; rather, it can be modeled by a hidden Markov chain. This allows the adversary to successfully estimate the obfuscation random variable $R_u$ as well as the $ p_u(i,l)$ values for each sequence, and hence successfully de-anonymize the sequences.


More specifically, as we will see below, there is a fundamental difference between the i.i.d.\ case and the Markov chain case. In the i.i.d.\ case, if the noise level is beyond a relatively small threshold, the adversary will be unable to de-anonymize the data and unable to recover the actual values of the data sets for users, \emph{regardless of the (large) size of $m=m(n)$}. On the other hand, in the Markov chain case, if $m=m(n)$ is large enough, then the adversary can easily de-anonymize the data. To better illustrate this, let's consider a simple example.

\begin{example}
Consider the scenario where there are only two states and the users' data samples change between the two states according to the Markov chain shown in Figure \ref{fig:MC-diagram}. What distinguishes the users is their different values of $p$. Now, suppose we use the same obfuscation method as before. That is, to create a noisy version of the sequences of data samples, for each user $u$, we generate the random variable $R_u$ that is the probability that the data sample of the user is changed to a different data sample by obfuscation. Specifically,
\[
{Z}_{u}(k)=\begin{cases}
{X}_{u}(k), & \textrm{with probability } 1-R_u.\\
1-{X}_{u}(k),& \textrm{with probability } R_u.
\end{cases}
\]

\begin{figure}[H]
\begin{center}
\[
\SelectTips {lu}{12 scaled 2500}
\xymatrixcolsep{6pc}\xymatrixrowsep{5pc}\xymatrix{
*++[o][F]{0}  \ar@/^1pc/[r]^{1}
& *++[o][F]{1} \ar@(dr,ur)[]_{1-p}  \ar@/^1pc/[l]^{p}
}
\]
\caption{A state transition diagram.}\label{fig:MC-diagram}
\end{center}
\end{figure}
To analyze this problem, we can construct the underlying Markov chain as follows. Each state in this Markov chain is identified by two values: the real state of the user, and the observed value by the adversary. In particular, we can write
\[\left(\text{Real value}, \text{Observed value}\right) \in \left\{\right(0,0), (0,1), (1,0), (1,1)\}.\]
Figure \ref{fig:MC-diagram2} shows the state transition diagram of this new Markov chain.

\begin{figure}[H]
\begin{center}
\[
\SelectTips {lu}{12 scaled 2000}
\xymatrixcolsep{10pc}\xymatrixrowsep{8pc}\xymatrix{
*++[o][F]{00} \ar@//[d]^{R} \ar@/_1pc/[dr]_>>>>>{1-R}
& *++[o][F]{01} \ar@//[d]^{1-R} \ar@/^1pc/[dl]^>>>>>{R} \\
*++[o][F]{10} \ar@(d,l)[]^{(1-p)R} \ar@/_2pc/[r]_{(1-p)(1-R)} \ar@/^2pc/[u]^{p(1-R)} \ar@/^1pc/[ur]^>>>>>{pR}
& *++[o][F]{11} \ar@(d,r)[]_{(1-p)(1-R)}  \ar@//[l]^{(1-p)R} \ar@/_2pc/[u]_{pR} \ar@/_1pc/[ul]_>>>>>{p(1-R)}
}
\]
\caption{The state transition diagram of the new Markov chain.}\label{fig:MC-diagram2}
\end{center}
\end{figure}
 We know
 \[ \pi_{00}=\pi_0(1-R)=\frac{p}{1+p}(1-R).\]
 \[ \pi_{01}=\pi_0R= \frac{p}{1+p}R.\]
 \[ \pi_{10}=\pi_1R=\frac{1}{1+p}R.\]
 \[ \pi_{11}=\pi_1(1-R)=\frac{1}{1+p}(1-R).\]

The observed process by the adversary is not a Markov chain; nevertheless, we can define limiting probabilities. In particular, let $\theta_0$ be the limiting probability of observing a zero. That is, we have
\[
\frac{M_0}{m} \xrightarrow{d} \theta_0,  \ \ \textrm{ as }n \rightarrow \infty,
\]
where $m$ is the total number of observations by the adversary, and $M_0$ is the number of $0$'s observed. Then,
\[\theta_0= \pi_{00}+\pi_{10} =\frac{(1-R)p+R}{1+p}.\]
Also, let $\theta_1$ be the limiting probability of observing a one, so
\[\theta_1= \pi_{01}+\pi_{11} =\frac{pR+(1-R)}{1+p}=1-\theta_0.\]


Now the adversary's estimate of $\theta_0$ is given by:
\begin{align}\label{eq1}
\hat{\theta}_0= \frac{(1-R)p+R}{1+p}.
\end{align}
Note that if the number of observations by the adversary can be arbitrarily large, the adversary can obtain an arbitrarily accurate estimate of $\theta_0$.
The adversary can obtain another equation easily, as follows.   Let $\theta_{01}$ be the limiting value of the portion of transitions from state $0$ to $1$ in the chain observed by the adversary. We can write
\begin{align}
%\nonumber
\no \theta_{01} &=P \left\{(00\rightarrow 01), (00\rightarrow 11), (10 \rightarrow 01), (10 \rightarrow 11) \right\}\\\
\nonumber &= \pi_{00}(1-R)+\pi_{10}PR+ \pi_{10}(1-p)(1-R).\ \
\end{align}
As a result,
\begin{align}\label{eq2}
\hat{\theta}_{01}= \frac{p(1-R)^2+R\left(PR(1-R)(1-p)\right)}{1+p}.
\end{align}
Again, if the number of observations can be arbitrarily large, the adversary can obtain an arbitrarily accurate estimate of $\theta_{01}$.
By solving the Equations \ref{eq1} and \ref{eq2}, the adversary can successfully recover $R$ and $p$; thus, he/she can successfully determine the users' data values.

\end{example}




==> Revised paper/introduction.tex <==
\section{Introduction}
\label{intro}

A number of emerging systems and applications work by analyzing the data submitted by their users in order to serve them; we call such systems \emph{User-Data Driven} (UDD) services. Examples of UDD services include smart cities, connected vehicles, smart homes, and connected healthcare devices, which have the promise of greatly improving users' lives. Unfortunately, the sheer volume of user data collected by these systems can compromise users' privacy~\cite{FTC2015}. Even the use of standard Privacy-Protection Mechanisms (PPMs), specifically anonymization of user identities and obfuscation of submitted data, does not guarantee users' privacy, as adversaries are able to use powerful statistical inference techniques to learn sensitive private information of the users~\cite{0Quest2016, 3ukil2014iot, 4Hosseinzadeh2014,iotCastle,matching}.

To illustrate the threat of privacy leakage, consider three popular UDD services: (1) {\em Health care:}  Wearable monitors that constantly track user health variables can be invaluable in assessing individual health trends and responding to emergencies.  However, such monitors produce long time-series of user data uniquely matched to the health characteristics of each user; (2) {\em Smart homes:} Emerging smart-home technologies such as fine-grained power measurement systems can help users and utility providers to address one of the key challenges of the twenty-first century:  energy conservation.  But the measurements of power by such devices can be mapped to users and reveal their lifestyle habits; and, (3) {\em Connected vehicles:}  The location data provided by connected vehicles promises to greatly improve everyday life by reducing congestion and traffic accidents.  However, the matching of such location traces to prior behavior not only allows for user tracking, but also reveals a user's habits.  In summary, despite their potential impact on society and their emerging popularity, these UDD services have one thing in common: their utility critically depends on their collection of user data, which puts users' privacy at significant risk.

There are two main approaches to augment privacy in UDD services: \emph{identity perturbation (anonymization)}~\cite{1corser2016evaluating,hoh2005protecting,freudiger2007mix, ma2009location, shokri2011quantifying2, Naini2016,soltani2017towards, soltani2018invisible}, and \emph{data perturbation (obfuscation)}~\cite{shokri2012protecting, gruteser2003anonymous, bordenabe2014optimal}. In anonymization techniques, privacy is obtained by concealing the mapping between users and data, and the mapping is changed periodically to thwart statistical inference attacks that try to de-anonymize the anonymized data traces by matching user data to known user profiles. Some approaches employ $k$-anonymity to keep each user's identity indistinguishable within a group of $k-1$ other users ~\cite{2zhang2016designing,11dewri2014exploiting, gedik2005location, zhong2009distributed, sweeney2002k, kalnis2007preventing,liu2013game}.  Other approaches employ users' pseudonyms within areas called mix-zones~\cite{beresford2003location, freudiger2009optimal, palanisamy2011mobimix}.
Obfuscation mechanisms aim at protecting privacy by perturbing user data, e.g., by adding noise to users' samples of data.   For instance, cloaking replaces each user's sample of data with a larger region~\cite{18shokri2014hiding,8zurbaran2015near,hoh2007preserving, wernke2014classification, chow2011spatial, um2010advanced}, while an alternative approach is to use dummy data in the set of possible data of the users~\cite{kido2005protection, shankar2009privately, chow2009faking, kido2005anonymous, lu2008pad}. In~\cite{randomizedresponse}, a mechanism of obfuscation was introduced where the answer was changed randomly with some small probability. Here we consider the fundamental limits of a similar obfuscation technique for providing privacy in the long time series of emerging applications.

%In~\cite{randomizedresponse}, the mechanism of obfuscation is similar to our work, but the context of this paper is different from our work. First, in~\cite{randomizedresponse}, only a single point of data was considered for each user; however, we consider a long time series of data for each user. Second, in~\cite{randomizedresponse}, no prior distribution for users' sample of data was considered, but we assume there is a prior distribution for each of the users' data samples. In addition, we assume the strongest adversary who has complete statistical knowledge about users. Finally, in~\cite{randomizedresponse}, the privacy of users was provided when there were only two states for users' sample of data, and the obfuscation mechanism for r-states model wasn't studied.

The anonymization and obfuscation mechanisms improve user privacy at the cost of user utility. The anonymization mechanism works by frequently changing the pseudonym mappings of users to reduce the length of time series that can be exploited by statistical analysis.  However, this frequent change may also decrease the usability by concealing the temporal relation between a user's sample of data, which may be critical in the utility of some systems, e.g., a dining recommendation system that makes suggestions based on the dining history of its users. On the other hand, obfuscation mechanisms work by adding noise to users' collected data, e.g., location information. The added noise may degrade the utility of UDD applications.  Thus, choosing the right level of the privacy-protection mechanism is an important question, and understanding what levels of anonymization and obfuscation can provide theoretical guarantees of privacy is of interest.

%Differential privacy aims at protecting queries on aggregated data.
%Particularly, several identity perturbation~\cite{lee2012differential, chatzikokolakis2015geo, nguyen2013differential, machanavajjhala2008privacy} and data perturbation ~\cite{chatzikokolakis2013broadening,shokri2014optimal, chatzikokolakis2015location,andres2013geo} PPMs are based on differential privacy techniques.
%Dewri~\cite{dewri2013local} combines k-anonymity and differential privacy to achieve higher privacy. In ~\cite{info2012}, it  is proved that differential privacy arises out of maximizing entropy principle which is equal to minimizing information leakage and is measured using the mutual information notion.~\cite{yeb17} tries to reduce the expected estimation loss by using differential privacy and constraining the privacy level.

In this paper, we will consider the ability of an adversary to perform statistical analyses on time series and match the series to descriptions of user behavior. In related work, Unnikrishnan~\cite{matching} provides a comprehensive analysis of the asymptotic (in the length of the time series) optimal matching of time series to source distributions. However, there are several key differences between that analysis and the work here. First, Unnikrishnan~\cite{matching} looks at the optimal matching tests, but does not consider any privacy metrics as considered in this paper, and a significant component of our study is demonstrating that mutual information converges to zero so that we can conclude there is no privacy leakage (hence, ``perfect privacy'').  Second, the setting of~\cite{matching} is different, as it does not consider: (a) obfuscation, which is one of the two major protection mechanisms; and (b) sources that are not independent and identically distributed (i.i.d.). Third, the setting of Unnikrishnan~\cite{matching} assumes a fixed distribution on sources (i.e., classical inference), whereas we assume the existence of general (but possibly unknown) prior distributions for the sources (i.e., a Bayesian setting).  Finally, we study the fundamental limits in terms of both the number of users and the number of observations, while Unnikrishnan~\cite{matching} focuses on the case where the number of users is a fixed, finite value.

Numerous researchers have put forward ideas for quantifying privacy-protection. Shokri et al.~\cite{shokri2011quantifying, shokri2011quantifying2} define the expected estimation error of the adversary as a metric to evaluate PPMs.  Ma et al.~\cite{ma2009location} use uncertainty about users' information to quantify user privacy in vehicular networks.
To defeat localization attacks and achieve privacy at the same time, Shokri et al.~\cite{shokri2012protecting} proposed a method which finds optimal PPM for an LBS given service quality constraints.
In~\cite{6li2016privacy} and~\cite{4olteanu2016quantifying}, privacy leakage of data sharing and interdependent privacy risks are quantified, respectively. A similar idea is proposed in \cite{14zhang2014privacy} where the quantification model is based on the Bayes conditional risk. %Yu et al. \cite{diff2017} combine two complementary notations, geo-indstingushability and expected inference error, to achieve location privacy. The geo-indstingushability is derived from differential privacy but cannot adequately protect users' location against inference attacks of adversary by using prior information, and the expected inference error as privacy metric doesn't consider posterior information obtained from  pseudo-location. As a result, combining both notations gives users the opportunity to have location privacy. In addition, users are allowed to personalized error bound for different locations.
Previously, mutual information has been used as a privacy metric in a number of settings,~\cite{kousha3,salamatian2013hide, csiszar1996almost, calmon2015fundamental, sankar2013utility, sankarISIT,sankar, yamamoto1983source, hyposankar}. However, the framework and problem formulation for our setting (Internet of Things (IoT) privacy) are quite different from those encountered in previous works. More specifically, the IoT privacy problem we consider here is based on a large set of time-series data that belongs to different users with different statistical patterns that has gone through a privacy-preserving mechanism, and the adversary is aiming at de-anonymizing and de-obfuscating the data.

The discussed studies demonstrate the growing importance of privacy. What is missing from the current literature is a solid theoretical framework for privacy that is general enough to encompass various privacy-preserving methods in the literature. Such a framework will allow us to achieve provable privacy guarantees, obtain fundamental trade-offs between privacy and performance, and provide analytical tools to optimally achieve provable privacy. We derive the fundamental limits of user privacy in UDD services in the presence of both anonymization and obfuscation protection mechanisms.  We build on our previous works on formalizing privacy in location-based services~\cite{tifs2016, ciss2017}, but we significantly expand those works here not just in application area but also user models and settings. In particular, our previous works introduced the notion of \emph{perfect privacy} for location-based services, and we derived the rate at which an anonymization mechanism should change the pseudonyms in order to achieve the defined perfect privacy. In this work, we expand the notion of perfect privacy to UDD services in general and derive the conditions for it to hold when \emph{both} anonymization and obfuscation-based protection mechanisms are employed.

In this paper, we consider two models for users' data: i.i.d.\ and Markov chains. After introducing the general framework in Section \ref{sec:framework}, we consider an i.i.d.\ model extensively in Section \ref{perfectsec} and the first half of Section \ref{converse}. We obtain achievability and converse results for the i.i.d.\ model. The i.i.d.\ model would apply directly to data that is sampled at a low rate. In addition, understanding the i.i.d.\ case can also be considered the first step toward understanding the more complicated case where there is dependency, as was done for anonymization-only Location Privacy-Preserving Mechanisms (LPPMs) in \cite{tifs2016}, and will be done in Section \ref{subsec:markov}. In particular, in Section \ref{subsec:markov}, a general Markov chain model is used to model users' data pattern to capture the dependency of the user' data pattern over time. There, we obtain converse results for privacy for this model. In Section \ref{sec:perfect-MC}, we provide some discussion about the achievability for the Markov chain case.


\subsection{Summary of the Results}

Given $n$, the total number of the users in a network, their degree of privacy depends
on two parameters: (1) The number of observations $m=m(n)$ by the adversary per user for a fixed anonymization mapping (i.e., the number of observations before the pseudonyms are changed);  and (2) the value of the noise added by the obfuscation technique (as defined in Section~\ref{sec:framework}, we quantify the obfuscation noise with a parameter $a_n$, where larger $a_n$ means a higher level of obfuscation).  Intuitively, smaller $m(n)$ and larger $a_n$ result in stronger privacy, at the expense of lower utility for the users.

Our goal is to identify values of $a_n$ and $m(n)$ that satisfy perfect privacy in the asymptote of a large number of users ($n \rightarrow \infty$).
%
When the users' datasets are governed by an i.i.d.\ process, we show that
the $m(n)- a_n$ plane can be divided into two areas.  In the first area, all users have perfect privacy (as defined in Section~\ref{sec:framework}), and, in the second area, users have no privacy.
Figure~\ref{fig:region} shows the limits of privacy in the entire $m(n)- a_n$ plane.
As the figure shows, in regions $1$, $2$, and $3$, users have perfect privacy, while in region $4$ users have no privacy.
\begin{figure}[h]
	\centering
	\includegraphics[width=0.7\linewidth, height=0.6 \linewidth]{fig/region}
	\caption{Limits of privacy in the entire $m(n)-a_n$ plane: in regions $1$, $2$, and $3$, users have perfect privacy, and in region $4$ users have no privacy.}
	\label{fig:region}
\end{figure}

For the case where the users' datasets are governed by irreducible and aperiodic Markov chains with $r$ states and $|E|$ edges, we show that users will have no privacy if $m =cn^{\frac{2}{|E|-r} +  \alpha}$ and $a_n =c'n^{-\left(\frac{1}{|E|-r}+\beta \right)}$, for any constants $c>0$, $c'>0$, $\alpha>0$, and $\beta>\frac{\alpha}{4}$. We also provide some insights for the opposite direction (under which conditions users have perfect privacy) for the case of Markov chains.









%\subsection{Summary of Results}

%When there are $n$ users in the network, the privacy level of the users depends on two parameters: (1) The %number of observations $m=m(n)$ by the adversary per user for a fixed anonymization mapping (i.e.~the %number of observations before the pseudonyms are changed);  (2) The noise level of the obfuscation %technique.  In this paper, the noise level of the obfuscation is increasing in a parameter $a_n$, which is %defined precisely in Section \ref{sec:framework}.  Intuitively, smaller $m(n)$ and larger $a_n$ result in %stronger location privacy but lower user utility. Thus, the fundamental question is, as the number of users %grows ($n \rightarrow \infty$), what values of $a_n$ and $m(n)$ are required to insure location privacy?

%In this paper, we answer the above question for the entire $m(n)- a_n$ plane for the case where each users' %movement is governed by an i.i.d process. We will prove that the $m(n)- a_n$ plane can be divided into two %areas.  In the first area, all users have perfect location privacy\cite{tifs2016}, as will be defined precisely in %Section \ref{sec:framework}, and, in the second area, users have no location privacy.  Figure~\ref{fig:region} %shows the limits of location privacy in the entire $m(n)- a_n$. In other words, according to %Figure~\ref{fig:region}, in regions $1$, $2$, and $3$, users have perfect location privacy, and  in region $4$ %users have no location privacy.
%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.9\linewidth, height=0.6 \linewidth]{fig/region}
%	\caption{Limits of location privacy in the entire $m(n)-a_n$ planes: in regions $1$, $2$, and $3$, users %have perfect location privacy, and in region $4$ users have no location privacy.}
%	\label{fig:region}
%\end{figure}
%
%Also, for the case where the users movements are governed by irreducible and aperiodic Markov chains with %$r$ states and $|E|$ edges, we show that users will have no privacy if $m =cn^{\frac{2}{|E|-r} +  \alpha}$ %and $a_n =c'n^{-\left(\frac{1}{|E|-r}+\alpha \right)}$ for some positive constants  $c, c'>0$  and %$0<\alpha<1$. Showing the opposite direction (under which conditions users have perfect privacy) for the %case of Markov chains is among the future work.

%In the rest of the paper we will provide the details of the results. Due to the space limitations, the proofs can %be found in the publicly available longer version of the paper ~\cite{longversion}.


==> Revised paper/introduction_dg.tex <==
\section{Introduction}
\label{intro}

Various emerging systems and applications work by analyzing
the data submitted by their users in order to serve them; we call such systems  \emph{user-data driven} (UDD) \amir{we need a name. how's this?} services. Examples of UDD services include  smart cities, connected vehicles, smart homes, and connected healthcare devices, which are 
 revolutionizing our lives in different ways.  
Unfortunately, 	the sheer volume of user data collected by these systems 
compromises users' privacy ostensibly~\cite{FTC2015}. 
Even the employment of  standard 
privacy-protection mechanisms (e.g.,  anonymization of user identities and obfuscation of submitted data) does not mitigate the privacy leakage as the adversaries are able to use powerful statistical inference techniques to infer sensitive private information~\cite{FTC2015,0Quest2016, 2nia2016comprehensive, 3ukil2014iot, 4Hosseinzadeh2014,iotCastle,matching}.
 
To illustrate   their privacy leakage, consider the following three popular UDD services. 
(1) {\em Health care:}  Wearable monitors that constantly track user health variables can be invaluable in assessing individual health trends and responding to emergencies.  However, such monitors produce long time-series of user data uniquely matched to the health characteristics of each  user; (2) {\em Smart homes:}  Emerging smart-home technologies such as fine-grained power measurement systems can help users and utility providers to address one of the key challenges of the twenty-first century:  energy conservation.  But the measurements of power by such devices can be  mapped to users and reveal their lifestyle habits; and, (3) 
	{\em Connected vehicles:}  The location data provided by connected vehicles promises to greatly improve everyday lives by reducing congestion and traffic accidents.  However, the matching of such location traces to prior behavior not only allows for user tracking, but also reveals a user's habits.
In summary, despite their critical importance to the society and their emerging popularity, these services have one thing in common: 
they collect  long time-series of user data, for them to operate, 
that puts users' privacy at significant risk.

There are two main approaches to augment privacy in UDD services: 
 \emph{identity perturbation (anonymization)}, and \emph{location perturbation (obfuscation)}.  In anonymization techniques, privacy is obtained by concealing the mapping between users and data, and the mapping is changed periodically to  thwart statistical inference attacks that try to deanonymize the anonymized data traces by matching user data to 
 known  user profiles. 
 On the other hands,  obfuscation mechanisms aim at protecting privacy by perturbing user data, e.g., by adding noise to user locations. 
% Both anonymization and obfuscation mechanisms manipulate user data time-series in a way to not significantly impact the utility of the underlying UDD services. 


Anonymization and obfuscation improve user privacy at the cost of user utility.  In anonymization, we need to change these pseudonym mappings frequently to achieve high privacy by reducing the length of time series exploited by statistical analysis.  However, this frequent change could decrease usability and functionality by concealing the temporal relation between a user's locations, which may be critical in the utility of some systems, e.g., a dining recommendation system that makes suggestions based on the dining places visited by a user in the past.  For obfuscation-based mechanisms, the added noise to the reported values of user locations will degrade the application utility; for example, user utility would be degraded by location obfuscation in ride-sharing systems.  Thus, choosing the right level of privacy-protection mechanism is an important question, and understanding what levels of anonymization and obfuscation can provide theoretical guarantees of privacy is of interest.

In this paper, we derive the fundamental limits of user privacy in UDD services in the presence of both anonymization and obfuscation protection mechanisms. This work is built on our previous work on formalizing privacy in location-based services~\cite{montazeri2016defining, Mont1610Achieving,tifs2016, ciss2017}, by extensively expanding not just the application area but also user models and settings. 
Particularly, our previous work introduced the notion of 
\emph{perfect privacy} for location-based services, and derives the rate at which an anonymization mechanism should change the pseudonyms in order to 
achieve the defined perfect privacy. 
In this work, we expand the notion of perfect privacy to UDD services in general, and derive the conditions for it to hold when \emph{both}
anonymization and obfuscation-based protection mechanisms are employed.   
 We study both achievability and converse results.  

%In~\cite{montazeri2016defining, Mont1610Achieving,tifs2016, ciss2017}, an approach was introduced to understand the fundamental limits of privacy when only anonymization is used in location-based services. There, users are characterized by the statistics of their locations, and the adversary then tries to match traces to those statistics to de-anonymize users.  Per above, anonymization thwarts such statistical analysis by reducing the time series available for such a matching, and thus \cite{montazeri2016defining, Mont1610Achieving,tifs2016} considers the rate at which pseudonyms must be changed so as to preserve perfect location privacy.   In this paper, the perfect privacy set-up of \cite{tifs2016} is again employed; however, in addition to anonymization, perturbation (obfuscation) is also considered; thus, the adversary attempts to infer information about the actual locations by observing the obfuscated \emph{and} anonymized version of the location data.  We study both achievability and converse results.  

\subsection{Summary of the Results}

Given $n$, the total number of the users in a network, their degree of privacy depends 
on two parameters: (1) The number of observations $m=m(n)$ by the adversary per user for a fixed anonymization mapping (i.e., the number of observations before the pseudonyms are changed);  and (2) the value of the noise added by the obfuscation technique (as defined in Section~\ref{sec:framework}, we quantify the obfuscation noise with a parameter $a_n$).  
Intuitively, smaller $m(n)$ and larger $a_n$ result in stronger privacy, at the expense of lower utility for the users. 

Our goal is to identify values of $a_n$ and $m(n)$  that satisfy perfect privacy as the number of users grows ($n \rightarrow \infty$).
%
We show that when the users' data sets are governed by an i.i.d.\ process, 
the $m(n)- a_n$ plane can be divided into two areas.  In the first area, all users have perfect privacy~\cite{tifs2016} (as defined in Section~\ref{sec:framework}), and, in the second area, users have no privacy.  
Figure~\ref{fig:region} shows the limits of privacy in the entire $m(n)- a_n$. 
As the figure shows, in regions $1$, $2$, and $3$, users have perfect privacy, while in region $4$ users have no privacy.
\begin{figure}[h]
	\centering
	\includegraphics[width=0.8\linewidth, height=0.8 \linewidth]{fig/region}
	\caption{Limits of privacy in the entire $m(n)-a_n$ plane: in regions $1$, $2$, and $3$, users have perfect privacy, and in region $4$ users have no privacy.}
	\label{fig:region}
\end{figure}

For the case where the users' data sets are governed by irreducible and aperiodic Markov chains with $r$ states and $|E|$ edges, we show that users will have no privacy if $m =cn^{\frac{2}{|E|-r} +  \alpha}$ and $a_n =c'n^{-\left(\frac{1}{|E|-r}+\beta \right)}$, for some constants $c>0$, $c'>0$, $\alpha>0$, and $\beta>\frac{\alpha}{4}$. We also provide some insights for the opposite direction (under which conditions users have perfect privacy) for the case of Markov chains. 




  




%\subsection{Summary of Results}

%When there are $n$ users in the network, the privacy level of the users depends on two parameters: (1) The %number of observations $m=m(n)$ by the adversary per user for a fixed anonymization mapping (i.e.~the %number of observations before the pseudonyms are changed);  (2) The noise level of the obfuscation %technique.  In this paper, the noise level of the obfuscation is increasing in a parameter $a_n$, which is %defined precisely in Section \ref{sec:framework}.  Intuitively, smaller $m(n)$ and larger $a_n$ result in %stronger location privacy but lower user utility. Thus, the fundamental question is, as the number of users %grows ($n \rightarrow \infty$), what values of $a_n$ and $m(n)$ are required to insure location privacy?

%In this paper, we answer the above question for the entire $m(n)- a_n$ plane for the case where each users' %movement is governed by an i.i.d process. We will prove that the $m(n)- a_n$ plane can be divided into two %areas.  In the first area, all users have perfect location privacy\cite{tifs2016}, as will be defined precisely in %Section \ref{sec:framework}, and, in the second area, users have no location privacy.  Figure~\ref{fig:region} %shows the limits of location privacy in the entire $m(n)- a_n$. In other words, according to %Figure~\ref{fig:region}, in regions $1$, $2$, and $3$, users have perfect location privacy, and  in region $4$ %users have no location privacy.
%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.9\linewidth, height=0.6 \linewidth]{fig/region}
%	\caption{Limits of location privacy in the entire $m(n)-a_n$ planes: in regions $1$, $2$, and $3$, users %have perfect location privacy, and in region $4$ users have no location privacy.}
%	\label{fig:region}
%\end{figure}
%
%Also, for the case where the users movements are governed by irreducible and aperiodic Markov chains with %$r$ states and $|E|$ edges, we show that users will have no privacy if $m =cn^{\frac{2}{|E|-r} +  \alpha}$ %and $a_n =c'n^{-\left(\frac{1}{|E|-r}+\alpha \right)}$ for some positive constants  $c, c'>0$  and %$0<\alpha<1$. Showing the opposite direction (under which conditions users have perfect privacy) for the %case of Markov chains is among the future work.

%In the rest of the paper we will provide the details of the results. Due to the space limitations, the proofs can %be found in the publicly available longer version of the paper ~\cite{longversion}.


==> Revised paper/ref.tex <==

\bibliographystyle{./IEEEtran}
\bibliography{./IEEEabrv,./IEEEexample}

@article{kousha2,
	title={Robust Privacy-Utility Tradeoffs Under Differential Privacy and Hamming Distortion},
	author={Kousha Kalantari and Lalitha Sankar and Anand D. Sarwate},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={13},
	number={11},
	pages={2816--2830},
	year={2018},
	publisher={IEEE}
}



@article{DBLP:ITjournal,
  author    = {Naanin Takbiri and
               Amir Houmansadr and
               Dennis Goeckel and
               Hossein Pishro-Nik},
  title     = {Matching Anonymized and Obfuscated Time Series to Users' Profiles
},
  journal   = {CoRR},
  volume    = {abs/1710.00197},
  year      = {2017},
  url       = {https://arxiv.org/abs/1710.00197},
  archivePrefix = {arXiv},
  eprint    = {1710.00197},
  timestamp = {Sat, 30 Sep 2017 13:03:19 GMT},
}


@inproceedings{KeConferance,
   title={Bayesian Time Series Matching and Privacy},
    author={Ke Le and 	Hossein Pishro-Nik and Dennis Goeckel},
	booktitle={51th Asilomar Conference on Signals, Systems and Computers},
   year={2017},
  	address={Pacific Grove, CA}
   }	

@article{DBLP:journals/corr/LiaoSCT17,
  author    = {Jiachun Liao and
               Lalitha Sankar and
               Fl{\'{a}}vio du Pin Calmon and
               Vincent Yan Fu Tan},
  title     = {Hypothesis Testing under Maximal Leakage Privacy Constraints},
  journal   = {CoRR},
  volume    = {abs/1701.07099},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.07099},
  timestamp = {Wed, 07 Jun 2017 14:40:47 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LiaoSCT17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{sankar,
    title={On information-theoretic privacy with general distortion cost functions},
    author={Kalantari, Kousha and Sankar, Lalitha and  Kosut, Oliver},
    booktitle={2017 IEEE International Symposium on Information Theory (ISIT)},
    year={2017},
      	address={Aachen, Germany},

    organization={IEEE}
    
  }	


@article{hyposankar,
  author    = {Jiachun Liao and
               Lalitha Sankar and
               Vincent Y. F. Tan and
               Fl{\'{a}}vio du Pin Calmon},
  title     = {Hypothesis Testing in the High Privacy Limit},
  journal   = {CoRR},
  volume    = {abs/1607.00533},
  year      = {2016},
  url       = {http://arxiv.org/abs/1607.00533},
  timestamp = {Wed, 07 Jun 2017 14:41:19 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LiaoSTC16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{battery15,
  author    = {Simon Li and
               Ashish Khisti and
               Aditya Mahajan},
  title     = {Privacy-Optimal Strategies for Smart Metering Systems with a Rechargeable
               Battery},
  journal   = {CoRR},
  volume    = {abs/1510.07170},
  year      = {2015},
  url       = {http://arxiv.org/abs/1510.07170},
  timestamp = {Wed, 07 Jun 2017 14:40:53 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LiKM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{geo2013,
   title={Geo-indistinguishability: differential privacy for location-based systems},
    author={Miguel E. Andres and Nicolas E. Bordenabe and Konstantinos Chatzikokolakis and Catuscia Palamidessi},
	booktitle={Proceedings of the 2013 ACM SIGSAC conference on Computer and communications security},

   year={2013},
   pages={901--914},
  	address={New York, NY}
   }	

@article{Yeb17,
  author    = {Min Ye and
               Alexander Barg},
  title     = {Optimal Schemes for Discrete Distribution Estimation under Locally
               Differential Privacy},
  journal   = {CoRR},
  volume    = {abs/1702.00610},
  year      = {2017},
  url       = {http://arxiv.org/abs/1702.00610},
  timestamp = {Wed, 07 Jun 2017 14:41:08 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/YeB17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{info2012,
    title={Information-Theoretic Foundations of Differential Privacy},
    author={Mir J. Darakhshan},
    booktitle={International Symposium on Foundations and Practice of Security},
    year={2012},
    organization={Springer}
  }	

@inproceedings{diff2017,
    title={Dynamic Differential Location Privacy with Personalized Error Bounds},
    author={Lei Yu and Ling Liu and Calton Pu},
    booktitle={The Network and Distributed System Security Symposium},
    year={2017}
  }	

@inproceedings{ciss2017,
    title={Fundamental Limits of Location Privacy using Anonymization},
    author={N. Takbiri and A. Houmansadr and D.L. Goeckel and H. Pishro-Nik},
    booktitle={Annual Conference on Information Science and Systems (CISS)},
    year={2017},
    organization={IEEE}
  }	

@inproceedings{sit2017,
    title={Limits of Location Privacy under Anonymization and Obfuscation},
    author={Nazanin Takbiri and Amir Houmansadr and Dennis L. Goeckel and Hossein Pishro-Nik},
    booktitle={International Symposium on Information Theory (ISIT)},
    year={2017},
    organization={IEEE}
  }	



@article{tifs2016,
	Author = {Z. Montazeri and A. Houmansadr and H. Pishro-Nik},
	Journal = {IEEE Transaction on Information Forensics and Security, to appear},
	Publisher = {IEEE},
	Title = {{Achieving Perfect Location Privacy in Wireless Devices Using Anonymization}},
	Year = {2017}}
	
	@article{matching,
  title={Asymptotically Optimal Matching of Multiple Sequences to Source Distributions and Training Sequences},
  author={Jayakrishnan Unnikrishnan},
  journal={IEEE Transactions on Information Theory},
  volume={61},
  number={1},
  pages={452-468},
  year={2015},
  publisher={IEEE}
}

@article{Naini2016,
	Author = {F. Naini and J. Unnikrishnan and P. Thiran and M. Vetterli},
	Journal = {IEEE Transactions on Information Forensics and Security},
	Publisher = {IEEE},
	Title = {Where You Are Is Who You Are: User Identification by Matching Statistics},
	 volume={11},
    number={2},
     pages={358--372},
    Year = {2016}
}



@inproceedings{montazeri2016defining,
    title={Defining perfect location privacy using anonymization},
    author={Montazeri, Zarrin and Houmansadr, Amir and Pishro-Nik, Hossein},
    booktitle={2016 Annual Conference on Information Science and Systems (CISS)},
    pages={204--209},
    year={2016},
    organization={IEEE}
  }	
	
	
@inproceedings{Mont1610Achieving,
  title={Achieving Perfect Location Privacy in Markov Models Using Anonymization},
  author={Montazeri, Zarrin and Houmansadr, Amir and H.Pishro-Nik},
  booktitle="2016 International Symposium on Information Theory and its Applications
  (ISITA2016)",
  address="Monterey, USA",
  days=30,
  month="oct",
  year=2016,
}

@misc{uber-stats,
title = {{By The Numbers 24 Amazing Uber Statistics}},
author = {Craig Smith},
note = {\url{http://expandedramblings.com/index.php/uber-statistics/}},
year=2015,
month= "September"
}


@misc{GMaps-users,
title = {{55\% of U.S. iOS users with Google Maps use it weekly}},
author = {Mike Dano},
note = {\url{http://www.fiercemobileit.com/story/55-us-ios-users-google-maps-use-it-weekly/2013-08-27}},
year=2013
}

@misc{Google-stats,
title = {{Statistics and facts about Google}},
note = {\url{http://www.statista.com/topics/1001/google/}},
}

@misc{yelp-stats,
title = {{By The Numbers: 45 Amazing Yelp Statistics}},
author = {Craig Smith},
note = {\url{http://expandedramblings.com/index.php/yelp-statistics/}},
year=2015,
month= "May"
}


@misc{Uber-hacker,
title = {{Is Uber's rider database a sitting duck for hackers?}},
author = {Craig Timberg},
note = {\url{https://www.washingtonpost.com/news/the-switch/wp/2014/12/01/is-ubers-rider-database-a-sitting-duck-for-hackers/}},
year=2014,
month= "December"
}

@misc{Uber-godview,
title = {{``God View'': Uber Investigates Its Top New York Executive For Privacy Violations}},
note = {\url{https://www.washingtonpost.com/news/the-switch/wp/2014/12/01/is-ubers-rider-database-a-sitting-duck-for-hackers/}},
year=2014,
month= "November"
}


@misc{Uber-breach-statement,
title = {{Uber Statement}},
note = {\url{http://newsroom.uber.com/2015/02/uber-statement/}},
year=2015,
month= "February"
}



@inproceedings{zhou2007privacy,
  title={Privacy-preserving detection of sybil attacks in vehicular ad hoc networks},
  author={Zhou, Tong and Choudhury, Romit Roy and Ning, Peng and Chakrabarty, Krishnendu},
  booktitle={Mobile and Ubiquitous Systems: Networking \& Services, 2007. MobiQuitous 2007. Fourth Annual International Conference on},
  pages={1--8},
  year={2007},
  organization={IEEE}
}

@article{chang2012footprint,
  title={Footprint: Detecting sybil attacks in urban vehicular networks},
  author={Chang, Shan and Qi, Yong and Zhu, Hongzi and Zhao, Jizhong and Shen, Xuemin Sherman},
  journal={Parallel and Distributed Systems, IEEE Transactions on},
  volume={23},
  number={6},
  pages={1103--1114},
  year={2012},
  publisher={IEEE}
}

@inproceedings{shokri2012protecting,
	Author = {Shokri, Reza and Theodorakopoulos, George and Troncoso, Carmela and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
	Booktitle = {Proceedings of the 2012 ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {617--627},
	Title = {Protecting location privacy: optimal strategy against localization attacks},
	Year = {2012}}


@inproceedings{gruteser2003anonymous,
	Author = {Gruteser, Marco and Grunwald, Dirk},
	Booktitle = {Proceedings of the 1st international conference on Mobile systems, applications and services},
	Organization = {ACM},
	Pages = {31--42},
	Title = {Anonymous usage of location-based services through spatial and temporal cloaking},
	Year = {2003}}



@inproceedings{hoh2007preserving,
	Author = {Hoh, Baik and Gruteser, Marco and Xiong, Hui and Alrabady, Ansaf},
	Booktitle = {Proceedings of the 14th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {161--171},
	Title = {Preserving privacy in gps traces via uncertainty-aware path cloaking},
	Year = {2007}}


@inproceedings{shokri2011quantifying,
	Author = {Shokri, Reza and Theodorakopoulos, George and Le Boudec, Jean-Yves and Hubaux, Jean-Pierre},
	Booktitle = {Security and Privacy (SP), 2011 IEEE Symposium on},
	Organization = {IEEE},
	Pages = {247--262},
	Title = {Quantifying location privacy},
	Year = {2011}}


@inproceedings{bordenabe2014optimal,
	Author = {Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2014 ACM SIGSAC Conference on Computer and Communications Security},
	Organization = {ACM},
	Pages = {251--262},
	Title = {Optimal geo-indistinguishable mechanisms for location privacy},
	Year = {2014}}




@inproceedings{freudiger2009non,
	Author = {Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
	Booktitle = {Proceedings of the 16th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {324--337},
	Title = {On non-cooperative location privacy: a game-theoretic analysis},
	Year = {2009}}

@inproceedings{ma2009location,
	Author = {Ma, Zhendong and Kargl, Frank and Weber, Michael},
	Booktitle = {Sarnoff Symposium, 2009. SARNOFF'09. IEEE},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {A location privacy metric for v2x communication systems},
	Year = {2009}}

@article{1corser2016evaluating,
  title={Evaluating Location Privacy in Vehicular Communications and Applications},
  author={Corser, George P and Fu, Huirong and Banihani, Abdelnasser},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={17},
  number={9},
  pages={2658-2667},
  year={2016},
  publisher={IEEE}
}
@article{2zhang2016designing,
  title={On Designing Satisfaction-Ratio-Aware Truthful Incentive Mechanisms for k-Anonymity Location Privacy},
  author={Zhang, Yuan and Tong, Wei and Zhong, Sheng},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={11},
  number={11},
  pages={2528--2541},
  year={2016},
  publisher={IEEE}
}

@article{11dewri2014exploiting,
  title={Exploiting service similarity for privacy in location-based search queries},
  author={Dewri, Rinku and Thurimella, Ramakrisha},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={25},
  number={2},
  pages={374--383},
  year={2014},
  publisher={IEEE}
}

@inproceedings{gedik2005location,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Booktitle = {Distributed Computing Systems, 2005. ICDCS 2005. Proceedings. 25th IEEE International Conference on},
	Organization = {IEEE},
	Pages = {620--629},
	Title = {Location privacy in mobile systems: A personalized anonymization model},
	Year = {2005}}

@inproceedings{zhong2009distributed,
	Author = {Zhong, Ge and Hengartner, Urs},
	Booktitle = {Pervasive Computing and Communications, 2009. PerCom 2009. IEEE International Conference on},
	Organization = {IEEE},
	Pages = {1--10},
	Title = {A distributed k-anonymity protocol for location privacy},
	Year = {2009}}

@inproceedings{mokbel2006new,
	Author = {Mokbel, Mohamed F and Chow, Chi-Yin and Aref, Walid G},
	Booktitle = {Proceedings of the 32nd international conference on Very large data bases},
	Organization = {VLDB Endowment},
	Pages = {763--774},
	Title = {The new Casper: query processing for location services without compromising privacy},
	Year = {2006}}

@article{kalnis2007preventing,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {12},
	Pages = {1719--1733},
	Publisher = {IEEE},
	Title = {Preventing location-based identity inference in anonymous spatial queries},
	Volume = {19},
	Year = {2007}}


@article{sweeney2002k,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {557--570},
	Publisher = {World Scientific},
	Title = {k-anonymity: A model for protecting privacy},
	Volume = {10},
	Year = {2002}}

@article{sweeney2002achieving,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {571-588},
	Publisher = {World Scientific},
	Title = {Achieving k-anonymity privacy protection using generalization and suppression},
	Volume = {10},
	Year = {2002}}

@inproceedings{liu2013game,
	Author = {Liu, Xinxin and Liu, Kaikai and Guo, Linke and Li, Xiaolin and Fang, Yuguang},
	Booktitle = {INFOCOM, 2013 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {2985--2993},
	Title = {A game-theoretic approach for achieving k-anonymity in location based services},
	Year = {2013}}

@inproceedings{hoh2005protecting,
	Author = {Hoh, Baik and Gruteser, Marco},
	Booktitle = {Security and Privacy for Emerging Areas in Communications Networks, 2005. SecureComm 2005. First International Conference on},
	Organization = {IEEE},
	Pages = {194--205},
	Title = {Protecting location privacy through path confusion},
	Year = {2005}}

@article{beresford2003location,
	Author = {Beresford, Alastair R and Stajano, Frank},
	Journal = {IEEE Pervasive computing},
	Number = {1},
	Pages = {46--55},
	Publisher = {IEEE},
	Title = {Location privacy in pervasive computing},
	Year = {2003}}


@inproceedings{palanisamy2011mobimix,
	Author = {Palanisamy, Balaji and Liu, Ling},
	Booktitle = {Data Engineering (ICDE), 2011 IEEE 27th International Conference on},
	Organization = {IEEE},
	Pages = {494--505},
	Title = {Mobimix: Protecting location privacy with mix-zones over road networks},
	Year = {2011}}
@inproceedings{freudiger2009optimal,
	Author = {Freudiger, Julien and Shokri, Reza and Hubaux, Jean-Pierre},
	Booktitle = {Privacy enhancing technologies},
	Organization = {Springer},
	Pages = {216--234},
	Title = {On the optimal placement of mix zones},
	Year = {2009}}

@article{manshaei2013game,
	Author = {Manshaei, Mohammad Hossein and Zhu, Quanyan and Alpcan, Tansu and Bac{\c{s}}ar, Tamer and Hubaux, Jean-Pierre},
	Journal = {ACM Computing Surveys (CSUR)},
	Number = {3},
	Pages = {25},
	Publisher = {ACM},
	Title = {Game theory meets network security and privacy},
	Volume = {45},
	Year = {2013}}

@article{19freudiger2013non,
  title={Non-cooperative location privacy},
  author={Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
  journal={IEEE Transactions on Dependable and Secure Computing},
  volume={10},
  number={2},
  pages={84--98},
  year={2013},
  publisher={IEEE}
}


@article{paulet2014privacy,
	Author = {Paulet, Russell and Kaosar, Md Golam and Yi, Xun and Bertino, Elisa},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {5},
	Pages = {1200--1210},
	Publisher = {IEEE},
	Title = {Privacy-preserving and content-protecting location based queries},
	Volume = {26},
	Year = {2014}}

@article{khoshgozaran2011location,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus and Shirani-Mehr, Houtan},
	Journal = {Knowledge and Information Systems},
	Number = {3},
	Pages = {435--465},
	Publisher = {Springer},
	Title = {Location privacy: going beyond K-anonymity, cloaking and anonymizers},
	Volume = {26},
	Year = {2011}}

@article{18shokri2014hiding,
  title={Hiding in the mobile crowd: Locationprivacy through collaboration},
  author={Shokri, Reza and Theodorakopoulos, George and Papadimitratos, Panos and Kazemi, Ehsan and Hubaux, Jean-Pierre},
  journal={IEEE transactions on dependable and secure computing},
  volume={11},
  number={3},
  pages={266--279},
  year={2014},
  publisher={IEEE}
}

@article{8zurbaran2015near,
  title={Near-Rand: Noise-based Location Obfuscation Based on Random Neighboring Points},
  author={Zurbaran, Mayra Alejandra and Avila, Karen and Wightman, Pedro and Fernandez, Michael},
  journal={IEEE Latin America Transactions},
  volume={13},
  number={11},
  pages={3661--3667},
  year={2015},
  publisher={IEEE}
}

@inproceedings{hoh2007preserving,
	Author = {Hoh, Baik and Gruteser, Marco and Xiong, Hui and Alrabady, Ansaf},
	Booktitle = {Proceedings of the 14th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {161--171},
	Title = {Preserving privacy in gps traces via uncertainty-aware path cloaking},
	Year = {2007}}

@inproceedings{ho2011differential,
	Author = {Ho, Shen-Shyang and Ruan, Shuhua},
	Booktitle = {Proceedings of the 4th ACM SIGSPATIAL International Workshop on Security and Privacy in GIS and LBS},
	Organization = {ACM},
	Pages = {17--24},
	Title = {Differential privacy for location pattern mining},
	Year = {2011}}


@article{12hwang2014novel,
  title={A novel time-obfuscated algorithm for trajectory privacy protection},
  author={Hwang, Ren-Hung and Hsueh, Yu-Ling and Chung, Hao-Wei},
  journal={IEEE Transactions on Services Computing},
  volume={7},
  number={2},
  pages={126--139},
  year={2014},
  publisher={IEEE}
  }

  @article{16haghnegahdar2014privacy,
  title={Privacy Risks in Publishing Mobile Device Trajectories},
  author={Haghnegahdar, Alireza and Khabbazian, Majid and Bhargava, Vijay K},
  journal={IEEE Wireless Communications Letters},
  volume={3},
  number={3},
  pages={241--244},
  year={2014},
  publisher={IEEE}
}

@article{20gao2013trpf,
  title={TrPF: A trajectory privacy-preserving framework for participatory sensing},
  author={Gao, Sheng and Ma, Jianfeng and Shi, Weisong and Zhan, Guoxing and Sun, Cong},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={8},
  number={6},
  pages={874--887},
  year={2013},
  publisher={IEEE}
}

@article{21ma2013privacy,
  title={Privacy vulnerability of published anonymous mobility traces},
  author={Ma, Chris YT and Yau, David KY and Yip, Nung Kwan and Rao, Nageswara SV},
  journal={IEEE/ACM Transactions on Networking},
  volume={21},
  number={3},
  pages={720--733},
  year={2013},
  publisher={IEEE}
}

@article{6li2016privacy,
  title={Privacy Leakage of Location Sharing in Mobile Social Networks: Attacks and Defense},
  author={Li, Huaxin and Zhu, Haojin and Du, Suguo and Liang, Xiaohui and Shen, Xuemin},
  journal={IEEE Transactions on Dependable and Secure Computing},
  year={2016},
  volume={PP},
  number={99},
  publisher={IEEE}
}


@article{14zhang2014privacy,
  title={Privacy quantification model based on the Bayes conditional risk in Location-Based Services},
  author={Zhang, Xuejun and Gui, Xiaolin and Tian, Feng and Yu, Si and An, Jian},
  journal={Tsinghua Science and Technology},
  volume={19},
  number={5},
  pages={452--462},
  year={2014},
  publisher={TUP}
}

@article{4olteanu2016quantifying,
  title={Quantifying Interdependent Privacy Risks with Location Data},
  author={Olteanu, Alexandra-Mihaela and Huguenin, K{\'e}vin and Shokri, Reza and Humbert, Mathias and Hubaux, Jean-Pierre},
  journal={IEEE Transactions on Mobile Computing},
  year={2016},
  volume={PP},
  number={99},
  pages={1-1},
  publisher={IEEE}
}















@misc{Leberknight2010,
	Author = {Leberknight, C. and Chiang, M. and Poor, H. and Wong, F.},
	Howpublished = {\url{http://www.princeton.edu/~chiangm/anticensorship.pdf}},
	Title = {{A Taxonomy of Internet Censorship and Anti-censorship}},
	Year = {2010}}

@techreport{ultrasurf-analysis,
	Author = {Appelbaum, Jacob},
	Institution = {The Tor Project},
	Title = {{Technical analysis of the Ultrasurf proxying software}},
	Url = {http://scholar.google.com/scholar?hl=en\&btnG=Search\&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software\#0},
	Year = {2012},
	Bdsk-Url-1 = {http://scholar.google.com/scholar?hl=en%5C&btnG=Search%5C&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software%5C#0}}

@misc{gifc:07,
	Howpublished = {\url{http://www.internetfreedom.org/archive/Defeat\_Internet\_Censorship\_White\_Paper.pdf}},
	Key = {defeatcensorship},
	Publisher = {Global Internet Freedom Consortium (GIFC)},
	Title = {{Defeat Internet Censorship: Overview of Advanced Technologies and Products}},
	Type = {White Paper},
	Year = {2007}}

@article{pan2011survey,
	Author = {Pan, J. and Paul, S. and Jain, R.},
	Journal = {Communications Magazine, IEEE},
	Number = {7},
	Pages = {26--36},
	Publisher = {IEEE},
	Title = {{A Survey of the Research on Future Internet Architectures}},
	Volume = {49},
	Year = {2011}}

@misc{nsf-fia,
	Howpublished = {\url{http://www.nets-fia.net/}},
	Key = {FIA},
	Title = {{NSF Future Internet Architecture Project}}}

@misc{NDN,
	Howpublished = {\url{http://www.named- data.net}},
	Key = {NDN},
	Title = {{Named Data Networking Project}}}

@inproceedings{MobilityFirst,
	Author = {Seskar, I. and Nagaraja, K. and Nelson, S. and Raychaudhuri, D.},
	Booktitle = {Asian Internet Engineering Conference},
	Title = {{Mobilityfirst Future internet Architecture Project}},
	Year = {2011}}

@incollection{NEBULA,
	Author = {Anderson, T. and Birman, K. and Broberg, R. and Caesar, M. and Comer, D. and Cotton, C. and Freedman, M.~J. and Haeberlen, A. and Ives, Z.~G. and Krishnamurthy, A. and others},
	Booktitle = {The Future Internet},
	Pages = {16--26},
	Publisher = {Springer},
	Title = {{The NEBULA Future Internet Architecture}},
	Year = {2013}}

@inproceedings{XIA,
	Author = {Anand, A. and Dogar, F. and Han, D. and Li, B. and Lim, H. and Machado, M. and Wu, W. and Akella, A. and Andersen, D.~G. and Byers, J.~W. and others},
	Booktitle = {ACM Workshop on Hot Topics in Networks},
	Pages = {2},
	Title = {{XIA: An Architecture for an Evolvable and Trustworthy Internet}},
	Year = {2011}}

@inproceedings{ChoiceNet,
	Author = {Rouskas, G.~N. and Baldine, I. and Calvert, K.~L. and Dutta, R. and Griffioen, J. and Nagurney, A. and Wolf, T.},
	Booktitle = {ONDM},
	Title = {{ChoiceNet: Network Innovation Through Choice}},
	Year = {2013}}

@misc{nsf-find,
	Howpublished = {http://www.nets-find.net/},
	Title = {{NSF NeTS FIND Initiative}}}

@article{traid,
	Author = {Cheriton, D.~R. and Gritter, M.},
	Title = {{TRIAD: A New Next-Generation Internet Architecture}},
	Year = {2000}}

@inproceedings{dona,
	Author = {Koponen, T. and Chawla, M. and Chun, B-G. and Ermolinskiy, A. and Kim, K.~H. and Shenker, S. and Stoica, I.},
	Booktitle = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Organization = {ACM},
	Pages = {181--192},
	Title = {{A Data-Oriented (and Beyond) Network Architecture}},
	Volume = {37},
	Year = {2007}}

@misc{ultrasurf,
	Howpublished = {\url{http://www.ultrareach.com}},
	Key = {ultrasurf},
	Title = {{Ultrasurf}}}

@misc{tor-bridge,
	Author = {Dingledine, R. and Mathewson, N.},
	Howpublished = {\url{https://svn.torproject.org/svn/projects/design-paper/blocking.html}},
	Title = {{Design of a Blocking-Resistant Anonymity System}}}

@inproceedings{McLachlanH09,
	Author = {J. McLachlan and N. Hopper},
	Booktitle = {WPES},
	Title = {{On the Risks of Serving Whenever You Surf: Vulnerabilities in Tor's Blocking Resistance Design}},
	Year = {2009}}

@inproceedings{mahdian2010,
	Author = {Mahdian, M.},
	Booktitle = {{Fun with Algorithms}},
	Title = {{Fighting Censorship with Algorithms}},
	Year = {2010}}

@inproceedings{McCoy2011,
	Author = {McCoy, D. and Morales, J.~A. and Levchenko, K.},
	Booktitle = {FC},
	Title = {{Proximax: A Measurement Based System for Proxies Dissemination}},
	Year = {2011}}

@inproceedings{Sovran2008,
	Author = {Sovran, Y. and Libonati, A. and Li, J.},
	Booktitle = {IPTPS},
	Title = {{Pass it on: Social Networks Stymie Censors}},
	Year = {2008}}

@inproceedings{rbridge,
	Author = {Wang, Q. and Lin, Zi and Borisov, N. and Hopper, N.},
	Booktitle = {{NDSS}},
	Title = {{rBridge: User Reputation based Tor Bridge Distribution with Privacy Preservation}},
	Year = {2013}}

@inproceedings{telex,
	Author = {Wustrow, E. and Wolchok, S. and Goldberg, I. and Halderman, J.},
	Booktitle = {{USENIX Security}},
	Title = {{Telex: Anticensorship in the Network Infrastructure}},
	Year = {2011}}

@inproceedings{cirripede,
	Author = {Houmansadr, A. and Nguyen, G. and Caesar, M. and Borisov, N.},
	Booktitle = {CCS},
	Title = {{Cirripede: Circumvention Infrastructure Using Router Redirection with Plausible Deniability}},
	Year = {2011}}

@inproceedings{decoyrouting,
	Author = {Karlin, J. and Ellard, D. and Jackson, A. and Jones, C. and Lauer, G. and Mankins, D. and Strayer, W.},
	Booktitle = {{FOCI}},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = {2011}}

@inproceedings{routing-around-decoys,
	Author = {M.~Schuchard and J.~Geddes and C.~Thompson and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Routing Around Decoys}},
	Year = {2012}}

@inproceedings{parrot,
	Author = {A. Houmansadr and C. Brubaker and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{The Parrot is Dead: Observing Unobservable Network Communications}},
	Year = {2013}}

@misc{knock,
	Author = {T. Wilde},
	Howpublished = {\url{https://blog.torproject.org/blog/knock-knock-knockin-bridges-doors}},
	Title = {{Knock Knock Knockin' on Bridges' Doors}},
	Year = {2012}}

@inproceedings{china-tor,
	Author = {Winter, P. and Lindskog, S.},
	Booktitle = {{FOCI}},
	Title = {{How the Great Firewall of China Is Blocking Tor}},
	Year = {2012}}

@misc{discover-bridge,
	Howpublished = {\url{https://blog.torproject.org/blog/research-problems-ten-ways-discover-tor-bridges}},
	Key = {tenways},
	Title = {{Ten Ways to Discover Tor Bridges}}}

@inproceedings{freewave,
	Author = {A.~Houmansadr and T.~Riedl and N.~Borisov and A.~Singer},
	Booktitle = {{NDSS}},
	Title = {{I Want My Voice to Be Heard: IP over Voice-over-IP for Unobservable Censorship Circumvention}},
	Year = 2013}

@inproceedings{censorspoofer,
	Author = {Q. Wang and X. Gong and G. Nguyen and A. Houmansadr and N. Borisov},
	Booktitle = {CCS},
	Title = {{CensorSpoofer: Asymmetric Communication Using IP Spoofing for Censorship-Resistant Web Browsing}},
	Year = {2012}}

@inproceedings{skypemorph,
	Author = {H. Moghaddam and B. Li and M. Derakhshani and I. Goldberg},
	Booktitle = {CCS},
	Title = {{SkypeMorph: Protocol Obfuscation for Tor Bridges}},
	Year = {2012}}

@inproceedings{stegotorus,
	Author = {Weinberg, Z. and Wang, J. and Yegneswaran, V. and Briesemeister, L. and Cheung, S. and Wang, F. and Boneh, D.},
	Booktitle = {CCS},
	Title = {{StegoTorus: A Camouflage Proxy for the Tor Anonymity System}},
	Year = {2012}}

@techreport{dust,
	Author = {{B.~Wiley}},
	Howpublished = {\url{http://blanu.net/ Dust.pdf}},
	Institution = {School of Information, University of Texas at Austin},
	Title = {{Dust: A Blocking-Resistant Internet Transport Protocol}},
	Year = {2011}}

@inproceedings{FTE,
	Author = {K.~Dyer and S.~Coull and T.~Ristenpart and T.~Shrimpton},
	Booktitle = {CCS},
	Title = {{Protocol Misidentification Made Easy with Format-Transforming Encryption}},
	Year = {2013}}

@inproceedings{fp,
	Author = {Fifield, D. and Hardison, N. and Ellithrope, J. and Stark, E. and Dingledine, R. and Boneh, D. and Porras, P.},
	Booktitle = {PETS},
	Title = {{Evading Censorship with Browser-Based Proxies}},
	Year = {2012}}

@misc{obfsproxy,
	Howpublished = {\url{https://www.torproject.org/projects/obfsproxy.html.en}},
	Key = {obfsproxy},
	Publisher = {The Tor Project},
	Title = {{A Simple Obfuscating Proxy}}}

@inproceedings{Tor-instead-of-IP,
	Author = {Liu, V. and Han, S. and Krishnamurthy, A. and Anderson, T.},
	Booktitle = {HotNets},
	Title = {{Tor instead of IP}},
	Year = {2011}}

@misc{roger-slides,
	Howpublished = {\url{https://svn.torproject.org/svn/projects/presentations/slides-28c3.pdf}},
	Key = {torblocking},
	Title = {{How Governments Have Tried to Block Tor}}}

@inproceedings{infranet,
	Author = {Feamster, N. and Balazinska, M. and Harfst, G. and Balakrishnan, H. and Karger, D.},
	Booktitle = {USENIX Security},
	Title = {{Infranet: Circumventing Web Censorship and Surveillance}},
	Year = {2002}}

@inproceedings{collage,
	Author = {S.~Burnett and N.~Feamster and S.~Vempala},
	Booktitle = {USENIX Security},
	Title = {{Chipping Away at Censorship Firewalls with User-Generated Content}},
	Year = {2010}}

@article{anonymizer,
	Author = {Boyan, J.},
	Journal = {Computer-Mediated Communication Magazine},
	Month = sep,
	Number = {9},
	Title = {{The Anonymizer: Protecting User Privacy on the Web}},
	Volume = {4},
	Year = {1997}}

@article{schulze2009internet,
	Author = {Schulze, H. and Mochalski, K.},
	Journal = {IPOQUE Report},
	Pages = {351--362},
	Title = {Internet Study 2008/2009},
	Volume = {37},
	Year = {2009}}

@inproceedings{cya-ccs13,
	Author = {J.~Geddes and M.~Schuchard and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Cover Your ACKs: Pitfalls of Covert Channel Censorship Circumvention}},
	Year = {2013}}

@inproceedings{andana,
	Author = {DiBenedetto, S. and Gasti, P. and Tsudik, G. and Uzun, E.},
	Booktitle = {{NDSS}},
	Title = {{ANDaNA: Anonymous Named Data Networking Application}},
	Year = {2012}}

@inproceedings{darkly,
	Author = {Jana, S. and Narayanan, A. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{A Scanner Darkly: Protecting User Privacy From Perceptual Applications}},
	Year = {2013}}

@inproceedings{NS08,
	Author = {A.~Narayanan and V.~Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {Robust de-anonymization of large sparse datasets},
	Year = {2008}}

@inproceedings{NS09,
	Author = {A.~Narayanan and V.~Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {De-anonymizing social networks},
	Year = {2009}}

@inproceedings{memento,
	Author = {Jana, S. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{Memento: Learning secrets from process footprints}},
	Year = {2012}}

@misc{plugtor,
	Howpublished = {\url{https://www.torproject.org/docs/pluggable-transports.html.en}},
	Key = {PluggableTransports},
	Publisher = {The Tor Project},
	Title = {{Tor: Pluggable transports}}}

@misc{psiphon,
	Author = {J.~Jia and P.~Smith},
	Howpublished = {\url{http://www.cdf.toronto.edu/~csc494h/reports/2004-fall/psiphon_ae.html}},
	Title = {{Psiphon: Analysis and Estimation}},
	Year = 2004}

@misc{china-github,
	Howpublished = {\url{http://mobile.informationweek.com/80269/show/72e30386728f45f56b343ddfd0fdb119/}},
	Key = {github},
	Title = {{China's GitHub Censorship Dilemma}}}

@inproceedings{txbox,
	Author = {Jana, S. and Porter, D. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{TxBox: Building Secure, Efficient Sandboxes with System Transactions}},
	Year = {2011}}

@inproceedings{airavat,
	Author = {I. Roy and S. Setty and A. Kilzer and V. Shmatikov and E. Witchel},
	Booktitle = {NSDI},
	Title = {{Airavat: Security and Privacy for MapReduce}},
	Year = {2010}}

@inproceedings{osdi12,
	Author = {A. Dunn and M. Lee and S. Jana and S. Kim and M. Silberstein and Y. Xu and V. Shmatikov and E. Witchel},
	Booktitle = {OSDI},
	Title = {{Eternal Sunshine of the Spotless Machine: Protecting Privacy with Ephemeral Channels}},
	Year = {2012}}

@inproceedings{ymal,
	Author = {J. Calandrino and A. Kilzer and A. Narayanan and E. Felten and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{``You Might Also Like:'' Privacy Risks of Collaborative Filtering}},
	Year = {2011}}

@inproceedings{srivastava11,
	Author = {V. Srivastava and M. Bond and K. McKinley and V. Shmatikov},
	Booktitle = {PLDI},
	Title = {{A Security Policy Oracle: Detecting Security Holes Using Multiple API Implementations}},
	Year = {2011}}

@inproceedings{chen-oakland10,
	Author = {Chen, S. and Wang, R. and Wang, X. and Zhang, K.},
	Booktitle = {IEEE S\&P},
	Title = {{Side-Channel Leaks in Web Applications: A Reality Today, a Challenge Tomorrow}},
	Year = {2010}}

@book{kerck,
	Author = {Kerckhoffs, A.},
	Publisher = {University Microfilms},
	Title = {{La cryptographie militaire}},
	Year = {1978}}

@inproceedings{foci11,
	Author = {J. Karlin and D. Ellard and A.~Jackson and C.~ Jones and G. Lauer and D. Mankins and W.~T.~Strayer},
	Booktitle = {FOCI},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = 2011}

@inproceedings{sun02,
	Author = {Sun, Q. and Simon, D.~R. and Wang, Y. and Russell, W. and Padmanabhan, V. and Qiu, L.},
	Booktitle = {IEEE S\&P},
	Title = {{Statistical Identification of Encrypted Web Browsing Traffic}},
	Year = {2002}}

@inproceedings{danezis,
	Author = {Murdoch, S.~J. and Danezis, G.},
	Booktitle = {IEEE S\&P},
	Title = {{Low-Cost Traffic Analysis of Tor}},
	Year = {2005}}

@inproceedings{pakicensorship,
	Author = {Z.~Nabi},
	Booktitle = {FOCI},
	Title = {The Anatomy of {Web} Censorship in {Pakistan}},
	Year = {2013}}

@inproceedings{irancensorship,
	Author = {S.~Aryan and H.~Aryan and A.~Halderman},
	Booktitle = {FOCI},
	Title = {Internet Censorship in {Iran}: {A} First Look},
	Year = {2013}}

@inproceedings{ford10efficient,
	Author = {Amittai Aviram and Shu-Chun Weng and Sen Hu and Bryan Ford},
	Booktitle = {\bibconf[9th]{OSDI}{USENIX Symposium on Operating Systems Design and Implementation}},
	Location = {Vancouver, BC, Canada},
	Month = oct,
	Title = {Efficient System-Enforced Deterministic Parallelism},
	Year = 2010}

@inproceedings{ford10determinating,
	Author = {Amittai Aviram and Sen Hu and Bryan Ford and Ramakrishna Gummadi},
	Booktitle = {\bibconf{CCSW}{ACM Cloud Computing Security Workshop}},
	Location = {Chicago, IL},
	Month = oct,
	Title = {Determinating Timing Channels in Compute Clouds},
	Year = 2010}

@inproceedings{ford12plugging,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Plugging Side-Channel Leaks with Timing Information Flow Control},
	Year = 2012}

@inproceedings{ford12icebergs,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Icebergs in the Clouds: the {\em Other} Risks of Cloud Computing},
	Year = 2012}

@misc{mullenize,
	Author = {Washington Post},
	Howpublished = {\url{http://apps.washingtonpost.com/g/page/world/gchq-report-on-mullenize-program-to-stain-anonymous-electronic-traffic/502/}},
	Month = {oct},
	Title = {{GCHQ} report on {`MULLENIZE'} program to `stain' anonymous electronic traffic},
	Year = {2013}}

@inproceedings{shue13street,
	Author = {Craig A. Shue and Nathanael Paul and Curtis R. Taylor},
	Booktitle = {\bibbrev[7th]{WOOT}{USENIX Workshop on Offensive Technologies}},
	Month = aug,
	Title = {From an {IP} Address to a Street Address: Using Wireless Signals to Locate a Target},
	Year = 2013}

@inproceedings{knockel11three,
	Author = {Jeffrey Knockel and Jedidiah R. Crandall and Jared Saia},
	Booktitle = {\bibbrev{FOCI}{USENIX Workshop on Free and Open Communications on the Internet}},
	Location = {San Francisco, CA},
	Month = aug,
	Year = 2011}

@misc{rfc4960,
	Author = {R. {Stewart, ed.}},
	Month = sep,
	Note = {RFC 4960},
	Title = {Stream Control Transmission Protocol},
	Year = 2007}

@inproceedings{ford07structured,
	Author = {Bryan Ford},
	Booktitle = {\bibbrev{SIGCOMM}{ACM SIGCOMM}},
	Location = {Kyoto, Japan},
	Month = aug,
	Title = {Structured Streams: a New Transport Abstraction},
	Year = {2007}}

@misc{spdy,
	Author = {Google, Inc.},
	Note = {\url{http://www.chromium.org/spdy/spdy-whitepaper}},
	Title = {{SPDY}: An Experimental Protocol For a Faster {Web}}}

@misc{quic,
	Author = {Jim Roskind},
	Month = jun,
	Note = {\url{http://blog.chromium.org/2013/06/experimenting-with-quic.html}},
	Title = {Experimenting with {QUIC}},
	Year = 2013}

@misc{podjarny12not,
	Author = {G.~Podjarny},
	Month = jun,
	Note = {\url{http://www.guypo.com/technical/not-as-spdy-as-you-thought/}},
	Title = {{Not as SPDY as You Thought}},
	Year = 2012}

@inproceedings{cor,
	Author = {Jones, N.~A. and Arye, M. and Cesareo, J. and Freedman, M.~J.},
	Booktitle = {FOCI},
	Title = {{Hiding Amongst the Clouds: A Proposal for Cloud-based Onion Routing}},
	Year = {2011}}

@misc{torcloud,
	Howpublished = {\url{https://cloud.torproject.org/}},
	Key = {tor cloud},
	Title = {{The Tor Cloud Project}}}

@inproceedings{scramblesuit,
	Author = {Philipp Winter and Tobias Pulls and Juergen Fuss},
	Booktitle = {WPES},
	Title = {{ScrambleSuit: A Polymorphic Network Protocol to Circumvent Censorship}},
	Year = 2013}

@article{savage2000practical,
	Author = {Savage, S. and Wetherall, D. and Karlin, A. and Anderson, T.},
	Journal = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Pages = {295--306},
	Publisher = {ACM},
	Title = {Practical network support for IP traceback},
	Volume = {30},
	Year = {2000}}

@inproceedings{ooni,
	Author = {Filast, A. and Appelbaum, J.},
	Booktitle = {{FOCI}},
	Title = {{OONI : Open Observatory of Network Interference}},
	Year = {2012}}

@misc{caida-rank,
	Howpublished = {\url{http://as-rank.caida.org/}},
	Key = {caida rank},
	Title = {{AS Rank: AS Ranking}}}

@inproceedings{usersrouted-ccs13,
	Author = {A.~Johnson and C.~Wacek and R.~Jansen and M.~Sherr and P.~Syverson},
	Booktitle = {CCS},
	Title = {{Users Get Routed: Traffic Correlation on Tor by Realistic Adversaries}},
	Year = {2013}}

@inproceedings{edman2009awareness,
	Author = {Edman, M. and Syverson, P.},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2009}}

@inproceedings{DecoyCosts,
	Author = {A.~Houmansadr and E.~L.~Wong and V.~Shmatikov},
	Booktitle = {NDSS},
	Title = {{No Direction Home: The True Cost of Routing Around Decoys}},
	Year = {2014}}

@article{cordon,
	Author = {Elahi, T. and Goldberg, I.},
	Journal = {University of Waterloo CACR},
	Title = {{CORDON--A Taxonomy of Internet Censorship Resistance Strategies}},
	Volume = {33},
	Year = {2012}}

@inproceedings{privex,
	Author = {T.~Elahi and G.~Danezis and I.~Goldberg	},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2014}}

@inproceedings{changeGuards,
	Author = {T.~Elahi and K.~Bauer and M.~AlSabah and R.~Dingledine and I.~Goldberg},
	Booktitle = {{WPES}},
	Title = {{ Changing of the Guards: Framework for Understanding and Improving Entry Guard Selection in Tor}},
	Year = {2012}}

@article{RAINBOW:Journal,
	Author = {A.~Houmansadr and N.~Kiyavash and N.~Borisov},
	Journal = {IEEE/ACM Transactions on Networking},
	Title = {{Non-Blind Watermarking of Network Flows}},
	Year = 2014}

@inproceedings{info-tod,
	Author = {A.~Houmansadr and S.~Gorantla and T.~Coleman and N.~Kiyavash and and N.~Borisov},
	Booktitle = {{CCS (poster session)}},
	Title = {{On the Channel Capacity of Network Flow Watermarking}},
	Year = {2009}}

@inproceedings{johnson2014game,
	Author = {Johnson, B. and Laszka, A. and Grossklags, J. and Vasek, M. and Moore, T.},
	Booktitle = {Workshop on Bitcoin Research},
	Title = {{Game-theoretic Analysis of DDoS Attacks Against Bitcoin Mining Pools}},
	Year = {2014}}

@incollection{laszka2013mitigation,
	Author = {Laszka, A. and Johnson, B. and Grossklags, J.},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {175--191},
	Publisher = {Springer},
	Title = {{Mitigation of Targeted and Non-targeted Covert Attacks as a Timing Game}},
	Year = {2013}}

@inproceedings{schottle2013game,
	Author = {Schottle, P. and Laszka, A. and Johnson, B. and Grossklags, J. and Bohme, R.},
	Booktitle = {EUSIPCO},
	Title = {{A Game-theoretic Analysis of Content-adaptive Steganography with Independent Embedding}},
	Year = {2013}}

@inproceedings{CloudTransport,
	Author = {C.~Brubaker and A.~Houmansadr and V.~Shmatikov},
	Booktitle = {PETS},
	Title = {{CloudTransport: Using Cloud Storage for Censorship-Resistant Networking}},
	Year = {2014}}

@inproceedings{sweet,
	Author = {W.~Zhou and A.~Houmansadr and M.~Caesar and N.~Borisov},
	Booktitle = {HotPETs},
	Title = {{SWEET: Serving the Web by Exploiting Email Tunnels}},
	Year = {2013}}

@inproceedings{ahsan2002practical,
	Author = {Ahsan, K. and Kundur, D.},
	Booktitle = {Workshop on Multimedia Security},
	Title = {{Practical data hiding in TCP/IP}},
	Year = {2002}}

@incollection{danezis2011covert,
	Author = {Danezis, G.},
	Booktitle = {Security Protocols XVI},
	Pages = {198--214},
	Publisher = {Springer},
	Title = {{Covert Communications Despite Traffic Data Retention}},
	Year = {2011}}

@inproceedings{liu2009hide,
	Author = {Liu, Y. and Ghosal, D. and Armknecht, F. and Sadeghi, A.-R. and Schulz, S. and Katzenbeisser, S.},
	Booktitle = {ESORICS},
	Title = {{Hide and Seek in Time---Robust Covert Timing Channels}},
	Year = {2009}}

@misc{image-watermark-fing,
	Author = {Jonathan Bailey},
	Howpublished = {\url{https://www.plagiarismtoday.com/2009/12/02/image-detection-watermarking-vs-fingerprinting/}},
	Title = {{Image Detection: Watermarking vs. Fingerprinting}},
	Year = {2009}}

@inproceedings{Servetto98,
	Author = {S. D. Servetto and C. I. Podilchuk and K. Ramchandran},
	Booktitle = {Int. Conf. Image Processing},
	Title = {Capacity issues in digital image watermarking},
	Year = {1998}}

@inproceedings{Chen01,
	Author = {B. Chen and G.W.Wornell},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1423--1443},
	Title = {Quantization index modulation: A class of provably good methods for digital watermarking and information embedding},
	Year = {2001}}

@inproceedings{Karakos00,
	Author = {D. Karakos and A. Papamarcou},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {47},
	Title = {Relationship between quantization and distribution rates of digitally watermarked data},
	Year = {2000}}

@inproceedings{Sullivan98,
	Author = {J. A. OSullivan and P. Moulin and J. M. Ettinger},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {297},
	Title = {Information theoretic analysis of steganography},
	Year = {1998}}

@inproceedings{Merhav00,
	Author = {N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {420--430},
	Title = {On random coding error exponents of watermarking systems},
	Year = {2000}}

@inproceedings{Somekh01,
	Author = {A. Somekh-Baruch and N. Merhav},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {7},
	Title = {On the error exponent and capacity games of private watermarking systems},
	Year = {2001}}

@inproceedings{Steinberg01,
	Author = {Y. Steinberg and N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1410--1422},
	Title = {Identification in the presence of side information with application to watermarking},
	Year = {2001}}

@article{Moulin03,
	Author = {P. Moulin and J.A. O'Sullivan},
	Journal = {IEEE Trans. Info. Theory},
	Number = {3},
	Title = {Information-theoretic analysis of information hiding},
	Volume = 49,
	Year = 2003}

@article{Gelfand80,
	Author = {S.I.~Gelfand and M.S.~Pinsker},
	Journal = {Problems of Control and Information Theory},
	Number = {1},
	Pages = {19-31},
	Title = {{Coding for channel with random parameters}},
	Url = {citeseer.ist.psu.edu/anantharam96bits.html},
	Volume = {9},
	Year = {1980},
	Bdsk-Url-1 = {citeseer.ist.psu.edu/anantharam96bits.html}}

@book{Wolfowitz78,
	Author = {J. Wolfowitz},
	Edition = {3rd},
	Location = {New York},
	Publisher = {Springer-Verlag},
	Title = {Coding Theorems of Information Theory},
	Year = 1978}

@article{caire99,
	Author = {G. Caire and S. Shamai},
	Journal = {IEEE Transactions on Information Theory},
	Number = {6},
	Pages = {2007--2019},
	Title = {On the Capacity of Some Channels with Channel State Information},
	Volume = {45},
	Year = {1999}}

@inproceedings{wright2007language,
	Author = {Wright, Charles V and Ballard, Lucas and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {USENIX Security},
	Title = {{Language identification of encrypted VoIP traffic: Alejandra y Roberto or Alice and Bob?}},
	Year = {2007}}

@inproceedings{backes2010speaker,
	Author = {Backes, Michael and Doychev, Goran and D{\"u}rmuth, Markus and K{\"o}pf, Boris},
	Booktitle = {{European Symposium on Research in Computer Security (ESORICS)}},
	Pages = {508--523},
	Publisher = {Springer},
	Title = {{Speaker Recognition in Encrypted Voice Streams}},
	Year = {2010}}

@phdthesis{lu2009traffic,
	Author = {Lu, Yuanchao},
	School = {Cleveland State University},
	Title = {{On Traffic Analysis Attacks to Encrypted VoIP Calls}},
	Year = {2009}}

@inproceedings{wright2008spot,
	Author = {Wright, Charles V and Ballard, Lucas and Coull, Scott E and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {35--49},
	Title = {Spot me if you can: Uncovering spoken phrases in encrypted VoIP conversations},
	Year = {2008}}

@inproceedings{white2011phonotactic,
	Author = {White, Andrew M and Matthews, Austin R and Snow, Kevin Z and Monrose, Fabian},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {3--18},
	Title = {Phonotactic reconstruction of encrypted VoIP conversations: Hookt on fon-iks},
	Year = {2011}}

@inproceedings{fancy,
	Author = {Houmansadr, Amir and Borisov, Nikita},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {205--224},
	Title = {The Need for Flow Fingerprints to Link Correlated Network Flows},
	Year = {2013}}

@article{botmosaic,
	Author = {Amir Houmansadr and Nikita Borisov},
	Doi = {10.1016/j.jss.2012.11.005},
	Issn = {0164-1212},
	Journal = {Journal of Systems and Software},
	Keywords = {Network security},
	Number = {3},
	Pages = {707 - 715},
	Title = {BotMosaic: Collaborative network watermark for the detection of IRC-based botnets},
	Url = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Volume = {86},
	Year = {2013},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.jss.2012.11.005}}

@inproceedings{ramsbrock2008first,
	Author = {Ramsbrock, Daniel and Wang, Xinyuan and Jiang, Xuxian},
	Booktitle = {Recent Advances in Intrusion Detection},
	Organization = {Springer},
	Pages = {59--77},
	Title = {A first step towards live botmaster traceback},
	Year = {2008}}

@inproceedings{potdar2005survey,
	Author = {Potdar, Vidyasagar M and Han, Song and Chang, Elizabeth},
	Booktitle = {Industrial Informatics, 2005. INDIN'05. 2005 3rd IEEE International Conference on},
	Organization = {IEEE},
	Pages = {709--716},
	Title = {A survey of digital image watermarking techniques},
	Year = {2005}}

@book{cole2003hiding,
	Author = {Cole, Eric and Krutz, Ronald D},
	Publisher = {John Wiley \& Sons, Inc.},
	Title = {Hiding in plain sight: Steganography and the art of covert communication},
	Year = {2003}}

@incollection{akaike1998information,
	Author = {Akaike, Hirotogu},
	Booktitle = {Selected Papers of Hirotugu Akaike},
	Pages = {199--213},
	Publisher = {Springer},
	Title = {Information theory and an extension of the maximum likelihood principle},
	Year = {1998}}

@misc{central-command-hack,
	Author = {Everett Rosenfeld},
	Howpublished = {\url{http://www.cnbc.com/id/102330338}},
	Title = {{FBI investigating Central Command Twitter hack}},
	Year = {2015}}

@misc{sony-psp-ddos,
	Howpublished = {\url{http://n4g.com/news/1644853/sony-and-microsoft-cant-do-much-ddos-attacks-explained}},
	Key = {sony},
	Month = {December},
	Title = {{Sony and Microsoft cant do much -- DDoS attacks explained}},
	Year = {2014}}

@misc{sony-hack,
	Author = {David Bloom},
	Howpublished = {\url{http://goo.gl/MwR4A7}},
	Title = {{Online Game Networks Hacked, Sony Unit President Threatened}},
	Year = {2014}}

@misc{home-depot,
	Author = {Dune Lawrence},
	Howpublished = {\url{http://www.businessweek.com/articles/2014-09-02/home-depots-credit-card-breach-looks-just-like-the-target-hack}},
	Title = {{Home Depot's Suspected Breach Looks Just Like the Target Hack}},
	Year = {2014}}

@misc{target,
	Author = {Julio Ojeda-Zapata},
	Howpublished = {\url{http://www.mercurynews.com/business/ci_24765398/how-did-hackers-pull-off-target-data-heist}},
	Title = {{Target hack: How did they do it?}},
	Year = {2014}}


@article{probabilitycourse,
	Author = {H. Pishro-Nik},
	note = {\url{http://www.probabilitycourse.com}},
	Title = {Introduction to probability, statistics, and random processes},
    Year = {2014}}

@article{our-isit-location,
	Author = {Z. Montazeri and A. Houmansadr and H. Pishro-Nik},
	Journal = {To be submitted to IEEE ISIT},
	Title = {Location Privacy for Multi-State Networks},
	Year = {2016}}






@article{kafsi2013entropy,
	Author = {Kafsi, Mohamed and Grossglauser, Matthias and Thiran, Patrick},
	Journal = {Information Theory, IEEE Transactions on},
	Number = {9},
	Pages = {5577--5583},
	Publisher = {IEEE},
	Title = {The entropy of conditional Markov trajectories},
	Volume = {59},
	Year = {2013}}

@inproceedings{gruteser2003anonymous,
	Author = {Gruteser, Marco and Grunwald, Dirk},
	Booktitle = {Proceedings of the 1st international conference on Mobile systems, applications and services},
	Organization = {ACM},
	Pages = {31--42},
	Title = {Anonymous usage of location-based services through spatial and temporal cloaking},
	Year = {2003}}

@inproceedings{husted2010mobile,
	Author = {Husted, Nathaniel and Myers, Steven},
	Booktitle = {Proceedings of the 17th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {85--96},
	Title = {Mobile location tracking in metro areas: malnets and others},
	Year = {2010}}

@inproceedings{li2009tradeoff,
	Author = {Li, Tiancheng and Li, Ninghui},
	Booktitle = {Proceedings of the 15th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {517--526},
	Title = {On the tradeoff between privacy and utility in data publishing},
	Year = {2009}}





@incollection{humbert2010tracking,
	Author = {Humbert, Mathias and Manshaei, Mohammad Hossein and Freudiger, Julien and Hubaux, Jean-Pierre},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {38--57},
	Publisher = {Springer},
	Title = {Tracking games in mobile networks},
	Year = {2010}}


@article{palamidessi2006probabilistic,
	Author = {Palamidessi, Catuscia},
	Journal = {Electronic Notes in Theoretical Computer Science},
	Pages = {33--42},
	Publisher = {Elsevier},
	Title = {Probabilistic and nondeterministic aspects of anonymity},
	Volume = {155},
	Year = {2006}}



@inproceedings{freudiger2007mix,
	Author = {Freudiger, Julien and Raya, Maxim and F{\'e}legyh{\'a}zi, M{\'a}rk and Papadimitratos, Panos and Hubaux, Jean-Pierre},
	Booktitle = {CM Workshop on Wireless Networking for Intelligent Transportation Systems (WiN-ITS)},
	Title = {Mix-zones for location privacy in vehicular networks},
	Year = {2007}}



@inproceedings{niu2014achieving,
	Author = {Niu, Ben and Li, Qinghua and Zhu, Xiaoyan and Cao, Guohong and Li, Hui},
	Booktitle = {INFOCOM, 2014 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {754--762},
	Title = {Achieving k-anonymity in privacy-aware location-based services},
	Year = {2014}}



@inproceedings{kido2005protection,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Data Engineering Workshops, 2005. 21st International Conference on},
	Organization = {IEEE},
	Pages = {1248--1248},
	Title = {Protection of location privacy using dummies for location-based services},
	Year = {2005}}

@inproceedings{gedik2005location,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Booktitle = {Distributed Computing Systems, 2005. ICDCS 2005. Proceedings. 25th IEEE International Conference on},
	Organization = {IEEE},
	Pages = {620--629},
	Title = {Location privacy in mobile systems: A personalized anonymization model},
	Year = {2005}}


@incollection{duckham2005formal,
	Author = {Duckham, Matt and Kulik, Lars},
	Booktitle = {Pervasive computing},
	Pages = {152--170},
	Publisher = {Springer},
	Title = {A formal model of obfuscation and negotiation for location privacy},
	Year = {2005}}

@inproceedings{kido2005anonymous,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Pervasive Services, 2005. ICPS'05. Proceedings. International Conference on},
	Organization = {IEEE},
	Pages = {88--97},
	Title = {An anonymous communication technique using dummies for location-based services},
	Year = {2005}}

@incollection{duckham2006spatiotemporal,
	Author = {Duckham, Matt and Kulik, Lars and Birtley, Athol},
	Booktitle = {Geographic Information Science},
	Pages = {47--64},
	Publisher = {Springer},
	Title = {A spatiotemporal model of strategies and counter strategies for location privacy protection},
	Year = {2006}}

@inproceedings{shankar2009privately,
	Author = {Shankar, Pravin and Ganapathy, Vinod and Iftode, Liviu},
	Booktitle = {Proceedings of the 11th international conference on Ubiquitous computing},
	Organization = {ACM},
	Pages = {31--40},
	Title = {Privately querying location-based services with SybilQuery},
	Year = {2009}}

@inproceedings{chow2009faking,
	Author = {Chow, Richard and Golle, Philippe},
	Booktitle = {Proceedings of the 8th ACM workshop on Privacy in the electronic society},
	Organization = {ACM},
	Pages = {105--108},
	Title = {Faking contextual data for fun, profit, and privacy},
	Year = {2009}}

@incollection{xue2009location,
	Author = {Xue, Mingqiang and Kalnis, Panos and Pung, Hung Keng},
	Booktitle = {Location and Context Awareness},
	Pages = {70--87},
	Publisher = {Springer},
	Title = {Location diversity: Enhanced privacy protection in location based services},
	Year = {2009}}

@article{wernke2014classification,
	Author = {Wernke, Marius and Skvortsov, Pavel and D{\"u}rr, Frank and Rothermel, Kurt},
	Journal = {Personal and Ubiquitous Computing},
	Number = {1},
	Pages = {163--175},
	Publisher = {Springer-Verlag},
	Title = {A classification of location privacy attacks and approaches},
	Volume = {18},
	Year = {2014}}

@misc{cai2015cloaking,
	Author = {Cai, Y. and Xu, G.},
	Month = jan # {~1},
	Note = {US Patent App. 14/472,462},
	Publisher = {Google Patents},
	Title = {Cloaking with footprints to provide location privacy protection in location-based services},
	Url = {https://www.google.com/patents/US20150007341},
	Year = {2015},
	Bdsk-Url-1 = {https://www.google.com/patents/US20150007341}}

@article{gedik2008protecting,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {1},
	Pages = {1--18},
	Publisher = {IEEE},
	Title = {Protecting location privacy with personalized k-anonymity: Architecture and algorithms},
	Volume = {7},
	Year = {2008}}

@article{kalnis2006preserving,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Publisher = {TRB6/06},
	Title = {Preserving anonymity in location based services},
	Year = {2006}}



@article{terrovitis2011privacy,
	Author = {Terrovitis, Manolis},
	Journal = {ACM SIGKDD Explorations Newsletter},
	Number = {1},
	Pages = {6--18},
	Publisher = {ACM},
	Title = {Privacy preservation in the dissemination of location data},
	Volume = {13},
	Year = {2011}}

@article{shin2012privacy,
	Author = {Shin, Kang G and Ju, Xiaoen and Chen, Zhigang and Hu, Xin},
	Journal = {Wireless Communications, IEEE},
	Number = {1},
	Pages = {30--39},
	Publisher = {IEEE},
	Title = {Privacy protection for users of location-based services},
	Volume = {19},
	Year = {2012}}



@incollection{chatzikokolakis2015geo,
	Author = {Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
	Booktitle = {Distributed Computing and Internet Technology},
	Pages = {49--72},
	Publisher = {Springer},
	Title = {Geo-indistinguishability: A Principled Approach to Location Privacy},
	Year = {2015}}

@inproceedings{ngo2015location,
	Author = {Ngo, Hoa and Kim, Jong},
	Booktitle = {Computer Security Foundations Symposium (CSF), 2015 IEEE 28th},
	Organization = {IEEE},
	Pages = {63--74},
	Title = {Location Privacy via Differential Private Perturbation of Cloaking Area},
	Year = {2015}}


@inproceedings{um2010advanced,
	Author = {Um, Jung-Ho and Kim, Hee-Dae and Chang, Jae-Woo},
	Booktitle = {Social Computing (SocialCom), 2010 IEEE Second International Conference on},
	Organization = {IEEE},
	Pages = {1093--1098},
	Title = {An advanced cloaking algorithm using Hilbert curves for anonymous location based service},
	Year = {2010}}

@inproceedings{bamba2008supporting,
	Author = {Bamba, Bhuvan and Liu, Ling and Pesti, Peter and Wang, Ting},
	Booktitle = {Proceedings of the 17th international conference on World Wide Web},
	Organization = {ACM},
	Pages = {237--246},
	Title = {Supporting anonymous location queries in mobile environments with privacygrid},
	Year = {2008}}

@inproceedings{zhangwei2010distributed,
	Author = {Zhangwei, Huang and Mingjun, Xin},
	Booktitle = {Networks Security Wireless Communications and Trusted Computing (NSWCTC), 2010 Second International Conference on},
	Organization = {IEEE},
	Pages = {468--471},
	Title = {A distributed spatial cloaking protocol for location privacy},
	Volume = {2},
	Year = {2010}}

@article{chow2011spatial,
	Author = {Chow, Chi-Yin and Mokbel, Mohamed F and Liu, Xuan},
	Journal = {GeoInformatica},
	Number = {2},
	Pages = {351--380},
	Publisher = {Springer},
	Title = {Spatial cloaking for anonymous location-based services in mobile peer-to-peer environments},
	Volume = {15},
	Year = {2011}}

@inproceedings{lu2008pad,
	Author = {Lu, Hua and Jensen, Christian S and Yiu, Man Lung},
	Booktitle = {Proceedings of the Seventh ACM International Workshop on Data Engineering for Wireless and Mobile Access},
	Organization = {ACM},
	Pages = {16--23},
	Title = {Pad: privacy-area aware, dummy-based location privacy in mobile services},
	Year = {2008}}

@incollection{khoshgozaran2007blind,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus},
	Booktitle = {Advances in Spatial and Temporal Databases},
	Pages = {239--257},
	Publisher = {Springer},
	Title = {Blind evaluation of nearest neighbor queries using space transformation to preserve location privacy},
	Year = {2007}}

@inproceedings{ghinita2008private,
	Author = {Ghinita, Gabriel and Kalnis, Panos and Khoshgozaran, Ali and Shahabi, Cyrus and Tan, Kian-Lee},
	Booktitle = {Proceedings of the 2008 ACM SIGMOD international conference on Management of data},
	Organization = {ACM},
	Pages = {121--132},
	Title = {Private queries in location based services: anonymizers are not necessary},
	Year = {2008}}



@article{nguyen2013differential,
	Author = {Nguyen, Hiep H and Kim, Jong and Kim, Yoonho},
	Journal = {Journal of Computing Science and Engineering},
	Number = {3},
	Pages = {177--186},
	Title = {Differential privacy in practice},
	Volume = {7},
	Year = {2013}}

@inproceedings{lee2012differential,
	Author = {Lee, Jaewoo and Clifton, Chris},
	Booktitle = {Proceedings of the 18th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {1041--1049},
	Title = {Differential identifiability},
	Year = {2012}}

@inproceedings{andres2013geo,
	Author = {Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2013 ACM SIGSAC conference on Computer \& communications security},
	Organization = {ACM},
	Pages = {901--914},
	Title = {Geo-indistinguishability: Differential privacy for location-based systems},
	Year = {2013}}

@inproceedings{machanavajjhala2008privacy,
	Author = {Machanavajjhala, Ashwin and Kifer, Daniel and Abowd, John and Gehrke, Johannes and Vilhuber, Lars},
	Booktitle = {Data Engineering, 2008. ICDE 2008. IEEE 24th International Conference on},
	Organization = {IEEE},
	Pages = {277--286},
	Title = {Privacy: Theory meets practice on the map},
	Year = {2008}}

@article{dewri2013local,
	Author = {Dewri, Rinku},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {12},
	Pages = {2360--2372},
	Publisher = {IEEE},
	Title = {Local differential perturbations: Location privacy under approximate knowledge attackers},
	Volume = {12},
	Year = {2013}}

@inproceedings{chatzikokolakis2013broadening,
	Author = {Chatzikokolakis, Konstantinos and Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s Emilio and Palamidessi, Catuscia},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {82--102},
	Title = {Broadening the Scope of Differential Privacy Using Metrics.},
	Year = {2013}}



@inproceedings{cheng2006preserving,
	Author = {Cheng, Reynold and Zhang, Yu and Bertino, Elisa and Prabhakar, Sunil},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {393--412},
	Title = {Preserving user location privacy in mobile data management infrastructures},
	Year = {2006}}




@article{krumm2009survey,
	Author = {Krumm, John},
	Journal = {Personal and Ubiquitous Computing},
	Number = {6},
	Pages = {391--399},
	Publisher = {Springer},
	Title = {A survey of computational location privacy},
	Volume = {13},
	Year = {2009}}

@article{Rakhshan2015letter,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Wireless Communications Letter},
	Publisher = {IEEE},
	Title = {A Stochastic Geometry Model for Customized Vehicular Communication},
	Year = {2015, submitted}}

@article{Rakhshan2015Journal,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Publisher = {IEEE},
	Title = {Improving Safety on Highways by Customizing Vehicular Ad Hoc Networks},
	Year = {2015, submitted}}

@inproceedings{Rakhshan2015Cogsima,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Booktitle = {IEEE International Multi-Disciplinary Conference on Cognitive Methods in Situation Awareness and Decision Support},
	Organization = {IEEE},
	Title = {A New Approach to Customization of Accident Warning Systems to Individual Drivers},
	Year = {2015}}

@inproceedings{Rakhshan2015CISS,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Nekoui, Mohammad},
	Booktitle = {Conference on Information Sciences and Systems},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {Driver-based adaptation of Vehicular Ad Hoc Networks for design of active safety systems},
	Year = {2015}}

@inproceedings{Rakhshan2014IV,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Ray, Evan},
	Booktitle = {Intelligent Vehicles Symposium},
	Organization = {IEEE},
	Pages = {1181--1186},
	Title = {Real-time estimation of the distribution of brake response times for an individual driver using Vehicular Ad Hoc Network.},
	Year = {2014}}

@inproceedings{Rakhshan2013Globecom,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Fisher, Donald and Nekoui, Mohammad},
	Booktitle = {IEEE Global Communications Conference},
	Organization = {IEEE},
	Pages = {1333--1337},
	Title = {Tuning collision warning algorithms to individual drivers for design of active safety systems.},
	Year = {2013}}

@article{Nekoui2012Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Number = {8},
	Pages = {2895--2905},
	Publisher = {IEEE},
	Title = {Throughput Scaling laws for Vehicular Ad Hoc Networks},
	Volume = {11},
	Year = {2012}}

@article{Nekoui2013Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {Journal on Selected Areas in Communications, Special Issue on Emerging Technologies in Communications},
	Number = {9},
	Pages = {491--503},
	Publisher = {IEEE},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {31},
	Year = {2013}}

@article{Nekoui2011Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein and Ni, Daiheng},
	Journal = {International Journal of Vehicular Technology},
	Pages = {1--11},
	Publisher = {Hindawi Publishing Corporation},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {2011},
	Year = {2011}}

@inproceedings{Nekoui2011MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM workshop on VehiculAr InterNETworking},
	Organization = {ACM},
	Title = {Analytic Design of Active Vehicular Safety Systems in Sparse Traffic},
	Year = {2011}}

@inproceedings{Nekoui2011VTC,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Analytical Design of Inter-vehicular Communications for Collision Avoidance},
	Year = {2011}}

@inproceedings{Bovee2011VTC,
	Author = {Bovee, Ben Louis and Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Evaluation of the Universal Geocast Scheme For VANETs},
	Year = {2011}}

@inproceedings{Nekoui2010MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM},
	Organization = {ACM},
	Title = {Fundamental Tradeoffs in Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2010IVCS,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IVCS},
	Organization = {IEEE},
	Title = {A Universal Geocast Scheme for Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2009ITW,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IEEE Communications Society Conference on Sensor, Mesh and Ad Hoc Communications and Networks Workshops},
	Organization = {IEEE},
	Pages = {1--3},
	Title = {A Geometrical Analysis of Obstructed Wireless Networks},
	Year = {2009}}

@article{Eslami2013Journal,
	Author = {Eslami, Ali and Nekoui, Mohammad and Pishro-Nik, Hossein and Fekri, Faramarz},
	Journal = {ACM Transactions on Sensor Networks},
	Number = {4},
	Pages = {51},
	Publisher = {ACM},
	Title = {Results on finite wireless sensor networks: Connectivity and coverage},
	Volume = {9},
	Year = {2013}}

@article{shokri2014optimal,
	  title={Optimal user-centric data obfuscation},
 	 author={Shokri, Reza},
 	 journal={arXiv preprint arXiv:1402.3426},
 	 year={2014}
	}
@article{chatzikokolakis2015location,
  title={Location privacy via geo-indistinguishability},
  author={Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
  journal={ACM SIGLOG News},
  volume={2},
  number={3},
  pages={46--69},
  year={2015},
  publisher={ACM}

}
@inproceedings{shokri2011quantifying2,
  title={Quantifying location privacy: the case of sporadic location exposure},
  author={Shokri, Reza and Theodorakopoulos, George and Danezis, George and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
  booktitle={Privacy Enhancing Technologies},
  pages={57--76},
  year={2011},
  organization={Springer}
}

@inproceedings{calmon2015fundamental,
  title={Fundamental limits of perfect privacy},
  author={Calmon, Flavio P and Makhdoumi, Ali and M{\'e}dard, Muriel},
  booktitle={Information Theory (ISIT), 2015 IEEE International Symposium on},
  pages={1796--1800},
  year={2015},
  organization={IEEE}
}

@inproceedings{salamatian2013hide,
  title={How to hide the elephant-or the donkey-in the room: Practical privacy against statistical inference for large data.},
  author={Salamatian, Salman and Zhang, Amy and du Pin Calmon, Flavio and Bhamidipati, Sandilya and Fawaz, Nadia and Kveton, Branislav and Oliveira, Pedro and Taft, Nina},
  booktitle={GlobalSIP},
  pages={269--272},
  year={2013}
}

@article{sankar2013utility,
  title={Utility-privacy tradeoffs in databases: An information-theoretic approach},
  author={Sankar, Lalitha and Rajagopalan, S Raj and Poor, H Vincent},
  journal={Information Forensics and Security, IEEE Transactions on},
  volume={8},
  number={6},
  pages={838--852},
  year={2013},
  publisher={IEEE}
}
@inproceedings{ghinita2007prive,
  title={PRIVE: anonymous location-based queries in distributed mobile systems},
  author={Ghinita, Gabriel and Kalnis, Panos and Skiadopoulos, Spiros},
  booktitle={Proceedings of the 16th international conference on World Wide Web},
  pages={371--380},
  year={2007},
  organization={ACM}
}

@article{beresford2004mix,
  title={Mix zones: User privacy in location-aware services},
  author={Beresford, Alastair R and Stajano, Frank},
  year={2004},
  publisher={IEEE}
}


@article{csiszar1996almost,
  title={Almost independence and secrecy capacity},
  author={Csisz{\'a}r, Imre},
  journal={Problemy Peredachi Informatsii},
  volume={32},
  number={1},
  pages={48--57},
  year={1996},
  publisher={Russian Academy of Sciences, Branch of Informatics, Computer Equipment and Automatization}
}

@article{yamamoto1983source,
  title={A source coding problem for sources with additional outputs to keep secret from the receiver or wiretappers (corresp.)},
  author={Yamamoto, Hirosuke},
  journal={IEEE Transactions on Information Theory},
  volume={29},
  number={6},
  pages={918--923},
  year={1983},
  publisher={IEEE}
}



  @inproceedings{golle2009anonymity,
  title={On the anonymity of home/work location pairs},
  author={Golle, Philippe and Partridge, Kurt},
  booktitle={International Conference on Pervasive Computing},
  pages={390--397},
  year={2009},
  organization={Springer}
}

@inproceedings{zang2011anonymization,
  title={Anonymization of location data does not work: A large-scale measurement study},
  author={Zang, Hui and Bolot, Jean},
  booktitle={Proceedings of the 17th annual international conference on Mobile computing and networking},
  pages={145--156},
  year={2011},
  organization={ACM}
}
@article{wang2015privacy,
  title={Privacy-preserving collaborative spectrum sensing with multiple service providers},
  author={Wang, Wei and Zhang, Qian},
  journal={IEEE Transactions on Wireless Communications},
  volume={14},
  number={2},
  pages={1011--1019},
  year={2015},
  publisher={IEEE}
}

@article{wang2015toward,
  title={Toward long-term quality of protection in mobile networks: a context-aware perspective},
  author={Wang, Wei and Zhang, Qian},
  journal={IEEE Wireless Communications},
  volume={22},
  number={4},
  pages={34--40},
  year={2015},
  publisher={IEEE}
}

@inproceedings{niu2015enhancing,
  title={Enhancing privacy through caching in location-based services},
  author={Niu, Ben and Li, Qinghua and Zhu, Xiaoyan and Cao, Guohong and Li, Hui},
  booktitle={2015 IEEE Conference on Computer Communications (INFOCOM)},
  pages={1017--1025},
  year={2015},
  organization={IEEE}
}

%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Created for Zarrin Montazeri at 2015-11-09 18:45:31 -0500


%% Saved with string encoding Unicode (UTF-8)



%%%%%%%%%%%%%%IOT%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@article{osma2015,
	title={Impact of Time-to-Collision Information on Driving Behavior in Connected Vehicle Environments Using A Driving Simulator Test Bed},
	journal{Journal of Traffic and Logistics Engineering},
	author={Osama A. Osman, Julius Codjoe, and Sherif Ishak},
	volume={3},
	number={1},
	pages={18--24},
	year={2015}
}


@article{charisma2010,
	title={Dynamic Latent Plan Models},
	author={Charisma F. Choudhurya, Moshe Ben-Akivab and Maya Abou-Zeid},
	journal={Journal of Choice Modelling},
	volume={3},
	number={2},
	pages={50--70},
	year={2010},
	publisher={Elsvier}
}


@misc{noble2014,
	author = {A. M. Noble, Shane B. McLaughlin, Zachary R. Doerzaph and Thomas A. Dingus},
	title = {Crowd-sourced Connected-vehicle Warning Algorithm using Naturalistic Driving Data},
	howpublished = {Downloaded from \url{http://hdl.handle.net/10919/53978}},
	
	month = August,
	year = 2014
}


@phdthesis{charisma2007,
	title    = {Modeling Driving Decisions with Latent Plans},
	school   = {Massachusetts Institute of Technology },
	author   = {Charisma Farheen Choudhury},
	year     = {2007}, %other attributes omitted
}


@article{chrysler2015,
	title={Cost of Warning of Unseen Threats:Unintended Consequences of Connected Vehicle Alerts},
	author={S. T. Chrysler, J. M. Cooper and D. C. Marshall},
	journal={Transportation Research Record: Journal of the Transportation Research Board},
	volume={2518},
	pages={79--85},
	year={2015},
}





@article{FTC2015,
	title={Internet of Things: Privacy and Security in a Connected World},
	author={FTC Staff Report},
	year={2015}
}



%% Saved with string encoding Unicode (UTF-8)
@inproceedings{1zhou2014security,
	title={Security/privacy of wearable fitness tracking {I}o{T} devices},
	author={Zhou, Wei and Piramuthu, Selwyn},
	booktitle={Information Systems and Technologies (CISTI), 2014 9th Iberian Conference on},
	pages={1--5},
	year={2014},
	organization={IEEE}
}


@inproceedings{3ukil2014iot,
	title={{I}o{T}-privacy: To be private or not to be private},
	author={Arijit Ukil and Soma Bandyopadhyay and Arpan Pal},
	booktitle={Computer Communications Workshops (INFOCOM WKSHPS), IEEE Conference on},
	pages={123--124},
	year={2014},
	organization={IEEE}
}

@inproceedings{4Hosseinzadeh2014,
	title={Security in the Internet of Things through obfuscation and diversification},
	author={Hosseinzadeh, Shohreh and Rauti, Sampsa and Hyrynsalmi, Sami and Leppanen, Ville},
	booktitle={Computing, Communication and Security (ICCCS), IEEE Conference on},
	pages={123--124},
	year={2015},
	organization={IEEE}
}
@article{4arias2015privacy,
	title={Privacy and security in internet of things and wearable devices},
	author={Arias, Orlando and Wurm, Jacob and Hoang, Khoa and Jin, Yier},
	journal={IEEE Transactions on Multi-Scale Computing Systems},
	volume={1},
	number={2},
	pages={99--109},
	year={2015},
	publisher={IEEE}
}
@inproceedings{5ullah2016novel,
	title={A novel model for preserving Location Privacy in Internet of Things},
	author={Ullah, Ikram and Shah, Munam Ali},
	booktitle={Automation and Computing (ICAC), 2016 22nd International Conference on},
	pages={542--547},
	year={2016},
	organization={IEEE}
}
@inproceedings{6sathishkumar2016enhanced,
	title={Enhanced location privacy algorithm for wireless sensor network in Internet of Things},
	author={Sathishkumar, J and Patel, Dhiren R},
	booktitle={Internet of Things and Applications (IOTA), International Conference on},
	pages={208--212},
	year={2016},
	organization={IEEE}
}
@inproceedings{7zhou2012preserving,
	title={Preserving sensor location privacy in internet of things},
	author={Zhou, Liming and Wen, Qiaoyan and Zhang, Hua},
	booktitle={Computational and Information Sciences (ICCIS), 2012 Fourth International Conference on},
	pages={856--859},
	year={2012},
	organization={IEEE}
}

@inproceedings{8ukil2015privacy,
	title={Privacy for {I}o{T}: Involuntary privacy enablement for smart energy systems},
	author={Ukil, Arijit and Bandyopadhyay, Soma and Pal, Arpan},
	booktitle={Communications (ICC), 2015 IEEE International Conference on},
	pages={536--541},
	year={2015},
	organization={IEEE}
}

@inproceedings{9dalipi2016security,
	title={Security and Privacy Considerations for {I}o{T} Application on Smart Grids: Survey and Research Challenges},
	author={Dalipi, Fisnik and Yayilgan, Sule Yildirim},
	booktitle={Future Internet of Things and Cloud Workshops (FiCloudW), IEEE International Conference on},
	pages={63--68},
	year={2016},
	organization={IEEE}
}
@inproceedings{10harris2016security,
	title={Security and Privacy in Public {I}o{T} Spaces},
	author={Harris, Albert F and Sundaram, Hari and Kravets, Robin},
	booktitle={Computer Communication and Networks (ICCCN), 2016 25th International Conference on},
	pages={1--8},
	year={2016},
	organization={IEEE}
}

@inproceedings{11al2015security,
	title={Security and privacy framework for ubiquitous healthcare {I}o{T} devices},
	author={Al Alkeem, Ebrahim and Yeun, Chan Yeob and Zemerly, M Jamal},
	booktitle={Internet Technology and Secured Transactions (ICITST), 2015 10th International Conference for},
	pages={70--75},
	year={2015},
	organization={IEEE}
}
@inproceedings{12sivaraman2015network,
	title={Network-level security and privacy control for smart-home {I}o{T} devices},
	author={Sivaraman, Vijay and Gharakheili, Hassan Habibi and Vishwanath, Arun and Boreli, Roksana and Mehani, Olivier},
	booktitle={Wireless and Mobile Computing, Networking and Communications (WiMob), 2015 IEEE 11th International Conference on},
	pages={163--167},
	year={2015},
	organization={IEEE}
}

@inproceedings{13srinivasan2016privacy,
	title={Privacy conscious architecture for improving emergency response in smart cities},
	author={Srinivasan, Ramya and Mohan, Apurva and Srinivasan, Priyanka},
	booktitle={Smart City Security and Privacy Workshop (SCSP-W), 2016},
	pages={1--5},
	year={2016},
	organization={IEEE}
}
@inproceedings{14sadeghi2015security,
	title={Security and privacy challenges in industrial internet of things},
	author={Sadeghi, Ahmad-Reza and Wachsmann, Christian and Waidner, Michael},
	booktitle={Design Automation Conference (DAC), 2015 52nd ACM/EDAC/IEEE},
	pages={1--6},
	year={2015},
	organization={IEEE}
}
@inproceedings{15otgonbayar2016toward,
	title={Toward Anonymizing {I}o{T} Data Streams via Partitioning},
	author={Otgonbayar, Ankhbayar and Pervez, Zeeshan and Dahal, Keshav},
	booktitle={Mobile Ad Hoc and Sensor Systems (MASS), 2016 IEEE 13th International Conference on},
	pages={331--336},
	year={2016},
	organization={IEEE}
}
@inproceedings{16rutledge2016privacy,
	title={Privacy Impacts of {I}o{T} Devices: A SmartTV Case Study},
	author={Rutledge, Richard L and Massey, Aaron K and Ant{\'o}n, Annie I},
	booktitle={Requirements Engineering Conference Workshops (REW), IEEE International},
	pages={261--270},
	year={2016},
	organization={IEEE}
}

@inproceedings{17andrea2015internet,
	title={Internet of Things: Security vulnerabilities and challenges},
	author={Andrea, Ioannis and Chrysostomou, Chrysostomos and Hadjichristofi, George},
	booktitle={Computers and Communication (ISCC), 2015 IEEE Symposium on},
	pages={180--187},
	year={2015},
	organization={IEEE}
}






























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@misc{epfl-mobility-20090224,
	author = {Michal Piorkowski and Natasa Sarafijanovic-Djukic and Matthias Grossglauser},
	title = {{CRAWDAD} dataset epfl/mobility (v. 2009-02-24)},
	howpublished = {Downloaded from \url{http://crawdad.org/epfl/mobility/20090224}},
	doi = {10.15783/C7J010},
	month = feb,
	year = 2009
}

@misc{roma-taxi-20140717,
	author = {Lorenzo Bracciale and Marco Bonola and Pierpaolo Loreti and Giuseppe Bianchi and Raul Amici and Antonello Rabuffi},
	title = {{CRAWDAD} dataset roma/taxi (v. 2014-07-17)},
	howpublished = {Downloaded from \url{http://crawdad.org/roma/taxi/20140717}},
	doi = {10.15783/C7QC7M},
	month = jul,
	year = 2014
}

@misc{rice-ad_hoc_city-20030911,
	author = {Jorjeta G. Jetcheva and Yih-Chun Hu and Santashil PalChaudhuri and Amit Kumar Saha and David B. Johnson},
	title = {{CRAWDAD} dataset rice/ad\_hoc\_city (v. 2003-09-11)},
	howpublished = {Downloaded from \url{http://crawdad.org/rice/ad_hoc_city/20030911}},
	doi = {10.15783/C73K5B},
	month = sep,
	year = 2003
}

@misc{china:2012,
	author = {Microsoft Research Asia},
	title = {GeoLife GPS Trajectories},
	year = {2012},
	howpublished= {\url{https://www.microsoft.com/en-us/download/details.aspx?id=52367}},
}


@misc{china:2011,
	ALTauthor = {Microsoft Research Asia)},
	ALTeditor = {},
	title = {GeoLife GPS Trajectories,
	year = {2012},
	url = {https://www.microsoft.com/en-us/download/details.aspx?id=52367},
	}
	
	
	@misc{longversion,
	author = {N. Takbiri and A. Houmansadr and D.L. Goeckel and H. Pishro-Nik},
	title = {{Limits of Location Privacy under Anonymization and Obfuscation}},
	howpublished = "\url{https://dl.dropboxusercontent.com/u/49263048/ISIT_2017-2.pdf}",
	year = 2017,
	month= "January",
	note = "[Online; accessed 22-Jan-2017]"
	}
	
	
	
	@article{matching,
	title={Asymptotically Optimal Matching of Multiple Sequences to Source Distributions and Training Sequences},
	author={Jayakrishnan Unnikrishnan},
	journal={ IEEE Transactions on Information Theory},
	volume={61},
	number={1},
	pages={452-468},
	year={2015},
	publisher={IEEE}
	}
	
	
	@article{Naini2016,
	Author = {F. Naini and J. Unnikrishnan and P. Thiran and M. Vetterli},
	Journal = {IEEE Transactions on Information Forensics and Security},
	Publisher = {IEEE},
	Title = {Where You Are Is Who You Are: User Identification by Matching Statistics},
	volume={11},
	number={2},
	pages={358--372},
	Year = {2016}
	}
	
	
	
	@inproceedings{holowczak2015cachebrowser,
	title={{CacheBrowser: Bypassing Chinese Censorship without Proxies Using Cached Content}},
	author={Holowczak, John and Houmansadr, Amir},
	booktitle={Proceedings of the 22nd ACM SIGSAC Conference on Computer and Communications Security},
	pages={70--83},
	year={2015},
	organization={ACM}
	}
	@misc{cb-website,
	Howpublished = {\url{https://cachebrowser.net/#/}},
	Title = {{CacheBrowser}},
	key={cachebrowser}
	}
	
	@inproceedings{GameOfDecoys,
	title={{GAME OF DECOYS: Optimal Decoy Routing Through Game Theory}},
	author={Milad Nasr and Amir Houmansadr},
	booktitle={The $23^{rd}$ ACM Conference on Computer and Communications Security (CCS)},
	year={2016}
	}
	
	@inproceedings{CDNReaper,
	title={{Practical Censorship Evasion Leveraging Content Delivery Networks}},
	author={Hadi Zolfaghari and Amir Houmansadr},
	booktitle={The $23^{rd}$ ACM Conference on Computer and Communications Security (CCS)},
	year={2016}
	}
	
	@misc{Leberknight2010,
	Author = {Leberknight, C. and Chiang, M. and Poor, H. and Wong, F.},
	Howpublished = {\url{http://www.princeton.edu/~chiangm/anticensorship.pdf}},
	Title = {{A Taxonomy of Internet Censorship and Anti-censorship}},
	Year = {2010}}
	
	@techreport{ultrasurf-analysis,
	Author = {Appelbaum, Jacob},
	Institution = {The Tor Project},
	Title = {{Technical analysis of the Ultrasurf proxying software}},
	Url = {http://scholar.google.com/scholar?hl=en\&btnG=Search\&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software\#0},
	Year = {2012},
	Bdsk-Url-1 = {http://scholar.google.com/scholar?hl=en%5C&btnG=Search%5C&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software%5C#0}}
	
	@misc{gifc:07,
	Howpublished = {\url{http://www.internetfreedom.org/archive/Defeat\_Internet\_Censorship\_White\_Paper.pdf}},
	Key = {defeatcensorship},
	Publisher = {Global Internet Freedom Consortium (GIFC)},
	Title = {{Defeat Internet Censorship: Overview of Advanced Technologies and Products}},
	Type = {White Paper},
	Year = {2007}}
	
	@article{pan2011survey,
	Author = {Pan, J. and Paul, S. and Jain, R.},
	Journal = {Communications Magazine, IEEE},
	Number = {7},
	Pages = {26--36},
	Publisher = {IEEE},
	Title = {{A Survey of the Research on Future Internet Architectures}},
	Volume = {49},
	Year = {2011}}
	
	@misc{nsf-fia,
	Howpublished = {\url{http://www.nets-fia.net/}},
	Key = {FIA},
	Title = {{NSF Future Internet Architecture Project}}}
	
	@misc{NDN,
	Howpublished = {\url{http://www.named- data.net}},
	Key = {NDN},
	Title = {{Named Data Networking Project}}}
	
	@inproceedings{MobilityFirst,
	Author = {Seskar, I. and Nagaraja, K. and Nelson, S. and Raychaudhuri, D.},
	Booktitle = {Asian Internet Engineering Conference},
	Title = {{Mobilityfirst Future internet Architecture Project}},
	Year = {2011}}
	
	@incollection{NEBULA,
	Author = {Anderson, T. and Birman, K. and Broberg, R. and Caesar, M. and Comer, D. and Cotton, C. and Freedman, M.~J. and Haeberlen, A. and Ives, Z.~G. and Krishnamurthy, A. and others},
	Booktitle = {The Future Internet},
	Pages = {16--26},
	Publisher = {Springer},
	Title = {{The NEBULA Future Internet Architecture}},
	Year = {2013}}
	
	@inproceedings{XIA,
	Author = {Anand, A. and Dogar, F. and Han, D. and Li, B. and Lim, H. and Machado, M. and Wu, W. and Akella, A. and Andersen, D.~G. and Byers, J.~W. and others},
	Booktitle = {ACM Workshop on Hot Topics in Networks},
	Pages = {2},
	Title = {{XIA: An Architecture for an Evolvable and Trustworthy Internet}},
	Year = {2011}}
	
	@inproceedings{ChoiceNet,
	Author = {Rouskas, G.~N. and Baldine, I. and Calvert, K.~L. and Dutta, R. and Griffioen, J. and Nagurney, A. and Wolf, T.},
	Booktitle = {ONDM},
	Title = {{ChoiceNet: Network Innovation Through Choice}},
	Year = {2013}}
	
	@misc{nsf-find,
	Howpublished = {http://www.nets-find.net/},
	Title = {{NSF NeTS FIND Initiative}}}
	
	@article{traid,
	Author = {Cheriton, D.~R. and Gritter, M.},
	Title = {{TRIAD: A New Next-Generation Internet Architecture}},
	Year = {2000}}
	
	@inproceedings{dona,
	Author = {Koponen, T. and Chawla, M. and Chun, B-G. and Ermolinskiy, A. and Kim, K.~H. and Shenker, S. and Stoica, I.},
	Booktitle = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Organization = {ACM},
	Pages = {181--192},
	Title = {{A Data-Oriented (and Beyond) Network Architecture}},
	Volume = {37},
	Year = {2007}}
	
	@misc{ultrasurf,
	Howpublished = {\url{http://www.ultrareach.com}},
	Key = {ultrasurf},
	Title = {{Ultrasurf}}}
	
	@misc{tor-bridge,
	Author = {Dingledine, R. and Mathewson, N.},
	Howpublished = {\url{https://svn.torproject.org/svn/projects/design-paper/blocking.html}},
	Title = {{Design of a Blocking-Resistant Anonymity System}}}
	
	@inproceedings{McLachlanH09,
	Author = {J. McLachlan and N. Hopper},
	Booktitle = {WPES},
	Title = {{On the Risks of Serving Whenever You Surf: Vulnerabilities in Tor's Blocking Resistance Design}},
	Year = {2009}}
	
	@inproceedings{mahdian2010,
	Author = {Mahdian, M.},
	Booktitle = {{Fun with Algorithms}},
	Title = {{Fighting Censorship with Algorithms}},
	Year = {2010}}
	
	@inproceedings{McCoy2011,
	Author = {McCoy, D. and Morales, J.~A. and Levchenko, K.},
	Booktitle = {FC},
	Title = {{Proximax: A Measurement Based System for Proxies Dissemination}},
	Year = {2011}}
	
	@inproceedings{Sovran2008,
	Author = {Sovran, Y. and Libonati, A. and Li, J.},
	Booktitle = {IPTPS},
	Title = {{Pass it on: Social Networks Stymie Censors}},
	Year = {2008}}
	
	@inproceedings{rbridge,
	Author = {Wang, Q. and Lin, Zi and Borisov, N. and Hopper, N.},
	Booktitle = {{NDSS}},
	Title = {{rBridge: User Reputation based Tor Bridge Distribution with Privacy Preservation}},
	Year = {2013}}
	
	@inproceedings{telex,
	Author = {Wustrow, E. and Wolchok, S. and Goldberg, I. and Halderman, J.},
	Booktitle = {{USENIX Security}},
	Title = {{Telex: Anticensorship in the Network Infrastructure}},
	Year = {2011}}
	
	@inproceedings{cirripede,
	Author = {Houmansadr, A. and Nguyen, G. and Caesar, M. and Borisov, N.},
	Booktitle = {CCS},
	Title = {{Cirripede: Circumvention Infrastructure Using Router Redirection with Plausible Deniability}},
	Year = {2011}}
	
	@inproceedings{decoyrouting,
	Author = {Karlin, J. and Ellard, D. and Jackson, A. and Jones, C. and Lauer, G. and Mankins, D. and Strayer, W.},
	Booktitle = {{FOCI}},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = {2011}}
	
	@inproceedings{routing-around-decoys,
	Author = {M.~Schuchard and J.~Geddes and C.~Thompson and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Routing Around Decoys}},
	Year = {2012}}
	
	@inproceedings{parrot,
	Author = {A. Houmansadr and C. Brubaker and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{The Parrot is Dead: Observing Unobservable Network Communications}},
	Year = {2013}}
	
	@misc{knock,
	Author = {T. Wilde},
	Howpublished = {\url{https://blog.torproject.org/blog/knock-knock-knockin-bridges-doors}},
	Title = {{Knock Knock Knockin' on Bridges' Doors}},
	Year = {2012}}
	
	@inproceedings{china-tor,
	Author = {Winter, P. and Lindskog, S.},
	Booktitle = {{FOCI}},
	Title = {{How the Great Firewall of China Is Blocking Tor}},
	Year = {2012}}
	
	@misc{discover-bridge,
	Howpublished = {\url{https://blog.torproject.org/blog/research-problems-ten-ways-discover-tor-bridges}},
	Key = {tenways},
	Title = {{Ten Ways to Discover Tor Bridges}}}
	
	@inproceedings{freewave,
	Author = {A.~Houmansadr and T.~Riedl and N.~Borisov and A.~Singer},
	Booktitle = {{NDSS}},
	Title = {{I Want My Voice to Be Heard: IP over Voice-over-IP for Unobservable Censorship Circumvention}},
	Year = 2013}
	
	@inproceedings{censorspoofer,
	Author = {Q. Wang and X. Gong and G. Nguyen and A. Houmansadr and N. Borisov},
	Booktitle = {CCS},
	Title = {{CensorSpoofer: Asymmetric Communication Using IP Spoofing for Censorship-Resistant Web Browsing}},
	Year = {2012}}
	
	@inproceedings{skypemorph,
	Author = {H. Moghaddam and B. Li and M. Derakhshani and I. Goldberg},
	Booktitle = {CCS},
	Title = {{SkypeMorph: Protocol Obfuscation for Tor Bridges}},
	Year = {2012}}
	
	@inproceedings{stegotorus,
	Author = {Weinberg, Z. and Wang, J. and Yegneswaran, V. and Briesemeister, L. and Cheung, S. and Wang, F. and Boneh, D.},
	Booktitle = {CCS},
	Title = {{StegoTorus: A Camouflage Proxy for the Tor Anonymity System}},
	Year = {2012}}
	
	@techreport{dust,
	Author = {{B.~Wiley}},
	Howpublished = {\url{http://blanu.net/ Dust.pdf}},
	Institution = {School of Information, University of Texas at Austin},
	Title = {{Dust: A Blocking-Resistant Internet Transport Protocol}},
	Year = {2011}}
	
	@inproceedings{FTE,
	Author = {K.~Dyer and S.~Coull and T.~Ristenpart and T.~Shrimpton},
	Booktitle = {CCS},
	Title = {{Protocol Misidentification Made Easy with Format-Transforming Encryption}},
	Year = {2013}}
	
	@inproceedings{fp,
	Author = {Fifield, D. and Hardison, N. and Ellithrope, J. and Stark, E. and Dingledine, R. and Boneh, D. and Porras, P.},
	Booktitle = {PETS},
	Title = {{Evading Censorship with Browser-Based Proxies}},
	Year = {2012}}
	
	@misc{obfsproxy,
	Howpublished = {\url{https://www.torproject.org/projects/obfsproxy.html.en}},
	Key = {obfsproxy},
	Publisher = {The Tor Project},
	Title = {{A Simple Obfuscating Proxy}}}
	
	@inproceedings{Tor-instead-of-IP,
	Author = {Liu, V. and Han, S. and Krishnamurthy, A. and Anderson, T.},
	Booktitle = {HotNets},
	Title = {{Tor instead of IP}},
	Year = {2011}}
	
	@misc{roger-slides,
	Howpublished = {\url{https://svn.torproject.org/svn/projects/presentations/slides-28c3.pdf}},
	Key = {torblocking},
	Title = {{How Governments Have Tried to Block Tor}}}
	
	@inproceedings{infranet,
	Author = {Feamster, N. and Balazinska, M. and Harfst, G. and Balakrishnan, H. and Karger, D.},
	Booktitle = {USENIX Security},
	Title = {{Infranet: Circumventing Web Censorship and Surveillance}},
	Year = {2002}}
	
	@inproceedings{collage,
	Author = {S.~Burnett and N.~Feamster and S.~Vempala},
	Booktitle = {USENIX Security},
	Title = {{Chipping Away at Censorship Firewalls with User-Generated Content}},
	Year = {2010}}
	
	@article{anonymizer,
	Author = {Boyan, J.},
	Journal = {Computer-Mediated Communication Magazine},
	Month = sep,
	Number = {9},
	Title = {{The Anonymizer: Protecting User Privacy on the Web}},
	Volume = {4},
	Year = {1997}}
	
	@article{schulze2009internet,
	Author = {Schulze, H. and Mochalski, K.},
	Journal = {IPOQUE Report},
	Pages = {351--362},
	Title = {Internet Study 2008/2009},
	Volume = {37},
	Year = {2009}}
	
	@inproceedings{cya-ccs13,
	Author = {J.~Geddes and M.~Schuchard and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Cover Your ACKs: Pitfalls of Covert Channel Censorship Circumvention}},
	Year = {2013}}
	
	@inproceedings{andana,
	Author = {DiBenedetto, S. and Gasti, P. and Tsudik, G. and Uzun, E.},
	Booktitle = {{NDSS}},
	Title = {{ANDaNA: Anonymous Named Data Networking Application}},
	Year = {2012}}
	
	@inproceedings{darkly,
	Author = {Jana, S. and Narayanan, A. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{A Scanner Darkly: Protecting User Privacy From Perceptual Applications}},
	Year = {2013}}
	
	@inproceedings{NS08,
	Author = {A.~Narayanan and V.~Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {Robust de-anonymization of large sparse datasets},
	Year = {2008}}
	
	@inproceedings{NS09,
	Author = {A.~Narayanan and V.~Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {De-anonymizing social networks},
	Year = {2009}}
	
	@inproceedings{memento,
	Author = {Jana, S. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{Memento: Learning secrets from process footprints}},
	Year = {2012}}
	
	@misc{plugtor,
	Howpublished = {\url{https://www.torproject.org/docs/pluggable-transports.html.en}},
	Key = {PluggableTransports},
	Publisher = {The Tor Project},
	Title = {{Tor: Pluggable transports}}}
	
	@misc{psiphon,
	Author = {J.~Jia and P.~Smith},
	Howpublished = {\url{http://www.cdf.toronto.edu/~csc494h/reports/2004-fall/psiphon_ae.html}},
	Title = {{Psiphon: Analysis and Estimation}},
	Year = 2004}
	
	@misc{china-github,
	Howpublished = {\url{http://mobile.informationweek.com/80269/show/72e30386728f45f56b343ddfd0fdb119/}},
	Key = {github},
	Title = {{China's GitHub Censorship Dilemma}}}
	
	@inproceedings{txbox,
	Author = {Jana, S. and Porter, D. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{TxBox: Building Secure, Efficient Sandboxes with System Transactions}},
	Year = {2011}}
	
	@inproceedings{airavat,
	Author = {I. Roy and S. Setty and A. Kilzer and V. Shmatikov and E. Witchel},
	Booktitle = {NSDI},
	Title = {{Airavat: Security and Privacy for MapReduce}},
	Year = {2010}}
	
	@inproceedings{osdi12,
	Author = {A. Dunn and M. Lee and S. Jana and S. Kim and M. Silberstein and Y. Xu and V. Shmatikov and E. Witchel},
	Booktitle = {OSDI},
	Title = {{Eternal Sunshine of the Spotless Machine: Protecting Privacy with Ephemeral Channels}},
	Year = {2012}}
	
	@inproceedings{ymal,
	Author = {J. Calandrino and A. Kilzer and A. Narayanan and E. Felten and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{``You Might Also Like:'' Privacy Risks of Collaborative Filtering}},
	Year = {2011}}
	
	@inproceedings{srivastava11,
	Author = {V. Srivastava and M. Bond and K. McKinley and V. Shmatikov},
	Booktitle = {PLDI},
	Title = {{A Security Policy Oracle: Detecting Security Holes Using Multiple API Implementations}},
	Year = {2011}}
	
	@inproceedings{chen-oakland10,
	Author = {Chen, S. and Wang, R. and Wang, X. and Zhang, K.},
	Booktitle = {IEEE S\&P},
	Title = {{Side-Channel Leaks in Web Applications: A Reality Today, a Challenge Tomorrow}},
	Year = {2010}}
	
	@book{kerck,
	Author = {Kerckhoffs, A.},
	Publisher = {University Microfilms},
	Title = {{La cryptographie militaire}},
	Year = {1978}}
	
	@inproceedings{foci11,
	Author = {J. Karlin and D. Ellard and A.~Jackson and C.~ Jones and G. Lauer and D. Mankins and W.~T.~Strayer},
	Booktitle = {FOCI},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = 2011}
	
	@inproceedings{sun02,
	Author = {Sun, Q. and Simon, D.~R. and Wang, Y. and Russell, W. and Padmanabhan, V. and Qiu, L.},
	Booktitle = {IEEE S\&P},
	Title = {{Statistical Identification of Encrypted Web Browsing Traffic}},
	Year = {2002}}
	
	@inproceedings{danezis,
	Author = {Murdoch, S.~J. and Danezis, G.},
	Booktitle = {IEEE S\&P},
	Title = {{Low-Cost Traffic Analysis of Tor}},
	Year = {2005}}
	
	@inproceedings{pakicensorship,
	Author = {Z.~Nabi},
	Booktitle = {FOCI},
	Title = {The Anatomy of {Web} Censorship in {Pakistan}},
	Year = {2013}}
	
	@inproceedings{irancensorship,
	Author = {S.~Aryan and H.~Aryan and A.~Halderman},
	Booktitle = {FOCI},
	Title = {Internet Censorship in {Iran}: {A} First Look},
	Year = {2013}}
	
	@inproceedings{ford10efficient,
	Author = {Amittai Aviram and Shu-Chun Weng and Sen Hu and Bryan Ford},
	Booktitle = {\bibconf[9th]{OSDI}{USENIX Symposium on Operating Systems Design and Implementation}},
	Location = {Vancouver, BC, Canada},
	Month = oct,
	Title = {Efficient System-Enforced Deterministic Parallelism},
	Year = 2010}
	
	@inproceedings{ford10determinating,
	Author = {Amittai Aviram and Sen Hu and Bryan Ford and Ramakrishna Gummadi},
	Booktitle = {\bibconf{CCSW}{ACM Cloud Computing Security Workshop}},
	Location = {Chicago, IL},
	Month = oct,
	Title = {Determinating Timing Channels in Compute Clouds},
	Year = 2010}
	
	@inproceedings{ford12plugging,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Plugging Side-Channel Leaks with Timing Information Flow Control},
	Year = 2012}
	
	@inproceedings{ford12icebergs,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Icebergs in the Clouds: the {\em Other} Risks of Cloud Computing},
	Year = 2012}
	
	@misc{mullenize,
	Author = {Washington Post},
	Howpublished = {\url{http://apps.washingtonpost.com/g/page/world/gchq-report-on-mullenize-program-to-stain-anonymous-electronic-traffic/502/}},
	Month = {oct},
	Title = {{GCHQ} report on {`MULLENIZE'} program to `stain' anonymous electronic traffic},
	Year = {2013}}
	
	@inproceedings{shue13street,
	Author = {Craig A. Shue and Nathanael Paul and Curtis R. Taylor},
	Booktitle = {\bibbrev[7th]{WOOT}{USENIX Workshop on Offensive Technologies}},
	Month = aug,
	Title = {From an {IP} Address to a Street Address: Using Wireless Signals to Locate a Target},
	Year = 2013}
	
	@inproceedings{knockel11three,
	Author = {Jeffrey Knockel and Jedidiah R. Crandall and Jared Saia},
	Booktitle = {\bibbrev{FOCI}{USENIX Workshop on Free and Open Communications on the Internet}},
	Location = {San Francisco, CA},
	Month = aug,
	Year = 2011}
	
	@misc{rfc4960,
	Author = {R. {Stewart, ed.}},
	Month = sep,
	Note = {RFC 4960},
	Title = {Stream Control Transmission Protocol},
	Year = 2007}
	
	@inproceedings{ford07structured,
	Author = {Bryan Ford},
	Booktitle = {\bibbrev{SIGCOMM}{ACM SIGCOMM}},
	Location = {Kyoto, Japan},
	Month = aug,
	Title = {Structured Streams: a New Transport Abstraction},
	Year = {2007}}
	
	@misc{spdy,
	Author = {Google, Inc.},
	Note = {\url{http://www.chromium.org/spdy/spdy-whitepaper}},
	Title = {{SPDY}: An Experimental Protocol For a Faster {Web}}}
	
	@misc{quic,
	Author = {Jim Roskind},
	Month = jun,
	Note = {\url{http://blog.chromium.org/2013/06/experimenting-with-quic.html}},
	Title = {Experimenting with {QUIC}},
	Year = 2013}
	
	@misc{podjarny12not,
	Author = {G.~Podjarny},
	Month = jun,
	Note = {\url{http://www.guypo.com/technical/not-as-spdy-as-you-thought/}},
	Title = {{Not as SPDY as You Thought}},
	Year = 2012}
	
	@inproceedings{cor,
	Author = {Jones, N.~A. and Arye, M. and Cesareo, J. and Freedman, M.~J.},
	Booktitle = {FOCI},
	Title = {{Hiding Amongst the Clouds: A Proposal for Cloud-based Onion Routing}},
	Year = {2011}}
	
	@misc{torcloud,
	Howpublished = {\url{https://cloud.torproject.org/}},
	Key = {tor cloud},
	Title = {{The Tor Cloud Project}}}
	
	@inproceedings{scramblesuit,
	Author = {Philipp Winter and Tobias Pulls and Juergen Fuss},
	Booktitle = {WPES},
	Title = {{ScrambleSuit: A Polymorphic Network Protocol to Circumvent Censorship}},
	Year = 2013}
	
	@article{savage2000practical,
	Author = {Savage, S. and Wetherall, D. and Karlin, A. and Anderson, T.},
	Journal = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Pages = {295--306},
	Publisher = {ACM},
	Title = {Practical network support for IP traceback},
	Volume = {30},
	Year = {2000}}
	
	@inproceedings{ooni,
	Author = {Filast, A. and Appelbaum, J.},
	Booktitle = {{FOCI}},
	Title = {{OONI : Open Observatory of Network Interference}},
	Year = {2012}}
	
	@misc{caida-rank,
	Howpublished = {\url{http://as-rank.caida.org/}},
	Key = {caida rank},
	Title = {{AS Rank: AS Ranking}}}
	
	@inproceedings{usersrouted-ccs13,
	Author = {A.~Johnson and C.~Wacek and R.~Jansen and M.~Sherr and P.~Syverson},
	Booktitle = {CCS},
	Title = {{Users Get Routed: Traffic Correlation on Tor by Realistic Adversaries}},
	Year = {2013}}
	
	@inproceedings{edman2009awareness,
	Author = {Edman, M. and Syverson, P.},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2009}}
	
	@inproceedings{DecoyCosts,
	Author = {A.~Houmansadr and E.~L.~Wong and V.~Shmatikov},
	Booktitle = {NDSS},
	Title = {{No Direction Home: The True Cost of Routing Around Decoys}},
	Year = {2014}}
	
	@article{cordon,
	Author = {Elahi, T. and Goldberg, I.},
	Journal = {University of Waterloo CACR},
	Title = {{CORDON--A Taxonomy of Internet Censorship Resistance Strategies}},
	Volume = {33},
	Year = {2012}}
	
	@inproceedings{privex,
	Author = {T.~Elahi and G.~Danezis and I.~Goldberg	},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2014}}
	
	@inproceedings{changeGuards,
	Author = {T.~Elahi and K.~Bauer and M.~AlSabah and R.~Dingledine and I.~Goldberg},
	Booktitle = {{WPES}},
	Title = {{ Changing of the Guards: Framework for Understanding and Improving Entry Guard Selection in Tor}},
	Year = {2012}}
	
	@article{RAINBOW:Journal,
	Author = {A.~Houmansadr and N.~Kiyavash and N.~Borisov},
	Journal = {IEEE/ACM Transactions on Networking},
	Title = {{Non-Blind Watermarking of Network Flows}},
	Year = 2014}
	
	@inproceedings{info-tod,
	Author = {A.~Houmansadr and S.~Gorantla and T.~Coleman and N.~Kiyavash and and N.~Borisov},
	Booktitle = {{CCS (poster session)}},
	Title = {{On the Channel Capacity of Network Flow Watermarking}},
	Year = {2009}}
	
	@inproceedings{johnson2014game,
	Author = {Johnson, B. and Laszka, A. and Grossklags, J. and Vasek, M. and Moore, T.},
	Booktitle = {Workshop on Bitcoin Research},
	Title = {{Game-theoretic Analysis of DDoS Attacks Against Bitcoin Mining Pools}},
	Year = {2014}}
	
	@incollection{laszka2013mitigation,
	Author = {Laszka, A. and Johnson, B. and Grossklags, J.},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {175--191},
	Publisher = {Springer},
	Title = {{Mitigation of Targeted and Non-targeted Covert Attacks as a Timing Game}},
	Year = {2013}}
	
	@inproceedings{schottle2013game,
	Author = {Schottle, P. and Laszka, A. and Johnson, B. and Grossklags, J. and Bohme, R.},
	Booktitle = {EUSIPCO},
	Title = {{A Game-theoretic Analysis of Content-adaptive Steganography with Independent Embedding}},
	Year = {2013}}
	
	@inproceedings{CloudTransport,
	Author = {C.~Brubaker and A.~Houmansadr and V.~Shmatikov},
	Booktitle = {PETS},
	Title = {{CloudTransport: Using Cloud Storage for Censorship-Resistant Networking}},
	Year = {2014}}
	
	@inproceedings{sweet,
	Author = {W.~Zhou and A.~Houmansadr and M.~Caesar and N.~Borisov},
	Booktitle = {HotPETs},
	Title = {{SWEET: Serving the Web by Exploiting Email Tunnels}},
	Year = {2013}}
	
	@inproceedings{ahsan2002practical,
	Author = {Ahsan, K. and Kundur, D.},
	Booktitle = {Workshop on Multimedia Security},
	Title = {{Practical data hiding in TCP/IP}},
	Year = {2002}}
	
	@incollection{danezis2011covert,
	Author = {Danezis, G.},
	Booktitle = {Security Protocols XVI},
	Pages = {198--214},
	Publisher = {Springer},
	Title = {{Covert Communications Despite Traffic Data Retention}},
	Year = {2011}}
	
	@inproceedings{liu2009hide,
	Author = {Liu, Y. and Ghosal, D. and Armknecht, F. and Sadeghi, A.-R. and Schulz, S. and Katzenbeisser, S.},
	Booktitle = {ESORICS},
	Title = {{Hide and Seek in Time---Robust Covert Timing Channels}},
	Year = {2009}}
	
	@misc{image-watermark-fing,
	Author = {Jonathan Bailey},
	Howpublished = {\url{https://www.plagiarismtoday.com/2009/12/02/image-detection-watermarking-vs-fingerprinting/}},
	Title = {{Image Detection: Watermarking vs. Fingerprinting}},
	Year = {2009}}
	
	@inproceedings{Servetto98,
	Author = {S. D. Servetto and C. I. Podilchuk and K. Ramchandran},
	Booktitle = {Int. Conf. Image Processing},
	Title = {Capacity issues in digital image watermarking},
	Year = {1998}}
	
	@inproceedings{Chen01,
	Author = {B. Chen and G.W.Wornell},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1423--1443},
	Title = {Quantization index modulation: A class of provably good methods for digital watermarking and information embedding},
	Year = {2001}}
	
	@inproceedings{Karakos00,
	Author = {D. Karakos and A. Papamarcou},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {47},
	Title = {Relationship between quantization and distribution rates of digitally watermarked data},
	Year = {2000}}
	
	@inproceedings{Sullivan98,
	Author = {J. A. OSullivan and P. Moulin and J. M. Ettinger},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {297},
	Title = {Information theoretic analysis of steganography},
	Year = {1998}}
	
	@inproceedings{Merhav00,
	Author = {N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {420--430},
	Title = {On random coding error exponents of watermarking systems},
	Year = {2000}}
	
	@inproceedings{Somekh01,
	Author = {A. Somekh-Baruch and N. Merhav},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {7},
	Title = {On the error exponent and capacity games of private watermarking systems},
	Year = {2001}}
	
	@inproceedings{Steinberg01,
	Author = {Y. Steinberg and N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1410--1422},
	Title = {Identification in the presence of side information with application to watermarking},
	Year = {2001}}
	
	@article{Moulin03,
	Author = {P. Moulin and J.A. O'Sullivan},
	Journal = {IEEE Trans. Info. Theory},
	Number = {3},
	Title = {Information-theoretic analysis of information hiding},
	Volume = 49,
	Year = 2003}
	
	@article{Gelfand80,
	Author = {S.I.~Gelfand and M.S.~Pinsker},
	Journal = {Problems of Control and Information Theory},
	Number = {1},
	Pages = {19-31},
	Title = {{Coding for channel with random parameters}},
	Url = {citeseer.ist.psu.edu/anantharam96bits.html},
	Volume = {9},
	Year = {1980},
	Bdsk-Url-1 = {citeseer.ist.psu.edu/anantharam96bits.html}}
	
	@book{Wolfowitz78,
	Author = {J. Wolfowitz},
	Edition = {3rd},
	Location = {New York},
	Publisher = {Springer-Verlag},
	Title = {Coding Theorems of Information Theory},
	Year = 1978}
	
	@article{caire99,
	Author = {G. Caire and S. Shamai},
	Journal = {IEEE Transactions on Information Theory},
	Number = {6},
	Pages = {2007--2019},
	Title = {On the Capacity of Some Channels with Channel State Information},
	Volume = {45},
	Year = {1999}}
	
	@inproceedings{wright2007language,
	Author = {Wright, Charles V and Ballard, Lucas and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {USENIX Security},
	Title = {{Language identification of encrypted VoIP traffic: Alejandra y Roberto or Alice and Bob?}},
	Year = {2007}}
	
	@inproceedings{backes2010speaker,
	Author = {Backes, Michael and Doychev, Goran and D{\"u}rmuth, Markus and K{\"o}pf, Boris},
	Booktitle = {{European Symposium on Research in Computer Security (ESORICS)}},
	Pages = {508--523},
	Publisher = {Springer},
	Title = {{Speaker Recognition in Encrypted Voice Streams}},
	Year = {2010}}
	
	@phdthesis{lu2009traffic,
	Author = {Lu, Yuanchao},
	School = {Cleveland State University},
	Title = {{On Traffic Analysis Attacks to Encrypted VoIP Calls}},
	Year = {2009}}
	
	@inproceedings{wright2008spot,
	Author = {Wright, Charles V and Ballard, Lucas and Coull, Scott E and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {35--49},
	Title = {Spot me if you can: Uncovering spoken phrases in encrypted VoIP conversations},
	Year = {2008}}
	
	@inproceedings{white2011phonotactic,
	Author = {White, Andrew M and Matthews, Austin R and Snow, Kevin Z and Monrose, Fabian},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {3--18},
	Title = {Phonotactic reconstruction of encrypted VoIP conversations: Hookt on fon-iks},
	Year = {2011}}
	
	@inproceedings{fancy,
	Author = {Houmansadr, Amir and Borisov, Nikita},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {205--224},
	Title = {The Need for Flow Fingerprints to Link Correlated Network Flows},
	Year = {2013}}
	
	@article{botmosaic,
	Author = {Amir Houmansadr and Nikita Borisov},
	Doi = {10.1016/j.jss.2012.11.005},
	Issn = {0164-1212},
	Journal = {Journal of Systems and Software},
	Keywords = {Network security},
	Number = {3},
	Pages = {707 - 715},
	Title = {BotMosaic: Collaborative network watermark for the detection of IRC-based botnets},
	Url = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Volume = {86},
	Year = {2013},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.jss.2012.11.005}}
	
	@inproceedings{ramsbrock2008first,
	Author = {Ramsbrock, Daniel and Wang, Xinyuan and Jiang, Xuxian},
	Booktitle = {Recent Advances in Intrusion Detection},
	Organization = {Springer},
	Pages = {59--77},
	Title = {A first step towards live botmaster traceback},
	Year = {2008}}
	
	@inproceedings{potdar2005survey,
	Author = {Potdar, Vidyasagar M and Han, Song and Chang, Elizabeth},
	Booktitle = {Industrial Informatics, 2005. INDIN'05. 2005 3rd IEEE International Conference on},
	Organization = {IEEE},
	Pages = {709--716},
	Title = {A survey of digital image watermarking techniques},
	Year = {2005}}
	
	@book{cole2003hiding,
	Author = {Cole, Eric and Krutz, Ronald D},
	Publisher = {John Wiley \& Sons, Inc.},
	Title = {Hiding in plain sight: Steganography and the art of covert communication},
	Year = {2003}}
	
	@incollection{akaike1998information,
	Author = {Akaike, Hirotogu},
	Booktitle = {Selected Papers of Hirotugu Akaike},
	Pages = {199--213},
	Publisher = {Springer},
	Title = {Information theory and an extension of the maximum likelihood principle},
	Year = {1998}}
	
	@misc{central-command-hack,
	Author = {Everett Rosenfeld},
	Howpublished = {\url{http://www.cnbc.com/id/102330338}},
	Title = {{FBI investigating Central Command Twitter hack}},
	Year = {2015}}
	
	@misc{sony-psp-ddos,
	Howpublished = {\url{http://n4g.com/news/1644853/sony-and-microsoft-cant-do-much-ddos-attacks-explained}},
	Key = {sony},
	Month = {December},
	Title = {{Sony and Microsoft cant do much -- DDoS attacks explained}},
	Year = {2014}}
	
	@misc{sony-hack,
	Author = {David Bloom},
	Howpublished = {\url{http://goo.gl/MwR4A7}},
	Title = {{Online Game Networks Hacked, Sony Unit President Threatened}},
	Year = {2014}}
	
	@misc{home-depot,
	Author = {Dune Lawrence},
	Howpublished = {\url{http://www.businessweek.com/articles/2014-09-02/home-depots-credit-card-breach-looks-just-like-the-target-hack}},
	Title = {{Home Depot's Suspected Breach Looks Just Like the Target Hack}},
	Year = {2014}}
	
	@misc{target,
	Author = {Julio Ojeda-Zapata},
	Howpublished = {\url{http://www.mercurynews.com/business/ci_24765398/how-did-hackers-pull-off-target-data-heist}},
	Title = {{Target hack: How did they do it?}},
	Year = {2014}}
	
	
	@article{probabilitycourse,
	Author = {H. Pishro-Nik},
	note = {\url{http://www.probabilitycourse.com}},
	Title = {Introduction to probability, statistics, and random processes},
	Year = {2014}}
	
	
	
	@inproceedings{shokri2011quantifying,
	Author = {Shokri, Reza and Theodorakopoulos, George and Le Boudec, Jean-Yves and Hubaux, Jean-Pierre},
	Booktitle = {Security and Privacy (SP), 2011 IEEE Symposium on},
	Organization = {IEEE},
	Pages = {247--262},
	Title = {Quantifying location privacy},
	Year = {2011}}
	
	@inproceedings{hoh2007preserving,
	Author = {Hoh, Baik and Gruteser, Marco and Xiong, Hui and Alrabady, Ansaf},
	Booktitle = {Proceedings of the 14th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {161--171},
	Title = {Preserving privacy in gps traces via uncertainty-aware path cloaking},
	Year = {2007}}
	
	
	
	@article{kafsi2013entropy,
	Author = {Kafsi, Mohamed and Grossglauser, Matthias and Thiran, Patrick},
	Journal = {Information Theory, IEEE Transactions on},
	Number = {9},
	Pages = {5577--5583},
	Publisher = {IEEE},
	Title = {The entropy of conditional Markov trajectories},
	Volume = {59},
	Year = {2013}}
	
	@inproceedings{gruteser2003anonymous,
	Author = {Gruteser, Marco and Grunwald, Dirk},
	Booktitle = {Proceedings of the 1st international conference on Mobile systems, applications and services},
	Organization = {ACM},
	Pages = {31--42},
	Title = {Anonymous usage of location-based services through spatial and temporal cloaking},
	Year = {2003}}
	
	@inproceedings{husted2010mobile,
	Author = {Husted, Nathaniel and Myers, Steven},
	Booktitle = {Proceedings of the 17th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {85--96},
	Title = {Mobile location tracking in metro areas: malnets and others},
	Year = {2010}}
	
	@inproceedings{li2009tradeoff,
	Author = {Li, Tiancheng and Li, Ninghui},
	Booktitle = {Proceedings of the 15th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {517--526},
	Title = {On the tradeoff between privacy and utility in data publishing},
	Year = {2009}}
	
	@inproceedings{ma2009location,
	Author = {Ma, Zhendong and Kargl, Frank and Weber, Michael},
	Booktitle = {Sarnoff Symposium, 2009. SARNOFF'09. IEEE},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {A location privacy metric for v2x communication systems},
	Year = {2009}}
	
	@inproceedings{shokri2012protecting,
	Author = {Shokri, Reza and Theodorakopoulos, George and Troncoso, Carmela and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
	Booktitle = {Proceedings of the 2012 ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {617--627},
	Title = {Protecting location privacy: optimal strategy against localization attacks},
	Year = {2012}}
	
	@inproceedings{freudiger2009non,
	Author = {Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
	Booktitle = {Proceedings of the 16th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {324--337},
	Title = {On non-cooperative location privacy: a game-theoretic analysis},
	Year = {2009}}
	
	@incollection{humbert2010tracking,
	Author = {Humbert, Mathias and Manshaei, Mohammad Hossein and Freudiger, Julien and Hubaux, Jean-Pierre},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {38--57},
	Publisher = {Springer},
	Title = {Tracking games in mobile networks},
	Year = {2010}}
	
	@article{manshaei2013game,
	Author = {Manshaei, Mohammad Hossein and Zhu, Quanyan and Alpcan, Tansu and Bac{\c{s}}ar, Tamer and Hubaux, Jean-Pierre},
	Journal = {ACM Computing Surveys (CSUR)},
	Number = {3},
	Pages = {25},
	Publisher = {ACM},
	Title = {Game theory meets network security and privacy},
	Volume = {45},
	Year = {2013}}
	
	@article{palamidessi2006probabilistic,
	Author = {Palamidessi, Catuscia},
	Journal = {Electronic Notes in Theoretical Computer Science},
	Pages = {33--42},
	Publisher = {Elsevier},
	Title = {Probabilistic and nondeterministic aspects of anonymity},
	Volume = {155},
	Year = {2006}}
	
	@inproceedings{mokbel2006new,
	Author = {Mokbel, Mohamed F and Chow, Chi-Yin and Aref, Walid G},
	Booktitle = {Proceedings of the 32nd international conference on Very large data bases},
	Organization = {VLDB Endowment},
	Pages = {763--774},
	Title = {The new Casper: query processing for location services without compromising privacy},
	Year = {2006}}
	
	@article{kalnis2007preventing,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {12},
	Pages = {1719--1733},
	Publisher = {IEEE},
	Title = {Preventing location-based identity inference in anonymous spatial queries},
	Volume = {19},
	Year = {2007}}
	
	@article{freudiger2007mix,
	title={Mix-zones for location privacy in vehicular networks},
	author={Freudiger, Julien and Raya, Maxim and F{\'e}legyh{\'a}zi, M{\'a}rk and Papadimitratos, Panos and Hubaux, Jean-Pierre},
	year={2007}
	}
	@article{sweeney2002k,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {557--570},
	Publisher = {World Scientific},
	Title = {k-anonymity: A model for protecting privacy},
	Volume = {10},
	Year = {2002}}
	
	@article{sweeney2002achieving,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {571--588},
	Publisher = {World Scientific},
	Title = {Achieving k-anonymity privacy protection using generalization and suppression},
	Volume = {10},
	Year = {2002}}
	
	@inproceedings{niu2014achieving,
	Author = {Niu, Ben and Li, Qinghua and Zhu, Xiaoyan and Cao, Guohong and Li, Hui},
	Booktitle = {INFOCOM, 2014 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {754--762},
	Title = {Achieving k-anonymity in privacy-aware location-based services},
	Year = {2014}}
	
	@inproceedings{liu2013game,
	Author = {Liu, Xinxin and Liu, Kaikai and Guo, Linke and Li, Xiaolin and Fang, Yuguang},
	Booktitle = {INFOCOM, 2013 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {2985--2993},
	Title = {A game-theoretic approach for achieving k-anonymity in location based services},
	Year = {2013}}
	
	@inproceedings{kido2005protection,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Data Engineering Workshops, 2005. 21st International Conference on},
	Organization = {IEEE},
	Pages = {1248--1248},
	Title = {Protection of location privacy using dummies for location-based services},
	Year = {2005}}
	
	@inproceedings{gedik2005location,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Booktitle = {Distributed Computing Systems, 2005. ICDCS 2005. Proceedings. 25th IEEE International Conference on},
	Organization = {IEEE},
	Pages = {620--629},
	Title = {Location privacy in mobile systems: A personalized anonymization model},
	Year = {2005}}
	
	@inproceedings{bordenabe2014optimal,
	Author = {Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2014 ACM SIGSAC Conference on Computer and Communications Security},
	Organization = {ACM},
	Pages = {251--262},
	Title = {Optimal geo-indistinguishable mechanisms for location privacy},
	Year = {2014}}
	
	@incollection{duckham2005formal,
	Author = {Duckham, Matt and Kulik, Lars},
	Booktitle = {Pervasive computing},
	Pages = {152--170},
	Publisher = {Springer},
	Title = {A formal model of obfuscation and negotiation for location privacy},
	Year = {2005}}
	
	@inproceedings{kido2005anonymous,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Pervasive Services, 2005. ICPS'05. Proceedings. International Conference on},
	Organization = {IEEE},
	Pages = {88--97},
	Title = {An anonymous communication technique using dummies for location-based services},
	Year = {2005}}
	
	@incollection{duckham2006spatiotemporal,
	Author = {Duckham, Matt and Kulik, Lars and Birtley, Athol},
	Booktitle = {Geographic Information Science},
	Pages = {47--64},
	Publisher = {Springer},
	Title = {A spatiotemporal model of strategies and counter strategies for location privacy protection},
	Year = {2006}}
	
	@inproceedings{shankar2009privately,
	Author = {Shankar, Pravin and Ganapathy, Vinod and Iftode, Liviu},
	Booktitle = {Proceedings of the 11th international conference on Ubiquitous computing},
	Organization = {ACM},
	Pages = {31--40},
	Title = {Privately querying location-based services with SybilQuery},
	Year = {2009}}
	
	@inproceedings{chow2009faking,
	Author = {Chow, Richard and Golle, Philippe},
	Booktitle = {Proceedings of the 8th ACM workshop on Privacy in the electronic society},
	Organization = {ACM},
	Pages = {105--108},
	Title = {Faking contextual data for fun, profit, and privacy},
	Year = {2009}}
	
	@incollection{xue2009location,
	Author = {Xue, Mingqiang and Kalnis, Panos and Pung, Hung Keng},
	Booktitle = {Location and Context Awareness},
	Pages = {70--87},
	Publisher = {Springer},
	Title = {Location diversity: Enhanced privacy protection in location based services},
	Year = {2009}}
	
	@article{wernke2014classification,
	Author = {Wernke, Marius and Skvortsov, Pavel and D{\"u}rr, Frank and Rothermel, Kurt},
	Journal = {Personal and Ubiquitous Computing},
	Number = {1},
	Pages = {163--175},
	Publisher = {Springer-Verlag},
	Title = {A classification of location privacy attacks and approaches},
	Volume = {18},
	Year = {2014}}
	
	@misc{cai2015cloaking,
	Author = {Cai, Y. and Xu, G.},
	Month = jan # {~1},
	Note = {US Patent App. 14/472,462},
	Publisher = {Google Patents},
	Title = {Cloaking with footprints to provide location privacy protection in location-based services},
	Url = {https://www.google.com/patents/US20150007341},
	Year = {2015},
	Bdsk-Url-1 = {https://www.google.com/patents/US20150007341}}
	
	@article{gedik2008protecting,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {1},
	Pages = {1--18},
	Publisher = {IEEE},
	Title = {Protecting location privacy with personalized k-anonymity: Architecture and algorithms},
	Volume = {7},
	Year = {2008}}
	
	@article{kalnis2006preserving,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Publisher = {TRB6/06},
	Title = {Preserving anonymity in location based services},
	Year = {2006}}
	
	@inproceedings{hoh2005protecting,
	Author = {Hoh, Baik and Gruteser, Marco},
	Booktitle = {Security and Privacy for Emerging Areas in Communications Networks, 2005. SecureComm 2005. First International Conference on},
	Organization = {IEEE},
	Pages = {194--205},
	Title = {Protecting location privacy through path confusion},
	Year = {2005}}
	
	@article{terrovitis2011privacy,
	Author = {Terrovitis, Manolis},
	Journal = {ACM SIGKDD Explorations Newsletter},
	Number = {1},
	Pages = {6--18},
	Publisher = {ACM},
	Title = {Privacy preservation in the dissemination of location data},
	Volume = {13},
	Year = {2011}}
	
	@article{shin2012privacy,
	Author = {Shin, Kang G and Ju, Xiaoen and Chen, Zhigang and Hu, Xin},
	Journal = {Wireless Communications, IEEE},
	Number = {1},
	Pages = {30--39},
	Publisher = {IEEE},
	Title = {Privacy protection for users of location-based services},
	Volume = {19},
	Year = {2012}}
	
	@article{khoshgozaran2011location,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus and Shirani-Mehr, Houtan},
	Journal = {Knowledge and Information Systems},
	Number = {3},
	Pages = {435--465},
	Publisher = {Springer},
	Title = {Location privacy: going beyond K-anonymity, cloaking and anonymizers},
	Volume = {26},
	Year = {2011}}
	
	@incollection{chatzikokolakis2015geo,
	Author = {Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
	Booktitle = {Distributed Computing and Internet Technology},
	Pages = {49--72},
	Publisher = {Springer},
	Title = {Geo-indistinguishability: A Principled Approach to Location Privacy},
	Year = {2015}}
	
	@inproceedings{ngo2015location,
	Author = {Ngo, Hoa and Kim, Jong},
	Booktitle = {Computer Security Foundations Symposium (CSF), 2015 IEEE 28th},
	Organization = {IEEE},
	Pages = {63--74},
	Title = {Location Privacy via Differential Private Perturbation of Cloaking Area},
	Year = {2015}}
	
	@inproceedings{palanisamy2011mobimix,
	Author = {Palanisamy, Balaji and Liu, Ling},
	Booktitle = {Data Engineering (ICDE), 2011 IEEE 27th International Conference on},
	Organization = {IEEE},
	Pages = {494--505},
	Title = {Mobimix: Protecting location privacy with mix-zones over road networks},
	Year = {2011}}
	
	@inproceedings{um2010advanced,
	Author = {Um, Jung-Ho and Kim, Hee-Dae and Chang, Jae-Woo},
	Booktitle = {Social Computing (SocialCom), 2010 IEEE Second International Conference on},
	Organization = {IEEE},
	Pages = {1093--1098},
	Title = {An advanced cloaking algorithm using Hilbert curves for anonymous location based service},
	Year = {2010}}
	
	@inproceedings{bamba2008supporting,
	Author = {Bamba, Bhuvan and Liu, Ling and Pesti, Peter and Wang, Ting},
	Booktitle = {Proceedings of the 17th international conference on World Wide Web},
	Organization = {ACM},
	Pages = {237--246},
	Title = {Supporting anonymous location queries in mobile environments with privacygrid},
	Year = {2008}}
	
	@inproceedings{zhangwei2010distributed,
	Author = {Zhangwei, Huang and Mingjun, Xin},
	Booktitle = {Networks Security Wireless Communications and Trusted Computing (NSWCTC), 2010 Second International Conference on},
	Organization = {IEEE},
	Pages = {468--471},
	Title = {A distributed spatial cloaking protocol for location privacy},
	Volume = {2},
	Year = {2010}}
	
	@article{chow2011spatial,
	Author = {Chow, Chi-Yin and Mokbel, Mohamed F and Liu, Xuan},
	Journal = {GeoInformatica},
	Number = {2},
	Pages = {351--380},
	Publisher = {Springer},
	Title = {Spatial cloaking for anonymous location-based services in mobile peer-to-peer environments},
	Volume = {15},
	Year = {2011}}
	
	@inproceedings{lu2008pad,
	Author = {Lu, Hua and Jensen, Christian S and Yiu, Man Lung},
	Booktitle = {Proceedings of the Seventh ACM International Workshop on Data Engineering for Wireless and Mobile Access},
	Organization = {ACM},
	Pages = {16--23},
	Title = {Pad: privacy-area aware, dummy-based location privacy in mobile services},
	Year = {2008}}
	
	@incollection{khoshgozaran2007blind,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus},
	Booktitle = {Advances in Spatial and Temporal Databases},
	Pages = {239--257},
	Publisher = {Springer},
	Title = {Blind evaluation of nearest neighbor queries using space transformation to preserve location privacy},
	Year = {2007}}
	
	@inproceedings{ghinita2008private,
	Author = {Ghinita, Gabriel and Kalnis, Panos and Khoshgozaran, Ali and Shahabi, Cyrus and Tan, Kian-Lee},
	Booktitle = {Proceedings of the 2008 ACM SIGMOD international conference on Management of data},
	Organization = {ACM},
	Pages = {121--132},
	Title = {Private queries in location based services: anonymizers are not necessary},
	Year = {2008}}
	
	@article{paulet2014privacy,
	Author = {Paulet, Russell and Kaosar, Md Golam and Yi, Xun and Bertino, Elisa},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {5},
	Pages = {1200--1210},
	Publisher = {IEEE},
	Title = {Privacy-preserving and content-protecting location based queries},
	Volume = {26},
	Year = {2014}}
	
	@article{nguyen2013differential,
	Author = {Nguyen, Hiep H and Kim, Jong and Kim, Yoonho},
	Journal = {Journal of Computing Science and Engineering},
	Number = {3},
	Pages = {177--186},
	Title = {Differential privacy in practice},
	Volume = {7},
	Year = {2013}}
	
	@inproceedings{lee2012differential,
	Author = {Lee, Jaewoo and Clifton, Chris},
	Booktitle = {Proceedings of the 18th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {1041--1049},
	Title = {Differential identifiability},
	Year = {2012}}
	
	@inproceedings{andres2013geo,
	Author = {Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2013 ACM SIGSAC conference on Computer \& communications security},
	Organization = {ACM},
	Pages = {901--914},
	Title = {Geo-indistinguishability: Differential privacy for location-based systems},
	Year = {2013}}
	
	@inproceedings{machanavajjhala2008privacy,
	Author = {Machanavajjhala, Ashwin and Kifer, Daniel and Abowd, John and Gehrke, Johannes and Vilhuber, Lars},
	Booktitle = {Data Engineering, 2008. ICDE 2008. IEEE 24th International Conference on},
	Organization = {IEEE},
	Pages = {277--286},
	Title = {Privacy: Theory meets practice on the map},
	Year = {2008}}
	
	@article{dewri2013local,
	Author = {Dewri, Rinku},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {12},
	Pages = {2360--2372},
	Publisher = {IEEE},
	Title = {Local differential perturbations: Location privacy under approximate knowledge attackers},
	Volume = {12},
	Year = {2013}}
	
	@inproceedings{chatzikokolakis2013broadening,
	Author = {Chatzikokolakis, Konstantinos and Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s Emilio and Palamidessi, Catuscia},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {82--102},
	Title = {Broadening the Scope of Differential Privacy Using Metrics.},
	Year = {2013}}
	
	@inproceedings{zhong2009distributed,
	Author = {Zhong, Ge and Hengartner, Urs},
	Booktitle = {Pervasive Computing and Communications, 2009. PerCom 2009. IEEE International Conference on},
	Organization = {IEEE},
	Pages = {1--10},
	Title = {A distributed k-anonymity protocol for location privacy},
	Year = {2009}}
	
	@inproceedings{ho2011differential,
	Author = {Ho, Shen-Shyang and Ruan, Shuhua},
	Booktitle = {Proceedings of the 4th ACM SIGSPATIAL International Workshop on Security and Privacy in GIS and LBS},
	Organization = {ACM},
	Pages = {17--24},
	Title = {Differential privacy for location pattern mining},
	Year = {2011}}
	
	@inproceedings{cheng2006preserving,
	Author = {Cheng, Reynold and Zhang, Yu and Bertino, Elisa and Prabhakar, Sunil},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {393--412},
	Title = {Preserving user location privacy in mobile data management infrastructures},
	Year = {2006}}
	
	@article{beresford2003location,
	Author = {Beresford, Alastair R and Stajano, Frank},
	Journal = {IEEE Pervasive computing},
	Number = {1},
	Pages = {46--55},
	Publisher = {IEEE},
	Title = {Location privacy in pervasive computing},
	Year = {2003}}
	
	@inproceedings{freudiger2009optimal,
	Author = {Freudiger, Julien and Shokri, Reza and Hubaux, Jean-Pierre},
	Booktitle = {Privacy enhancing technologies},
	Organization = {Springer},
	Pages = {216--234},
	Title = {On the optimal placement of mix zones},
	Year = {2009}}
	
	@article{krumm2009survey,
	Author = {Krumm, John},
	Journal = {Personal and Ubiquitous Computing},
	Number = {6},
	Pages = {391--399},
	Publisher = {Springer},
	Title = {A survey of computational location privacy},
	Volume = {13},
	Year = {2009}}
	
	@article{Rakhshan2016letter,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Wireless Communications Letter},
	Publisher = {IEEE},
	Title = {Interference Models for Vehicular Ad Hoc Networks},
	Year = {2016, submitted}}
	
	@article{Rakhshan2015Journal,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Publisher = {IEEE},
	Title = {Improving Safety on Highways by Customizing Vehicular Ad Hoc Networks},
	Year = {to appear, 2017}}
	
	@inproceedings{Rakhshan2015Cogsima,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Booktitle = {IEEE International Multi-Disciplinary Conference on Cognitive Methods in Situation Awareness and Decision Support},
	Organization = {IEEE},
	Title = {A New Approach to Customization of Accident Warning Systems to Individual Drivers},
	Year = {2015}}
	
	@inproceedings{Rakhshan2015CISS,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Nekoui, Mohammad},
	Booktitle = {Conference on Information Sciences and Systems},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {Driver-based adaptation of Vehicular Ad Hoc Networks for design of active safety systems},
	Year = {2015}}
	
	@inproceedings{Rakhshan2014IV,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Ray, Evan},
	Booktitle = {Intelligent Vehicles Symposium},
	Organization = {IEEE},
	Pages = {1181--1186},
	Title = {Real-time estimation of the distribution of brake response times for an individual driver using Vehicular Ad Hoc Network.},
	Year = {2014}}
	
	@inproceedings{Rakhshan2013Globecom,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Fisher, Donald and Nekoui, Mohammad},
	Booktitle = {IEEE Global Communications Conference},
	Organization = {IEEE},
	Pages = {1333--1337},
	Title = {Tuning collision warning algorithms to individual drivers for design of active safety systems.},
	Year = {2013}}
	
	@article{Nekoui2012Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Number = {8},
	Pages = {2895--2905},
	Publisher = {IEEE},
	Title = {Throughput Scaling laws for Vehicular Ad Hoc Networks},
	Volume = {11},
	Year = {2012}}
	
	
	
	
	
	
	
	
	
	@article{Nekoui2011Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein and Ni, Daiheng},
	Journal = {International Journal of Vehicular Technology},
	Pages = {1--11},
	Publisher = {Hindawi Publishing Corporation},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {2011},
	Year = {2011}}
	
	
	
	
	
	
	@article{shokri2014optimal,
	title={Optimal user-centric data obfuscation},
	author={Shokri, Reza},
	journal={arXiv preprint arXiv:1402.3426},
	year={2014}
	}
	@article{chatzikokolakis2015location,
	title={Location privacy via geo-indistinguishability},
	author={Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
	journal={ACM SIGLOG News},
	volume={2},
	number={3},
	pages={46--69},
	year={2015},
	publisher={ACM}
	
	}
	@inproceedings{shokri2011quantifying2,
	title={Quantifying location privacy: the case of sporadic location exposure},
	author={Shokri, Reza and Theodorakopoulos, George and Danezis, George and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
	booktitle={Privacy Enhancing Technologies},
	pages={57--76},
	year={2011},
	organization={Springer}
	}
	
	
	@inproceedings{Mont1603:Defining,
	AUTHOR="Zarrin Montazeri and Amir Houmansadr and Hossein Pishro-Nik",
	TITLE="Defining Perfect Location Privacy Using Anonymization",
	BOOKTITLE="2016 Annual Conference on Information Science and Systems (CISS) (CISS
	2016)",
	ADDRESS="Princeton, USA",
	DAYS=16,
	MONTH=mar,
	YEAR=2016,
	KEYWORDS="Information Theoretic Privacy; location-based services; Location Privacy;
	Information Theory",
	ABSTRACT="The popularity of mobile devices and location-based services (LBS) have
	created great concerns regarding the location privacy of users of such
	devices and services. Anonymization is a common technique that is often
	being used to protect the location privacy of LBS users. In this paper, we
	provide a general information theoretic definition for location privacy. In
	particular, we define perfect location privacy. We show that under certain
	conditions, perfect privacy is achieved if the pseudonyms of users is
	changed after o(N^(2/r?1)) observations by the adversary, where N is the
	number of users and r is the number of sub-regions or locations.
	"
	}
	@article{our-isita-location,
	Author = {Zarrin Montazeri and Amir Houmansadr and Hossein Pishro-Nik},
	Journal = {IEEE International Symposium on Information Theory and Its Applications (ISITA)},
	Title = {Achieving Perfect Location Privacy in Markov Models Using Anonymization},
	Year = {2016}
	}
	@article{our-TIFS,
	Author = {Zarrin Montazeri and Hossein Pishro-Nik and Amir Houmansadr},
	Journal = {IEEE Transactions on Information Forensics and Security, under revison},
	Title = {Perfect Location Privacy Using Anonymization in Mobile Networks},
	Year = {2016},
	note={Available on arxiv.org}
	}
	
	
	
	@techreport{sampigethaya2005caravan,
	title={CARAVAN: Providing location privacy for VANET},
	author={Sampigethaya, Krishna and Huang, Leping and Li, Mingyan and Poovendran, Radha and Matsuura, Kanta and Sezaki, Kaoru},
	year={2005},
	institution={DTIC Document}
	}
	@incollection{buttyan2007effectiveness,
	title={On the effectiveness of changing pseudonyms to provide location privacy in VANETs},
	author={Butty{\'a}n, Levente and Holczer, Tam{\'a}s and Vajda, Istv{\'a}n},
	booktitle={Security and Privacy in Ad-hoc and Sensor Networks},
	pages={129--141},
	year={2007},
	publisher={Springer}
	}
	@article{sampigethaya2007amoeba,
	title={AMOEBA: Robust location privacy scheme for VANET},
	author={Sampigethaya, Krishna and Li, Mingyan and Huang, Leping and Poovendran, Radha},
	journal={Selected Areas in communications, IEEE Journal on},
	volume={25},
	number={8},
	pages={1569--1589},
	year={2007},
	publisher={IEEE}
	}
	
	@article{lu2012pseudonym,
	title={Pseudonym changing at social spots: An effective strategy for location privacy in vanets},
	author={Lu, Rongxing and Li, Xiaodong and Luan, Tom H and Liang, Xiaohui and Shen, Xuemin},
	journal={Vehicular Technology, IEEE Transactions on},
	volume={61},
	number={1},
	pages={86--96},
	year={2012},
	publisher={IEEE}
	}
	@inproceedings{lu2010sacrificing,
	title={Sacrificing the plum tree for the peach tree: A socialspot tactic for protecting receiver-location privacy in VANET},
	author={Lu, Rongxing and Lin, Xiaodong and Liang, Xiaohui and Shen, Xuemin},
	booktitle={Global Telecommunications Conference (GLOBECOM 2010), 2010 IEEE},
	pages={1--5},
	year={2010},
	organization={IEEE}
	}
	@inproceedings{lin2011stap,
	title={STAP: A social-tier-assisted packet forwarding protocol for achieving receiver-location privacy preservation in VANETs},
	author={Lin, Xiaodong and Lu, Rongxing and Liang, Xiaohui and Shen, Xuemin Sherman},
	booktitle={INFOCOM, 2011 Proceedings IEEE},
	pages={2147--2155},
	year={2011},
	organization={IEEE}
	}
	@inproceedings{gerlach2007privacy,
	title={Privacy in VANETs using changing pseudonyms-ideal and real},
	author={Gerlach, Matthias and Guttler, Felix},
	booktitle={Vehicular Technology Conference, 2007. VTC2007-Spring. IEEE 65th},
	pages={2521--2525},
	year={2007},
	organization={IEEE}
	}
	@inproceedings{el2002security,
	title={Security issues in a future vehicular network},
	author={El Zarki, Magda and Mehrotra, Sharad and Tsudik, Gene and Venkatasubramanian, Nalini},
	booktitle={European Wireless},
	volume={2},
	year={2002}
	}
	
	@article{hubaux2004security,
	title={The security and privacy of smart vehicles},
	author={Hubaux, Jean-Pierre and Capkun, Srdjan and Luo, Jun},
	journal={IEEE Security \& Privacy Magazine},
	volume={2},
	number={LCA-ARTICLE-2004-007},
	pages={49--55},
	year={2004}
	}
	
	
	
	@inproceedings{duri2002framework,
	title={Framework for security and privacy in automotive telematics},
	author={Duri, Sastry and Gruteser, Marco and Liu, Xuan and Moskowitz, Paul and Perez, Ronald and Singh, Moninder and Tang, Jung-Mu},
	booktitle={Proceedings of the 2nd international workshop on Mobile commerce},
	pages={25--32},
	year={2002},
	organization={ACM}
	}
	@misc{NS-3,
	Howpublished = {\url{https://www.nsnam.org/}}},
}
@misc{testbed,
	Howpublished = {\url{http://www.its.dot.gov/testbed/PDF/SE-MI-Resource-Guide-9-3-1.pdf}}},
@misc{NGSIM,
	Howpublished = {\url{http://ops.fhwa.dot.gov/trafficanalysistools/ngsim.htm}},
}

@misc{National-a2013,
	Author = {National Highway Traffic Safety Administration},
	Howpublished = {\url{http://ops.fhwa.dot.gov/trafficanalysistools/ngsim.htm}},
	Title = {2013 Motor Vehicle Crashes: Overview. Traffic Safety Factors},
	Year = {2013}
}

@inproceedings{karnadi2007rapid,
	title={Rapid generation of realistic mobility models for VANET},
	author={Karnadi, Feliz Kristianto and Mo, Zhi Hai and Lan, Kun-chan},
	booktitle={Wireless Communications and Networking Conference, 2007. WCNC 2007. IEEE},
	pages={2506--2511},
	year={2007},
	organization={IEEE}
}
@inproceedings{saha2004modeling,
	title={Modeling mobility for vehicular ad-hoc networks},
	author={Saha, Amit Kumar and Johnson, David B},
	booktitle={Proceedings of the 1st ACM international workshop on Vehicular ad hoc networks},
	pages={91--92},
	year={2004},
	organization={ACM}
}
@inproceedings{lee2006modeling,
	title={Modeling steady-state and transient behaviors of user mobility: formulation, analysis, and application},
	author={Lee, Jong-Kwon and Hou, Jennifer C},
	booktitle={Proceedings of the 7th ACM international symposium on Mobile ad hoc networking and computing},
	pages={85--96},
	year={2006},
	organization={ACM}
}
@inproceedings{yoon2006building,
	title={Building realistic mobility models from coarse-grained traces},
	author={Yoon, Jungkeun and Noble, Brian D and Liu, Mingyan and Kim, Minkyong},
	booktitle={Proceedings of the 4th international conference on Mobile systems, applications and services},
	pages={177--190},
	year={2006},
	organization={ACM}
}

@inproceedings{choffnes2005integrated,
	title={An integrated mobility and traffic model for vehicular wireless networks},
	author={Choffnes, David R and Bustamante, Fabi{\'a}n E},
	booktitle={Proceedings of the 2nd ACM international workshop on Vehicular ad hoc networks},
	pages={69--78},
	year={2005},
	organization={ACM}
}

@inproceedings{Qian2008Globecom,
	title={CA Secure VANET MAC Protocol for DSRC Applications},
	author={Yi, Q. and Lu, K. and Moyeri, N.{\'a}n E},
	booktitle={Proceedings of IEEE GLOBECOM 2008},
	pages={1--5},
	year={2008},
	organization={IEEE}
}





@inproceedings{naumov2006evaluation,
	title={An evaluation of inter-vehicle ad hoc networks based on realistic vehicular traces},
	author={Naumov, Valery and Baumann, Rainer and Gross, Thomas},
	booktitle={Proceedings of the 7th ACM international symposium on Mobile ad hoc networking and computing},
	pages={108--119},
	year={2006},
	organization={ACM}
}
@article{sommer2008progressing,
	title={Progressing toward realistic mobility models in VANET simulations},
	author={Sommer, Christoph and Dressler, Falko},
	journal={Communications Magazine, IEEE},
	volume={46},
	number={11},
	pages={132--137},
	year={2008},
	publisher={IEEE}
}




@inproceedings{mahajan2006urban,
	title={Urban mobility models for vanets},
	author={Mahajan, Atulya and Potnis, Niranjan and Gopalan, Kartik and Wang, Andy},
	booktitle={2nd IEEE International Workshop on Next Generation Wireless Networks},
	volume={33},
	year={2006}
}

@inproceedings{Rakhshan2016packet,
	title={Packet success probability derivation in a vehicular ad hoc network for a highway scenario},
	author={Rakhshan, Ali and Pishro-Nik, Hossein},
	booktitle={2016 Annual Conference on Information Science and Systems (CISS)},
	pages={210--215},
	year={2016},
	organization={IEEE}
}

@inproceedings{Rakhshan2016CISS,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Booktitle = {Conference on Information Sciences and Systems},
	Organization = {IEEE},
	Pages = {210--215},
	Title = {Packet Success Probability Derivation in a Vehicular Ad Hoc Network for a Highway Scenario},
	Year = {2016}}

@article{Nekoui2013Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {Journal on Selected Areas in Communications, Special Issue on Emerging Technologies in Communications},
	Number = {9},
	Pages = {491--503},
	Publisher = {IEEE},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {31},
	Year = {2013}}


@inproceedings{Nekoui2011MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM workshop on VehiculAr InterNETworking},
	Organization = {ACM},
	Title = {Analytic Design of Active Vehicular Safety Systems in Sparse Traffic},
	Year = {2011}}

@inproceedings{Nekoui2011VTC,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Analytical Design of Inter-vehicular Communications for Collision Avoidance},
	Year = {2011}}

@inproceedings{Bovee2011VTC,
	Author = {Bovee, Ben Louis and Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Evaluation of the Universal Geocast Scheme For VANETs},
	Year = {2011}}

@inproceedings{Nekoui2010MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM},
	Organization = {ACM},
	Title = {Fundamental Tradeoffs in Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2010IVCS,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IVCS},
	Organization = {IEEE},
	Title = {A Universal Geocast Scheme for Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2009ITW,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IEEE Communications Society Conference on Sensor, Mesh and Ad Hoc Communications and Networks Workshops},
	Organization = {IEEE},
	Pages = {1--3},
	Title = {A Geometrical Analysis of Obstructed Wireless Networks},
	Year = {2009}}

@article{Eslami2013Journal,
	Author = {Eslami, Ali and Nekoui, Mohammad and Pishro-Nik, Hossein and Fekri, Faramarz},
	Journal = {ACM Transactions on Sensor Networks},
	Number = {4},
	Pages = {51},
	Publisher = {ACM},
	Title = {Results on finite wireless sensor networks: Connectivity and coverage},
	Volume = {9},
	Year = {2013}}


@article{Jiafu2014Journal,
	Author = {Jiafu, W. and Zhang, D. and Zhao, S. and Yang, L. and Lloret, J.},
	Journal = {Communications Magazine},
	Number = {8},
	Pages = {106-113},
	Publisher = {IEEE},
	Title = {Context-aware vehicular cyber-physical systems with cloud support: architecture, challenges, and solutions},
	Volume = {52},
	Year = {2014}}

@inproceedings{Haas2010ACM,
	Author = {Haas, J.J. and Hu, Y.},
	Booktitle = {international workshop on VehiculAr InterNETworking},
	Organization = {ACM},
	Title = {Communication requirements for crash avoidance.},
	Year = {2010}}

@inproceedings{Yi2008GLOBECOM,
	Author = {Yi, Q. and Lu, K. and Moayeri, N.},
	Booktitle = {GLOBECOM},
	Organization = {IEEE},
	Title = {CA Secure VANET MAC Protocol for DSRC Applications.},
	Year = {2008}}

@inproceedings{Mughal2010ITSim,
	Author = {Mughal, B.M. and Wagan, A. and Hasbullah, H.},
	Booktitle = {International Symposium on Information Technology (ITSim)},
	Organization = {IEEE},
	Title = {Efficient congestion control in VANET for safety messaging.},
	Year = {2010}}

@article{Chang2011Journal,
	Author = {Chang, Y. and Lee, C. and Copeland, J.},
	Journal = {Selected Areas in Communications},
	Pages = {236 â€“249},
	Publisher = {IEEE},
	Title = {Goodput enhancement of VANETs in noisy CSMA/CA channels},
	Volume = {29},
	Year = {2011}}

@article{Garcia-Costa2011Journal,
	Author = {Garcia-Costa, C. and Egea-Lopez, E. and Tomas-Gabarron, J. B. and Garcia-Haro, J. and Haas, Z. J.},
	Journal = {Transactions on Intelligent Transportation Systems},
	Pages = {1 â€“16},
	Publisher = {IEEE},
	Title = {A stochastic model for chain collisions of vehicles equipped with vehicular communications},
	Volume = {99},
	Year = {2011}}

@article{Carbaugh2011Journal,
	Author = {Carbaugh, J. and Godbole,  D. N. and Sengupta, R. and Garcia-Haro, J. and Haas, Z. J.},
	Publisher = {Transportation Research Part C (Emerging Technologies)},
	Title = {Safety and capacity analysis of automated and manual highway systems},
	Year = {1997}}

@article{Goh2004Journal,
	Author = {Goh, P. and Wong, Y.},
	Publisher = {Appl Health Econ Health Policy},
	Title = {Driver perception response time during the signal change interval},
	Year = {2004}}

@article{Chang1985Journal,
	Author = {Chang, M.S. and Santiago, A.J.},
	Pages = {20-30},
	Publisher = {Transportation Research Record},
	Title = {Timing traffic signal changes based on driver behavior},
	Volume = {1027},
	Year = {1985}}

@article{Green2000Journal,
	Author = {Green, M.},
	Pages = {195-216},
	Publisher = {Transportation Human Factors},
	Title = {How long does it take to stop? Methodological analysis of driver perception-brake times.},
	Year = {2000}}

@article{Koppa2005,
	Author = {Koppa, R.J.},
	Pages = {195-216},
	Publisher = {http://www.fhwa.dot.gov/publications/},
	Title = {Human Factors},
	Year = {2005}}

@inproceedings{Maxwell2010ETC,
	Author = {Maxwell, A. and Wood, K.},
	Booktitle = {Europian Transport Conference},
	Organization = {http://www.etcproceedings.org/paper/review-of-traffic-signals-on-high-speed-roads},
	Title = {Review of Traffic Signals on High Speed Road},
	Year = {2010}}

@article{Wortman1983,
	Author = {Wortman, R.H. and Matthias, J.S.},
	Publisher = {Arizona Department of Transportation},
	Title = {An Evaluation of Driver Behavior at Signalized Intersections},
	Year = {1983}}
@inproceedings{Zhang2007IASTED,
	Author = {Zhang, X. and Bham, G.H.},
	Booktitle = {18th IASTED International Conference: modeling and simulation},
	Title = {Estimation of driver reaction time from detailed vehicle trajectory data.},
	Year = {2007}}


@inproceedings{bai2003important,
	title={IMPORTANT: A framework to systematically analyze the Impact of Mobility on Performance of RouTing protocols for Adhoc NeTworks},
	author={Bai, Fan and Sadagopan, Narayanan and Helmy, Ahmed},
	booktitle={INFOCOM 2003. Twenty-second annual joint conference of the IEEE computer and communications. IEEE societies},
	volume={2},
	pages={825--835},
	year={2003},
	organization={IEEE}
}


@inproceedings{abedi2008enhancing,
	title={Enhancing AODV routing protocol using mobility parameters in VANET},
	author={Abedi, Omid and Fathy, Mahmood and Taghiloo, Jamshid},
	booktitle={Computer Systems and Applications, 2008. AICCSA 2008. IEEE/ACS International Conference on},
	pages={229--235},
	year={2008},
	organization={IEEE}
}


@article{AlSultan2013Journal,
	Author = {Al-Sultan, Saif and Al-Bayatti, Ali H. and Zedan, Hussien},
	Journal = {IEEE Transactions on Vehicular Technology},
	Number = {9},
	Pages = {4264-4275},
	Publisher = {IEEE},
	Title = {Context Aware Driver Behaviour Detection System in Intelligent Transportation Systems},
	Volume = {62},
	Year = {2013}}






@article{Leow2008ITS,
	Author = {Leow, Woei Ling and Ni, Daiheng and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Intelligent Transportation Systems},
	Number = {2},
	Pages = {369--374},
	Publisher = {IEEE},
	Title = {A Sampling Theorem Approach to Traffic Sensor Optimization},
	Volume = {9},
	Year = {2008}}



@article{REU2007,
	Author = {D. Ni and H. Pishro-Nik and R. Prasad and M. R. Kanjee and H. Zhu and T. Nguyen},
	Journal = {in 14th World Congress on Intelligent Transport Systems},
	Title = {Development of a prototype intersection collision avoidance system under VII},
	Year = {2007}}




@inproceedings{salamatian2013hide,
	title={How to hide the elephant-or the donkey-in the room: Practical privacy against statistical inference for large data.},
	author={Salamatian, Salman and Zhang, Amy and du Pin Calmon, Flavio and Bhamidipati, Sandilya and Fawaz, Nadia and Kveton, Branislav and Oliveira, Pedro and Taft, Nina},
	booktitle={GlobalSIP},
	pages={269--272},
	year={2013}
}

@article{sankar2013utility,
	title={Utility-privacy tradeoffs in databases: An information-theoretic approach},
	author={Sankar, Lalitha and Rajagopalan, S Raj and Poor, H Vincent},
	journal={Information Forensics and Security, IEEE Transactions on},
	volume={8},
	number={6},
	pages={838--852},
	year={2013},
	publisher={IEEE}
}
@inproceedings{ghinita2007prive,
	title={PRIVE: anonymous location-based queries in distributed mobile systems},
	author={Ghinita, Gabriel and Kalnis, Panos and Skiadopoulos, Spiros},
	booktitle={Proceedings of the 16th international conference on World Wide Web},
	pages={371--380},
	year={2007},
	organization={ACM}
}

@article{beresford2004mix,
	title={Mix zones: User privacy in location-aware services},
	author={Beresford, Alastair R and Stajano, Frank},
	year={2004},
	publisher={IEEE}
}

%@inproceedings{Mont1610Achieving,
	%  title={Achieving Perfect Location Privacy in Markov Models Using Anonymization},
	%  author={Montazeri, Zarrin and Houmansadr, Amir and H.Pishro-Nik},
	%  booktitle="2016 International Symposium on Information Theory and its Applications
	%  (ISITA2016)",
	%  address="Monterey, USA",
	%  days=30,
	%  month=oct,
	%  year=2016,
	%}

@article{csiszar1996almost,
	title={Almost independence and secrecy capacity},
	author={Csisz{\'a}r, Imre},
	journal={Problemy Peredachi Informatsii},
	volume={32},
	number={1},
	pages={48--57},
	year={1996},
	publisher={Russian Academy of Sciences, Branch of Informatics, Computer Equipment and Automatization}
}

@article{yamamoto1983source,
	title={A source coding problem for sources with additional outputs to keep secret from the receiver or wiretappers (corresp.)},
	author={Yamamoto, Hirosuke},
	journal={IEEE Transactions on Information Theory},
	volume={29},
	number={6},
	pages={918--923},
	year={1983},
	publisher={IEEE}
}


@inproceedings{calmon2015fundamental,
	title={Fundamental limits of perfect privacy},
	author={Calmon, Flavio P and Makhdoumi, Ali and M{\'e}dard, Muriel},
	booktitle={Information Theory (ISIT), 2015 IEEE International Symposium on},
	pages={1796--1800},
	year={2015},
	organization={IEEE}
}



@inproceedings{Lehman1999Large-Sample-Theory,
	title={Elements of Large Sample Theory},
	author={E. L. Lehman},
	organization={Springer},
	year={1999}
}


@inproceedings{Ferguson1999Large-Sample-Theory,
	title={A Course in Large Sample Theory},
	author={Thomas S. Ferguson},
	organization={CRC Press},
	year={1996}
}



@inproceedings{Dembo1999Large-Deviations,
	title={Large Deviation Techniques and Applications, Second Edition},
	author={A. Dembo and O. Zeitouni},
	organization={Springer},
	year={1998}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Hossein's Coding Journals
%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{myoptics,
	AUTHOR =       "H. Pishro-Nik and N. Rahnavard and J. Ha and F. Fekri and A. Adibi ",
	TITLE =        "Low-density parity-check codes for volume holographic memory systems",
	JOURNAL =      " Appl. Opt.",
	YEAR =         "2003",
	volume =       "42",
	pages =        "861-870  "
}






@ARTICLE{myit,
	AUTHOR =       "H. Pishro-Nik and F. Fekri  ",
	TITLE =        "On Decoding of Low-Density Parity-Check Codes on the Binary Erasure Channel",
	JOURNAL =      "IEEE Trans. Inform. Theory",
	YEAR =         "2004",
	volume =       "50",
	pages =        "439--454"
}




@ARTICLE{myitpuncture,
	AUTHOR =       "H. Pishro-Nik and F. Fekri  ",
	TITLE =        "Results on Punctured Low-Density Parity-Check Codes and Improved Iterative Decoding Techniques",
	JOURNAL =      "IEEE Trans. on Inform. Theory",
	YEAR =         "2007",
	volume =       "53",
	number=        "2",
	pages =        "599--614",
	month= "February"
}




@ARTICLE{myitlinmimdist,
	AUTHOR =       "H. Pishro-Nik and F. Fekri",
	TITLE =        "Performance of Low-Density Parity-Check Codes With Linear Minimum Distance",
	JOURNAL =         "IEEE Trans. Inform. Theory ",
	YEAR =         "2006",
	volume =       "52",
	number="1",
	pages =        "292 --300"
}






@ARTICLE{myitnonuni,
	AUTHOR =       "H. Pishro-Nik and N. Rahnavard and F. Fekri  ",
	TITLE =        "Non-uniform Error Correction Using Low-Density Parity-Check Codes",
	JOURNAL =      "IEEE Trans. Inform. Theory",
	YEAR =         "2005",
	volume =       "51",
	number=  "7",
	pages =        "2702--2714"
}





@article{eslamitcomhybrid10,
	author = {A. Eslami and S. Vangala and H. Pishro-Nik},
	title = {Hybrid channel codes for highly efficient FSO/RF communication systems},
	journal = {IEEE Transactions on Communications},
	volume = {58},
	number = {10},
	year = {2010},
	pages = {2926--2938},
}


@article{eslamitcompolar13,
	author = {A. Eslami and H. Pishro-Nik},
	title = {On Finite-Length Performance of Polar Codes: Stopping Sets, Error Floor, and Concatenated Design},
	journal = {IEEE Transactions on Communications},
	volume = {61},
	number = {13},
	year = {2013},
	pages = {919--929},
}



@article{saeeditcom11,
	author = {H. Saeedi and H. Pishro-Nik and  A. H. Banihashemi},
	title = {Successive maximization for the systematic design of universally capacity approaching rate-compatible
	sequences of LDPC code ensembles over binary-input output-symmetric memoryless channels},
	journal = {IEEE Transactions on Communications},
	year = {2011},
	volume={59},
	number = {7}
}


@article{rahnavard07,
	author = {Rahnavard, N. and Pishro-Nik, H. and Fekri, F.},
	title = {Unequal Error Protection Using Partially Regular LDPC Codes},
	journal = {IEEE Transactions on Communications},
	year = {2007},
	volume = {55},
	number = {3},
	pages = {387 -- 391}
}


@article{hosseinira04,
	author = {H. Pishro-Nik and F. Fekri},
	title = {Irregular repeat-accumulate codes for volume holographic memory systems},
	journal = {Journal of Applied Optics},
	year = {2004},
	volume = {43},
	number = {27},
	pages = {5222--5227},
}


@article{azadeh2015Ephemeralkey,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
	journal = {IEEE Transactions on Wireless Communications},
	year = {2015},
	volume = {14},
	number = {11},
	pages = {6072--6081},
}


@article{azadeh2014Everlasting,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Everlasting secrecy in disadvantaged wireless environments against sophisticated eavesdroppers},
	journal = {48th Asilomar Conference on Signals, Systems and Computers},
	year = {2014},
	pages = {1994--1998},
}


@article{azadeh2013ISIT,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Artificial intersymbol interference (ISI) to exploit receiver imperfections for secrecy},
	journal = {IEEE International Symposium on Information Theory (ISIT)},
	year = {2013},
}


@article{azadeh2013Jsac,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
	journal = {IEEE Journal on Selected Areas in Communications},
	year = {2013},
	volume = {31},
	number = {9},
	pages = {1828--1839},
}


@article{azadeh2012Allerton,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Exploiting the non-commutativity of nonlinear operators for information-theoretic security in disadvantaged wireless environments},
	journal = {50th Annual Allerton Conference on Communication, Control, and Computing},
	year = {2012},
	pages = {233--240},
}


@article{azadeh2012Infocom,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
	journal = {IEEE INFOCOM},
	year = {2012},
	pages = {1179--1187},
}

@article{1corser2016evaluating,
	title={Evaluating Location Privacy in Vehicular Communications and Applications},
	author={Corser, George P and Fu, Huirong and Banihani, Abdelnasser},
	journal={IEEE Transactions on Intelligent Transportation Systems},
	volume={17},
	number={9},
	pages={2658-2667},
	year={2016},
	publisher={IEEE}
}
@article{2zhang2016designing,
	title={On Designing Satisfaction-Ratio-Aware Truthful Incentive Mechanisms for k-Anonymity Location Privacy},
	author={Zhang, Yuan and Tong, Wei and Zhong, Sheng},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={11},
	number={11},
	pages={2528--2541},
	year={2016},
	publisher={IEEE}
}
@article{3li2016privacy,
	title={Privacy-preserving Location Proof for Securing Large-scale Database-driven Cognitive Radio Networks},
	author={Li, Yi and Zhou, Lu and Zhu, Haojin and Sun, Limin},
	journal={IEEE Internet of Things Journal},
	volume={3},
	number={4},
	pages={563-571},
	year={2016},
	publisher={IEEE}
}
@article{4olteanu2016quantifying,
	title={Quantifying Interdependent Privacy Risks with Location Data},
	author={Olteanu, Alexandra-Mihaela and Huguenin, K{\'e}vin and Shokri, Reza and Humbert, Mathias and Hubaux, Jean-Pierre},
	journal={IEEE Transactions on Mobile Computing},
	year={2016},
	volume={PP},
	number={99},
	pages={1-1},
	publisher={IEEE}
}
@article{5yi2016practical,
	title={Practical Approximate k Nearest Neighbor Queries with Location and Query Privacy},
	author={Yi, Xun and Paulet, Russell and Bertino, Elisa and Varadharajan, Vijay},
	journal={IEEE Transactions on Knowledge and Data Engineering},
	volume={28},
	number={6},
	pages={1546--1559},
	year={2016},
	publisher={IEEE}
}
@article{6li2016privacy,
	title={Privacy Leakage of Location Sharing in Mobile Social Networks: Attacks and Defense},
	author={Li, Huaxin and Zhu, Haojin and Du, Suguo and Liang, Xiaohui and Shen, Xuemin},
	journal={IEEE Transactions on Dependable and Secure Computing},
	year={2016},
	volume={PP},
	number={99},
	publisher={IEEE}
}

@article{7murakami2016localization,
	title={Localization Attacks Using Matrix and Tensor Factorization},
	author={Murakami, Takao and Watanabe, Hajime},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={11},
	number={8},
	pages={1647--1660},
	year={2016},
	publisher={IEEE}
}
@article{8zurbaran2015near,
	title={Near-Rand: Noise-based Location Obfuscation Based on Random Neighboring Points},
	author={Zurbaran, Mayra Alejandra and Avila, Karen and Wightman, Pedro and Fernandez, Michael},
	journal={IEEE Latin America Transactions},
	volume={13},
	number={11},
	pages={3661--3667},
	year={2015},
	publisher={IEEE}
}

@article{9tan2014anti,
	title={An anti-tracking source-location privacy protection protocol in wsns based on path extension},
	author={Tan, Wei and Xu, Ke and Wang, Dan},
	journal={IEEE Internet of Things Journal},
	volume={1},
	number={5},
	pages={461--471},
	year={2014},
	publisher={IEEE}
}

@article{10peng2014enhanced,
	title={Enhanced Location Privacy Preserving Scheme in Location-Based Services},
	author={Peng, Tao and Liu, Qin and Wang, Guojun},
	journal={IEEE Systems Journal},
	year={2014},
	volume={PP},
	number={99},
	pages={1-12},
	publisher={IEEE}
}
@article{11dewri2014exploiting,
	title={Exploiting service similarity for privacy in location-based search queries},
	author={Dewri, Rinku and Thurimella, Ramakrisha},
	journal={IEEE Transactions on Parallel and Distributed Systems},
	volume={25},
	number={2},
	pages={374--383},
	year={2014},
	publisher={IEEE}
}

@article{12hwang2014novel,
	title={A novel time-obfuscated algorithm for trajectory privacy protection},
	author={Hwang, Ren-Hung and Hsueh, Yu-Ling and Chung, Hao-Wei},
	journal={IEEE Transactions on Services Computing},
	volume={7},
	number={2},
	pages={126--139},
	year={2014},
	publisher={IEEE}
}
@article{13puttaswamy2014preserving,
	title={Preserving location privacy in geosocial applications},
	author={Puttaswamy, Krishna PN and Wang, Shiyuan and Steinbauer, Troy and Agrawal, Divyakant and El Abbadi, Amr and Kruegel, Christopher and Zhao, Ben Y},
	journal={IEEE Transactions on Mobile Computing},
	volume={13},
	number={1},
	pages={159--173},
	year={2014},
	publisher={IEEE}
}

@article{14zhang2014privacy,
	title={Privacy quantification model based on the Bayes conditional risk in Location-Based Services},
	author={Zhang, Xuejun and Gui, Xiaolin and Tian, Feng and Yu, Si and An, Jian},
	journal={Tsinghua Science and Technology},
	volume={19},
	number={5},
	pages={452--462},
	year={2014},
	publisher={TUP}
}

@article{15bilogrevic2014privacy,
	title={Privacy-preserving optimal meeting location determination on mobile devices},
	author={Bilogrevic, Igor and Jadliwala, Murtuza and Joneja, Vishal and Kalkan, K{\"u}bra and Hubaux, Jean-Pierre and Aad, Imad},
	journal={IEEE transactions on information forensics and security},
	volume={9},
	number={7},
	pages={1141--1156},
	year={2014},
	publisher={IEEE}
}
@article{16haghnegahdar2014privacy,
	title={Privacy Risks in Publishing Mobile Device Trajectories},
	author={Haghnegahdar, Alireza and Khabbazian, Majid and Bhargava, Vijay K},
	journal={IEEE Wireless Communications Letters},
	volume={3},
	number={3},
	pages={241--244},
	year={2014},
	publisher={IEEE}
}
@article{17malandrino2014verification,
	title={Verification and inference of positions in vehicular networks through anonymous beaconing},
	author={Malandrino, Francesco and Borgiattino, Carlo and Casetti, Claudio and Chiasserini, Carla-Fabiana and Fiore, Marco and Sadao, Roberto},
	journal={IEEE Transactions on Mobile Computing},
	volume={13},
	number={10},
	pages={2415--2428},
	year={2014},
	publisher={IEEE}
}
@article{18shokri2014hiding,
	title={Hiding in the mobile crowd: Locationprivacy through collaboration},
	author={Shokri, Reza and Theodorakopoulos, George and Papadimitratos, Panos and Kazemi, Ehsan and Hubaux, Jean-Pierre},
	journal={IEEE transactions on dependable and secure computing},
	volume={11},
	number={3},
	pages={266--279},
	year={2014},
	publisher={IEEE}
}
@article{19freudiger2013non,
	title={Non-cooperative location privacy},
	author={Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
	journal={IEEE Transactions on Dependable and Secure Computing},
	volume={10},
	number={2},
	pages={84--98},
	year={2013},
	publisher={IEEE}
}
@article{20gao2013trpf,
	title={TrPF: A trajectory privacy-preserving framework for participatory sensing},
	author={Gao, Sheng and Ma, Jianfeng and Shi, Weisong and Zhan, Guoxing and Sun, Cong},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={8},
	number={6},
	pages={874--887},
	year={2013},
	publisher={IEEE}
}
@article{21ma2013privacy,
	title={Privacy vulnerability of published anonymous mobility traces},
	author={Ma, Chris YT and Yau, David KY and Yip, Nung Kwan and Rao, Nageswara SV},
	journal={IEEE/ACM Transactions on Networking},
	volume={21},
	number={3},
	pages={720--733},
	year={2013},
	publisher={IEEE}
}
@article{22niu2013pseudo,
	title={Pseudo-Location Updating System for privacy-preserving location-based services},
	author={Niu, Ben and Zhu, Xiaoyan and Chi, Haotian and Li, Hui},
	journal={China Communications},
	volume={10},
	number={9},
	pages={1--12},
	year={2013},
	publisher={IEEE}
}
@article{23dewri2013local,
	title={Local differential perturbations: Location privacy under approximate knowledge attackers},
	author={Dewri, Rinku},
	journal={IEEE Transactions on Mobile Computing},
	volume={12},
	number={12},
	pages={2360--2372},
	year={2013},
	publisher={IEEE}
}
@inproceedings{24kanoria2012tractable,
	title={Tractable bayesian social learning on trees},
	author={Kanoria, Yashodhan and Tamuz, Omer},
	booktitle={Information Theory Proceedings (ISIT), 2012 IEEE International Symposium on},
	pages={2721--2725},
	year={2012},
	organization={IEEE}
}
@inproceedings{25farias2005universal,
	title={A universal scheme for learning},
	author={Farias, Vivek F and Moallemi, Ciamac C and Van Roy, Benjamin and Weissman, Tsachy},
	booktitle={Proceedings. International Symposium on Information Theory, 2005. ISIT 2005.},
	pages={1158--1162},
	year={2005},
	organization={IEEE}
}
@inproceedings{26misra2013unsupervised,
	title={Unsupervised learning and universal communication},
	author={Misra, Vinith and Weissman, Tsachy},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={261--265},
	year={2013},
	organization={IEEE}
}
@inproceedings{27ryabko2013time,
	title={Time-series information and learning},
	author={Ryabko, Daniil},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={1392--1395},
	year={2013},
	organization={IEEE}
}
@inproceedings{28krzakala2013phase,
	title={Phase diagram and approximate message passing for blind calibration and dictionary learning},
	author={Krzakala, Florent and M{\'e}zard, Marc and Zdeborov{\'a}, Lenka},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={659--663},
	year={2013},
	organization={IEEE}
}
@inproceedings{29sakata2013sample,
	title={Sample complexity of Bayesian optimal dictionary learning},
	author={Sakata, Ayaka and Kabashima, Yoshiyuki},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={669--673},
	year={2013},
	organization={IEEE}
}
@inproceedings{30predd2004consistency,
	title={Consistency in a model for distributed learning with specialists},
	author={Predd, Joel B and Kulkarni, Sanjeev R and Poor, H Vincent},
	booktitle={IEEE International Symposium on Information Theory},
	year={2004},
	organization={IEEE}
}
@inproceedings{31nokleby2016rate,
	title={Rate-Distortion Bounds on Bayes Risk in Supervised Learning},
	author={Nokleby, Matthew and Beirami, Ahmad and Calderbank, Robert},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={2099-2103},
	year={2016},
	organization={IEEE}
}

@inproceedings{32le2016imperfect,
	title={Are imperfect reviews helpful in social learning?},
	author={Le, Tho Ngoc and Subramanian, Vijay G and Berry, Randall A},
	booktitle={Information Theory (ISIT), 2016 IEEE International Symposium on},
	pages={2089--2093},
	year={2016},
	organization={IEEE}
}
@inproceedings{33gadde2016active,
	title={Active Learning for Community Detection in Stochastic Block Models},
	author={Gadde, Akshay and Gad, Eyal En and Avestimehr, Salman and Ortega, Antonio},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={1889-1893},
	year={2016}
}
@inproceedings{34shakeri2016minimax,
	title={Minimax Lower Bounds for Kronecker-Structured Dictionary Learning},
	author={Shakeri, Zahra and Bajwa, Waheed U and Sarwate, Anand D},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={1148-1152},
	year={2016}
}
@article{35lee2015speeding,
	title={Speeding up distributed machine learning using codes},
	author={Lee, Kangwook and Lam, Maximilian and Pedarsani, Ramtin and Papailiopoulos, Dimitris and Ramchandran, Kannan},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={1143-1147},
	year={2016}
}
@article{36oneto2016statistical,
	title={Statistical Learning Theory and ELM for Big Social Data Analysis},
	author={Oneto, Luca and Bisio, Federica and Cambria, Erik and Anguita, Davide},
	journal={ieee CompUTATionAl inTelliGenCe mAGAzine},
	volume={11},
	number={3},
	pages={45--55},
	year={2016},
	publisher={IEEE}
}
@article{37lin2015probabilistic,
	title={Probabilistic approach to modeling and parameter learning of indirect drive robots from incomplete data},
	author={Lin, Chung-Yen and Tomizuka, Masayoshi},
	journal={IEEE/ASME Transactions on Mechatronics},
	volume={20},
	number={3},
	pages={1036--1045},
	year={2015},
	publisher={IEEE}
}
@article{38wang2016towards,
	title={Towards Bayesian Deep Learning: A Framework and Some Existing Methods},
	author={Wang, Hao and Yeung, Dit-Yan},
	journal={IEEE Transactions on Knowledge and Data Engineering},
	volume={PP},
	number={99},
	year={2016},
	publisher={IEEE}
}


%%%%%Informationtheoreticsecurity%%%%%%%%%%%%%%%%%%%%%%%




@inproceedings{Bloch2011PhysicalSecBook,
	title={Physical-Layer Security},
	author={M. Bloch and J. Barros},
	organization={Cambridge University Press},
	year={2011}
}



@inproceedings{Liang2009InfoSecBook,
	title={Information Theoretic Security},
	author={Y. Liang and H. V. Poor and S. Shamai (Shitz)},
	organization={Now Publishers Inc.},
	year={2009}
}


@inproceedings{Zhou2013PhysicalSecBook,
	title={Physical Layer Security in Wireless Communications},
	author={ X. Zhou and L. Song and Y. Zhang},
	organization={CRC Press},
	year={2013}
}

@article{Ni2012IEA,
	Author = {D. Ni and H. Liu and W. Ding and  Y. Xie and H. Wang and H. Pishro-Nik and Q. Yu},
	Journal = {IEA/AIE},
	Title = {Cyber-Physical Integration to Connect Vehicles for Transformed Transportation Safety and Efficiency},
	Year = {2012}}



@inproceedings{Ni2012Inproceedings,
	Author = {D. Ni, H. Liu, Y. Xie, W. Ding, H. Wang, H. Pishro-Nik, Q. Yu and M. Ferreira},
	Booktitle = {Spring Simulation Multiconference},
	Date-Added = {2016-09-04 14:18:42 +0000},
	Date-Modified = {2016-09-06 16:22:14 +0000},
	Title = {Virtual Lab of Connected Vehicle Technology},
	Year = {2012}}

@inproceedings{Ni2012Inproceedings,
	Author = {D. Ni, H. Liu, W. Ding, Y. Xie, H. Wang, H. Pishro-Nik and Q. Yu,},
	Booktitle = {IEA/AIE},
	Date-Added = {2016-09-04 09:11:02 +0000},
	Date-Modified = {2016-09-06 14:46:53 +0000},
	Title = {Cyber-Physical Integration to Connect Vehicles for Transformed Transportation Safety and Efficiency},
	Year = {2012}}


@article{Nekoui_IJIPT_2009,
	Author = {M. Nekoui and D. Ni and H. Pishro-Nik and R. Prasad and M. Kanjee and H. Zhu and T. Nguyen},
	Journal = {International Journal of Internet Protocol Technology (IJIPT)},
	Number = {3},
	Pages = {},
	Publisher = {},
	Title = {Development of a VII-Enabled Prototype Intersection Collision Warning System},
	Volume = {4},
	Year = {2009}}


@inproceedings{Pishro_Ganz_Ni,
	Author = {H. Pishro-Nik, A. Ganz, and Daiheng Ni},
	Booktitle = {Forty-Fifth Annual Allerton Conference on Communication, Control, and Computing. Allerton House, Monticello, IL},
	Date-Added = {},
	Date-Modified = {},
	Number = {},
	Pages = {},
	Title = {The capacity of vehicular ad hoc networks},
	Volume = {},
	Year = {September 26-28, 2007}}

@inproceedings{Leow_Pishro_Ni_1,
	Author = {W. L. Leow, H. Pishro-Nik and Daiheng Ni},
	Booktitle = {IEEE Global Telecommunications Conference, Washington, D.C.},
	Date-Added = {},
	Date-Modified = {},
	Number = {},
	Pages = {},
	Title = {Delay and Energy Tradeoff in Multi-state Wireless Sensor Networks},
	Volume = {},
	Year = {November 26-30, 2007}}


@misc{UMass-Trans,
	title = {{UMass Transportation Center}},
	note = {\url{http://www.umasstransportationcenter.org/}},
}


@inproceedings{Haenggi2013book,
	title={Stochastic geometry for wireless networks},
	author={M. Haenggi},
	organization={Cambridge Uinversity Press},
	year={2013}
}


%%%%%%%%%%%%%%%%personalization%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{osma2015,
	title={Impact of Time-to-Collision Information on Driving Behavior in Connected Vehicle Environments Using A Driving Simulator Test Bed},
	journal{Journal of Traffic and Logistics Engineering},
	author={Osama A. Osman, Julius Codjoe, and Sherif Ishak},
	volume={3},
	number={1},
	pages={18--24},
	year={2015}
}


@article{charisma2010,
	title={Dynamic Latent Plan Models},
	author={Charisma F. Choudhurya, Moshe Ben-Akivab and Maya Abou-Zeid},
	journal={Journal of Choice Modelling},
	volume={3},
	number={2},
	pages={50--70},
	year={2010},
	publisher={Elsvier}
}


@misc{noble2014,
	author = {A. M. Noble, Shane B. McLaughlin, Zachary R. Doerzaph and Thomas A. Dingus},
	title = {Crowd-sourced Connected-vehicle Warning Algorithm using Naturalistic Driving Data},
	howpublished = {Downloaded from \url{http://hdl.handle.net/10919/53978}},
	
	month = August,
	year = 2014
}


@phdthesis{charisma2007,
	title    = {Modeling Driving Decisions with Latent Plans},
	school   = {Massachusetts Institute of Technology },
	author   = {Charisma Farheen Choudhury},
	year     = {2007}, %other attributes omitted
}


@article{chrysler2015,
	title={Cost of Warning of Unseen Threats:Unintended Consequences of Connected Vehicle Alerts},
	author={S. T. Chrysler, J. M. Cooper and D. C. Marshall},
	journal={Transportation Research Record: Journal of the Transportation Research Board},
	volume={2518},
	pages={79--85},
	year={2015},
}

@misc{nsf_cps,
	title = {Cyber-Physical Systems (CPS) PROGRAM SOLICITATION NSF 17-529},
	howpublished = {Downloaded from \url{https://www.nsf.gov/publications/pub_summ.jsp?WT.z_pims_id=503286&ods_key=nsf17529}},
}



%%%%%%%%%%%%%%IOT%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




@article{FTC2015,
	title={Internet of Things: Privacy and Security in a Connected World},
	author={FTC Staff Report},
	year={2015}
}



%% Saved with string encoding Unicode (UTF-8)
@inproceedings{1zhou2014security,
	title={Security/privacy of wearable fitness tracking {I}o{T} devices},
	author={Zhou, Wei and Piramuthu, Selwyn},
	booktitle={Information Systems and Technologies (CISTI), 2014 9th Iberian Conference on},
	pages={1--5},
	year={2014},
	organization={IEEE}
}

@article{2nia2016comprehensive,
	title={A comprehensive study of security of internet-of-things},
	author={Mohsenia, Arsalan and Jha, Niraj K},
	journal={IEEE Transactions on Emerging Topics in Computing},
	volum={5},
	number={4},
	pages={586--602},
	year={2017},
	publisher={IEEE}
}

@inproceedings{3ukil2014iot,
	title={{I}o{T}-privacy: To be private or not to be private},
	author={Ukil, Arijit and Bandyopadhyay, Soma and Pal, Arpan},
	booktitle={Computer Communications Workshops (INFOCOM WKSHPS), IEEE Conference on},
	pages={123--124},
	year={2014},
	organization={IEEE}
}

@article{4arias2015privacy,
	title={Privacy and security in internet of things and wearable devices},
	author={Arias, Orlando and Wurm, Jacob and Hoang, Khoa and Jin, Yier},
	journal={IEEE Transactions on Multi-Scale Computing Systems},
	volume={1},
	number={2},
	pages={99--109},
	year={2015},
	publisher={IEEE}
}
@inproceedings{5ullah2016novel,
	title={A novel model for preserving Location Privacy in Internet of Things},
	author={Ullah, Ikram and Shah, Munam Ali},
	booktitle={Automation and Computing (ICAC), 2016 22nd International Conference on},
	pages={542--547},
	year={2016},
	organization={IEEE}
}
@inproceedings{6sathishkumar2016enhanced,
	title={Enhanced location privacy algorithm for wireless sensor network in Internet of Things},
	author={Sathishkumar, J and Patel, Dhiren R},
	booktitle={Internet of Things and Applications (IOTA), International Conference on},
	pages={208--212},
	year={2016},
	organization={IEEE}
}
@inproceedings{7zhou2012preserving,
	title={Preserving sensor location privacy in internet of things},
	author={Zhou, Liming and Wen, Qiaoyan and Zhang, Hua},
	booktitle={Computational and Information Sciences (ICCIS), 2012 Fourth International Conference on},
	pages={856--859},
	year={2012},
	organization={IEEE}
}

@inproceedings{8ukil2015privacy,
	title={Privacy for {I}o{T}: Involuntary privacy enablement for smart energy systems},
	author={Ukil, Arijit and Bandyopadhyay, Soma and Pal, Arpan},
	booktitle={Communications (ICC), 2015 IEEE International Conference on},
	pages={536--541},
	year={2015},
	organization={IEEE}
}

@inproceedings{9dalipi2016security,
	title={Security and Privacy Considerations for {I}o{T} Application on Smart Grids: Survey and Research Challenges},
	author={Dalipi, Fisnik and Yayilgan, Sule Yildirim},
	booktitle={Future Internet of Things and Cloud Workshops (FiCloudW), IEEE International Conference on},
	pages={63--68},
	year={2016},
	organization={IEEE}
}
@inproceedings{10harris2016security,
	title={Security and Privacy in Public {I}o{T} Spaces},
	author={Harris, Albert F and Sundaram, Hari and Kravets, Robin},
	booktitle={Computer Communication and Networks (ICCCN), 2016 25th International Conference on},
	pages={1--8},
	year={2016},
	organization={IEEE}
}

@inproceedings{11al2015security,
	title={Security and privacy framework for ubiquitous healthcare {I}o{T} devices},
	author={Al Alkeem, Ebrahim and Yeun, Chan Yeob and Zemerly, M Jamal},
	booktitle={Internet Technology and Secured Transactions (ICITST), 2015 10th International Conference for},
	pages={70--75},
	year={2015},
	organization={IEEE}
}
@inproceedings{12sivaraman2015network,
	title={Network-level security and privacy control for smart-home {I}o{T} devices},
	author={Sivaraman, Vijay and Gharakheili, Hassan Habibi and Vishwanath, Arun and Boreli, Roksana and Mehani, Olivier},
	booktitle={Wireless and Mobile Computing, Networking and Communications (WiMob), 2015 IEEE 11th International Conference on},
	pages={163--167},
	year={2015},
	organization={IEEE}
}

@inproceedings{13srinivasan2016privacy,
	title={Privacy conscious architecture for improving emergency response in smart cities},
	author={Srinivasan, Ramya and Mohan, Apurva and Srinivasan, Priyanka},
	booktitle={Smart City Security and Privacy Workshop (SCSP-W), 2016},
	pages={1--5},
	year={2016},
	organization={IEEE}
}
@inproceedings{14sadeghi2015security,
	title={Security and privacy challenges in industrial internet of things},
	author={Sadeghi, Ahmad-Reza and Wachsmann, Christian and Waidner, Michael},
	booktitle={Design Automation Conference (DAC), 2015 52nd ACM/EDAC/IEEE},
	pages={1--6},
	year={2015},
	organization={IEEE}
}
@inproceedings{15otgonbayar2016toward,
	title={Toward Anonymizing {I}o{T} Data Streams via Partitioning},
	author={Otgonbayar, Ankhbayar and Pervez, Zeeshan and Dahal, Keshav},
	booktitle={Mobile Ad Hoc and Sensor Systems (MASS), 2016 IEEE 13th International Conference on},
	pages={331--336},
	year={2016},
	organization={IEEE}
}
@inproceedings{16rutledge2016privacy,
	title={Privacy Impacts of {I}o{T} Devices: A SmartTV Case Study},
	author={Rutledge, Richard L and Massey, Aaron K and Ant{\'o}n, Annie I},
	booktitle={Requirements Engineering Conference Workshops (REW), IEEE International},
	pages={261--270},
	year={2016},
	organization={IEEE}
}

@inproceedings{17andrea2015internet,
	title={Internet of Things: Security vulnerabilities and challenges},
	author={Andrea, Ioannis and Chrysostomou, Chrysostomos and Hadjichristofi, George},
	booktitle={Computers and Communication (ISCC), 2015 IEEE Symposium on},
	pages={180--187},
	year={2015},
	organization={IEEE}
}






























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@misc{epfl-mobility-20090224,
	author = {Michal Piorkowski and Natasa Sarafijanovic-Djukic and Matthias Grossglauser},
	title = {{CRAWDAD} dataset epfl/mobility (v. 2009-02-24)},
	howpublished = {Downloaded from \url{http://crawdad.org/epfl/mobility/20090224}},
	doi = {10.15783/C7J010},
	month = feb,
	year = 2009
}

@misc{roma-taxi-20140717,
	author = {Lorenzo Bracciale and Marco Bonola and Pierpaolo Loreti and Giuseppe Bianchi and Raul Amici and Antonello Rabuffi},
	title = {{CRAWDAD} dataset roma/taxi (v. 2014-07-17)},
	howpublished = {Downloaded from \url{http://crawdad.org/roma/taxi/20140717}},
	doi = {10.15783/C7QC7M},
	month = jul,
	year = 2014
}

@misc{rice-ad_hoc_city-20030911,
	author = {Jorjeta G. Jetcheva and Yih-Chun Hu and Santashil PalChaudhuri and Amit Kumar Saha and David B. Johnson},
	title = {{CRAWDAD} dataset rice/ad\_hoc\_city (v. 2003-09-11)},
	howpublished = {Downloaded from \url{http://crawdad.org/rice/ad_hoc_city/20030911}},
	doi = {10.15783/C73K5B},
	month = sep,
	year = 2003
}

@misc{china:2012,
	author = {Microsoft Research Asia},
	title = {GeoLife GPS Trajectories},
	year = {2012},
	howpublished= {\url{https://www.microsoft.com/en-us/download/details.aspx?id=52367}},
}


@misc{china:2011,
	ALTauthor = {Microsoft Research Asia)},
	ALTeditor = {},
	title = {GeoLife GPS Trajectories,
	year = {2012},
	url = {https://www.microsoft.com/en-us/download/details.aspx?id=52367},
	}
	
	
	@misc{longversion,
	author = {N. Takbiri and A. Houmansadr and D.L. Goeckel and H. Pishro-Nik},
	title = {{Limits of Location Privacy under Anonymization and Obfuscation}},
	howpublished = "\url{http://www.ecs.umass.edu/ece/pishro/Papers/ISIT_2017-2.pdf}",
	year = 2017,
	month= "January",
	note = "Summarized version submitted to IEEE ISIT 2017"
	}
	
	@misc{isit_ke,
	author = {K. Li and D. Goeckel and H. Pishro-Nik},
	title = {{Bayesian Time Series Matching and Privacy}},
	note = "submitted to IEEE ISIT 2017"
	}
	
	@article{matching,
	title={Asymptotically Optimal Matching of Multiple Sequences to Source Distributions and Training Sequences},
	author={Jayakrishnan Unnikrishnan},
	journal={ IEEE Transactions on Information Theory},
	volume={61},
	number={1},
	pages={452-468},
	year={2015},
	publisher={IEEE}
	}
	
	
	@article{Naini2016,
	Author = {F. Naini and J. Unnikrishnan and P. Thiran and M. Vetterli},
	Journal = {IEEE Transactions on Information Forensics and Security},
	Publisher = {IEEE},
	Title = {Where You Are Is Who You Are: User Identification by Matching Statistics},
	volume={11},
	number={2},
	pages={358--372},
	Year = {2016}
	}
	
	
	
	@inproceedings{holowczak2015cachebrowser,
	title={{CacheBrowser: Bypassing Chinese Censorship without Proxies Using Cached Content}},
	author={Holowczak, John and Houmansadr, Amir},
	booktitle={Proceedings of the 22nd ACM SIGSAC Conference on Computer and Communications Security},
	pages={70--83},
	year={2015},
	organization={ACM}
	}
	@misc{cb-website,
	Howpublished = {\url{https://cachebrowser.net/#/}},
	Title = {{CacheBrowser}},
	key={cachebrowser}
	}
	
	@inproceedings{GameOfDecoys,
	title={{GAME OF DECOYS: Optimal Decoy Routing Through Game Theory}},
	author={Milad Nasr and Amir Houmansadr},
	booktitle={The $23^{rd}$ ACM Conference on Computer and Communications Security (CCS)},
	year={2016}
	}
	
	@inproceedings{CDNReaper,
	title={{Practical Censorship Evasion Leveraging Content Delivery Networks}},
	author={Hadi Zolfaghari and Amir Houmansadr},
	booktitle={The $23^{rd}$ ACM Conference on Computer and Communications Security (CCS)},
	year={2016}
	}
	
	@misc{Leberknight2010,
	Author = {Leberknight, C. and Chiang, M. and Poor, H. and Wong, F.},
	Howpublished = {\url{http://www.princeton.edu/~chiangm/anticensorship.pdf}},
	Title = {{A Taxonomy of Internet Censorship and Anti-censorship}},
	Year = {2010}}
	
	@techreport{ultrasurf-analysis,
	Author = {Appelbaum, Jacob},
	Institution = {The Tor Project},
	Title = {{Technical analysis of the Ultrasurf proxying software}},
	Url = {http://scholar.google.com/scholar?hl=en\&btnG=Search\&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software\#0},
	Year = {2012},
	Bdsk-Url-1 = {http://scholar.google.com/scholar?hl=en%5C&btnG=Search%5C&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software%5C#0}}
	
	@misc{gifc:07,
	Howpublished = {\url{http://www.internetfreedom.org/archive/Defeat\_Internet\_Censorship\_White\_Paper.pdf}},
	Key = {defeatcensorship},
	Publisher = {Global Internet Freedom Consortium (GIFC)},
	Title = {{Defeat Internet Censorship: Overview of Advanced Technologies and Products}},
	Type = {White Paper},
	Year = {2007}}
	
	@article{pan2011survey,
	Author = {Pan, J. and Paul, S. and Jain, R.},
	Journal = {Communications Magazine, IEEE},
	Number = {7},
	Pages = {26--36},
	Publisher = {IEEE},
	Title = {{A Survey of the Research on Future Internet Architectures}},
	Volume = {49},
	Year = {2011}}
	
	@misc{nsf-fia,
	Howpublished = {\url{http://www.nets-fia.net/}},
	Key = {FIA},
	Title = {{NSF Future Internet Architecture Project}}}
	
	@misc{NDN,
	Howpublished = {\url{http://www.named- data.net}},
	Key = {NDN},
	Title = {{Named Data Networking Project}}}
	
	@inproceedings{MobilityFirst,
	Author = {Seskar, I. and Nagaraja, K. and Nelson, S. and Raychaudhuri, D.},
	Booktitle = {Asian Internet Engineering Conference},
	Title = {{Mobilityfirst Future internet Architecture Project}},
	Year = {2011}}
	
	@incollection{NEBULA,
	Author = {Anderson, T. and Birman, K. and Broberg, R. and Caesar, M. and Comer, D. and Cotton, C. and Freedman, M.~J. and Haeberlen, A. and Ives, Z.~G. and Krishnamurthy, A. and others},
	Booktitle = {The Future Internet},
	Pages = {16--26},
	Publisher = {Springer},
	Title = {{The NEBULA Future Internet Architecture}},
	Year = {2013}}
	
	@inproceedings{XIA,
	Author = {Anand, A. and Dogar, F. and Han, D. and Li, B. and Lim, H. and Machado, M. and Wu, W. and Akella, A. and Andersen, D.~G. and Byers, J.~W. and others},
	Booktitle = {ACM Workshop on Hot Topics in Networks},
	Pages = {2},
	Title = {{XIA: An Architecture for an Evolvable and Trustworthy Internet}},
	Year = {2011}}
	
	@inproceedings{ChoiceNet,
	Author = {Rouskas, G.~N. and Baldine, I. and Calvert, K.~L. and Dutta, R. and Griffioen, J. and Nagurney, A. and Wolf, T.},
	Booktitle = {ONDM},
	Title = {{ChoiceNet: Network Innovation Through Choice}},
	Year = {2013}}
	
	@misc{nsf-find,
	Howpublished = {http://www.nets-find.net/},
	Title = {{NSF NeTS FIND Initiative}}}
	
	@article{traid,
	Author = {Cheriton, D.~R. and Gritter, M.},
	Title = {{TRIAD: A New Next-Generation Internet Architecture}},
	Year = {2000}}
	
	@inproceedings{dona,
	Author = {Koponen, T. and Chawla, M. and Chun, B-G. and Ermolinskiy, A. and Kim, K.~H. and Shenker, S. and Stoica, I.},
	Booktitle = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Organization = {ACM},
	Pages = {181--192},
	Title = {{A Data-Oriented (and Beyond) Network Architecture}},
	Volume = {37},
	Year = {2007}}
	
	@misc{ultrasurf,
	Howpublished = {\url{http://www.ultrareach.com}},
	Key = {ultrasurf},
	Title = {{Ultrasurf}}}
	
	@misc{tor-bridge,
	Author = {Dingledine, R. and Mathewson, N.},
	Howpublished = {\url{https://svn.torproject.org/svn/projects/design-paper/blocking.html}},
	Title = {{Design of a Blocking-Resistant Anonymity System}}}
	
	@inproceedings{McLachlanH09,
	Author = {J. McLachlan and N. Hopper},
	Booktitle = {WPES},
	Title = {{On the Risks of Serving Whenever You Surf: Vulnerabilities in Tor's Blocking Resistance Design}},
	Year = {2009}}
	
	@inproceedings{mahdian2010,
	Author = {Mahdian, M.},
	Booktitle = {{Fun with Algorithms}},
	Title = {{Fighting Censorship with Algorithms}},
	Year = {2010}}
	
	@inproceedings{McCoy2011,
	Author = {McCoy, D. and Morales, J.~A. and Levchenko, K.},
	Booktitle = {FC},
	Title = {{Proximax: A Measurement Based System for Proxies Dissemination}},
	Year = {2011}}
	
	@inproceedings{Sovran2008,
	Author = {Sovran, Y. and Libonati, A. and Li, J.},
	Booktitle = {IPTPS},
	Title = {{Pass it on: Social Networks Stymie Censors}},
	Year = {2008}}
	
	@inproceedings{rbridge,
	Author = {Wang, Q. and Lin, Zi and Borisov, N. and Hopper, N.},
	Booktitle = {{NDSS}},
	Title = {{rBridge: User Reputation based Tor Bridge Distribution with Privacy Preservation}},
	Year = {2013}}
	
	@inproceedings{telex,
	Author = {Wustrow, E. and Wolchok, S. and Goldberg, I. and Halderman, J.},
	Booktitle = {{USENIX Security}},
	Title = {{Telex: Anticensorship in the Network Infrastructure}},
	Year = {2011}}
	
	@inproceedings{cirripede,
	Author = {Houmansadr, A. and Nguyen, G. and Caesar, M. and Borisov, N.},
	Booktitle = {CCS},
	Title = {{Cirripede: Circumvention Infrastructure Using Router Redirection with Plausible Deniability}},
	Year = {2011}}
	
	@inproceedings{decoyrouting,
	Author = {Karlin, J. and Ellard, D. and Jackson, A. and Jones, C. and Lauer, G. and Mankins, D. and Strayer, W.},
	Booktitle = {{FOCI}},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = {2011}}
	
	@inproceedings{routing-around-decoys,
	Author = {M.~Schuchard and J.~Geddes and C.~Thompson and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Routing Around Decoys}},
	Year = {2012}}
	
	@inproceedings{parrot,
	Author = {A. Houmansadr and C. Brubaker and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{The Parrot is Dead: Observing Unobservable Network Communications}},
	Year = {2013}}
	
	@misc{knock,
	Author = {T. Wilde},
	Howpublished = {\url{https://blog.torproject.org/blog/knock-knock-knockin-bridges-doors}},
	Title = {{Knock Knock Knockin' on Bridges' Doors}},
	Year = {2012}}
	
	@inproceedings{china-tor,
	Author = {Winter, P. and Lindskog, S.},
	Booktitle = {{FOCI}},
	Title = {{How the Great Firewall of China Is Blocking Tor}},
	Year = {2012}}
	
	@misc{discover-bridge,
	Howpublished = {\url{https://blog.torproject.org/blog/research-problems-ten-ways-discover-tor-bridges}},
	Key = {tenways},
	Title = {{Ten Ways to Discover Tor Bridges}}}
	
	@inproceedings{freewave,
	Author = {A.~Houmansadr and T.~Riedl and N.~Borisov and A.~Singer},
	Booktitle = {{NDSS}},
	Title = {{I Want My Voice to Be Heard: IP over Voice-over-IP for Unobservable Censorship Circumvention}},
	Year = 2013}
	
	@inproceedings{censorspoofer,
	Author = {Q. Wang and X. Gong and G. Nguyen and A. Houmansadr and N. Borisov},
	Booktitle = {CCS},
	Title = {{CensorSpoofer: Asymmetric Communication Using IP Spoofing for Censorship-Resistant Web Browsing}},
	Year = {2012}}
	
	@inproceedings{skypemorph,
	Author = {H. Moghaddam and B. Li and M. Derakhshani and I. Goldberg},
	Booktitle = {CCS},
	Title = {{SkypeMorph: Protocol Obfuscation for Tor Bridges}},
	Year = {2012}}
	
	@inproceedings{stegotorus,
	Author = {Weinberg, Z. and Wang, J. and Yegneswaran, V. and Briesemeister, L. and Cheung, S. and Wang, F. and Boneh, D.},
	Booktitle = {CCS},
	Title = {{StegoTorus: A Camouflage Proxy for the Tor Anonymity System}},
	Year = {2012}}
	
	@techreport{dust,
	Author = {{B.~Wiley}},
	Howpublished = {\url{http://blanu.net/ Dust.pdf}},
	Institution = {School of Information, University of Texas at Austin},
	Title = {{Dust: A Blocking-Resistant Internet Transport Protocol}},
	Year = {2011}}
	
	@inproceedings{FTE,
	Author = {K.~Dyer and S.~Coull and T.~Ristenpart and T.~Shrimpton},
	Booktitle = {CCS},
	Title = {{Protocol Misidentification Made Easy with Format-Transforming Encryption}},
	Year = {2013}}
	
	@inproceedings{fp,
	Author = {Fifield, D. and Hardison, N. and Ellithrope, J. and Stark, E. and Dingledine, R. and Boneh, D. and Porras, P.},
	Booktitle = {PETS},
	Title = {{Evading Censorship with Browser-Based Proxies}},
	Year = {2012}}
	
	@misc{obfsproxy,
	Howpublished = {\url{https://www.torproject.org/projects/obfsproxy.html.en}},
	Key = {obfsproxy},
	Publisher = {The Tor Project},
	Title = {{A Simple Obfuscating Proxy}}}
	
	@inproceedings{Tor-instead-of-IP,
	Author = {Liu, V. and Han, S. and Krishnamurthy, A. and Anderson, T.},
	Booktitle = {HotNets},
	Title = {{Tor instead of IP}},
	Year = {2011}}
	
	@misc{roger-slides,
	Howpublished = {\url{https://svn.torproject.org/svn/projects/presentations/slides-28c3.pdf}},
	Key = {torblocking},
	Title = {{How Governments Have Tried to Block Tor}}}
	
	@inproceedings{infranet,
	Author = {Feamster, N. and Balazinska, M. and Harfst, G. and Balakrishnan, H. and Karger, D.},
	Booktitle = {USENIX Security},
	Title = {{Infranet: Circumventing Web Censorship and Surveillance}},
	Year = {2002}}
	
	@inproceedings{collage,
	Author = {S.~Burnett and N.~Feamster and S.~Vempala},
	Booktitle = {USENIX Security},
	Title = {{Chipping Away at Censorship Firewalls with User-Generated Content}},
	Year = {2010}}
	
	@article{anonymizer,
	Author = {Boyan, J.},
	Journal = {Computer-Mediated Communication Magazine},
	Month = sep,
	Number = {9},
	Title = {{The Anonymizer: Protecting User Privacy on the Web}},
	Volume = {4},
	Year = {1997}}
	
	@article{schulze2009internet,
	Author = {Schulze, H. and Mochalski, K.},
	Journal = {IPOQUE Report},
	Pages = {351--362},
	Title = {Internet Study 2008/2009},
	Volume = {37},
	Year = {2009}}
	
	@inproceedings{cya-ccs13,
	Author = {J.~Geddes and M.~Schuchard and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Cover Your ACKs: Pitfalls of Covert Channel Censorship Circumvention}},
	Year = {2013}}
	
	@inproceedings{andana,
	Author = {DiBenedetto, S. and Gasti, P. and Tsudik, G. and Uzun, E.},
	Booktitle = {{NDSS}},
	Title = {{ANDaNA: Anonymous Named Data Networking Application}},
	Year = {2012}}
	
	@inproceedings{darkly,
	Author = {Jana, S. and Narayanan, A. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{A Scanner Darkly: Protecting User Privacy From Perceptual Applications}},
	Year = {2013}}
	
	@inproceedings{NS08,
	Author = {A.~Narayanan and V.~Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {Robust de-anonymization of large sparse datasets},
	Year = {2008}}
	
	@inproceedings{NS09,
	Author = {Arvind Narayanan and Vitaly Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {De-anonymizing Social Networks},
	Year = {2009}}
	
	@inproceedings{memento,
	Author = {Jana, S. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{Memento: Learning secrets from process footprints}},
	Year = {2012}}
	
	@misc{plugtor,
	Howpublished = {\url{https://www.torproject.org/docs/pluggable-transports.html.en}},
	Key = {PluggableTransports},
	Publisher = {The Tor Project},
	Title = {{Tor: Pluggable transports}}}
	
	@misc{psiphon,
	Author = {J.~Jia and P.~Smith},
	Howpublished = {\url{http://www.cdf.toronto.edu/~csc494h/reports/2004-fall/psiphon_ae.html}},
	Title = {{Psiphon: Analysis and Estimation}},
	Year = 2004}
	
	@misc{china-github,
	Howpublished = {\url{http://mobile.informationweek.com/80269/show/72e30386728f45f56b343ddfd0fdb119/}},
	Key = {github},
	Title = {{China's GitHub Censorship Dilemma}}}
	
	@inproceedings{txbox,
	Author = {Jana, S. and Porter, D. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{TxBox: Building Secure, Efficient Sandboxes with System Transactions}},
	Year = {2011}}
	
	@inproceedings{airavat,
	Author = {I. Roy and S. Setty and A. Kilzer and V. Shmatikov and E. Witchel},
	Booktitle = {NSDI},
	Title = {{Airavat: Security and Privacy for MapReduce}},
	Year = {2010}}
	
	@inproceedings{osdi12,
	Author = {A. Dunn and M. Lee and S. Jana and S. Kim and M. Silberstein and Y. Xu and V. Shmatikov and E. Witchel},
	Booktitle = {OSDI},
	Title = {{Eternal Sunshine of the Spotless Machine: Protecting Privacy with Ephemeral Channels}},
	Year = {2012}}
	
	@inproceedings{ymal,
	Author = {J. Calandrino and A. Kilzer and A. Narayanan and E. Felten and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{``You Might Also Like:'' Privacy Risks of Collaborative Filtering}},
	Year = {2011}}
	
	@inproceedings{srivastava11,
	Author = {V. Srivastava and M. Bond and K. McKinley and V. Shmatikov},
	Booktitle = {PLDI},
	Title = {{A Security Policy Oracle: Detecting Security Holes Using Multiple API Implementations}},
	Year = {2011}}
	
	@inproceedings{chen-oakland10,
	Author = {Chen, S. and Wang, R. and Wang, X. and Zhang, K.},
	Booktitle = {IEEE S\&P},
	Title = {{Side-Channel Leaks in Web Applications: A Reality Today, a Challenge Tomorrow}},
	Year = {2010}}
	
	@book{kerck,
	Author = {Kerckhoffs, A.},
	Publisher = {University Microfilms},
	Title = {{La cryptographie militaire}},
	Year = {1978}}
	
	@inproceedings{foci11,
	Author = {J. Karlin and D. Ellard and A.~Jackson and C.~ Jones and G. Lauer and D. Mankins and W.~T.~Strayer},
	Booktitle = {FOCI},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = 2011}
	
	@inproceedings{sun02,
	Author = {Sun, Q. and Simon, D.~R. and Wang, Y. and Russell, W. and Padmanabhan, V. and Qiu, L.},
	Booktitle = {IEEE S\&P},
	Title = {{Statistical Identification of Encrypted Web Browsing Traffic}},
	Year = {2002}}
	
	@inproceedings{danezis,
	Author = {Murdoch, S.~J. and Danezis, G.},
	Booktitle = {IEEE S\&P},
	Title = {{Low-Cost Traffic Analysis of Tor}},
	Year = {2005}}
	
	@inproceedings{pakicensorship,
	Author = {Z.~Nabi},
	Booktitle = {FOCI},
	Title = {The Anatomy of {Web} Censorship in {Pakistan}},
	Year = {2013}}
	
	@inproceedings{irancensorship,
	Author = {S.~Aryan and H.~Aryan and A.~Halderman},
	Booktitle = {FOCI},
	Title = {Internet Censorship in {Iran}: {A} First Look},
	Year = {2013}}
	
	@inproceedings{ford10efficient,
	Author = {Amittai Aviram and Shu-Chun Weng and Sen Hu and Bryan Ford},
	Booktitle = {\bibconf[9th]{OSDI}{USENIX Symposium on Operating Systems Design and Implementation}},
	Location = {Vancouver, BC, Canada},
	Month = oct,
	Title = {Efficient System-Enforced Deterministic Parallelism},
	Year = 2010}
	
	@inproceedings{ford10determinating,
	Author = {Amittai Aviram and Sen Hu and Bryan Ford and Ramakrishna Gummadi},
	Booktitle = {\bibconf{CCSW}{ACM Cloud Computing Security Workshop}},
	Location = {Chicago, IL},
	Month = oct,
	Title = {Determinating Timing Channels in Compute Clouds},
	Year = 2010}
	
	@inproceedings{ford12plugging,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Plugging Side-Channel Leaks with Timing Information Flow Control},
	Year = 2012}
	
	@inproceedings{ford12icebergs,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Icebergs in the Clouds: the {\em Other} Risks of Cloud Computing},
	Year = 2012}
	
	@misc{mullenize,
	Author = {Washington Post},
	Howpublished = {\url{http://apps.washingtonpost.com/g/page/world/gchq-report-on-mullenize-program-to-stain-anonymous-electronic-traffic/502/}},
	Month = {oct},
	Title = {{GCHQ} report on {`MULLENIZE'} program to `stain' anonymous electronic traffic},
	Year = {2013}}
	
	@inproceedings{shue13street,
	Author = {Craig A. Shue and Nathanael Paul and Curtis R. Taylor},
	Booktitle = {\bibbrev[7th]{WOOT}{USENIX Workshop on Offensive Technologies}},
	Month = aug,
	Title = {From an {IP} Address to a Street Address: Using Wireless Signals to Locate a Target},
	Year = 2013}
	
	@inproceedings{knockel11three,
	Author = {Jeffrey Knockel and Jedidiah R. Crandall and Jared Saia},
	Booktitle = {\bibbrev{FOCI}{USENIX Workshop on Free and Open Communications on the Internet}},
	Location = {San Francisco, CA},
	Month = aug,
	Year = 2011}
	
	@misc{rfc4960,
	Author = {R. {Stewart, ed.}},
	Month = sep,
	Note = {RFC 4960},
	Title = {Stream Control Transmission Protocol},
	Year = 2007}
	
	@inproceedings{ford07structured,
	Author = {Bryan Ford},
	Booktitle = {\bibbrev{SIGCOMM}{ACM SIGCOMM}},
	Location = {Kyoto, Japan},
	Month = aug,
	Title = {Structured Streams: a New Transport Abstraction},
	Year = {2007}}
	
	@misc{spdy,
	Author = {Google, Inc.},
	Note = {\url{http://www.chromium.org/spdy/spdy-whitepaper}},
	Title = {{SPDY}: An Experimental Protocol For a Faster {Web}}}
	
	@misc{quic,
	Author = {Jim Roskind},
	Month = jun,
	Note = {\url{http://blog.chromium.org/2013/06/experimenting-with-quic.html}},
	Title = {Experimenting with {QUIC}},
	Year = 2013}
	
	@misc{podjarny12not,
	Author = {G.~Podjarny},
	Month = jun,
	Note = {\url{http://www.guypo.com/technical/not-as-spdy-as-you-thought/}},
	Title = {{Not as SPDY as You Thought}},
	Year = 2012}
	
	@inproceedings{cor,
	Author = {Jones, N.~A. and Arye, M. and Cesareo, J. and Freedman, M.~J.},
	Booktitle = {FOCI},
	Title = {{Hiding Amongst the Clouds: A Proposal for Cloud-based Onion Routing}},
	Year = {2011}}
	
	@misc{torcloud,
	Howpublished = {\url{https://cloud.torproject.org/}},
	Key = {tor cloud},
	Title = {{The Tor Cloud Project}}}
	
	@inproceedings{scramblesuit,
	Author = {Philipp Winter and Tobias Pulls and Juergen Fuss},
	Booktitle = {WPES},
	Title = {{ScrambleSuit: A Polymorphic Network Protocol to Circumvent Censorship}},
	Year = 2013}
	
	@article{savage2000practical,
	Author = {Savage, S. and Wetherall, D. and Karlin, A. and Anderson, T.},
	Journal = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Pages = {295--306},
	Publisher = {ACM},
	Title = {Practical network support for IP traceback},
	Volume = {30},
	Year = {2000}}
	
	@inproceedings{ooni,
	Author = {Filast, A. and Appelbaum, J.},
	Booktitle = {{FOCI}},
	Title = {{OONI : Open Observatory of Network Interference}},
	Year = {2012}}
	
	@misc{caida-rank,
	Howpublished = {\url{http://as-rank.caida.org/}},
	Key = {caida rank},
	Title = {{AS Rank: AS Ranking}}}
	
	@inproceedings{usersrouted-ccs13,
	Author = {A.~Johnson and C.~Wacek and R.~Jansen and M.~Sherr and P.~Syverson},
	Booktitle = {CCS},
	Title = {{Users Get Routed: Traffic Correlation on Tor by Realistic Adversaries}},
	Year = {2013}}
	
	@inproceedings{edman2009awareness,
	Author = {Edman, M. and Syverson, P.},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2009}}
	
	@inproceedings{DecoyCosts,
	Author = {A.~Houmansadr and E.~L.~Wong and V.~Shmatikov},
	Booktitle = {NDSS},
	Title = {{No Direction Home: The True Cost of Routing Around Decoys}},
	Year = {2014}}
	
	@article{cordon,
	Author = {Elahi, T. and Goldberg, I.},
	Journal = {University of Waterloo CACR},
	Title = {{CORDON--A Taxonomy of Internet Censorship Resistance Strategies}},
	Volume = {33},
	Year = {2012}}
	
	@inproceedings{privex,
	Author = {T.~Elahi and G.~Danezis and I.~Goldberg	},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2014}}
	
	@inproceedings{changeGuards,
	Author = {T.~Elahi and K.~Bauer and M.~AlSabah and R.~Dingledine and I.~Goldberg},
	Booktitle = {{WPES}},
	Title = {{ Changing of the Guards: Framework for Understanding and Improving Entry Guard Selection in Tor}},
	Year = {2012}}
	
	@article{RAINBOW:Journal,
	Author = {A.~Houmansadr and N.~Kiyavash and N.~Borisov},
	Journal = {IEEE/ACM Transactions on Networking},
	Title = {{Non-Blind Watermarking of Network Flows}},
	Year = 2014}
	
	@inproceedings{info-tod,
	Author = {A.~Houmansadr and S.~Gorantla and T.~Coleman and N.~Kiyavash and and N.~Borisov},
	Booktitle = {{CCS (poster session)}},
	Title = {{On the Channel Capacity of Network Flow Watermarking}},
	Year = {2009}}
	
	@inproceedings{johnson2014game,
	Author = {Johnson, B. and Laszka, A. and Grossklags, J. and Vasek, M. and Moore, T.},
	Booktitle = {Workshop on Bitcoin Research},
	Title = {{Game-theoretic Analysis of DDoS Attacks Against Bitcoin Mining Pools}},
	Year = {2014}}
	
	@incollection{laszka2013mitigation,
	Author = {Laszka, A. and Johnson, B. and Grossklags, J.},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {175--191},
	Publisher = {Springer},
	Title = {{Mitigation of Targeted and Non-targeted Covert Attacks as a Timing Game}},
	Year = {2013}}
	
	@inproceedings{schottle2013game,
	Author = {Schottle, P. and Laszka, A. and Johnson, B. and Grossklags, J. and Bohme, R.},
	Booktitle = {EUSIPCO},
	Title = {{A Game-theoretic Analysis of Content-adaptive Steganography with Independent Embedding}},
	Year = {2013}}
	
	@inproceedings{CloudTransport,
	Author = {C.~Brubaker and A.~Houmansadr and V.~Shmatikov},
	Booktitle = {PETS},
	Title = {{CloudTransport: Using Cloud Storage for Censorship-Resistant Networking}},
	Year = {2014}}
	
	@inproceedings{sweet,
	Author = {W.~Zhou and A.~Houmansadr and M.~Caesar and N.~Borisov},
	Booktitle = {HotPETs},
	Title = {{SWEET: Serving the Web by Exploiting Email Tunnels}},
	Year = {2013}}
	
	@inproceedings{ahsan2002practical,
	Author = {Ahsan, K. and Kundur, D.},
	Booktitle = {Workshop on Multimedia Security},
	Title = {{Practical data hiding in TCP/IP}},
	Year = {2002}}
	
	@incollection{danezis2011covert,
	Author = {Danezis, G.},
	Booktitle = {Security Protocols XVI},
	Pages = {198--214},
	Publisher = {Springer},
	Title = {{Covert Communications Despite Traffic Data Retention}},
	Year = {2011}}
	
	@inproceedings{liu2009hide,
	Author = {Liu, Y. and Ghosal, D. and Armknecht, F. and Sadeghi, A.-R. and Schulz, S. and Katzenbeisser, S.},
	Booktitle = {ESORICS},
	Title = {{Hide and Seek in Time---Robust Covert Timing Channels}},
	Year = {2009}}
	
	@misc{image-watermark-fing,
	Author = {Jonathan Bailey},
	Howpublished = {\url{https://www.plagiarismtoday.com/2009/12/02/image-detection-watermarking-vs-fingerprinting/}},
	Title = {{Image Detection: Watermarking vs. Fingerprinting}},
	Year = {2009}}
	
	@inproceedings{Servetto98,
	Author = {S. D. Servetto and C. I. Podilchuk and K. Ramchandran},
	Booktitle = {Int. Conf. Image Processing},
	Title = {Capacity issues in digital image watermarking},
	Year = {1998}}
	
	@inproceedings{Chen01,
	Author = {B. Chen and G.W.Wornell},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1423--1443},
	Title = {Quantization index modulation: A class of provably good methods for digital watermarking and information embedding},
	Year = {2001}}
	
	@inproceedings{Karakos00,
	Author = {D. Karakos and A. Papamarcou},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {47},
	Title = {Relationship between quantization and distribution rates of digitally watermarked data},
	Year = {2000}}
	
	@inproceedings{Sullivan98,
	Author = {J. A. OSullivan and P. Moulin and J. M. Ettinger},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {297},
	Title = {Information theoretic analysis of steganography},
	Year = {1998}}
	
	@inproceedings{Merhav00,
	Author = {N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {420--430},
	Title = {On random coding error exponents of watermarking systems},
	Year = {2000}}
	
	@inproceedings{Somekh01,
	Author = {A. Somekh-Baruch and N. Merhav},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {7},
	Title = {On the error exponent and capacity games of private watermarking systems},
	Year = {2001}}
	
	@inproceedings{Steinberg01,
	Author = {Y. Steinberg and N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1410--1422},
	Title = {Identification in the presence of side information with application to watermarking},
	Year = {2001}}
	
	@article{Moulin03,
	Author = {P. Moulin and J.A. O'Sullivan},
	Journal = {IEEE Trans. Info. Theory},
	Number = {3},
	Title = {Information-theoretic analysis of information hiding},
	Volume = 49,
	Year = 2003}
	
	@article{Gelfand80,
	Author = {S.I.~Gelfand and M.S.~Pinsker},
	Journal = {Problems of Control and Information Theory},
	Number = {1},
	Pages = {19-31},
	Title = {{Coding for channel with random parameters}},
	Url = {citeseer.ist.psu.edu/anantharam96bits.html},
	Volume = {9},
	Year = {1980},
	Bdsk-Url-1 = {citeseer.ist.psu.edu/anantharam96bits.html}}
	
	@book{Wolfowitz78,
	Author = {J. Wolfowitz},
	Edition = {3rd},
	Location = {New York},
	Publisher = {Springer-Verlag},
	Title = {Coding Theorems of Information Theory},
	Year = 1978}
	
	@article{caire99,
	Author = {G. Caire and S. Shamai},
	Journal = {IEEE Transactions on Information Theory},
	Number = {6},
	Pages = {2007--2019},
	Title = {On the Capacity of Some Channels with Channel State Information},
	Volume = {45},
	Year = {1999}}
	
	@inproceedings{wright2007language,
	Author = {Wright, Charles V and Ballard, Lucas and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {USENIX Security},
	Title = {{Language identification of encrypted VoIP traffic: Alejandra y Roberto or Alice and Bob?}},
	Year = {2007}}
	
	@inproceedings{backes2010speaker,
	Author = {Backes, Michael and Doychev, Goran and D{\"u}rmuth, Markus and K{\"o}pf, Boris},
	Booktitle = {{European Symposium on Research in Computer Security (ESORICS)}},
	Pages = {508--523},
	Publisher = {Springer},
	Title = {{Speaker Recognition in Encrypted Voice Streams}},
	Year = {2010}}
	
	@phdthesis{lu2009traffic,
	Author = {Lu, Yuanchao},
	School = {Cleveland State University},
	Title = {{On Traffic Analysis Attacks to Encrypted VoIP Calls}},
	Year = {2009}}
	
	@inproceedings{wright2008spot,
	Author = {Wright, Charles V and Ballard, Lucas and Coull, Scott E and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {35--49},
	Title = {Spot me if you can: Uncovering spoken phrases in encrypted VoIP conversations},
	Year = {2008}}
	
	@inproceedings{white2011phonotactic,
	Author = {White, Andrew M and Matthews, Austin R and Snow, Kevin Z and Monrose, Fabian},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {3--18},
	Title = {Phonotactic reconstruction of encrypted VoIP conversations: Hookt on fon-iks},
	Year = {2011}}
	
	@inproceedings{fancy,
	Author = {Houmansadr, Amir and Borisov, Nikita},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {205--224},
	Title = {The Need for Flow Fingerprints to Link Correlated Network Flows},
	Year = {2013}}
	
	@article{botmosaic,
	Author = {Amir Houmansadr and Nikita Borisov},
	Doi = {10.1016/j.jss.2012.11.005},
	Issn = {0164-1212},
	Journal = {Journal of Systems and Software},
	Keywords = {Network security},
	Number = {3},
	Pages = {707 - 715},
	Title = {BotMosaic: Collaborative network watermark for the detection of IRC-based botnets},
	Url = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Volume = {86},
	Year = {2013},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.jss.2012.11.005}}
	
	@inproceedings{ramsbrock2008first,
	Author = {Ramsbrock, Daniel and Wang, Xinyuan and Jiang, Xuxian},
	Booktitle = {Recent Advances in Intrusion Detection},
	Organization = {Springer},
	Pages = {59--77},
	Title = {A first step towards live botmaster traceback},
	Year = {2008}}
	
	@inproceedings{potdar2005survey,
	Author = {Potdar, Vidyasagar M and Han, Song and Chang, Elizabeth},
	Booktitle = {Industrial Informatics, 2005. INDIN'05. 2005 3rd IEEE International Conference on},
	Organization = {IEEE},
	Pages = {709--716},
	Title = {A survey of digital image watermarking techniques},
	Year = {2005}}
	
	@book{cole2003hiding,
	Author = {Cole, Eric and Krutz, Ronald D},
	Publisher = {John Wiley \& Sons, Inc.},
	Title = {Hiding in plain sight: Steganography and the art of covert communication},
	Year = {2003}}
	
	@incollection{akaike1998information,
	Author = {Akaike, Hirotogu},
	Booktitle = {Selected Papers of Hirotugu Akaike},
	Pages = {199--213},
	Publisher = {Springer},
	Title = {Information theory and an extension of the maximum likelihood principle},
	Year = {1998}}
	
	@misc{central-command-hack,
	Author = {Everett Rosenfeld},
	Howpublished = {\url{http://www.cnbc.com/id/102330338}},
	Title = {{FBI investigating Central Command Twitter hack}},
	Year = {2015}}
	
	@misc{sony-psp-ddos,
	Howpublished = {\url{http://n4g.com/news/1644853/sony-and-microsoft-cant-do-much-ddos-attacks-explained}},
	Key = {sony},
	Month = {December},
	Title = {{Sony and Microsoft cant do much -- DDoS attacks explained}},
	Year = {2014}}
	
	@misc{sony-hack,
	Author = {David Bloom},
	Howpublished = {\url{http://goo.gl/MwR4A7}},
	Title = {{Online Game Networks Hacked, Sony Unit President Threatened}},
	Year = {2014}}
	
	@misc{home-depot,
	Author = {Dune Lawrence},
	Howpublished = {\url{http://www.businessweek.com/articles/2014-09-02/home-depots-credit-card-breach-looks-just-like-the-target-hack}},
	Title = {{Home Depot's Suspected Breach Looks Just Like the Target Hack}},
	Year = {2014}}
	
	@misc{target,
	Author = {Julio Ojeda-Zapata},
	Howpublished = {\url{http://www.mercurynews.com/business/ci_24765398/how-did-hackers-pull-off-target-data-heist}},
	Title = {{Target hack: How did they do it?}},
	Year = {2014}}
	
	
	@article{probabilitycourse,
	Author = {H. Pishro-Nik},
	note = {\url{http://www.probabilitycourse.com}},
	Title = {Introduction to probability, statistics, and random processes},
	Year = {2014}}
	
	
	
	@inproceedings{shokri2011quantifying,
	Author = {Shokri, Reza and Theodorakopoulos, George and Le Boudec, Jean-Yves and Hubaux, Jean-Pierre},
	Booktitle = {Security and Privacy (SP), 2011 IEEE Symposium on},
	Organization = {IEEE},
	Pages = {247--262},
	Title = {Quantifying location privacy},
	Year = {2011}}
	
	@inproceedings{hoh2007preserving,
	Author = {Hoh, Baik and Gruteser, Marco and Xiong, Hui and Alrabady, Ansaf},
	Booktitle = {Proceedings of the 14th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {161--171},
	Title = {Preserving privacy in gps traces via uncertainty-aware path cloaking},
	Year = {2007}}
	
	
	
	@article{kafsi2013entropy,
	Author = {Kafsi, Mohamed and Grossglauser, Matthias and Thiran, Patrick},
	Journal = {Information Theory, IEEE Transactions on},
	Number = {9},
	Pages = {5577--5583},
	Publisher = {IEEE},
	Title = {The entropy of conditional Markov trajectories},
	Volume = {59},
	Year = {2013}}
	
	@inproceedings{gruteser2003anonymous,
	Author = {Gruteser, Marco and Grunwald, Dirk},
	Booktitle = {Proceedings of the 1st international conference on Mobile systems, applications and services},
	Organization = {ACM},
	Pages = {31--42},
	Title = {Anonymous usage of location-based services through spatial and temporal cloaking},
	Year = {2003}}
	
	@inproceedings{husted2010mobile,
	Author = {Husted, Nathaniel and Myers, Steven},
	Booktitle = {Proceedings of the 17th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {85--96},
	Title = {Mobile location tracking in metro areas: malnets and others},
	Year = {2010}}
	
	@inproceedings{li2009tradeoff,
	Author = {Li, Tiancheng and Li, Ninghui},
	Booktitle = {Proceedings of the 15th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {517--526},
	Title = {On the tradeoff between privacy and utility in data publishing},
	Year = {2009}}
	
	@inproceedings{ma2009location,
	Author = {Ma, Zhendong and Kargl, Frank and Weber, Michael},
	Booktitle = {Sarnoff Symposium, 2009. SARNOFF'09. IEEE},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {A location privacy metric for v2x communication systems},
	Year = {2009}}
	
	@inproceedings{shokri2012protecting,
	Author = {Shokri, Reza and Theodorakopoulos, George and Troncoso, Carmela and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
	Booktitle = {Proceedings of the 2012 ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {617--627},
	Title = {Protecting location privacy: optimal strategy against localization attacks},
	Year = {2012}}
	
	@inproceedings{freudiger2009non,
	Author = {Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
	Booktitle = {Proceedings of the 16th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {324--337},
	Title = {On non-cooperative location privacy: a game-theoretic analysis},
	Year = {2009}}
	
	@incollection{humbert2010tracking,
	Author = {Humbert, Mathias and Manshaei, Mohammad Hossein and Freudiger, Julien and Hubaux, Jean-Pierre},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {38--57},
	Publisher = {Springer},
	Title = {Tracking games in mobile networks},
	Year = {2010}}
	
	@article{manshaei2013game,
	Author = {Manshaei, Mohammad Hossein and Zhu, Quanyan and Alpcan, Tansu and Bac{\c{s}}ar, Tamer and Hubaux, Jean-Pierre},
	Journal = {ACM Computing Surveys (CSUR)},
	Number = {3},
	Pages = {25},
	Publisher = {ACM},
	Title = {Game theory meets network security and privacy},
	Volume = {45},
	Year = {2013}}
	
	@article{palamidessi2006probabilistic,
	Author = {Palamidessi, Catuscia},
	Journal = {Electronic Notes in Theoretical Computer Science},
	Pages = {33--42},
	Publisher = {Elsevier},
	Title = {Probabilistic and nondeterministic aspects of anonymity},
	Volume = {155},
	Year = {2006}}
	
	@inproceedings{mokbel2006new,
	Author = {Mokbel, Mohamed F and Chow, Chi-Yin and Aref, Walid G},
	Booktitle = {Proceedings of the 32nd international conference on Very large data bases},
	Organization = {VLDB Endowment},
	Pages = {763--774},
	Title = {The new Casper: query processing for location services without compromising privacy},
	Year = {2006}}
	
	@article{kalnis2007preventing,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {12},
	Pages = {1719--1733},
	Publisher = {IEEE},
	Title = {Preventing location-based identity inference in anonymous spatial queries},
	Volume = {19},
	Year = {2007}}
	
	@article{freudiger2007mix,
	title={Mix-zones for location privacy in vehicular networks},
	author={Freudiger, Julien and Raya, Maxim and F{\'e}legyh{\'a}zi, M{\'a}rk and Papadimitratos, Panos and Hubaux, Jean-Pierre},
	year={2007}
	}
	@article{sweeney2002k,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {557--570},
	Publisher = {World Scientific},
	Title = {k-anonymity: A model for protecting privacy},
	Volume = {10},
	Year = {2002}}
	
	@article{sweeney2002achieving,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {571--588},
	Publisher = {World Scientific},
	Title = {Achieving k-anonymity privacy protection using generalization and suppression},
	Volume = {10},
	Year = {2002}}
	
	@inproceedings{niu2014achieving,
	Author = {Niu, Ben and Li, Qinghua and Zhu, Xiaoyan and Cao, Guohong and Li, Hui},
	Booktitle = {INFOCOM, 2014 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {754--762},
	Title = {Achieving k-anonymity in privacy-aware location-based services},
	Year = {2014}}
	
	@inproceedings{liu2013game,
	Author = {Liu, Xinxin and Liu, Kaikai and Guo, Linke and Li, Xiaolin and Fang, Yuguang},
	Booktitle = {INFOCOM, 2013 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {2985--2993},
	Title = {A game-theoretic approach for achieving k-anonymity in location based services},
	Year = {2013}}
	
	@inproceedings{kido2005protection,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Data Engineering Workshops, 2005. 21st International Conference on},
	Organization = {IEEE},
	Pages = {1248--1248},
	Title = {Protection of location privacy using dummies for location-based services},
	Year = {2005}}
	
	@inproceedings{gedik2005location,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Booktitle = {Distributed Computing Systems, 2005. ICDCS 2005. Proceedings. 25th IEEE International Conference on},
	Organization = {IEEE},
	Pages = {620--629},
	Title = {Location privacy in mobile systems: A personalized anonymization model},
	Year = {2005}}
	
	@inproceedings{bordenabe2014optimal,
	Author = {Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2014 ACM SIGSAC Conference on Computer and Communications Security},
	Organization = {ACM},
	Pages = {251--262},
	Title = {Optimal geo-indistinguishable mechanisms for location privacy},
	Year = {2014}}
	
	@incollection{duckham2005formal,
	Author = {Duckham, Matt and Kulik, Lars},
	Booktitle = {Pervasive computing},
	Pages = {152--170},
	Publisher = {Springer},
	Title = {A formal model of obfuscation and negotiation for location privacy},
	Year = {2005}}
	
	@inproceedings{kido2005anonymous,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Pervasive Services, 2005. ICPS'05. Proceedings. International Conference on},
	Organization = {IEEE},
	Pages = {88--97},
	Title = {An anonymous communication technique using dummies for location-based services},
	Year = {2005}}
	
	@incollection{duckham2006spatiotemporal,
	Author = {Duckham, Matt and Kulik, Lars and Birtley, Athol},
	Booktitle = {Geographic Information Science},
	Pages = {47--64},
	Publisher = {Springer},
	Title = {A spatiotemporal model of strategies and counter strategies for location privacy protection},
	Year = {2006}}
	
	@inproceedings{shankar2009privately,
	Author = {Shankar, Pravin and Ganapathy, Vinod and Iftode, Liviu},
	Booktitle = {Proceedings of the 11th international conference on Ubiquitous computing},
	Organization = {ACM},
	Pages = {31--40},
	Title = {Privately querying location-based services with SybilQuery},
	Year = {2009}}
	
	@inproceedings{chow2009faking,
	Author = {Chow, Richard and Golle, Philippe},
	Booktitle = {Proceedings of the 8th ACM workshop on Privacy in the electronic society},
	Organization = {ACM},
	Pages = {105--108},
	Title = {Faking contextual data for fun, profit, and privacy},
	Year = {2009}}
	
	@incollection{xue2009location,
	Author = {Xue, Mingqiang and Kalnis, Panos and Pung, Hung Keng},
	Booktitle = {Location and Context Awareness},
	Pages = {70--87},
	Publisher = {Springer},
	Title = {Location diversity: Enhanced privacy protection in location based services},
	Year = {2009}}
	
	@article{wernke2014classification,
	Author = {Wernke, Marius and Skvortsov, Pavel and D{\"u}rr, Frank and Rothermel, Kurt},
	Journal = {Personal and Ubiquitous Computing},
	Number = {1},
	Pages = {163--175},
	Publisher = {Springer-Verlag},
	Title = {A classification of location privacy attacks and approaches},
	Volume = {18},
	Year = {2014}}
	
	@misc{cai2015cloaking,
	Author = {Cai, Y. and Xu, G.},
	Month = jan # {~1},
	Note = {US Patent App. 14/472,462},
	Publisher = {Google Patents},
	Title = {Cloaking with footprints to provide location privacy protection in location-based services},
	Url = {https://www.google.com/patents/US20150007341},
	Year = {2015},
	Bdsk-Url-1 = {https://www.google.com/patents/US20150007341}}
	
	@article{gedik2008protecting,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {1},
	Pages = {1--18},
	Publisher = {IEEE},
	Title = {Protecting location privacy with personalized k-anonymity: Architecture and algorithms},
	Volume = {7},
	Year = {2008}}
	
	@article{kalnis2006preserving,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Publisher = {TRB6/06},
	Title = {Preserving anonymity in location based services},
	Year = {2006}}
	
	@inproceedings{hoh2005protecting,
	Author = {Hoh, Baik and Gruteser, Marco},
	Booktitle = {Security and Privacy for Emerging Areas in Communications Networks, 2005. SecureComm 2005. First International Conference on},
	Organization = {IEEE},
	Pages = {194--205},
	Title = {Protecting location privacy through path confusion},
	Year = {2005}}
	
	@article{terrovitis2011privacy,
	Author = {Terrovitis, Manolis},
	Journal = {ACM SIGKDD Explorations Newsletter},
	Number = {1},
	Pages = {6--18},
	Publisher = {ACM},
	Title = {Privacy preservation in the dissemination of location data},
	Volume = {13},
	Year = {2011}}
	
	@article{shin2012privacy,
	Author = {Shin, Kang G and Ju, Xiaoen and Chen, Zhigang and Hu, Xin},
	Journal = {Wireless Communications, IEEE},
	Number = {1},
	Pages = {30--39},
	Publisher = {IEEE},
	Title = {Privacy protection for users of location-based services},
	Volume = {19},
	Year = {2012}}
	
	@article{khoshgozaran2011location,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus and Shirani-Mehr, Houtan},
	Journal = {Knowledge and Information Systems},
	Number = {3},
	Pages = {435--465},
	Publisher = {Springer},
	Title = {Location privacy: going beyond K-anonymity, cloaking and anonymizers},
	Volume = {26},
	Year = {2011}}
	
	@incollection{chatzikokolakis2015geo,
	Author = {Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
	Booktitle = {Distributed Computing and Internet Technology},
	Pages = {49--72},
	Publisher = {Springer},
	Title = {Geo-indistinguishability: A Principled Approach to Location Privacy},
	Year = {2015}}
	
	@inproceedings{ngo2015location,
	Author = {Ngo, Hoa and Kim, Jong},
	Booktitle = {Computer Security Foundations Symposium (CSF), 2015 IEEE 28th},
	Organization = {IEEE},
	Pages = {63--74},
	Title = {Location Privacy via Differential Private Perturbation of Cloaking Area},
	Year = {2015}}
	
	@inproceedings{palanisamy2011mobimix,
	Author = {Palanisamy, Balaji and Liu, Ling},
	Booktitle = {Data Engineering (ICDE), 2011 IEEE 27th International Conference on},
	Organization = {IEEE},
	Pages = {494--505},
	Title = {Mobimix: Protecting location privacy with mix-zones over road networks},
	Year = {2011}}
	
	@inproceedings{um2010advanced,
	Author = {Um, Jung-Ho and Kim, Hee-Dae and Chang, Jae-Woo},
	Booktitle = {Social Computing (SocialCom), 2010 IEEE Second International Conference on},
	Organization = {IEEE},
	Pages = {1093--1098},
	Title = {An advanced cloaking algorithm using Hilbert curves for anonymous location based service},
	Year = {2010}}
	
	@inproceedings{bamba2008supporting,
	Author = {Bamba, Bhuvan and Liu, Ling and Pesti, Peter and Wang, Ting},
	Booktitle = {Proceedings of the 17th international conference on World Wide Web},
	Organization = {ACM},
	Pages = {237--246},
	Title = {Supporting anonymous location queries in mobile environments with privacygrid},
	Year = {2008}}
	
	@inproceedings{zhangwei2010distributed,
	Author = {Zhangwei, Huang and Mingjun, Xin},
	Booktitle = {Networks Security Wireless Communications and Trusted Computing (NSWCTC), 2010 Second International Conference on},
	Organization = {IEEE},
	Pages = {468--471},
	Title = {A distributed spatial cloaking protocol for location privacy},
	Volume = {2},
	Year = {2010}}
	
	@article{chow2011spatial,
	Author = {Chow, Chi-Yin and Mokbel, Mohamed F and Liu, Xuan},
	Journal = {GeoInformatica},
	Number = {2},
	Pages = {351--380},
	Publisher = {Springer},
	Title = {Spatial cloaking for anonymous location-based services in mobile peer-to-peer environments},
	Volume = {15},
	Year = {2011}}
	
	@inproceedings{lu2008pad,
	Author = {Lu, Hua and Jensen, Christian S and Yiu, Man Lung},
	Booktitle = {Proceedings of the Seventh ACM International Workshop on Data Engineering for Wireless and Mobile Access},
	Organization = {ACM},
	Pages = {16--23},
	Title = {Pad: privacy-area aware, dummy-based location privacy in mobile services},
	Year = {2008}}
	
	@incollection{khoshgozaran2007blind,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus},
	Booktitle = {Advances in Spatial and Temporal Databases},
	Pages = {239--257},
	Publisher = {Springer},
	Title = {Blind evaluation of nearest neighbor queries using space transformation to preserve location privacy},
	Year = {2007}}
	
	@inproceedings{ghinita2008private,
	Author = {Ghinita, Gabriel and Kalnis, Panos and Khoshgozaran, Ali and Shahabi, Cyrus and Tan, Kian-Lee},
	Booktitle = {Proceedings of the 2008 ACM SIGMOD international conference on Management of data},
	Organization = {ACM},
	Pages = {121--132},
	Title = {Private queries in location based services: anonymizers are not necessary},
	Year = {2008}}
	
	@article{paulet2014privacy,
	Author = {Paulet, Russell and Kaosar, Md Golam and Yi, Xun and Bertino, Elisa},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {5},
	Pages = {1200--1210},
	Publisher = {IEEE},
	Title = {Privacy-preserving and content-protecting location based queries},
	Volume = {26},
	Year = {2014}}
	
	@article{nguyen2013differential,
	Author = {Nguyen, Hiep H and Kim, Jong and Kim, Yoonho},
	Journal = {Journal of Computing Science and Engineering},
	Number = {3},
	Pages = {177--186},
	Title = {Differential privacy in practice},
	Volume = {7},
	Year = {2013}}
	
	@inproceedings{lee2012differential,
	Author = {Lee, Jaewoo and Clifton, Chris},
	Booktitle = {Proceedings of the 18th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {1041--1049},
	Title = {Differential identifiability},
	Year = {2012}}
	
	@inproceedings{andres2013geo,
	Author = {Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2013 ACM SIGSAC conference on Computer \& communications security},
	Organization = {ACM},
	Pages = {901--914},
	Title = {Geo-indistinguishability: Differential privacy for location-based systems},
	Year = {2013}}
	
	@inproceedings{machanavajjhala2008privacy,
	Author = {Machanavajjhala, Ashwin and Kifer, Daniel and Abowd, John and Gehrke, Johannes and Vilhuber, Lars},
	Booktitle = {Data Engineering, 2008. ICDE 2008. IEEE 24th International Conference on},
	Organization = {IEEE},
	Pages = {277--286},
	Title = {Privacy: Theory meets practice on the map},
	Year = {2008}}
	
	@article{dewri2013local,
	Author = {Dewri, Rinku},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {12},
	Pages = {2360--2372},
	Publisher = {IEEE},
	Title = {Local differential perturbations: Location privacy under approximate knowledge attackers},
	Volume = {12},
	Year = {2013}}
	
	@inproceedings{chatzikokolakis2013broadening,
	Author = {Chatzikokolakis, Konstantinos and Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s Emilio and Palamidessi, Catuscia},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {82--102},
	Title = {Broadening the Scope of Differential Privacy Using Metrics.},
	Year = {2013}}
	
	@inproceedings{zhong2009distributed,
	Author = {Zhong, Ge and Hengartner, Urs},
	Booktitle = {Pervasive Computing and Communications, 2009. PerCom 2009. IEEE International Conference on},
	Organization = {IEEE},
	Pages = {1--10},
	Title = {A distributed k-anonymity protocol for location privacy},
	Year = {2009}}
	
	@inproceedings{ho2011differential,
	Author = {Ho, Shen-Shyang and Ruan, Shuhua},
	Booktitle = {Proceedings of the 4th ACM SIGSPATIAL International Workshop on Security and Privacy in GIS and LBS},
	Organization = {ACM},
	Pages = {17--24},
	Title = {Differential privacy for location pattern mining},
	Year = {2011}}
	
	@inproceedings{cheng2006preserving,
	Author = {Cheng, Reynold and Zhang, Yu and Bertino, Elisa and Prabhakar, Sunil},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {393--412},
	Title = {Preserving user location privacy in mobile data management infrastructures},
	Year = {2006}}
	
	@article{beresford2003location,
	Author = {Beresford, Alastair R and Stajano, Frank},
	Journal = {IEEE Pervasive computing},
	Number = {1},
	Pages = {46--55},
	Publisher = {IEEE},
	Title = {Location privacy in pervasive computing},
	Year = {2003}}
	
	@inproceedings{freudiger2009optimal,
	Author = {Freudiger, Julien and Shokri, Reza and Hubaux, Jean-Pierre},
	Booktitle = {Privacy enhancing technologies},
	Organization = {Springer},
	Pages = {216--234},
	Title = {On the optimal placement of mix zones},
	Year = {2009}}
	
	@article{krumm2009survey,
	Author = {Krumm, John},
	Journal = {Personal and Ubiquitous Computing},
	Number = {6},
	Pages = {391--399},
	Publisher = {Springer},
	Title = {A survey of computational location privacy},
	Volume = {13},
	Year = {2009}}
	
	@article{Rakhshan2016letter,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Wireless Communications Letter},
	Publisher = {IEEE},
	Title = {Interference Models for Vehicular Ad Hoc Networks},
	Year = {2016, submitted}}
	
	@article{Rakhshan2015Journal,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Publisher = {IEEE},
	Title = {Improving Safety on Highways by Customizing Vehicular Ad Hoc Networks},
	Year = {to appear, 2017}}
	
	@inproceedings{Rakhshan2015Cogsima,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Booktitle = {IEEE International Multi-Disciplinary Conference on Cognitive Methods in Situation Awareness and Decision Support},
	Organization = {IEEE},
	Title = {A New Approach to Customization of Accident Warning Systems to Individual Drivers},
	Year = {2015}}
	
	@inproceedings{Rakhshan2015CISS,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Nekoui, Mohammad},
	Booktitle = {Conference on Information Sciences and Systems},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {Driver-based adaptation of Vehicular Ad Hoc Networks for design of active safety systems},
	Year = {2015}}
	
	@inproceedings{Rakhshan2014IV,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Ray, Evan},
	Booktitle = {Intelligent Vehicles Symposium},
	Organization = {IEEE},
	Pages = {1181--1186},
	Title = {Real-time estimation of the distribution of brake response times for an individual driver using Vehicular Ad Hoc Network.},
	Year = {2014}}
	
	@inproceedings{Rakhshan2013Globecom,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Fisher, Donald and Nekoui, Mohammad},
	Booktitle = {IEEE Global Communications Conference},
	Organization = {IEEE},
	Pages = {1333--1337},
	Title = {Tuning collision warning algorithms to individual drivers for design of active safety systems.},
	Year = {2013}}
	
	@article{Nekoui2012Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Number = {8},
	Pages = {2895--2905},
	Publisher = {IEEE},
	Title = {Throughput Scaling laws for Vehicular Ad Hoc Networks},
	Volume = {11},
	Year = {2012}}
	
	
	
	
	
	
	
	
	
	@article{Nekoui2011Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein and Ni, Daiheng},
	Journal = {International Journal of Vehicular Technology},
	Pages = {1--11},
	Publisher = {Hindawi Publishing Corporation},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {2011},
	Year = {2011}}
	
	
	
	
	
	
	@article{shokri2014optimal,
	title={Optimal user-centric data obfuscation},
	author={Shokri, Reza},
	journal={arXiv preprint arXiv:1402.3426},
	year={2014}
	}
	@article{chatzikokolakis2015location,
	title={Location privacy via geo-indistinguishability},
	author={Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
	journal={ACM SIGLOG News},
	volume={2},
	number={3},
	pages={46--69},
	year={2015},
	publisher={ACM}
	
	}
	@inproceedings{shokri2011quantifying2,
	title={Quantifying location privacy: the case of sporadic location exposure},
	author={Shokri, Reza and Theodorakopoulos, George and Danezis, George and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
	booktitle={Privacy Enhancing Technologies},
	pages={57--76},
	year={2011},
	organization={Springer}
	}
	
	
	@inproceedings{Mont1603:Defining,
	AUTHOR="Zarrin Montazeri and Amir Houmansadr and Hossein Pishro-Nik",
	TITLE="Defining Perfect Location Privacy Using Anonymization",
	BOOKTITLE="2016 Annual Conference on Information Science and Systems (CISS) (CISS
	2016)",
	ADDRESS="Princeton, USA",
	DAYS=16,
	MONTH=mar,
	YEAR=2016,
	KEYWORDS="Information Theoretic Privacy; location-based services; Location Privacy;
	Information Theory",
	ABSTRACT="The popularity of mobile devices and location-based services (LBS) have
	created great concerns regarding the location privacy of users of such
	devices and services. Anonymization is a common technique that is often
	being used to protect the location privacy of LBS users. In this paper, we
	provide a general information theoretic definition for location privacy. In
	particular, we define perfect location privacy. We show that under certain
	conditions, perfect privacy is achieved if the pseudonyms of users is
	changed after o(N^(2/r?1)) observations by the adversary, where N is the
	number of users and r is the number of sub-regions or locations.
	"
	}
	@article{our-isita-location,
	Author = {Zarrin Montazeri and Amir Houmansadr and Hossein Pishro-Nik},
	Journal = {IEEE International Symposium on Information Theory and Its Applications (ISITA)},
	Title = {Achieving Perfect Location Privacy in Markov Models Using Anonymization},
	Year = {2016}
	}
	@article{our-TIFS,
	Author = {Zarrin Montazeri and Hossein Pishro-Nik and Amir Houmansadr},
	Journal = {IEEE Transactions on Information Forensics and Security, accepted with mandatory minor revisions},
	Title = {Perfect Location Privacy Using Anonymization in Mobile Networks},
	Year = {2017},
	note={Available on arxiv.org}
	}
	
	
	
	@techreport{sampigethaya2005caravan,
	title={CARAVAN: Providing location privacy for VANET},
	author={Sampigethaya, Krishna and Huang, Leping and Li, Mingyan and Poovendran, Radha and Matsuura, Kanta and Sezaki, Kaoru},
	year={2005},
	institution={DTIC Document}
	}
	@incollection{buttyan2007effectiveness,
	title={On the effectiveness of changing pseudonyms to provide location privacy in VANETs},
	author={Butty{\'a}n, Levente and Holczer, Tam{\'a}s and Vajda, Istv{\'a}n},
	booktitle={Security and Privacy in Ad-hoc and Sensor Networks},
	pages={129--141},
	year={2007},
	publisher={Springer}
	}
	@article{sampigethaya2007amoeba,
	title={AMOEBA: Robust location privacy scheme for VANET},
	author={Sampigethaya, Krishna and Li, Mingyan and Huang, Leping and Poovendran, Radha},
	journal={Selected Areas in communications, IEEE Journal on},
	volume={25},
	number={8},
	pages={1569--1589},
	year={2007},
	publisher={IEEE}
	}
	
	@article{lu2012pseudonym,
	title={Pseudonym changing at social spots: An effective strategy for location privacy in vanets},
	author={Lu, Rongxing and Li, Xiaodong and Luan, Tom H and Liang, Xiaohui and Shen, Xuemin},
	journal={Vehicular Technology, IEEE Transactions on},
	volume={61},
	number={1},
	pages={86--96},
	year={2012},
	publisher={IEEE}
	}
	@inproceedings{lu2010sacrificing,
	title={Sacrificing the plum tree for the peach tree: A socialspot tactic for protecting receiver-location privacy in VANET},
	author={Lu, Rongxing and Lin, Xiaodong and Liang, Xiaohui and Shen, Xuemin},
	booktitle={Global Telecommunications Conference (GLOBECOM 2010), 2010 IEEE},
	pages={1--5},
	year={2010},
	organization={IEEE}
	}
	@inproceedings{lin2011stap,
	title={STAP: A social-tier-assisted packet forwarding protocol for achieving receiver-location privacy preservation in VANETs},
	author={Lin, Xiaodong and Lu, Rongxing and Liang, Xiaohui and Shen, Xuemin Sherman},
	booktitle={INFOCOM, 2011 Proceedings IEEE},
	pages={2147--2155},
	year={2011},
	organization={IEEE}
	}
	@inproceedings{gerlach2007privacy,
	title={Privacy in VANETs using changing pseudonyms-ideal and real},
	author={Gerlach, Matthias and Guttler, Felix},
	booktitle={Vehicular Technology Conference, 2007. VTC2007-Spring. IEEE 65th},
	pages={2521--2525},
	year={2007},
	organization={IEEE}
	}
	@inproceedings{el2002security,
	title={Security issues in a future vehicular network},
	author={El Zarki, Magda and Mehrotra, Sharad and Tsudik, Gene and Venkatasubramanian, Nalini},
	booktitle={European Wireless},
	volume={2},
	year={2002}
	}
	
	@article{hubaux2004security,
	title={The security and privacy of smart vehicles},
	author={Hubaux, Jean-Pierre and Capkun, Srdjan and Luo, Jun},
	journal={IEEE Security \& Privacy Magazine},
	volume={2},
	number={LCA-ARTICLE-2004-007},
	pages={49--55},
	year={2004}
	}
	
	
	
	@inproceedings{duri2002framework,
	title={Framework for security and privacy in automotive telematics},
	author={Duri, Sastry and Gruteser, Marco and Liu, Xuan and Moskowitz, Paul and Perez, Ronald and Singh, Moninder and Tang, Jung-Mu},
	booktitle={Proceedings of the 2nd international workshop on Mobile commerce},
	pages={25--32},
	year={2002},
	organization={ACM}
	}
	@misc{NS-3,
	Howpublished = {\url{https://www.nsnam.org/}}},
}
@misc{testbed,
	Howpublished = {\url{http://www.its.dot.gov/testbed/PDF/SE-MI-Resource-Guide-9-3-1.pdf}}},
@misc{NGSIM,
	Howpublished = {\url{http://ops.fhwa.dot.gov/trafficanalysistools/ngsim.htm}},
}

@misc{National-a2013,
	Author = {National Highway Traffic Safety Administration},
	Howpublished = {\url{http://ops.fhwa.dot.gov/trafficanalysistools/ngsim.htm}},
	Title = {2013 Motor Vehicle Crashes: Overview. Traffic Safety Factors},
	Year = {2013}
}

@inproceedings{karnadi2007rapid,
	title={Rapid generation of realistic mobility models for VANET},
	author={Karnadi, Feliz Kristianto and Mo, Zhi Hai and Lan, Kun-chan},
	booktitle={Wireless Communications and Networking Conference, 2007. WCNC 2007. IEEE},
	pages={2506--2511},
	year={2007},
	organization={IEEE}
}
@inproceedings{saha2004modeling,
	title={Modeling mobility for vehicular ad-hoc networks},
	author={Saha, Amit Kumar and Johnson, David B},
	booktitle={Proceedings of the 1st ACM international workshop on Vehicular ad hoc networks},
	pages={91--92},
	year={2004},
	organization={ACM}
}
@inproceedings{lee2006modeling,
	title={Modeling steady-state and transient behaviors of user mobility: formulation, analysis, and application},
	author={Lee, Jong-Kwon and Hou, Jennifer C},
	booktitle={Proceedings of the 7th ACM international symposium on Mobile ad hoc networking and computing},
	pages={85--96},
	year={2006},
	organization={ACM}
}
@inproceedings{yoon2006building,
	title={Building realistic mobility models from coarse-grained traces},
	author={Yoon, Jungkeun and Noble, Brian D and Liu, Mingyan and Kim, Minkyong},
	booktitle={Proceedings of the 4th international conference on Mobile systems, applications and services},
	pages={177--190},
	year={2006},
	organization={ACM}
}

@inproceedings{choffnes2005integrated,
	title={An integrated mobility and traffic model for vehicular wireless networks},
	author={Choffnes, David R and Bustamante, Fabi{\'a}n E},
	booktitle={Proceedings of the 2nd ACM international workshop on Vehicular ad hoc networks},
	pages={69--78},
	year={2005},
	organization={ACM}
}

@inproceedings{Qian2008Globecom,
	title={CA Secure VANET MAC Protocol for DSRC Applications},
	author={Yi, Q. and Lu, K. and Moyeri, N.{\'a}n E},
	booktitle={Proceedings of IEEE GLOBECOM 2008},
	pages={1--5},
	year={2008},
	organization={IEEE}
}





@inproceedings{naumov2006evaluation,
	title={An evaluation of inter-vehicle ad hoc networks based on realistic vehicular traces},
	author={Naumov, Valery and Baumann, Rainer and Gross, Thomas},
	booktitle={Proceedings of the 7th ACM international symposium on Mobile ad hoc networking and computing},
	pages={108--119},
	year={2006},
	organization={ACM}
}
@article{sommer2008progressing,
	title={Progressing toward realistic mobility models in VANET simulations},
	author={Sommer, Christoph and Dressler, Falko},
	journal={Communications Magazine, IEEE},
	volume={46},
	number={11},
	pages={132--137},
	year={2008},
	publisher={IEEE}
}




@inproceedings{mahajan2006urban,
	title={Urban mobility models for vanets},
	author={Mahajan, Atulya and Potnis, Niranjan and Gopalan, Kartik and Wang, Andy},
	booktitle={2nd IEEE International Workshop on Next Generation Wireless Networks},
	volume={33},
	year={2006}
}

@inproceedings{Rakhshan2016packet,
	title={Packet success probability derivation in a vehicular ad hoc network for a highway scenario},
	author={Rakhshan, Ali and Pishro-Nik, Hossein},
	booktitle={2016 Annual Conference on Information Science and Systems (CISS)},
	pages={210--215},
	year={2016},
	organization={IEEE}
}

@inproceedings{Rakhshan2016CISS,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Booktitle = {Conference on Information Sciences and Systems},
	Organization = {IEEE},
	Pages = {210--215},
	Title = {Packet Success Probability Derivation in a Vehicular Ad Hoc Network for a Highway Scenario},
	Year = {2016}}

@article{Nekoui2013Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {Journal on Selected Areas in Communications, Special Issue on Emerging Technologies in Communications},
	Number = {9},
	Pages = {491--503},
	Publisher = {IEEE},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {31},
	Year = {2013}}


@inproceedings{Nekoui2011MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM workshop on VehiculAr InterNETworking},
	Organization = {ACM},
	Title = {Analytic Design of Active Vehicular Safety Systems in Sparse Traffic},
	Year = {2011}}

@inproceedings{Nekoui2011VTC,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Analytical Design of Inter-vehicular Communications for Collision Avoidance},
	Year = {2011}}

@inproceedings{Bovee2011VTC,
	Author = {Bovee, Ben Louis and Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Evaluation of the Universal Geocast Scheme For VANETs},
	Year = {2011}}

@inproceedings{Nekoui2010MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM},
	Organization = {ACM},
	Title = {Fundamental Tradeoffs in Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2010IVCS,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IVCS},
	Organization = {IEEE},
	Title = {A Universal Geocast Scheme for Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2009ITW,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IEEE Communications Society Conference on Sensor, Mesh and Ad Hoc Communications and Networks Workshops},
	Organization = {IEEE},
	Pages = {1--3},
	Title = {A Geometrical Analysis of Obstructed Wireless Networks},
	Year = {2009}}

@article{Eslami2013Journal,
	Author = {Eslami, Ali and Nekoui, Mohammad and Pishro-Nik, Hossein and Fekri, Faramarz},
	Journal = {ACM Transactions on Sensor Networks},
	Number = {4},
	Pages = {51},
	Publisher = {ACM},
	Title = {Results on finite wireless sensor networks: Connectivity and coverage},
	Volume = {9},
	Year = {2013}}


@article{Jiafu2014Journal,
	Author = {Jiafu, W. and Zhang, D. and Zhao, S. and Yang, L. and Lloret, J.},
	Journal = {Communications Magazine},
	Number = {8},
	Pages = {106-113},
	Publisher = {IEEE},
	Title = {Context-aware vehicular cyber-physical systems with cloud support: architecture, challenges, and solutions},
	Volume = {52},
	Year = {2014}}

@inproceedings{Haas2010ACM,
	Author = {Haas, J.J. and Hu, Y.},
	Booktitle = {international workshop on VehiculAr InterNETworking},
	Organization = {ACM},
	Title = {Communication requirements for crash avoidance.},
	Year = {2010}}

@inproceedings{Yi2008GLOBECOM,
	Author = {Yi, Q. and Lu, K. and Moayeri, N.},
	Booktitle = {GLOBECOM},
	Organization = {IEEE},
	Title = {CA Secure VANET MAC Protocol for DSRC Applications.},
	Year = {2008}}

@inproceedings{Mughal2010ITSim,
	Author = {Mughal, B.M. and Wagan, A. and Hasbullah, H.},
	Booktitle = {International Symposium on Information Technology (ITSim)},
	Organization = {IEEE},
	Title = {Efficient congestion control in VANET for safety messaging.},
	Year = {2010}}

@article{Chang2011Journal,
	Author = {Chang, Y. and Lee, C. and Copeland, J.},
	Journal = {Selected Areas in Communications},
	Pages = {236 â€“249},
	Publisher = {IEEE},
	Title = {Goodput enhancement of VANETs in noisy CSMA/CA channels},
	Volume = {29},
	Year = {2011}}

@article{Garcia-Costa2011Journal,
	Author = {Garcia-Costa, C. and Egea-Lopez, E. and Tomas-Gabarron, J. B. and Garcia-Haro, J. and Haas, Z. J.},
	Journal = {Transactions on Intelligent Transportation Systems},
	Pages = {1 â€“16},
	Publisher = {IEEE},
	Title = {A stochastic model for chain collisions of vehicles equipped with vehicular communications},
	Volume = {99},
	Year = {2011}}

@article{Carbaugh2011Journal,
	Author = {Carbaugh, J. and Godbole,  D. N. and Sengupta, R. and Garcia-Haro, J. and Haas, Z. J.},
	Publisher = {Transportation Research Part C (Emerging Technologies)},
	Title = {Safety and capacity analysis of automated and manual highway systems},
	Year = {1997}}

@article{Goh2004Journal,
	Author = {Goh, P. and Wong, Y.},
	Publisher = {Appl Health Econ Health Policy},
	Title = {Driver perception response time during the signal change interval},
	Year = {2004}}

@article{Chang1985Journal,
	Author = {Chang, M.S. and Santiago, A.J.},
	Pages = {20-30},
	Publisher = {Transportation Research Record},
	Title = {Timing traffic signal changes based on driver behavior},
	Volume = {1027},
	Year = {1985}}

@article{Green2000Journal,
	Author = {Green, M.},
	Pages = {195-216},
	Publisher = {Transportation Human Factors},
	Title = {How long does it take to stop? Methodological analysis of driver perception-brake times.},
	Year = {2000}}

@article{Koppa2005,
	Author = {Koppa, R.J.},
	Pages = {195-216},
	Publisher = {http://www.fhwa.dot.gov/publications/},
	Title = {Human Factors},
	Year = {2005}}

@inproceedings{Maxwell2010ETC,
	Author = {Maxwell, A. and Wood, K.},
	Booktitle = {Europian Transport Conference},
	Organization = {http://www.etcproceedings.org/paper/review-of-traffic-signals-on-high-speed-roads},
	Title = {Review of Traffic Signals on High Speed Road},
	Year = {2010}}

@article{Wortman1983,
	Author = {Wortman, R.H. and Matthias, J.S.},
	Publisher = {Arizona Department of Transportation},
	Title = {An Evaluation of Driver Behavior at Signalized Intersections},
	Year = {1983}}
@inproceedings{Zhang2007IASTED,
	Author = {Zhang, X. and Bham, G.H.},
	Booktitle = {18th IASTED International Conference: modeling and simulation},
	Title = {Estimation of driver reaction time from detailed vehicle trajectory data.},
	Year = {2007}}


@inproceedings{bai2003important,
	title={IMPORTANT: A framework to systematically analyze the Impact of Mobility on Performance of RouTing protocols for Adhoc NeTworks},
	author={Bai, Fan and Sadagopan, Narayanan and Helmy, Ahmed},
	booktitle={INFOCOM 2003. Twenty-second annual joint conference of the IEEE computer and communications. IEEE societies},
	volume={2},
	pages={825--835},
	year={2003},
	organization={IEEE}
}


@inproceedings{abedi2008enhancing,
	title={Enhancing AODV routing protocol using mobility parameters in VANET},
	author={Abedi, Omid and Fathy, Mahmood and Taghiloo, Jamshid},
	booktitle={Computer Systems and Applications, 2008. AICCSA 2008. IEEE/ACS International Conference on},
	pages={229--235},
	year={2008},
	organization={IEEE}
}


@article{AlSultan2013Journal,
	Author = {Al-Sultan, Saif and Al-Bayatti, Ali H. and Zedan, Hussien},
	Journal = {IEEE Transactions on Vehicular Technology},
	Number = {9},
	Pages = {4264-4275},
	Publisher = {IEEE},
	Title = {Context Aware Driver Behaviour Detection System in Intelligent Transportation Systems},
	Volume = {62},
	Year = {2013}}






@article{Leow2008ITS,
	Author = {Leow, Woei Ling and Ni, Daiheng and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Intelligent Transportation Systems},
	Number = {2},
	Pages = {369--374},
	Publisher = {IEEE},
	Title = {A Sampling Theorem Approach to Traffic Sensor Optimization},
	Volume = {9},
	Year = {2008}}



@article{REU2007,
	Author = {D. Ni and H. Pishro-Nik and R. Prasad and M. R. Kanjee and H. Zhu and T. Nguyen},
	Journal = {in 14th World Congress on Intelligent Transport Systems},
	Title = {Development of a prototype intersection collision avoidance system under VII},
	Year = {2007}}




@inproceedings{salamatian2013hide,
	title={How to hide the elephant-or the donkey-in the room: Practical privacy against statistical inference for large data.},
	author={Salamatian, Salman and Zhang, Amy and du Pin Calmon, Flavio and Bhamidipati, Sandilya and Fawaz, Nadia and Kveton, Branislav and Oliveira, Pedro and Taft, Nina},
	booktitle={GlobalSIP},
	pages={269--272},
	year={2013}
}

@article{sankar2013utility,
	title={Utility-privacy tradeoffs in databases: An information-theoretic approach},
	author={Sankar, Lalitha and Rajagopalan, S Raj and Poor, H Vincent},
	journal={Information Forensics and Security, IEEE Transactions on},
	volume={8},
	number={6},
	pages={838--852},
	year={2013},
	publisher={IEEE}
}
@inproceedings{ghinita2007prive,
	title={PRIVE: anonymous location-based queries in distributed mobile systems},
	author={Ghinita, Gabriel and Kalnis, Panos and Skiadopoulos, Spiros},
	booktitle={Proceedings of the 16th international conference on World Wide Web},
	pages={371--380},
	year={2007},
	organization={ACM}
}

@article{beresford2004mix,
	title={Mix zones: User privacy in location-aware services},
	author={Beresford, Alastair R and Stajano, Frank},
	year={2004},
	publisher={IEEE}
}

%@inproceedings{Mont1610Achieving,
	%  title={Achieving Perfect Location Privacy in Markov Models Using Anonymization},
	%  author={Montazeri, Zarrin and Houmansadr, Amir and H.Pishro-Nik},
	%  booktitle="2016 International Symposium on Information Theory and its Applications
	%  (ISITA2016)",
	%  address="Monterey, USA",
	%  days=30,
	%  month=oct,
	%  year=2016,
	%}

@article{csiszar1996almost,
	title={Almost independence and secrecy capacity},
	author={Csisz{\'a}r, Imre},
	journal={Problemy Peredachi Informatsii},
	volume={32},
	number={1},
	pages={48--57},
	year={1996},
	publisher={Russian Academy of Sciences, Branch of Informatics, Computer Equipment and Automatization}
}

@article{yamamoto1983source,
	title={A source coding problem for sources with additional outputs to keep secret from the receiver or wiretappers (corresp.)},
	author={Yamamoto, Hirosuke},
	journal={IEEE Transactions on Information Theory},
	volume={29},
	number={6},
	pages={918--923},
	year={1983},
	publisher={IEEE}
}


@inproceedings{calmon2015fundamental,
	title={Fundamental limits of perfect privacy},
	author={Calmon, Flavio P and Makhdoumi, Ali and M{\'e}dard, Muriel},
	booktitle={Information Theory (ISIT), 2015 IEEE International Symposium on},
	pages={1796--1800},
	year={2015},
	organization={IEEE}
}



@inproceedings{Lehman1999Large-Sample-Theory,
	title={Elements of Large Sample Theory},
	author={E. L. Lehman},
	organization={Springer},
	year={1999}
}


@inproceedings{Ferguson1999Large-Sample-Theory,
	title={A Course in Large Sample Theory},
	author={Thomas S. Ferguson},
	organization={CRC Press},
	year={1996}
}



@inproceedings{Dembo1999Large-Deviations,
	title={Large Deviation Techniques and Applications, Second Edition},
	author={A. Dembo and O. Zeitouni},
	organization={Springer},
	year={1998}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Hossein's Coding Journals
%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{myoptics,
	AUTHOR =       "H. Pishro-Nik and N. Rahnavard and J. Ha and F. Fekri and A. Adibi ",
	TITLE =        "Low-density parity-check codes for volume holographic memory systems",
	JOURNAL =      " Appl. Opt.",
	YEAR =         "2003",
	volume =       "42",
	pages =        "861-870  "
}






@ARTICLE{myit,
	AUTHOR =       "H. Pishro-Nik and F. Fekri  ",
	TITLE =        "On Decoding of Low-Density Parity-Check Codes on the Binary Erasure Channel",
	JOURNAL =      "IEEE Trans. Inform. Theory",
	YEAR =         "2004",
	volume =       "50",
	pages =        "439--454"
}




@ARTICLE{myitpuncture,
	AUTHOR =       "H. Pishro-Nik and F. Fekri  ",
	TITLE =        "Results on Punctured Low-Density Parity-Check Codes and Improved Iterative Decoding Techniques",
	JOURNAL =      "IEEE Trans. on Inform. Theory",
	YEAR =         "2007",
	volume =       "53",
	number=        "2",
	pages =        "599--614",
	month= "February"
}




@ARTICLE{myitlinmimdist,
	AUTHOR =       "H. Pishro-Nik and F. Fekri",
	TITLE =        "Performance of Low-Density Parity-Check Codes With Linear Minimum Distance",
	JOURNAL =         "IEEE Trans. Inform. Theory ",
	YEAR =         "2006",
	volume =       "52",
	number="1",
	pages =        "292 --300"
}






@ARTICLE{myitnonuni,
	AUTHOR =       "H. Pishro-Nik and N. Rahnavard and F. Fekri  ",
	TITLE =        "Non-uniform Error Correction Using Low-Density Parity-Check Codes",
	JOURNAL =      "IEEE Trans. Inform. Theory",
	YEAR =         "2005",
	volume =       "51",
	number=  "7",
	pages =        "2702--2714"
}





@article{eslamitcomhybrid10,
	author = {A. Eslami and S. Vangala and H. Pishro-Nik},
	title = {Hybrid channel codes for highly efficient FSO/RF communication systems},
	journal = {IEEE Transactions on Communications},
	volume = {58},
	number = {10},
	year = {2010},
	pages = {2926--2938},
}


@article{eslamitcompolar13,
	author = {A. Eslami and H. Pishro-Nik},
	title = {On Finite-Length Performance of Polar Codes: Stopping Sets, Error Floor, and Concatenated Design},
	journal = {IEEE Transactions on Communications},
	volume = {61},
	number = {13},
	year = {2013},
	pages = {919--929},
}



@article{saeeditcom11,
	author = {H. Saeedi and H. Pishro-Nik and  A. H. Banihashemi},
	title = {Successive maximization for the systematic design of universally capacity approaching rate-compatible
	sequences of LDPC code ensembles over binary-input output-symmetric memoryless channels},
	journal = {IEEE Transactions on Communications},
	year = {2011},
	volume={59},
	number = {7}
}


@article{rahnavard07,
	author = {Rahnavard, N. and Pishro-Nik, H. and Fekri, F.},
	title = {Unequal Error Protection Using Partially Regular LDPC Codes},
	journal = {IEEE Transactions on Communications},
	year = {2007},
	volume = {55},
	number = {3},
	pages = {387 -- 391}
}


@article{hosseinira04,
	author = {H. Pishro-Nik and F. Fekri},
	title = {Irregular repeat-accumulate codes for volume holographic memory systems},
	journal = {Journal of Applied Optics},
	year = {2004},
	volume = {43},
	number = {27},
	pages = {5222--5227},
}


@article{azadeh2015Ephemeralkey,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
	journal = {IEEE Transactions on Wireless Communications},
	year = {2015},
	volume = {14},
	number = {11},
	pages = {6072--6081},
}


@article{azadeh2014Everlasting,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Everlasting secrecy in disadvantaged wireless environments against sophisticated eavesdroppers},
	journal = {48th Asilomar Conference on Signals, Systems and Computers},
	year = {2014},
	pages = {1994--1998},
}


@article{azadeh2013ISIT,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Artificial intersymbol interference (ISI) to exploit receiver imperfections for secrecy},
	journal = {IEEE International Symposium on Information Theory (ISIT)},
	year = {2013},
}


@article{azadeh2013Jsac,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
	journal = {IEEE Journal on Selected Areas in Communications},
	year = {2013},
	volume = {31},
	number = {9},
	pages = {1828--1839},
}


@article{azadeh2012Allerton,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Exploiting the non-commutativity of nonlinear operators for information-theoretic security in disadvantaged wireless environments},
	journal = {50th Annual Allerton Conference on Communication, Control, and Computing},
	year = {2012},
	pages = {233--240},
}


@article{azadeh2012Infocom,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
	journal = {IEEE INFOCOM},
	year = {2012},
	pages = {1179--1187},
}

@article{1corser2016evaluating,
	title={Evaluating Location Privacy in Vehicular Communications and Applications},
	author={Corser, George P and Fu, Huirong and Banihani, Abdelnasser},
	journal={IEEE Transactions on Intelligent Transportation Systems},
	volume={17},
	number={9},
	pages={2658-2667},
	year={2016},
	publisher={IEEE}
}
@article{2zhang2016designing,
	title={On Designing Satisfaction-Ratio-Aware Truthful Incentive Mechanisms for k-Anonymity Location Privacy},
	author={Zhang, Yuan and Tong, Wei and Zhong, Sheng},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={11},
	number={11},
	pages={2528--2541},
	year={2016},
	publisher={IEEE}
}
@article{3li2016privacy,
	title={Privacy-preserving Location Proof for Securing Large-scale Database-driven Cognitive Radio Networks},
	author={Li, Yi and Zhou, Lu and Zhu, Haojin and Sun, Limin},
	journal={IEEE Internet of Things Journal},
	volume={3},
	number={4},
	pages={563-571},
	year={2016},
	publisher={IEEE}
}
@article{4olteanu2016quantifying,
	title={Quantifying Interdependent Privacy Risks with Location Data},
	author={Olteanu, Alexandra-Mihaela and Huguenin, K{\'e}vin and Shokri, Reza and Humbert, Mathias and Hubaux, Jean-Pierre},
	journal={IEEE Transactions on Mobile Computing},
	year={2016},
	volume={PP},
	number={99},
	pages={1-1},
	publisher={IEEE}
}
@article{5yi2016practical,
	title={Practical Approximate k Nearest Neighbor Queries with Location and Query Privacy},
	author={Yi, Xun and Paulet, Russell and Bertino, Elisa and Varadharajan, Vijay},
	journal={IEEE Transactions on Knowledge and Data Engineering},
	volume={28},
	number={6},
	pages={1546--1559},
	year={2016},
	publisher={IEEE}
}
@article{6li2016privacy,
	title={Privacy Leakage of Location Sharing in Mobile Social Networks: Attacks and Defense},
	author={Li, Huaxin and Zhu, Haojin and Du, Suguo and Liang, Xiaohui and Shen, Xuemin},
	journal={IEEE Transactions on Dependable and Secure Computing},
	year={2016},
	volume={PP},
	number={99},
	publisher={IEEE}
}

@article{7murakami2016localization,
	title={Localization Attacks Using Matrix and Tensor Factorization},
	author={Murakami, Takao and Watanabe, Hajime},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={11},
	number={8},
	pages={1647--1660},
	year={2016},
	publisher={IEEE}
}
@article{8zurbaran2015near,
	title={Near-Rand: Noise-based Location Obfuscation Based on Random Neighboring Points},
	author={Zurbaran, Mayra Alejandra and Avila, Karen and Wightman, Pedro and Fernandez, Michael},
	journal={IEEE Latin America Transactions},
	volume={13},
	number={11},
	pages={3661--3667},
	year={2015},
	publisher={IEEE}
}

@article{9tan2014anti,
	title={An anti-tracking source-location privacy protection protocol in wsns based on path extension},
	author={Tan, Wei and Xu, Ke and Wang, Dan},
	journal={IEEE Internet of Things Journal},
	volume={1},
	number={5},
	pages={461--471},
	year={2014},
	publisher={IEEE}
}

@article{10peng2014enhanced,
	title={Enhanced Location Privacy Preserving Scheme in Location-Based Services},
	author={Peng, Tao and Liu, Qin and Wang, Guojun},
	journal={IEEE Systems Journal},
	year={2014},
	volume={PP},
	number={99},
	pages={1-12},
	publisher={IEEE}
}
@article{11dewri2014exploiting,
	title={Exploiting service similarity for privacy in location-based search queries},
	author={Dewri, Rinku and Thurimella, Ramakrisha},
	journal={IEEE Transactions on Parallel and Distributed Systems},
	volume={25},
	number={2},
	pages={374--383},
	year={2014},
	publisher={IEEE}
}

@article{12hwang2014novel,
	title={A novel time-obfuscated algorithm for trajectory privacy protection},
	author={Hwang, Ren-Hung and Hsueh, Yu-Ling and Chung, Hao-Wei},
	journal={IEEE Transactions on Services Computing},
	volume={7},
	number={2},
	pages={126--139},
	year={2014},
	publisher={IEEE}
}
@article{13puttaswamy2014preserving,
	title={Preserving location privacy in geosocial applications},
	author={Puttaswamy, Krishna PN and Wang, Shiyuan and Steinbauer, Troy and Agrawal, Divyakant and El Abbadi, Amr and Kruegel, Christopher and Zhao, Ben Y},
	journal={IEEE Transactions on Mobile Computing},
	volume={13},
	number={1},
	pages={159--173},
	year={2014},
	publisher={IEEE}
}

@article{14zhang2014privacy,
	title={Privacy quantification model based on the Bayes conditional risk in Location-Based Services},
	author={Zhang, Xuejun and Gui, Xiaolin and Tian, Feng and Yu, Si and An, Jian},
	journal={Tsinghua Science and Technology},
	volume={19},
	number={5},
	pages={452--462},
	year={2014},
	publisher={TUP}
}

@article{15bilogrevic2014privacy,
	title={Privacy-preserving optimal meeting location determination on mobile devices},
	author={Bilogrevic, Igor and Jadliwala, Murtuza and Joneja, Vishal and Kalkan, K{\"u}bra and Hubaux, Jean-Pierre and Aad, Imad},
	journal={IEEE transactions on information forensics and security},
	volume={9},
	number={7},
	pages={1141--1156},
	year={2014},
	publisher={IEEE}
}
@article{16haghnegahdar2014privacy,
	title={Privacy Risks in Publishing Mobile Device Trajectories},
	author={Haghnegahdar, Alireza and Khabbazian, Majid and Bhargava, Vijay K},
	journal={IEEE Wireless Communications Letters},
	volume={3},
	number={3},
	pages={241--244},
	year={2014},
	publisher={IEEE}
}
@article{17malandrino2014verification,
	title={Verification and inference of positions in vehicular networks through anonymous beaconing},
	author={Malandrino, Francesco and Borgiattino, Carlo and Casetti, Claudio and Chiasserini, Carla-Fabiana and Fiore, Marco and Sadao, Roberto},
	journal={IEEE Transactions on Mobile Computing},
	volume={13},
	number={10},
	pages={2415--2428},
	year={2014},
	publisher={IEEE}
}
@article{18shokri2014hiding,
	title={Hiding in the mobile crowd: Locationprivacy through collaboration},
	author={Shokri, Reza and Theodorakopoulos, George and Papadimitratos, Panos and Kazemi, Ehsan and Hubaux, Jean-Pierre},
	journal={IEEE transactions on dependable and secure computing},
	volume={11},
	number={3},
	pages={266--279},
	year={2014},
	publisher={IEEE}
}
@article{19freudiger2013non,
	title={Non-cooperative location privacy},
	author={Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
	journal={IEEE Transactions on Dependable and Secure Computing},
	volume={10},
	number={2},
	pages={84--98},
	year={2013},
	publisher={IEEE}
}
@article{20gao2013trpf,
	title={TrPF: A trajectory privacy-preserving framework for participatory sensing},
	author={Gao, Sheng and Ma, Jianfeng and Shi, Weisong and Zhan, Guoxing and Sun, Cong},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={8},
	number={6},
	pages={874--887},
	year={2013},
	publisher={IEEE}
}
@article{21ma2013privacy,
	title={Privacy vulnerability of published anonymous mobility traces},
	author={Ma, Chris YT and Yau, David KY and Yip, Nung Kwan and Rao, Nageswara SV},
	journal={IEEE/ACM Transactions on Networking},
	volume={21},
	number={3},
	pages={720--733},
	year={2013},
	publisher={IEEE}
}
@article{22niu2013pseudo,
	title={Pseudo-Location Updating System for privacy-preserving location-based services},
	author={Niu, Ben and Zhu, Xiaoyan and Chi, Haotian and Li, Hui},
	journal={China Communications},
	volume={10},
	number={9},
	pages={1--12},
	year={2013},
	publisher={IEEE}
}
@article{23dewri2013local,
	title={Local differential perturbations: Location privacy under approximate knowledge attackers},
	author={Dewri, Rinku},
	journal={IEEE Transactions on Mobile Computing},
	volume={12},
	number={12},
	pages={2360--2372},
	year={2013},
	publisher={IEEE}
}
@inproceedings{24kanoria2012tractable,
	title={Tractable bayesian social learning on trees},
	author={Kanoria, Yashodhan and Tamuz, Omer},
	booktitle={Information Theory Proceedings (ISIT), 2012 IEEE International Symposium on},
	pages={2721--2725},
	year={2012},
	organization={IEEE}
}
@inproceedings{25farias2005universal,
	title={A universal scheme for learning},
	author={Farias, Vivek F and Moallemi, Ciamac C and Van Roy, Benjamin and Weissman, Tsachy},
	booktitle={Proceedings. International Symposium on Information Theory, 2005. ISIT 2005.},
	pages={1158--1162},
	year={2005},
	organization={IEEE}
}
@inproceedings{26misra2013unsupervised,
	title={Unsupervised learning and universal communication},
	author={Misra, Vinith and Weissman, Tsachy},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={261--265},
	year={2013},
	organization={IEEE}
}
@inproceedings{27ryabko2013time,
	title={Time-series information and learning},
	author={Ryabko, Daniil},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={1392--1395},
	year={2013},
	organization={IEEE}
}
@inproceedings{28krzakala2013phase,
	title={Phase diagram and approximate message passing for blind calibration and dictionary learning},
	author={Krzakala, Florent and M{\'e}zard, Marc and Zdeborov{\'a}, Lenka},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={659--663},
	year={2013},
	organization={IEEE}
}
@inproceedings{29sakata2013sample,
	title={Sample complexity of Bayesian optimal dictionary learning},
	author={Sakata, Ayaka and Kabashima, Yoshiyuki},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={669--673},
	year={2013},
	organization={IEEE}
}
@inproceedings{30predd2004consistency,
	title={Consistency in a model for distributed learning with specialists},
	author={Predd, Joel B and Kulkarni, Sanjeev R and Poor, H Vincent},
	booktitle={IEEE International Symposium on Information Theory},
	year={2004},
	organization={IEEE}
}
@inproceedings{31nokleby2016rate,
	title={Rate-Distortion Bounds on Bayes Risk in Supervised Learning},
	author={Nokleby, Matthew and Beirami, Ahmad and Calderbank, Robert},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={2099-2103},
	year={2016},
	organization={IEEE}
}

@inproceedings{32le2016imperfect,
	title={Are imperfect reviews helpful in social learning?},
	author={Le, Tho Ngoc and Subramanian, Vijay G and Berry, Randall A},
	booktitle={Information Theory (ISIT), 2016 IEEE International Symposium on},
	pages={2089--2093},
	year={2016},
	organization={IEEE}
}
@inproceedings{33gadde2016active,
	title={Active Learning for Community Detection in Stochastic Block Models},
	author={Gadde, Akshay and Gad, Eyal En and Avestimehr, Salman and Ortega, Antonio},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={1889-1893},
	year={2016}
}
@inproceedings{34shakeri2016minimax,
	title={Minimax Lower Bounds for Kronecker-Structured Dictionary Learning},
	author={Shakeri, Zahra and Bajwa, Waheed U and Sarwate, Anand D},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={1148-1152},
	year={2016}
}
@article{35lee2015speeding,
	title={Speeding up distributed machine learning using codes},
	author={Lee, Kangwook and Lam, Maximilian and Pedarsani, Ramtin and Papailiopoulos, Dimitris and Ramchandran, Kannan},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={1143-1147},
	year={2016}
}
@article{36oneto2016statistical,
	title={Statistical Learning Theory and ELM for Big Social Data Analysis},
	author={Oneto, Luca and Bisio, Federica and Cambria, Erik and Anguita, Davide},
	journal={ieee CompUTATionAl inTelliGenCe mAGAzine},
	volume={11},
	number={3},
	pages={45--55},
	year={2016},
	publisher={IEEE}
}
@article{37lin2015probabilistic,
	title={Probabilistic approach to modeling and parameter learning of indirect drive robots from incomplete data},
	author={Lin, Chung-Yen and Tomizuka, Masayoshi},
	journal={IEEE/ASME Transactions on Mechatronics},
	volume={20},
	number={3},
	pages={1036--1045},
	year={2015},
	publisher={IEEE}
}
@article{38wang2016towards,
	title={Towards Bayesian Deep Learning: A Framework and Some Existing Methods},
	author={Wang, Hao and Yeung, Dit-Yan},
	journal={IEEE Transactions on Knowledge and Data Engineering},
	volume={PP},
	number={99},
	year={2016},
	publisher={IEEE}
}


%%%%%Informationtheoreticsecurity%%%%%%%%%%%%%%%%%%%%%%%




@inproceedings{Bloch2011PhysicalSecBook,
	title={Physical-Layer Security},
	author={M. Bloch and J. Barros},
	organization={Cambridge University Press},
	year={2011}
}



@inproceedings{Liang2009InfoSecBook,
	title={Information Theoretic Security},
	author={Y. Liang and H. V. Poor and S. Shamai (Shitz)},
	organization={Now Publishers Inc.},
	year={2009}
}


@inproceedings{Zhou2013PhysicalSecBook,
	title={Physical Layer Security in Wireless Communications},
	author={ X. Zhou and L. Song and Y. Zhang},
	organization={CRC Press},
	year={2013}
}

@article{Ni2012IEA,
	Author = {D. Ni and H. Liu and W. Ding and  Y. Xie and H. Wang and H. Pishro-Nik and Q. Yu},
	Journal = {IEA/AIE},
	Title = {Cyber-Physical Integration to Connect Vehicles for Transformed Transportation Safety and Efficiency},
	Year = {2012}}



@inproceedings{Ni2012Inproceedings,
	Author = {D. Ni, H. Liu, Y. Xie, W. Ding, H. Wang, H. Pishro-Nik, Q. Yu and M. Ferreira},
	Booktitle = {Spring Simulation Multiconference},
	Date-Added = {2016-09-04 14:18:42 +0000},
	Date-Modified = {2016-09-06 16:22:14 +0000},
	Title = {Virtual Lab of Connected Vehicle Technology},
	Year = {2012}}

@inproceedings{Ni2012Inproceedings,
	Author = {D. Ni, H. Liu, W. Ding, Y. Xie, H. Wang, H. Pishro-Nik and Q. Yu,},
	Booktitle = {IEA/AIE},
	Date-Added = {2016-09-04 09:11:02 +0000},
	Date-Modified = {2016-09-06 14:46:53 +0000},
	Title = {Cyber-Physical Integration to Connect Vehicles for Transformed Transportation Safety and Efficiency},
	Year = {2012}}


@article{Nekoui_IJIPT_2009,
	Author = {M. Nekoui and D. Ni and H. Pishro-Nik and R. Prasad and M. Kanjee and H. Zhu and T. Nguyen},
	Journal = {International Journal of Internet Protocol Technology (IJIPT)},
	Number = {3},
	Pages = {},
	Publisher = {},
	Title = {Development of a VII-Enabled Prototype Intersection Collision Warning System},
	Volume = {4},
	Year = {2009}}


@inproceedings{Pishro_Ganz_Ni,
	Author = {H. Pishro-Nik, A. Ganz, and Daiheng Ni},
	Booktitle = {Forty-Fifth Annual Allerton Conference on Communication, Control, and Computing. Allerton House, Monticello, IL},
	Date-Added = {},
	Date-Modified = {},
	Number = {},
	Pages = {},
	Title = {The capacity of vehicular ad hoc networks},
	Volume = {},
	Year = {September 26-28, 2007}}

@inproceedings{Leow_Pishro_Ni_1,
	Author = {W. L. Leow, H. Pishro-Nik and Daiheng Ni},
	Booktitle = {IEEE Global Telecommunications Conference, Washington, D.C.},
	Date-Added = {},
	Date-Modified = {},
	Number = {},
	Pages = {},
	Title = {Delay and Energy Tradeoff in Multi-state Wireless Sensor Networks},
	Volume = {},
	Year = {November 26-30, 2007}}


@misc{UMass-Trans,
	title = {{UMass Transportation Center}},
	note = {\url{http://www.umasstransportationcenter.org/}},
}


@inproceedings{Haenggi2013book,
	title={Stochastic geometry for wireless networks},
	author={M. Haenggi},
	organization={Cambridge Uinversity Press},
	year={2013}
}


%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Created for Zarrin Montazeri at 2015-11-09 18:45:31 -0500


%% Saved with string encoding Unicode (UTF-8)


%%%%%%%%%%%%%%%%personalization%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{osma2015,
	title={Impact of Time-to-Collision Information on Driving Behavior in Connected Vehicle Environments Using A Driving Simulator Test Bed},
	journal{Journal of Traffic and Logistics Engineering},
	author={Osama A. Osman, Julius Codjoe, and Sherif Ishak},
	volume={3},
	number={1},
	 pages={18--24},
	year={2015}
}


@article{charisma2010,
	title={Dynamic Latent Plan Models},
	author={Charisma F. Choudhurya, Moshe Ben-Akivab and Maya Abou-Zeid},
	journal={Journal of Choice Modelling},
	volume={3},
	number={2},
	pages={50--70},
	year={2010},
	publisher={Elsvier}
}


@misc{noble2014,
	author = {A. M. Noble, Shane B. McLaughlin, Zachary R. Doerzaph and Thomas A. Dingus},
	title = {Crowd-sourced Connected-vehicle Warning Algorithm using Naturalistic Driving Data},
	howpublished = {Downloaded from \url{http://hdl.handle.net/10919/53978}},

	month = August,
	year = 2014
}


@phdthesis{charisma2007,
	title    = {Modeling Driving Decisions with Latent Plans},
	school   = {Massachusetts Institute of Technology },
	author   = {Charisma Farheen Choudhury},
	year     = {2007}, %other attributes omitted
}


@article{chrysler2015,
	title={Cost of Warning of Unseen Threats:Unintended Consequences of Connected Vehicle Alerts},
	author={S. T. Chrysler, J. M. Cooper and D. C. Marshall},
	journal={Transportation Research Record: Journal of the Transportation Research Board},
	volume={2518},
	pages={79--85},
	year={2015},
}

@misc{nsf_cps,
        title = {Cyber-Physical Systems (CPS) PROGRAM SOLICITATION NSF 17-529},
        howpublished = {Downloaded from \url{https://www.nsf.gov/publications/pub_summ.jsp?WT.z_pims_id=503286&ods_key=nsf17529}},
}



%%%%%%%%%%%%%%IOT%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




@article{FTC2015,
  title={Internet of Things: Privacy and Security in a Connected World},
  author={FTC Staff Report},
  year={2015}
}



@article{0Quest2016,
  title={The Quest for Privacy in the Internet of Things},
  author={ Pawani Porambag and Mika Ylianttila and Corinna Schmitt and  Pardeep Kumar and  Andrei Gurtov and  Athanasios V. Vasilakos},
  journal={IEEE Cloud Computing},
  volum={3},
  number={2},
  year={2016},
  publisher={IEEE}
}

%% Saved with string encoding Unicode (UTF-8)
@inproceedings{1zhou2014security,
  title={Security/privacy of wearable fitness tracking {I}o{T} devices},
  author={Zhou, Wei and Piramuthu, Selwyn},
  booktitle={Information Systems and Technologies (CISTI), 2014 9th Iberian Conference on},
  pages={1--5},
  year={2014},
  organization={IEEE}
}


@inproceedings{3ukil2014iot,
  title={{I}o{T}-privacy: To be private or not to be private},
  author={Ukil, Arijit and Bandyopadhyay, Soma and Pal, Arpan},
  booktitle={Computer Communications Workshops (INFOCOM WKSHPS), IEEE Conference on},
  pages={123--124},
  year={2014},
  organization={IEEE}
}


@article{4arias2015privacy,
  title={Privacy and security in internet of things and wearable devices},
  author={Arias, Orlando and Wurm, Jacob and Hoang, Khoa and Jin, Yier},
  journal={IEEE Transactions on Multi-Scale Computing Systems},
  volume={1},
  number={2},
  pages={99--109},
  year={2015},
  publisher={IEEE}
}
@inproceedings{5ullah2016novel,
  title={A novel model for preserving Location Privacy in Internet of Things},
  author={Ullah, Ikram and Shah, Munam Ali},
  booktitle={Automation and Computing (ICAC), 2016 22nd International Conference on},
  pages={542--547},
  year={2016},
  organization={IEEE}
}
@inproceedings{6sathishkumar2016enhanced,
  title={Enhanced location privacy algorithm for wireless sensor network in Internet of Things},
  author={Sathishkumar, J and Patel, Dhiren R},
  booktitle={Internet of Things and Applications (IOTA), International Conference on},
  pages={208--212},
  year={2016},
  organization={IEEE}
}
@inproceedings{7zhou2012preserving,
  title={Preserving sensor location privacy in internet of things},
  author={Zhou, Liming and Wen, Qiaoyan and Zhang, Hua},
  booktitle={Computational and Information Sciences (ICCIS), 2012 Fourth International Conference on},
  pages={856--859},
  year={2012},
  organization={IEEE}
}

@inproceedings{8ukil2015privacy,
  title={Privacy for {I}o{T}: Involuntary privacy enablement for smart energy systems},
  author={Ukil, Arijit and Bandyopadhyay, Soma and Pal, Arpan},
  booktitle={Communications (ICC), 2015 IEEE International Conference on},
  pages={536--541},
  year={2015},
  organization={IEEE}
}

@inproceedings{9dalipi2016security,
  title={Security and Privacy Considerations for {I}o{T} Application on Smart Grids: Survey and Research Challenges},
  author={Dalipi, Fisnik and Yayilgan, Sule Yildirim},
  booktitle={Future Internet of Things and Cloud Workshops (FiCloudW), IEEE International Conference on},
  pages={63--68},
  year={2016},
  organization={IEEE}
}
@inproceedings{10harris2016security,
  title={Security and Privacy in Public {I}o{T} Spaces},
  author={Harris, Albert F and Sundaram, Hari and Kravets, Robin},
  booktitle={Computer Communication and Networks (ICCCN), 2016 25th International Conference on},
  pages={1--8},
  year={2016},
  organization={IEEE}
}

@inproceedings{11al2015security,
  title={Security and privacy framework for ubiquitous healthcare {I}o{T} devices},
  author={Al Alkeem, Ebrahim and Yeun, Chan Yeob and Zemerly, M Jamal},
  booktitle={Internet Technology and Secured Transactions (ICITST), 2015 10th International Conference for},
  pages={70--75},
  year={2015},
  organization={IEEE}
}
@inproceedings{12sivaraman2015network,
  title={Network-level security and privacy control for smart-home {I}o{T} devices},
  author={Sivaraman, Vijay and Gharakheili, Hassan Habibi and Vishwanath, Arun and Boreli, Roksana and Mehani, Olivier},
  booktitle={Wireless and Mobile Computing, Networking and Communications (WiMob), 2015 IEEE 11th International Conference on},
  pages={163--167},
  year={2015},
  organization={IEEE}
}

@inproceedings{13srinivasan2016privacy,
  title={Privacy conscious architecture for improving emergency response in smart cities},
  author={Srinivasan, Ramya and Mohan, Apurva and Srinivasan, Priyanka},
  booktitle={Smart City Security and Privacy Workshop (SCSP-W), 2016},
  pages={1--5},
  year={2016},
  organization={IEEE}
}
@inproceedings{14sadeghi2015security,
  title={Security and privacy challenges in industrial internet of things},
  author={Sadeghi, Ahmad-Reza and Wachsmann, Christian and Waidner, Michael},
  booktitle={Design Automation Conference (DAC), 2015 52nd ACM/EDAC/IEEE},
  pages={1--6},
  year={2015},
  organization={IEEE}
}
@inproceedings{15otgonbayar2016toward,
  title={Toward Anonymizing {I}o{T} Data Streams via Partitioning},
  author={Otgonbayar, Ankhbayar and Pervez, Zeeshan and Dahal, Keshav},
  booktitle={Mobile Ad Hoc and Sensor Systems (MASS), 2016 IEEE 13th International Conference on},
  pages={331--336},
  year={2016},
  organization={IEEE}
}
@inproceedings{16rutledge2016privacy,
  title={Privacy Impacts of {I}o{T} Devices: A SmartTV Case Study},
  author={Rutledge, Richard L and Massey, Aaron K and Ant{\'o}n, Annie I},
  booktitle={Requirements Engineering Conference Workshops (REW), IEEE International},
  pages={261--270},
  year={2016},
  organization={IEEE}
}

@inproceedings{17andrea2015internet,
  title={Internet of Things: Security vulnerabilities and challenges},
  author={Andrea, Ioannis and Chrysostomou, Chrysostomos and Hadjichristofi, George},
  booktitle={Computers and Communication (ISCC), 2015 IEEE Symposium on},
  pages={180--187},
  year={2015},
  organization={IEEE}
}






























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@misc{epfl-mobility-20090224,
    author = {Michal Piorkowski and Natasa Sarafijanovic-Djukic and Matthias Grossglauser},
    title = {{CRAWDAD} dataset epfl/mobility (v. 2009-02-24)},
    howpublished = {Downloaded from \url{http://crawdad.org/epfl/mobility/20090224}},
    doi = {10.15783/C7J010},
    month = feb,
    year = 2009
}

@misc{roma-taxi-20140717,
    author = {Lorenzo Bracciale and Marco Bonola and Pierpaolo Loreti and Giuseppe Bianchi and Raul Amici and Antonello Rabuffi},
    title = {{CRAWDAD} dataset roma/taxi (v. 2014-07-17)},
    howpublished = {Downloaded from \url{http://crawdad.org/roma/taxi/20140717}},
    doi = {10.15783/C7QC7M},
    month = jul,
    year = 2014
}

@misc{rice-ad_hoc_city-20030911,
    author = {Jorjeta G. Jetcheva and Yih-Chun Hu and Santashil PalChaudhuri and Amit Kumar Saha and David B. Johnson},
    title = {{CRAWDAD} dataset rice/ad\_hoc\_city (v. 2003-09-11)},
    howpublished = {Downloaded from \url{http://crawdad.org/rice/ad_hoc_city/20030911}},
    doi = {10.15783/C73K5B},
    month = sep,
    year = 2003
}

@misc{china:2012,
author = {Microsoft Research Asia},
title = {GeoLife GPS Trajectories},
year = {2012},
howpublished= {\url{https://www.microsoft.com/en-us/download/details.aspx?id=52367}},
}


@misc{china:2011,
ALTauthor = {Microsoft Research Asia)},
ALTeditor = {},
title = {GeoLife GPS Trajectories,
year = {2012},
url = {https://www.microsoft.com/en-us/download/details.aspx?id=52367},
}


@misc{longversion,
  author = {N. Takbiri and A. Houmansadr and D.L. Goeckel and H. Pishro-Nik},
  title = {{Limits of Location Privacy under Anonymization and Obfuscation}},
  howpublished = "\url{http://www.ecs.umass.edu/ece/pishro/Papers/ISIT_2017-2.pdf}",
  year = 2017,
month= "January",
  note = "Summarized version submitted to IEEE ISIT 2017"
}

@misc{isit_ke,
  author = {K. Li and D. Goeckel and H. Pishro-Nik},
  title = {{Bayesian Time Series Matching and Privacy}},
  note = "submitted to IEEE ISIT 2017"
}

@article{matching,
  title={Asymptotically Optimal Matching of Multiple Sequences to Source Distributions and Training Sequences},
  author={Jayakrishnan Unnikrishnan},
  journal={ IEEE Transactions on Information Theory},
  volume={61},
  number={1},
  pages={452-468},
  year={2015},
  publisher={IEEE}
}


@article{Naini2016,
	Author = {F. Naini and J. Unnikrishnan and P. Thiran and M. Vetterli},
	Journal = {IEEE Transactions on Information Forensics and Security},
	Publisher = {IEEE},
	Title = {Where You Are Is Who You Are: User Identification by Matching Statistics},
	 volume={11},
    number={2},
     pages={358--372},
    Year = {2016}
}



@inproceedings{holowczak2015cachebrowser,
  title={{CacheBrowser: Bypassing Chinese Censorship without Proxies Using Cached Content}},
  author={Holowczak, John and Houmansadr, Amir},
  booktitle={Proceedings of the 22nd ACM SIGSAC Conference on Computer and Communications Security},
  pages={70--83},
  year={2015},
  organization={ACM}
}
@misc{cb-website,
	Howpublished = {\url{https://cachebrowser.net/#/}},
	Title = {{CacheBrowser}},
	key={cachebrowser}
}

@inproceedings{GameOfDecoys,
 title={{GAME OF DECOYS: Optimal Decoy Routing Through Game Theory}},
 author={Milad Nasr and Amir Houmansadr},
 booktitle={The $23^{rd}$ ACM Conference on Computer and Communications Security (CCS)},
 year={2016}
}

@inproceedings{CDNReaper,
 title={{Practical Censorship Evasion Leveraging Content Delivery Networks}},
 author={Hadi Zolfaghari and Amir Houmansadr},
 booktitle={The $23^{rd}$ ACM Conference on Computer and Communications Security (CCS)},
 year={2016}
}

@misc{Leberknight2010,
	Author = {Leberknight, C. and Chiang, M. and Poor, H. and Wong, F.},
	Howpublished = {\url{http://www.princeton.edu/~chiangm/anticensorship.pdf}},
	Title = {{A Taxonomy of Internet Censorship and Anti-censorship}},
	Year = {2010}}

@techreport{ultrasurf-analysis,
	Author = {Appelbaum, Jacob},
	Institution = {The Tor Project},
	Title = {{Technical analysis of the Ultrasurf proxying software}},
	Url = {http://scholar.google.com/scholar?hl=en\&btnG=Search\&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software\#0},
	Year = {2012},
	Bdsk-Url-1 = {http://scholar.google.com/scholar?hl=en%5C&btnG=Search%5C&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software%5C#0}}

@misc{gifc:07,
	Howpublished = {\url{http://www.internetfreedom.org/archive/Defeat\_Internet\_Censorship\_White\_Paper.pdf}},
	Key = {defeatcensorship},
	Publisher = {Global Internet Freedom Consortium (GIFC)},
	Title = {{Defeat Internet Censorship: Overview of Advanced Technologies and Products}},
	Type = {White Paper},
	Year = {2007}}

@article{pan2011survey,
	Author = {Pan, J. and Paul, S. and Jain, R.},
	Journal = {Communications Magazine, IEEE},
	Number = {7},
	Pages = {26--36},
	Publisher = {IEEE},
	Title = {{A Survey of the Research on Future Internet Architectures}},
	Volume = {49},
	Year = {2011}}

@misc{nsf-fia,
	Howpublished = {\url{http://www.nets-fia.net/}},
	Key = {FIA},
	Title = {{NSF Future Internet Architecture Project}}}

@misc{NDN,
	Howpublished = {\url{http://www.named- data.net}},
	Key = {NDN},
	Title = {{Named Data Networking Project}}}

@inproceedings{MobilityFirst,
	Author = {Seskar, I. and Nagaraja, K. and Nelson, S. and Raychaudhuri, D.},
	Booktitle = {Asian Internet Engineering Conference},
	Title = {{Mobilityfirst Future internet Architecture Project}},
	Year = {2011}}

@incollection{NEBULA,
	Author = {Anderson, T. and Birman, K. and Broberg, R. and Caesar, M. and Comer, D. and Cotton, C. and Freedman, M.~J. and Haeberlen, A. and Ives, Z.~G. and Krishnamurthy, A. and others},
	Booktitle = {The Future Internet},
	Pages = {16--26},
	Publisher = {Springer},
	Title = {{The NEBULA Future Internet Architecture}},
	Year = {2013}}

@inproceedings{XIA,
	Author = {Anand, A. and Dogar, F. and Han, D. and Li, B. and Lim, H. and Machado, M. and Wu, W. and Akella, A. and Andersen, D.~G. and Byers, J.~W. and others},
	Booktitle = {ACM Workshop on Hot Topics in Networks},
	Pages = {2},
	Title = {{XIA: An Architecture for an Evolvable and Trustworthy Internet}},
	Year = {2011}}

@inproceedings{ChoiceNet,
	Author = {Rouskas, G.~N. and Baldine, I. and Calvert, K.~L. and Dutta, R. and Griffioen, J. and Nagurney, A. and Wolf, T.},
	Booktitle = {ONDM},
	Title = {{ChoiceNet: Network Innovation Through Choice}},
	Year = {2013}}

@misc{nsf-find,
	Howpublished = {http://www.nets-find.net/},
	Title = {{NSF NeTS FIND Initiative}}}

@article{traid,
	Author = {Cheriton, D.~R. and Gritter, M.},
	Title = {{TRIAD: A New Next-Generation Internet Architecture}},
	Year = {2000}}

@inproceedings{dona,
	Author = {Koponen, T. and Chawla, M. and Chun, B-G. and Ermolinskiy, A. and Kim, K.~H. and Shenker, S. and Stoica, I.},
	Booktitle = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Organization = {ACM},
	Pages = {181--192},
	Title = {{A Data-Oriented (and Beyond) Network Architecture}},
	Volume = {37},
	Year = {2007}}

@misc{ultrasurf,
	Howpublished = {\url{http://www.ultrareach.com}},
	Key = {ultrasurf},
	Title = {{Ultrasurf}}}

@misc{tor-bridge,
	Author = {Dingledine, R. and Mathewson, N.},
	Howpublished = {\url{https://svn.torproject.org/svn/projects/design-paper/blocking.html}},
	Title = {{Design of a Blocking-Resistant Anonymity System}}}

@inproceedings{McLachlanH09,
	Author = {J. McLachlan and N. Hopper},
	Booktitle = {WPES},
	Title = {{On the Risks of Serving Whenever You Surf: Vulnerabilities in Tor's Blocking Resistance Design}},
	Year = {2009}}

@inproceedings{mahdian2010,
	Author = {Mahdian, M.},
	Booktitle = {{Fun with Algorithms}},
	Title = {{Fighting Censorship with Algorithms}},
	Year = {2010}}

@inproceedings{McCoy2011,
	Author = {McCoy, D. and Morales, J.~A. and Levchenko, K.},
	Booktitle = {FC},
	Title = {{Proximax: A Measurement Based System for Proxies Dissemination}},
	Year = {2011}}

@inproceedings{Sovran2008,
	Author = {Sovran, Y. and Libonati, A. and Li, J.},
	Booktitle = {IPTPS},
	Title = {{Pass it on: Social Networks Stymie Censors}},
	Year = {2008}}

@inproceedings{rbridge,
	Author = {Wang, Q. and Lin, Zi and Borisov, N. and Hopper, N.},
	Booktitle = {{NDSS}},
	Title = {{rBridge: User Reputation based Tor Bridge Distribution with Privacy Preservation}},
	Year = {2013}}

@inproceedings{telex,
	Author = {Wustrow, E. and Wolchok, S. and Goldberg, I. and Halderman, J.},
	Booktitle = {{USENIX Security}},
	Title = {{Telex: Anticensorship in the Network Infrastructure}},
	Year = {2011}}

@inproceedings{cirripede,
	Author = {Houmansadr, A. and Nguyen, G. and Caesar, M. and Borisov, N.},
	Booktitle = {CCS},
	Title = {{Cirripede: Circumvention Infrastructure Using Router Redirection with Plausible Deniability}},
	Year = {2011}}

@inproceedings{decoyrouting,
	Author = {Karlin, J. and Ellard, D. and Jackson, A. and Jones, C. and Lauer, G. and Mankins, D. and Strayer, W.},
	Booktitle = {{FOCI}},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = {2011}}

@inproceedings{routing-around-decoys,
	Author = {M.~Schuchard and J.~Geddes and C.~Thompson and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Routing Around Decoys}},
	Year = {2012}}

@inproceedings{parrot,
	Author = {A. Houmansadr and C. Brubaker and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{The Parrot is Dead: Observing Unobservable Network Communications}},
	Year = {2013}}

@misc{knock,
	Author = {T. Wilde},
	Howpublished = {\url{https://blog.torproject.org/blog/knock-knock-knockin-bridges-doors}},
	Title = {{Knock Knock Knockin' on Bridges' Doors}},
	Year = {2012}}

@inproceedings{china-tor,
	Author = {Winter, P. and Lindskog, S.},
	Booktitle = {{FOCI}},
	Title = {{How the Great Firewall of China Is Blocking Tor}},
	Year = {2012}}

@misc{discover-bridge,
	Howpublished = {\url{https://blog.torproject.org/blog/research-problems-ten-ways-discover-tor-bridges}},
	Key = {tenways},
	Title = {{Ten Ways to Discover Tor Bridges}}}

@inproceedings{freewave,
	Author = {A.~Houmansadr and T.~Riedl and N.~Borisov and A.~Singer},
	Booktitle = {{NDSS}},
	Title = {{I Want My Voice to Be Heard: IP over Voice-over-IP for Unobservable Censorship Circumvention}},
	Year = 2013}

@inproceedings{censorspoofer,
	Author = {Q. Wang and X. Gong and G. Nguyen and A. Houmansadr and N. Borisov},
	Booktitle = {CCS},
	Title = {{CensorSpoofer: Asymmetric Communication Using IP Spoofing for Censorship-Resistant Web Browsing}},
	Year = {2012}}

@inproceedings{skypemorph,
	Author = {H. Moghaddam and B. Li and M. Derakhshani and I. Goldberg},
	Booktitle = {CCS},
	Title = {{SkypeMorph: Protocol Obfuscation for Tor Bridges}},
	Year = {2012}}

@inproceedings{stegotorus,
	Author = {Weinberg, Z. and Wang, J. and Yegneswaran, V. and Briesemeister, L. and Cheung, S. and Wang, F. and Boneh, D.},
	Booktitle = {CCS},
	Title = {{StegoTorus: A Camouflage Proxy for the Tor Anonymity System}},
	Year = {2012}}

@techreport{dust,
	Author = {{B.~Wiley}},
	Howpublished = {\url{http://blanu.net/ Dust.pdf}},
	Institution = {School of Information, University of Texas at Austin},
	Title = {{Dust: A Blocking-Resistant Internet Transport Protocol}},
	Year = {2011}}

@inproceedings{FTE,
	Author = {K.~Dyer and S.~Coull and T.~Ristenpart and T.~Shrimpton},
	Booktitle = {CCS},
	Title = {{Protocol Misidentification Made Easy with Format-Transforming Encryption}},
	Year = {2013}}

@inproceedings{fp,
	Author = {Fifield, D. and Hardison, N. and Ellithrope, J. and Stark, E. and Dingledine, R. and Boneh, D. and Porras, P.},
	Booktitle = {PETS},
	Title = {{Evading Censorship with Browser-Based Proxies}},
	Year = {2012}}

@misc{obfsproxy,
	Howpublished = {\url{https://www.torproject.org/projects/obfsproxy.html.en}},
	Key = {obfsproxy},
	Publisher = {The Tor Project},
	Title = {{A Simple Obfuscating Proxy}}}

@inproceedings{Tor-instead-of-IP,
	Author = {Liu, V. and Han, S. and Krishnamurthy, A. and Anderson, T.},
	Booktitle = {HotNets},
	Title = {{Tor instead of IP}},
	Year = {2011}}

@misc{roger-slides,
	Howpublished = {\url{https://svn.torproject.org/svn/projects/presentations/slides-28c3.pdf}},
	Key = {torblocking},
	Title = {{How Governments Have Tried to Block Tor}}}

@inproceedings{infranet,
	Author = {Feamster, N. and Balazinska, M. and Harfst, G. and Balakrishnan, H. and Karger, D.},
	Booktitle = {USENIX Security},
	Title = {{Infranet: Circumventing Web Censorship and Surveillance}},
	Year = {2002}}

@inproceedings{collage,
	Author = {S.~Burnett and N.~Feamster and S.~Vempala},
	Booktitle = {USENIX Security},
	Title = {{Chipping Away at Censorship Firewalls with User-Generated Content}},
	Year = {2010}}

@article{anonymizer,
	Author = {Boyan, J.},
	Journal = {Computer-Mediated Communication Magazine},
	Month = sep,
	Number = {9},
	Title = {{The Anonymizer: Protecting User Privacy on the Web}},
	Volume = {4},
	Year = {1997}}

@article{schulze2009internet,
	Author = {Schulze, H. and Mochalski, K.},
	Journal = {IPOQUE Report},
	Pages = {351--362},
	Title = {Internet Study 2008/2009},
	Volume = {37},
	Year = {2009}}

@inproceedings{cya-ccs13,
	Author = {J.~Geddes and M.~Schuchard and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Cover Your ACKs: Pitfalls of Covert Channel Censorship Circumvention}},
	Year = {2013}}

@inproceedings{andana,
	Author = {DiBenedetto, S. and Gasti, P. and Tsudik, G. and Uzun, E.},
	Booktitle = {{NDSS}},
	Title = {{ANDaNA: Anonymous Named Data Networking Application}},
	Year = {2012}}

@inproceedings{darkly,
	Author = {Jana, S. and Narayanan, A. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{A Scanner Darkly: Protecting User Privacy From Perceptual Applications}},
	Year = {2013}}

@inproceedings{NS08,
	Author = {A.~Narayanan and V.~Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {Robust de-anonymization of large sparse datasets},
	Year = {2008}}

@inproceedings{NS09,
	Author = {A.~Narayanan and V.~Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {De-anonymizing social networks},
	Year = {2009}}

@inproceedings{memento,
	Author = {Jana, S. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{Memento: Learning secrets from process footprints}},
	Year = {2012}}

@misc{plugtor,
	Howpublished = {\url{https://www.torproject.org/docs/pluggable-transports.html.en}},
	Key = {PluggableTransports},
	Publisher = {The Tor Project},
	Title = {{Tor: Pluggable transports}}}

@misc{psiphon,
	Author = {J.~Jia and P.~Smith},
	Howpublished = {\url{http://www.cdf.toronto.edu/~csc494h/reports/2004-fall/psiphon_ae.html}},
	Title = {{Psiphon: Analysis and Estimation}},
	Year = 2004}

@misc{china-github,
	Howpublished = {\url{http://mobile.informationweek.com/80269/show/72e30386728f45f56b343ddfd0fdb119/}},
	Key = {github},
	Title = {{China's GitHub Censorship Dilemma}}}

@inproceedings{txbox,
	Author = {Jana, S. and Porter, D. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{TxBox: Building Secure, Efficient Sandboxes with System Transactions}},
	Year = {2011}}

@inproceedings{airavat,
	Author = {I. Roy and S. Setty and A. Kilzer and V. Shmatikov and E. Witchel},
	Booktitle = {NSDI},
	Title = {{Airavat: Security and Privacy for MapReduce}},
	Year = {2010}}

@inproceedings{osdi12,
	Author = {A. Dunn and M. Lee and S. Jana and S. Kim and M. Silberstein and Y. Xu and V. Shmatikov and E. Witchel},
	Booktitle = {OSDI},
	Title = {{Eternal Sunshine of the Spotless Machine: Protecting Privacy with Ephemeral Channels}},
	Year = {2012}}

@inproceedings{ymal,
	Author = {J. Calandrino and A. Kilzer and A. Narayanan and E. Felten and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{``You Might Also Like:'' Privacy Risks of Collaborative Filtering}},
	Year = {2011}}

@inproceedings{srivastava11,
	Author = {V. Srivastava and M. Bond and K. McKinley and V. Shmatikov},
	Booktitle = {PLDI},
	Title = {{A Security Policy Oracle: Detecting Security Holes Using Multiple API Implementations}},
	Year = {2011}}

@inproceedings{chen-oakland10,
	Author = {Chen, S. and Wang, R. and Wang, X. and Zhang, K.},
	Booktitle = {IEEE S\&P},
	Title = {{Side-Channel Leaks in Web Applications: A Reality Today, a Challenge Tomorrow}},
	Year = {2010}}

@book{kerck,
	Author = {Kerckhoffs, A.},
	Publisher = {University Microfilms},
	Title = {{La cryptographie militaire}},
	Year = {1978}}

@inproceedings{foci11,
	Author = {J. Karlin and D. Ellard and A.~Jackson and C.~ Jones and G. Lauer and D. Mankins and W.~T.~Strayer},
	Booktitle = {FOCI},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = 2011}

@inproceedings{sun02,
	Author = {Sun, Q. and Simon, D.~R. and Wang, Y. and Russell, W. and Padmanabhan, V. and Qiu, L.},
	Booktitle = {IEEE S\&P},
	Title = {{Statistical Identification of Encrypted Web Browsing Traffic}},
	Year = {2002}}

@inproceedings{danezis,
	Author = {Murdoch, S.~J. and Danezis, G.},
	Booktitle = {IEEE S\&P},
	Title = {{Low-Cost Traffic Analysis of Tor}},
	Year = {2005}}

@inproceedings{pakicensorship,
	Author = {Z.~Nabi},
	Booktitle = {FOCI},
	Title = {The Anatomy of {Web} Censorship in {Pakistan}},
	Year = {2013}}

@inproceedings{irancensorship,
	Author = {S.~Aryan and H.~Aryan and A.~Halderman},
	Booktitle = {FOCI},
	Title = {Internet Censorship in {Iran}: {A} First Look},
	Year = {2013}}

@inproceedings{ford10efficient,
	Author = {Amittai Aviram and Shu-Chun Weng and Sen Hu and Bryan Ford},
	Booktitle = {\bibconf[9th]{OSDI}{USENIX Symposium on Operating Systems Design and Implementation}},
	Location = {Vancouver, BC, Canada},
	Month = oct,
	Title = {Efficient System-Enforced Deterministic Parallelism},
	Year = 2010}

@inproceedings{ford10determinating,
	Author = {Amittai Aviram and Sen Hu and Bryan Ford and Ramakrishna Gummadi},
	Booktitle = {\bibconf{CCSW}{ACM Cloud Computing Security Workshop}},
	Location = {Chicago, IL},
	Month = oct,
	Title = {Determinating Timing Channels in Compute Clouds},
	Year = 2010}

@inproceedings{ford12plugging,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Plugging Side-Channel Leaks with Timing Information Flow Control},
	Year = 2012}

@inproceedings{ford12icebergs,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Icebergs in the Clouds: the {\em Other} Risks of Cloud Computing},
	Year = 2012}

@misc{mullenize,
	Author = {Washington Post},
	Howpublished = {\url{http://apps.washingtonpost.com/g/page/world/gchq-report-on-mullenize-program-to-stain-anonymous-electronic-traffic/502/}},
	Month = {oct},
	Title = {{GCHQ} report on {`MULLENIZE'} program to `stain' anonymous electronic traffic},
	Year = {2013}}

@inproceedings{shue13street,
	Author = {Craig A. Shue and Nathanael Paul and Curtis R. Taylor},
	Booktitle = {\bibbrev[7th]{WOOT}{USENIX Workshop on Offensive Technologies}},
	Month = aug,
	Title = {From an {IP} Address to a Street Address: Using Wireless Signals to Locate a Target},
	Year = 2013}

@inproceedings{knockel11three,
	Author = {Jeffrey Knockel and Jedidiah R. Crandall and Jared Saia},
	Booktitle = {\bibbrev{FOCI}{USENIX Workshop on Free and Open Communications on the Internet}},
	Location = {San Francisco, CA},
	Month = aug,
	Year = 2011}

@misc{rfc4960,
	Author = {R. {Stewart, ed.}},
	Month = sep,
	Note = {RFC 4960},
	Title = {Stream Control Transmission Protocol},
	Year = 2007}

@inproceedings{ford07structured,
	Author = {Bryan Ford},
	Booktitle = {\bibbrev{SIGCOMM}{ACM SIGCOMM}},
	Location = {Kyoto, Japan},
	Month = aug,
	Title = {Structured Streams: a New Transport Abstraction},
	Year = {2007}}

@misc{spdy,
	Author = {Google, Inc.},
	Note = {\url{http://www.chromium.org/spdy/spdy-whitepaper}},
	Title = {{SPDY}: An Experimental Protocol For a Faster {Web}}}

@misc{quic,
	Author = {Jim Roskind},
	Month = jun,
	Note = {\url{http://blog.chromium.org/2013/06/experimenting-with-quic.html}},
	Title = {Experimenting with {QUIC}},
	Year = 2013}

@misc{podjarny12not,
	Author = {G.~Podjarny},
	Month = jun,
	Note = {\url{http://www.guypo.com/technical/not-as-spdy-as-you-thought/}},
	Title = {{Not as SPDY as You Thought}},
	Year = 2012}

@inproceedings{cor,
	Author = {Jones, N.~A. and Arye, M. and Cesareo, J. and Freedman, M.~J.},
	Booktitle = {FOCI},
	Title = {{Hiding Amongst the Clouds: A Proposal for Cloud-based Onion Routing}},
	Year = {2011}}

@misc{torcloud,
	Howpublished = {\url{https://cloud.torproject.org/}},
	Key = {tor cloud},
	Title = {{The Tor Cloud Project}}}

@inproceedings{scramblesuit,
	Author = {Philipp Winter and Tobias Pulls and Juergen Fuss},
	Booktitle = {WPES},
	Title = {{ScrambleSuit: A Polymorphic Network Protocol to Circumvent Censorship}},
	Year = 2013}

@article{savage2000practical,
	Author = {Savage, S. and Wetherall, D. and Karlin, A. and Anderson, T.},
	Journal = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Pages = {295--306},
	Publisher = {ACM},
	Title = {Practical network support for IP traceback},
	Volume = {30},
	Year = {2000}}

@inproceedings{ooni,
	Author = {Filast, A. and Appelbaum, J.},
	Booktitle = {{FOCI}},
	Title = {{OONI : Open Observatory of Network Interference}},
	Year = {2012}}

@misc{caida-rank,
	Howpublished = {\url{http://as-rank.caida.org/}},
	Key = {caida rank},
	Title = {{AS Rank: AS Ranking}}}

@inproceedings{usersrouted-ccs13,
	Author = {A.~Johnson and C.~Wacek and R.~Jansen and M.~Sherr and P.~Syverson},
	Booktitle = {CCS},
	Title = {{Users Get Routed: Traffic Correlation on Tor by Realistic Adversaries}},
	Year = {2013}}

@inproceedings{edman2009awareness,
	Author = {Edman, M. and Syverson, P.},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2009}}

@inproceedings{DecoyCosts,
	Author = {A.~Houmansadr and E.~L.~Wong and V.~Shmatikov},
	Booktitle = {NDSS},
	Title = {{No Direction Home: The True Cost of Routing Around Decoys}},
	Year = {2014}}

@article{cordon,
	Author = {Elahi, T. and Goldberg, I.},
	Journal = {University of Waterloo CACR},
	Title = {{CORDON--A Taxonomy of Internet Censorship Resistance Strategies}},
	Volume = {33},
	Year = {2012}}

@inproceedings{privex,
	Author = {T.~Elahi and G.~Danezis and I.~Goldberg	},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2014}}

@inproceedings{changeGuards,
	Author = {T.~Elahi and K.~Bauer and M.~AlSabah and R.~Dingledine and I.~Goldberg},
	Booktitle = {{WPES}},
	Title = {{ Changing of the Guards: Framework for Understanding and Improving Entry Guard Selection in Tor}},
	Year = {2012}}

@article{RAINBOW:Journal,
	Author = {A.~Houmansadr and N.~Kiyavash and N.~Borisov},
	Journal = {IEEE/ACM Transactions on Networking},
	Title = {{Non-Blind Watermarking of Network Flows}},
	Year = 2014}

@inproceedings{info-tod,
	Author = {A.~Houmansadr and S.~Gorantla and T.~Coleman and N.~Kiyavash and and N.~Borisov},
	Booktitle = {{CCS (poster session)}},
	Title = {{On the Channel Capacity of Network Flow Watermarking}},
	Year = {2009}}

@inproceedings{johnson2014game,
	Author = {Johnson, B. and Laszka, A. and Grossklags, J. and Vasek, M. and Moore, T.},
	Booktitle = {Workshop on Bitcoin Research},
	Title = {{Game-theoretic Analysis of DDoS Attacks Against Bitcoin Mining Pools}},
	Year = {2014}}

@incollection{laszka2013mitigation,
	Author = {Laszka, A. and Johnson, B. and Grossklags, J.},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {175--191},
	Publisher = {Springer},
	Title = {{Mitigation of Targeted and Non-targeted Covert Attacks as a Timing Game}},
	Year = {2013}}

@inproceedings{schottle2013game,
	Author = {Schottle, P. and Laszka, A. and Johnson, B. and Grossklags, J. and Bohme, R.},
	Booktitle = {EUSIPCO},
	Title = {{A Game-theoretic Analysis of Content-adaptive Steganography with Independent Embedding}},
	Year = {2013}}

@inproceedings{CloudTransport,
	Author = {C.~Brubaker and A.~Houmansadr and V.~Shmatikov},
	Booktitle = {PETS},
	Title = {{CloudTransport: Using Cloud Storage for Censorship-Resistant Networking}},
	Year = {2014}}

@inproceedings{sweet,
	Author = {W.~Zhou and A.~Houmansadr and M.~Caesar and N.~Borisov},
	Booktitle = {HotPETs},
	Title = {{SWEET: Serving the Web by Exploiting Email Tunnels}},
	Year = {2013}}

@inproceedings{ahsan2002practical,
	Author = {Ahsan, K. and Kundur, D.},
	Booktitle = {Workshop on Multimedia Security},
	Title = {{Practical data hiding in TCP/IP}},
	Year = {2002}}

@incollection{danezis2011covert,
	Author = {Danezis, G.},
	Booktitle = {Security Protocols XVI},
	Pages = {198--214},
	Publisher = {Springer},
	Title = {{Covert Communications Despite Traffic Data Retention}},
	Year = {2011}}

@inproceedings{liu2009hide,
	Author = {Liu, Y. and Ghosal, D. and Armknecht, F. and Sadeghi, A.-R. and Schulz, S. and Katzenbeisser, S.},
	Booktitle = {ESORICS},
	Title = {{Hide and Seek in Time---Robust Covert Timing Channels}},
	Year = {2009}}

@misc{image-watermark-fing,
	Author = {Jonathan Bailey},
	Howpublished = {\url{https://www.plagiarismtoday.com/2009/12/02/image-detection-watermarking-vs-fingerprinting/}},
	Title = {{Image Detection: Watermarking vs. Fingerprinting}},
	Year = {2009}}

@inproceedings{Servetto98,
	Author = {S. D. Servetto and C. I. Podilchuk and K. Ramchandran},
	Booktitle = {Int. Conf. Image Processing},
	Title = {Capacity issues in digital image watermarking},
	Year = {1998}}

@inproceedings{Chen01,
	Author = {B. Chen and G.W.Wornell},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1423--1443},
	Title = {Quantization index modulation: A class of provably good methods for digital watermarking and information embedding},
	Year = {2001}}

@inproceedings{Karakos00,
	Author = {D. Karakos and A. Papamarcou},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {47},
	Title = {Relationship between quantization and distribution rates of digitally watermarked data},
	Year = {2000}}

@inproceedings{Sullivan98,
	Author = {J. A. OSullivan and P. Moulin and J. M. Ettinger},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {297},
	Title = {Information theoretic analysis of steganography},
	Year = {1998}}

@inproceedings{Merhav00,
	Author = {N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {420--430},
	Title = {On random coding error exponents of watermarking systems},
	Year = {2000}}

@inproceedings{Somekh01,
	Author = {A. Somekh-Baruch and N. Merhav},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {7},
	Title = {On the error exponent and capacity games of private watermarking systems},
	Year = {2001}}

@inproceedings{Steinberg01,
	Author = {Y. Steinberg and N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1410--1422},
	Title = {Identification in the presence of side information with application to watermarking},
	Year = {2001}}

@article{Moulin03,
	Author = {P. Moulin and J.A. O'Sullivan},
	Journal = {IEEE Trans. Info. Theory},
	Number = {3},
	Title = {Information-theoretic analysis of information hiding},
	Volume = 49,
	Year = 2003}

@article{Gelfand80,
	Author = {S.I.~Gelfand and M.S.~Pinsker},
	Journal = {Problems of Control and Information Theory},
	Number = {1},
	Pages = {19-31},
	Title = {{Coding for channel with random parameters}},
	Url = {citeseer.ist.psu.edu/anantharam96bits.html},
	Volume = {9},
	Year = {1980},
	Bdsk-Url-1 = {citeseer.ist.psu.edu/anantharam96bits.html}}

@book{Wolfowitz78,
	Author = {J. Wolfowitz},
	Edition = {3rd},
	Location = {New York},
	Publisher = {Springer-Verlag},
	Title = {Coding Theorems of Information Theory},
	Year = 1978}

@article{caire99,
	Author = {G. Caire and S. Shamai},
	Journal = {IEEE Transactions on Information Theory},
	Number = {6},
	Pages = {2007--2019},
	Title = {On the Capacity of Some Channels with Channel State Information},
	Volume = {45},
	Year = {1999}}

@inproceedings{wright2007language,
	Author = {Wright, Charles V and Ballard, Lucas and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {USENIX Security},
	Title = {{Language identification of encrypted VoIP traffic: Alejandra y Roberto or Alice and Bob?}},
	Year = {2007}}

@inproceedings{backes2010speaker,
	Author = {Backes, Michael and Doychev, Goran and D{\"u}rmuth, Markus and K{\"o}pf, Boris},
	Booktitle = {{European Symposium on Research in Computer Security (ESORICS)}},
	Pages = {508--523},
	Publisher = {Springer},
	Title = {{Speaker Recognition in Encrypted Voice Streams}},
	Year = {2010}}

@phdthesis{lu2009traffic,
	Author = {Lu, Yuanchao},
	School = {Cleveland State University},
	Title = {{On Traffic Analysis Attacks to Encrypted VoIP Calls}},
	Year = {2009}}

@inproceedings{wright2008spot,
	Author = {Wright, Charles V and Ballard, Lucas and Coull, Scott E and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {35--49},
	Title = {Spot me if you can: Uncovering spoken phrases in encrypted VoIP conversations},
	Year = {2008}}

@inproceedings{white2011phonotactic,
	Author = {White, Andrew M and Matthews, Austin R and Snow, Kevin Z and Monrose, Fabian},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {3--18},
	Title = {Phonotactic reconstruction of encrypted VoIP conversations: Hookt on fon-iks},
	Year = {2011}}

@inproceedings{fancy,
	Author = {Houmansadr, Amir and Borisov, Nikita},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {205--224},
	Title = {The Need for Flow Fingerprints to Link Correlated Network Flows},
	Year = {2013}}

@article{botmosaic,
	Author = {Amir Houmansadr and Nikita Borisov},
	Doi = {10.1016/j.jss.2012.11.005},
	Issn = {0164-1212},
	Journal = {Journal of Systems and Software},
	Keywords = {Network security},
	Number = {3},
	Pages = {707 - 715},
	Title = {BotMosaic: Collaborative network watermark for the detection of IRC-based botnets},
	Url = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Volume = {86},
	Year = {2013},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.jss.2012.11.005}}

@inproceedings{ramsbrock2008first,
	Author = {Ramsbrock, Daniel and Wang, Xinyuan and Jiang, Xuxian},
	Booktitle = {Recent Advances in Intrusion Detection},
	Organization = {Springer},
	Pages = {59--77},
	Title = {A first step towards live botmaster traceback},
	Year = {2008}}

@inproceedings{potdar2005survey,
	Author = {Potdar, Vidyasagar M and Han, Song and Chang, Elizabeth},
	Booktitle = {Industrial Informatics, 2005. INDIN'05. 2005 3rd IEEE International Conference on},
	Organization = {IEEE},
	Pages = {709--716},
	Title = {A survey of digital image watermarking techniques},
	Year = {2005}}

@book{cole2003hiding,
	Author = {Cole, Eric and Krutz, Ronald D},
	Publisher = {John Wiley \& Sons, Inc.},
	Title = {Hiding in plain sight: Steganography and the art of covert communication},
	Year = {2003}}

@incollection{akaike1998information,
	Author = {Akaike, Hirotogu},
	Booktitle = {Selected Papers of Hirotugu Akaike},
	Pages = {199--213},
	Publisher = {Springer},
	Title = {Information theory and an extension of the maximum likelihood principle},
	Year = {1998}}

@misc{central-command-hack,
	Author = {Everett Rosenfeld},
	Howpublished = {\url{http://www.cnbc.com/id/102330338}},
	Title = {{FBI investigating Central Command Twitter hack}},
	Year = {2015}}

@misc{sony-psp-ddos,
	Howpublished = {\url{http://n4g.com/news/1644853/sony-and-microsoft-cant-do-much-ddos-attacks-explained}},
	Key = {sony},
	Month = {December},
	Title = {{Sony and Microsoft cant do much -- DDoS attacks explained}},
	Year = {2014}}

@misc{sony-hack,
	Author = {David Bloom},
	Howpublished = {\url{http://goo.gl/MwR4A7}},
	Title = {{Online Game Networks Hacked, Sony Unit President Threatened}},
	Year = {2014}}

@misc{home-depot,
	Author = {Dune Lawrence},
	Howpublished = {\url{http://www.businessweek.com/articles/2014-09-02/home-depots-credit-card-breach-looks-just-like-the-target-hack}},
	Title = {{Home Depot's Suspected Breach Looks Just Like the Target Hack}},
	Year = {2014}}

@misc{target,
	Author = {Julio Ojeda-Zapata},
	Howpublished = {\url{http://www.mercurynews.com/business/ci_24765398/how-did-hackers-pull-off-target-data-heist}},
	Title = {{Target hack: How did they do it?}},
	Year = {2014}}


@article{probabilitycourse,
	Author = {H. Pishro-Nik},
	note = {\url{http://www.probabilitycourse.com}},
	Title = {Introduction to probability, statistics, and random processes},
    Year = {2014}}



@inproceedings{shokri2011quantifying,
	Author = {Shokri, Reza and Theodorakopoulos, George and Le Boudec, Jean-Yves and Hubaux, Jean-Pierre},
	Booktitle = {Security and Privacy (SP), 2011 IEEE Symposium on},
	Organization = {IEEE},
	Pages = {247--262},
	Title = {Quantifying location privacy},
	Year = {2011}}

@inproceedings{hoh2007preserving,
	Author = {Hoh, Baik and Gruteser, Marco and Xiong, Hui and Alrabady, Ansaf},
	Booktitle = {Proceedings of the 14th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {161--171},
	Title = {Preserving privacy in gps traces via uncertainty-aware path cloaking},
	Year = {2007}}



@article{kafsi2013entropy,
	Author = {Kafsi, Mohamed and Grossglauser, Matthias and Thiran, Patrick},
	Journal = {Information Theory, IEEE Transactions on},
	Number = {9},
	Pages = {5577--5583},
	Publisher = {IEEE},
	Title = {The entropy of conditional Markov trajectories},
	Volume = {59},
	Year = {2013}}

@inproceedings{gruteser2003anonymous,
	Author = {Gruteser, Marco and Grunwald, Dirk},
	Booktitle = {Proceedings of the 1st international conference on Mobile systems, applications and services},
	Organization = {ACM},
	Pages = {31--42},
	Title = {Anonymous usage of location-based services through spatial and temporal cloaking},
	Year = {2003}}

@inproceedings{husted2010mobile,
	Author = {Husted, Nathaniel and Myers, Steven},
	Booktitle = {Proceedings of the 17th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {85--96},
	Title = {Mobile location tracking in metro areas: malnets and others},
	Year = {2010}}

@inproceedings{li2009tradeoff,
	Author = {Li, Tiancheng and Li, Ninghui},
	Booktitle = {Proceedings of the 15th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {517--526},
	Title = {On the tradeoff between privacy and utility in data publishing},
	Year = {2009}}

@inproceedings{ma2009location,
	Author = {Ma, Zhendong and Kargl, Frank and Weber, Michael},
	Booktitle = {Sarnoff Symposium, 2009. SARNOFF'09. IEEE},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {A location privacy metric for v2x communication systems},
	Year = {2009}}

@inproceedings{shokri2012protecting,
	Author = {Shokri, Reza and Theodorakopoulos, George and Troncoso, Carmela and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
	Booktitle = {Proceedings of the 2012 ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {617--627},
	Title = {Protecting location privacy: optimal strategy against localization attacks},
	Year = {2012}}

@inproceedings{freudiger2009non,
	Author = {Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
	Booktitle = {Proceedings of the 16th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {324--337},
	Title = {On non-cooperative location privacy: a game-theoretic analysis},
	Year = {2009}}

@incollection{humbert2010tracking,
	Author = {Humbert, Mathias and Manshaei, Mohammad Hossein and Freudiger, Julien and Hubaux, Jean-Pierre},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {38--57},
	Publisher = {Springer},
	Title = {Tracking games in mobile networks},
	Year = {2010}}

@article{manshaei2013game,
	Author = {Manshaei, Mohammad Hossein and Zhu, Quanyan and Alpcan, Tansu and Bac{\c{s}}ar, Tamer and Hubaux, Jean-Pierre},
	Journal = {ACM Computing Surveys (CSUR)},
	Number = {3},
	Pages = {25},
	Publisher = {ACM},
	Title = {Game theory meets network security and privacy},
	Volume = {45},
	Year = {2013}}

@article{palamidessi2006probabilistic,
	Author = {Palamidessi, Catuscia},
	Journal = {Electronic Notes in Theoretical Computer Science},
	Pages = {33--42},
	Publisher = {Elsevier},
	Title = {Probabilistic and nondeterministic aspects of anonymity},
	Volume = {155},
	Year = {2006}}

@inproceedings{mokbel2006new,
	Author = {Mokbel, Mohamed F and Chow, Chi-Yin and Aref, Walid G},
	Booktitle = {Proceedings of the 32nd international conference on Very large data bases},
	Organization = {VLDB Endowment},
	Pages = {763--774},
	Title = {The new Casper: query processing for location services without compromising privacy},
	Year = {2006}}

@article{kalnis2007preventing,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {12},
	Pages = {1719--1733},
	Publisher = {IEEE},
	Title = {Preventing location-based identity inference in anonymous spatial queries},
	Volume = {19},
	Year = {2007}}
	
@article{freudiger2007mix,
  title={Mix-zones for location privacy in vehicular networks},
  author={Freudiger, Julien and Raya, Maxim and F{\'e}legyh{\'a}zi, M{\'a}rk and Papadimitratos, Panos and Hubaux, Jean-Pierre},
  year={2007}
}
@article{sweeney2002k,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {557--570},
	Publisher = {World Scientific},
	Title = {k-anonymity: A model for protecting privacy},
	Volume = {10},
	Year = {2002}}

@article{sweeney2002achieving,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {571--588},
	Publisher = {World Scientific},
	Title = {Achieving k-anonymity privacy protection using generalization and suppression},
	Volume = {10},
	Year = {2002}}

@inproceedings{niu2014achieving,
	Author = {Niu, Ben and Li, Qinghua and Zhu, Xiaoyan and Cao, Guohong and Li, Hui},
	Booktitle = {INFOCOM, 2014 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {754--762},
	Title = {Achieving k-anonymity in privacy-aware location-based services},
	Year = {2014}}

@inproceedings{liu2013game,
	Author = {Liu, Xinxin and Liu, Kaikai and Guo, Linke and Li, Xiaolin and Fang, Yuguang},
	Booktitle = {INFOCOM, 2013 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {2985--2993},
	Title = {A game-theoretic approach for achieving k-anonymity in location based services},
	Year = {2013}}

@inproceedings{kido2005protection,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Data Engineering Workshops, 2005. 21st International Conference on},
	Organization = {IEEE},
	Pages = {1248--1248},
	Title = {Protection of location privacy using dummies for location-based services},
	Year = {2005}}

@inproceedings{gedik2005location,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Booktitle = {Distributed Computing Systems, 2005. ICDCS 2005. Proceedings. 25th IEEE International Conference on},
	Organization = {IEEE},
	Pages = {620--629},
	Title = {Location privacy in mobile systems: A personalized anonymization model},
	Year = {2005}}

@inproceedings{bordenabe2014optimal,
	Author = {Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2014 ACM SIGSAC Conference on Computer and Communications Security},
	Organization = {ACM},
	Pages = {251--262},
	Title = {Optimal geo-indistinguishable mechanisms for location privacy},
	Year = {2014}}

@incollection{duckham2005formal,
	Author = {Duckham, Matt and Kulik, Lars},
	Booktitle = {Pervasive computing},
	Pages = {152--170},
	Publisher = {Springer},
	Title = {A formal model of obfuscation and negotiation for location privacy},
	Year = {2005}}

@inproceedings{kido2005anonymous,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Pervasive Services, 2005. ICPS'05. Proceedings. International Conference on},
	Organization = {IEEE},
	Pages = {88--97},
	Title = {An anonymous communication technique using dummies for location-based services},
	Year = {2005}}

@incollection{duckham2006spatiotemporal,
	Author = {Duckham, Matt and Kulik, Lars and Birtley, Athol},
	Booktitle = {Geographic Information Science},
	Pages = {47--64},
	Publisher = {Springer},
	Title = {A spatiotemporal model of strategies and counter strategies for location privacy protection},
	Year = {2006}}

@inproceedings{shankar2009privately,
	Author = {Shankar, Pravin and Ganapathy, Vinod and Iftode, Liviu},
	Booktitle = {Proceedings of the 11th international conference on Ubiquitous computing},
	Organization = {ACM},
	Pages = {31--40},
	Title = {Privately querying location-based services with SybilQuery},
	Year = {2009}}

@inproceedings{chow2009faking,
	Author = {Chow, Richard and Golle, Philippe},
	Booktitle = {Proceedings of the 8th ACM workshop on Privacy in the electronic society},
	Organization = {ACM},
	Pages = {105--108},
	Title = {Faking contextual data for fun, profit, and privacy},
	Year = {2009}}

@incollection{xue2009location,
	Author = {Xue, Mingqiang and Kalnis, Panos and Pung, Hung Keng},
	Booktitle = {Location and Context Awareness},
	Pages = {70--87},
	Publisher = {Springer},
	Title = {Location diversity: Enhanced privacy protection in location based services},
	Year = {2009}}

@article{wernke2014classification,
	Author = {Wernke, Marius and Skvortsov, Pavel and D{\"u}rr, Frank and Rothermel, Kurt},
	Journal = {Personal and Ubiquitous Computing},
	Number = {1},
	Pages = {163--175},
	Publisher = {Springer-Verlag},
	Title = {A classification of location privacy attacks and approaches},
	Volume = {18},
	Year = {2014}}

@misc{cai2015cloaking,
	Author = {Cai, Y. and Xu, G.},
	Month = jan # {~1},
	Note = {US Patent App. 14/472,462},
	Publisher = {Google Patents},
	Title = {Cloaking with footprints to provide location privacy protection in location-based services},
	Url = {https://www.google.com/patents/US20150007341},
	Year = {2015},
	Bdsk-Url-1 = {https://www.google.com/patents/US20150007341}}

@article{gedik2008protecting,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {1},
	Pages = {1--18},
	Publisher = {IEEE},
	Title = {Protecting location privacy with personalized k-anonymity: Architecture and algorithms},
	Volume = {7},
	Year = {2008}}

@article{kalnis2006preserving,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Publisher = {TRB6/06},
	Title = {Preserving anonymity in location based services},
	Year = {2006}}

@inproceedings{hoh2005protecting,
	Author = {Hoh, Baik and Gruteser, Marco},
	Booktitle = {Security and Privacy for Emerging Areas in Communications Networks, 2005. SecureComm 2005. First International Conference on},
	Organization = {IEEE},
	Pages = {194--205},
	Title = {Protecting location privacy through path confusion},
	Year = {2005}}

@article{terrovitis2011privacy,
	Author = {Terrovitis, Manolis},
	Journal = {ACM SIGKDD Explorations Newsletter},
	Number = {1},
	Pages = {6--18},
	Publisher = {ACM},
	Title = {Privacy preservation in the dissemination of location data},
	Volume = {13},
	Year = {2011}}

@article{shin2012privacy,
	Author = {Shin, Kang G and Ju, Xiaoen and Chen, Zhigang and Hu, Xin},
	Journal = {Wireless Communications, IEEE},
	Number = {1},
	Pages = {30--39},
	Publisher = {IEEE},
	Title = {Privacy protection for users of location-based services},
	Volume = {19},
	Year = {2012}}

@article{khoshgozaran2011location,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus and Shirani-Mehr, Houtan},
	Journal = {Knowledge and Information Systems},
	Number = {3},
	Pages = {435--465},
	Publisher = {Springer},
	Title = {Location privacy: going beyond K-anonymity, cloaking and anonymizers},
	Volume = {26},
	Year = {2011}}

@incollection{chatzikokolakis2015geo,
	Author = {Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
	Booktitle = {Distributed Computing and Internet Technology},
	Pages = {49--72},
	Publisher = {Springer},
	Title = {Geo-indistinguishability: A Principled Approach to Location Privacy},
	Year = {2015}}

@inproceedings{ngo2015location,
	Author = {Ngo, Hoa and Kim, Jong},
	Booktitle = {Computer Security Foundations Symposium (CSF), 2015 IEEE 28th},
	Organization = {IEEE},
	Pages = {63--74},
	Title = {Location Privacy via Differential Private Perturbation of Cloaking Area},
	Year = {2015}}

@inproceedings{palanisamy2011mobimix,
	Author = {Palanisamy, Balaji and Liu, Ling},
	Booktitle = {Data Engineering (ICDE), 2011 IEEE 27th International Conference on},
	Organization = {IEEE},
	Pages = {494--505},
	Title = {Mobimix: Protecting location privacy with mix-zones over road networks},
	Year = {2011}}

@inproceedings{um2010advanced,
	Author = {Um, Jung-Ho and Kim, Hee-Dae and Chang, Jae-Woo},
	Booktitle = {Social Computing (SocialCom), 2010 IEEE Second International Conference on},
	Organization = {IEEE},
	Pages = {1093--1098},
	Title = {An advanced cloaking algorithm using Hilbert curves for anonymous location based service},
	Year = {2010}}

@inproceedings{bamba2008supporting,
	Author = {Bamba, Bhuvan and Liu, Ling and Pesti, Peter and Wang, Ting},
	Booktitle = {Proceedings of the 17th international conference on World Wide Web},
	Organization = {ACM},
	Pages = {237--246},
	Title = {Supporting anonymous location queries in mobile environments with privacygrid},
	Year = {2008}}

@inproceedings{zhangwei2010distributed,
	Author = {Zhangwei, Huang and Mingjun, Xin},
	Booktitle = {Networks Security Wireless Communications and Trusted Computing (NSWCTC), 2010 Second International Conference on},
	Organization = {IEEE},
	Pages = {468--471},
	Title = {A distributed spatial cloaking protocol for location privacy},
	Volume = {2},
	Year = {2010}}

@article{chow2011spatial,
	Author = {Chow, Chi-Yin and Mokbel, Mohamed F and Liu, Xuan},
	Journal = {GeoInformatica},
	Number = {2},
	Pages = {351--380},
	Publisher = {Springer},
	Title = {Spatial cloaking for anonymous location-based services in mobile peer-to-peer environments},
	Volume = {15},
	Year = {2011}}

@inproceedings{lu2008pad,
	Author = {Lu, Hua and Jensen, Christian S and Yiu, Man Lung},
	Booktitle = {Proceedings of the Seventh ACM International Workshop on Data Engineering for Wireless and Mobile Access},
	Organization = {ACM},
	Pages = {16--23},
	Title = {Pad: privacy-area aware, dummy-based location privacy in mobile services},
	Year = {2008}}

@incollection{khoshgozaran2007blind,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus},
	Booktitle = {Advances in Spatial and Temporal Databases},
	Pages = {239--257},
	Publisher = {Springer},
	Title = {Blind evaluation of nearest neighbor queries using space transformation to preserve location privacy},
	Year = {2007}}

@inproceedings{ghinita2008private,
	Author = {Ghinita, Gabriel and Kalnis, Panos and Khoshgozaran, Ali and Shahabi, Cyrus and Tan, Kian-Lee},
	Booktitle = {Proceedings of the 2008 ACM SIGMOD international conference on Management of data},
	Organization = {ACM},
	Pages = {121--132},
	Title = {Private queries in location based services: anonymizers are not necessary},
	Year = {2008}}

@article{paulet2014privacy,
	Author = {Paulet, Russell and Kaosar, Md Golam and Yi, Xun and Bertino, Elisa},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {5},
	Pages = {1200--1210},
	Publisher = {IEEE},
	Title = {Privacy-preserving and content-protecting location based queries},
	Volume = {26},
	Year = {2014}}

@article{nguyen2013differential,
	Author = {Nguyen, Hiep H and Kim, Jong and Kim, Yoonho},
	Journal = {Journal of Computing Science and Engineering},
	Number = {3},
	Pages = {177--186},
	Title = {Differential privacy in practice},
	Volume = {7},
	Year = {2013}}

@inproceedings{lee2012differential,
	Author = {Lee, Jaewoo and Clifton, Chris},
	Booktitle = {Proceedings of the 18th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {1041--1049},
	Title = {Differential identifiability},
	Year = {2012}}

@inproceedings{andres2013geo,
	Author = {Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2013 ACM SIGSAC conference on Computer \& communications security},
	Organization = {ACM},
	Pages = {901--914},
	Title = {Geo-indistinguishability: Differential privacy for location-based systems},
	Year = {2013}}

@inproceedings{machanavajjhala2008privacy,
	Author = {Machanavajjhala, Ashwin and Kifer, Daniel and Abowd, John and Gehrke, Johannes and Vilhuber, Lars},
	Booktitle = {Data Engineering, 2008. ICDE 2008. IEEE 24th International Conference on},
	Organization = {IEEE},
	Pages = {277--286},
	Title = {Privacy: Theory meets practice on the map},
	Year = {2008}}

@article{dewri2013local,
	Author = {Dewri, Rinku},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {12},
	Pages = {2360--2372},
	Publisher = {IEEE},
	Title = {Local differential perturbations: Location privacy under approximate knowledge attackers},
	Volume = {12},
	Year = {2013}}

@inproceedings{chatzikokolakis2013broadening,
	Author = {Chatzikokolakis, Konstantinos and Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s Emilio and Palamidessi, Catuscia},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {82--102},
	Title = {Broadening the Scope of Differential Privacy Using Metrics.},
	Year = {2013}}

@inproceedings{zhong2009distributed,
	Author = {Zhong, Ge and Hengartner, Urs},
	Booktitle = {Pervasive Computing and Communications, 2009. PerCom 2009. IEEE International Conference on},
	Organization = {IEEE},
	Pages = {1--10},
	Title = {A distributed k-anonymity protocol for location privacy},
	Year = {2009}}

@inproceedings{ho2011differential,
	Author = {Ho, Shen-Shyang and Ruan, Shuhua},
	Booktitle = {Proceedings of the 4th ACM SIGSPATIAL International Workshop on Security and Privacy in GIS and LBS},
	Organization = {ACM},
	Pages = {17--24},
	Title = {Differential privacy for location pattern mining},
	Year = {2011}}

@inproceedings{cheng2006preserving,
	Author = {Cheng, Reynold and Zhang, Yu and Bertino, Elisa and Prabhakar, Sunil},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {393--412},
	Title = {Preserving user location privacy in mobile data management infrastructures},
	Year = {2006}}

@article{beresford2003location,
	Author = {Beresford, Alastair R and Stajano, Frank},
	Journal = {IEEE Pervasive computing},
	Number = {1},
	Pages = {46--55},
	Publisher = {IEEE},
	Title = {Location privacy in pervasive computing},
	Year = {2003}}

@inproceedings{freudiger2009optimal,
	Author = {Freudiger, Julien and Shokri, Reza and Hubaux, Jean-Pierre},
	Booktitle = {Privacy enhancing technologies},
	Organization = {Springer},
	Pages = {216--234},
	Title = {On the optimal placement of mix zones},
	Year = {2009}}

@article{krumm2009survey,
	Author = {Krumm, John},
	Journal = {Personal and Ubiquitous Computing},
	Number = {6},
	Pages = {391--399},
	Publisher = {Springer},
	Title = {A survey of computational location privacy},
	Volume = {13},
	Year = {2009}}

@article{Rakhshan2016letter,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Wireless Communications Letter},
	Publisher = {IEEE},
	Title = {Interference Models for Vehicular Ad Hoc Networks},
	Year = {2016, submitted}}

@article{Rakhshan2015Journal,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Publisher = {IEEE},
	Title = {Improving Safety on Highways by Customizing Vehicular Ad Hoc Networks},
	Year = {to appear, 2017}}

@inproceedings{Rakhshan2015Cogsima,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Booktitle = {IEEE International Multi-Disciplinary Conference on Cognitive Methods in Situation Awareness and Decision Support},
	Organization = {IEEE},
	Title = {A New Approach to Customization of Accident Warning Systems to Individual Drivers},
	Year = {2015}}

@inproceedings{Rakhshan2015CISS,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Nekoui, Mohammad},
	Booktitle = {Conference on Information Sciences and Systems},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {Driver-based adaptation of Vehicular Ad Hoc Networks for design of active safety systems},
	Year = {2015}}

@inproceedings{Rakhshan2014IV,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Ray, Evan},
	Booktitle = {Intelligent Vehicles Symposium},
	Organization = {IEEE},
	Pages = {1181--1186},
	Title = {Real-time estimation of the distribution of brake response times for an individual driver using Vehicular Ad Hoc Network.},
	Year = {2014}}

@inproceedings{Rakhshan2013Globecom,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Fisher, Donald and Nekoui, Mohammad},
	Booktitle = {IEEE Global Communications Conference},
	Organization = {IEEE},
	Pages = {1333--1337},
	Title = {Tuning collision warning algorithms to individual drivers for design of active safety systems.},
	Year = {2013}}

@article{Nekoui2012Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Number = {8},
	Pages = {2895--2905},
	Publisher = {IEEE},
	Title = {Throughput Scaling laws for Vehicular Ad Hoc Networks},
	Volume = {11},
	Year = {2012}}









@article{Nekoui2011Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein and Ni, Daiheng},
	Journal = {International Journal of Vehicular Technology},
	Pages = {1--11},
	Publisher = {Hindawi Publishing Corporation},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {2011},
	Year = {2011}}





	
@article{shokri2014optimal,
	  title={Optimal user-centric data obfuscation},
 	 author={Shokri, Reza},
 	 journal={arXiv preprint arXiv:1402.3426},
 	 year={2014}
	}
@article{chatzikokolakis2015location,
  title={Location privacy via geo-indistinguishability},
  author={Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
  journal={ACM SIGLOG News},
  volume={2},
  number={3},
  pages={46--69},
  year={2015},
  publisher={ACM}

}
@inproceedings{shokri2011quantifying2,
  title={Quantifying location privacy: the case of sporadic location exposure},
  author={Shokri, Reza and Theodorakopoulos, George and Danezis, George and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
  booktitle={Privacy Enhancing Technologies},
  pages={57--76},
  year={2011},
  organization={Springer}
}


@inproceedings{Mont1603:Defining,
AUTHOR="Zarrin Montazeri and Amir Houmansadr and Hossein Pishro-Nik",
TITLE="Defining Perfect Location Privacy Using Anonymization",
BOOKTITLE="2016 Annual Conference on Information Science and Systems (CISS) (CISS
2016)",
ADDRESS="Princeton, USA",
DAYS=16,
MONTH=mar,
YEAR=2016,
KEYWORDS="Information Theoretic Privacy; location-based services; Location Privacy;
Information Theory",
ABSTRACT="The popularity of mobile devices and location-based services (LBS) have
created great concerns regarding the location privacy of users of such
devices and services. Anonymization is a common technique that is often
being used to protect the location privacy of LBS users. In this paper, we
provide a general information theoretic definition for location privacy. In
particular, we define perfect location privacy. We show that under certain
conditions, perfect privacy is achieved if the pseudonyms of users is
changed after o(N^(2/r?1)) observations by the adversary, where N is the
number of users and r is the number of sub-regions or locations.
"
}
@article{our-isita-location,
	Author = {Zarrin Montazeri and Amir Houmansadr and Hossein Pishro-Nik},
	Journal = {IEEE International Symposium on Information Theory and Its Applications (ISITA)},
	Title = {Achieving Perfect Location Privacy in Markov Models Using Anonymization},
	Year = {2016}
	}
@article{our-TIFS,
	Author = {Zarrin Montazeri and Hossein Pishro-Nik and Amir Houmansadr},
	Journal = {IEEE Transactions on Information Forensics and Security, accepted with mandatory minor revisions},
	Title = {Perfect Location Privacy Using Anonymization in Mobile Networks},
	Year = {2017},
    note={Available on arxiv.org}
	}



@techreport{sampigethaya2005caravan,
  title={CARAVAN: Providing location privacy for VANET},
  author={Sampigethaya, Krishna and Huang, Leping and Li, Mingyan and Poovendran, Radha and Matsuura, Kanta and Sezaki, Kaoru},
  year={2005},
  institution={DTIC Document}
}
@incollection{buttyan2007effectiveness,
  title={On the effectiveness of changing pseudonyms to provide location privacy in VANETs},
  author={Butty{\'a}n, Levente and Holczer, Tam{\'a}s and Vajda, Istv{\'a}n},
  booktitle={Security and Privacy in Ad-hoc and Sensor Networks},
  pages={129--141},
  year={2007},
  publisher={Springer}
}
@article{sampigethaya2007amoeba,
  title={AMOEBA: Robust location privacy scheme for VANET},
  author={Sampigethaya, Krishna and Li, Mingyan and Huang, Leping and Poovendran, Radha},
  journal={Selected Areas in communications, IEEE Journal on},
  volume={25},
  number={8},
  pages={1569--1589},
  year={2007},
  publisher={IEEE}
}

@article{lu2012pseudonym,
  title={Pseudonym changing at social spots: An effective strategy for location privacy in vanets},
  author={Lu, Rongxing and Li, Xiaodong and Luan, Tom H and Liang, Xiaohui and Shen, Xuemin},
  journal={Vehicular Technology, IEEE Transactions on},
  volume={61},
  number={1},
  pages={86--96},
  year={2012},
  publisher={IEEE}
}
@inproceedings{lu2010sacrificing,
  title={Sacrificing the plum tree for the peach tree: A socialspot tactic for protecting receiver-location privacy in VANET},
  author={Lu, Rongxing and Lin, Xiaodong and Liang, Xiaohui and Shen, Xuemin},
  booktitle={Global Telecommunications Conference (GLOBECOM 2010), 2010 IEEE},
  pages={1--5},
  year={2010},
  organization={IEEE}
}
@inproceedings{lin2011stap,
  title={STAP: A social-tier-assisted packet forwarding protocol for achieving receiver-location privacy preservation in VANETs},
  author={Lin, Xiaodong and Lu, Rongxing and Liang, Xiaohui and Shen, Xuemin Sherman},
  booktitle={INFOCOM, 2011 Proceedings IEEE},
  pages={2147--2155},
  year={2011},
  organization={IEEE}
}
@inproceedings{gerlach2007privacy,
  title={Privacy in VANETs using changing pseudonyms-ideal and real},
  author={Gerlach, Matthias and Guttler, Felix},
  booktitle={Vehicular Technology Conference, 2007. VTC2007-Spring. IEEE 65th},
  pages={2521--2525},
  year={2007},
  organization={IEEE}
}
@inproceedings{el2002security,
  title={Security issues in a future vehicular network},
  author={El Zarki, Magda and Mehrotra, Sharad and Tsudik, Gene and Venkatasubramanian, Nalini},
  booktitle={European Wireless},
  volume={2},
  year={2002}
}

@article{hubaux2004security,
  title={The security and privacy of smart vehicles},
  author={Hubaux, Jean-Pierre and Capkun, Srdjan and Luo, Jun},
  journal={IEEE Security \& Privacy Magazine},
  volume={2},
  number={LCA-ARTICLE-2004-007},
  pages={49--55},
  year={2004}
}



@inproceedings{duri2002framework,
  title={Framework for security and privacy in automotive telematics},
  author={Duri, Sastry and Gruteser, Marco and Liu, Xuan and Moskowitz, Paul and Perez, Ronald and Singh, Moninder and Tang, Jung-Mu},
  booktitle={Proceedings of the 2nd international workshop on Mobile commerce},
  pages={25--32},
  year={2002},
  organization={ACM}
}
@misc{NS-3,
	Howpublished = {\url{https://www.nsnam.org/}}},
}
@misc{testbed,
	Howpublished = {\url{http://www.its.dot.gov/testbed/PDF/SE-MI-Resource-Guide-9-3-1.pdf}}},
@misc{NGSIM,
	Howpublished = {\url{http://ops.fhwa.dot.gov/trafficanalysistools/ngsim.htm}},
	}

@misc{National-a2013,
	Author = {National Highway Traffic Safety Administration},
	Howpublished = {\url{http://ops.fhwa.dot.gov/trafficanalysistools/ngsim.htm}},
	Title = {2013 Motor Vehicle Crashes: Overview. Traffic Safety Factors},
	Year = {2013}
	}

	@inproceedings{karnadi2007rapid,
	  title={Rapid generation of realistic mobility models for VANET},
	  author={Karnadi, Feliz Kristianto and Mo, Zhi Hai and Lan, Kun-chan},
	  booktitle={Wireless Communications and Networking Conference, 2007. WCNC 2007. IEEE},
	  pages={2506--2511},
	  year={2007},
	  organization={IEEE}
	}
	@inproceedings{saha2004modeling,
  title={Modeling mobility for vehicular ad-hoc networks},
  author={Saha, Amit Kumar and Johnson, David B},
  booktitle={Proceedings of the 1st ACM international workshop on Vehicular ad hoc networks},
  pages={91--92},
  year={2004},
  organization={ACM}
}
@inproceedings{lee2006modeling,
  title={Modeling steady-state and transient behaviors of user mobility: formulation, analysis, and application},
  author={Lee, Jong-Kwon and Hou, Jennifer C},
  booktitle={Proceedings of the 7th ACM international symposium on Mobile ad hoc networking and computing},
  pages={85--96},
  year={2006},
  organization={ACM}
}
@inproceedings{yoon2006building,
  title={Building realistic mobility models from coarse-grained traces},
  author={Yoon, Jungkeun and Noble, Brian D and Liu, Mingyan and Kim, Minkyong},
  booktitle={Proceedings of the 4th international conference on Mobile systems, applications and services},
  pages={177--190},
  year={2006},
  organization={ACM}
}

@inproceedings{choffnes2005integrated,
	title={An integrated mobility and traffic model for vehicular wireless networks},
	author={Choffnes, David R and Bustamante, Fabi{\'a}n E},
	booktitle={Proceedings of the 2nd ACM international workshop on Vehicular ad hoc networks},
	pages={69--78},
	year={2005},
	organization={ACM}
}

@inproceedings{Qian2008Globecom,
	title={CA Secure VANET MAC Protocol for DSRC Applications},
	author={Yi, Q. and Lu, K. and Moyeri, N.{\'a}n E},
	booktitle={Proceedings of IEEE GLOBECOM 2008},
	pages={1--5},
	year={2008},
	organization={IEEE}
}





	@inproceedings{naumov2006evaluation,
  title={An evaluation of inter-vehicle ad hoc networks based on realistic vehicular traces},
  author={Naumov, Valery and Baumann, Rainer and Gross, Thomas},
  booktitle={Proceedings of the 7th ACM international symposium on Mobile ad hoc networking and computing},
  pages={108--119},
  year={2006},
  organization={ACM}
}
	@article{sommer2008progressing,
  title={Progressing toward realistic mobility models in VANET simulations},
  author={Sommer, Christoph and Dressler, Falko},
  journal={Communications Magazine, IEEE},
  volume={46},
  number={11},
  pages={132--137},
  year={2008},
  publisher={IEEE}
}




	@inproceedings{mahajan2006urban,
  title={Urban mobility models for vanets},
  author={Mahajan, Atulya and Potnis, Niranjan and Gopalan, Kartik and Wang, Andy},
  booktitle={2nd IEEE International Workshop on Next Generation Wireless Networks},
  volume={33},
  year={2006}
}

@inproceedings{Rakhshan2016packet,
  title={Packet success probability derivation in a vehicular ad hoc network for a highway scenario},
  author={Rakhshan, Ali and Pishro-Nik, Hossein},
  booktitle={2016 Annual Conference on Information Science and Systems (CISS)},
  pages={210--215},
  year={2016},
  organization={IEEE}
}

@inproceedings{Rakhshan2016CISS,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Booktitle = {Conference on Information Sciences and Systems},
	Organization = {IEEE},
	Pages = {210--215},
	Title = {Packet Success Probability Derivation in a Vehicular Ad Hoc Network for a Highway Scenario},
	Year = {2016}}

@article{Nekoui2013Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {Journal on Selected Areas in Communications, Special Issue on Emerging Technologies in Communications},
	Number = {9},
	Pages = {491--503},
	Publisher = {IEEE},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {31},
	Year = {2013}}


@inproceedings{Nekoui2011MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM workshop on VehiculAr InterNETworking},
	Organization = {ACM},
	Title = {Analytic Design of Active Vehicular Safety Systems in Sparse Traffic},
	Year = {2011}}

@inproceedings{Nekoui2011VTC,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Analytical Design of Inter-vehicular Communications for Collision Avoidance},
	Year = {2011}}

@inproceedings{Bovee2011VTC,
	Author = {Bovee, Ben Louis and Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Evaluation of the Universal Geocast Scheme For VANETs},
	Year = {2011}}

@inproceedings{Nekoui2010MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM},
	Organization = {ACM},
	Title = {Fundamental Tradeoffs in Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2010IVCS,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IVCS},
	Organization = {IEEE},
	Title = {A Universal Geocast Scheme for Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2009ITW,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IEEE Communications Society Conference on Sensor, Mesh and Ad Hoc Communications and Networks Workshops},
	Organization = {IEEE},
	Pages = {1--3},
	Title = {A Geometrical Analysis of Obstructed Wireless Networks},
	Year = {2009}}

@article{Eslami2013Journal,
	Author = {Eslami, Ali and Nekoui, Mohammad and Pishro-Nik, Hossein and Fekri, Faramarz},
	Journal = {ACM Transactions on Sensor Networks},
	Number = {4},
	Pages = {51},
	Publisher = {ACM},
	Title = {Results on finite wireless sensor networks: Connectivity and coverage},
	Volume = {9},
	Year = {2013}}


@article{Jiafu2014Journal,
	Author = {Jiafu, W. and Zhang, D. and Zhao, S. and Yang, L. and Lloret, J.},
	Journal = {Communications Magazine},
	Number = {8},
	Pages = {106-113},
	Publisher = {IEEE},
	Title = {Context-aware vehicular cyber-physical systems with cloud support: architecture, challenges, and solutions},
	Volume = {52},
	Year = {2014}}

@inproceedings{Haas2010ACM,
	Author = {Haas, J.J. and Hu, Y.},
	Booktitle = {international workshop on VehiculAr InterNETworking},
	Organization = {ACM},
	Title = {Communication requirements for crash avoidance.},
	Year = {2010}}

@inproceedings{Yi2008GLOBECOM,
	Author = {Yi, Q. and Lu, K. and Moayeri, N.},
	Booktitle = {GLOBECOM},
	Organization = {IEEE},
	Title = {CA Secure VANET MAC Protocol for DSRC Applications.},
	Year = {2008}}

@inproceedings{Mughal2010ITSim,
	Author = {Mughal, B.M. and Wagan, A. and Hasbullah, H.},
	Booktitle = {International Symposium on Information Technology (ITSim)},
	Organization = {IEEE},
	Title = {Efficient congestion control in VANET for safety messaging.},
	Year = {2010}}

@article{Chang2011Journal,
	Author = {Chang, Y. and Lee, C. and Copeland, J.},
	Journal = {Selected Areas in Communications},
	Pages = {236 –249},
	Publisher = {IEEE},
	Title = {Goodput enhancement of VANETs in noisy CSMA/CA channels},
	Volume = {29},
	Year = {2011}}

@article{Garcia-Costa2011Journal,
	Author = {Garcia-Costa, C. and Egea-Lopez, E. and Tomas-Gabarron, J. B. and Garcia-Haro, J. and Haas, Z. J.},
	Journal = {Transactions on Intelligent Transportation Systems},
	Pages = {1 –16},
	Publisher = {IEEE},
	Title = {A stochastic model for chain collisions of vehicles equipped with vehicular communications},
	Volume = {99},
	Year = {2011}}

@article{Carbaugh2011Journal,
	Author = {Carbaugh, J. and Godbole,  D. N. and Sengupta, R. and Garcia-Haro, J. and Haas, Z. J.},
	Publisher = {Transportation Research Part C (Emerging Technologies)},
	Title = {Safety and capacity analysis of automated and manual highway systems},
	Year = {1997}}

@article{Goh2004Journal,
	Author = {Goh, P. and Wong, Y.},
	Publisher = {Appl Health Econ Health Policy},
	Title = {Driver perception response time during the signal change interval},
	Year = {2004}}

@article{Chang1985Journal,
	Author = {Chang, M.S. and Santiago, A.J.},
	Pages = {20-30},
	Publisher = {Transportation Research Record},
	Title = {Timing traffic signal changes based on driver behavior},
	Volume = {1027},
	Year = {1985}}

@article{Green2000Journal,
	Author = {Green, M.},
	Pages = {195-216},
	Publisher = {Transportation Human Factors},
	Title = {How long does it take to stop? Methodological analysis of driver perception-brake times.},
	Year = {2000}}

@article{Koppa2005,
	Author = {Koppa, R.J.},
	Pages = {195-216},
	Publisher = {http://www.fhwa.dot.gov/publications/},
	Title = {Human Factors},
	Year = {2005}}

@inproceedings{Maxwell2010ETC,
	Author = {Maxwell, A. and Wood, K.},
	Booktitle = {Europian Transport Conference},
	Organization = {http://www.etcproceedings.org/paper/review-of-traffic-signals-on-high-speed-roads},
	Title = {Review of Traffic Signals on High Speed Road},
	Year = {2010}}

@article{Wortman1983,
	Author = {Wortman, R.H. and Matthias, J.S.},
	Publisher = {Arizona Department of Transportation},
	Title = {An Evaluation of Driver Behavior at Signalized Intersections},
	Year = {1983}}
@inproceedings{Zhang2007IASTED,
	Author = {Zhang, X. and Bham, G.H.},
	Booktitle = {18th IASTED International Conference: modeling and simulation},
	Title = {Estimation of driver reaction time from detailed vehicle trajectory data.},
	Year = {2007}}


@inproceedings{bai2003important,
  title={IMPORTANT: A framework to systematically analyze the Impact of Mobility on Performance of RouTing protocols for Adhoc NeTworks},
  author={Bai, Fan and Sadagopan, Narayanan and Helmy, Ahmed},
  booktitle={INFOCOM 2003. Twenty-second annual joint conference of the IEEE computer and communications. IEEE societies},
  volume={2},
  pages={825--835},
  year={2003},
  organization={IEEE}
}


@inproceedings{abedi2008enhancing,
	  title={Enhancing AODV routing protocol using mobility parameters in VANET},
	  author={Abedi, Omid and Fathy, Mahmood and Taghiloo, Jamshid},
	  booktitle={Computer Systems and Applications, 2008. AICCSA 2008. IEEE/ACS International Conference on},
	  pages={229--235},
	  year={2008},
	  organization={IEEE}
	}


@article{AlSultan2013Journal,
	Author = {Al-Sultan, Saif and Al-Bayatti, Ali H. and Zedan, Hussien},
	Journal = {IEEE Transactions on Vehicular Technology},
	Number = {9},
	Pages = {4264-4275},
	Publisher = {IEEE},
	Title = {Context Aware Driver Behaviour Detection System in Intelligent Transportation Systems},
	Volume = {62},
	Year = {2013}}






@article{Leow2008ITS,
	Author = {Leow, Woei Ling and Ni, Daiheng and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Intelligent Transportation Systems},
	Number = {2},
	Pages = {369--374},
	Publisher = {IEEE},
	Title = {A Sampling Theorem Approach to Traffic Sensor Optimization},
	Volume = {9},
	Year = {2008}}



@article{REU2007,
	Author = {D. Ni and H. Pishro-Nik and R. Prasad and M. R. Kanjee and H. Zhu and T. Nguyen},
	Journal = {in 14th World Congress on Intelligent Transport Systems},
	Title = {Development of a prototype intersection collision avoidance system under VII},
	Year = {2007}}




@inproceedings{salamatian2013hide,
  title={How to hide the elephant-or the donkey-in the room: Practical privacy against statistical inference for large data.},
  author={Salamatian, Salman and Zhang, Amy and du Pin Calmon, Flavio and Bhamidipati, Sandilya and Fawaz, Nadia and Kveton, Branislav and Oliveira, Pedro and Taft, Nina},
  booktitle={GlobalSIP},
  pages={269--272},
  year={2013}
}

@article{sankar2013utility,
  title={Utility-privacy tradeoffs in databases: An information-theoretic approach},
  author={Sankar, Lalitha and Rajagopalan, S Raj and Poor, H Vincent},
  journal={Information Forensics and Security, IEEE Transactions on},
  volume={8},
  number={6},
  pages={838--852},
  year={2013},
  publisher={IEEE}
}
@inproceedings{ghinita2007prive,
  title={PRIVE: anonymous location-based queries in distributed mobile systems},
  author={Ghinita, Gabriel and Kalnis, Panos and Skiadopoulos, Spiros},
  booktitle={Proceedings of the 16th international conference on World Wide Web},
  pages={371--380},
  year={2007},
  organization={ACM}
}

@article{beresford2004mix,
  title={Mix zones: User privacy in location-aware services},
  author={Beresford, Alastair R and Stajano, Frank},
  year={2004},
  publisher={IEEE}
}

%@inproceedings{Mont1610Achieving,
%  title={Achieving Perfect Location Privacy in Markov Models Using Anonymization},
%  author={Montazeri, Zarrin and Houmansadr, Amir and H.Pishro-Nik},
%  booktitle="2016 International Symposium on Information Theory and its Applications
%  (ISITA2016)",
%  address="Monterey, USA",
%  days=30,
%  month=oct,
%  year=2016,
%}

@article{csiszar1996almost,
  title={Almost independence and secrecy capacity},
  author={Csisz{\'a}r, Imre},
  journal={Problemy Peredachi Informatsii},
  volume={32},
  number={1},
  pages={48--57},
  year={1996},
  publisher={Russian Academy of Sciences, Branch of Informatics, Computer Equipment and Automatization}
}

@article{yamamoto1983source,
  title={A source coding problem for sources with additional outputs to keep secret from the receiver or wiretappers (corresp.)},
  author={Yamamoto, Hirosuke},
  journal={IEEE Transactions on Information Theory},
  volume={29},
  number={6},
  pages={918--923},
  year={1983},
  publisher={IEEE}
}


@inproceedings{calmon2015fundamental,
  title={Fundamental limits of perfect privacy},
  author={Calmon, Flavio P and Makhdoumi, Ali and M{\'e}dard, Muriel},
  booktitle={Information Theory (ISIT), 2015 IEEE International Symposium on},
  pages={1796--1800},
  year={2015},
  organization={IEEE}
}



@inproceedings{Lehman1999Large-Sample-Theory,
	title={Elements of Large Sample Theory},
	author={E. L. Lehman},
	organization={Springer},
	year={1999}
}


@inproceedings{Ferguson1999Large-Sample-Theory,
	title={A Course in Large Sample Theory},
	author={Thomas S. Ferguson},
	organization={CRC Press},
	year={1996}
}



@inproceedings{Dembo1999Large-Deviations,
	title={Large Deviation Techniques and Applications, Second Edition},
	author={A. Dembo and O. Zeitouni},
	organization={Springer},
	year={1998}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Hossein's Coding Journals
%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{myoptics,
  AUTHOR =       "H. Pishro-Nik and N. Rahnavard and J. Ha and F. Fekri and A. Adibi ",
  TITLE =        "Low-density parity-check codes for volume holographic memory systems",
  JOURNAL =      " Appl. Opt.",
  YEAR =         "2003",
  volume =       "42",
  pages =        "861-870  "
 }






@ARTICLE{myit,
  AUTHOR =       "H. Pishro-Nik and F. Fekri  ",
  TITLE =        "On Decoding of Low-Density Parity-Check Codes on the Binary Erasure Channel",
  JOURNAL =      "IEEE Trans. Inform. Theory",
  YEAR =         "2004",
  volume =       "50",
  pages =        "439--454"
  }




@ARTICLE{myitpuncture,
  AUTHOR =       "H. Pishro-Nik and F. Fekri  ",
  TITLE =        "Results on Punctured Low-Density Parity-Check Codes and Improved Iterative Decoding Techniques",
  JOURNAL =      "IEEE Trans. on Inform. Theory",
  YEAR =         "2007",
  volume =       "53",
  number=        "2",
  pages =        "599--614",
  month= "February"
  }




@ARTICLE{myitlinmimdist,
  AUTHOR =       "H. Pishro-Nik and F. Fekri",
  TITLE =        "Performance of Low-Density Parity-Check Codes With Linear Minimum Distance",
  JOURNAL =         "IEEE Trans. Inform. Theory ",
  YEAR =         "2006",
  volume =       "52",
  number="1",
  pages =        "292 --300"
  }






@ARTICLE{myitnonuni,
  AUTHOR =       "H. Pishro-Nik and N. Rahnavard and F. Fekri  ",
  TITLE =        "Non-uniform Error Correction Using Low-Density Parity-Check Codes",
  JOURNAL =      "IEEE Trans. Inform. Theory",
  YEAR =         "2005",
  volume =       "51",
  number=  "7",
  pages =        "2702--2714"
 }





@article{eslamitcomhybrid10,
 author = {A. Eslami and S. Vangala and H. Pishro-Nik},
 title = {Hybrid channel codes for highly efficient FSO/RF communication systems},
 journal = {IEEE Transactions on Communications},
 volume = {58},
 number = {10},
 year = {2010},
 pages = {2926--2938},
 }


@article{eslamitcompolar13,
 author = {A. Eslami and H. Pishro-Nik},
 title = {On Finite-Length Performance of Polar Codes: Stopping Sets, Error Floor, and Concatenated Design},
 journal = {IEEE Transactions on Communications},
 volume = {61},
 number = {13},
 year = {2013},
 pages = {919--929},
 }



 @article{saeeditcom11,
 author = {H. Saeedi and H. Pishro-Nik and  A. H. Banihashemi},
 title = {Successive maximization for the systematic design of universally capacity approaching rate-compatible
 sequences of LDPC code ensembles over binary-input output-symmetric memoryless channels},
 journal = {IEEE Transactions on Communications},
 year = {2011},
 volume={59},
 number = {7}
 }


@article{rahnavard07,
 author = {Rahnavard, N. and Pishro-Nik, H. and Fekri, F.},
 title = {Unequal Error Protection Using Partially Regular LDPC Codes},
 journal = {IEEE Transactions on Communications},
 year = {2007},
 volume = {55},
 number = {3},
 pages = {387 -- 391}
 }


 @article{hosseinira04,
 author = {H. Pishro-Nik and F. Fekri},
 title = {Irregular repeat-accumulate codes for volume holographic memory systems},
 journal = {Journal of Applied Optics},
 year = {2004},
 volume = {43},
 number = {27},
 pages = {5222--5227},
 }


@article{azadeh2015Ephemeralkey,
 author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
 title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
 journal = {IEEE Transactions on Wireless Communications},
 year = {2015},
 volume = {14},
 number = {11},
 pages = {6072--6081},
}


@article{azadeh2014Everlasting,
 author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
 title = {Everlasting secrecy in disadvantaged wireless environments against sophisticated eavesdroppers},
 journal = {48th Asilomar Conference on Signals, Systems and Computers},
 year = {2014},
 pages = {1994--1998},
}


@article{azadeh2013ISIT,
 author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
 title = {Artificial intersymbol interference (ISI) to exploit receiver imperfections for secrecy},
 journal = {IEEE International Symposium on Information Theory (ISIT)},
 year = {2013},
}


@article{azadeh2013Jsac,
 author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
 title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
 journal = {IEEE Journal on Selected Areas in Communications},
 year = {2013},
 volume = {31},
 number = {9},
 pages = {1828--1839},
}


@article{azadeh2012Allerton,
 author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
 title = {Exploiting the non-commutativity of nonlinear operators for information-theoretic security in disadvantaged wireless environments},
 journal = {50th Annual Allerton Conference on Communication, Control, and Computing},
 year = {2012},
 pages = {233--240},
}


@article{azadeh2012Infocom,
 author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
 title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
 journal = {IEEE INFOCOM},
 year = {2012},
 pages = {1179--1187},
}

@article{1corser2016evaluating,
  title={Evaluating Location Privacy in Vehicular Communications and Applications},
  author={Corser, George P and Fu, Huirong and Banihani, Abdelnasser},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={17},
  number={9},
  pages={2658-2667},
  year={2016},
  publisher={IEEE}
}
@article{2zhang2016designing,
  title={On Designing Satisfaction-Ratio-Aware Truthful Incentive Mechanisms for k-Anonymity Location Privacy},
  author={Zhang, Yuan and Tong, Wei and Zhong, Sheng},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={11},
  number={11},
  pages={2528--2541},
  year={2016},
  publisher={IEEE}
}
@article{3li2016privacy,
  title={Privacy-preserving Location Proof for Securing Large-scale Database-driven Cognitive Radio Networks},
  author={Li, Yi and Zhou, Lu and Zhu, Haojin and Sun, Limin},
  journal={IEEE Internet of Things Journal},
  volume={3},
  number={4},
  pages={563-571},
  year={2016},
  publisher={IEEE}
}
@article{4olteanu2016quantifying,
  title={Quantifying Interdependent Privacy Risks with Location Data},
  author={Olteanu, Alexandra-Mihaela and Huguenin, K{\'e}vin and Shokri, Reza and Humbert, Mathias and Hubaux, Jean-Pierre},
  journal={IEEE Transactions on Mobile Computing},
  year={2016},
  volume={PP},
  number={99},
  pages={1-1},
  publisher={IEEE}
}
@article{5yi2016practical,
  title={Practical Approximate k Nearest Neighbor Queries with Location and Query Privacy},
  author={Yi, Xun and Paulet, Russell and Bertino, Elisa and Varadharajan, Vijay},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={28},
  number={6},
  pages={1546--1559},
  year={2016},
  publisher={IEEE}
}
@article{6li2016privacy,
  title={Privacy Leakage of Location Sharing in Mobile Social Networks: Attacks and Defense},
  author={Li, Huaxin and Zhu, Haojin and Du, Suguo and Liang, Xiaohui and Shen, Xuemin},
  journal={IEEE Transactions on Dependable and Secure Computing},
  year={2016},
  volume={PP},
  number={99},
  publisher={IEEE}
}

@article{7murakami2016localization,
  title={Localization Attacks Using Matrix and Tensor Factorization},
  author={Murakami, Takao and Watanabe, Hajime},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={11},
  number={8},
  pages={1647--1660},
  year={2016},
  publisher={IEEE}
}
@article{8zurbaran2015near,
  title={Near-Rand: Noise-based Location Obfuscation Based on Random Neighboring Points},
  author={Zurbaran, Mayra Alejandra and Avila, Karen and Wightman, Pedro and Fernandez, Michael},
  journal={IEEE Latin America Transactions},
  volume={13},
  number={11},
  pages={3661--3667},
  year={2015},
  publisher={IEEE}
}

@article{9tan2014anti,
  title={An anti-tracking source-location privacy protection protocol in wsns based on path extension},
  author={Tan, Wei and Xu, Ke and Wang, Dan},
  journal={IEEE Internet of Things Journal},
  volume={1},
  number={5},
  pages={461--471},
  year={2014},
  publisher={IEEE}
}

@article{10peng2014enhanced,
  title={Enhanced Location Privacy Preserving Scheme in Location-Based Services},
  author={Peng, Tao and Liu, Qin and Wang, Guojun},
  journal={IEEE Systems Journal},
  year={2014},
  volume={PP},
  number={99},
  pages={1-12},
  publisher={IEEE}
}
@article{11dewri2014exploiting,
  title={Exploiting service similarity for privacy in location-based search queries},
  author={Dewri, Rinku and Thurimella, Ramakrisha},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={25},
  number={2},
  pages={374--383},
  year={2014},
  publisher={IEEE}
}

@article{12hwang2014novel,
  title={A novel time-obfuscated algorithm for trajectory privacy protection},
  author={Hwang, Ren-Hung and Hsueh, Yu-Ling and Chung, Hao-Wei},
  journal={IEEE Transactions on Services Computing},
  volume={7},
  number={2},
  pages={126--139},
  year={2014},
  publisher={IEEE}
}
@article{13puttaswamy2014preserving,
  title={Preserving location privacy in geosocial applications},
  author={Puttaswamy, Krishna PN and Wang, Shiyuan and Steinbauer, Troy and Agrawal, Divyakant and El Abbadi, Amr and Kruegel, Christopher and Zhao, Ben Y},
  journal={IEEE Transactions on Mobile Computing},
  volume={13},
  number={1},
  pages={159--173},
  year={2014},
  publisher={IEEE}
}

@article{14zhang2014privacy,
  title={Privacy quantification model based on the Bayes conditional risk in Location-Based Services},
  author={Zhang, Xuejun and Gui, Xiaolin and Tian, Feng and Yu, Si and An, Jian},
  journal={Tsinghua Science and Technology},
  volume={19},
  number={5},
  pages={452--462},
  year={2014},
  publisher={TUP}
}

@article{15bilogrevic2014privacy,
  title={Privacy-preserving optimal meeting location determination on mobile devices},
  author={Bilogrevic, Igor and Jadliwala, Murtuza and Joneja, Vishal and Kalkan, K{\"u}bra and Hubaux, Jean-Pierre and Aad, Imad},
  journal={IEEE transactions on information forensics and security},
  volume={9},
  number={7},
  pages={1141--1156},
  year={2014},
  publisher={IEEE}
}
@article{16haghnegahdar2014privacy,
  title={Privacy Risks in Publishing Mobile Device Trajectories},
  author={Haghnegahdar, Alireza and Khabbazian, Majid and Bhargava, Vijay K},
  journal={IEEE Wireless Communications Letters},
  volume={3},
  number={3},
  pages={241--244},
  year={2014},
  publisher={IEEE}
}
@article{17malandrino2014verification,
  title={Verification and inference of positions in vehicular networks through anonymous beaconing},
  author={Malandrino, Francesco and Borgiattino, Carlo and Casetti, Claudio and Chiasserini, Carla-Fabiana and Fiore, Marco and Sadao, Roberto},
  journal={IEEE Transactions on Mobile Computing},
  volume={13},
  number={10},
  pages={2415--2428},
  year={2014},
  publisher={IEEE}
}
@article{18shokri2014hiding,
  title={Hiding in the mobile crowd: Locationprivacy through collaboration},
  author={Shokri, Reza and Theodorakopoulos, George and Papadimitratos, Panos and Kazemi, Ehsan and Hubaux, Jean-Pierre},
  journal={IEEE transactions on dependable and secure computing},
  volume={11},
  number={3},
  pages={266--279},
  year={2014},
  publisher={IEEE}
}
@article{19freudiger2013non,
  title={Non-cooperative location privacy},
  author={Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
  journal={IEEE Transactions on Dependable and Secure Computing},
  volume={10},
  number={2},
  pages={84--98},
  year={2013},
  publisher={IEEE}
}
@article{20gao2013trpf,
  title={TrPF: A trajectory privacy-preserving framework for participatory sensing},
  author={Gao, Sheng and Ma, Jianfeng and Shi, Weisong and Zhan, Guoxing and Sun, Cong},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={8},
  number={6},
  pages={874--887},
  year={2013},
  publisher={IEEE}
}
@article{21ma2013privacy,
  title={Privacy vulnerability of published anonymous mobility traces},
  author={Ma, Chris YT and Yau, David KY and Yip, Nung Kwan and Rao, Nageswara SV},
  journal={IEEE/ACM Transactions on Networking},
  volume={21},
  number={3},
  pages={720--733},
  year={2013},
  publisher={IEEE}
}
@article{22niu2013pseudo,
  title={Pseudo-Location Updating System for privacy-preserving location-based services},
  author={Niu, Ben and Zhu, Xiaoyan and Chi, Haotian and Li, Hui},
  journal={China Communications},
  volume={10},
  number={9},
  pages={1--12},
  year={2013},
  publisher={IEEE}
}
@article{23dewri2013local,
  title={Local differential perturbations: Location privacy under approximate knowledge attackers},
  author={Dewri, Rinku},
  journal={IEEE Transactions on Mobile Computing},
  volume={12},
  number={12},
  pages={2360--2372},
  year={2013},
  publisher={IEEE}
}
@inproceedings{24kanoria2012tractable,
  title={Tractable bayesian social learning on trees},
  author={Kanoria, Yashodhan and Tamuz, Omer},
  booktitle={Information Theory Proceedings (ISIT), 2012 IEEE International Symposium on},
  pages={2721--2725},
  year={2012},
  organization={IEEE}
}
@inproceedings{25farias2005universal,
  title={A universal scheme for learning},
  author={Farias, Vivek F and Moallemi, Ciamac C and Van Roy, Benjamin and Weissman, Tsachy},
  booktitle={Proceedings. International Symposium on Information Theory, 2005. ISIT 2005.},
  pages={1158--1162},
  year={2005},
  organization={IEEE}
}
@inproceedings{26misra2013unsupervised,
  title={Unsupervised learning and universal communication},
  author={Misra, Vinith and Weissman, Tsachy},
  booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
  pages={261--265},
  year={2013},
  organization={IEEE}
}
@inproceedings{27ryabko2013time,
  title={Time-series information and learning},
  author={Ryabko, Daniil},
  booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
  pages={1392--1395},
  year={2013},
  organization={IEEE}
}
@inproceedings{28krzakala2013phase,
  title={Phase diagram and approximate message passing for blind calibration and dictionary learning},
  author={Krzakala, Florent and M{\'e}zard, Marc and Zdeborov{\'a}, Lenka},
  booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
  pages={659--663},
  year={2013},
  organization={IEEE}
}
@inproceedings{29sakata2013sample,
  title={Sample complexity of Bayesian optimal dictionary learning},
  author={Sakata, Ayaka and Kabashima, Yoshiyuki},
  booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
  pages={669--673},
  year={2013},
  organization={IEEE}
}
@inproceedings{30predd2004consistency,
  title={Consistency in a model for distributed learning with specialists},
  author={Predd, Joel B and Kulkarni, Sanjeev R and Poor, H Vincent},
  booktitle={IEEE International Symposium on Information Theory},
  year={2004},
organization={IEEE}
}
@inproceedings{31nokleby2016rate,
  title={Rate-Distortion Bounds on Bayes Risk in Supervised Learning},
  author={Nokleby, Matthew and Beirami, Ahmad and Calderbank, Robert},
  booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
pages={2099-2103},
  year={2016},
organization={IEEE}
}

@inproceedings{32le2016imperfect,
  title={Are imperfect reviews helpful in social learning?},
  author={Le, Tho Ngoc and Subramanian, Vijay G and Berry, Randall A},
  booktitle={Information Theory (ISIT), 2016 IEEE International Symposium on},
  pages={2089--2093},
  year={2016},
  organization={IEEE}
}
@inproceedings{33gadde2016active,
  title={Active Learning for Community Detection in Stochastic Block Models},
  author={Gadde, Akshay and Gad, Eyal En and Avestimehr, Salman and Ortega, Antonio},
  booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
  pages={1889-1893},
  year={2016}
}
@inproceedings{34shakeri2016minimax,
  title={Minimax Lower Bounds for Kronecker-Structured Dictionary Learning},
  author={Shakeri, Zahra and Bajwa, Waheed U and Sarwate, Anand D},
  booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
  pages={1148-1152},
  year={2016}
}
@article{35lee2015speeding,
  title={Speeding up distributed machine learning using codes},
  author={Lee, Kangwook and Lam, Maximilian and Pedarsani, Ramtin and Papailiopoulos, Dimitris and Ramchandran, Kannan},
  booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
  pages={1143-1147},
  year={2016}
}
@article{36oneto2016statistical,
  title={Statistical Learning Theory and ELM for Big Social Data Analysis},
  author={Oneto, Luca and Bisio, Federica and Cambria, Erik and Anguita, Davide},
  journal={ieee CompUTATionAl inTelliGenCe mAGAzine},
  volume={11},
  number={3},
  pages={45--55},
  year={2016},
  publisher={IEEE}
}
@article{37lin2015probabilistic,
  title={Probabilistic approach to modeling and parameter learning of indirect drive robots from incomplete data},
  author={Lin, Chung-Yen and Tomizuka, Masayoshi},
  journal={IEEE/ASME Transactions on Mechatronics},
  volume={20},
  number={3},
  pages={1036--1045},
  year={2015},
  publisher={IEEE}
}
@article{38wang2016towards,
  title={Towards Bayesian Deep Learning: A Framework and Some Existing Methods},
  author={Wang, Hao and Yeung, Dit-Yan},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={PP},
  number={99},
  year={2016},
  publisher={IEEE}
}


%%%%%Informationtheoreticsecurity%%%%%%%%%%%%%%%%%%%%%%%




@inproceedings{Bloch2011PhysicalSecBook,
	title={Physical-Layer Security},
	author={M. Bloch and J. Barros},
	organization={Cambridge University Press},
	year={2011}
}



@inproceedings{Liang2009InfoSecBook,
	title={Information Theoretic Security},
	author={Y. Liang and H. V. Poor and S. Shamai (Shitz)},
	organization={Now Publishers Inc.},
	year={2009}
}


@inproceedings{Zhou2013PhysicalSecBook,
	title={Physical Layer Security in Wireless Communications},
	author={ X. Zhou and L. Song and Y. Zhang},
	organization={CRC Press},
	year={2013}
}

@article{Ni2012IEA,
	Author = {D. Ni and H. Liu and W. Ding and  Y. Xie and H. Wang and H. Pishro-Nik and Q. Yu},
	Journal = {IEA/AIE},
	Title = {Cyber-Physical Integration to Connect Vehicles for Transformed Transportation Safety and Efficiency},
	Year = {2012}}



@inproceedings{Ni2012Inproceedings,
	Author = {D. Ni, H. Liu, Y. Xie, W. Ding, H. Wang, H. Pishro-Nik, Q. Yu and M. Ferreira},
	Booktitle = {Spring Simulation Multiconference},
	Date-Added = {2016-09-04 14:18:42 +0000},
	Date-Modified = {2016-09-06 16:22:14 +0000},
	Title = {Virtual Lab of Connected Vehicle Technology},
	Year = {2012}}

@inproceedings{Ni2012Inproceedings,
	Author = {D. Ni, H. Liu, W. Ding, Y. Xie, H. Wang, H. Pishro-Nik and Q. Yu,},
	Booktitle = {IEA/AIE},
	Date-Added = {2016-09-04 09:11:02 +0000},
	Date-Modified = {2016-09-06 14:46:53 +0000},
	Title = {Cyber-Physical Integration to Connect Vehicles for Transformed Transportation Safety and Efficiency},
	Year = {2012}}


@article{Nekoui_IJIPT_2009,
	Author = {M. Nekoui and D. Ni and H. Pishro-Nik and R. Prasad and M. Kanjee and H. Zhu and T. Nguyen},
	Journal = {International Journal of Internet Protocol Technology (IJIPT)},
	Number = {3},
	Pages = {},
	Publisher = {},
	Title = {Development of a VII-Enabled Prototype Intersection Collision Warning System},
	Volume = {4},
	Year = {2009}}


@inproceedings{Pishro_Ganz_Ni,
	Author = {H. Pishro-Nik, A. Ganz, and Daiheng Ni},
	Booktitle = {Forty-Fifth Annual Allerton Conference on Communication, Control, and Computing. Allerton House, Monticello, IL},
	Date-Added = {},
	Date-Modified = {},
	Number = {},
	Pages = {},
	Title = {The capacity of vehicular ad hoc networks},
	Volume = {},
	Year = {September 26-28, 2007}}

@inproceedings{Leow_Pishro_Ni_1,
	Author = {W. L. Leow, H. Pishro-Nik and Daiheng Ni},
	Booktitle = {IEEE Global Telecommunications Conference, Washington, D.C.},
	Date-Added = {},
	Date-Modified = {},
	Number = {},
	Pages = {},
	Title = {Delay and Energy Tradeoff in Multi-state Wireless Sensor Networks},
	Volume = {},
	Year = {November 26-30, 2007}}


@misc{UMass-Trans,
title = {{UMass Transportation Center}},
note = {\url{http://www.umasstransportationcenter.org/}},
}


@inproceedings{Haenggi2013book,
	title={Stochastic geometry for wireless networks},
	author={M. Haenggi},
	organization={Cambridge Uinversity Press},
	year={2013}
}


==> Revised paper/relatedwork.tex <==
\section{Related Work}
\label{relatedwork}

Previously, mutual information has been used as a privacy metric in a number of settings,~\cite{salamatian2013hide, csiszar1996almost, calmon2015fundamental, sankar2013utility, sankarISIT,sankar, yamamoto1983source, hyposankar}. However, the framework and problem formulation for our setting (Internet of Things (IoT) privacy) is quite different from those encountered in previous work. More specifically, the IoT privacy problem we consider here is based on a large set of time-series data that belong to different users with different statistical patterns that has gone through a privacy-preserving mechanism, and the adversary is aiming at de-anonymizing and de-obfuscating the data.


Next, consider related works in smart-home/public environment Internet of Things (IoT) systems. The authors in \cite{8ukil2015privacy} investigate privacy for IoT smart energy metering where the concern results from the fact that any privacy breach can reveal in-house activity. A `Dynamic Privacy Analyzer' scheme is proposed as an attempt towards achieving a unique privacy metric that is derived from fundamental principles like robust statistics and information theory.
To deal with concerns in different smart-home IoT devices such as lights, smoke-alarms, power switches, baby monitors, and weighing scales, which again makes it possible for the entities to snoop and intrude into the family's activities, the authors in \cite{12sivaraman2015network} suggest that device-level protections be augmented with network-level security solutions. This can be achieved through software defined networking technology when used to dynamically block/quarantine suspicious devices. In \cite{10harris2016security}, the authors consider the privacy issues in public environments such as an IoT-enabled retail store. An IoT-enable retail store has the potential to provide rich, targeted information and services to users within the environment. However, to fully realize such potential, users must be willing to share certain data regarding their habits and preferences with the public IoT facility. To encourage users to share such information, the paper proposes a protocol to ensure the customers that their data will not be leaked to third parties.

As far as other applications of IoT is concerned, authors in \cite{9dalipi2016security} investigate privacy considerations for IoT applications on Smart Grids. In particular, the authors address three types of challenge domains: customer domain, information and communication domain, and the grid domain. In \cite{battery15}, the author tried to provide privacy for smart-metering systems with rechargeable batteries by obscuring the user's power demand.
In \cite{11al2015security}, the authors consider the privacy issue of wearable devices. These devices make it possible for health care services start a new phase in serving patients' needs and monitor their health remotely. Finally, authors in \cite{14sadeghi2015security}, overview the privacy challenges in  industrial IoT systems.

Among these applications, location privacy constitutes one of the most important aspects of IoT privacy. Location privacy preserving mechanisms (LPPMs) can be categorized into two main classes:
identity perturbation LPPMs (anonymization) ~\cite{1corser2016evaluating,hoh2005protecting,freudiger2007mix, ma2009location, shokri2011quantifying, Naini2016}
and location perturbation LPPMs (obfuscation)~\cite{shokri2012protecting, gruteser2003anonymous,  bordenabe2014optimal}.

There are various approaches suggested for identity perturbation LPPMs. Particularly,  k-anonymity approaches help to keep each user's identity indistinguishable within a group of $k-1$ other users ~\cite{1corser2016evaluating,2zhang2016designing,11dewri2014exploiting, gedik2005location, zhong2009distributed, mokbel2006new, sweeney2002k, bordenabe2014optimal, kalnis2007preventing,liu2013game}. Another proposal changes users' pseudonyms within areas called mix-zones~\cite{hoh2005protecting, beresford2003location, freudiger2009optimal, beresford2003location, palanisamy2011mobimix}. There are also various approaches used by location perturbation LPPMs.  For instance, cloaking replaces each user's location information with a larger region~\cite{18shokri2014hiding,8zurbaran2015near,hoh2007preserving, gruteser2003anonymous, gedik2005location, gedik2008protecting, bordenabe2014optimal, duckham2005formal, duckham2006spatiotemporal, xue2009location, wernke2014classification, cai2015cloaking, chow2011spatial, cheng2006preserving, mokbel2006new, kalnis2006preserving, khoshgozaran2011location, bamba2008supporting, um2010advanced, zhangwei2010distributed}, while an alternative direction is to use dummy locations in the set of possible locations of users~\cite{kido2005protection, krumm2009survey, shankar2009privately, chow2009faking, kido2005anonymous, lu2008pad}.
Some prior works combine techniques to achieve stronger location privacy. For instance, Freudiger et al.\ combine techniques from cryptography with mix-zones to improve location privacy~\cite{freudiger2007mix}.




Differential privacy, which aims at protecting queries on aggregated data, has also been applied to the problem of location privacy.
Particularly, several identity perturbation~\cite{lee2012differential, bordenabe2014optimal, chatzikokolakis2015geo, nguyen2013differential, machanavajjhala2008privacy} and location perturbation ~\cite{chatzikokolakis2013broadening,shokri2014optimal, chatzikokolakis2015location,andres2013geo,bordenabe2014optimal} LPPMs are based on differential privacy techniques.
Dewri~\cite{dewri2013local} combines k-anonymity and differential privacy to achieve higher location privacy. Alternatively, Andres et al.\ hide the exact location of a user in a region by adding Laplacian distributed noise  to achieve a desired level of geo-indistinguishability~\cite{andres2013geo}. In ~\cite{info2012}, it  is proved that differential privacy arises out of maximizing entropy principle which is equal to minimizing information leakage and is measured using the mutual information notion. ~\cite{yeb17} tries to reduce the expected estonimation loss by using differential privacy and constraining the privacy level.




Several studies aim at quantifying location privacy protection.  Shokri et al.~\cite{shokri2011quantifying, shokri2011quantifying2} define the expected estimation error of the adversary  as a metric to evaluate LPPM mechanisms.  Ma et al.~\cite{ma2009location}  use  uncertainty about users' location information to quantify user location privacy in vehicular networks.
To defeat localization attacks and achieve privacy at the same time, Shokri et al.~\cite{shokri2012protecting} proposed a method which finds optimal LPPM for an LBS given service quality constraints. Shokri et al.~\cite{shokri2012protecting} design LPPM mechanisms that will defeat localization attacks.
% To defeat localization attack and reach privacy at the same time, \cite{shokri2012protecting} proposed a method which finds optimal LPPM for LSB given service quality constraints.
In \cite{6li2016privacy} and \cite{4olteanu2016quantifying}, privacy leakage of location sharing and interdependent location privacy risks are quantified, respectively. A similar idea is proposed in \cite{14zhang2014privacy} where the quantification model is based on the Bayes conditional risk. Yu et al. \cite{diff2017} combine two complementary notations, geo-indstingushability and expected inference error, to achieve location privacy. The geo-indstingushability is derived from differential privacy but cannot adequately protect users' location against inference attacks of adversary by using prior information, and the expected inference error as privacy metric doesn't consider posterior information obtained from  pseudo-location. As a result, combining both notations gives users the opportunity to have location privacy. In addition, users are allowed to personalized error bound for different locations.

In \cite{5ullah2016novel}, the authors propose a novel model for preserving location privacy in IoT in which they propose the so-called Enhanced Semantic Obfuscation Technique (ESOT).
In \cite{7zhou2012preserving}, in the context of IoT based wireless sensor networks, the authors propose a flexible routing strategy, called Multi-routing Random Walk, which protects the sensor's location. Another approach has been proposed in \cite{6sathishkumar2016enhanced}.

The discussed studies demonstrate the growing importance of privacy. What is missing from the current literature is a solid theoretical framework for privacy that is general enough to encompass various privacy preserving methods in the literature. Such a framework will allow us to achieve provable privacy guarantees, obtain fundamental trade-offs between privacy and performance, and provide analytical tools to optimally achieve provable privacy.   The closest works to this paper are ~\cite{montazeri2016defining, Mont1610Achieving,tifs2016,sit2017,ciss2017}. As mentioned, these works only consider anonymization and only achiveability. In this paper, by considering obfuscation and anonymization, we characterize the limits of privacy in the entire $m(n)-a_n$ plane by considering both achievability and converse results.




























==> introduction_dg.tex <==
\section{Introduction}
\label{intro}

Various emerging systems and applications work by analyzing
the data submitted by their users in order to serve them; we call such systems  \emph{user-data driven} (UDD) \amir{we need a name. how's this?} services. Examples of UDD services include  smart cities, connected vehicles, smart homes, and connected healthcare devices, which are 
 revolutionizing our lives in different ways.  
Unfortunately, 	the sheer volume of user data collected by these systems 
compromises users' privacy ostensibly~\cite{FTC2015}. 
Even the employment of  standard 
privacy-protection mechanisms (e.g.,  anonymization of user identities and obfuscation of submitted data) does not mitigate the privacy leakage as the adversaries are able to use powerful statistical inference techniques to infer sensitive private information~\cite{FTC2015,0Quest2016, 2nia2016comprehensive, 3ukil2014iot, 4Hosseinzadeh2014,iotCastle,matching}.
 
To illustrate   their privacy leakage, consider the following three popular UDD services. 
(1) {\em Health care:}  Wearable monitors that constantly track user health variables can be invaluable in assessing individual health trends and responding to emergencies.  However, such monitors produce long time-series of user data uniquely matched to the health characteristics of each  user; (2) {\em Smart homes:}  Emerging smart-home technologies such as fine-grained power measurement systems can help users and utility providers to address one of the key challenges of the twenty-first century:  energy conservation.  But the measurements of power by such devices can be  mapped to users and reveal their lifestyle habits; and, (3) 
	{\em Connected vehicles:}  The location data provided by connected vehicles promises to greatly improve everyday lives by reducing congestion and traffic accidents.  However, the matching of such location traces to prior behavior not only allows for user tracking, but also reveals a user's habits.
In summary, despite their critical importance to the society and their emerging popularity, these services have one thing in common: 
they collect  long time-series of user data, for them to operate, 
that puts users' privacy at significant risk.

There are two main approaches to augment privacy in UDD services: 
 \emph{identity perturbation (anonymization)}, and \emph{location perturbation (obfuscation)}.  In anonymization techniques, privacy is obtained by concealing the mapping between users and data, and the mapping is changed periodically to  thwart statistical inference attacks that try to deanonymize the anonymized data traces by matching user data to 
 known  user profiles. 
 On the other hands,  obfuscation mechanisms aim at protecting privacy by perturbing user data, e.g., by adding noise to user locations. 
% Both anonymization and obfuscation mechanisms manipulate user data time-series in a way to not significantly impact the utility of the underlying UDD services. 


Anonymization and obfuscation improve user privacy at the cost of user utility.  In anonymization, we need to change these pseudonym mappings frequently to achieve high privacy by reducing the length of time series exploited by statistical analysis.  However, this frequent change could decrease usability and functionality by concealing the temporal relation between a user's locations, which may be critical in the utility of some systems, e.g., a dining recommendation system that makes suggestions based on the dining places visited by a user in the past.  For obfuscation-based mechanisms, the added noise to the reported values of user locations will degrade the application utility; for example, user utility would be degraded by location obfuscation in ride-sharing systems.  Thus, choosing the right level of privacy-protection mechanism is an important question, and understanding what levels of anonymization and obfuscation can provide theoretical guarantees of privacy is of interest.

In this paper, we derive the fundamental limits of user privacy in UDD services in the presence of both anonymization and obfuscation protection mechanisms. This work is built on our previous work on formalizing privacy in location-based services~\cite{montazeri2016defining, Mont1610Achieving,tifs2016, ciss2017}, by extensively expanding not just the application area but also user models and settings. 
Particularly, our previous work introduced the notion of 
\emph{perfect privacy} for location-based services, and derives the rate at which an anonymization mechanism should change the pseudonyms in order to 
achieve the defined perfect privacy. 
In this work, we expand the notion of perfect privacy to UDD services in general, and derive the conditions for it to hold when \emph{both}
anonymization and obfuscation-based protection mechanisms are employed.   
 We study both achievability and converse results.  

%In~\cite{montazeri2016defining, Mont1610Achieving,tifs2016, ciss2017}, an approach was introduced to understand the fundamental limits of privacy when only anonymization is used in location-based services. There, users are characterized by the statistics of their locations, and the adversary then tries to match traces to those statistics to de-anonymize users.  Per above, anonymization thwarts such statistical analysis by reducing the time series available for such a matching, and thus \cite{montazeri2016defining, Mont1610Achieving,tifs2016} considers the rate at which pseudonyms must be changed so as to preserve perfect location privacy.   In this paper, the perfect privacy set-up of \cite{tifs2016} is again employed; however, in addition to anonymization, perturbation (obfuscation) is also considered; thus, the adversary attempts to infer information about the actual locations by observing the obfuscated \emph{and} anonymized version of the location data.  We study both achievability and converse results.  

\subsection{Summary of the Results}

Given $n$, the total number of the users in a network, their degree of privacy depends 
on two parameters: (1) The number of observations $m=m(n)$ by the adversary per user for a fixed anonymization mapping (i.e., the number of observations before the pseudonyms are changed);  and (2) the value of the noise added by the obfuscation technique (as defined in Section~\ref{sec:framework}, we quantify the obfuscation noise with a parameter $a_n$).  
Intuitively, smaller $m(n)$ and larger $a_n$ result in stronger privacy, at the expense of lower utility for the users. 

Our goal is to identify values of $a_n$ and $m(n)$  that satisfy perfect privacy as the number of users grows ($n \rightarrow \infty$).
%
We show that when the users' data sets are governed by an i.i.d.\ process, 
the $m(n)- a_n$ plane can be divided into two areas.  In the first area, all users have perfect privacy~\cite{tifs2016} (as defined in Section~\ref{sec:framework}), and, in the second area, users have no privacy.  
Figure~\ref{fig:region} shows the limits of privacy in the entire $m(n)- a_n$. 
As the figure shows, in regions $1$, $2$, and $3$, users have perfect privacy, while in region $4$ users have no privacy.
\begin{figure}[h]
	\centering
	\includegraphics[width=0.8\linewidth, height=0.8 \linewidth]{fig/region}
	\caption{Limits of privacy in the entire $m(n)-a_n$ plane: in regions $1$, $2$, and $3$, users have perfect privacy, and in region $4$ users have no privacy.}
	\label{fig:region}
\end{figure}

For the case where the users' data sets are governed by irreducible and aperiodic Markov chains with $r$ states and $|E|$ edges, we show that users will have no privacy if $m =cn^{\frac{2}{|E|-r} +  \alpha}$ and $a_n =c'n^{-\left(\frac{1}{|E|-r}+\beta \right)}$, for some constants $c>0$, $c'>0$, $\alpha>0$, and $\beta>\frac{\alpha}{4}$. We also provide some insights for the opposite direction (under which conditions users have perfect privacy) for the case of Markov chains. 




  




%\subsection{Summary of Results}

%When there are $n$ users in the network, the privacy level of the users depends on two parameters: (1) The %number of observations $m=m(n)$ by the adversary per user for a fixed anonymization mapping (i.e.~the %number of observations before the pseudonyms are changed);  (2) The noise level of the obfuscation %technique.  In this paper, the noise level of the obfuscation is increasing in a parameter $a_n$, which is %defined precisely in Section \ref{sec:framework}.  Intuitively, smaller $m(n)$ and larger $a_n$ result in %stronger location privacy but lower user utility. Thus, the fundamental question is, as the number of users %grows ($n \rightarrow \infty$), what values of $a_n$ and $m(n)$ are required to insure location privacy?

%In this paper, we answer the above question for the entire $m(n)- a_n$ plane for the case where each users' %movement is governed by an i.i.d process. We will prove that the $m(n)- a_n$ plane can be divided into two %areas.  In the first area, all users have perfect location privacy\cite{tifs2016}, as will be defined precisely in %Section \ref{sec:framework}, and, in the second area, users have no location privacy.  Figure~\ref{fig:region} %shows the limits of location privacy in the entire $m(n)- a_n$. In other words, according to %Figure~\ref{fig:region}, in regions $1$, $2$, and $3$, users have perfect location privacy, and  in region $4$ %users have no location privacy.
%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.9\linewidth, height=0.6 \linewidth]{fig/region}
%	\caption{Limits of location privacy in the entire $m(n)-a_n$ planes: in regions $1$, $2$, and $3$, users %have perfect location privacy, and in region $4$ users have no location privacy.}
%	\label{fig:region}
%\end{figure}
%
%Also, for the case where the users movements are governed by irreducible and aperiodic Markov chains with %$r$ states and $|E|$ edges, we show that users will have no privacy if $m =cn^{\frac{2}{|E|-r} +  \alpha}$ %and $a_n =c'n^{-\left(\frac{1}{|E|-r}+\alpha \right)}$ for some positive constants  $c, c'>0$  and %$0<\alpha<1$. Showing the opposite direction (under which conditions users have perfect privacy) for the %case of Markov chains is among the future work.

%In the rest of the paper we will provide the details of the results. Due to the space limitations, the proofs can %be found in the publicly available longer version of the paper ~\cite{longversion}.


==> ref.tex <==

\bibliographystyle{./IEEEtran}
\bibliography{./IEEEabrv,./IEEEexample}

@article{kousha2,
	title={Robust Privacy-Utility Tradeoffs Under Differential Privacy and Hamming Distortion},
	author={Kousha Kalantari and Lalitha Sankar and Anand D. Sarwate},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={13},
	number={11},
	pages={2816--2830},
	year={2018},
	publisher={IEEE}
}



@article{DBLP:ITjournal,
  author    = {Naanin Takbiri and
               Amir Houmansadr and
               Dennis Goeckel and
               Hossein Pishro-Nik},
  title     = {Matching Anonymized and Obfuscated Time Series to Users' Profiles
},
  journal   = {CoRR},
  volume    = {abs/1710.00197},
  year      = {2017},
  url       = {https://arxiv.org/abs/1710.00197},
  archivePrefix = {arXiv},
  eprint    = {1710.00197},
  timestamp = {Sat, 30 Sep 2017 13:03:19 GMT},
}


@inproceedings{KeConferance,
   title={Bayesian Time Series Matching and Privacy},
    author={Ke Le and 	Hossein Pishro-Nik and Dennis Goeckel},
	booktitle={51th Asilomar Conference on Signals, Systems and Computers},
   year={2017},
  	address={Pacific Grove, CA}
   }	

@article{DBLP:journals/corr/LiaoSCT17,
  author    = {Jiachun Liao and
               Lalitha Sankar and
               Fl{\'{a}}vio du Pin Calmon and
               Vincent Yan Fu Tan},
  title     = {Hypothesis Testing under Maximal Leakage Privacy Constraints},
  journal   = {CoRR},
  volume    = {abs/1701.07099},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.07099},
  timestamp = {Wed, 07 Jun 2017 14:40:47 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LiaoSCT17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{sankar,
    title={On information-theoretic privacy with general distortion cost functions},
    author={Kalantari, Kousha and Sankar, Lalitha and  Kosut, Oliver},
    booktitle={2017 IEEE International Symposium on Information Theory (ISIT)},
    year={2017},
      	address={Aachen, Germany},

    organization={IEEE}
    
  }	


@article{hyposankar,
  author    = {Jiachun Liao and
               Lalitha Sankar and
               Vincent Y. F. Tan and
               Fl{\'{a}}vio du Pin Calmon},
  title     = {Hypothesis Testing in the High Privacy Limit},
  journal   = {CoRR},
  volume    = {abs/1607.00533},
  year      = {2016},
  url       = {http://arxiv.org/abs/1607.00533},
  timestamp = {Wed, 07 Jun 2017 14:41:19 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LiaoSTC16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{battery15,
  author    = {Simon Li and
               Ashish Khisti and
               Aditya Mahajan},
  title     = {Privacy-Optimal Strategies for Smart Metering Systems with a Rechargeable
               Battery},
  journal   = {CoRR},
  volume    = {abs/1510.07170},
  year      = {2015},
  url       = {http://arxiv.org/abs/1510.07170},
  timestamp = {Wed, 07 Jun 2017 14:40:53 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/LiKM15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{geo2013,
   title={Geo-indistinguishability: differential privacy for location-based systems},
    author={Miguel E. Andres and Nicolas E. Bordenabe and Konstantinos Chatzikokolakis and Catuscia Palamidessi},
	booktitle={Proceedings of the 2013 ACM SIGSAC conference on Computer and communications security},

   year={2013},
   pages={901--914},
  	address={New York, NY}
   }	

@article{Yeb17,
  author    = {Min Ye and
               Alexander Barg},
  title     = {Optimal Schemes for Discrete Distribution Estimation under Locally
               Differential Privacy},
  journal   = {CoRR},
  volume    = {abs/1702.00610},
  year      = {2017},
  url       = {http://arxiv.org/abs/1702.00610},
  timestamp = {Wed, 07 Jun 2017 14:41:08 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/YeB17},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{info2012,
    title={Information-Theoretic Foundations of Differential Privacy},
    author={Mir J. Darakhshan},
    booktitle={International Symposium on Foundations and Practice of Security},
    year={2012},
    organization={Springer}
  }	

@inproceedings{diff2017,
    title={Dynamic Differential Location Privacy with Personalized Error Bounds},
    author={Lei Yu and Ling Liu and Calton Pu},
    booktitle={The Network and Distributed System Security Symposium},
    year={2017}
  }	

@inproceedings{ciss2017,
    title={Fundamental Limits of Location Privacy using Anonymization},
    author={N. Takbiri and A. Houmansadr and D.L. Goeckel and H. Pishro-Nik},
    booktitle={Annual Conference on Information Science and Systems (CISS)},
    year={2017},
    organization={IEEE}
  }	

@inproceedings{sit2017,
    title={Limits of Location Privacy under Anonymization and Obfuscation},
    author={Nazanin Takbiri and Amir Houmansadr and Dennis L. Goeckel and Hossein Pishro-Nik},
    booktitle={International Symposium on Information Theory (ISIT)},
    year={2017},
    organization={IEEE}
  }	



@article{tifs2016,
	Author = {Z. Montazeri and A. Houmansadr and H. Pishro-Nik},
	Journal = {IEEE Transaction on Information Forensics and Security, to appear},
	Publisher = {IEEE},
	Title = {{Achieving Perfect Location Privacy in Wireless Devices Using Anonymization}},
	Year = {2017}}
	
	@article{matching,
  title={Asymptotically Optimal Matching of Multiple Sequences to Source Distributions and Training Sequences},
  author={Jayakrishnan Unnikrishnan},
  journal={IEEE Transactions on Information Theory},
  volume={61},
  number={1},
  pages={452-468},
  year={2015},
  publisher={IEEE}
}

@article{Naini2016,
	Author = {F. Naini and J. Unnikrishnan and P. Thiran and M. Vetterli},
	Journal = {IEEE Transactions on Information Forensics and Security},
	Publisher = {IEEE},
	Title = {Where You Are Is Who You Are: User Identification by Matching Statistics},
	 volume={11},
    number={2},
     pages={358--372},
    Year = {2016}
}



@inproceedings{montazeri2016defining,
    title={Defining perfect location privacy using anonymization},
    author={Montazeri, Zarrin and Houmansadr, Amir and Pishro-Nik, Hossein},
    booktitle={2016 Annual Conference on Information Science and Systems (CISS)},
    pages={204--209},
    year={2016},
    organization={IEEE}
  }	
	
	
@inproceedings{Mont1610Achieving,
  title={Achieving Perfect Location Privacy in Markov Models Using Anonymization},
  author={Montazeri, Zarrin and Houmansadr, Amir and H.Pishro-Nik},
  booktitle="2016 International Symposium on Information Theory and its Applications
  (ISITA2016)",
  address="Monterey, USA",
  days=30,
  month="oct",
  year=2016,
}

@misc{uber-stats,
title = {{By The Numbers 24 Amazing Uber Statistics}},
author = {Craig Smith},
note = {\url{http://expandedramblings.com/index.php/uber-statistics/}},
year=2015,
month= "September"
}


@misc{GMaps-users,
title = {{55\% of U.S. iOS users with Google Maps use it weekly}},
author = {Mike Dano},
note = {\url{http://www.fiercemobileit.com/story/55-us-ios-users-google-maps-use-it-weekly/2013-08-27}},
year=2013
}

@misc{Google-stats,
title = {{Statistics and facts about Google}},
note = {\url{http://www.statista.com/topics/1001/google/}},
}

@misc{yelp-stats,
title = {{By The Numbers: 45 Amazing Yelp Statistics}},
author = {Craig Smith},
note = {\url{http://expandedramblings.com/index.php/yelp-statistics/}},
year=2015,
month= "May"
}


@misc{Uber-hacker,
title = {{Is Uber's rider database a sitting duck for hackers?}},
author = {Craig Timberg},
note = {\url{https://www.washingtonpost.com/news/the-switch/wp/2014/12/01/is-ubers-rider-database-a-sitting-duck-for-hackers/}},
year=2014,
month= "December"
}

@misc{Uber-godview,
title = {{``God View'': Uber Investigates Its Top New York Executive For Privacy Violations}},
note = {\url{https://www.washingtonpost.com/news/the-switch/wp/2014/12/01/is-ubers-rider-database-a-sitting-duck-for-hackers/}},
year=2014,
month= "November"
}


@misc{Uber-breach-statement,
title = {{Uber Statement}},
note = {\url{http://newsroom.uber.com/2015/02/uber-statement/}},
year=2015,
month= "February"
}



@inproceedings{zhou2007privacy,
  title={Privacy-preserving detection of sybil attacks in vehicular ad hoc networks},
  author={Zhou, Tong and Choudhury, Romit Roy and Ning, Peng and Chakrabarty, Krishnendu},
  booktitle={Mobile and Ubiquitous Systems: Networking \& Services, 2007. MobiQuitous 2007. Fourth Annual International Conference on},
  pages={1--8},
  year={2007},
  organization={IEEE}
}

@article{chang2012footprint,
  title={Footprint: Detecting sybil attacks in urban vehicular networks},
  author={Chang, Shan and Qi, Yong and Zhu, Hongzi and Zhao, Jizhong and Shen, Xuemin Sherman},
  journal={Parallel and Distributed Systems, IEEE Transactions on},
  volume={23},
  number={6},
  pages={1103--1114},
  year={2012},
  publisher={IEEE}
}

@inproceedings{shokri2012protecting,
	Author = {Shokri, Reza and Theodorakopoulos, George and Troncoso, Carmela and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
	Booktitle = {Proceedings of the 2012 ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {617--627},
	Title = {Protecting location privacy: optimal strategy against localization attacks},
	Year = {2012}}


@inproceedings{gruteser2003anonymous,
	Author = {Gruteser, Marco and Grunwald, Dirk},
	Booktitle = {Proceedings of the 1st international conference on Mobile systems, applications and services},
	Organization = {ACM},
	Pages = {31--42},
	Title = {Anonymous usage of location-based services through spatial and temporal cloaking},
	Year = {2003}}



@inproceedings{hoh2007preserving,
	Author = {Hoh, Baik and Gruteser, Marco and Xiong, Hui and Alrabady, Ansaf},
	Booktitle = {Proceedings of the 14th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {161--171},
	Title = {Preserving privacy in gps traces via uncertainty-aware path cloaking},
	Year = {2007}}


@inproceedings{shokri2011quantifying,
	Author = {Shokri, Reza and Theodorakopoulos, George and Le Boudec, Jean-Yves and Hubaux, Jean-Pierre},
	Booktitle = {Security and Privacy (SP), 2011 IEEE Symposium on},
	Organization = {IEEE},
	Pages = {247--262},
	Title = {Quantifying location privacy},
	Year = {2011}}


@inproceedings{bordenabe2014optimal,
	Author = {Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2014 ACM SIGSAC Conference on Computer and Communications Security},
	Organization = {ACM},
	Pages = {251--262},
	Title = {Optimal geo-indistinguishable mechanisms for location privacy},
	Year = {2014}}




@inproceedings{freudiger2009non,
	Author = {Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
	Booktitle = {Proceedings of the 16th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {324--337},
	Title = {On non-cooperative location privacy: a game-theoretic analysis},
	Year = {2009}}

@inproceedings{ma2009location,
	Author = {Ma, Zhendong and Kargl, Frank and Weber, Michael},
	Booktitle = {Sarnoff Symposium, 2009. SARNOFF'09. IEEE},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {A location privacy metric for v2x communication systems},
	Year = {2009}}

@article{1corser2016evaluating,
  title={Evaluating Location Privacy in Vehicular Communications and Applications},
  author={Corser, George P and Fu, Huirong and Banihani, Abdelnasser},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={17},
  number={9},
  pages={2658-2667},
  year={2016},
  publisher={IEEE}
}
@article{2zhang2016designing,
  title={On Designing Satisfaction-Ratio-Aware Truthful Incentive Mechanisms for k-Anonymity Location Privacy},
  author={Zhang, Yuan and Tong, Wei and Zhong, Sheng},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={11},
  number={11},
  pages={2528--2541},
  year={2016},
  publisher={IEEE}
}

@article{11dewri2014exploiting,
  title={Exploiting service similarity for privacy in location-based search queries},
  author={Dewri, Rinku and Thurimella, Ramakrisha},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={25},
  number={2},
  pages={374--383},
  year={2014},
  publisher={IEEE}
}

@inproceedings{gedik2005location,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Booktitle = {Distributed Computing Systems, 2005. ICDCS 2005. Proceedings. 25th IEEE International Conference on},
	Organization = {IEEE},
	Pages = {620--629},
	Title = {Location privacy in mobile systems: A personalized anonymization model},
	Year = {2005}}

@inproceedings{zhong2009distributed,
	Author = {Zhong, Ge and Hengartner, Urs},
	Booktitle = {Pervasive Computing and Communications, 2009. PerCom 2009. IEEE International Conference on},
	Organization = {IEEE},
	Pages = {1--10},
	Title = {A distributed k-anonymity protocol for location privacy},
	Year = {2009}}

@inproceedings{mokbel2006new,
	Author = {Mokbel, Mohamed F and Chow, Chi-Yin and Aref, Walid G},
	Booktitle = {Proceedings of the 32nd international conference on Very large data bases},
	Organization = {VLDB Endowment},
	Pages = {763--774},
	Title = {The new Casper: query processing for location services without compromising privacy},
	Year = {2006}}

@article{kalnis2007preventing,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {12},
	Pages = {1719--1733},
	Publisher = {IEEE},
	Title = {Preventing location-based identity inference in anonymous spatial queries},
	Volume = {19},
	Year = {2007}}


@article{sweeney2002k,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {557--570},
	Publisher = {World Scientific},
	Title = {k-anonymity: A model for protecting privacy},
	Volume = {10},
	Year = {2002}}

@article{sweeney2002achieving,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {571-588},
	Publisher = {World Scientific},
	Title = {Achieving k-anonymity privacy protection using generalization and suppression},
	Volume = {10},
	Year = {2002}}

@inproceedings{liu2013game,
	Author = {Liu, Xinxin and Liu, Kaikai and Guo, Linke and Li, Xiaolin and Fang, Yuguang},
	Booktitle = {INFOCOM, 2013 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {2985--2993},
	Title = {A game-theoretic approach for achieving k-anonymity in location based services},
	Year = {2013}}

@inproceedings{hoh2005protecting,
	Author = {Hoh, Baik and Gruteser, Marco},
	Booktitle = {Security and Privacy for Emerging Areas in Communications Networks, 2005. SecureComm 2005. First International Conference on},
	Organization = {IEEE},
	Pages = {194--205},
	Title = {Protecting location privacy through path confusion},
	Year = {2005}}

@article{beresford2003location,
	Author = {Beresford, Alastair R and Stajano, Frank},
	Journal = {IEEE Pervasive computing},
	Number = {1},
	Pages = {46--55},
	Publisher = {IEEE},
	Title = {Location privacy in pervasive computing},
	Year = {2003}}


@inproceedings{palanisamy2011mobimix,
	Author = {Palanisamy, Balaji and Liu, Ling},
	Booktitle = {Data Engineering (ICDE), 2011 IEEE 27th International Conference on},
	Organization = {IEEE},
	Pages = {494--505},
	Title = {Mobimix: Protecting location privacy with mix-zones over road networks},
	Year = {2011}}
@inproceedings{freudiger2009optimal,
	Author = {Freudiger, Julien and Shokri, Reza and Hubaux, Jean-Pierre},
	Booktitle = {Privacy enhancing technologies},
	Organization = {Springer},
	Pages = {216--234},
	Title = {On the optimal placement of mix zones},
	Year = {2009}}

@article{manshaei2013game,
	Author = {Manshaei, Mohammad Hossein and Zhu, Quanyan and Alpcan, Tansu and Bac{\c{s}}ar, Tamer and Hubaux, Jean-Pierre},
	Journal = {ACM Computing Surveys (CSUR)},
	Number = {3},
	Pages = {25},
	Publisher = {ACM},
	Title = {Game theory meets network security and privacy},
	Volume = {45},
	Year = {2013}}

@article{19freudiger2013non,
  title={Non-cooperative location privacy},
  author={Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
  journal={IEEE Transactions on Dependable and Secure Computing},
  volume={10},
  number={2},
  pages={84--98},
  year={2013},
  publisher={IEEE}
}


@article{paulet2014privacy,
	Author = {Paulet, Russell and Kaosar, Md Golam and Yi, Xun and Bertino, Elisa},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {5},
	Pages = {1200--1210},
	Publisher = {IEEE},
	Title = {Privacy-preserving and content-protecting location based queries},
	Volume = {26},
	Year = {2014}}

@article{khoshgozaran2011location,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus and Shirani-Mehr, Houtan},
	Journal = {Knowledge and Information Systems},
	Number = {3},
	Pages = {435--465},
	Publisher = {Springer},
	Title = {Location privacy: going beyond K-anonymity, cloaking and anonymizers},
	Volume = {26},
	Year = {2011}}

@article{18shokri2014hiding,
  title={Hiding in the mobile crowd: Locationprivacy through collaboration},
  author={Shokri, Reza and Theodorakopoulos, George and Papadimitratos, Panos and Kazemi, Ehsan and Hubaux, Jean-Pierre},
  journal={IEEE transactions on dependable and secure computing},
  volume={11},
  number={3},
  pages={266--279},
  year={2014},
  publisher={IEEE}
}

@article{8zurbaran2015near,
  title={Near-Rand: Noise-based Location Obfuscation Based on Random Neighboring Points},
  author={Zurbaran, Mayra Alejandra and Avila, Karen and Wightman, Pedro and Fernandez, Michael},
  journal={IEEE Latin America Transactions},
  volume={13},
  number={11},
  pages={3661--3667},
  year={2015},
  publisher={IEEE}
}

@inproceedings{hoh2007preserving,
	Author = {Hoh, Baik and Gruteser, Marco and Xiong, Hui and Alrabady, Ansaf},
	Booktitle = {Proceedings of the 14th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {161--171},
	Title = {Preserving privacy in gps traces via uncertainty-aware path cloaking},
	Year = {2007}}

@inproceedings{ho2011differential,
	Author = {Ho, Shen-Shyang and Ruan, Shuhua},
	Booktitle = {Proceedings of the 4th ACM SIGSPATIAL International Workshop on Security and Privacy in GIS and LBS},
	Organization = {ACM},
	Pages = {17--24},
	Title = {Differential privacy for location pattern mining},
	Year = {2011}}


@article{12hwang2014novel,
  title={A novel time-obfuscated algorithm for trajectory privacy protection},
  author={Hwang, Ren-Hung and Hsueh, Yu-Ling and Chung, Hao-Wei},
  journal={IEEE Transactions on Services Computing},
  volume={7},
  number={2},
  pages={126--139},
  year={2014},
  publisher={IEEE}
  }

  @article{16haghnegahdar2014privacy,
  title={Privacy Risks in Publishing Mobile Device Trajectories},
  author={Haghnegahdar, Alireza and Khabbazian, Majid and Bhargava, Vijay K},
  journal={IEEE Wireless Communications Letters},
  volume={3},
  number={3},
  pages={241--244},
  year={2014},
  publisher={IEEE}
}

@article{20gao2013trpf,
  title={TrPF: A trajectory privacy-preserving framework for participatory sensing},
  author={Gao, Sheng and Ma, Jianfeng and Shi, Weisong and Zhan, Guoxing and Sun, Cong},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={8},
  number={6},
  pages={874--887},
  year={2013},
  publisher={IEEE}
}

@article{21ma2013privacy,
  title={Privacy vulnerability of published anonymous mobility traces},
  author={Ma, Chris YT and Yau, David KY and Yip, Nung Kwan and Rao, Nageswara SV},
  journal={IEEE/ACM Transactions on Networking},
  volume={21},
  number={3},
  pages={720--733},
  year={2013},
  publisher={IEEE}
}

@article{6li2016privacy,
  title={Privacy Leakage of Location Sharing in Mobile Social Networks: Attacks and Defense},
  author={Li, Huaxin and Zhu, Haojin and Du, Suguo and Liang, Xiaohui and Shen, Xuemin},
  journal={IEEE Transactions on Dependable and Secure Computing},
  year={2016},
  volume={PP},
  number={99},
  publisher={IEEE}
}


@article{14zhang2014privacy,
  title={Privacy quantification model based on the Bayes conditional risk in Location-Based Services},
  author={Zhang, Xuejun and Gui, Xiaolin and Tian, Feng and Yu, Si and An, Jian},
  journal={Tsinghua Science and Technology},
  volume={19},
  number={5},
  pages={452--462},
  year={2014},
  publisher={TUP}
}

@article{4olteanu2016quantifying,
  title={Quantifying Interdependent Privacy Risks with Location Data},
  author={Olteanu, Alexandra-Mihaela and Huguenin, K{\'e}vin and Shokri, Reza and Humbert, Mathias and Hubaux, Jean-Pierre},
  journal={IEEE Transactions on Mobile Computing},
  year={2016},
  volume={PP},
  number={99},
  pages={1-1},
  publisher={IEEE}
}















@misc{Leberknight2010,
	Author = {Leberknight, C. and Chiang, M. and Poor, H. and Wong, F.},
	Howpublished = {\url{http://www.princeton.edu/~chiangm/anticensorship.pdf}},
	Title = {{A Taxonomy of Internet Censorship and Anti-censorship}},
	Year = {2010}}

@techreport{ultrasurf-analysis,
	Author = {Appelbaum, Jacob},
	Institution = {The Tor Project},
	Title = {{Technical analysis of the Ultrasurf proxying software}},
	Url = {http://scholar.google.com/scholar?hl=en\&btnG=Search\&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software\#0},
	Year = {2012},
	Bdsk-Url-1 = {http://scholar.google.com/scholar?hl=en%5C&btnG=Search%5C&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software%5C#0}}

@misc{gifc:07,
	Howpublished = {\url{http://www.internetfreedom.org/archive/Defeat\_Internet\_Censorship\_White\_Paper.pdf}},
	Key = {defeatcensorship},
	Publisher = {Global Internet Freedom Consortium (GIFC)},
	Title = {{Defeat Internet Censorship: Overview of Advanced Technologies and Products}},
	Type = {White Paper},
	Year = {2007}}

@article{pan2011survey,
	Author = {Pan, J. and Paul, S. and Jain, R.},
	Journal = {Communications Magazine, IEEE},
	Number = {7},
	Pages = {26--36},
	Publisher = {IEEE},
	Title = {{A Survey of the Research on Future Internet Architectures}},
	Volume = {49},
	Year = {2011}}

@misc{nsf-fia,
	Howpublished = {\url{http://www.nets-fia.net/}},
	Key = {FIA},
	Title = {{NSF Future Internet Architecture Project}}}

@misc{NDN,
	Howpublished = {\url{http://www.named- data.net}},
	Key = {NDN},
	Title = {{Named Data Networking Project}}}

@inproceedings{MobilityFirst,
	Author = {Seskar, I. and Nagaraja, K. and Nelson, S. and Raychaudhuri, D.},
	Booktitle = {Asian Internet Engineering Conference},
	Title = {{Mobilityfirst Future internet Architecture Project}},
	Year = {2011}}

@incollection{NEBULA,
	Author = {Anderson, T. and Birman, K. and Broberg, R. and Caesar, M. and Comer, D. and Cotton, C. and Freedman, M.~J. and Haeberlen, A. and Ives, Z.~G. and Krishnamurthy, A. and others},
	Booktitle = {The Future Internet},
	Pages = {16--26},
	Publisher = {Springer},
	Title = {{The NEBULA Future Internet Architecture}},
	Year = {2013}}

@inproceedings{XIA,
	Author = {Anand, A. and Dogar, F. and Han, D. and Li, B. and Lim, H. and Machado, M. and Wu, W. and Akella, A. and Andersen, D.~G. and Byers, J.~W. and others},
	Booktitle = {ACM Workshop on Hot Topics in Networks},
	Pages = {2},
	Title = {{XIA: An Architecture for an Evolvable and Trustworthy Internet}},
	Year = {2011}}

@inproceedings{ChoiceNet,
	Author = {Rouskas, G.~N. and Baldine, I. and Calvert, K.~L. and Dutta, R. and Griffioen, J. and Nagurney, A. and Wolf, T.},
	Booktitle = {ONDM},
	Title = {{ChoiceNet: Network Innovation Through Choice}},
	Year = {2013}}

@misc{nsf-find,
	Howpublished = {http://www.nets-find.net/},
	Title = {{NSF NeTS FIND Initiative}}}

@article{traid,
	Author = {Cheriton, D.~R. and Gritter, M.},
	Title = {{TRIAD: A New Next-Generation Internet Architecture}},
	Year = {2000}}

@inproceedings{dona,
	Author = {Koponen, T. and Chawla, M. and Chun, B-G. and Ermolinskiy, A. and Kim, K.~H. and Shenker, S. and Stoica, I.},
	Booktitle = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Organization = {ACM},
	Pages = {181--192},
	Title = {{A Data-Oriented (and Beyond) Network Architecture}},
	Volume = {37},
	Year = {2007}}

@misc{ultrasurf,
	Howpublished = {\url{http://www.ultrareach.com}},
	Key = {ultrasurf},
	Title = {{Ultrasurf}}}

@misc{tor-bridge,
	Author = {Dingledine, R. and Mathewson, N.},
	Howpublished = {\url{https://svn.torproject.org/svn/projects/design-paper/blocking.html}},
	Title = {{Design of a Blocking-Resistant Anonymity System}}}

@inproceedings{McLachlanH09,
	Author = {J. McLachlan and N. Hopper},
	Booktitle = {WPES},
	Title = {{On the Risks of Serving Whenever You Surf: Vulnerabilities in Tor's Blocking Resistance Design}},
	Year = {2009}}

@inproceedings{mahdian2010,
	Author = {Mahdian, M.},
	Booktitle = {{Fun with Algorithms}},
	Title = {{Fighting Censorship with Algorithms}},
	Year = {2010}}

@inproceedings{McCoy2011,
	Author = {McCoy, D. and Morales, J.~A. and Levchenko, K.},
	Booktitle = {FC},
	Title = {{Proximax: A Measurement Based System for Proxies Dissemination}},
	Year = {2011}}

@inproceedings{Sovran2008,
	Author = {Sovran, Y. and Libonati, A. and Li, J.},
	Booktitle = {IPTPS},
	Title = {{Pass it on: Social Networks Stymie Censors}},
	Year = {2008}}

@inproceedings{rbridge,
	Author = {Wang, Q. and Lin, Zi and Borisov, N. and Hopper, N.},
	Booktitle = {{NDSS}},
	Title = {{rBridge: User Reputation based Tor Bridge Distribution with Privacy Preservation}},
	Year = {2013}}

@inproceedings{telex,
	Author = {Wustrow, E. and Wolchok, S. and Goldberg, I. and Halderman, J.},
	Booktitle = {{USENIX Security}},
	Title = {{Telex: Anticensorship in the Network Infrastructure}},
	Year = {2011}}

@inproceedings{cirripede,
	Author = {Houmansadr, A. and Nguyen, G. and Caesar, M. and Borisov, N.},
	Booktitle = {CCS},
	Title = {{Cirripede: Circumvention Infrastructure Using Router Redirection with Plausible Deniability}},
	Year = {2011}}

@inproceedings{decoyrouting,
	Author = {Karlin, J. and Ellard, D. and Jackson, A. and Jones, C. and Lauer, G. and Mankins, D. and Strayer, W.},
	Booktitle = {{FOCI}},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = {2011}}

@inproceedings{routing-around-decoys,
	Author = {M.~Schuchard and J.~Geddes and C.~Thompson and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Routing Around Decoys}},
	Year = {2012}}

@inproceedings{parrot,
	Author = {A. Houmansadr and C. Brubaker and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{The Parrot is Dead: Observing Unobservable Network Communications}},
	Year = {2013}}

@misc{knock,
	Author = {T. Wilde},
	Howpublished = {\url{https://blog.torproject.org/blog/knock-knock-knockin-bridges-doors}},
	Title = {{Knock Knock Knockin' on Bridges' Doors}},
	Year = {2012}}

@inproceedings{china-tor,
	Author = {Winter, P. and Lindskog, S.},
	Booktitle = {{FOCI}},
	Title = {{How the Great Firewall of China Is Blocking Tor}},
	Year = {2012}}

@misc{discover-bridge,
	Howpublished = {\url{https://blog.torproject.org/blog/research-problems-ten-ways-discover-tor-bridges}},
	Key = {tenways},
	Title = {{Ten Ways to Discover Tor Bridges}}}

@inproceedings{freewave,
	Author = {A.~Houmansadr and T.~Riedl and N.~Borisov and A.~Singer},
	Booktitle = {{NDSS}},
	Title = {{I Want My Voice to Be Heard: IP over Voice-over-IP for Unobservable Censorship Circumvention}},
	Year = 2013}

@inproceedings{censorspoofer,
	Author = {Q. Wang and X. Gong and G. Nguyen and A. Houmansadr and N. Borisov},
	Booktitle = {CCS},
	Title = {{CensorSpoofer: Asymmetric Communication Using IP Spoofing for Censorship-Resistant Web Browsing}},
	Year = {2012}}

@inproceedings{skypemorph,
	Author = {H. Moghaddam and B. Li and M. Derakhshani and I. Goldberg},
	Booktitle = {CCS},
	Title = {{SkypeMorph: Protocol Obfuscation for Tor Bridges}},
	Year = {2012}}

@inproceedings{stegotorus,
	Author = {Weinberg, Z. and Wang, J. and Yegneswaran, V. and Briesemeister, L. and Cheung, S. and Wang, F. and Boneh, D.},
	Booktitle = {CCS},
	Title = {{StegoTorus: A Camouflage Proxy for the Tor Anonymity System}},
	Year = {2012}}

@techreport{dust,
	Author = {{B.~Wiley}},
	Howpublished = {\url{http://blanu.net/ Dust.pdf}},
	Institution = {School of Information, University of Texas at Austin},
	Title = {{Dust: A Blocking-Resistant Internet Transport Protocol}},
	Year = {2011}}

@inproceedings{FTE,
	Author = {K.~Dyer and S.~Coull and T.~Ristenpart and T.~Shrimpton},
	Booktitle = {CCS},
	Title = {{Protocol Misidentification Made Easy with Format-Transforming Encryption}},
	Year = {2013}}

@inproceedings{fp,
	Author = {Fifield, D. and Hardison, N. and Ellithrope, J. and Stark, E. and Dingledine, R. and Boneh, D. and Porras, P.},
	Booktitle = {PETS},
	Title = {{Evading Censorship with Browser-Based Proxies}},
	Year = {2012}}

@misc{obfsproxy,
	Howpublished = {\url{https://www.torproject.org/projects/obfsproxy.html.en}},
	Key = {obfsproxy},
	Publisher = {The Tor Project},
	Title = {{A Simple Obfuscating Proxy}}}

@inproceedings{Tor-instead-of-IP,
	Author = {Liu, V. and Han, S. and Krishnamurthy, A. and Anderson, T.},
	Booktitle = {HotNets},
	Title = {{Tor instead of IP}},
	Year = {2011}}

@misc{roger-slides,
	Howpublished = {\url{https://svn.torproject.org/svn/projects/presentations/slides-28c3.pdf}},
	Key = {torblocking},
	Title = {{How Governments Have Tried to Block Tor}}}

@inproceedings{infranet,
	Author = {Feamster, N. and Balazinska, M. and Harfst, G. and Balakrishnan, H. and Karger, D.},
	Booktitle = {USENIX Security},
	Title = {{Infranet: Circumventing Web Censorship and Surveillance}},
	Year = {2002}}

@inproceedings{collage,
	Author = {S.~Burnett and N.~Feamster and S.~Vempala},
	Booktitle = {USENIX Security},
	Title = {{Chipping Away at Censorship Firewalls with User-Generated Content}},
	Year = {2010}}

@article{anonymizer,
	Author = {Boyan, J.},
	Journal = {Computer-Mediated Communication Magazine},
	Month = sep,
	Number = {9},
	Title = {{The Anonymizer: Protecting User Privacy on the Web}},
	Volume = {4},
	Year = {1997}}

@article{schulze2009internet,
	Author = {Schulze, H. and Mochalski, K.},
	Journal = {IPOQUE Report},
	Pages = {351--362},
	Title = {Internet Study 2008/2009},
	Volume = {37},
	Year = {2009}}

@inproceedings{cya-ccs13,
	Author = {J.~Geddes and M.~Schuchard and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Cover Your ACKs: Pitfalls of Covert Channel Censorship Circumvention}},
	Year = {2013}}

@inproceedings{andana,
	Author = {DiBenedetto, S. and Gasti, P. and Tsudik, G. and Uzun, E.},
	Booktitle = {{NDSS}},
	Title = {{ANDaNA: Anonymous Named Data Networking Application}},
	Year = {2012}}

@inproceedings{darkly,
	Author = {Jana, S. and Narayanan, A. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{A Scanner Darkly: Protecting User Privacy From Perceptual Applications}},
	Year = {2013}}

@inproceedings{NS08,
	Author = {A.~Narayanan and V.~Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {Robust de-anonymization of large sparse datasets},
	Year = {2008}}

@inproceedings{NS09,
	Author = {A.~Narayanan and V.~Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {De-anonymizing social networks},
	Year = {2009}}

@inproceedings{memento,
	Author = {Jana, S. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{Memento: Learning secrets from process footprints}},
	Year = {2012}}

@misc{plugtor,
	Howpublished = {\url{https://www.torproject.org/docs/pluggable-transports.html.en}},
	Key = {PluggableTransports},
	Publisher = {The Tor Project},
	Title = {{Tor: Pluggable transports}}}

@misc{psiphon,
	Author = {J.~Jia and P.~Smith},
	Howpublished = {\url{http://www.cdf.toronto.edu/~csc494h/reports/2004-fall/psiphon_ae.html}},
	Title = {{Psiphon: Analysis and Estimation}},
	Year = 2004}

@misc{china-github,
	Howpublished = {\url{http://mobile.informationweek.com/80269/show/72e30386728f45f56b343ddfd0fdb119/}},
	Key = {github},
	Title = {{China's GitHub Censorship Dilemma}}}

@inproceedings{txbox,
	Author = {Jana, S. and Porter, D. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{TxBox: Building Secure, Efficient Sandboxes with System Transactions}},
	Year = {2011}}

@inproceedings{airavat,
	Author = {I. Roy and S. Setty and A. Kilzer and V. Shmatikov and E. Witchel},
	Booktitle = {NSDI},
	Title = {{Airavat: Security and Privacy for MapReduce}},
	Year = {2010}}

@inproceedings{osdi12,
	Author = {A. Dunn and M. Lee and S. Jana and S. Kim and M. Silberstein and Y. Xu and V. Shmatikov and E. Witchel},
	Booktitle = {OSDI},
	Title = {{Eternal Sunshine of the Spotless Machine: Protecting Privacy with Ephemeral Channels}},
	Year = {2012}}

@inproceedings{ymal,
	Author = {J. Calandrino and A. Kilzer and A. Narayanan and E. Felten and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{``You Might Also Like:'' Privacy Risks of Collaborative Filtering}},
	Year = {2011}}

@inproceedings{srivastava11,
	Author = {V. Srivastava and M. Bond and K. McKinley and V. Shmatikov},
	Booktitle = {PLDI},
	Title = {{A Security Policy Oracle: Detecting Security Holes Using Multiple API Implementations}},
	Year = {2011}}

@inproceedings{chen-oakland10,
	Author = {Chen, S. and Wang, R. and Wang, X. and Zhang, K.},
	Booktitle = {IEEE S\&P},
	Title = {{Side-Channel Leaks in Web Applications: A Reality Today, a Challenge Tomorrow}},
	Year = {2010}}

@book{kerck,
	Author = {Kerckhoffs, A.},
	Publisher = {University Microfilms},
	Title = {{La cryptographie militaire}},
	Year = {1978}}

@inproceedings{foci11,
	Author = {J. Karlin and D. Ellard and A.~Jackson and C.~ Jones and G. Lauer and D. Mankins and W.~T.~Strayer},
	Booktitle = {FOCI},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = 2011}

@inproceedings{sun02,
	Author = {Sun, Q. and Simon, D.~R. and Wang, Y. and Russell, W. and Padmanabhan, V. and Qiu, L.},
	Booktitle = {IEEE S\&P},
	Title = {{Statistical Identification of Encrypted Web Browsing Traffic}},
	Year = {2002}}

@inproceedings{danezis,
	Author = {Murdoch, S.~J. and Danezis, G.},
	Booktitle = {IEEE S\&P},
	Title = {{Low-Cost Traffic Analysis of Tor}},
	Year = {2005}}

@inproceedings{pakicensorship,
	Author = {Z.~Nabi},
	Booktitle = {FOCI},
	Title = {The Anatomy of {Web} Censorship in {Pakistan}},
	Year = {2013}}

@inproceedings{irancensorship,
	Author = {S.~Aryan and H.~Aryan and A.~Halderman},
	Booktitle = {FOCI},
	Title = {Internet Censorship in {Iran}: {A} First Look},
	Year = {2013}}

@inproceedings{ford10efficient,
	Author = {Amittai Aviram and Shu-Chun Weng and Sen Hu and Bryan Ford},
	Booktitle = {\bibconf[9th]{OSDI}{USENIX Symposium on Operating Systems Design and Implementation}},
	Location = {Vancouver, BC, Canada},
	Month = oct,
	Title = {Efficient System-Enforced Deterministic Parallelism},
	Year = 2010}

@inproceedings{ford10determinating,
	Author = {Amittai Aviram and Sen Hu and Bryan Ford and Ramakrishna Gummadi},
	Booktitle = {\bibconf{CCSW}{ACM Cloud Computing Security Workshop}},
	Location = {Chicago, IL},
	Month = oct,
	Title = {Determinating Timing Channels in Compute Clouds},
	Year = 2010}

@inproceedings{ford12plugging,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Plugging Side-Channel Leaks with Timing Information Flow Control},
	Year = 2012}

@inproceedings{ford12icebergs,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Icebergs in the Clouds: the {\em Other} Risks of Cloud Computing},
	Year = 2012}

@misc{mullenize,
	Author = {Washington Post},
	Howpublished = {\url{http://apps.washingtonpost.com/g/page/world/gchq-report-on-mullenize-program-to-stain-anonymous-electronic-traffic/502/}},
	Month = {oct},
	Title = {{GCHQ} report on {`MULLENIZE'} program to `stain' anonymous electronic traffic},
	Year = {2013}}

@inproceedings{shue13street,
	Author = {Craig A. Shue and Nathanael Paul and Curtis R. Taylor},
	Booktitle = {\bibbrev[7th]{WOOT}{USENIX Workshop on Offensive Technologies}},
	Month = aug,
	Title = {From an {IP} Address to a Street Address: Using Wireless Signals to Locate a Target},
	Year = 2013}

@inproceedings{knockel11three,
	Author = {Jeffrey Knockel and Jedidiah R. Crandall and Jared Saia},
	Booktitle = {\bibbrev{FOCI}{USENIX Workshop on Free and Open Communications on the Internet}},
	Location = {San Francisco, CA},
	Month = aug,
	Year = 2011}

@misc{rfc4960,
	Author = {R. {Stewart, ed.}},
	Month = sep,
	Note = {RFC 4960},
	Title = {Stream Control Transmission Protocol},
	Year = 2007}

@inproceedings{ford07structured,
	Author = {Bryan Ford},
	Booktitle = {\bibbrev{SIGCOMM}{ACM SIGCOMM}},
	Location = {Kyoto, Japan},
	Month = aug,
	Title = {Structured Streams: a New Transport Abstraction},
	Year = {2007}}

@misc{spdy,
	Author = {Google, Inc.},
	Note = {\url{http://www.chromium.org/spdy/spdy-whitepaper}},
	Title = {{SPDY}: An Experimental Protocol For a Faster {Web}}}

@misc{quic,
	Author = {Jim Roskind},
	Month = jun,
	Note = {\url{http://blog.chromium.org/2013/06/experimenting-with-quic.html}},
	Title = {Experimenting with {QUIC}},
	Year = 2013}

@misc{podjarny12not,
	Author = {G.~Podjarny},
	Month = jun,
	Note = {\url{http://www.guypo.com/technical/not-as-spdy-as-you-thought/}},
	Title = {{Not as SPDY as You Thought}},
	Year = 2012}

@inproceedings{cor,
	Author = {Jones, N.~A. and Arye, M. and Cesareo, J. and Freedman, M.~J.},
	Booktitle = {FOCI},
	Title = {{Hiding Amongst the Clouds: A Proposal for Cloud-based Onion Routing}},
	Year = {2011}}

@misc{torcloud,
	Howpublished = {\url{https://cloud.torproject.org/}},
	Key = {tor cloud},
	Title = {{The Tor Cloud Project}}}

@inproceedings{scramblesuit,
	Author = {Philipp Winter and Tobias Pulls and Juergen Fuss},
	Booktitle = {WPES},
	Title = {{ScrambleSuit: A Polymorphic Network Protocol to Circumvent Censorship}},
	Year = 2013}

@article{savage2000practical,
	Author = {Savage, S. and Wetherall, D. and Karlin, A. and Anderson, T.},
	Journal = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Pages = {295--306},
	Publisher = {ACM},
	Title = {Practical network support for IP traceback},
	Volume = {30},
	Year = {2000}}

@inproceedings{ooni,
	Author = {Filast, A. and Appelbaum, J.},
	Booktitle = {{FOCI}},
	Title = {{OONI : Open Observatory of Network Interference}},
	Year = {2012}}

@misc{caida-rank,
	Howpublished = {\url{http://as-rank.caida.org/}},
	Key = {caida rank},
	Title = {{AS Rank: AS Ranking}}}

@inproceedings{usersrouted-ccs13,
	Author = {A.~Johnson and C.~Wacek and R.~Jansen and M.~Sherr and P.~Syverson},
	Booktitle = {CCS},
	Title = {{Users Get Routed: Traffic Correlation on Tor by Realistic Adversaries}},
	Year = {2013}}

@inproceedings{edman2009awareness,
	Author = {Edman, M. and Syverson, P.},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2009}}

@inproceedings{DecoyCosts,
	Author = {A.~Houmansadr and E.~L.~Wong and V.~Shmatikov},
	Booktitle = {NDSS},
	Title = {{No Direction Home: The True Cost of Routing Around Decoys}},
	Year = {2014}}

@article{cordon,
	Author = {Elahi, T. and Goldberg, I.},
	Journal = {University of Waterloo CACR},
	Title = {{CORDON--A Taxonomy of Internet Censorship Resistance Strategies}},
	Volume = {33},
	Year = {2012}}

@inproceedings{privex,
	Author = {T.~Elahi and G.~Danezis and I.~Goldberg	},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2014}}

@inproceedings{changeGuards,
	Author = {T.~Elahi and K.~Bauer and M.~AlSabah and R.~Dingledine and I.~Goldberg},
	Booktitle = {{WPES}},
	Title = {{ Changing of the Guards: Framework for Understanding and Improving Entry Guard Selection in Tor}},
	Year = {2012}}

@article{RAINBOW:Journal,
	Author = {A.~Houmansadr and N.~Kiyavash and N.~Borisov},
	Journal = {IEEE/ACM Transactions on Networking},
	Title = {{Non-Blind Watermarking of Network Flows}},
	Year = 2014}

@inproceedings{info-tod,
	Author = {A.~Houmansadr and S.~Gorantla and T.~Coleman and N.~Kiyavash and and N.~Borisov},
	Booktitle = {{CCS (poster session)}},
	Title = {{On the Channel Capacity of Network Flow Watermarking}},
	Year = {2009}}

@inproceedings{johnson2014game,
	Author = {Johnson, B. and Laszka, A. and Grossklags, J. and Vasek, M. and Moore, T.},
	Booktitle = {Workshop on Bitcoin Research},
	Title = {{Game-theoretic Analysis of DDoS Attacks Against Bitcoin Mining Pools}},
	Year = {2014}}

@incollection{laszka2013mitigation,
	Author = {Laszka, A. and Johnson, B. and Grossklags, J.},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {175--191},
	Publisher = {Springer},
	Title = {{Mitigation of Targeted and Non-targeted Covert Attacks as a Timing Game}},
	Year = {2013}}

@inproceedings{schottle2013game,
	Author = {Schottle, P. and Laszka, A. and Johnson, B. and Grossklags, J. and Bohme, R.},
	Booktitle = {EUSIPCO},
	Title = {{A Game-theoretic Analysis of Content-adaptive Steganography with Independent Embedding}},
	Year = {2013}}

@inproceedings{CloudTransport,
	Author = {C.~Brubaker and A.~Houmansadr and V.~Shmatikov},
	Booktitle = {PETS},
	Title = {{CloudTransport: Using Cloud Storage for Censorship-Resistant Networking}},
	Year = {2014}}

@inproceedings{sweet,
	Author = {W.~Zhou and A.~Houmansadr and M.~Caesar and N.~Borisov},
	Booktitle = {HotPETs},
	Title = {{SWEET: Serving the Web by Exploiting Email Tunnels}},
	Year = {2013}}

@inproceedings{ahsan2002practical,
	Author = {Ahsan, K. and Kundur, D.},
	Booktitle = {Workshop on Multimedia Security},
	Title = {{Practical data hiding in TCP/IP}},
	Year = {2002}}

@incollection{danezis2011covert,
	Author = {Danezis, G.},
	Booktitle = {Security Protocols XVI},
	Pages = {198--214},
	Publisher = {Springer},
	Title = {{Covert Communications Despite Traffic Data Retention}},
	Year = {2011}}

@inproceedings{liu2009hide,
	Author = {Liu, Y. and Ghosal, D. and Armknecht, F. and Sadeghi, A.-R. and Schulz, S. and Katzenbeisser, S.},
	Booktitle = {ESORICS},
	Title = {{Hide and Seek in Time---Robust Covert Timing Channels}},
	Year = {2009}}

@misc{image-watermark-fing,
	Author = {Jonathan Bailey},
	Howpublished = {\url{https://www.plagiarismtoday.com/2009/12/02/image-detection-watermarking-vs-fingerprinting/}},
	Title = {{Image Detection: Watermarking vs. Fingerprinting}},
	Year = {2009}}

@inproceedings{Servetto98,
	Author = {S. D. Servetto and C. I. Podilchuk and K. Ramchandran},
	Booktitle = {Int. Conf. Image Processing},
	Title = {Capacity issues in digital image watermarking},
	Year = {1998}}

@inproceedings{Chen01,
	Author = {B. Chen and G.W.Wornell},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1423--1443},
	Title = {Quantization index modulation: A class of provably good methods for digital watermarking and information embedding},
	Year = {2001}}

@inproceedings{Karakos00,
	Author = {D. Karakos and A. Papamarcou},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {47},
	Title = {Relationship between quantization and distribution rates of digitally watermarked data},
	Year = {2000}}

@inproceedings{Sullivan98,
	Author = {J. A. OSullivan and P. Moulin and J. M. Ettinger},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {297},
	Title = {Information theoretic analysis of steganography},
	Year = {1998}}

@inproceedings{Merhav00,
	Author = {N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {420--430},
	Title = {On random coding error exponents of watermarking systems},
	Year = {2000}}

@inproceedings{Somekh01,
	Author = {A. Somekh-Baruch and N. Merhav},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {7},
	Title = {On the error exponent and capacity games of private watermarking systems},
	Year = {2001}}

@inproceedings{Steinberg01,
	Author = {Y. Steinberg and N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1410--1422},
	Title = {Identification in the presence of side information with application to watermarking},
	Year = {2001}}

@article{Moulin03,
	Author = {P. Moulin and J.A. O'Sullivan},
	Journal = {IEEE Trans. Info. Theory},
	Number = {3},
	Title = {Information-theoretic analysis of information hiding},
	Volume = 49,
	Year = 2003}

@article{Gelfand80,
	Author = {S.I.~Gelfand and M.S.~Pinsker},
	Journal = {Problems of Control and Information Theory},
	Number = {1},
	Pages = {19-31},
	Title = {{Coding for channel with random parameters}},
	Url = {citeseer.ist.psu.edu/anantharam96bits.html},
	Volume = {9},
	Year = {1980},
	Bdsk-Url-1 = {citeseer.ist.psu.edu/anantharam96bits.html}}

@book{Wolfowitz78,
	Author = {J. Wolfowitz},
	Edition = {3rd},
	Location = {New York},
	Publisher = {Springer-Verlag},
	Title = {Coding Theorems of Information Theory},
	Year = 1978}

@article{caire99,
	Author = {G. Caire and S. Shamai},
	Journal = {IEEE Transactions on Information Theory},
	Number = {6},
	Pages = {2007--2019},
	Title = {On the Capacity of Some Channels with Channel State Information},
	Volume = {45},
	Year = {1999}}

@inproceedings{wright2007language,
	Author = {Wright, Charles V and Ballard, Lucas and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {USENIX Security},
	Title = {{Language identification of encrypted VoIP traffic: Alejandra y Roberto or Alice and Bob?}},
	Year = {2007}}

@inproceedings{backes2010speaker,
	Author = {Backes, Michael and Doychev, Goran and D{\"u}rmuth, Markus and K{\"o}pf, Boris},
	Booktitle = {{European Symposium on Research in Computer Security (ESORICS)}},
	Pages = {508--523},
	Publisher = {Springer},
	Title = {{Speaker Recognition in Encrypted Voice Streams}},
	Year = {2010}}

@phdthesis{lu2009traffic,
	Author = {Lu, Yuanchao},
	School = {Cleveland State University},
	Title = {{On Traffic Analysis Attacks to Encrypted VoIP Calls}},
	Year = {2009}}

@inproceedings{wright2008spot,
	Author = {Wright, Charles V and Ballard, Lucas and Coull, Scott E and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {35--49},
	Title = {Spot me if you can: Uncovering spoken phrases in encrypted VoIP conversations},
	Year = {2008}}

@inproceedings{white2011phonotactic,
	Author = {White, Andrew M and Matthews, Austin R and Snow, Kevin Z and Monrose, Fabian},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {3--18},
	Title = {Phonotactic reconstruction of encrypted VoIP conversations: Hookt on fon-iks},
	Year = {2011}}

@inproceedings{fancy,
	Author = {Houmansadr, Amir and Borisov, Nikita},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {205--224},
	Title = {The Need for Flow Fingerprints to Link Correlated Network Flows},
	Year = {2013}}

@article{botmosaic,
	Author = {Amir Houmansadr and Nikita Borisov},
	Doi = {10.1016/j.jss.2012.11.005},
	Issn = {0164-1212},
	Journal = {Journal of Systems and Software},
	Keywords = {Network security},
	Number = {3},
	Pages = {707 - 715},
	Title = {BotMosaic: Collaborative network watermark for the detection of IRC-based botnets},
	Url = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Volume = {86},
	Year = {2013},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.jss.2012.11.005}}

@inproceedings{ramsbrock2008first,
	Author = {Ramsbrock, Daniel and Wang, Xinyuan and Jiang, Xuxian},
	Booktitle = {Recent Advances in Intrusion Detection},
	Organization = {Springer},
	Pages = {59--77},
	Title = {A first step towards live botmaster traceback},
	Year = {2008}}

@inproceedings{potdar2005survey,
	Author = {Potdar, Vidyasagar M and Han, Song and Chang, Elizabeth},
	Booktitle = {Industrial Informatics, 2005. INDIN'05. 2005 3rd IEEE International Conference on},
	Organization = {IEEE},
	Pages = {709--716},
	Title = {A survey of digital image watermarking techniques},
	Year = {2005}}

@book{cole2003hiding,
	Author = {Cole, Eric and Krutz, Ronald D},
	Publisher = {John Wiley \& Sons, Inc.},
	Title = {Hiding in plain sight: Steganography and the art of covert communication},
	Year = {2003}}

@incollection{akaike1998information,
	Author = {Akaike, Hirotogu},
	Booktitle = {Selected Papers of Hirotugu Akaike},
	Pages = {199--213},
	Publisher = {Springer},
	Title = {Information theory and an extension of the maximum likelihood principle},
	Year = {1998}}

@misc{central-command-hack,
	Author = {Everett Rosenfeld},
	Howpublished = {\url{http://www.cnbc.com/id/102330338}},
	Title = {{FBI investigating Central Command Twitter hack}},
	Year = {2015}}

@misc{sony-psp-ddos,
	Howpublished = {\url{http://n4g.com/news/1644853/sony-and-microsoft-cant-do-much-ddos-attacks-explained}},
	Key = {sony},
	Month = {December},
	Title = {{Sony and Microsoft cant do much -- DDoS attacks explained}},
	Year = {2014}}

@misc{sony-hack,
	Author = {David Bloom},
	Howpublished = {\url{http://goo.gl/MwR4A7}},
	Title = {{Online Game Networks Hacked, Sony Unit President Threatened}},
	Year = {2014}}

@misc{home-depot,
	Author = {Dune Lawrence},
	Howpublished = {\url{http://www.businessweek.com/articles/2014-09-02/home-depots-credit-card-breach-looks-just-like-the-target-hack}},
	Title = {{Home Depot's Suspected Breach Looks Just Like the Target Hack}},
	Year = {2014}}

@misc{target,
	Author = {Julio Ojeda-Zapata},
	Howpublished = {\url{http://www.mercurynews.com/business/ci_24765398/how-did-hackers-pull-off-target-data-heist}},
	Title = {{Target hack: How did they do it?}},
	Year = {2014}}


@article{probabilitycourse,
	Author = {H. Pishro-Nik},
	note = {\url{http://www.probabilitycourse.com}},
	Title = {Introduction to probability, statistics, and random processes},
    Year = {2014}}

@article{our-isit-location,
	Author = {Z. Montazeri and A. Houmansadr and H. Pishro-Nik},
	Journal = {To be submitted to IEEE ISIT},
	Title = {Location Privacy for Multi-State Networks},
	Year = {2016}}






@article{kafsi2013entropy,
	Author = {Kafsi, Mohamed and Grossglauser, Matthias and Thiran, Patrick},
	Journal = {Information Theory, IEEE Transactions on},
	Number = {9},
	Pages = {5577--5583},
	Publisher = {IEEE},
	Title = {The entropy of conditional Markov trajectories},
	Volume = {59},
	Year = {2013}}

@inproceedings{gruteser2003anonymous,
	Author = {Gruteser, Marco and Grunwald, Dirk},
	Booktitle = {Proceedings of the 1st international conference on Mobile systems, applications and services},
	Organization = {ACM},
	Pages = {31--42},
	Title = {Anonymous usage of location-based services through spatial and temporal cloaking},
	Year = {2003}}

@inproceedings{husted2010mobile,
	Author = {Husted, Nathaniel and Myers, Steven},
	Booktitle = {Proceedings of the 17th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {85--96},
	Title = {Mobile location tracking in metro areas: malnets and others},
	Year = {2010}}

@inproceedings{li2009tradeoff,
	Author = {Li, Tiancheng and Li, Ninghui},
	Booktitle = {Proceedings of the 15th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {517--526},
	Title = {On the tradeoff between privacy and utility in data publishing},
	Year = {2009}}





@incollection{humbert2010tracking,
	Author = {Humbert, Mathias and Manshaei, Mohammad Hossein and Freudiger, Julien and Hubaux, Jean-Pierre},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {38--57},
	Publisher = {Springer},
	Title = {Tracking games in mobile networks},
	Year = {2010}}


@article{palamidessi2006probabilistic,
	Author = {Palamidessi, Catuscia},
	Journal = {Electronic Notes in Theoretical Computer Science},
	Pages = {33--42},
	Publisher = {Elsevier},
	Title = {Probabilistic and nondeterministic aspects of anonymity},
	Volume = {155},
	Year = {2006}}



@inproceedings{freudiger2007mix,
	Author = {Freudiger, Julien and Raya, Maxim and F{\'e}legyh{\'a}zi, M{\'a}rk and Papadimitratos, Panos and Hubaux, Jean-Pierre},
	Booktitle = {CM Workshop on Wireless Networking for Intelligent Transportation Systems (WiN-ITS)},
	Title = {Mix-zones for location privacy in vehicular networks},
	Year = {2007}}



@inproceedings{niu2014achieving,
	Author = {Niu, Ben and Li, Qinghua and Zhu, Xiaoyan and Cao, Guohong and Li, Hui},
	Booktitle = {INFOCOM, 2014 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {754--762},
	Title = {Achieving k-anonymity in privacy-aware location-based services},
	Year = {2014}}



@inproceedings{kido2005protection,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Data Engineering Workshops, 2005. 21st International Conference on},
	Organization = {IEEE},
	Pages = {1248--1248},
	Title = {Protection of location privacy using dummies for location-based services},
	Year = {2005}}

@inproceedings{gedik2005location,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Booktitle = {Distributed Computing Systems, 2005. ICDCS 2005. Proceedings. 25th IEEE International Conference on},
	Organization = {IEEE},
	Pages = {620--629},
	Title = {Location privacy in mobile systems: A personalized anonymization model},
	Year = {2005}}


@incollection{duckham2005formal,
	Author = {Duckham, Matt and Kulik, Lars},
	Booktitle = {Pervasive computing},
	Pages = {152--170},
	Publisher = {Springer},
	Title = {A formal model of obfuscation and negotiation for location privacy},
	Year = {2005}}

@inproceedings{kido2005anonymous,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Pervasive Services, 2005. ICPS'05. Proceedings. International Conference on},
	Organization = {IEEE},
	Pages = {88--97},
	Title = {An anonymous communication technique using dummies for location-based services},
	Year = {2005}}

@incollection{duckham2006spatiotemporal,
	Author = {Duckham, Matt and Kulik, Lars and Birtley, Athol},
	Booktitle = {Geographic Information Science},
	Pages = {47--64},
	Publisher = {Springer},
	Title = {A spatiotemporal model of strategies and counter strategies for location privacy protection},
	Year = {2006}}

@inproceedings{shankar2009privately,
	Author = {Shankar, Pravin and Ganapathy, Vinod and Iftode, Liviu},
	Booktitle = {Proceedings of the 11th international conference on Ubiquitous computing},
	Organization = {ACM},
	Pages = {31--40},
	Title = {Privately querying location-based services with SybilQuery},
	Year = {2009}}

@inproceedings{chow2009faking,
	Author = {Chow, Richard and Golle, Philippe},
	Booktitle = {Proceedings of the 8th ACM workshop on Privacy in the electronic society},
	Organization = {ACM},
	Pages = {105--108},
	Title = {Faking contextual data for fun, profit, and privacy},
	Year = {2009}}

@incollection{xue2009location,
	Author = {Xue, Mingqiang and Kalnis, Panos and Pung, Hung Keng},
	Booktitle = {Location and Context Awareness},
	Pages = {70--87},
	Publisher = {Springer},
	Title = {Location diversity: Enhanced privacy protection in location based services},
	Year = {2009}}

@article{wernke2014classification,
	Author = {Wernke, Marius and Skvortsov, Pavel and D{\"u}rr, Frank and Rothermel, Kurt},
	Journal = {Personal and Ubiquitous Computing},
	Number = {1},
	Pages = {163--175},
	Publisher = {Springer-Verlag},
	Title = {A classification of location privacy attacks and approaches},
	Volume = {18},
	Year = {2014}}

@misc{cai2015cloaking,
	Author = {Cai, Y. and Xu, G.},
	Month = jan # {~1},
	Note = {US Patent App. 14/472,462},
	Publisher = {Google Patents},
	Title = {Cloaking with footprints to provide location privacy protection in location-based services},
	Url = {https://www.google.com/patents/US20150007341},
	Year = {2015},
	Bdsk-Url-1 = {https://www.google.com/patents/US20150007341}}

@article{gedik2008protecting,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {1},
	Pages = {1--18},
	Publisher = {IEEE},
	Title = {Protecting location privacy with personalized k-anonymity: Architecture and algorithms},
	Volume = {7},
	Year = {2008}}

@article{kalnis2006preserving,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Publisher = {TRB6/06},
	Title = {Preserving anonymity in location based services},
	Year = {2006}}



@article{terrovitis2011privacy,
	Author = {Terrovitis, Manolis},
	Journal = {ACM SIGKDD Explorations Newsletter},
	Number = {1},
	Pages = {6--18},
	Publisher = {ACM},
	Title = {Privacy preservation in the dissemination of location data},
	Volume = {13},
	Year = {2011}}

@article{shin2012privacy,
	Author = {Shin, Kang G and Ju, Xiaoen and Chen, Zhigang and Hu, Xin},
	Journal = {Wireless Communications, IEEE},
	Number = {1},
	Pages = {30--39},
	Publisher = {IEEE},
	Title = {Privacy protection for users of location-based services},
	Volume = {19},
	Year = {2012}}



@incollection{chatzikokolakis2015geo,
	Author = {Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
	Booktitle = {Distributed Computing and Internet Technology},
	Pages = {49--72},
	Publisher = {Springer},
	Title = {Geo-indistinguishability: A Principled Approach to Location Privacy},
	Year = {2015}}

@inproceedings{ngo2015location,
	Author = {Ngo, Hoa and Kim, Jong},
	Booktitle = {Computer Security Foundations Symposium (CSF), 2015 IEEE 28th},
	Organization = {IEEE},
	Pages = {63--74},
	Title = {Location Privacy via Differential Private Perturbation of Cloaking Area},
	Year = {2015}}


@inproceedings{um2010advanced,
	Author = {Um, Jung-Ho and Kim, Hee-Dae and Chang, Jae-Woo},
	Booktitle = {Social Computing (SocialCom), 2010 IEEE Second International Conference on},
	Organization = {IEEE},
	Pages = {1093--1098},
	Title = {An advanced cloaking algorithm using Hilbert curves for anonymous location based service},
	Year = {2010}}

@inproceedings{bamba2008supporting,
	Author = {Bamba, Bhuvan and Liu, Ling and Pesti, Peter and Wang, Ting},
	Booktitle = {Proceedings of the 17th international conference on World Wide Web},
	Organization = {ACM},
	Pages = {237--246},
	Title = {Supporting anonymous location queries in mobile environments with privacygrid},
	Year = {2008}}

@inproceedings{zhangwei2010distributed,
	Author = {Zhangwei, Huang and Mingjun, Xin},
	Booktitle = {Networks Security Wireless Communications and Trusted Computing (NSWCTC), 2010 Second International Conference on},
	Organization = {IEEE},
	Pages = {468--471},
	Title = {A distributed spatial cloaking protocol for location privacy},
	Volume = {2},
	Year = {2010}}

@article{chow2011spatial,
	Author = {Chow, Chi-Yin and Mokbel, Mohamed F and Liu, Xuan},
	Journal = {GeoInformatica},
	Number = {2},
	Pages = {351--380},
	Publisher = {Springer},
	Title = {Spatial cloaking for anonymous location-based services in mobile peer-to-peer environments},
	Volume = {15},
	Year = {2011}}

@inproceedings{lu2008pad,
	Author = {Lu, Hua and Jensen, Christian S and Yiu, Man Lung},
	Booktitle = {Proceedings of the Seventh ACM International Workshop on Data Engineering for Wireless and Mobile Access},
	Organization = {ACM},
	Pages = {16--23},
	Title = {Pad: privacy-area aware, dummy-based location privacy in mobile services},
	Year = {2008}}

@incollection{khoshgozaran2007blind,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus},
	Booktitle = {Advances in Spatial and Temporal Databases},
	Pages = {239--257},
	Publisher = {Springer},
	Title = {Blind evaluation of nearest neighbor queries using space transformation to preserve location privacy},
	Year = {2007}}

@inproceedings{ghinita2008private,
	Author = {Ghinita, Gabriel and Kalnis, Panos and Khoshgozaran, Ali and Shahabi, Cyrus and Tan, Kian-Lee},
	Booktitle = {Proceedings of the 2008 ACM SIGMOD international conference on Management of data},
	Organization = {ACM},
	Pages = {121--132},
	Title = {Private queries in location based services: anonymizers are not necessary},
	Year = {2008}}



@article{nguyen2013differential,
	Author = {Nguyen, Hiep H and Kim, Jong and Kim, Yoonho},
	Journal = {Journal of Computing Science and Engineering},
	Number = {3},
	Pages = {177--186},
	Title = {Differential privacy in practice},
	Volume = {7},
	Year = {2013}}

@inproceedings{lee2012differential,
	Author = {Lee, Jaewoo and Clifton, Chris},
	Booktitle = {Proceedings of the 18th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {1041--1049},
	Title = {Differential identifiability},
	Year = {2012}}

@inproceedings{andres2013geo,
	Author = {Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2013 ACM SIGSAC conference on Computer \& communications security},
	Organization = {ACM},
	Pages = {901--914},
	Title = {Geo-indistinguishability: Differential privacy for location-based systems},
	Year = {2013}}

@inproceedings{machanavajjhala2008privacy,
	Author = {Machanavajjhala, Ashwin and Kifer, Daniel and Abowd, John and Gehrke, Johannes and Vilhuber, Lars},
	Booktitle = {Data Engineering, 2008. ICDE 2008. IEEE 24th International Conference on},
	Organization = {IEEE},
	Pages = {277--286},
	Title = {Privacy: Theory meets practice on the map},
	Year = {2008}}

@article{dewri2013local,
	Author = {Dewri, Rinku},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {12},
	Pages = {2360--2372},
	Publisher = {IEEE},
	Title = {Local differential perturbations: Location privacy under approximate knowledge attackers},
	Volume = {12},
	Year = {2013}}

@inproceedings{chatzikokolakis2013broadening,
	Author = {Chatzikokolakis, Konstantinos and Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s Emilio and Palamidessi, Catuscia},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {82--102},
	Title = {Broadening the Scope of Differential Privacy Using Metrics.},
	Year = {2013}}



@inproceedings{cheng2006preserving,
	Author = {Cheng, Reynold and Zhang, Yu and Bertino, Elisa and Prabhakar, Sunil},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {393--412},
	Title = {Preserving user location privacy in mobile data management infrastructures},
	Year = {2006}}




@article{krumm2009survey,
	Author = {Krumm, John},
	Journal = {Personal and Ubiquitous Computing},
	Number = {6},
	Pages = {391--399},
	Publisher = {Springer},
	Title = {A survey of computational location privacy},
	Volume = {13},
	Year = {2009}}

@article{Rakhshan2015letter,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Wireless Communications Letter},
	Publisher = {IEEE},
	Title = {A Stochastic Geometry Model for Customized Vehicular Communication},
	Year = {2015, submitted}}

@article{Rakhshan2015Journal,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Publisher = {IEEE},
	Title = {Improving Safety on Highways by Customizing Vehicular Ad Hoc Networks},
	Year = {2015, submitted}}

@inproceedings{Rakhshan2015Cogsima,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Booktitle = {IEEE International Multi-Disciplinary Conference on Cognitive Methods in Situation Awareness and Decision Support},
	Organization = {IEEE},
	Title = {A New Approach to Customization of Accident Warning Systems to Individual Drivers},
	Year = {2015}}

@inproceedings{Rakhshan2015CISS,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Nekoui, Mohammad},
	Booktitle = {Conference on Information Sciences and Systems},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {Driver-based adaptation of Vehicular Ad Hoc Networks for design of active safety systems},
	Year = {2015}}

@inproceedings{Rakhshan2014IV,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Ray, Evan},
	Booktitle = {Intelligent Vehicles Symposium},
	Organization = {IEEE},
	Pages = {1181--1186},
	Title = {Real-time estimation of the distribution of brake response times for an individual driver using Vehicular Ad Hoc Network.},
	Year = {2014}}

@inproceedings{Rakhshan2013Globecom,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Fisher, Donald and Nekoui, Mohammad},
	Booktitle = {IEEE Global Communications Conference},
	Organization = {IEEE},
	Pages = {1333--1337},
	Title = {Tuning collision warning algorithms to individual drivers for design of active safety systems.},
	Year = {2013}}

@article{Nekoui2012Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Number = {8},
	Pages = {2895--2905},
	Publisher = {IEEE},
	Title = {Throughput Scaling laws for Vehicular Ad Hoc Networks},
	Volume = {11},
	Year = {2012}}

@article{Nekoui2013Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {Journal on Selected Areas in Communications, Special Issue on Emerging Technologies in Communications},
	Number = {9},
	Pages = {491--503},
	Publisher = {IEEE},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {31},
	Year = {2013}}

@article{Nekoui2011Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein and Ni, Daiheng},
	Journal = {International Journal of Vehicular Technology},
	Pages = {1--11},
	Publisher = {Hindawi Publishing Corporation},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {2011},
	Year = {2011}}

@inproceedings{Nekoui2011MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM workshop on VehiculAr InterNETworking},
	Organization = {ACM},
	Title = {Analytic Design of Active Vehicular Safety Systems in Sparse Traffic},
	Year = {2011}}

@inproceedings{Nekoui2011VTC,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Analytical Design of Inter-vehicular Communications for Collision Avoidance},
	Year = {2011}}

@inproceedings{Bovee2011VTC,
	Author = {Bovee, Ben Louis and Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Evaluation of the Universal Geocast Scheme For VANETs},
	Year = {2011}}

@inproceedings{Nekoui2010MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM},
	Organization = {ACM},
	Title = {Fundamental Tradeoffs in Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2010IVCS,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IVCS},
	Organization = {IEEE},
	Title = {A Universal Geocast Scheme for Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2009ITW,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IEEE Communications Society Conference on Sensor, Mesh and Ad Hoc Communications and Networks Workshops},
	Organization = {IEEE},
	Pages = {1--3},
	Title = {A Geometrical Analysis of Obstructed Wireless Networks},
	Year = {2009}}

@article{Eslami2013Journal,
	Author = {Eslami, Ali and Nekoui, Mohammad and Pishro-Nik, Hossein and Fekri, Faramarz},
	Journal = {ACM Transactions on Sensor Networks},
	Number = {4},
	Pages = {51},
	Publisher = {ACM},
	Title = {Results on finite wireless sensor networks: Connectivity and coverage},
	Volume = {9},
	Year = {2013}}

@article{shokri2014optimal,
	  title={Optimal user-centric data obfuscation},
 	 author={Shokri, Reza},
 	 journal={arXiv preprint arXiv:1402.3426},
 	 year={2014}
	}
@article{chatzikokolakis2015location,
  title={Location privacy via geo-indistinguishability},
  author={Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
  journal={ACM SIGLOG News},
  volume={2},
  number={3},
  pages={46--69},
  year={2015},
  publisher={ACM}

}
@inproceedings{shokri2011quantifying2,
  title={Quantifying location privacy: the case of sporadic location exposure},
  author={Shokri, Reza and Theodorakopoulos, George and Danezis, George and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
  booktitle={Privacy Enhancing Technologies},
  pages={57--76},
  year={2011},
  organization={Springer}
}

@inproceedings{calmon2015fundamental,
  title={Fundamental limits of perfect privacy},
  author={Calmon, Flavio P and Makhdoumi, Ali and M{\'e}dard, Muriel},
  booktitle={Information Theory (ISIT), 2015 IEEE International Symposium on},
  pages={1796--1800},
  year={2015},
  organization={IEEE}
}

@inproceedings{salamatian2013hide,
  title={How to hide the elephant-or the donkey-in the room: Practical privacy against statistical inference for large data.},
  author={Salamatian, Salman and Zhang, Amy and du Pin Calmon, Flavio and Bhamidipati, Sandilya and Fawaz, Nadia and Kveton, Branislav and Oliveira, Pedro and Taft, Nina},
  booktitle={GlobalSIP},
  pages={269--272},
  year={2013}
}

@article{sankar2013utility,
  title={Utility-privacy tradeoffs in databases: An information-theoretic approach},
  author={Sankar, Lalitha and Rajagopalan, S Raj and Poor, H Vincent},
  journal={Information Forensics and Security, IEEE Transactions on},
  volume={8},
  number={6},
  pages={838--852},
  year={2013},
  publisher={IEEE}
}
@inproceedings{ghinita2007prive,
  title={PRIVE: anonymous location-based queries in distributed mobile systems},
  author={Ghinita, Gabriel and Kalnis, Panos and Skiadopoulos, Spiros},
  booktitle={Proceedings of the 16th international conference on World Wide Web},
  pages={371--380},
  year={2007},
  organization={ACM}
}

@article{beresford2004mix,
  title={Mix zones: User privacy in location-aware services},
  author={Beresford, Alastair R and Stajano, Frank},
  year={2004},
  publisher={IEEE}
}


@article{csiszar1996almost,
  title={Almost independence and secrecy capacity},
  author={Csisz{\'a}r, Imre},
  journal={Problemy Peredachi Informatsii},
  volume={32},
  number={1},
  pages={48--57},
  year={1996},
  publisher={Russian Academy of Sciences, Branch of Informatics, Computer Equipment and Automatization}
}

@article{yamamoto1983source,
  title={A source coding problem for sources with additional outputs to keep secret from the receiver or wiretappers (corresp.)},
  author={Yamamoto, Hirosuke},
  journal={IEEE Transactions on Information Theory},
  volume={29},
  number={6},
  pages={918--923},
  year={1983},
  publisher={IEEE}
}



  @inproceedings{golle2009anonymity,
  title={On the anonymity of home/work location pairs},
  author={Golle, Philippe and Partridge, Kurt},
  booktitle={International Conference on Pervasive Computing},
  pages={390--397},
  year={2009},
  organization={Springer}
}

@inproceedings{zang2011anonymization,
  title={Anonymization of location data does not work: A large-scale measurement study},
  author={Zang, Hui and Bolot, Jean},
  booktitle={Proceedings of the 17th annual international conference on Mobile computing and networking},
  pages={145--156},
  year={2011},
  organization={ACM}
}
@article{wang2015privacy,
  title={Privacy-preserving collaborative spectrum sensing with multiple service providers},
  author={Wang, Wei and Zhang, Qian},
  journal={IEEE Transactions on Wireless Communications},
  volume={14},
  number={2},
  pages={1011--1019},
  year={2015},
  publisher={IEEE}
}

@article{wang2015toward,
  title={Toward long-term quality of protection in mobile networks: a context-aware perspective},
  author={Wang, Wei and Zhang, Qian},
  journal={IEEE Wireless Communications},
  volume={22},
  number={4},
  pages={34--40},
  year={2015},
  publisher={IEEE}
}

@inproceedings{niu2015enhancing,
  title={Enhancing privacy through caching in location-based services},
  author={Niu, Ben and Li, Qinghua and Zhu, Xiaoyan and Cao, Guohong and Li, Hui},
  booktitle={2015 IEEE Conference on Computer Communications (INFOCOM)},
  pages={1017--1025},
  year={2015},
  organization={IEEE}
}

%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Created for Zarrin Montazeri at 2015-11-09 18:45:31 -0500


%% Saved with string encoding Unicode (UTF-8)



%%%%%%%%%%%%%%IOT%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@article{osma2015,
	title={Impact of Time-to-Collision Information on Driving Behavior in Connected Vehicle Environments Using A Driving Simulator Test Bed},
	journal{Journal of Traffic and Logistics Engineering},
	author={Osama A. Osman, Julius Codjoe, and Sherif Ishak},
	volume={3},
	number={1},
	pages={18--24},
	year={2015}
}


@article{charisma2010,
	title={Dynamic Latent Plan Models},
	author={Charisma F. Choudhurya, Moshe Ben-Akivab and Maya Abou-Zeid},
	journal={Journal of Choice Modelling},
	volume={3},
	number={2},
	pages={50--70},
	year={2010},
	publisher={Elsvier}
}


@misc{noble2014,
	author = {A. M. Noble, Shane B. McLaughlin, Zachary R. Doerzaph and Thomas A. Dingus},
	title = {Crowd-sourced Connected-vehicle Warning Algorithm using Naturalistic Driving Data},
	howpublished = {Downloaded from \url{http://hdl.handle.net/10919/53978}},
	
	month = August,
	year = 2014
}


@phdthesis{charisma2007,
	title    = {Modeling Driving Decisions with Latent Plans},
	school   = {Massachusetts Institute of Technology },
	author   = {Charisma Farheen Choudhury},
	year     = {2007}, %other attributes omitted
}


@article{chrysler2015,
	title={Cost of Warning of Unseen Threats:Unintended Consequences of Connected Vehicle Alerts},
	author={S. T. Chrysler, J. M. Cooper and D. C. Marshall},
	journal={Transportation Research Record: Journal of the Transportation Research Board},
	volume={2518},
	pages={79--85},
	year={2015},
}





@article{FTC2015,
	title={Internet of Things: Privacy and Security in a Connected World},
	author={FTC Staff Report},
	year={2015}
}



%% Saved with string encoding Unicode (UTF-8)
@inproceedings{1zhou2014security,
	title={Security/privacy of wearable fitness tracking {I}o{T} devices},
	author={Zhou, Wei and Piramuthu, Selwyn},
	booktitle={Information Systems and Technologies (CISTI), 2014 9th Iberian Conference on},
	pages={1--5},
	year={2014},
	organization={IEEE}
}


@inproceedings{3ukil2014iot,
	title={{I}o{T}-privacy: To be private or not to be private},
	author={Arijit Ukil and Soma Bandyopadhyay and Arpan Pal},
	booktitle={Computer Communications Workshops (INFOCOM WKSHPS), IEEE Conference on},
	pages={123--124},
	year={2014},
	organization={IEEE}
}

@inproceedings{4Hosseinzadeh2014,
	title={Security in the Internet of Things through obfuscation and diversification},
	author={Hosseinzadeh, Shohreh and Rauti, Sampsa and Hyrynsalmi, Sami and Leppanen, Ville},
	booktitle={Computing, Communication and Security (ICCCS), IEEE Conference on},
	pages={123--124},
	year={2015},
	organization={IEEE}
}
@article{4arias2015privacy,
	title={Privacy and security in internet of things and wearable devices},
	author={Arias, Orlando and Wurm, Jacob and Hoang, Khoa and Jin, Yier},
	journal={IEEE Transactions on Multi-Scale Computing Systems},
	volume={1},
	number={2},
	pages={99--109},
	year={2015},
	publisher={IEEE}
}
@inproceedings{5ullah2016novel,
	title={A novel model for preserving Location Privacy in Internet of Things},
	author={Ullah, Ikram and Shah, Munam Ali},
	booktitle={Automation and Computing (ICAC), 2016 22nd International Conference on},
	pages={542--547},
	year={2016},
	organization={IEEE}
}
@inproceedings{6sathishkumar2016enhanced,
	title={Enhanced location privacy algorithm for wireless sensor network in Internet of Things},
	author={Sathishkumar, J and Patel, Dhiren R},
	booktitle={Internet of Things and Applications (IOTA), International Conference on},
	pages={208--212},
	year={2016},
	organization={IEEE}
}
@inproceedings{7zhou2012preserving,
	title={Preserving sensor location privacy in internet of things},
	author={Zhou, Liming and Wen, Qiaoyan and Zhang, Hua},
	booktitle={Computational and Information Sciences (ICCIS), 2012 Fourth International Conference on},
	pages={856--859},
	year={2012},
	organization={IEEE}
}

@inproceedings{8ukil2015privacy,
	title={Privacy for {I}o{T}: Involuntary privacy enablement for smart energy systems},
	author={Ukil, Arijit and Bandyopadhyay, Soma and Pal, Arpan},
	booktitle={Communications (ICC), 2015 IEEE International Conference on},
	pages={536--541},
	year={2015},
	organization={IEEE}
}

@inproceedings{9dalipi2016security,
	title={Security and Privacy Considerations for {I}o{T} Application on Smart Grids: Survey and Research Challenges},
	author={Dalipi, Fisnik and Yayilgan, Sule Yildirim},
	booktitle={Future Internet of Things and Cloud Workshops (FiCloudW), IEEE International Conference on},
	pages={63--68},
	year={2016},
	organization={IEEE}
}
@inproceedings{10harris2016security,
	title={Security and Privacy in Public {I}o{T} Spaces},
	author={Harris, Albert F and Sundaram, Hari and Kravets, Robin},
	booktitle={Computer Communication and Networks (ICCCN), 2016 25th International Conference on},
	pages={1--8},
	year={2016},
	organization={IEEE}
}

@inproceedings{11al2015security,
	title={Security and privacy framework for ubiquitous healthcare {I}o{T} devices},
	author={Al Alkeem, Ebrahim and Yeun, Chan Yeob and Zemerly, M Jamal},
	booktitle={Internet Technology and Secured Transactions (ICITST), 2015 10th International Conference for},
	pages={70--75},
	year={2015},
	organization={IEEE}
}
@inproceedings{12sivaraman2015network,
	title={Network-level security and privacy control for smart-home {I}o{T} devices},
	author={Sivaraman, Vijay and Gharakheili, Hassan Habibi and Vishwanath, Arun and Boreli, Roksana and Mehani, Olivier},
	booktitle={Wireless and Mobile Computing, Networking and Communications (WiMob), 2015 IEEE 11th International Conference on},
	pages={163--167},
	year={2015},
	organization={IEEE}
}

@inproceedings{13srinivasan2016privacy,
	title={Privacy conscious architecture for improving emergency response in smart cities},
	author={Srinivasan, Ramya and Mohan, Apurva and Srinivasan, Priyanka},
	booktitle={Smart City Security and Privacy Workshop (SCSP-W), 2016},
	pages={1--5},
	year={2016},
	organization={IEEE}
}
@inproceedings{14sadeghi2015security,
	title={Security and privacy challenges in industrial internet of things},
	author={Sadeghi, Ahmad-Reza and Wachsmann, Christian and Waidner, Michael},
	booktitle={Design Automation Conference (DAC), 2015 52nd ACM/EDAC/IEEE},
	pages={1--6},
	year={2015},
	organization={IEEE}
}
@inproceedings{15otgonbayar2016toward,
	title={Toward Anonymizing {I}o{T} Data Streams via Partitioning},
	author={Otgonbayar, Ankhbayar and Pervez, Zeeshan and Dahal, Keshav},
	booktitle={Mobile Ad Hoc and Sensor Systems (MASS), 2016 IEEE 13th International Conference on},
	pages={331--336},
	year={2016},
	organization={IEEE}
}
@inproceedings{16rutledge2016privacy,
	title={Privacy Impacts of {I}o{T} Devices: A SmartTV Case Study},
	author={Rutledge, Richard L and Massey, Aaron K and Ant{\'o}n, Annie I},
	booktitle={Requirements Engineering Conference Workshops (REW), IEEE International},
	pages={261--270},
	year={2016},
	organization={IEEE}
}

@inproceedings{17andrea2015internet,
	title={Internet of Things: Security vulnerabilities and challenges},
	author={Andrea, Ioannis and Chrysostomou, Chrysostomos and Hadjichristofi, George},
	booktitle={Computers and Communication (ISCC), 2015 IEEE Symposium on},
	pages={180--187},
	year={2015},
	organization={IEEE}
}






























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@misc{epfl-mobility-20090224,
	author = {Michal Piorkowski and Natasa Sarafijanovic-Djukic and Matthias Grossglauser},
	title = {{CRAWDAD} dataset epfl/mobility (v. 2009-02-24)},
	howpublished = {Downloaded from \url{http://crawdad.org/epfl/mobility/20090224}},
	doi = {10.15783/C7J010},
	month = feb,
	year = 2009
}

@misc{roma-taxi-20140717,
	author = {Lorenzo Bracciale and Marco Bonola and Pierpaolo Loreti and Giuseppe Bianchi and Raul Amici and Antonello Rabuffi},
	title = {{CRAWDAD} dataset roma/taxi (v. 2014-07-17)},
	howpublished = {Downloaded from \url{http://crawdad.org/roma/taxi/20140717}},
	doi = {10.15783/C7QC7M},
	month = jul,
	year = 2014
}

@misc{rice-ad_hoc_city-20030911,
	author = {Jorjeta G. Jetcheva and Yih-Chun Hu and Santashil PalChaudhuri and Amit Kumar Saha and David B. Johnson},
	title = {{CRAWDAD} dataset rice/ad\_hoc\_city (v. 2003-09-11)},
	howpublished = {Downloaded from \url{http://crawdad.org/rice/ad_hoc_city/20030911}},
	doi = {10.15783/C73K5B},
	month = sep,
	year = 2003
}

@misc{china:2012,
	author = {Microsoft Research Asia},
	title = {GeoLife GPS Trajectories},
	year = {2012},
	howpublished= {\url{https://www.microsoft.com/en-us/download/details.aspx?id=52367}},
}


@misc{china:2011,
	ALTauthor = {Microsoft Research Asia)},
	ALTeditor = {},
	title = {GeoLife GPS Trajectories,
	year = {2012},
	url = {https://www.microsoft.com/en-us/download/details.aspx?id=52367},
	}
	
	
	@misc{longversion,
	author = {N. Takbiri and A. Houmansadr and D.L. Goeckel and H. Pishro-Nik},
	title = {{Limits of Location Privacy under Anonymization and Obfuscation}},
	howpublished = "\url{https://dl.dropboxusercontent.com/u/49263048/ISIT_2017-2.pdf}",
	year = 2017,
	month= "January",
	note = "[Online; accessed 22-Jan-2017]"
	}
	
	
	
	@article{matching,
	title={Asymptotically Optimal Matching of Multiple Sequences to Source Distributions and Training Sequences},
	author={Jayakrishnan Unnikrishnan},
	journal={ IEEE Transactions on Information Theory},
	volume={61},
	number={1},
	pages={452-468},
	year={2015},
	publisher={IEEE}
	}
	
	
	@article{Naini2016,
	Author = {F. Naini and J. Unnikrishnan and P. Thiran and M. Vetterli},
	Journal = {IEEE Transactions on Information Forensics and Security},
	Publisher = {IEEE},
	Title = {Where You Are Is Who You Are: User Identification by Matching Statistics},
	volume={11},
	number={2},
	pages={358--372},
	Year = {2016}
	}
	
	
	
	@inproceedings{holowczak2015cachebrowser,
	title={{CacheBrowser: Bypassing Chinese Censorship without Proxies Using Cached Content}},
	author={Holowczak, John and Houmansadr, Amir},
	booktitle={Proceedings of the 22nd ACM SIGSAC Conference on Computer and Communications Security},
	pages={70--83},
	year={2015},
	organization={ACM}
	}
	@misc{cb-website,
	Howpublished = {\url{https://cachebrowser.net/#/}},
	Title = {{CacheBrowser}},
	key={cachebrowser}
	}
	
	@inproceedings{GameOfDecoys,
	title={{GAME OF DECOYS: Optimal Decoy Routing Through Game Theory}},
	author={Milad Nasr and Amir Houmansadr},
	booktitle={The $23^{rd}$ ACM Conference on Computer and Communications Security (CCS)},
	year={2016}
	}
	
	@inproceedings{CDNReaper,
	title={{Practical Censorship Evasion Leveraging Content Delivery Networks}},
	author={Hadi Zolfaghari and Amir Houmansadr},
	booktitle={The $23^{rd}$ ACM Conference on Computer and Communications Security (CCS)},
	year={2016}
	}
	
	@misc{Leberknight2010,
	Author = {Leberknight, C. and Chiang, M. and Poor, H. and Wong, F.},
	Howpublished = {\url{http://www.princeton.edu/~chiangm/anticensorship.pdf}},
	Title = {{A Taxonomy of Internet Censorship and Anti-censorship}},
	Year = {2010}}
	
	@techreport{ultrasurf-analysis,
	Author = {Appelbaum, Jacob},
	Institution = {The Tor Project},
	Title = {{Technical analysis of the Ultrasurf proxying software}},
	Url = {http://scholar.google.com/scholar?hl=en\&btnG=Search\&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software\#0},
	Year = {2012},
	Bdsk-Url-1 = {http://scholar.google.com/scholar?hl=en%5C&btnG=Search%5C&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software%5C#0}}
	
	@misc{gifc:07,
	Howpublished = {\url{http://www.internetfreedom.org/archive/Defeat\_Internet\_Censorship\_White\_Paper.pdf}},
	Key = {defeatcensorship},
	Publisher = {Global Internet Freedom Consortium (GIFC)},
	Title = {{Defeat Internet Censorship: Overview of Advanced Technologies and Products}},
	Type = {White Paper},
	Year = {2007}}
	
	@article{pan2011survey,
	Author = {Pan, J. and Paul, S. and Jain, R.},
	Journal = {Communications Magazine, IEEE},
	Number = {7},
	Pages = {26--36},
	Publisher = {IEEE},
	Title = {{A Survey of the Research on Future Internet Architectures}},
	Volume = {49},
	Year = {2011}}
	
	@misc{nsf-fia,
	Howpublished = {\url{http://www.nets-fia.net/}},
	Key = {FIA},
	Title = {{NSF Future Internet Architecture Project}}}
	
	@misc{NDN,
	Howpublished = {\url{http://www.named- data.net}},
	Key = {NDN},
	Title = {{Named Data Networking Project}}}
	
	@inproceedings{MobilityFirst,
	Author = {Seskar, I. and Nagaraja, K. and Nelson, S. and Raychaudhuri, D.},
	Booktitle = {Asian Internet Engineering Conference},
	Title = {{Mobilityfirst Future internet Architecture Project}},
	Year = {2011}}
	
	@incollection{NEBULA,
	Author = {Anderson, T. and Birman, K. and Broberg, R. and Caesar, M. and Comer, D. and Cotton, C. and Freedman, M.~J. and Haeberlen, A. and Ives, Z.~G. and Krishnamurthy, A. and others},
	Booktitle = {The Future Internet},
	Pages = {16--26},
	Publisher = {Springer},
	Title = {{The NEBULA Future Internet Architecture}},
	Year = {2013}}
	
	@inproceedings{XIA,
	Author = {Anand, A. and Dogar, F. and Han, D. and Li, B. and Lim, H. and Machado, M. and Wu, W. and Akella, A. and Andersen, D.~G. and Byers, J.~W. and others},
	Booktitle = {ACM Workshop on Hot Topics in Networks},
	Pages = {2},
	Title = {{XIA: An Architecture for an Evolvable and Trustworthy Internet}},
	Year = {2011}}
	
	@inproceedings{ChoiceNet,
	Author = {Rouskas, G.~N. and Baldine, I. and Calvert, K.~L. and Dutta, R. and Griffioen, J. and Nagurney, A. and Wolf, T.},
	Booktitle = {ONDM},
	Title = {{ChoiceNet: Network Innovation Through Choice}},
	Year = {2013}}
	
	@misc{nsf-find,
	Howpublished = {http://www.nets-find.net/},
	Title = {{NSF NeTS FIND Initiative}}}
	
	@article{traid,
	Author = {Cheriton, D.~R. and Gritter, M.},
	Title = {{TRIAD: A New Next-Generation Internet Architecture}},
	Year = {2000}}
	
	@inproceedings{dona,
	Author = {Koponen, T. and Chawla, M. and Chun, B-G. and Ermolinskiy, A. and Kim, K.~H. and Shenker, S. and Stoica, I.},
	Booktitle = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Organization = {ACM},
	Pages = {181--192},
	Title = {{A Data-Oriented (and Beyond) Network Architecture}},
	Volume = {37},
	Year = {2007}}
	
	@misc{ultrasurf,
	Howpublished = {\url{http://www.ultrareach.com}},
	Key = {ultrasurf},
	Title = {{Ultrasurf}}}
	
	@misc{tor-bridge,
	Author = {Dingledine, R. and Mathewson, N.},
	Howpublished = {\url{https://svn.torproject.org/svn/projects/design-paper/blocking.html}},
	Title = {{Design of a Blocking-Resistant Anonymity System}}}
	
	@inproceedings{McLachlanH09,
	Author = {J. McLachlan and N. Hopper},
	Booktitle = {WPES},
	Title = {{On the Risks of Serving Whenever You Surf: Vulnerabilities in Tor's Blocking Resistance Design}},
	Year = {2009}}
	
	@inproceedings{mahdian2010,
	Author = {Mahdian, M.},
	Booktitle = {{Fun with Algorithms}},
	Title = {{Fighting Censorship with Algorithms}},
	Year = {2010}}
	
	@inproceedings{McCoy2011,
	Author = {McCoy, D. and Morales, J.~A. and Levchenko, K.},
	Booktitle = {FC},
	Title = {{Proximax: A Measurement Based System for Proxies Dissemination}},
	Year = {2011}}
	
	@inproceedings{Sovran2008,
	Author = {Sovran, Y. and Libonati, A. and Li, J.},
	Booktitle = {IPTPS},
	Title = {{Pass it on: Social Networks Stymie Censors}},
	Year = {2008}}
	
	@inproceedings{rbridge,
	Author = {Wang, Q. and Lin, Zi and Borisov, N. and Hopper, N.},
	Booktitle = {{NDSS}},
	Title = {{rBridge: User Reputation based Tor Bridge Distribution with Privacy Preservation}},
	Year = {2013}}
	
	@inproceedings{telex,
	Author = {Wustrow, E. and Wolchok, S. and Goldberg, I. and Halderman, J.},
	Booktitle = {{USENIX Security}},
	Title = {{Telex: Anticensorship in the Network Infrastructure}},
	Year = {2011}}
	
	@inproceedings{cirripede,
	Author = {Houmansadr, A. and Nguyen, G. and Caesar, M. and Borisov, N.},
	Booktitle = {CCS},
	Title = {{Cirripede: Circumvention Infrastructure Using Router Redirection with Plausible Deniability}},
	Year = {2011}}
	
	@inproceedings{decoyrouting,
	Author = {Karlin, J. and Ellard, D. and Jackson, A. and Jones, C. and Lauer, G. and Mankins, D. and Strayer, W.},
	Booktitle = {{FOCI}},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = {2011}}
	
	@inproceedings{routing-around-decoys,
	Author = {M.~Schuchard and J.~Geddes and C.~Thompson and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Routing Around Decoys}},
	Year = {2012}}
	
	@inproceedings{parrot,
	Author = {A. Houmansadr and C. Brubaker and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{The Parrot is Dead: Observing Unobservable Network Communications}},
	Year = {2013}}
	
	@misc{knock,
	Author = {T. Wilde},
	Howpublished = {\url{https://blog.torproject.org/blog/knock-knock-knockin-bridges-doors}},
	Title = {{Knock Knock Knockin' on Bridges' Doors}},
	Year = {2012}}
	
	@inproceedings{china-tor,
	Author = {Winter, P. and Lindskog, S.},
	Booktitle = {{FOCI}},
	Title = {{How the Great Firewall of China Is Blocking Tor}},
	Year = {2012}}
	
	@misc{discover-bridge,
	Howpublished = {\url{https://blog.torproject.org/blog/research-problems-ten-ways-discover-tor-bridges}},
	Key = {tenways},
	Title = {{Ten Ways to Discover Tor Bridges}}}
	
	@inproceedings{freewave,
	Author = {A.~Houmansadr and T.~Riedl and N.~Borisov and A.~Singer},
	Booktitle = {{NDSS}},
	Title = {{I Want My Voice to Be Heard: IP over Voice-over-IP for Unobservable Censorship Circumvention}},
	Year = 2013}
	
	@inproceedings{censorspoofer,
	Author = {Q. Wang and X. Gong and G. Nguyen and A. Houmansadr and N. Borisov},
	Booktitle = {CCS},
	Title = {{CensorSpoofer: Asymmetric Communication Using IP Spoofing for Censorship-Resistant Web Browsing}},
	Year = {2012}}
	
	@inproceedings{skypemorph,
	Author = {H. Moghaddam and B. Li and M. Derakhshani and I. Goldberg},
	Booktitle = {CCS},
	Title = {{SkypeMorph: Protocol Obfuscation for Tor Bridges}},
	Year = {2012}}
	
	@inproceedings{stegotorus,
	Author = {Weinberg, Z. and Wang, J. and Yegneswaran, V. and Briesemeister, L. and Cheung, S. and Wang, F. and Boneh, D.},
	Booktitle = {CCS},
	Title = {{StegoTorus: A Camouflage Proxy for the Tor Anonymity System}},
	Year = {2012}}
	
	@techreport{dust,
	Author = {{B.~Wiley}},
	Howpublished = {\url{http://blanu.net/ Dust.pdf}},
	Institution = {School of Information, University of Texas at Austin},
	Title = {{Dust: A Blocking-Resistant Internet Transport Protocol}},
	Year = {2011}}
	
	@inproceedings{FTE,
	Author = {K.~Dyer and S.~Coull and T.~Ristenpart and T.~Shrimpton},
	Booktitle = {CCS},
	Title = {{Protocol Misidentification Made Easy with Format-Transforming Encryption}},
	Year = {2013}}
	
	@inproceedings{fp,
	Author = {Fifield, D. and Hardison, N. and Ellithrope, J. and Stark, E. and Dingledine, R. and Boneh, D. and Porras, P.},
	Booktitle = {PETS},
	Title = {{Evading Censorship with Browser-Based Proxies}},
	Year = {2012}}
	
	@misc{obfsproxy,
	Howpublished = {\url{https://www.torproject.org/projects/obfsproxy.html.en}},
	Key = {obfsproxy},
	Publisher = {The Tor Project},
	Title = {{A Simple Obfuscating Proxy}}}
	
	@inproceedings{Tor-instead-of-IP,
	Author = {Liu, V. and Han, S. and Krishnamurthy, A. and Anderson, T.},
	Booktitle = {HotNets},
	Title = {{Tor instead of IP}},
	Year = {2011}}
	
	@misc{roger-slides,
	Howpublished = {\url{https://svn.torproject.org/svn/projects/presentations/slides-28c3.pdf}},
	Key = {torblocking},
	Title = {{How Governments Have Tried to Block Tor}}}
	
	@inproceedings{infranet,
	Author = {Feamster, N. and Balazinska, M. and Harfst, G. and Balakrishnan, H. and Karger, D.},
	Booktitle = {USENIX Security},
	Title = {{Infranet: Circumventing Web Censorship and Surveillance}},
	Year = {2002}}
	
	@inproceedings{collage,
	Author = {S.~Burnett and N.~Feamster and S.~Vempala},
	Booktitle = {USENIX Security},
	Title = {{Chipping Away at Censorship Firewalls with User-Generated Content}},
	Year = {2010}}
	
	@article{anonymizer,
	Author = {Boyan, J.},
	Journal = {Computer-Mediated Communication Magazine},
	Month = sep,
	Number = {9},
	Title = {{The Anonymizer: Protecting User Privacy on the Web}},
	Volume = {4},
	Year = {1997}}
	
	@article{schulze2009internet,
	Author = {Schulze, H. and Mochalski, K.},
	Journal = {IPOQUE Report},
	Pages = {351--362},
	Title = {Internet Study 2008/2009},
	Volume = {37},
	Year = {2009}}
	
	@inproceedings{cya-ccs13,
	Author = {J.~Geddes and M.~Schuchard and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Cover Your ACKs: Pitfalls of Covert Channel Censorship Circumvention}},
	Year = {2013}}
	
	@inproceedings{andana,
	Author = {DiBenedetto, S. and Gasti, P. and Tsudik, G. and Uzun, E.},
	Booktitle = {{NDSS}},
	Title = {{ANDaNA: Anonymous Named Data Networking Application}},
	Year = {2012}}
	
	@inproceedings{darkly,
	Author = {Jana, S. and Narayanan, A. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{A Scanner Darkly: Protecting User Privacy From Perceptual Applications}},
	Year = {2013}}
	
	@inproceedings{NS08,
	Author = {A.~Narayanan and V.~Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {Robust de-anonymization of large sparse datasets},
	Year = {2008}}
	
	@inproceedings{NS09,
	Author = {A.~Narayanan and V.~Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {De-anonymizing social networks},
	Year = {2009}}
	
	@inproceedings{memento,
	Author = {Jana, S. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{Memento: Learning secrets from process footprints}},
	Year = {2012}}
	
	@misc{plugtor,
	Howpublished = {\url{https://www.torproject.org/docs/pluggable-transports.html.en}},
	Key = {PluggableTransports},
	Publisher = {The Tor Project},
	Title = {{Tor: Pluggable transports}}}
	
	@misc{psiphon,
	Author = {J.~Jia and P.~Smith},
	Howpublished = {\url{http://www.cdf.toronto.edu/~csc494h/reports/2004-fall/psiphon_ae.html}},
	Title = {{Psiphon: Analysis and Estimation}},
	Year = 2004}
	
	@misc{china-github,
	Howpublished = {\url{http://mobile.informationweek.com/80269/show/72e30386728f45f56b343ddfd0fdb119/}},
	Key = {github},
	Title = {{China's GitHub Censorship Dilemma}}}
	
	@inproceedings{txbox,
	Author = {Jana, S. and Porter, D. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{TxBox: Building Secure, Efficient Sandboxes with System Transactions}},
	Year = {2011}}
	
	@inproceedings{airavat,
	Author = {I. Roy and S. Setty and A. Kilzer and V. Shmatikov and E. Witchel},
	Booktitle = {NSDI},
	Title = {{Airavat: Security and Privacy for MapReduce}},
	Year = {2010}}
	
	@inproceedings{osdi12,
	Author = {A. Dunn and M. Lee and S. Jana and S. Kim and M. Silberstein and Y. Xu and V. Shmatikov and E. Witchel},
	Booktitle = {OSDI},
	Title = {{Eternal Sunshine of the Spotless Machine: Protecting Privacy with Ephemeral Channels}},
	Year = {2012}}
	
	@inproceedings{ymal,
	Author = {J. Calandrino and A. Kilzer and A. Narayanan and E. Felten and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{``You Might Also Like:'' Privacy Risks of Collaborative Filtering}},
	Year = {2011}}
	
	@inproceedings{srivastava11,
	Author = {V. Srivastava and M. Bond and K. McKinley and V. Shmatikov},
	Booktitle = {PLDI},
	Title = {{A Security Policy Oracle: Detecting Security Holes Using Multiple API Implementations}},
	Year = {2011}}
	
	@inproceedings{chen-oakland10,
	Author = {Chen, S. and Wang, R. and Wang, X. and Zhang, K.},
	Booktitle = {IEEE S\&P},
	Title = {{Side-Channel Leaks in Web Applications: A Reality Today, a Challenge Tomorrow}},
	Year = {2010}}
	
	@book{kerck,
	Author = {Kerckhoffs, A.},
	Publisher = {University Microfilms},
	Title = {{La cryptographie militaire}},
	Year = {1978}}
	
	@inproceedings{foci11,
	Author = {J. Karlin and D. Ellard and A.~Jackson and C.~ Jones and G. Lauer and D. Mankins and W.~T.~Strayer},
	Booktitle = {FOCI},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = 2011}
	
	@inproceedings{sun02,
	Author = {Sun, Q. and Simon, D.~R. and Wang, Y. and Russell, W. and Padmanabhan, V. and Qiu, L.},
	Booktitle = {IEEE S\&P},
	Title = {{Statistical Identification of Encrypted Web Browsing Traffic}},
	Year = {2002}}
	
	@inproceedings{danezis,
	Author = {Murdoch, S.~J. and Danezis, G.},
	Booktitle = {IEEE S\&P},
	Title = {{Low-Cost Traffic Analysis of Tor}},
	Year = {2005}}
	
	@inproceedings{pakicensorship,
	Author = {Z.~Nabi},
	Booktitle = {FOCI},
	Title = {The Anatomy of {Web} Censorship in {Pakistan}},
	Year = {2013}}
	
	@inproceedings{irancensorship,
	Author = {S.~Aryan and H.~Aryan and A.~Halderman},
	Booktitle = {FOCI},
	Title = {Internet Censorship in {Iran}: {A} First Look},
	Year = {2013}}
	
	@inproceedings{ford10efficient,
	Author = {Amittai Aviram and Shu-Chun Weng and Sen Hu and Bryan Ford},
	Booktitle = {\bibconf[9th]{OSDI}{USENIX Symposium on Operating Systems Design and Implementation}},
	Location = {Vancouver, BC, Canada},
	Month = oct,
	Title = {Efficient System-Enforced Deterministic Parallelism},
	Year = 2010}
	
	@inproceedings{ford10determinating,
	Author = {Amittai Aviram and Sen Hu and Bryan Ford and Ramakrishna Gummadi},
	Booktitle = {\bibconf{CCSW}{ACM Cloud Computing Security Workshop}},
	Location = {Chicago, IL},
	Month = oct,
	Title = {Determinating Timing Channels in Compute Clouds},
	Year = 2010}
	
	@inproceedings{ford12plugging,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Plugging Side-Channel Leaks with Timing Information Flow Control},
	Year = 2012}
	
	@inproceedings{ford12icebergs,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Icebergs in the Clouds: the {\em Other} Risks of Cloud Computing},
	Year = 2012}
	
	@misc{mullenize,
	Author = {Washington Post},
	Howpublished = {\url{http://apps.washingtonpost.com/g/page/world/gchq-report-on-mullenize-program-to-stain-anonymous-electronic-traffic/502/}},
	Month = {oct},
	Title = {{GCHQ} report on {`MULLENIZE'} program to `stain' anonymous electronic traffic},
	Year = {2013}}
	
	@inproceedings{shue13street,
	Author = {Craig A. Shue and Nathanael Paul and Curtis R. Taylor},
	Booktitle = {\bibbrev[7th]{WOOT}{USENIX Workshop on Offensive Technologies}},
	Month = aug,
	Title = {From an {IP} Address to a Street Address: Using Wireless Signals to Locate a Target},
	Year = 2013}
	
	@inproceedings{knockel11three,
	Author = {Jeffrey Knockel and Jedidiah R. Crandall and Jared Saia},
	Booktitle = {\bibbrev{FOCI}{USENIX Workshop on Free and Open Communications on the Internet}},
	Location = {San Francisco, CA},
	Month = aug,
	Year = 2011}
	
	@misc{rfc4960,
	Author = {R. {Stewart, ed.}},
	Month = sep,
	Note = {RFC 4960},
	Title = {Stream Control Transmission Protocol},
	Year = 2007}
	
	@inproceedings{ford07structured,
	Author = {Bryan Ford},
	Booktitle = {\bibbrev{SIGCOMM}{ACM SIGCOMM}},
	Location = {Kyoto, Japan},
	Month = aug,
	Title = {Structured Streams: a New Transport Abstraction},
	Year = {2007}}
	
	@misc{spdy,
	Author = {Google, Inc.},
	Note = {\url{http://www.chromium.org/spdy/spdy-whitepaper}},
	Title = {{SPDY}: An Experimental Protocol For a Faster {Web}}}
	
	@misc{quic,
	Author = {Jim Roskind},
	Month = jun,
	Note = {\url{http://blog.chromium.org/2013/06/experimenting-with-quic.html}},
	Title = {Experimenting with {QUIC}},
	Year = 2013}
	
	@misc{podjarny12not,
	Author = {G.~Podjarny},
	Month = jun,
	Note = {\url{http://www.guypo.com/technical/not-as-spdy-as-you-thought/}},
	Title = {{Not as SPDY as You Thought}},
	Year = 2012}
	
	@inproceedings{cor,
	Author = {Jones, N.~A. and Arye, M. and Cesareo, J. and Freedman, M.~J.},
	Booktitle = {FOCI},
	Title = {{Hiding Amongst the Clouds: A Proposal for Cloud-based Onion Routing}},
	Year = {2011}}
	
	@misc{torcloud,
	Howpublished = {\url{https://cloud.torproject.org/}},
	Key = {tor cloud},
	Title = {{The Tor Cloud Project}}}
	
	@inproceedings{scramblesuit,
	Author = {Philipp Winter and Tobias Pulls and Juergen Fuss},
	Booktitle = {WPES},
	Title = {{ScrambleSuit: A Polymorphic Network Protocol to Circumvent Censorship}},
	Year = 2013}
	
	@article{savage2000practical,
	Author = {Savage, S. and Wetherall, D. and Karlin, A. and Anderson, T.},
	Journal = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Pages = {295--306},
	Publisher = {ACM},
	Title = {Practical network support for IP traceback},
	Volume = {30},
	Year = {2000}}
	
	@inproceedings{ooni,
	Author = {Filast, A. and Appelbaum, J.},
	Booktitle = {{FOCI}},
	Title = {{OONI : Open Observatory of Network Interference}},
	Year = {2012}}
	
	@misc{caida-rank,
	Howpublished = {\url{http://as-rank.caida.org/}},
	Key = {caida rank},
	Title = {{AS Rank: AS Ranking}}}
	
	@inproceedings{usersrouted-ccs13,
	Author = {A.~Johnson and C.~Wacek and R.~Jansen and M.~Sherr and P.~Syverson},
	Booktitle = {CCS},
	Title = {{Users Get Routed: Traffic Correlation on Tor by Realistic Adversaries}},
	Year = {2013}}
	
	@inproceedings{edman2009awareness,
	Author = {Edman, M. and Syverson, P.},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2009}}
	
	@inproceedings{DecoyCosts,
	Author = {A.~Houmansadr and E.~L.~Wong and V.~Shmatikov},
	Booktitle = {NDSS},
	Title = {{No Direction Home: The True Cost of Routing Around Decoys}},
	Year = {2014}}
	
	@article{cordon,
	Author = {Elahi, T. and Goldberg, I.},
	Journal = {University of Waterloo CACR},
	Title = {{CORDON--A Taxonomy of Internet Censorship Resistance Strategies}},
	Volume = {33},
	Year = {2012}}
	
	@inproceedings{privex,
	Author = {T.~Elahi and G.~Danezis and I.~Goldberg	},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2014}}
	
	@inproceedings{changeGuards,
	Author = {T.~Elahi and K.~Bauer and M.~AlSabah and R.~Dingledine and I.~Goldberg},
	Booktitle = {{WPES}},
	Title = {{ Changing of the Guards: Framework for Understanding and Improving Entry Guard Selection in Tor}},
	Year = {2012}}
	
	@article{RAINBOW:Journal,
	Author = {A.~Houmansadr and N.~Kiyavash and N.~Borisov},
	Journal = {IEEE/ACM Transactions on Networking},
	Title = {{Non-Blind Watermarking of Network Flows}},
	Year = 2014}
	
	@inproceedings{info-tod,
	Author = {A.~Houmansadr and S.~Gorantla and T.~Coleman and N.~Kiyavash and and N.~Borisov},
	Booktitle = {{CCS (poster session)}},
	Title = {{On the Channel Capacity of Network Flow Watermarking}},
	Year = {2009}}
	
	@inproceedings{johnson2014game,
	Author = {Johnson, B. and Laszka, A. and Grossklags, J. and Vasek, M. and Moore, T.},
	Booktitle = {Workshop on Bitcoin Research},
	Title = {{Game-theoretic Analysis of DDoS Attacks Against Bitcoin Mining Pools}},
	Year = {2014}}
	
	@incollection{laszka2013mitigation,
	Author = {Laszka, A. and Johnson, B. and Grossklags, J.},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {175--191},
	Publisher = {Springer},
	Title = {{Mitigation of Targeted and Non-targeted Covert Attacks as a Timing Game}},
	Year = {2013}}
	
	@inproceedings{schottle2013game,
	Author = {Schottle, P. and Laszka, A. and Johnson, B. and Grossklags, J. and Bohme, R.},
	Booktitle = {EUSIPCO},
	Title = {{A Game-theoretic Analysis of Content-adaptive Steganography with Independent Embedding}},
	Year = {2013}}
	
	@inproceedings{CloudTransport,
	Author = {C.~Brubaker and A.~Houmansadr and V.~Shmatikov},
	Booktitle = {PETS},
	Title = {{CloudTransport: Using Cloud Storage for Censorship-Resistant Networking}},
	Year = {2014}}
	
	@inproceedings{sweet,
	Author = {W.~Zhou and A.~Houmansadr and M.~Caesar and N.~Borisov},
	Booktitle = {HotPETs},
	Title = {{SWEET: Serving the Web by Exploiting Email Tunnels}},
	Year = {2013}}
	
	@inproceedings{ahsan2002practical,
	Author = {Ahsan, K. and Kundur, D.},
	Booktitle = {Workshop on Multimedia Security},
	Title = {{Practical data hiding in TCP/IP}},
	Year = {2002}}
	
	@incollection{danezis2011covert,
	Author = {Danezis, G.},
	Booktitle = {Security Protocols XVI},
	Pages = {198--214},
	Publisher = {Springer},
	Title = {{Covert Communications Despite Traffic Data Retention}},
	Year = {2011}}
	
	@inproceedings{liu2009hide,
	Author = {Liu, Y. and Ghosal, D. and Armknecht, F. and Sadeghi, A.-R. and Schulz, S. and Katzenbeisser, S.},
	Booktitle = {ESORICS},
	Title = {{Hide and Seek in Time---Robust Covert Timing Channels}},
	Year = {2009}}
	
	@misc{image-watermark-fing,
	Author = {Jonathan Bailey},
	Howpublished = {\url{https://www.plagiarismtoday.com/2009/12/02/image-detection-watermarking-vs-fingerprinting/}},
	Title = {{Image Detection: Watermarking vs. Fingerprinting}},
	Year = {2009}}
	
	@inproceedings{Servetto98,
	Author = {S. D. Servetto and C. I. Podilchuk and K. Ramchandran},
	Booktitle = {Int. Conf. Image Processing},
	Title = {Capacity issues in digital image watermarking},
	Year = {1998}}
	
	@inproceedings{Chen01,
	Author = {B. Chen and G.W.Wornell},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1423--1443},
	Title = {Quantization index modulation: A class of provably good methods for digital watermarking and information embedding},
	Year = {2001}}
	
	@inproceedings{Karakos00,
	Author = {D. Karakos and A. Papamarcou},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {47},
	Title = {Relationship between quantization and distribution rates of digitally watermarked data},
	Year = {2000}}
	
	@inproceedings{Sullivan98,
	Author = {J. A. OSullivan and P. Moulin and J. M. Ettinger},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {297},
	Title = {Information theoretic analysis of steganography},
	Year = {1998}}
	
	@inproceedings{Merhav00,
	Author = {N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {420--430},
	Title = {On random coding error exponents of watermarking systems},
	Year = {2000}}
	
	@inproceedings{Somekh01,
	Author = {A. Somekh-Baruch and N. Merhav},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {7},
	Title = {On the error exponent and capacity games of private watermarking systems},
	Year = {2001}}
	
	@inproceedings{Steinberg01,
	Author = {Y. Steinberg and N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1410--1422},
	Title = {Identification in the presence of side information with application to watermarking},
	Year = {2001}}
	
	@article{Moulin03,
	Author = {P. Moulin and J.A. O'Sullivan},
	Journal = {IEEE Trans. Info. Theory},
	Number = {3},
	Title = {Information-theoretic analysis of information hiding},
	Volume = 49,
	Year = 2003}
	
	@article{Gelfand80,
	Author = {S.I.~Gelfand and M.S.~Pinsker},
	Journal = {Problems of Control and Information Theory},
	Number = {1},
	Pages = {19-31},
	Title = {{Coding for channel with random parameters}},
	Url = {citeseer.ist.psu.edu/anantharam96bits.html},
	Volume = {9},
	Year = {1980},
	Bdsk-Url-1 = {citeseer.ist.psu.edu/anantharam96bits.html}}
	
	@book{Wolfowitz78,
	Author = {J. Wolfowitz},
	Edition = {3rd},
	Location = {New York},
	Publisher = {Springer-Verlag},
	Title = {Coding Theorems of Information Theory},
	Year = 1978}
	
	@article{caire99,
	Author = {G. Caire and S. Shamai},
	Journal = {IEEE Transactions on Information Theory},
	Number = {6},
	Pages = {2007--2019},
	Title = {On the Capacity of Some Channels with Channel State Information},
	Volume = {45},
	Year = {1999}}
	
	@inproceedings{wright2007language,
	Author = {Wright, Charles V and Ballard, Lucas and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {USENIX Security},
	Title = {{Language identification of encrypted VoIP traffic: Alejandra y Roberto or Alice and Bob?}},
	Year = {2007}}
	
	@inproceedings{backes2010speaker,
	Author = {Backes, Michael and Doychev, Goran and D{\"u}rmuth, Markus and K{\"o}pf, Boris},
	Booktitle = {{European Symposium on Research in Computer Security (ESORICS)}},
	Pages = {508--523},
	Publisher = {Springer},
	Title = {{Speaker Recognition in Encrypted Voice Streams}},
	Year = {2010}}
	
	@phdthesis{lu2009traffic,
	Author = {Lu, Yuanchao},
	School = {Cleveland State University},
	Title = {{On Traffic Analysis Attacks to Encrypted VoIP Calls}},
	Year = {2009}}
	
	@inproceedings{wright2008spot,
	Author = {Wright, Charles V and Ballard, Lucas and Coull, Scott E and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {35--49},
	Title = {Spot me if you can: Uncovering spoken phrases in encrypted VoIP conversations},
	Year = {2008}}
	
	@inproceedings{white2011phonotactic,
	Author = {White, Andrew M and Matthews, Austin R and Snow, Kevin Z and Monrose, Fabian},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {3--18},
	Title = {Phonotactic reconstruction of encrypted VoIP conversations: Hookt on fon-iks},
	Year = {2011}}
	
	@inproceedings{fancy,
	Author = {Houmansadr, Amir and Borisov, Nikita},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {205--224},
	Title = {The Need for Flow Fingerprints to Link Correlated Network Flows},
	Year = {2013}}
	
	@article{botmosaic,
	Author = {Amir Houmansadr and Nikita Borisov},
	Doi = {10.1016/j.jss.2012.11.005},
	Issn = {0164-1212},
	Journal = {Journal of Systems and Software},
	Keywords = {Network security},
	Number = {3},
	Pages = {707 - 715},
	Title = {BotMosaic: Collaborative network watermark for the detection of IRC-based botnets},
	Url = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Volume = {86},
	Year = {2013},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.jss.2012.11.005}}
	
	@inproceedings{ramsbrock2008first,
	Author = {Ramsbrock, Daniel and Wang, Xinyuan and Jiang, Xuxian},
	Booktitle = {Recent Advances in Intrusion Detection},
	Organization = {Springer},
	Pages = {59--77},
	Title = {A first step towards live botmaster traceback},
	Year = {2008}}
	
	@inproceedings{potdar2005survey,
	Author = {Potdar, Vidyasagar M and Han, Song and Chang, Elizabeth},
	Booktitle = {Industrial Informatics, 2005. INDIN'05. 2005 3rd IEEE International Conference on},
	Organization = {IEEE},
	Pages = {709--716},
	Title = {A survey of digital image watermarking techniques},
	Year = {2005}}
	
	@book{cole2003hiding,
	Author = {Cole, Eric and Krutz, Ronald D},
	Publisher = {John Wiley \& Sons, Inc.},
	Title = {Hiding in plain sight: Steganography and the art of covert communication},
	Year = {2003}}
	
	@incollection{akaike1998information,
	Author = {Akaike, Hirotogu},
	Booktitle = {Selected Papers of Hirotugu Akaike},
	Pages = {199--213},
	Publisher = {Springer},
	Title = {Information theory and an extension of the maximum likelihood principle},
	Year = {1998}}
	
	@misc{central-command-hack,
	Author = {Everett Rosenfeld},
	Howpublished = {\url{http://www.cnbc.com/id/102330338}},
	Title = {{FBI investigating Central Command Twitter hack}},
	Year = {2015}}
	
	@misc{sony-psp-ddos,
	Howpublished = {\url{http://n4g.com/news/1644853/sony-and-microsoft-cant-do-much-ddos-attacks-explained}},
	Key = {sony},
	Month = {December},
	Title = {{Sony and Microsoft cant do much -- DDoS attacks explained}},
	Year = {2014}}
	
	@misc{sony-hack,
	Author = {David Bloom},
	Howpublished = {\url{http://goo.gl/MwR4A7}},
	Title = {{Online Game Networks Hacked, Sony Unit President Threatened}},
	Year = {2014}}
	
	@misc{home-depot,
	Author = {Dune Lawrence},
	Howpublished = {\url{http://www.businessweek.com/articles/2014-09-02/home-depots-credit-card-breach-looks-just-like-the-target-hack}},
	Title = {{Home Depot's Suspected Breach Looks Just Like the Target Hack}},
	Year = {2014}}
	
	@misc{target,
	Author = {Julio Ojeda-Zapata},
	Howpublished = {\url{http://www.mercurynews.com/business/ci_24765398/how-did-hackers-pull-off-target-data-heist}},
	Title = {{Target hack: How did they do it?}},
	Year = {2014}}
	
	
	@article{probabilitycourse,
	Author = {H. Pishro-Nik},
	note = {\url{http://www.probabilitycourse.com}},
	Title = {Introduction to probability, statistics, and random processes},
	Year = {2014}}
	
	
	
	@inproceedings{shokri2011quantifying,
	Author = {Shokri, Reza and Theodorakopoulos, George and Le Boudec, Jean-Yves and Hubaux, Jean-Pierre},
	Booktitle = {Security and Privacy (SP), 2011 IEEE Symposium on},
	Organization = {IEEE},
	Pages = {247--262},
	Title = {Quantifying location privacy},
	Year = {2011}}
	
	@inproceedings{hoh2007preserving,
	Author = {Hoh, Baik and Gruteser, Marco and Xiong, Hui and Alrabady, Ansaf},
	Booktitle = {Proceedings of the 14th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {161--171},
	Title = {Preserving privacy in gps traces via uncertainty-aware path cloaking},
	Year = {2007}}
	
	
	
	@article{kafsi2013entropy,
	Author = {Kafsi, Mohamed and Grossglauser, Matthias and Thiran, Patrick},
	Journal = {Information Theory, IEEE Transactions on},
	Number = {9},
	Pages = {5577--5583},
	Publisher = {IEEE},
	Title = {The entropy of conditional Markov trajectories},
	Volume = {59},
	Year = {2013}}
	
	@inproceedings{gruteser2003anonymous,
	Author = {Gruteser, Marco and Grunwald, Dirk},
	Booktitle = {Proceedings of the 1st international conference on Mobile systems, applications and services},
	Organization = {ACM},
	Pages = {31--42},
	Title = {Anonymous usage of location-based services through spatial and temporal cloaking},
	Year = {2003}}
	
	@inproceedings{husted2010mobile,
	Author = {Husted, Nathaniel and Myers, Steven},
	Booktitle = {Proceedings of the 17th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {85--96},
	Title = {Mobile location tracking in metro areas: malnets and others},
	Year = {2010}}
	
	@inproceedings{li2009tradeoff,
	Author = {Li, Tiancheng and Li, Ninghui},
	Booktitle = {Proceedings of the 15th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {517--526},
	Title = {On the tradeoff between privacy and utility in data publishing},
	Year = {2009}}
	
	@inproceedings{ma2009location,
	Author = {Ma, Zhendong and Kargl, Frank and Weber, Michael},
	Booktitle = {Sarnoff Symposium, 2009. SARNOFF'09. IEEE},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {A location privacy metric for v2x communication systems},
	Year = {2009}}
	
	@inproceedings{shokri2012protecting,
	Author = {Shokri, Reza and Theodorakopoulos, George and Troncoso, Carmela and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
	Booktitle = {Proceedings of the 2012 ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {617--627},
	Title = {Protecting location privacy: optimal strategy against localization attacks},
	Year = {2012}}
	
	@inproceedings{freudiger2009non,
	Author = {Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
	Booktitle = {Proceedings of the 16th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {324--337},
	Title = {On non-cooperative location privacy: a game-theoretic analysis},
	Year = {2009}}
	
	@incollection{humbert2010tracking,
	Author = {Humbert, Mathias and Manshaei, Mohammad Hossein and Freudiger, Julien and Hubaux, Jean-Pierre},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {38--57},
	Publisher = {Springer},
	Title = {Tracking games in mobile networks},
	Year = {2010}}
	
	@article{manshaei2013game,
	Author = {Manshaei, Mohammad Hossein and Zhu, Quanyan and Alpcan, Tansu and Bac{\c{s}}ar, Tamer and Hubaux, Jean-Pierre},
	Journal = {ACM Computing Surveys (CSUR)},
	Number = {3},
	Pages = {25},
	Publisher = {ACM},
	Title = {Game theory meets network security and privacy},
	Volume = {45},
	Year = {2013}}
	
	@article{palamidessi2006probabilistic,
	Author = {Palamidessi, Catuscia},
	Journal = {Electronic Notes in Theoretical Computer Science},
	Pages = {33--42},
	Publisher = {Elsevier},
	Title = {Probabilistic and nondeterministic aspects of anonymity},
	Volume = {155},
	Year = {2006}}
	
	@inproceedings{mokbel2006new,
	Author = {Mokbel, Mohamed F and Chow, Chi-Yin and Aref, Walid G},
	Booktitle = {Proceedings of the 32nd international conference on Very large data bases},
	Organization = {VLDB Endowment},
	Pages = {763--774},
	Title = {The new Casper: query processing for location services without compromising privacy},
	Year = {2006}}
	
	@article{kalnis2007preventing,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {12},
	Pages = {1719--1733},
	Publisher = {IEEE},
	Title = {Preventing location-based identity inference in anonymous spatial queries},
	Volume = {19},
	Year = {2007}}
	
	@article{freudiger2007mix,
	title={Mix-zones for location privacy in vehicular networks},
	author={Freudiger, Julien and Raya, Maxim and F{\'e}legyh{\'a}zi, M{\'a}rk and Papadimitratos, Panos and Hubaux, Jean-Pierre},
	year={2007}
	}
	@article{sweeney2002k,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {557--570},
	Publisher = {World Scientific},
	Title = {k-anonymity: A model for protecting privacy},
	Volume = {10},
	Year = {2002}}
	
	@article{sweeney2002achieving,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {571--588},
	Publisher = {World Scientific},
	Title = {Achieving k-anonymity privacy protection using generalization and suppression},
	Volume = {10},
	Year = {2002}}
	
	@inproceedings{niu2014achieving,
	Author = {Niu, Ben and Li, Qinghua and Zhu, Xiaoyan and Cao, Guohong and Li, Hui},
	Booktitle = {INFOCOM, 2014 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {754--762},
	Title = {Achieving k-anonymity in privacy-aware location-based services},
	Year = {2014}}
	
	@inproceedings{liu2013game,
	Author = {Liu, Xinxin and Liu, Kaikai and Guo, Linke and Li, Xiaolin and Fang, Yuguang},
	Booktitle = {INFOCOM, 2013 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {2985--2993},
	Title = {A game-theoretic approach for achieving k-anonymity in location based services},
	Year = {2013}}
	
	@inproceedings{kido2005protection,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Data Engineering Workshops, 2005. 21st International Conference on},
	Organization = {IEEE},
	Pages = {1248--1248},
	Title = {Protection of location privacy using dummies for location-based services},
	Year = {2005}}
	
	@inproceedings{gedik2005location,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Booktitle = {Distributed Computing Systems, 2005. ICDCS 2005. Proceedings. 25th IEEE International Conference on},
	Organization = {IEEE},
	Pages = {620--629},
	Title = {Location privacy in mobile systems: A personalized anonymization model},
	Year = {2005}}
	
	@inproceedings{bordenabe2014optimal,
	Author = {Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2014 ACM SIGSAC Conference on Computer and Communications Security},
	Organization = {ACM},
	Pages = {251--262},
	Title = {Optimal geo-indistinguishable mechanisms for location privacy},
	Year = {2014}}
	
	@incollection{duckham2005formal,
	Author = {Duckham, Matt and Kulik, Lars},
	Booktitle = {Pervasive computing},
	Pages = {152--170},
	Publisher = {Springer},
	Title = {A formal model of obfuscation and negotiation for location privacy},
	Year = {2005}}
	
	@inproceedings{kido2005anonymous,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Pervasive Services, 2005. ICPS'05. Proceedings. International Conference on},
	Organization = {IEEE},
	Pages = {88--97},
	Title = {An anonymous communication technique using dummies for location-based services},
	Year = {2005}}
	
	@incollection{duckham2006spatiotemporal,
	Author = {Duckham, Matt and Kulik, Lars and Birtley, Athol},
	Booktitle = {Geographic Information Science},
	Pages = {47--64},
	Publisher = {Springer},
	Title = {A spatiotemporal model of strategies and counter strategies for location privacy protection},
	Year = {2006}}
	
	@inproceedings{shankar2009privately,
	Author = {Shankar, Pravin and Ganapathy, Vinod and Iftode, Liviu},
	Booktitle = {Proceedings of the 11th international conference on Ubiquitous computing},
	Organization = {ACM},
	Pages = {31--40},
	Title = {Privately querying location-based services with SybilQuery},
	Year = {2009}}
	
	@inproceedings{chow2009faking,
	Author = {Chow, Richard and Golle, Philippe},
	Booktitle = {Proceedings of the 8th ACM workshop on Privacy in the electronic society},
	Organization = {ACM},
	Pages = {105--108},
	Title = {Faking contextual data for fun, profit, and privacy},
	Year = {2009}}
	
	@incollection{xue2009location,
	Author = {Xue, Mingqiang and Kalnis, Panos and Pung, Hung Keng},
	Booktitle = {Location and Context Awareness},
	Pages = {70--87},
	Publisher = {Springer},
	Title = {Location diversity: Enhanced privacy protection in location based services},
	Year = {2009}}
	
	@article{wernke2014classification,
	Author = {Wernke, Marius and Skvortsov, Pavel and D{\"u}rr, Frank and Rothermel, Kurt},
	Journal = {Personal and Ubiquitous Computing},
	Number = {1},
	Pages = {163--175},
	Publisher = {Springer-Verlag},
	Title = {A classification of location privacy attacks and approaches},
	Volume = {18},
	Year = {2014}}
	
	@misc{cai2015cloaking,
	Author = {Cai, Y. and Xu, G.},
	Month = jan # {~1},
	Note = {US Patent App. 14/472,462},
	Publisher = {Google Patents},
	Title = {Cloaking with footprints to provide location privacy protection in location-based services},
	Url = {https://www.google.com/patents/US20150007341},
	Year = {2015},
	Bdsk-Url-1 = {https://www.google.com/patents/US20150007341}}
	
	@article{gedik2008protecting,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {1},
	Pages = {1--18},
	Publisher = {IEEE},
	Title = {Protecting location privacy with personalized k-anonymity: Architecture and algorithms},
	Volume = {7},
	Year = {2008}}
	
	@article{kalnis2006preserving,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Publisher = {TRB6/06},
	Title = {Preserving anonymity in location based services},
	Year = {2006}}
	
	@inproceedings{hoh2005protecting,
	Author = {Hoh, Baik and Gruteser, Marco},
	Booktitle = {Security and Privacy for Emerging Areas in Communications Networks, 2005. SecureComm 2005. First International Conference on},
	Organization = {IEEE},
	Pages = {194--205},
	Title = {Protecting location privacy through path confusion},
	Year = {2005}}
	
	@article{terrovitis2011privacy,
	Author = {Terrovitis, Manolis},
	Journal = {ACM SIGKDD Explorations Newsletter},
	Number = {1},
	Pages = {6--18},
	Publisher = {ACM},
	Title = {Privacy preservation in the dissemination of location data},
	Volume = {13},
	Year = {2011}}
	
	@article{shin2012privacy,
	Author = {Shin, Kang G and Ju, Xiaoen and Chen, Zhigang and Hu, Xin},
	Journal = {Wireless Communications, IEEE},
	Number = {1},
	Pages = {30--39},
	Publisher = {IEEE},
	Title = {Privacy protection for users of location-based services},
	Volume = {19},
	Year = {2012}}
	
	@article{khoshgozaran2011location,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus and Shirani-Mehr, Houtan},
	Journal = {Knowledge and Information Systems},
	Number = {3},
	Pages = {435--465},
	Publisher = {Springer},
	Title = {Location privacy: going beyond K-anonymity, cloaking and anonymizers},
	Volume = {26},
	Year = {2011}}
	
	@incollection{chatzikokolakis2015geo,
	Author = {Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
	Booktitle = {Distributed Computing and Internet Technology},
	Pages = {49--72},
	Publisher = {Springer},
	Title = {Geo-indistinguishability: A Principled Approach to Location Privacy},
	Year = {2015}}
	
	@inproceedings{ngo2015location,
	Author = {Ngo, Hoa and Kim, Jong},
	Booktitle = {Computer Security Foundations Symposium (CSF), 2015 IEEE 28th},
	Organization = {IEEE},
	Pages = {63--74},
	Title = {Location Privacy via Differential Private Perturbation of Cloaking Area},
	Year = {2015}}
	
	@inproceedings{palanisamy2011mobimix,
	Author = {Palanisamy, Balaji and Liu, Ling},
	Booktitle = {Data Engineering (ICDE), 2011 IEEE 27th International Conference on},
	Organization = {IEEE},
	Pages = {494--505},
	Title = {Mobimix: Protecting location privacy with mix-zones over road networks},
	Year = {2011}}
	
	@inproceedings{um2010advanced,
	Author = {Um, Jung-Ho and Kim, Hee-Dae and Chang, Jae-Woo},
	Booktitle = {Social Computing (SocialCom), 2010 IEEE Second International Conference on},
	Organization = {IEEE},
	Pages = {1093--1098},
	Title = {An advanced cloaking algorithm using Hilbert curves for anonymous location based service},
	Year = {2010}}
	
	@inproceedings{bamba2008supporting,
	Author = {Bamba, Bhuvan and Liu, Ling and Pesti, Peter and Wang, Ting},
	Booktitle = {Proceedings of the 17th international conference on World Wide Web},
	Organization = {ACM},
	Pages = {237--246},
	Title = {Supporting anonymous location queries in mobile environments with privacygrid},
	Year = {2008}}
	
	@inproceedings{zhangwei2010distributed,
	Author = {Zhangwei, Huang and Mingjun, Xin},
	Booktitle = {Networks Security Wireless Communications and Trusted Computing (NSWCTC), 2010 Second International Conference on},
	Organization = {IEEE},
	Pages = {468--471},
	Title = {A distributed spatial cloaking protocol for location privacy},
	Volume = {2},
	Year = {2010}}
	
	@article{chow2011spatial,
	Author = {Chow, Chi-Yin and Mokbel, Mohamed F and Liu, Xuan},
	Journal = {GeoInformatica},
	Number = {2},
	Pages = {351--380},
	Publisher = {Springer},
	Title = {Spatial cloaking for anonymous location-based services in mobile peer-to-peer environments},
	Volume = {15},
	Year = {2011}}
	
	@inproceedings{lu2008pad,
	Author = {Lu, Hua and Jensen, Christian S and Yiu, Man Lung},
	Booktitle = {Proceedings of the Seventh ACM International Workshop on Data Engineering for Wireless and Mobile Access},
	Organization = {ACM},
	Pages = {16--23},
	Title = {Pad: privacy-area aware, dummy-based location privacy in mobile services},
	Year = {2008}}
	
	@incollection{khoshgozaran2007blind,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus},
	Booktitle = {Advances in Spatial and Temporal Databases},
	Pages = {239--257},
	Publisher = {Springer},
	Title = {Blind evaluation of nearest neighbor queries using space transformation to preserve location privacy},
	Year = {2007}}
	
	@inproceedings{ghinita2008private,
	Author = {Ghinita, Gabriel and Kalnis, Panos and Khoshgozaran, Ali and Shahabi, Cyrus and Tan, Kian-Lee},
	Booktitle = {Proceedings of the 2008 ACM SIGMOD international conference on Management of data},
	Organization = {ACM},
	Pages = {121--132},
	Title = {Private queries in location based services: anonymizers are not necessary},
	Year = {2008}}
	
	@article{paulet2014privacy,
	Author = {Paulet, Russell and Kaosar, Md Golam and Yi, Xun and Bertino, Elisa},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {5},
	Pages = {1200--1210},
	Publisher = {IEEE},
	Title = {Privacy-preserving and content-protecting location based queries},
	Volume = {26},
	Year = {2014}}
	
	@article{nguyen2013differential,
	Author = {Nguyen, Hiep H and Kim, Jong and Kim, Yoonho},
	Journal = {Journal of Computing Science and Engineering},
	Number = {3},
	Pages = {177--186},
	Title = {Differential privacy in practice},
	Volume = {7},
	Year = {2013}}
	
	@inproceedings{lee2012differential,
	Author = {Lee, Jaewoo and Clifton, Chris},
	Booktitle = {Proceedings of the 18th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {1041--1049},
	Title = {Differential identifiability},
	Year = {2012}}
	
	@inproceedings{andres2013geo,
	Author = {Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2013 ACM SIGSAC conference on Computer \& communications security},
	Organization = {ACM},
	Pages = {901--914},
	Title = {Geo-indistinguishability: Differential privacy for location-based systems},
	Year = {2013}}
	
	@inproceedings{machanavajjhala2008privacy,
	Author = {Machanavajjhala, Ashwin and Kifer, Daniel and Abowd, John and Gehrke, Johannes and Vilhuber, Lars},
	Booktitle = {Data Engineering, 2008. ICDE 2008. IEEE 24th International Conference on},
	Organization = {IEEE},
	Pages = {277--286},
	Title = {Privacy: Theory meets practice on the map},
	Year = {2008}}
	
	@article{dewri2013local,
	Author = {Dewri, Rinku},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {12},
	Pages = {2360--2372},
	Publisher = {IEEE},
	Title = {Local differential perturbations: Location privacy under approximate knowledge attackers},
	Volume = {12},
	Year = {2013}}
	
	@inproceedings{chatzikokolakis2013broadening,
	Author = {Chatzikokolakis, Konstantinos and Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s Emilio and Palamidessi, Catuscia},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {82--102},
	Title = {Broadening the Scope of Differential Privacy Using Metrics.},
	Year = {2013}}
	
	@inproceedings{zhong2009distributed,
	Author = {Zhong, Ge and Hengartner, Urs},
	Booktitle = {Pervasive Computing and Communications, 2009. PerCom 2009. IEEE International Conference on},
	Organization = {IEEE},
	Pages = {1--10},
	Title = {A distributed k-anonymity protocol for location privacy},
	Year = {2009}}
	
	@inproceedings{ho2011differential,
	Author = {Ho, Shen-Shyang and Ruan, Shuhua},
	Booktitle = {Proceedings of the 4th ACM SIGSPATIAL International Workshop on Security and Privacy in GIS and LBS},
	Organization = {ACM},
	Pages = {17--24},
	Title = {Differential privacy for location pattern mining},
	Year = {2011}}
	
	@inproceedings{cheng2006preserving,
	Author = {Cheng, Reynold and Zhang, Yu and Bertino, Elisa and Prabhakar, Sunil},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {393--412},
	Title = {Preserving user location privacy in mobile data management infrastructures},
	Year = {2006}}
	
	@article{beresford2003location,
	Author = {Beresford, Alastair R and Stajano, Frank},
	Journal = {IEEE Pervasive computing},
	Number = {1},
	Pages = {46--55},
	Publisher = {IEEE},
	Title = {Location privacy in pervasive computing},
	Year = {2003}}
	
	@inproceedings{freudiger2009optimal,
	Author = {Freudiger, Julien and Shokri, Reza and Hubaux, Jean-Pierre},
	Booktitle = {Privacy enhancing technologies},
	Organization = {Springer},
	Pages = {216--234},
	Title = {On the optimal placement of mix zones},
	Year = {2009}}
	
	@article{krumm2009survey,
	Author = {Krumm, John},
	Journal = {Personal and Ubiquitous Computing},
	Number = {6},
	Pages = {391--399},
	Publisher = {Springer},
	Title = {A survey of computational location privacy},
	Volume = {13},
	Year = {2009}}
	
	@article{Rakhshan2016letter,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Wireless Communications Letter},
	Publisher = {IEEE},
	Title = {Interference Models for Vehicular Ad Hoc Networks},
	Year = {2016, submitted}}
	
	@article{Rakhshan2015Journal,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Publisher = {IEEE},
	Title = {Improving Safety on Highways by Customizing Vehicular Ad Hoc Networks},
	Year = {to appear, 2017}}
	
	@inproceedings{Rakhshan2015Cogsima,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Booktitle = {IEEE International Multi-Disciplinary Conference on Cognitive Methods in Situation Awareness and Decision Support},
	Organization = {IEEE},
	Title = {A New Approach to Customization of Accident Warning Systems to Individual Drivers},
	Year = {2015}}
	
	@inproceedings{Rakhshan2015CISS,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Nekoui, Mohammad},
	Booktitle = {Conference on Information Sciences and Systems},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {Driver-based adaptation of Vehicular Ad Hoc Networks for design of active safety systems},
	Year = {2015}}
	
	@inproceedings{Rakhshan2014IV,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Ray, Evan},
	Booktitle = {Intelligent Vehicles Symposium},
	Organization = {IEEE},
	Pages = {1181--1186},
	Title = {Real-time estimation of the distribution of brake response times for an individual driver using Vehicular Ad Hoc Network.},
	Year = {2014}}
	
	@inproceedings{Rakhshan2013Globecom,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Fisher, Donald and Nekoui, Mohammad},
	Booktitle = {IEEE Global Communications Conference},
	Organization = {IEEE},
	Pages = {1333--1337},
	Title = {Tuning collision warning algorithms to individual drivers for design of active safety systems.},
	Year = {2013}}
	
	@article{Nekoui2012Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Number = {8},
	Pages = {2895--2905},
	Publisher = {IEEE},
	Title = {Throughput Scaling laws for Vehicular Ad Hoc Networks},
	Volume = {11},
	Year = {2012}}
	
	
	
	
	
	
	
	
	
	@article{Nekoui2011Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein and Ni, Daiheng},
	Journal = {International Journal of Vehicular Technology},
	Pages = {1--11},
	Publisher = {Hindawi Publishing Corporation},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {2011},
	Year = {2011}}
	
	
	
	
	
	
	@article{shokri2014optimal,
	title={Optimal user-centric data obfuscation},
	author={Shokri, Reza},
	journal={arXiv preprint arXiv:1402.3426},
	year={2014}
	}
	@article{chatzikokolakis2015location,
	title={Location privacy via geo-indistinguishability},
	author={Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
	journal={ACM SIGLOG News},
	volume={2},
	number={3},
	pages={46--69},
	year={2015},
	publisher={ACM}
	
	}
	@inproceedings{shokri2011quantifying2,
	title={Quantifying location privacy: the case of sporadic location exposure},
	author={Shokri, Reza and Theodorakopoulos, George and Danezis, George and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
	booktitle={Privacy Enhancing Technologies},
	pages={57--76},
	year={2011},
	organization={Springer}
	}
	
	
	@inproceedings{Mont1603:Defining,
	AUTHOR="Zarrin Montazeri and Amir Houmansadr and Hossein Pishro-Nik",
	TITLE="Defining Perfect Location Privacy Using Anonymization",
	BOOKTITLE="2016 Annual Conference on Information Science and Systems (CISS) (CISS
	2016)",
	ADDRESS="Princeton, USA",
	DAYS=16,
	MONTH=mar,
	YEAR=2016,
	KEYWORDS="Information Theoretic Privacy; location-based services; Location Privacy;
	Information Theory",
	ABSTRACT="The popularity of mobile devices and location-based services (LBS) have
	created great concerns regarding the location privacy of users of such
	devices and services. Anonymization is a common technique that is often
	being used to protect the location privacy of LBS users. In this paper, we
	provide a general information theoretic definition for location privacy. In
	particular, we define perfect location privacy. We show that under certain
	conditions, perfect privacy is achieved if the pseudonyms of users is
	changed after o(N^(2/r?1)) observations by the adversary, where N is the
	number of users and r is the number of sub-regions or locations.
	"
	}
	@article{our-isita-location,
	Author = {Zarrin Montazeri and Amir Houmansadr and Hossein Pishro-Nik},
	Journal = {IEEE International Symposium on Information Theory and Its Applications (ISITA)},
	Title = {Achieving Perfect Location Privacy in Markov Models Using Anonymization},
	Year = {2016}
	}
	@article{our-TIFS,
	Author = {Zarrin Montazeri and Hossein Pishro-Nik and Amir Houmansadr},
	Journal = {IEEE Transactions on Information Forensics and Security, under revison},
	Title = {Perfect Location Privacy Using Anonymization in Mobile Networks},
	Year = {2016},
	note={Available on arxiv.org}
	}
	
	
	
	@techreport{sampigethaya2005caravan,
	title={CARAVAN: Providing location privacy for VANET},
	author={Sampigethaya, Krishna and Huang, Leping and Li, Mingyan and Poovendran, Radha and Matsuura, Kanta and Sezaki, Kaoru},
	year={2005},
	institution={DTIC Document}
	}
	@incollection{buttyan2007effectiveness,
	title={On the effectiveness of changing pseudonyms to provide location privacy in VANETs},
	author={Butty{\'a}n, Levente and Holczer, Tam{\'a}s and Vajda, Istv{\'a}n},
	booktitle={Security and Privacy in Ad-hoc and Sensor Networks},
	pages={129--141},
	year={2007},
	publisher={Springer}
	}
	@article{sampigethaya2007amoeba,
	title={AMOEBA: Robust location privacy scheme for VANET},
	author={Sampigethaya, Krishna and Li, Mingyan and Huang, Leping and Poovendran, Radha},
	journal={Selected Areas in communications, IEEE Journal on},
	volume={25},
	number={8},
	pages={1569--1589},
	year={2007},
	publisher={IEEE}
	}
	
	@article{lu2012pseudonym,
	title={Pseudonym changing at social spots: An effective strategy for location privacy in vanets},
	author={Lu, Rongxing and Li, Xiaodong and Luan, Tom H and Liang, Xiaohui and Shen, Xuemin},
	journal={Vehicular Technology, IEEE Transactions on},
	volume={61},
	number={1},
	pages={86--96},
	year={2012},
	publisher={IEEE}
	}
	@inproceedings{lu2010sacrificing,
	title={Sacrificing the plum tree for the peach tree: A socialspot tactic for protecting receiver-location privacy in VANET},
	author={Lu, Rongxing and Lin, Xiaodong and Liang, Xiaohui and Shen, Xuemin},
	booktitle={Global Telecommunications Conference (GLOBECOM 2010), 2010 IEEE},
	pages={1--5},
	year={2010},
	organization={IEEE}
	}
	@inproceedings{lin2011stap,
	title={STAP: A social-tier-assisted packet forwarding protocol for achieving receiver-location privacy preservation in VANETs},
	author={Lin, Xiaodong and Lu, Rongxing and Liang, Xiaohui and Shen, Xuemin Sherman},
	booktitle={INFOCOM, 2011 Proceedings IEEE},
	pages={2147--2155},
	year={2011},
	organization={IEEE}
	}
	@inproceedings{gerlach2007privacy,
	title={Privacy in VANETs using changing pseudonyms-ideal and real},
	author={Gerlach, Matthias and Guttler, Felix},
	booktitle={Vehicular Technology Conference, 2007. VTC2007-Spring. IEEE 65th},
	pages={2521--2525},
	year={2007},
	organization={IEEE}
	}
	@inproceedings{el2002security,
	title={Security issues in a future vehicular network},
	author={El Zarki, Magda and Mehrotra, Sharad and Tsudik, Gene and Venkatasubramanian, Nalini},
	booktitle={European Wireless},
	volume={2},
	year={2002}
	}
	
	@article{hubaux2004security,
	title={The security and privacy of smart vehicles},
	author={Hubaux, Jean-Pierre and Capkun, Srdjan and Luo, Jun},
	journal={IEEE Security \& Privacy Magazine},
	volume={2},
	number={LCA-ARTICLE-2004-007},
	pages={49--55},
	year={2004}
	}
	
	
	
	@inproceedings{duri2002framework,
	title={Framework for security and privacy in automotive telematics},
	author={Duri, Sastry and Gruteser, Marco and Liu, Xuan and Moskowitz, Paul and Perez, Ronald and Singh, Moninder and Tang, Jung-Mu},
	booktitle={Proceedings of the 2nd international workshop on Mobile commerce},
	pages={25--32},
	year={2002},
	organization={ACM}
	}
	@misc{NS-3,
	Howpublished = {\url{https://www.nsnam.org/}}},
}
@misc{testbed,
	Howpublished = {\url{http://www.its.dot.gov/testbed/PDF/SE-MI-Resource-Guide-9-3-1.pdf}}},
@misc{NGSIM,
	Howpublished = {\url{http://ops.fhwa.dot.gov/trafficanalysistools/ngsim.htm}},
}

@misc{National-a2013,
	Author = {National Highway Traffic Safety Administration},
	Howpublished = {\url{http://ops.fhwa.dot.gov/trafficanalysistools/ngsim.htm}},
	Title = {2013 Motor Vehicle Crashes: Overview. Traffic Safety Factors},
	Year = {2013}
}

@inproceedings{karnadi2007rapid,
	title={Rapid generation of realistic mobility models for VANET},
	author={Karnadi, Feliz Kristianto and Mo, Zhi Hai and Lan, Kun-chan},
	booktitle={Wireless Communications and Networking Conference, 2007. WCNC 2007. IEEE},
	pages={2506--2511},
	year={2007},
	organization={IEEE}
}
@inproceedings{saha2004modeling,
	title={Modeling mobility for vehicular ad-hoc networks},
	author={Saha, Amit Kumar and Johnson, David B},
	booktitle={Proceedings of the 1st ACM international workshop on Vehicular ad hoc networks},
	pages={91--92},
	year={2004},
	organization={ACM}
}
@inproceedings{lee2006modeling,
	title={Modeling steady-state and transient behaviors of user mobility: formulation, analysis, and application},
	author={Lee, Jong-Kwon and Hou, Jennifer C},
	booktitle={Proceedings of the 7th ACM international symposium on Mobile ad hoc networking and computing},
	pages={85--96},
	year={2006},
	organization={ACM}
}
@inproceedings{yoon2006building,
	title={Building realistic mobility models from coarse-grained traces},
	author={Yoon, Jungkeun and Noble, Brian D and Liu, Mingyan and Kim, Minkyong},
	booktitle={Proceedings of the 4th international conference on Mobile systems, applications and services},
	pages={177--190},
	year={2006},
	organization={ACM}
}

@inproceedings{choffnes2005integrated,
	title={An integrated mobility and traffic model for vehicular wireless networks},
	author={Choffnes, David R and Bustamante, Fabi{\'a}n E},
	booktitle={Proceedings of the 2nd ACM international workshop on Vehicular ad hoc networks},
	pages={69--78},
	year={2005},
	organization={ACM}
}

@inproceedings{Qian2008Globecom,
	title={CA Secure VANET MAC Protocol for DSRC Applications},
	author={Yi, Q. and Lu, K. and Moyeri, N.{\'a}n E},
	booktitle={Proceedings of IEEE GLOBECOM 2008},
	pages={1--5},
	year={2008},
	organization={IEEE}
}





@inproceedings{naumov2006evaluation,
	title={An evaluation of inter-vehicle ad hoc networks based on realistic vehicular traces},
	author={Naumov, Valery and Baumann, Rainer and Gross, Thomas},
	booktitle={Proceedings of the 7th ACM international symposium on Mobile ad hoc networking and computing},
	pages={108--119},
	year={2006},
	organization={ACM}
}
@article{sommer2008progressing,
	title={Progressing toward realistic mobility models in VANET simulations},
	author={Sommer, Christoph and Dressler, Falko},
	journal={Communications Magazine, IEEE},
	volume={46},
	number={11},
	pages={132--137},
	year={2008},
	publisher={IEEE}
}




@inproceedings{mahajan2006urban,
	title={Urban mobility models for vanets},
	author={Mahajan, Atulya and Potnis, Niranjan and Gopalan, Kartik and Wang, Andy},
	booktitle={2nd IEEE International Workshop on Next Generation Wireless Networks},
	volume={33},
	year={2006}
}

@inproceedings{Rakhshan2016packet,
	title={Packet success probability derivation in a vehicular ad hoc network for a highway scenario},
	author={Rakhshan, Ali and Pishro-Nik, Hossein},
	booktitle={2016 Annual Conference on Information Science and Systems (CISS)},
	pages={210--215},
	year={2016},
	organization={IEEE}
}

@inproceedings{Rakhshan2016CISS,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Booktitle = {Conference on Information Sciences and Systems},
	Organization = {IEEE},
	Pages = {210--215},
	Title = {Packet Success Probability Derivation in a Vehicular Ad Hoc Network for a Highway Scenario},
	Year = {2016}}

@article{Nekoui2013Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {Journal on Selected Areas in Communications, Special Issue on Emerging Technologies in Communications},
	Number = {9},
	Pages = {491--503},
	Publisher = {IEEE},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {31},
	Year = {2013}}


@inproceedings{Nekoui2011MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM workshop on VehiculAr InterNETworking},
	Organization = {ACM},
	Title = {Analytic Design of Active Vehicular Safety Systems in Sparse Traffic},
	Year = {2011}}

@inproceedings{Nekoui2011VTC,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Analytical Design of Inter-vehicular Communications for Collision Avoidance},
	Year = {2011}}

@inproceedings{Bovee2011VTC,
	Author = {Bovee, Ben Louis and Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Evaluation of the Universal Geocast Scheme For VANETs},
	Year = {2011}}

@inproceedings{Nekoui2010MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM},
	Organization = {ACM},
	Title = {Fundamental Tradeoffs in Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2010IVCS,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IVCS},
	Organization = {IEEE},
	Title = {A Universal Geocast Scheme for Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2009ITW,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IEEE Communications Society Conference on Sensor, Mesh and Ad Hoc Communications and Networks Workshops},
	Organization = {IEEE},
	Pages = {1--3},
	Title = {A Geometrical Analysis of Obstructed Wireless Networks},
	Year = {2009}}

@article{Eslami2013Journal,
	Author = {Eslami, Ali and Nekoui, Mohammad and Pishro-Nik, Hossein and Fekri, Faramarz},
	Journal = {ACM Transactions on Sensor Networks},
	Number = {4},
	Pages = {51},
	Publisher = {ACM},
	Title = {Results on finite wireless sensor networks: Connectivity and coverage},
	Volume = {9},
	Year = {2013}}


@article{Jiafu2014Journal,
	Author = {Jiafu, W. and Zhang, D. and Zhao, S. and Yang, L. and Lloret, J.},
	Journal = {Communications Magazine},
	Number = {8},
	Pages = {106-113},
	Publisher = {IEEE},
	Title = {Context-aware vehicular cyber-physical systems with cloud support: architecture, challenges, and solutions},
	Volume = {52},
	Year = {2014}}

@inproceedings{Haas2010ACM,
	Author = {Haas, J.J. and Hu, Y.},
	Booktitle = {international workshop on VehiculAr InterNETworking},
	Organization = {ACM},
	Title = {Communication requirements for crash avoidance.},
	Year = {2010}}

@inproceedings{Yi2008GLOBECOM,
	Author = {Yi, Q. and Lu, K. and Moayeri, N.},
	Booktitle = {GLOBECOM},
	Organization = {IEEE},
	Title = {CA Secure VANET MAC Protocol for DSRC Applications.},
	Year = {2008}}

@inproceedings{Mughal2010ITSim,
	Author = {Mughal, B.M. and Wagan, A. and Hasbullah, H.},
	Booktitle = {International Symposium on Information Technology (ITSim)},
	Organization = {IEEE},
	Title = {Efficient congestion control in VANET for safety messaging.},
	Year = {2010}}

@article{Chang2011Journal,
	Author = {Chang, Y. and Lee, C. and Copeland, J.},
	Journal = {Selected Areas in Communications},
	Pages = {236 â€“249},
	Publisher = {IEEE},
	Title = {Goodput enhancement of VANETs in noisy CSMA/CA channels},
	Volume = {29},
	Year = {2011}}

@article{Garcia-Costa2011Journal,
	Author = {Garcia-Costa, C. and Egea-Lopez, E. and Tomas-Gabarron, J. B. and Garcia-Haro, J. and Haas, Z. J.},
	Journal = {Transactions on Intelligent Transportation Systems},
	Pages = {1 â€“16},
	Publisher = {IEEE},
	Title = {A stochastic model for chain collisions of vehicles equipped with vehicular communications},
	Volume = {99},
	Year = {2011}}

@article{Carbaugh2011Journal,
	Author = {Carbaugh, J. and Godbole,  D. N. and Sengupta, R. and Garcia-Haro, J. and Haas, Z. J.},
	Publisher = {Transportation Research Part C (Emerging Technologies)},
	Title = {Safety and capacity analysis of automated and manual highway systems},
	Year = {1997}}

@article{Goh2004Journal,
	Author = {Goh, P. and Wong, Y.},
	Publisher = {Appl Health Econ Health Policy},
	Title = {Driver perception response time during the signal change interval},
	Year = {2004}}

@article{Chang1985Journal,
	Author = {Chang, M.S. and Santiago, A.J.},
	Pages = {20-30},
	Publisher = {Transportation Research Record},
	Title = {Timing traffic signal changes based on driver behavior},
	Volume = {1027},
	Year = {1985}}

@article{Green2000Journal,
	Author = {Green, M.},
	Pages = {195-216},
	Publisher = {Transportation Human Factors},
	Title = {How long does it take to stop? Methodological analysis of driver perception-brake times.},
	Year = {2000}}

@article{Koppa2005,
	Author = {Koppa, R.J.},
	Pages = {195-216},
	Publisher = {http://www.fhwa.dot.gov/publications/},
	Title = {Human Factors},
	Year = {2005}}

@inproceedings{Maxwell2010ETC,
	Author = {Maxwell, A. and Wood, K.},
	Booktitle = {Europian Transport Conference},
	Organization = {http://www.etcproceedings.org/paper/review-of-traffic-signals-on-high-speed-roads},
	Title = {Review of Traffic Signals on High Speed Road},
	Year = {2010}}

@article{Wortman1983,
	Author = {Wortman, R.H. and Matthias, J.S.},
	Publisher = {Arizona Department of Transportation},
	Title = {An Evaluation of Driver Behavior at Signalized Intersections},
	Year = {1983}}
@inproceedings{Zhang2007IASTED,
	Author = {Zhang, X. and Bham, G.H.},
	Booktitle = {18th IASTED International Conference: modeling and simulation},
	Title = {Estimation of driver reaction time from detailed vehicle trajectory data.},
	Year = {2007}}


@inproceedings{bai2003important,
	title={IMPORTANT: A framework to systematically analyze the Impact of Mobility on Performance of RouTing protocols for Adhoc NeTworks},
	author={Bai, Fan and Sadagopan, Narayanan and Helmy, Ahmed},
	booktitle={INFOCOM 2003. Twenty-second annual joint conference of the IEEE computer and communications. IEEE societies},
	volume={2},
	pages={825--835},
	year={2003},
	organization={IEEE}
}


@inproceedings{abedi2008enhancing,
	title={Enhancing AODV routing protocol using mobility parameters in VANET},
	author={Abedi, Omid and Fathy, Mahmood and Taghiloo, Jamshid},
	booktitle={Computer Systems and Applications, 2008. AICCSA 2008. IEEE/ACS International Conference on},
	pages={229--235},
	year={2008},
	organization={IEEE}
}


@article{AlSultan2013Journal,
	Author = {Al-Sultan, Saif and Al-Bayatti, Ali H. and Zedan, Hussien},
	Journal = {IEEE Transactions on Vehicular Technology},
	Number = {9},
	Pages = {4264-4275},
	Publisher = {IEEE},
	Title = {Context Aware Driver Behaviour Detection System in Intelligent Transportation Systems},
	Volume = {62},
	Year = {2013}}






@article{Leow2008ITS,
	Author = {Leow, Woei Ling and Ni, Daiheng and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Intelligent Transportation Systems},
	Number = {2},
	Pages = {369--374},
	Publisher = {IEEE},
	Title = {A Sampling Theorem Approach to Traffic Sensor Optimization},
	Volume = {9},
	Year = {2008}}



@article{REU2007,
	Author = {D. Ni and H. Pishro-Nik and R. Prasad and M. R. Kanjee and H. Zhu and T. Nguyen},
	Journal = {in 14th World Congress on Intelligent Transport Systems},
	Title = {Development of a prototype intersection collision avoidance system under VII},
	Year = {2007}}




@inproceedings{salamatian2013hide,
	title={How to hide the elephant-or the donkey-in the room: Practical privacy against statistical inference for large data.},
	author={Salamatian, Salman and Zhang, Amy and du Pin Calmon, Flavio and Bhamidipati, Sandilya and Fawaz, Nadia and Kveton, Branislav and Oliveira, Pedro and Taft, Nina},
	booktitle={GlobalSIP},
	pages={269--272},
	year={2013}
}

@article{sankar2013utility,
	title={Utility-privacy tradeoffs in databases: An information-theoretic approach},
	author={Sankar, Lalitha and Rajagopalan, S Raj and Poor, H Vincent},
	journal={Information Forensics and Security, IEEE Transactions on},
	volume={8},
	number={6},
	pages={838--852},
	year={2013},
	publisher={IEEE}
}
@inproceedings{ghinita2007prive,
	title={PRIVE: anonymous location-based queries in distributed mobile systems},
	author={Ghinita, Gabriel and Kalnis, Panos and Skiadopoulos, Spiros},
	booktitle={Proceedings of the 16th international conference on World Wide Web},
	pages={371--380},
	year={2007},
	organization={ACM}
}

@article{beresford2004mix,
	title={Mix zones: User privacy in location-aware services},
	author={Beresford, Alastair R and Stajano, Frank},
	year={2004},
	publisher={IEEE}
}

%@inproceedings{Mont1610Achieving,
	%  title={Achieving Perfect Location Privacy in Markov Models Using Anonymization},
	%  author={Montazeri, Zarrin and Houmansadr, Amir and H.Pishro-Nik},
	%  booktitle="2016 International Symposium on Information Theory and its Applications
	%  (ISITA2016)",
	%  address="Monterey, USA",
	%  days=30,
	%  month=oct,
	%  year=2016,
	%}

@article{csiszar1996almost,
	title={Almost independence and secrecy capacity},
	author={Csisz{\'a}r, Imre},
	journal={Problemy Peredachi Informatsii},
	volume={32},
	number={1},
	pages={48--57},
	year={1996},
	publisher={Russian Academy of Sciences, Branch of Informatics, Computer Equipment and Automatization}
}

@article{yamamoto1983source,
	title={A source coding problem for sources with additional outputs to keep secret from the receiver or wiretappers (corresp.)},
	author={Yamamoto, Hirosuke},
	journal={IEEE Transactions on Information Theory},
	volume={29},
	number={6},
	pages={918--923},
	year={1983},
	publisher={IEEE}
}


@inproceedings{calmon2015fundamental,
	title={Fundamental limits of perfect privacy},
	author={Calmon, Flavio P and Makhdoumi, Ali and M{\'e}dard, Muriel},
	booktitle={Information Theory (ISIT), 2015 IEEE International Symposium on},
	pages={1796--1800},
	year={2015},
	organization={IEEE}
}



@inproceedings{Lehman1999Large-Sample-Theory,
	title={Elements of Large Sample Theory},
	author={E. L. Lehman},
	organization={Springer},
	year={1999}
}


@inproceedings{Ferguson1999Large-Sample-Theory,
	title={A Course in Large Sample Theory},
	author={Thomas S. Ferguson},
	organization={CRC Press},
	year={1996}
}



@inproceedings{Dembo1999Large-Deviations,
	title={Large Deviation Techniques and Applications, Second Edition},
	author={A. Dembo and O. Zeitouni},
	organization={Springer},
	year={1998}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Hossein's Coding Journals
%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{myoptics,
	AUTHOR =       "H. Pishro-Nik and N. Rahnavard and J. Ha and F. Fekri and A. Adibi ",
	TITLE =        "Low-density parity-check codes for volume holographic memory systems",
	JOURNAL =      " Appl. Opt.",
	YEAR =         "2003",
	volume =       "42",
	pages =        "861-870  "
}






@ARTICLE{myit,
	AUTHOR =       "H. Pishro-Nik and F. Fekri  ",
	TITLE =        "On Decoding of Low-Density Parity-Check Codes on the Binary Erasure Channel",
	JOURNAL =      "IEEE Trans. Inform. Theory",
	YEAR =         "2004",
	volume =       "50",
	pages =        "439--454"
}




@ARTICLE{myitpuncture,
	AUTHOR =       "H. Pishro-Nik and F. Fekri  ",
	TITLE =        "Results on Punctured Low-Density Parity-Check Codes and Improved Iterative Decoding Techniques",
	JOURNAL =      "IEEE Trans. on Inform. Theory",
	YEAR =         "2007",
	volume =       "53",
	number=        "2",
	pages =        "599--614",
	month= "February"
}




@ARTICLE{myitlinmimdist,
	AUTHOR =       "H. Pishro-Nik and F. Fekri",
	TITLE =        "Performance of Low-Density Parity-Check Codes With Linear Minimum Distance",
	JOURNAL =         "IEEE Trans. Inform. Theory ",
	YEAR =         "2006",
	volume =       "52",
	number="1",
	pages =        "292 --300"
}






@ARTICLE{myitnonuni,
	AUTHOR =       "H. Pishro-Nik and N. Rahnavard and F. Fekri  ",
	TITLE =        "Non-uniform Error Correction Using Low-Density Parity-Check Codes",
	JOURNAL =      "IEEE Trans. Inform. Theory",
	YEAR =         "2005",
	volume =       "51",
	number=  "7",
	pages =        "2702--2714"
}





@article{eslamitcomhybrid10,
	author = {A. Eslami and S. Vangala and H. Pishro-Nik},
	title = {Hybrid channel codes for highly efficient FSO/RF communication systems},
	journal = {IEEE Transactions on Communications},
	volume = {58},
	number = {10},
	year = {2010},
	pages = {2926--2938},
}


@article{eslamitcompolar13,
	author = {A. Eslami and H. Pishro-Nik},
	title = {On Finite-Length Performance of Polar Codes: Stopping Sets, Error Floor, and Concatenated Design},
	journal = {IEEE Transactions on Communications},
	volume = {61},
	number = {13},
	year = {2013},
	pages = {919--929},
}



@article{saeeditcom11,
	author = {H. Saeedi and H. Pishro-Nik and  A. H. Banihashemi},
	title = {Successive maximization for the systematic design of universally capacity approaching rate-compatible
	sequences of LDPC code ensembles over binary-input output-symmetric memoryless channels},
	journal = {IEEE Transactions on Communications},
	year = {2011},
	volume={59},
	number = {7}
}


@article{rahnavard07,
	author = {Rahnavard, N. and Pishro-Nik, H. and Fekri, F.},
	title = {Unequal Error Protection Using Partially Regular LDPC Codes},
	journal = {IEEE Transactions on Communications},
	year = {2007},
	volume = {55},
	number = {3},
	pages = {387 -- 391}
}


@article{hosseinira04,
	author = {H. Pishro-Nik and F. Fekri},
	title = {Irregular repeat-accumulate codes for volume holographic memory systems},
	journal = {Journal of Applied Optics},
	year = {2004},
	volume = {43},
	number = {27},
	pages = {5222--5227},
}


@article{azadeh2015Ephemeralkey,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
	journal = {IEEE Transactions on Wireless Communications},
	year = {2015},
	volume = {14},
	number = {11},
	pages = {6072--6081},
}


@article{azadeh2014Everlasting,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Everlasting secrecy in disadvantaged wireless environments against sophisticated eavesdroppers},
	journal = {48th Asilomar Conference on Signals, Systems and Computers},
	year = {2014},
	pages = {1994--1998},
}


@article{azadeh2013ISIT,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Artificial intersymbol interference (ISI) to exploit receiver imperfections for secrecy},
	journal = {IEEE International Symposium on Information Theory (ISIT)},
	year = {2013},
}


@article{azadeh2013Jsac,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
	journal = {IEEE Journal on Selected Areas in Communications},
	year = {2013},
	volume = {31},
	number = {9},
	pages = {1828--1839},
}


@article{azadeh2012Allerton,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Exploiting the non-commutativity of nonlinear operators for information-theoretic security in disadvantaged wireless environments},
	journal = {50th Annual Allerton Conference on Communication, Control, and Computing},
	year = {2012},
	pages = {233--240},
}


@article{azadeh2012Infocom,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
	journal = {IEEE INFOCOM},
	year = {2012},
	pages = {1179--1187},
}

@article{1corser2016evaluating,
	title={Evaluating Location Privacy in Vehicular Communications and Applications},
	author={Corser, George P and Fu, Huirong and Banihani, Abdelnasser},
	journal={IEEE Transactions on Intelligent Transportation Systems},
	volume={17},
	number={9},
	pages={2658-2667},
	year={2016},
	publisher={IEEE}
}
@article{2zhang2016designing,
	title={On Designing Satisfaction-Ratio-Aware Truthful Incentive Mechanisms for k-Anonymity Location Privacy},
	author={Zhang, Yuan and Tong, Wei and Zhong, Sheng},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={11},
	number={11},
	pages={2528--2541},
	year={2016},
	publisher={IEEE}
}
@article{3li2016privacy,
	title={Privacy-preserving Location Proof for Securing Large-scale Database-driven Cognitive Radio Networks},
	author={Li, Yi and Zhou, Lu and Zhu, Haojin and Sun, Limin},
	journal={IEEE Internet of Things Journal},
	volume={3},
	number={4},
	pages={563-571},
	year={2016},
	publisher={IEEE}
}
@article{4olteanu2016quantifying,
	title={Quantifying Interdependent Privacy Risks with Location Data},
	author={Olteanu, Alexandra-Mihaela and Huguenin, K{\'e}vin and Shokri, Reza and Humbert, Mathias and Hubaux, Jean-Pierre},
	journal={IEEE Transactions on Mobile Computing},
	year={2016},
	volume={PP},
	number={99},
	pages={1-1},
	publisher={IEEE}
}
@article{5yi2016practical,
	title={Practical Approximate k Nearest Neighbor Queries with Location and Query Privacy},
	author={Yi, Xun and Paulet, Russell and Bertino, Elisa and Varadharajan, Vijay},
	journal={IEEE Transactions on Knowledge and Data Engineering},
	volume={28},
	number={6},
	pages={1546--1559},
	year={2016},
	publisher={IEEE}
}
@article{6li2016privacy,
	title={Privacy Leakage of Location Sharing in Mobile Social Networks: Attacks and Defense},
	author={Li, Huaxin and Zhu, Haojin and Du, Suguo and Liang, Xiaohui and Shen, Xuemin},
	journal={IEEE Transactions on Dependable and Secure Computing},
	year={2016},
	volume={PP},
	number={99},
	publisher={IEEE}
}

@article{7murakami2016localization,
	title={Localization Attacks Using Matrix and Tensor Factorization},
	author={Murakami, Takao and Watanabe, Hajime},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={11},
	number={8},
	pages={1647--1660},
	year={2016},
	publisher={IEEE}
}
@article{8zurbaran2015near,
	title={Near-Rand: Noise-based Location Obfuscation Based on Random Neighboring Points},
	author={Zurbaran, Mayra Alejandra and Avila, Karen and Wightman, Pedro and Fernandez, Michael},
	journal={IEEE Latin America Transactions},
	volume={13},
	number={11},
	pages={3661--3667},
	year={2015},
	publisher={IEEE}
}

@article{9tan2014anti,
	title={An anti-tracking source-location privacy protection protocol in wsns based on path extension},
	author={Tan, Wei and Xu, Ke and Wang, Dan},
	journal={IEEE Internet of Things Journal},
	volume={1},
	number={5},
	pages={461--471},
	year={2014},
	publisher={IEEE}
}

@article{10peng2014enhanced,
	title={Enhanced Location Privacy Preserving Scheme in Location-Based Services},
	author={Peng, Tao and Liu, Qin and Wang, Guojun},
	journal={IEEE Systems Journal},
	year={2014},
	volume={PP},
	number={99},
	pages={1-12},
	publisher={IEEE}
}
@article{11dewri2014exploiting,
	title={Exploiting service similarity for privacy in location-based search queries},
	author={Dewri, Rinku and Thurimella, Ramakrisha},
	journal={IEEE Transactions on Parallel and Distributed Systems},
	volume={25},
	number={2},
	pages={374--383},
	year={2014},
	publisher={IEEE}
}

@article{12hwang2014novel,
	title={A novel time-obfuscated algorithm for trajectory privacy protection},
	author={Hwang, Ren-Hung and Hsueh, Yu-Ling and Chung, Hao-Wei},
	journal={IEEE Transactions on Services Computing},
	volume={7},
	number={2},
	pages={126--139},
	year={2014},
	publisher={IEEE}
}
@article{13puttaswamy2014preserving,
	title={Preserving location privacy in geosocial applications},
	author={Puttaswamy, Krishna PN and Wang, Shiyuan and Steinbauer, Troy and Agrawal, Divyakant and El Abbadi, Amr and Kruegel, Christopher and Zhao, Ben Y},
	journal={IEEE Transactions on Mobile Computing},
	volume={13},
	number={1},
	pages={159--173},
	year={2014},
	publisher={IEEE}
}

@article{14zhang2014privacy,
	title={Privacy quantification model based on the Bayes conditional risk in Location-Based Services},
	author={Zhang, Xuejun and Gui, Xiaolin and Tian, Feng and Yu, Si and An, Jian},
	journal={Tsinghua Science and Technology},
	volume={19},
	number={5},
	pages={452--462},
	year={2014},
	publisher={TUP}
}

@article{15bilogrevic2014privacy,
	title={Privacy-preserving optimal meeting location determination on mobile devices},
	author={Bilogrevic, Igor and Jadliwala, Murtuza and Joneja, Vishal and Kalkan, K{\"u}bra and Hubaux, Jean-Pierre and Aad, Imad},
	journal={IEEE transactions on information forensics and security},
	volume={9},
	number={7},
	pages={1141--1156},
	year={2014},
	publisher={IEEE}
}
@article{16haghnegahdar2014privacy,
	title={Privacy Risks in Publishing Mobile Device Trajectories},
	author={Haghnegahdar, Alireza and Khabbazian, Majid and Bhargava, Vijay K},
	journal={IEEE Wireless Communications Letters},
	volume={3},
	number={3},
	pages={241--244},
	year={2014},
	publisher={IEEE}
}
@article{17malandrino2014verification,
	title={Verification and inference of positions in vehicular networks through anonymous beaconing},
	author={Malandrino, Francesco and Borgiattino, Carlo and Casetti, Claudio and Chiasserini, Carla-Fabiana and Fiore, Marco and Sadao, Roberto},
	journal={IEEE Transactions on Mobile Computing},
	volume={13},
	number={10},
	pages={2415--2428},
	year={2014},
	publisher={IEEE}
}
@article{18shokri2014hiding,
	title={Hiding in the mobile crowd: Locationprivacy through collaboration},
	author={Shokri, Reza and Theodorakopoulos, George and Papadimitratos, Panos and Kazemi, Ehsan and Hubaux, Jean-Pierre},
	journal={IEEE transactions on dependable and secure computing},
	volume={11},
	number={3},
	pages={266--279},
	year={2014},
	publisher={IEEE}
}
@article{19freudiger2013non,
	title={Non-cooperative location privacy},
	author={Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
	journal={IEEE Transactions on Dependable and Secure Computing},
	volume={10},
	number={2},
	pages={84--98},
	year={2013},
	publisher={IEEE}
}
@article{20gao2013trpf,
	title={TrPF: A trajectory privacy-preserving framework for participatory sensing},
	author={Gao, Sheng and Ma, Jianfeng and Shi, Weisong and Zhan, Guoxing and Sun, Cong},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={8},
	number={6},
	pages={874--887},
	year={2013},
	publisher={IEEE}
}
@article{21ma2013privacy,
	title={Privacy vulnerability of published anonymous mobility traces},
	author={Ma, Chris YT and Yau, David KY and Yip, Nung Kwan and Rao, Nageswara SV},
	journal={IEEE/ACM Transactions on Networking},
	volume={21},
	number={3},
	pages={720--733},
	year={2013},
	publisher={IEEE}
}
@article{22niu2013pseudo,
	title={Pseudo-Location Updating System for privacy-preserving location-based services},
	author={Niu, Ben and Zhu, Xiaoyan and Chi, Haotian and Li, Hui},
	journal={China Communications},
	volume={10},
	number={9},
	pages={1--12},
	year={2013},
	publisher={IEEE}
}
@article{23dewri2013local,
	title={Local differential perturbations: Location privacy under approximate knowledge attackers},
	author={Dewri, Rinku},
	journal={IEEE Transactions on Mobile Computing},
	volume={12},
	number={12},
	pages={2360--2372},
	year={2013},
	publisher={IEEE}
}
@inproceedings{24kanoria2012tractable,
	title={Tractable bayesian social learning on trees},
	author={Kanoria, Yashodhan and Tamuz, Omer},
	booktitle={Information Theory Proceedings (ISIT), 2012 IEEE International Symposium on},
	pages={2721--2725},
	year={2012},
	organization={IEEE}
}
@inproceedings{25farias2005universal,
	title={A universal scheme for learning},
	author={Farias, Vivek F and Moallemi, Ciamac C and Van Roy, Benjamin and Weissman, Tsachy},
	booktitle={Proceedings. International Symposium on Information Theory, 2005. ISIT 2005.},
	pages={1158--1162},
	year={2005},
	organization={IEEE}
}
@inproceedings{26misra2013unsupervised,
	title={Unsupervised learning and universal communication},
	author={Misra, Vinith and Weissman, Tsachy},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={261--265},
	year={2013},
	organization={IEEE}
}
@inproceedings{27ryabko2013time,
	title={Time-series information and learning},
	author={Ryabko, Daniil},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={1392--1395},
	year={2013},
	organization={IEEE}
}
@inproceedings{28krzakala2013phase,
	title={Phase diagram and approximate message passing for blind calibration and dictionary learning},
	author={Krzakala, Florent and M{\'e}zard, Marc and Zdeborov{\'a}, Lenka},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={659--663},
	year={2013},
	organization={IEEE}
}
@inproceedings{29sakata2013sample,
	title={Sample complexity of Bayesian optimal dictionary learning},
	author={Sakata, Ayaka and Kabashima, Yoshiyuki},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={669--673},
	year={2013},
	organization={IEEE}
}
@inproceedings{30predd2004consistency,
	title={Consistency in a model for distributed learning with specialists},
	author={Predd, Joel B and Kulkarni, Sanjeev R and Poor, H Vincent},
	booktitle={IEEE International Symposium on Information Theory},
	year={2004},
	organization={IEEE}
}
@inproceedings{31nokleby2016rate,
	title={Rate-Distortion Bounds on Bayes Risk in Supervised Learning},
	author={Nokleby, Matthew and Beirami, Ahmad and Calderbank, Robert},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={2099-2103},
	year={2016},
	organization={IEEE}
}

@inproceedings{32le2016imperfect,
	title={Are imperfect reviews helpful in social learning?},
	author={Le, Tho Ngoc and Subramanian, Vijay G and Berry, Randall A},
	booktitle={Information Theory (ISIT), 2016 IEEE International Symposium on},
	pages={2089--2093},
	year={2016},
	organization={IEEE}
}
@inproceedings{33gadde2016active,
	title={Active Learning for Community Detection in Stochastic Block Models},
	author={Gadde, Akshay and Gad, Eyal En and Avestimehr, Salman and Ortega, Antonio},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={1889-1893},
	year={2016}
}
@inproceedings{34shakeri2016minimax,
	title={Minimax Lower Bounds for Kronecker-Structured Dictionary Learning},
	author={Shakeri, Zahra and Bajwa, Waheed U and Sarwate, Anand D},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={1148-1152},
	year={2016}
}
@article{35lee2015speeding,
	title={Speeding up distributed machine learning using codes},
	author={Lee, Kangwook and Lam, Maximilian and Pedarsani, Ramtin and Papailiopoulos, Dimitris and Ramchandran, Kannan},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={1143-1147},
	year={2016}
}
@article{36oneto2016statistical,
	title={Statistical Learning Theory and ELM for Big Social Data Analysis},
	author={Oneto, Luca and Bisio, Federica and Cambria, Erik and Anguita, Davide},
	journal={ieee CompUTATionAl inTelliGenCe mAGAzine},
	volume={11},
	number={3},
	pages={45--55},
	year={2016},
	publisher={IEEE}
}
@article{37lin2015probabilistic,
	title={Probabilistic approach to modeling and parameter learning of indirect drive robots from incomplete data},
	author={Lin, Chung-Yen and Tomizuka, Masayoshi},
	journal={IEEE/ASME Transactions on Mechatronics},
	volume={20},
	number={3},
	pages={1036--1045},
	year={2015},
	publisher={IEEE}
}
@article{38wang2016towards,
	title={Towards Bayesian Deep Learning: A Framework and Some Existing Methods},
	author={Wang, Hao and Yeung, Dit-Yan},
	journal={IEEE Transactions on Knowledge and Data Engineering},
	volume={PP},
	number={99},
	year={2016},
	publisher={IEEE}
}


%%%%%Informationtheoreticsecurity%%%%%%%%%%%%%%%%%%%%%%%




@inproceedings{Bloch2011PhysicalSecBook,
	title={Physical-Layer Security},
	author={M. Bloch and J. Barros},
	organization={Cambridge University Press},
	year={2011}
}



@inproceedings{Liang2009InfoSecBook,
	title={Information Theoretic Security},
	author={Y. Liang and H. V. Poor and S. Shamai (Shitz)},
	organization={Now Publishers Inc.},
	year={2009}
}


@inproceedings{Zhou2013PhysicalSecBook,
	title={Physical Layer Security in Wireless Communications},
	author={ X. Zhou and L. Song and Y. Zhang},
	organization={CRC Press},
	year={2013}
}

@article{Ni2012IEA,
	Author = {D. Ni and H. Liu and W. Ding and  Y. Xie and H. Wang and H. Pishro-Nik and Q. Yu},
	Journal = {IEA/AIE},
	Title = {Cyber-Physical Integration to Connect Vehicles for Transformed Transportation Safety and Efficiency},
	Year = {2012}}



@inproceedings{Ni2012Inproceedings,
	Author = {D. Ni, H. Liu, Y. Xie, W. Ding, H. Wang, H. Pishro-Nik, Q. Yu and M. Ferreira},
	Booktitle = {Spring Simulation Multiconference},
	Date-Added = {2016-09-04 14:18:42 +0000},
	Date-Modified = {2016-09-06 16:22:14 +0000},
	Title = {Virtual Lab of Connected Vehicle Technology},
	Year = {2012}}

@inproceedings{Ni2012Inproceedings,
	Author = {D. Ni, H. Liu, W. Ding, Y. Xie, H. Wang, H. Pishro-Nik and Q. Yu,},
	Booktitle = {IEA/AIE},
	Date-Added = {2016-09-04 09:11:02 +0000},
	Date-Modified = {2016-09-06 14:46:53 +0000},
	Title = {Cyber-Physical Integration to Connect Vehicles for Transformed Transportation Safety and Efficiency},
	Year = {2012}}


@article{Nekoui_IJIPT_2009,
	Author = {M. Nekoui and D. Ni and H. Pishro-Nik and R. Prasad and M. Kanjee and H. Zhu and T. Nguyen},
	Journal = {International Journal of Internet Protocol Technology (IJIPT)},
	Number = {3},
	Pages = {},
	Publisher = {},
	Title = {Development of a VII-Enabled Prototype Intersection Collision Warning System},
	Volume = {4},
	Year = {2009}}


@inproceedings{Pishro_Ganz_Ni,
	Author = {H. Pishro-Nik, A. Ganz, and Daiheng Ni},
	Booktitle = {Forty-Fifth Annual Allerton Conference on Communication, Control, and Computing. Allerton House, Monticello, IL},
	Date-Added = {},
	Date-Modified = {},
	Number = {},
	Pages = {},
	Title = {The capacity of vehicular ad hoc networks},
	Volume = {},
	Year = {September 26-28, 2007}}

@inproceedings{Leow_Pishro_Ni_1,
	Author = {W. L. Leow, H. Pishro-Nik and Daiheng Ni},
	Booktitle = {IEEE Global Telecommunications Conference, Washington, D.C.},
	Date-Added = {},
	Date-Modified = {},
	Number = {},
	Pages = {},
	Title = {Delay and Energy Tradeoff in Multi-state Wireless Sensor Networks},
	Volume = {},
	Year = {November 26-30, 2007}}


@misc{UMass-Trans,
	title = {{UMass Transportation Center}},
	note = {\url{http://www.umasstransportationcenter.org/}},
}


@inproceedings{Haenggi2013book,
	title={Stochastic geometry for wireless networks},
	author={M. Haenggi},
	organization={Cambridge Uinversity Press},
	year={2013}
}


%%%%%%%%%%%%%%%%personalization%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{osma2015,
	title={Impact of Time-to-Collision Information on Driving Behavior in Connected Vehicle Environments Using A Driving Simulator Test Bed},
	journal{Journal of Traffic and Logistics Engineering},
	author={Osama A. Osman, Julius Codjoe, and Sherif Ishak},
	volume={3},
	number={1},
	pages={18--24},
	year={2015}
}


@article{charisma2010,
	title={Dynamic Latent Plan Models},
	author={Charisma F. Choudhurya, Moshe Ben-Akivab and Maya Abou-Zeid},
	journal={Journal of Choice Modelling},
	volume={3},
	number={2},
	pages={50--70},
	year={2010},
	publisher={Elsvier}
}


@misc{noble2014,
	author = {A. M. Noble, Shane B. McLaughlin, Zachary R. Doerzaph and Thomas A. Dingus},
	title = {Crowd-sourced Connected-vehicle Warning Algorithm using Naturalistic Driving Data},
	howpublished = {Downloaded from \url{http://hdl.handle.net/10919/53978}},
	
	month = August,
	year = 2014
}


@phdthesis{charisma2007,
	title    = {Modeling Driving Decisions with Latent Plans},
	school   = {Massachusetts Institute of Technology },
	author   = {Charisma Farheen Choudhury},
	year     = {2007}, %other attributes omitted
}


@article{chrysler2015,
	title={Cost of Warning of Unseen Threats:Unintended Consequences of Connected Vehicle Alerts},
	author={S. T. Chrysler, J. M. Cooper and D. C. Marshall},
	journal={Transportation Research Record: Journal of the Transportation Research Board},
	volume={2518},
	pages={79--85},
	year={2015},
}

@misc{nsf_cps,
	title = {Cyber-Physical Systems (CPS) PROGRAM SOLICITATION NSF 17-529},
	howpublished = {Downloaded from \url{https://www.nsf.gov/publications/pub_summ.jsp?WT.z_pims_id=503286&ods_key=nsf17529}},
}



%%%%%%%%%%%%%%IOT%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




@article{FTC2015,
	title={Internet of Things: Privacy and Security in a Connected World},
	author={FTC Staff Report},
	year={2015}
}



%% Saved with string encoding Unicode (UTF-8)
@inproceedings{1zhou2014security,
	title={Security/privacy of wearable fitness tracking {I}o{T} devices},
	author={Zhou, Wei and Piramuthu, Selwyn},
	booktitle={Information Systems and Technologies (CISTI), 2014 9th Iberian Conference on},
	pages={1--5},
	year={2014},
	organization={IEEE}
}

@article{2nia2016comprehensive,
	title={A comprehensive study of security of internet-of-things},
	author={Mohsenia, Arsalan and Jha, Niraj K},
	journal={IEEE Transactions on Emerging Topics in Computing},
	volum={5},
	number={4},
	pages={586--602},
	year={2017},
	publisher={IEEE}
}

@inproceedings{3ukil2014iot,
	title={{I}o{T}-privacy: To be private or not to be private},
	author={Ukil, Arijit and Bandyopadhyay, Soma and Pal, Arpan},
	booktitle={Computer Communications Workshops (INFOCOM WKSHPS), IEEE Conference on},
	pages={123--124},
	year={2014},
	organization={IEEE}
}

@article{4arias2015privacy,
	title={Privacy and security in internet of things and wearable devices},
	author={Arias, Orlando and Wurm, Jacob and Hoang, Khoa and Jin, Yier},
	journal={IEEE Transactions on Multi-Scale Computing Systems},
	volume={1},
	number={2},
	pages={99--109},
	year={2015},
	publisher={IEEE}
}
@inproceedings{5ullah2016novel,
	title={A novel model for preserving Location Privacy in Internet of Things},
	author={Ullah, Ikram and Shah, Munam Ali},
	booktitle={Automation and Computing (ICAC), 2016 22nd International Conference on},
	pages={542--547},
	year={2016},
	organization={IEEE}
}
@inproceedings{6sathishkumar2016enhanced,
	title={Enhanced location privacy algorithm for wireless sensor network in Internet of Things},
	author={Sathishkumar, J and Patel, Dhiren R},
	booktitle={Internet of Things and Applications (IOTA), International Conference on},
	pages={208--212},
	year={2016},
	organization={IEEE}
}
@inproceedings{7zhou2012preserving,
	title={Preserving sensor location privacy in internet of things},
	author={Zhou, Liming and Wen, Qiaoyan and Zhang, Hua},
	booktitle={Computational and Information Sciences (ICCIS), 2012 Fourth International Conference on},
	pages={856--859},
	year={2012},
	organization={IEEE}
}

@inproceedings{8ukil2015privacy,
	title={Privacy for {I}o{T}: Involuntary privacy enablement for smart energy systems},
	author={Ukil, Arijit and Bandyopadhyay, Soma and Pal, Arpan},
	booktitle={Communications (ICC), 2015 IEEE International Conference on},
	pages={536--541},
	year={2015},
	organization={IEEE}
}

@inproceedings{9dalipi2016security,
	title={Security and Privacy Considerations for {I}o{T} Application on Smart Grids: Survey and Research Challenges},
	author={Dalipi, Fisnik and Yayilgan, Sule Yildirim},
	booktitle={Future Internet of Things and Cloud Workshops (FiCloudW), IEEE International Conference on},
	pages={63--68},
	year={2016},
	organization={IEEE}
}
@inproceedings{10harris2016security,
	title={Security and Privacy in Public {I}o{T} Spaces},
	author={Harris, Albert F and Sundaram, Hari and Kravets, Robin},
	booktitle={Computer Communication and Networks (ICCCN), 2016 25th International Conference on},
	pages={1--8},
	year={2016},
	organization={IEEE}
}

@inproceedings{11al2015security,
	title={Security and privacy framework for ubiquitous healthcare {I}o{T} devices},
	author={Al Alkeem, Ebrahim and Yeun, Chan Yeob and Zemerly, M Jamal},
	booktitle={Internet Technology and Secured Transactions (ICITST), 2015 10th International Conference for},
	pages={70--75},
	year={2015},
	organization={IEEE}
}
@inproceedings{12sivaraman2015network,
	title={Network-level security and privacy control for smart-home {I}o{T} devices},
	author={Sivaraman, Vijay and Gharakheili, Hassan Habibi and Vishwanath, Arun and Boreli, Roksana and Mehani, Olivier},
	booktitle={Wireless and Mobile Computing, Networking and Communications (WiMob), 2015 IEEE 11th International Conference on},
	pages={163--167},
	year={2015},
	organization={IEEE}
}

@inproceedings{13srinivasan2016privacy,
	title={Privacy conscious architecture for improving emergency response in smart cities},
	author={Srinivasan, Ramya and Mohan, Apurva and Srinivasan, Priyanka},
	booktitle={Smart City Security and Privacy Workshop (SCSP-W), 2016},
	pages={1--5},
	year={2016},
	organization={IEEE}
}
@inproceedings{14sadeghi2015security,
	title={Security and privacy challenges in industrial internet of things},
	author={Sadeghi, Ahmad-Reza and Wachsmann, Christian and Waidner, Michael},
	booktitle={Design Automation Conference (DAC), 2015 52nd ACM/EDAC/IEEE},
	pages={1--6},
	year={2015},
	organization={IEEE}
}
@inproceedings{15otgonbayar2016toward,
	title={Toward Anonymizing {I}o{T} Data Streams via Partitioning},
	author={Otgonbayar, Ankhbayar and Pervez, Zeeshan and Dahal, Keshav},
	booktitle={Mobile Ad Hoc and Sensor Systems (MASS), 2016 IEEE 13th International Conference on},
	pages={331--336},
	year={2016},
	organization={IEEE}
}
@inproceedings{16rutledge2016privacy,
	title={Privacy Impacts of {I}o{T} Devices: A SmartTV Case Study},
	author={Rutledge, Richard L and Massey, Aaron K and Ant{\'o}n, Annie I},
	booktitle={Requirements Engineering Conference Workshops (REW), IEEE International},
	pages={261--270},
	year={2016},
	organization={IEEE}
}

@inproceedings{17andrea2015internet,
	title={Internet of Things: Security vulnerabilities and challenges},
	author={Andrea, Ioannis and Chrysostomou, Chrysostomos and Hadjichristofi, George},
	booktitle={Computers and Communication (ISCC), 2015 IEEE Symposium on},
	pages={180--187},
	year={2015},
	organization={IEEE}
}






























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@misc{epfl-mobility-20090224,
	author = {Michal Piorkowski and Natasa Sarafijanovic-Djukic and Matthias Grossglauser},
	title = {{CRAWDAD} dataset epfl/mobility (v. 2009-02-24)},
	howpublished = {Downloaded from \url{http://crawdad.org/epfl/mobility/20090224}},
	doi = {10.15783/C7J010},
	month = feb,
	year = 2009
}

@misc{roma-taxi-20140717,
	author = {Lorenzo Bracciale and Marco Bonola and Pierpaolo Loreti and Giuseppe Bianchi and Raul Amici and Antonello Rabuffi},
	title = {{CRAWDAD} dataset roma/taxi (v. 2014-07-17)},
	howpublished = {Downloaded from \url{http://crawdad.org/roma/taxi/20140717}},
	doi = {10.15783/C7QC7M},
	month = jul,
	year = 2014
}

@misc{rice-ad_hoc_city-20030911,
	author = {Jorjeta G. Jetcheva and Yih-Chun Hu and Santashil PalChaudhuri and Amit Kumar Saha and David B. Johnson},
	title = {{CRAWDAD} dataset rice/ad\_hoc\_city (v. 2003-09-11)},
	howpublished = {Downloaded from \url{http://crawdad.org/rice/ad_hoc_city/20030911}},
	doi = {10.15783/C73K5B},
	month = sep,
	year = 2003
}

@misc{china:2012,
	author = {Microsoft Research Asia},
	title = {GeoLife GPS Trajectories},
	year = {2012},
	howpublished= {\url{https://www.microsoft.com/en-us/download/details.aspx?id=52367}},
}


@misc{china:2011,
	ALTauthor = {Microsoft Research Asia)},
	ALTeditor = {},
	title = {GeoLife GPS Trajectories,
	year = {2012},
	url = {https://www.microsoft.com/en-us/download/details.aspx?id=52367},
	}
	
	
	@misc{longversion,
	author = {N. Takbiri and A. Houmansadr and D.L. Goeckel and H. Pishro-Nik},
	title = {{Limits of Location Privacy under Anonymization and Obfuscation}},
	howpublished = "\url{http://www.ecs.umass.edu/ece/pishro/Papers/ISIT_2017-2.pdf}",
	year = 2017,
	month= "January",
	note = "Summarized version submitted to IEEE ISIT 2017"
	}
	
	@misc{isit_ke,
	author = {K. Li and D. Goeckel and H. Pishro-Nik},
	title = {{Bayesian Time Series Matching and Privacy}},
	note = "submitted to IEEE ISIT 2017"
	}
	
	@article{matching,
	title={Asymptotically Optimal Matching of Multiple Sequences to Source Distributions and Training Sequences},
	author={Jayakrishnan Unnikrishnan},
	journal={ IEEE Transactions on Information Theory},
	volume={61},
	number={1},
	pages={452-468},
	year={2015},
	publisher={IEEE}
	}
	
	
	@article{Naini2016,
	Author = {F. Naini and J. Unnikrishnan and P. Thiran and M. Vetterli},
	Journal = {IEEE Transactions on Information Forensics and Security},
	Publisher = {IEEE},
	Title = {Where You Are Is Who You Are: User Identification by Matching Statistics},
	volume={11},
	number={2},
	pages={358--372},
	Year = {2016}
	}
	
	
	
	@inproceedings{holowczak2015cachebrowser,
	title={{CacheBrowser: Bypassing Chinese Censorship without Proxies Using Cached Content}},
	author={Holowczak, John and Houmansadr, Amir},
	booktitle={Proceedings of the 22nd ACM SIGSAC Conference on Computer and Communications Security},
	pages={70--83},
	year={2015},
	organization={ACM}
	}
	@misc{cb-website,
	Howpublished = {\url{https://cachebrowser.net/#/}},
	Title = {{CacheBrowser}},
	key={cachebrowser}
	}
	
	@inproceedings{GameOfDecoys,
	title={{GAME OF DECOYS: Optimal Decoy Routing Through Game Theory}},
	author={Milad Nasr and Amir Houmansadr},
	booktitle={The $23^{rd}$ ACM Conference on Computer and Communications Security (CCS)},
	year={2016}
	}
	
	@inproceedings{CDNReaper,
	title={{Practical Censorship Evasion Leveraging Content Delivery Networks}},
	author={Hadi Zolfaghari and Amir Houmansadr},
	booktitle={The $23^{rd}$ ACM Conference on Computer and Communications Security (CCS)},
	year={2016}
	}
	
	@misc{Leberknight2010,
	Author = {Leberknight, C. and Chiang, M. and Poor, H. and Wong, F.},
	Howpublished = {\url{http://www.princeton.edu/~chiangm/anticensorship.pdf}},
	Title = {{A Taxonomy of Internet Censorship and Anti-censorship}},
	Year = {2010}}
	
	@techreport{ultrasurf-analysis,
	Author = {Appelbaum, Jacob},
	Institution = {The Tor Project},
	Title = {{Technical analysis of the Ultrasurf proxying software}},
	Url = {http://scholar.google.com/scholar?hl=en\&btnG=Search\&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software\#0},
	Year = {2012},
	Bdsk-Url-1 = {http://scholar.google.com/scholar?hl=en%5C&btnG=Search%5C&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software%5C#0}}
	
	@misc{gifc:07,
	Howpublished = {\url{http://www.internetfreedom.org/archive/Defeat\_Internet\_Censorship\_White\_Paper.pdf}},
	Key = {defeatcensorship},
	Publisher = {Global Internet Freedom Consortium (GIFC)},
	Title = {{Defeat Internet Censorship: Overview of Advanced Technologies and Products}},
	Type = {White Paper},
	Year = {2007}}
	
	@article{pan2011survey,
	Author = {Pan, J. and Paul, S. and Jain, R.},
	Journal = {Communications Magazine, IEEE},
	Number = {7},
	Pages = {26--36},
	Publisher = {IEEE},
	Title = {{A Survey of the Research on Future Internet Architectures}},
	Volume = {49},
	Year = {2011}}
	
	@misc{nsf-fia,
	Howpublished = {\url{http://www.nets-fia.net/}},
	Key = {FIA},
	Title = {{NSF Future Internet Architecture Project}}}
	
	@misc{NDN,
	Howpublished = {\url{http://www.named- data.net}},
	Key = {NDN},
	Title = {{Named Data Networking Project}}}
	
	@inproceedings{MobilityFirst,
	Author = {Seskar, I. and Nagaraja, K. and Nelson, S. and Raychaudhuri, D.},
	Booktitle = {Asian Internet Engineering Conference},
	Title = {{Mobilityfirst Future internet Architecture Project}},
	Year = {2011}}
	
	@incollection{NEBULA,
	Author = {Anderson, T. and Birman, K. and Broberg, R. and Caesar, M. and Comer, D. and Cotton, C. and Freedman, M.~J. and Haeberlen, A. and Ives, Z.~G. and Krishnamurthy, A. and others},
	Booktitle = {The Future Internet},
	Pages = {16--26},
	Publisher = {Springer},
	Title = {{The NEBULA Future Internet Architecture}},
	Year = {2013}}
	
	@inproceedings{XIA,
	Author = {Anand, A. and Dogar, F. and Han, D. and Li, B. and Lim, H. and Machado, M. and Wu, W. and Akella, A. and Andersen, D.~G. and Byers, J.~W. and others},
	Booktitle = {ACM Workshop on Hot Topics in Networks},
	Pages = {2},
	Title = {{XIA: An Architecture for an Evolvable and Trustworthy Internet}},
	Year = {2011}}
	
	@inproceedings{ChoiceNet,
	Author = {Rouskas, G.~N. and Baldine, I. and Calvert, K.~L. and Dutta, R. and Griffioen, J. and Nagurney, A. and Wolf, T.},
	Booktitle = {ONDM},
	Title = {{ChoiceNet: Network Innovation Through Choice}},
	Year = {2013}}
	
	@misc{nsf-find,
	Howpublished = {http://www.nets-find.net/},
	Title = {{NSF NeTS FIND Initiative}}}
	
	@article{traid,
	Author = {Cheriton, D.~R. and Gritter, M.},
	Title = {{TRIAD: A New Next-Generation Internet Architecture}},
	Year = {2000}}
	
	@inproceedings{dona,
	Author = {Koponen, T. and Chawla, M. and Chun, B-G. and Ermolinskiy, A. and Kim, K.~H. and Shenker, S. and Stoica, I.},
	Booktitle = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Organization = {ACM},
	Pages = {181--192},
	Title = {{A Data-Oriented (and Beyond) Network Architecture}},
	Volume = {37},
	Year = {2007}}
	
	@misc{ultrasurf,
	Howpublished = {\url{http://www.ultrareach.com}},
	Key = {ultrasurf},
	Title = {{Ultrasurf}}}
	
	@misc{tor-bridge,
	Author = {Dingledine, R. and Mathewson, N.},
	Howpublished = {\url{https://svn.torproject.org/svn/projects/design-paper/blocking.html}},
	Title = {{Design of a Blocking-Resistant Anonymity System}}}
	
	@inproceedings{McLachlanH09,
	Author = {J. McLachlan and N. Hopper},
	Booktitle = {WPES},
	Title = {{On the Risks of Serving Whenever You Surf: Vulnerabilities in Tor's Blocking Resistance Design}},
	Year = {2009}}
	
	@inproceedings{mahdian2010,
	Author = {Mahdian, M.},
	Booktitle = {{Fun with Algorithms}},
	Title = {{Fighting Censorship with Algorithms}},
	Year = {2010}}
	
	@inproceedings{McCoy2011,
	Author = {McCoy, D. and Morales, J.~A. and Levchenko, K.},
	Booktitle = {FC},
	Title = {{Proximax: A Measurement Based System for Proxies Dissemination}},
	Year = {2011}}
	
	@inproceedings{Sovran2008,
	Author = {Sovran, Y. and Libonati, A. and Li, J.},
	Booktitle = {IPTPS},
	Title = {{Pass it on: Social Networks Stymie Censors}},
	Year = {2008}}
	
	@inproceedings{rbridge,
	Author = {Wang, Q. and Lin, Zi and Borisov, N. and Hopper, N.},
	Booktitle = {{NDSS}},
	Title = {{rBridge: User Reputation based Tor Bridge Distribution with Privacy Preservation}},
	Year = {2013}}
	
	@inproceedings{telex,
	Author = {Wustrow, E. and Wolchok, S. and Goldberg, I. and Halderman, J.},
	Booktitle = {{USENIX Security}},
	Title = {{Telex: Anticensorship in the Network Infrastructure}},
	Year = {2011}}
	
	@inproceedings{cirripede,
	Author = {Houmansadr, A. and Nguyen, G. and Caesar, M. and Borisov, N.},
	Booktitle = {CCS},
	Title = {{Cirripede: Circumvention Infrastructure Using Router Redirection with Plausible Deniability}},
	Year = {2011}}
	
	@inproceedings{decoyrouting,
	Author = {Karlin, J. and Ellard, D. and Jackson, A. and Jones, C. and Lauer, G. and Mankins, D. and Strayer, W.},
	Booktitle = {{FOCI}},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = {2011}}
	
	@inproceedings{routing-around-decoys,
	Author = {M.~Schuchard and J.~Geddes and C.~Thompson and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Routing Around Decoys}},
	Year = {2012}}
	
	@inproceedings{parrot,
	Author = {A. Houmansadr and C. Brubaker and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{The Parrot is Dead: Observing Unobservable Network Communications}},
	Year = {2013}}
	
	@misc{knock,
	Author = {T. Wilde},
	Howpublished = {\url{https://blog.torproject.org/blog/knock-knock-knockin-bridges-doors}},
	Title = {{Knock Knock Knockin' on Bridges' Doors}},
	Year = {2012}}
	
	@inproceedings{china-tor,
	Author = {Winter, P. and Lindskog, S.},
	Booktitle = {{FOCI}},
	Title = {{How the Great Firewall of China Is Blocking Tor}},
	Year = {2012}}
	
	@misc{discover-bridge,
	Howpublished = {\url{https://blog.torproject.org/blog/research-problems-ten-ways-discover-tor-bridges}},
	Key = {tenways},
	Title = {{Ten Ways to Discover Tor Bridges}}}
	
	@inproceedings{freewave,
	Author = {A.~Houmansadr and T.~Riedl and N.~Borisov and A.~Singer},
	Booktitle = {{NDSS}},
	Title = {{I Want My Voice to Be Heard: IP over Voice-over-IP for Unobservable Censorship Circumvention}},
	Year = 2013}
	
	@inproceedings{censorspoofer,
	Author = {Q. Wang and X. Gong and G. Nguyen and A. Houmansadr and N. Borisov},
	Booktitle = {CCS},
	Title = {{CensorSpoofer: Asymmetric Communication Using IP Spoofing for Censorship-Resistant Web Browsing}},
	Year = {2012}}
	
	@inproceedings{skypemorph,
	Author = {H. Moghaddam and B. Li and M. Derakhshani and I. Goldberg},
	Booktitle = {CCS},
	Title = {{SkypeMorph: Protocol Obfuscation for Tor Bridges}},
	Year = {2012}}
	
	@inproceedings{stegotorus,
	Author = {Weinberg, Z. and Wang, J. and Yegneswaran, V. and Briesemeister, L. and Cheung, S. and Wang, F. and Boneh, D.},
	Booktitle = {CCS},
	Title = {{StegoTorus: A Camouflage Proxy for the Tor Anonymity System}},
	Year = {2012}}
	
	@techreport{dust,
	Author = {{B.~Wiley}},
	Howpublished = {\url{http://blanu.net/ Dust.pdf}},
	Institution = {School of Information, University of Texas at Austin},
	Title = {{Dust: A Blocking-Resistant Internet Transport Protocol}},
	Year = {2011}}
	
	@inproceedings{FTE,
	Author = {K.~Dyer and S.~Coull and T.~Ristenpart and T.~Shrimpton},
	Booktitle = {CCS},
	Title = {{Protocol Misidentification Made Easy with Format-Transforming Encryption}},
	Year = {2013}}
	
	@inproceedings{fp,
	Author = {Fifield, D. and Hardison, N. and Ellithrope, J. and Stark, E. and Dingledine, R. and Boneh, D. and Porras, P.},
	Booktitle = {PETS},
	Title = {{Evading Censorship with Browser-Based Proxies}},
	Year = {2012}}
	
	@misc{obfsproxy,
	Howpublished = {\url{https://www.torproject.org/projects/obfsproxy.html.en}},
	Key = {obfsproxy},
	Publisher = {The Tor Project},
	Title = {{A Simple Obfuscating Proxy}}}
	
	@inproceedings{Tor-instead-of-IP,
	Author = {Liu, V. and Han, S. and Krishnamurthy, A. and Anderson, T.},
	Booktitle = {HotNets},
	Title = {{Tor instead of IP}},
	Year = {2011}}
	
	@misc{roger-slides,
	Howpublished = {\url{https://svn.torproject.org/svn/projects/presentations/slides-28c3.pdf}},
	Key = {torblocking},
	Title = {{How Governments Have Tried to Block Tor}}}
	
	@inproceedings{infranet,
	Author = {Feamster, N. and Balazinska, M. and Harfst, G. and Balakrishnan, H. and Karger, D.},
	Booktitle = {USENIX Security},
	Title = {{Infranet: Circumventing Web Censorship and Surveillance}},
	Year = {2002}}
	
	@inproceedings{collage,
	Author = {S.~Burnett and N.~Feamster and S.~Vempala},
	Booktitle = {USENIX Security},
	Title = {{Chipping Away at Censorship Firewalls with User-Generated Content}},
	Year = {2010}}
	
	@article{anonymizer,
	Author = {Boyan, J.},
	Journal = {Computer-Mediated Communication Magazine},
	Month = sep,
	Number = {9},
	Title = {{The Anonymizer: Protecting User Privacy on the Web}},
	Volume = {4},
	Year = {1997}}
	
	@article{schulze2009internet,
	Author = {Schulze, H. and Mochalski, K.},
	Journal = {IPOQUE Report},
	Pages = {351--362},
	Title = {Internet Study 2008/2009},
	Volume = {37},
	Year = {2009}}
	
	@inproceedings{cya-ccs13,
	Author = {J.~Geddes and M.~Schuchard and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Cover Your ACKs: Pitfalls of Covert Channel Censorship Circumvention}},
	Year = {2013}}
	
	@inproceedings{andana,
	Author = {DiBenedetto, S. and Gasti, P. and Tsudik, G. and Uzun, E.},
	Booktitle = {{NDSS}},
	Title = {{ANDaNA: Anonymous Named Data Networking Application}},
	Year = {2012}}
	
	@inproceedings{darkly,
	Author = {Jana, S. and Narayanan, A. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{A Scanner Darkly: Protecting User Privacy From Perceptual Applications}},
	Year = {2013}}
	
	@inproceedings{NS08,
	Author = {A.~Narayanan and V.~Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {Robust de-anonymization of large sparse datasets},
	Year = {2008}}
	
	@inproceedings{NS09,
	Author = {Arvind Narayanan and Vitaly Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {De-anonymizing Social Networks},
	Year = {2009}}
	
	@inproceedings{memento,
	Author = {Jana, S. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{Memento: Learning secrets from process footprints}},
	Year = {2012}}
	
	@misc{plugtor,
	Howpublished = {\url{https://www.torproject.org/docs/pluggable-transports.html.en}},
	Key = {PluggableTransports},
	Publisher = {The Tor Project},
	Title = {{Tor: Pluggable transports}}}
	
	@misc{psiphon,
	Author = {J.~Jia and P.~Smith},
	Howpublished = {\url{http://www.cdf.toronto.edu/~csc494h/reports/2004-fall/psiphon_ae.html}},
	Title = {{Psiphon: Analysis and Estimation}},
	Year = 2004}
	
	@misc{china-github,
	Howpublished = {\url{http://mobile.informationweek.com/80269/show/72e30386728f45f56b343ddfd0fdb119/}},
	Key = {github},
	Title = {{China's GitHub Censorship Dilemma}}}
	
	@inproceedings{txbox,
	Author = {Jana, S. and Porter, D. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{TxBox: Building Secure, Efficient Sandboxes with System Transactions}},
	Year = {2011}}
	
	@inproceedings{airavat,
	Author = {I. Roy and S. Setty and A. Kilzer and V. Shmatikov and E. Witchel},
	Booktitle = {NSDI},
	Title = {{Airavat: Security and Privacy for MapReduce}},
	Year = {2010}}
	
	@inproceedings{osdi12,
	Author = {A. Dunn and M. Lee and S. Jana and S. Kim and M. Silberstein and Y. Xu and V. Shmatikov and E. Witchel},
	Booktitle = {OSDI},
	Title = {{Eternal Sunshine of the Spotless Machine: Protecting Privacy with Ephemeral Channels}},
	Year = {2012}}
	
	@inproceedings{ymal,
	Author = {J. Calandrino and A. Kilzer and A. Narayanan and E. Felten and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{``You Might Also Like:'' Privacy Risks of Collaborative Filtering}},
	Year = {2011}}
	
	@inproceedings{srivastava11,
	Author = {V. Srivastava and M. Bond and K. McKinley and V. Shmatikov},
	Booktitle = {PLDI},
	Title = {{A Security Policy Oracle: Detecting Security Holes Using Multiple API Implementations}},
	Year = {2011}}
	
	@inproceedings{chen-oakland10,
	Author = {Chen, S. and Wang, R. and Wang, X. and Zhang, K.},
	Booktitle = {IEEE S\&P},
	Title = {{Side-Channel Leaks in Web Applications: A Reality Today, a Challenge Tomorrow}},
	Year = {2010}}
	
	@book{kerck,
	Author = {Kerckhoffs, A.},
	Publisher = {University Microfilms},
	Title = {{La cryptographie militaire}},
	Year = {1978}}
	
	@inproceedings{foci11,
	Author = {J. Karlin and D. Ellard and A.~Jackson and C.~ Jones and G. Lauer and D. Mankins and W.~T.~Strayer},
	Booktitle = {FOCI},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = 2011}
	
	@inproceedings{sun02,
	Author = {Sun, Q. and Simon, D.~R. and Wang, Y. and Russell, W. and Padmanabhan, V. and Qiu, L.},
	Booktitle = {IEEE S\&P},
	Title = {{Statistical Identification of Encrypted Web Browsing Traffic}},
	Year = {2002}}
	
	@inproceedings{danezis,
	Author = {Murdoch, S.~J. and Danezis, G.},
	Booktitle = {IEEE S\&P},
	Title = {{Low-Cost Traffic Analysis of Tor}},
	Year = {2005}}
	
	@inproceedings{pakicensorship,
	Author = {Z.~Nabi},
	Booktitle = {FOCI},
	Title = {The Anatomy of {Web} Censorship in {Pakistan}},
	Year = {2013}}
	
	@inproceedings{irancensorship,
	Author = {S.~Aryan and H.~Aryan and A.~Halderman},
	Booktitle = {FOCI},
	Title = {Internet Censorship in {Iran}: {A} First Look},
	Year = {2013}}
	
	@inproceedings{ford10efficient,
	Author = {Amittai Aviram and Shu-Chun Weng and Sen Hu and Bryan Ford},
	Booktitle = {\bibconf[9th]{OSDI}{USENIX Symposium on Operating Systems Design and Implementation}},
	Location = {Vancouver, BC, Canada},
	Month = oct,
	Title = {Efficient System-Enforced Deterministic Parallelism},
	Year = 2010}
	
	@inproceedings{ford10determinating,
	Author = {Amittai Aviram and Sen Hu and Bryan Ford and Ramakrishna Gummadi},
	Booktitle = {\bibconf{CCSW}{ACM Cloud Computing Security Workshop}},
	Location = {Chicago, IL},
	Month = oct,
	Title = {Determinating Timing Channels in Compute Clouds},
	Year = 2010}
	
	@inproceedings{ford12plugging,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Plugging Side-Channel Leaks with Timing Information Flow Control},
	Year = 2012}
	
	@inproceedings{ford12icebergs,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Icebergs in the Clouds: the {\em Other} Risks of Cloud Computing},
	Year = 2012}
	
	@misc{mullenize,
	Author = {Washington Post},
	Howpublished = {\url{http://apps.washingtonpost.com/g/page/world/gchq-report-on-mullenize-program-to-stain-anonymous-electronic-traffic/502/}},
	Month = {oct},
	Title = {{GCHQ} report on {`MULLENIZE'} program to `stain' anonymous electronic traffic},
	Year = {2013}}
	
	@inproceedings{shue13street,
	Author = {Craig A. Shue and Nathanael Paul and Curtis R. Taylor},
	Booktitle = {\bibbrev[7th]{WOOT}{USENIX Workshop on Offensive Technologies}},
	Month = aug,
	Title = {From an {IP} Address to a Street Address: Using Wireless Signals to Locate a Target},
	Year = 2013}
	
	@inproceedings{knockel11three,
	Author = {Jeffrey Knockel and Jedidiah R. Crandall and Jared Saia},
	Booktitle = {\bibbrev{FOCI}{USENIX Workshop on Free and Open Communications on the Internet}},
	Location = {San Francisco, CA},
	Month = aug,
	Year = 2011}
	
	@misc{rfc4960,
	Author = {R. {Stewart, ed.}},
	Month = sep,
	Note = {RFC 4960},
	Title = {Stream Control Transmission Protocol},
	Year = 2007}
	
	@inproceedings{ford07structured,
	Author = {Bryan Ford},
	Booktitle = {\bibbrev{SIGCOMM}{ACM SIGCOMM}},
	Location = {Kyoto, Japan},
	Month = aug,
	Title = {Structured Streams: a New Transport Abstraction},
	Year = {2007}}
	
	@misc{spdy,
	Author = {Google, Inc.},
	Note = {\url{http://www.chromium.org/spdy/spdy-whitepaper}},
	Title = {{SPDY}: An Experimental Protocol For a Faster {Web}}}
	
	@misc{quic,
	Author = {Jim Roskind},
	Month = jun,
	Note = {\url{http://blog.chromium.org/2013/06/experimenting-with-quic.html}},
	Title = {Experimenting with {QUIC}},
	Year = 2013}
	
	@misc{podjarny12not,
	Author = {G.~Podjarny},
	Month = jun,
	Note = {\url{http://www.guypo.com/technical/not-as-spdy-as-you-thought/}},
	Title = {{Not as SPDY as You Thought}},
	Year = 2012}
	
	@inproceedings{cor,
	Author = {Jones, N.~A. and Arye, M. and Cesareo, J. and Freedman, M.~J.},
	Booktitle = {FOCI},
	Title = {{Hiding Amongst the Clouds: A Proposal for Cloud-based Onion Routing}},
	Year = {2011}}
	
	@misc{torcloud,
	Howpublished = {\url{https://cloud.torproject.org/}},
	Key = {tor cloud},
	Title = {{The Tor Cloud Project}}}
	
	@inproceedings{scramblesuit,
	Author = {Philipp Winter and Tobias Pulls and Juergen Fuss},
	Booktitle = {WPES},
	Title = {{ScrambleSuit: A Polymorphic Network Protocol to Circumvent Censorship}},
	Year = 2013}
	
	@article{savage2000practical,
	Author = {Savage, S. and Wetherall, D. and Karlin, A. and Anderson, T.},
	Journal = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Pages = {295--306},
	Publisher = {ACM},
	Title = {Practical network support for IP traceback},
	Volume = {30},
	Year = {2000}}
	
	@inproceedings{ooni,
	Author = {Filast, A. and Appelbaum, J.},
	Booktitle = {{FOCI}},
	Title = {{OONI : Open Observatory of Network Interference}},
	Year = {2012}}
	
	@misc{caida-rank,
	Howpublished = {\url{http://as-rank.caida.org/}},
	Key = {caida rank},
	Title = {{AS Rank: AS Ranking}}}
	
	@inproceedings{usersrouted-ccs13,
	Author = {A.~Johnson and C.~Wacek and R.~Jansen and M.~Sherr and P.~Syverson},
	Booktitle = {CCS},
	Title = {{Users Get Routed: Traffic Correlation on Tor by Realistic Adversaries}},
	Year = {2013}}
	
	@inproceedings{edman2009awareness,
	Author = {Edman, M. and Syverson, P.},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2009}}
	
	@inproceedings{DecoyCosts,
	Author = {A.~Houmansadr and E.~L.~Wong and V.~Shmatikov},
	Booktitle = {NDSS},
	Title = {{No Direction Home: The True Cost of Routing Around Decoys}},
	Year = {2014}}
	
	@article{cordon,
	Author = {Elahi, T. and Goldberg, I.},
	Journal = {University of Waterloo CACR},
	Title = {{CORDON--A Taxonomy of Internet Censorship Resistance Strategies}},
	Volume = {33},
	Year = {2012}}
	
	@inproceedings{privex,
	Author = {T.~Elahi and G.~Danezis and I.~Goldberg	},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2014}}
	
	@inproceedings{changeGuards,
	Author = {T.~Elahi and K.~Bauer and M.~AlSabah and R.~Dingledine and I.~Goldberg},
	Booktitle = {{WPES}},
	Title = {{ Changing of the Guards: Framework for Understanding and Improving Entry Guard Selection in Tor}},
	Year = {2012}}
	
	@article{RAINBOW:Journal,
	Author = {A.~Houmansadr and N.~Kiyavash and N.~Borisov},
	Journal = {IEEE/ACM Transactions on Networking},
	Title = {{Non-Blind Watermarking of Network Flows}},
	Year = 2014}
	
	@inproceedings{info-tod,
	Author = {A.~Houmansadr and S.~Gorantla and T.~Coleman and N.~Kiyavash and and N.~Borisov},
	Booktitle = {{CCS (poster session)}},
	Title = {{On the Channel Capacity of Network Flow Watermarking}},
	Year = {2009}}
	
	@inproceedings{johnson2014game,
	Author = {Johnson, B. and Laszka, A. and Grossklags, J. and Vasek, M. and Moore, T.},
	Booktitle = {Workshop on Bitcoin Research},
	Title = {{Game-theoretic Analysis of DDoS Attacks Against Bitcoin Mining Pools}},
	Year = {2014}}
	
	@incollection{laszka2013mitigation,
	Author = {Laszka, A. and Johnson, B. and Grossklags, J.},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {175--191},
	Publisher = {Springer},
	Title = {{Mitigation of Targeted and Non-targeted Covert Attacks as a Timing Game}},
	Year = {2013}}
	
	@inproceedings{schottle2013game,
	Author = {Schottle, P. and Laszka, A. and Johnson, B. and Grossklags, J. and Bohme, R.},
	Booktitle = {EUSIPCO},
	Title = {{A Game-theoretic Analysis of Content-adaptive Steganography with Independent Embedding}},
	Year = {2013}}
	
	@inproceedings{CloudTransport,
	Author = {C.~Brubaker and A.~Houmansadr and V.~Shmatikov},
	Booktitle = {PETS},
	Title = {{CloudTransport: Using Cloud Storage for Censorship-Resistant Networking}},
	Year = {2014}}
	
	@inproceedings{sweet,
	Author = {W.~Zhou and A.~Houmansadr and M.~Caesar and N.~Borisov},
	Booktitle = {HotPETs},
	Title = {{SWEET: Serving the Web by Exploiting Email Tunnels}},
	Year = {2013}}
	
	@inproceedings{ahsan2002practical,
	Author = {Ahsan, K. and Kundur, D.},
	Booktitle = {Workshop on Multimedia Security},
	Title = {{Practical data hiding in TCP/IP}},
	Year = {2002}}
	
	@incollection{danezis2011covert,
	Author = {Danezis, G.},
	Booktitle = {Security Protocols XVI},
	Pages = {198--214},
	Publisher = {Springer},
	Title = {{Covert Communications Despite Traffic Data Retention}},
	Year = {2011}}
	
	@inproceedings{liu2009hide,
	Author = {Liu, Y. and Ghosal, D. and Armknecht, F. and Sadeghi, A.-R. and Schulz, S. and Katzenbeisser, S.},
	Booktitle = {ESORICS},
	Title = {{Hide and Seek in Time---Robust Covert Timing Channels}},
	Year = {2009}}
	
	@misc{image-watermark-fing,
	Author = {Jonathan Bailey},
	Howpublished = {\url{https://www.plagiarismtoday.com/2009/12/02/image-detection-watermarking-vs-fingerprinting/}},
	Title = {{Image Detection: Watermarking vs. Fingerprinting}},
	Year = {2009}}
	
	@inproceedings{Servetto98,
	Author = {S. D. Servetto and C. I. Podilchuk and K. Ramchandran},
	Booktitle = {Int. Conf. Image Processing},
	Title = {Capacity issues in digital image watermarking},
	Year = {1998}}
	
	@inproceedings{Chen01,
	Author = {B. Chen and G.W.Wornell},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1423--1443},
	Title = {Quantization index modulation: A class of provably good methods for digital watermarking and information embedding},
	Year = {2001}}
	
	@inproceedings{Karakos00,
	Author = {D. Karakos and A. Papamarcou},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {47},
	Title = {Relationship between quantization and distribution rates of digitally watermarked data},
	Year = {2000}}
	
	@inproceedings{Sullivan98,
	Author = {J. A. OSullivan and P. Moulin and J. M. Ettinger},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {297},
	Title = {Information theoretic analysis of steganography},
	Year = {1998}}
	
	@inproceedings{Merhav00,
	Author = {N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {420--430},
	Title = {On random coding error exponents of watermarking systems},
	Year = {2000}}
	
	@inproceedings{Somekh01,
	Author = {A. Somekh-Baruch and N. Merhav},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {7},
	Title = {On the error exponent and capacity games of private watermarking systems},
	Year = {2001}}
	
	@inproceedings{Steinberg01,
	Author = {Y. Steinberg and N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1410--1422},
	Title = {Identification in the presence of side information with application to watermarking},
	Year = {2001}}
	
	@article{Moulin03,
	Author = {P. Moulin and J.A. O'Sullivan},
	Journal = {IEEE Trans. Info. Theory},
	Number = {3},
	Title = {Information-theoretic analysis of information hiding},
	Volume = 49,
	Year = 2003}
	
	@article{Gelfand80,
	Author = {S.I.~Gelfand and M.S.~Pinsker},
	Journal = {Problems of Control and Information Theory},
	Number = {1},
	Pages = {19-31},
	Title = {{Coding for channel with random parameters}},
	Url = {citeseer.ist.psu.edu/anantharam96bits.html},
	Volume = {9},
	Year = {1980},
	Bdsk-Url-1 = {citeseer.ist.psu.edu/anantharam96bits.html}}
	
	@book{Wolfowitz78,
	Author = {J. Wolfowitz},
	Edition = {3rd},
	Location = {New York},
	Publisher = {Springer-Verlag},
	Title = {Coding Theorems of Information Theory},
	Year = 1978}
	
	@article{caire99,
	Author = {G. Caire and S. Shamai},
	Journal = {IEEE Transactions on Information Theory},
	Number = {6},
	Pages = {2007--2019},
	Title = {On the Capacity of Some Channels with Channel State Information},
	Volume = {45},
	Year = {1999}}
	
	@inproceedings{wright2007language,
	Author = {Wright, Charles V and Ballard, Lucas and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {USENIX Security},
	Title = {{Language identification of encrypted VoIP traffic: Alejandra y Roberto or Alice and Bob?}},
	Year = {2007}}
	
	@inproceedings{backes2010speaker,
	Author = {Backes, Michael and Doychev, Goran and D{\"u}rmuth, Markus and K{\"o}pf, Boris},
	Booktitle = {{European Symposium on Research in Computer Security (ESORICS)}},
	Pages = {508--523},
	Publisher = {Springer},
	Title = {{Speaker Recognition in Encrypted Voice Streams}},
	Year = {2010}}
	
	@phdthesis{lu2009traffic,
	Author = {Lu, Yuanchao},
	School = {Cleveland State University},
	Title = {{On Traffic Analysis Attacks to Encrypted VoIP Calls}},
	Year = {2009}}
	
	@inproceedings{wright2008spot,
	Author = {Wright, Charles V and Ballard, Lucas and Coull, Scott E and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {35--49},
	Title = {Spot me if you can: Uncovering spoken phrases in encrypted VoIP conversations},
	Year = {2008}}
	
	@inproceedings{white2011phonotactic,
	Author = {White, Andrew M and Matthews, Austin R and Snow, Kevin Z and Monrose, Fabian},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {3--18},
	Title = {Phonotactic reconstruction of encrypted VoIP conversations: Hookt on fon-iks},
	Year = {2011}}
	
	@inproceedings{fancy,
	Author = {Houmansadr, Amir and Borisov, Nikita},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {205--224},
	Title = {The Need for Flow Fingerprints to Link Correlated Network Flows},
	Year = {2013}}
	
	@article{botmosaic,
	Author = {Amir Houmansadr and Nikita Borisov},
	Doi = {10.1016/j.jss.2012.11.005},
	Issn = {0164-1212},
	Journal = {Journal of Systems and Software},
	Keywords = {Network security},
	Number = {3},
	Pages = {707 - 715},
	Title = {BotMosaic: Collaborative network watermark for the detection of IRC-based botnets},
	Url = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Volume = {86},
	Year = {2013},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.jss.2012.11.005}}
	
	@inproceedings{ramsbrock2008first,
	Author = {Ramsbrock, Daniel and Wang, Xinyuan and Jiang, Xuxian},
	Booktitle = {Recent Advances in Intrusion Detection},
	Organization = {Springer},
	Pages = {59--77},
	Title = {A first step towards live botmaster traceback},
	Year = {2008}}
	
	@inproceedings{potdar2005survey,
	Author = {Potdar, Vidyasagar M and Han, Song and Chang, Elizabeth},
	Booktitle = {Industrial Informatics, 2005. INDIN'05. 2005 3rd IEEE International Conference on},
	Organization = {IEEE},
	Pages = {709--716},
	Title = {A survey of digital image watermarking techniques},
	Year = {2005}}
	
	@book{cole2003hiding,
	Author = {Cole, Eric and Krutz, Ronald D},
	Publisher = {John Wiley \& Sons, Inc.},
	Title = {Hiding in plain sight: Steganography and the art of covert communication},
	Year = {2003}}
	
	@incollection{akaike1998information,
	Author = {Akaike, Hirotogu},
	Booktitle = {Selected Papers of Hirotugu Akaike},
	Pages = {199--213},
	Publisher = {Springer},
	Title = {Information theory and an extension of the maximum likelihood principle},
	Year = {1998}}
	
	@misc{central-command-hack,
	Author = {Everett Rosenfeld},
	Howpublished = {\url{http://www.cnbc.com/id/102330338}},
	Title = {{FBI investigating Central Command Twitter hack}},
	Year = {2015}}
	
	@misc{sony-psp-ddos,
	Howpublished = {\url{http://n4g.com/news/1644853/sony-and-microsoft-cant-do-much-ddos-attacks-explained}},
	Key = {sony},
	Month = {December},
	Title = {{Sony and Microsoft cant do much -- DDoS attacks explained}},
	Year = {2014}}
	
	@misc{sony-hack,
	Author = {David Bloom},
	Howpublished = {\url{http://goo.gl/MwR4A7}},
	Title = {{Online Game Networks Hacked, Sony Unit President Threatened}},
	Year = {2014}}
	
	@misc{home-depot,
	Author = {Dune Lawrence},
	Howpublished = {\url{http://www.businessweek.com/articles/2014-09-02/home-depots-credit-card-breach-looks-just-like-the-target-hack}},
	Title = {{Home Depot's Suspected Breach Looks Just Like the Target Hack}},
	Year = {2014}}
	
	@misc{target,
	Author = {Julio Ojeda-Zapata},
	Howpublished = {\url{http://www.mercurynews.com/business/ci_24765398/how-did-hackers-pull-off-target-data-heist}},
	Title = {{Target hack: How did they do it?}},
	Year = {2014}}
	
	
	@article{probabilitycourse,
	Author = {H. Pishro-Nik},
	note = {\url{http://www.probabilitycourse.com}},
	Title = {Introduction to probability, statistics, and random processes},
	Year = {2014}}
	
	
	
	@inproceedings{shokri2011quantifying,
	Author = {Shokri, Reza and Theodorakopoulos, George and Le Boudec, Jean-Yves and Hubaux, Jean-Pierre},
	Booktitle = {Security and Privacy (SP), 2011 IEEE Symposium on},
	Organization = {IEEE},
	Pages = {247--262},
	Title = {Quantifying location privacy},
	Year = {2011}}
	
	@inproceedings{hoh2007preserving,
	Author = {Hoh, Baik and Gruteser, Marco and Xiong, Hui and Alrabady, Ansaf},
	Booktitle = {Proceedings of the 14th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {161--171},
	Title = {Preserving privacy in gps traces via uncertainty-aware path cloaking},
	Year = {2007}}
	
	
	
	@article{kafsi2013entropy,
	Author = {Kafsi, Mohamed and Grossglauser, Matthias and Thiran, Patrick},
	Journal = {Information Theory, IEEE Transactions on},
	Number = {9},
	Pages = {5577--5583},
	Publisher = {IEEE},
	Title = {The entropy of conditional Markov trajectories},
	Volume = {59},
	Year = {2013}}
	
	@inproceedings{gruteser2003anonymous,
	Author = {Gruteser, Marco and Grunwald, Dirk},
	Booktitle = {Proceedings of the 1st international conference on Mobile systems, applications and services},
	Organization = {ACM},
	Pages = {31--42},
	Title = {Anonymous usage of location-based services through spatial and temporal cloaking},
	Year = {2003}}
	
	@inproceedings{husted2010mobile,
	Author = {Husted, Nathaniel and Myers, Steven},
	Booktitle = {Proceedings of the 17th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {85--96},
	Title = {Mobile location tracking in metro areas: malnets and others},
	Year = {2010}}
	
	@inproceedings{li2009tradeoff,
	Author = {Li, Tiancheng and Li, Ninghui},
	Booktitle = {Proceedings of the 15th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {517--526},
	Title = {On the tradeoff between privacy and utility in data publishing},
	Year = {2009}}
	
	@inproceedings{ma2009location,
	Author = {Ma, Zhendong and Kargl, Frank and Weber, Michael},
	Booktitle = {Sarnoff Symposium, 2009. SARNOFF'09. IEEE},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {A location privacy metric for v2x communication systems},
	Year = {2009}}
	
	@inproceedings{shokri2012protecting,
	Author = {Shokri, Reza and Theodorakopoulos, George and Troncoso, Carmela and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
	Booktitle = {Proceedings of the 2012 ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {617--627},
	Title = {Protecting location privacy: optimal strategy against localization attacks},
	Year = {2012}}
	
	@inproceedings{freudiger2009non,
	Author = {Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
	Booktitle = {Proceedings of the 16th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {324--337},
	Title = {On non-cooperative location privacy: a game-theoretic analysis},
	Year = {2009}}
	
	@incollection{humbert2010tracking,
	Author = {Humbert, Mathias and Manshaei, Mohammad Hossein and Freudiger, Julien and Hubaux, Jean-Pierre},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {38--57},
	Publisher = {Springer},
	Title = {Tracking games in mobile networks},
	Year = {2010}}
	
	@article{manshaei2013game,
	Author = {Manshaei, Mohammad Hossein and Zhu, Quanyan and Alpcan, Tansu and Bac{\c{s}}ar, Tamer and Hubaux, Jean-Pierre},
	Journal = {ACM Computing Surveys (CSUR)},
	Number = {3},
	Pages = {25},
	Publisher = {ACM},
	Title = {Game theory meets network security and privacy},
	Volume = {45},
	Year = {2013}}
	
	@article{palamidessi2006probabilistic,
	Author = {Palamidessi, Catuscia},
	Journal = {Electronic Notes in Theoretical Computer Science},
	Pages = {33--42},
	Publisher = {Elsevier},
	Title = {Probabilistic and nondeterministic aspects of anonymity},
	Volume = {155},
	Year = {2006}}
	
	@inproceedings{mokbel2006new,
	Author = {Mokbel, Mohamed F and Chow, Chi-Yin and Aref, Walid G},
	Booktitle = {Proceedings of the 32nd international conference on Very large data bases},
	Organization = {VLDB Endowment},
	Pages = {763--774},
	Title = {The new Casper: query processing for location services without compromising privacy},
	Year = {2006}}
	
	@article{kalnis2007preventing,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {12},
	Pages = {1719--1733},
	Publisher = {IEEE},
	Title = {Preventing location-based identity inference in anonymous spatial queries},
	Volume = {19},
	Year = {2007}}
	
	@article{freudiger2007mix,
	title={Mix-zones for location privacy in vehicular networks},
	author={Freudiger, Julien and Raya, Maxim and F{\'e}legyh{\'a}zi, M{\'a}rk and Papadimitratos, Panos and Hubaux, Jean-Pierre},
	year={2007}
	}
	@article{sweeney2002k,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {557--570},
	Publisher = {World Scientific},
	Title = {k-anonymity: A model for protecting privacy},
	Volume = {10},
	Year = {2002}}
	
	@article{sweeney2002achieving,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {571--588},
	Publisher = {World Scientific},
	Title = {Achieving k-anonymity privacy protection using generalization and suppression},
	Volume = {10},
	Year = {2002}}
	
	@inproceedings{niu2014achieving,
	Author = {Niu, Ben and Li, Qinghua and Zhu, Xiaoyan and Cao, Guohong and Li, Hui},
	Booktitle = {INFOCOM, 2014 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {754--762},
	Title = {Achieving k-anonymity in privacy-aware location-based services},
	Year = {2014}}
	
	@inproceedings{liu2013game,
	Author = {Liu, Xinxin and Liu, Kaikai and Guo, Linke and Li, Xiaolin and Fang, Yuguang},
	Booktitle = {INFOCOM, 2013 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {2985--2993},
	Title = {A game-theoretic approach for achieving k-anonymity in location based services},
	Year = {2013}}
	
	@inproceedings{kido2005protection,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Data Engineering Workshops, 2005. 21st International Conference on},
	Organization = {IEEE},
	Pages = {1248--1248},
	Title = {Protection of location privacy using dummies for location-based services},
	Year = {2005}}
	
	@inproceedings{gedik2005location,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Booktitle = {Distributed Computing Systems, 2005. ICDCS 2005. Proceedings. 25th IEEE International Conference on},
	Organization = {IEEE},
	Pages = {620--629},
	Title = {Location privacy in mobile systems: A personalized anonymization model},
	Year = {2005}}
	
	@inproceedings{bordenabe2014optimal,
	Author = {Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2014 ACM SIGSAC Conference on Computer and Communications Security},
	Organization = {ACM},
	Pages = {251--262},
	Title = {Optimal geo-indistinguishable mechanisms for location privacy},
	Year = {2014}}
	
	@incollection{duckham2005formal,
	Author = {Duckham, Matt and Kulik, Lars},
	Booktitle = {Pervasive computing},
	Pages = {152--170},
	Publisher = {Springer},
	Title = {A formal model of obfuscation and negotiation for location privacy},
	Year = {2005}}
	
	@inproceedings{kido2005anonymous,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Pervasive Services, 2005. ICPS'05. Proceedings. International Conference on},
	Organization = {IEEE},
	Pages = {88--97},
	Title = {An anonymous communication technique using dummies for location-based services},
	Year = {2005}}
	
	@incollection{duckham2006spatiotemporal,
	Author = {Duckham, Matt and Kulik, Lars and Birtley, Athol},
	Booktitle = {Geographic Information Science},
	Pages = {47--64},
	Publisher = {Springer},
	Title = {A spatiotemporal model of strategies and counter strategies for location privacy protection},
	Year = {2006}}
	
	@inproceedings{shankar2009privately,
	Author = {Shankar, Pravin and Ganapathy, Vinod and Iftode, Liviu},
	Booktitle = {Proceedings of the 11th international conference on Ubiquitous computing},
	Organization = {ACM},
	Pages = {31--40},
	Title = {Privately querying location-based services with SybilQuery},
	Year = {2009}}
	
	@inproceedings{chow2009faking,
	Author = {Chow, Richard and Golle, Philippe},
	Booktitle = {Proceedings of the 8th ACM workshop on Privacy in the electronic society},
	Organization = {ACM},
	Pages = {105--108},
	Title = {Faking contextual data for fun, profit, and privacy},
	Year = {2009}}
	
	@incollection{xue2009location,
	Author = {Xue, Mingqiang and Kalnis, Panos and Pung, Hung Keng},
	Booktitle = {Location and Context Awareness},
	Pages = {70--87},
	Publisher = {Springer},
	Title = {Location diversity: Enhanced privacy protection in location based services},
	Year = {2009}}
	
	@article{wernke2014classification,
	Author = {Wernke, Marius and Skvortsov, Pavel and D{\"u}rr, Frank and Rothermel, Kurt},
	Journal = {Personal and Ubiquitous Computing},
	Number = {1},
	Pages = {163--175},
	Publisher = {Springer-Verlag},
	Title = {A classification of location privacy attacks and approaches},
	Volume = {18},
	Year = {2014}}
	
	@misc{cai2015cloaking,
	Author = {Cai, Y. and Xu, G.},
	Month = jan # {~1},
	Note = {US Patent App. 14/472,462},
	Publisher = {Google Patents},
	Title = {Cloaking with footprints to provide location privacy protection in location-based services},
	Url = {https://www.google.com/patents/US20150007341},
	Year = {2015},
	Bdsk-Url-1 = {https://www.google.com/patents/US20150007341}}
	
	@article{gedik2008protecting,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {1},
	Pages = {1--18},
	Publisher = {IEEE},
	Title = {Protecting location privacy with personalized k-anonymity: Architecture and algorithms},
	Volume = {7},
	Year = {2008}}
	
	@article{kalnis2006preserving,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Publisher = {TRB6/06},
	Title = {Preserving anonymity in location based services},
	Year = {2006}}
	
	@inproceedings{hoh2005protecting,
	Author = {Hoh, Baik and Gruteser, Marco},
	Booktitle = {Security and Privacy for Emerging Areas in Communications Networks, 2005. SecureComm 2005. First International Conference on},
	Organization = {IEEE},
	Pages = {194--205},
	Title = {Protecting location privacy through path confusion},
	Year = {2005}}
	
	@article{terrovitis2011privacy,
	Author = {Terrovitis, Manolis},
	Journal = {ACM SIGKDD Explorations Newsletter},
	Number = {1},
	Pages = {6--18},
	Publisher = {ACM},
	Title = {Privacy preservation in the dissemination of location data},
	Volume = {13},
	Year = {2011}}
	
	@article{shin2012privacy,
	Author = {Shin, Kang G and Ju, Xiaoen and Chen, Zhigang and Hu, Xin},
	Journal = {Wireless Communications, IEEE},
	Number = {1},
	Pages = {30--39},
	Publisher = {IEEE},
	Title = {Privacy protection for users of location-based services},
	Volume = {19},
	Year = {2012}}
	
	@article{khoshgozaran2011location,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus and Shirani-Mehr, Houtan},
	Journal = {Knowledge and Information Systems},
	Number = {3},
	Pages = {435--465},
	Publisher = {Springer},
	Title = {Location privacy: going beyond K-anonymity, cloaking and anonymizers},
	Volume = {26},
	Year = {2011}}
	
	@incollection{chatzikokolakis2015geo,
	Author = {Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
	Booktitle = {Distributed Computing and Internet Technology},
	Pages = {49--72},
	Publisher = {Springer},
	Title = {Geo-indistinguishability: A Principled Approach to Location Privacy},
	Year = {2015}}
	
	@inproceedings{ngo2015location,
	Author = {Ngo, Hoa and Kim, Jong},
	Booktitle = {Computer Security Foundations Symposium (CSF), 2015 IEEE 28th},
	Organization = {IEEE},
	Pages = {63--74},
	Title = {Location Privacy via Differential Private Perturbation of Cloaking Area},
	Year = {2015}}
	
	@inproceedings{palanisamy2011mobimix,
	Author = {Palanisamy, Balaji and Liu, Ling},
	Booktitle = {Data Engineering (ICDE), 2011 IEEE 27th International Conference on},
	Organization = {IEEE},
	Pages = {494--505},
	Title = {Mobimix: Protecting location privacy with mix-zones over road networks},
	Year = {2011}}
	
	@inproceedings{um2010advanced,
	Author = {Um, Jung-Ho and Kim, Hee-Dae and Chang, Jae-Woo},
	Booktitle = {Social Computing (SocialCom), 2010 IEEE Second International Conference on},
	Organization = {IEEE},
	Pages = {1093--1098},
	Title = {An advanced cloaking algorithm using Hilbert curves for anonymous location based service},
	Year = {2010}}
	
	@inproceedings{bamba2008supporting,
	Author = {Bamba, Bhuvan and Liu, Ling and Pesti, Peter and Wang, Ting},
	Booktitle = {Proceedings of the 17th international conference on World Wide Web},
	Organization = {ACM},
	Pages = {237--246},
	Title = {Supporting anonymous location queries in mobile environments with privacygrid},
	Year = {2008}}
	
	@inproceedings{zhangwei2010distributed,
	Author = {Zhangwei, Huang and Mingjun, Xin},
	Booktitle = {Networks Security Wireless Communications and Trusted Computing (NSWCTC), 2010 Second International Conference on},
	Organization = {IEEE},
	Pages = {468--471},
	Title = {A distributed spatial cloaking protocol for location privacy},
	Volume = {2},
	Year = {2010}}
	
	@article{chow2011spatial,
	Author = {Chow, Chi-Yin and Mokbel, Mohamed F and Liu, Xuan},
	Journal = {GeoInformatica},
	Number = {2},
	Pages = {351--380},
	Publisher = {Springer},
	Title = {Spatial cloaking for anonymous location-based services in mobile peer-to-peer environments},
	Volume = {15},
	Year = {2011}}
	
	@inproceedings{lu2008pad,
	Author = {Lu, Hua and Jensen, Christian S and Yiu, Man Lung},
	Booktitle = {Proceedings of the Seventh ACM International Workshop on Data Engineering for Wireless and Mobile Access},
	Organization = {ACM},
	Pages = {16--23},
	Title = {Pad: privacy-area aware, dummy-based location privacy in mobile services},
	Year = {2008}}
	
	@incollection{khoshgozaran2007blind,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus},
	Booktitle = {Advances in Spatial and Temporal Databases},
	Pages = {239--257},
	Publisher = {Springer},
	Title = {Blind evaluation of nearest neighbor queries using space transformation to preserve location privacy},
	Year = {2007}}
	
	@inproceedings{ghinita2008private,
	Author = {Ghinita, Gabriel and Kalnis, Panos and Khoshgozaran, Ali and Shahabi, Cyrus and Tan, Kian-Lee},
	Booktitle = {Proceedings of the 2008 ACM SIGMOD international conference on Management of data},
	Organization = {ACM},
	Pages = {121--132},
	Title = {Private queries in location based services: anonymizers are not necessary},
	Year = {2008}}
	
	@article{paulet2014privacy,
	Author = {Paulet, Russell and Kaosar, Md Golam and Yi, Xun and Bertino, Elisa},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {5},
	Pages = {1200--1210},
	Publisher = {IEEE},
	Title = {Privacy-preserving and content-protecting location based queries},
	Volume = {26},
	Year = {2014}}
	
	@article{nguyen2013differential,
	Author = {Nguyen, Hiep H and Kim, Jong and Kim, Yoonho},
	Journal = {Journal of Computing Science and Engineering},
	Number = {3},
	Pages = {177--186},
	Title = {Differential privacy in practice},
	Volume = {7},
	Year = {2013}}
	
	@inproceedings{lee2012differential,
	Author = {Lee, Jaewoo and Clifton, Chris},
	Booktitle = {Proceedings of the 18th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {1041--1049},
	Title = {Differential identifiability},
	Year = {2012}}
	
	@inproceedings{andres2013geo,
	Author = {Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2013 ACM SIGSAC conference on Computer \& communications security},
	Organization = {ACM},
	Pages = {901--914},
	Title = {Geo-indistinguishability: Differential privacy for location-based systems},
	Year = {2013}}
	
	@inproceedings{machanavajjhala2008privacy,
	Author = {Machanavajjhala, Ashwin and Kifer, Daniel and Abowd, John and Gehrke, Johannes and Vilhuber, Lars},
	Booktitle = {Data Engineering, 2008. ICDE 2008. IEEE 24th International Conference on},
	Organization = {IEEE},
	Pages = {277--286},
	Title = {Privacy: Theory meets practice on the map},
	Year = {2008}}
	
	@article{dewri2013local,
	Author = {Dewri, Rinku},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {12},
	Pages = {2360--2372},
	Publisher = {IEEE},
	Title = {Local differential perturbations: Location privacy under approximate knowledge attackers},
	Volume = {12},
	Year = {2013}}
	
	@inproceedings{chatzikokolakis2013broadening,
	Author = {Chatzikokolakis, Konstantinos and Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s Emilio and Palamidessi, Catuscia},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {82--102},
	Title = {Broadening the Scope of Differential Privacy Using Metrics.},
	Year = {2013}}
	
	@inproceedings{zhong2009distributed,
	Author = {Zhong, Ge and Hengartner, Urs},
	Booktitle = {Pervasive Computing and Communications, 2009. PerCom 2009. IEEE International Conference on},
	Organization = {IEEE},
	Pages = {1--10},
	Title = {A distributed k-anonymity protocol for location privacy},
	Year = {2009}}
	
	@inproceedings{ho2011differential,
	Author = {Ho, Shen-Shyang and Ruan, Shuhua},
	Booktitle = {Proceedings of the 4th ACM SIGSPATIAL International Workshop on Security and Privacy in GIS and LBS},
	Organization = {ACM},
	Pages = {17--24},
	Title = {Differential privacy for location pattern mining},
	Year = {2011}}
	
	@inproceedings{cheng2006preserving,
	Author = {Cheng, Reynold and Zhang, Yu and Bertino, Elisa and Prabhakar, Sunil},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {393--412},
	Title = {Preserving user location privacy in mobile data management infrastructures},
	Year = {2006}}
	
	@article{beresford2003location,
	Author = {Beresford, Alastair R and Stajano, Frank},
	Journal = {IEEE Pervasive computing},
	Number = {1},
	Pages = {46--55},
	Publisher = {IEEE},
	Title = {Location privacy in pervasive computing},
	Year = {2003}}
	
	@inproceedings{freudiger2009optimal,
	Author = {Freudiger, Julien and Shokri, Reza and Hubaux, Jean-Pierre},
	Booktitle = {Privacy enhancing technologies},
	Organization = {Springer},
	Pages = {216--234},
	Title = {On the optimal placement of mix zones},
	Year = {2009}}
	
	@article{krumm2009survey,
	Author = {Krumm, John},
	Journal = {Personal and Ubiquitous Computing},
	Number = {6},
	Pages = {391--399},
	Publisher = {Springer},
	Title = {A survey of computational location privacy},
	Volume = {13},
	Year = {2009}}
	
	@article{Rakhshan2016letter,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Wireless Communications Letter},
	Publisher = {IEEE},
	Title = {Interference Models for Vehicular Ad Hoc Networks},
	Year = {2016, submitted}}
	
	@article{Rakhshan2015Journal,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Publisher = {IEEE},
	Title = {Improving Safety on Highways by Customizing Vehicular Ad Hoc Networks},
	Year = {to appear, 2017}}
	
	@inproceedings{Rakhshan2015Cogsima,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Booktitle = {IEEE International Multi-Disciplinary Conference on Cognitive Methods in Situation Awareness and Decision Support},
	Organization = {IEEE},
	Title = {A New Approach to Customization of Accident Warning Systems to Individual Drivers},
	Year = {2015}}
	
	@inproceedings{Rakhshan2015CISS,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Nekoui, Mohammad},
	Booktitle = {Conference on Information Sciences and Systems},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {Driver-based adaptation of Vehicular Ad Hoc Networks for design of active safety systems},
	Year = {2015}}
	
	@inproceedings{Rakhshan2014IV,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Ray, Evan},
	Booktitle = {Intelligent Vehicles Symposium},
	Organization = {IEEE},
	Pages = {1181--1186},
	Title = {Real-time estimation of the distribution of brake response times for an individual driver using Vehicular Ad Hoc Network.},
	Year = {2014}}
	
	@inproceedings{Rakhshan2013Globecom,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Fisher, Donald and Nekoui, Mohammad},
	Booktitle = {IEEE Global Communications Conference},
	Organization = {IEEE},
	Pages = {1333--1337},
	Title = {Tuning collision warning algorithms to individual drivers for design of active safety systems.},
	Year = {2013}}
	
	@article{Nekoui2012Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Number = {8},
	Pages = {2895--2905},
	Publisher = {IEEE},
	Title = {Throughput Scaling laws for Vehicular Ad Hoc Networks},
	Volume = {11},
	Year = {2012}}
	
	
	
	
	
	
	
	
	
	@article{Nekoui2011Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein and Ni, Daiheng},
	Journal = {International Journal of Vehicular Technology},
	Pages = {1--11},
	Publisher = {Hindawi Publishing Corporation},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {2011},
	Year = {2011}}
	
	
	
	
	
	
	@article{shokri2014optimal,
	title={Optimal user-centric data obfuscation},
	author={Shokri, Reza},
	journal={arXiv preprint arXiv:1402.3426},
	year={2014}
	}
	@article{chatzikokolakis2015location,
	title={Location privacy via geo-indistinguishability},
	author={Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
	journal={ACM SIGLOG News},
	volume={2},
	number={3},
	pages={46--69},
	year={2015},
	publisher={ACM}
	
	}
	@inproceedings{shokri2011quantifying2,
	title={Quantifying location privacy: the case of sporadic location exposure},
	author={Shokri, Reza and Theodorakopoulos, George and Danezis, George and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
	booktitle={Privacy Enhancing Technologies},
	pages={57--76},
	year={2011},
	organization={Springer}
	}
	
	
	@inproceedings{Mont1603:Defining,
	AUTHOR="Zarrin Montazeri and Amir Houmansadr and Hossein Pishro-Nik",
	TITLE="Defining Perfect Location Privacy Using Anonymization",
	BOOKTITLE="2016 Annual Conference on Information Science and Systems (CISS) (CISS
	2016)",
	ADDRESS="Princeton, USA",
	DAYS=16,
	MONTH=mar,
	YEAR=2016,
	KEYWORDS="Information Theoretic Privacy; location-based services; Location Privacy;
	Information Theory",
	ABSTRACT="The popularity of mobile devices and location-based services (LBS) have
	created great concerns regarding the location privacy of users of such
	devices and services. Anonymization is a common technique that is often
	being used to protect the location privacy of LBS users. In this paper, we
	provide a general information theoretic definition for location privacy. In
	particular, we define perfect location privacy. We show that under certain
	conditions, perfect privacy is achieved if the pseudonyms of users is
	changed after o(N^(2/r?1)) observations by the adversary, where N is the
	number of users and r is the number of sub-regions or locations.
	"
	}
	@article{our-isita-location,
	Author = {Zarrin Montazeri and Amir Houmansadr and Hossein Pishro-Nik},
	Journal = {IEEE International Symposium on Information Theory and Its Applications (ISITA)},
	Title = {Achieving Perfect Location Privacy in Markov Models Using Anonymization},
	Year = {2016}
	}
	@article{our-TIFS,
	Author = {Zarrin Montazeri and Hossein Pishro-Nik and Amir Houmansadr},
	Journal = {IEEE Transactions on Information Forensics and Security, accepted with mandatory minor revisions},
	Title = {Perfect Location Privacy Using Anonymization in Mobile Networks},
	Year = {2017},
	note={Available on arxiv.org}
	}
	
	
	
	@techreport{sampigethaya2005caravan,
	title={CARAVAN: Providing location privacy for VANET},
	author={Sampigethaya, Krishna and Huang, Leping and Li, Mingyan and Poovendran, Radha and Matsuura, Kanta and Sezaki, Kaoru},
	year={2005},
	institution={DTIC Document}
	}
	@incollection{buttyan2007effectiveness,
	title={On the effectiveness of changing pseudonyms to provide location privacy in VANETs},
	author={Butty{\'a}n, Levente and Holczer, Tam{\'a}s and Vajda, Istv{\'a}n},
	booktitle={Security and Privacy in Ad-hoc and Sensor Networks},
	pages={129--141},
	year={2007},
	publisher={Springer}
	}
	@article{sampigethaya2007amoeba,
	title={AMOEBA: Robust location privacy scheme for VANET},
	author={Sampigethaya, Krishna and Li, Mingyan and Huang, Leping and Poovendran, Radha},
	journal={Selected Areas in communications, IEEE Journal on},
	volume={25},
	number={8},
	pages={1569--1589},
	year={2007},
	publisher={IEEE}
	}
	
	@article{lu2012pseudonym,
	title={Pseudonym changing at social spots: An effective strategy for location privacy in vanets},
	author={Lu, Rongxing and Li, Xiaodong and Luan, Tom H and Liang, Xiaohui and Shen, Xuemin},
	journal={Vehicular Technology, IEEE Transactions on},
	volume={61},
	number={1},
	pages={86--96},
	year={2012},
	publisher={IEEE}
	}
	@inproceedings{lu2010sacrificing,
	title={Sacrificing the plum tree for the peach tree: A socialspot tactic for protecting receiver-location privacy in VANET},
	author={Lu, Rongxing and Lin, Xiaodong and Liang, Xiaohui and Shen, Xuemin},
	booktitle={Global Telecommunications Conference (GLOBECOM 2010), 2010 IEEE},
	pages={1--5},
	year={2010},
	organization={IEEE}
	}
	@inproceedings{lin2011stap,
	title={STAP: A social-tier-assisted packet forwarding protocol for achieving receiver-location privacy preservation in VANETs},
	author={Lin, Xiaodong and Lu, Rongxing and Liang, Xiaohui and Shen, Xuemin Sherman},
	booktitle={INFOCOM, 2011 Proceedings IEEE},
	pages={2147--2155},
	year={2011},
	organization={IEEE}
	}
	@inproceedings{gerlach2007privacy,
	title={Privacy in VANETs using changing pseudonyms-ideal and real},
	author={Gerlach, Matthias and Guttler, Felix},
	booktitle={Vehicular Technology Conference, 2007. VTC2007-Spring. IEEE 65th},
	pages={2521--2525},
	year={2007},
	organization={IEEE}
	}
	@inproceedings{el2002security,
	title={Security issues in a future vehicular network},
	author={El Zarki, Magda and Mehrotra, Sharad and Tsudik, Gene and Venkatasubramanian, Nalini},
	booktitle={European Wireless},
	volume={2},
	year={2002}
	}
	
	@article{hubaux2004security,
	title={The security and privacy of smart vehicles},
	author={Hubaux, Jean-Pierre and Capkun, Srdjan and Luo, Jun},
	journal={IEEE Security \& Privacy Magazine},
	volume={2},
	number={LCA-ARTICLE-2004-007},
	pages={49--55},
	year={2004}
	}
	
	
	
	@inproceedings{duri2002framework,
	title={Framework for security and privacy in automotive telematics},
	author={Duri, Sastry and Gruteser, Marco and Liu, Xuan and Moskowitz, Paul and Perez, Ronald and Singh, Moninder and Tang, Jung-Mu},
	booktitle={Proceedings of the 2nd international workshop on Mobile commerce},
	pages={25--32},
	year={2002},
	organization={ACM}
	}
	@misc{NS-3,
	Howpublished = {\url{https://www.nsnam.org/}}},
}
@misc{testbed,
	Howpublished = {\url{http://www.its.dot.gov/testbed/PDF/SE-MI-Resource-Guide-9-3-1.pdf}}},
@misc{NGSIM,
	Howpublished = {\url{http://ops.fhwa.dot.gov/trafficanalysistools/ngsim.htm}},
}

@misc{National-a2013,
	Author = {National Highway Traffic Safety Administration},
	Howpublished = {\url{http://ops.fhwa.dot.gov/trafficanalysistools/ngsim.htm}},
	Title = {2013 Motor Vehicle Crashes: Overview. Traffic Safety Factors},
	Year = {2013}
}

@inproceedings{karnadi2007rapid,
	title={Rapid generation of realistic mobility models for VANET},
	author={Karnadi, Feliz Kristianto and Mo, Zhi Hai and Lan, Kun-chan},
	booktitle={Wireless Communications and Networking Conference, 2007. WCNC 2007. IEEE},
	pages={2506--2511},
	year={2007},
	organization={IEEE}
}
@inproceedings{saha2004modeling,
	title={Modeling mobility for vehicular ad-hoc networks},
	author={Saha, Amit Kumar and Johnson, David B},
	booktitle={Proceedings of the 1st ACM international workshop on Vehicular ad hoc networks},
	pages={91--92},
	year={2004},
	organization={ACM}
}
@inproceedings{lee2006modeling,
	title={Modeling steady-state and transient behaviors of user mobility: formulation, analysis, and application},
	author={Lee, Jong-Kwon and Hou, Jennifer C},
	booktitle={Proceedings of the 7th ACM international symposium on Mobile ad hoc networking and computing},
	pages={85--96},
	year={2006},
	organization={ACM}
}
@inproceedings{yoon2006building,
	title={Building realistic mobility models from coarse-grained traces},
	author={Yoon, Jungkeun and Noble, Brian D and Liu, Mingyan and Kim, Minkyong},
	booktitle={Proceedings of the 4th international conference on Mobile systems, applications and services},
	pages={177--190},
	year={2006},
	organization={ACM}
}

@inproceedings{choffnes2005integrated,
	title={An integrated mobility and traffic model for vehicular wireless networks},
	author={Choffnes, David R and Bustamante, Fabi{\'a}n E},
	booktitle={Proceedings of the 2nd ACM international workshop on Vehicular ad hoc networks},
	pages={69--78},
	year={2005},
	organization={ACM}
}

@inproceedings{Qian2008Globecom,
	title={CA Secure VANET MAC Protocol for DSRC Applications},
	author={Yi, Q. and Lu, K. and Moyeri, N.{\'a}n E},
	booktitle={Proceedings of IEEE GLOBECOM 2008},
	pages={1--5},
	year={2008},
	organization={IEEE}
}





@inproceedings{naumov2006evaluation,
	title={An evaluation of inter-vehicle ad hoc networks based on realistic vehicular traces},
	author={Naumov, Valery and Baumann, Rainer and Gross, Thomas},
	booktitle={Proceedings of the 7th ACM international symposium on Mobile ad hoc networking and computing},
	pages={108--119},
	year={2006},
	organization={ACM}
}
@article{sommer2008progressing,
	title={Progressing toward realistic mobility models in VANET simulations},
	author={Sommer, Christoph and Dressler, Falko},
	journal={Communications Magazine, IEEE},
	volume={46},
	number={11},
	pages={132--137},
	year={2008},
	publisher={IEEE}
}




@inproceedings{mahajan2006urban,
	title={Urban mobility models for vanets},
	author={Mahajan, Atulya and Potnis, Niranjan and Gopalan, Kartik and Wang, Andy},
	booktitle={2nd IEEE International Workshop on Next Generation Wireless Networks},
	volume={33},
	year={2006}
}

@inproceedings{Rakhshan2016packet,
	title={Packet success probability derivation in a vehicular ad hoc network for a highway scenario},
	author={Rakhshan, Ali and Pishro-Nik, Hossein},
	booktitle={2016 Annual Conference on Information Science and Systems (CISS)},
	pages={210--215},
	year={2016},
	organization={IEEE}
}

@inproceedings{Rakhshan2016CISS,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Booktitle = {Conference on Information Sciences and Systems},
	Organization = {IEEE},
	Pages = {210--215},
	Title = {Packet Success Probability Derivation in a Vehicular Ad Hoc Network for a Highway Scenario},
	Year = {2016}}

@article{Nekoui2013Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {Journal on Selected Areas in Communications, Special Issue on Emerging Technologies in Communications},
	Number = {9},
	Pages = {491--503},
	Publisher = {IEEE},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {31},
	Year = {2013}}


@inproceedings{Nekoui2011MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM workshop on VehiculAr InterNETworking},
	Organization = {ACM},
	Title = {Analytic Design of Active Vehicular Safety Systems in Sparse Traffic},
	Year = {2011}}

@inproceedings{Nekoui2011VTC,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Analytical Design of Inter-vehicular Communications for Collision Avoidance},
	Year = {2011}}

@inproceedings{Bovee2011VTC,
	Author = {Bovee, Ben Louis and Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Evaluation of the Universal Geocast Scheme For VANETs},
	Year = {2011}}

@inproceedings{Nekoui2010MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM},
	Organization = {ACM},
	Title = {Fundamental Tradeoffs in Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2010IVCS,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IVCS},
	Organization = {IEEE},
	Title = {A Universal Geocast Scheme for Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2009ITW,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IEEE Communications Society Conference on Sensor, Mesh and Ad Hoc Communications and Networks Workshops},
	Organization = {IEEE},
	Pages = {1--3},
	Title = {A Geometrical Analysis of Obstructed Wireless Networks},
	Year = {2009}}

@article{Eslami2013Journal,
	Author = {Eslami, Ali and Nekoui, Mohammad and Pishro-Nik, Hossein and Fekri, Faramarz},
	Journal = {ACM Transactions on Sensor Networks},
	Number = {4},
	Pages = {51},
	Publisher = {ACM},
	Title = {Results on finite wireless sensor networks: Connectivity and coverage},
	Volume = {9},
	Year = {2013}}


@article{Jiafu2014Journal,
	Author = {Jiafu, W. and Zhang, D. and Zhao, S. and Yang, L. and Lloret, J.},
	Journal = {Communications Magazine},
	Number = {8},
	Pages = {106-113},
	Publisher = {IEEE},
	Title = {Context-aware vehicular cyber-physical systems with cloud support: architecture, challenges, and solutions},
	Volume = {52},
	Year = {2014}}

@inproceedings{Haas2010ACM,
	Author = {Haas, J.J. and Hu, Y.},
	Booktitle = {international workshop on VehiculAr InterNETworking},
	Organization = {ACM},
	Title = {Communication requirements for crash avoidance.},
	Year = {2010}}

@inproceedings{Yi2008GLOBECOM,
	Author = {Yi, Q. and Lu, K. and Moayeri, N.},
	Booktitle = {GLOBECOM},
	Organization = {IEEE},
	Title = {CA Secure VANET MAC Protocol for DSRC Applications.},
	Year = {2008}}

@inproceedings{Mughal2010ITSim,
	Author = {Mughal, B.M. and Wagan, A. and Hasbullah, H.},
	Booktitle = {International Symposium on Information Technology (ITSim)},
	Organization = {IEEE},
	Title = {Efficient congestion control in VANET for safety messaging.},
	Year = {2010}}

@article{Chang2011Journal,
	Author = {Chang, Y. and Lee, C. and Copeland, J.},
	Journal = {Selected Areas in Communications},
	Pages = {236 â€“249},
	Publisher = {IEEE},
	Title = {Goodput enhancement of VANETs in noisy CSMA/CA channels},
	Volume = {29},
	Year = {2011}}

@article{Garcia-Costa2011Journal,
	Author = {Garcia-Costa, C. and Egea-Lopez, E. and Tomas-Gabarron, J. B. and Garcia-Haro, J. and Haas, Z. J.},
	Journal = {Transactions on Intelligent Transportation Systems},
	Pages = {1 â€“16},
	Publisher = {IEEE},
	Title = {A stochastic model for chain collisions of vehicles equipped with vehicular communications},
	Volume = {99},
	Year = {2011}}

@article{Carbaugh2011Journal,
	Author = {Carbaugh, J. and Godbole,  D. N. and Sengupta, R. and Garcia-Haro, J. and Haas, Z. J.},
	Publisher = {Transportation Research Part C (Emerging Technologies)},
	Title = {Safety and capacity analysis of automated and manual highway systems},
	Year = {1997}}

@article{Goh2004Journal,
	Author = {Goh, P. and Wong, Y.},
	Publisher = {Appl Health Econ Health Policy},
	Title = {Driver perception response time during the signal change interval},
	Year = {2004}}

@article{Chang1985Journal,
	Author = {Chang, M.S. and Santiago, A.J.},
	Pages = {20-30},
	Publisher = {Transportation Research Record},
	Title = {Timing traffic signal changes based on driver behavior},
	Volume = {1027},
	Year = {1985}}

@article{Green2000Journal,
	Author = {Green, M.},
	Pages = {195-216},
	Publisher = {Transportation Human Factors},
	Title = {How long does it take to stop? Methodological analysis of driver perception-brake times.},
	Year = {2000}}

@article{Koppa2005,
	Author = {Koppa, R.J.},
	Pages = {195-216},
	Publisher = {http://www.fhwa.dot.gov/publications/},
	Title = {Human Factors},
	Year = {2005}}

@inproceedings{Maxwell2010ETC,
	Author = {Maxwell, A. and Wood, K.},
	Booktitle = {Europian Transport Conference},
	Organization = {http://www.etcproceedings.org/paper/review-of-traffic-signals-on-high-speed-roads},
	Title = {Review of Traffic Signals on High Speed Road},
	Year = {2010}}

@article{Wortman1983,
	Author = {Wortman, R.H. and Matthias, J.S.},
	Publisher = {Arizona Department of Transportation},
	Title = {An Evaluation of Driver Behavior at Signalized Intersections},
	Year = {1983}}
@inproceedings{Zhang2007IASTED,
	Author = {Zhang, X. and Bham, G.H.},
	Booktitle = {18th IASTED International Conference: modeling and simulation},
	Title = {Estimation of driver reaction time from detailed vehicle trajectory data.},
	Year = {2007}}


@inproceedings{bai2003important,
	title={IMPORTANT: A framework to systematically analyze the Impact of Mobility on Performance of RouTing protocols for Adhoc NeTworks},
	author={Bai, Fan and Sadagopan, Narayanan and Helmy, Ahmed},
	booktitle={INFOCOM 2003. Twenty-second annual joint conference of the IEEE computer and communications. IEEE societies},
	volume={2},
	pages={825--835},
	year={2003},
	organization={IEEE}
}


@inproceedings{abedi2008enhancing,
	title={Enhancing AODV routing protocol using mobility parameters in VANET},
	author={Abedi, Omid and Fathy, Mahmood and Taghiloo, Jamshid},
	booktitle={Computer Systems and Applications, 2008. AICCSA 2008. IEEE/ACS International Conference on},
	pages={229--235},
	year={2008},
	organization={IEEE}
}


@article{AlSultan2013Journal,
	Author = {Al-Sultan, Saif and Al-Bayatti, Ali H. and Zedan, Hussien},
	Journal = {IEEE Transactions on Vehicular Technology},
	Number = {9},
	Pages = {4264-4275},
	Publisher = {IEEE},
	Title = {Context Aware Driver Behaviour Detection System in Intelligent Transportation Systems},
	Volume = {62},
	Year = {2013}}






@article{Leow2008ITS,
	Author = {Leow, Woei Ling and Ni, Daiheng and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Intelligent Transportation Systems},
	Number = {2},
	Pages = {369--374},
	Publisher = {IEEE},
	Title = {A Sampling Theorem Approach to Traffic Sensor Optimization},
	Volume = {9},
	Year = {2008}}



@article{REU2007,
	Author = {D. Ni and H. Pishro-Nik and R. Prasad and M. R. Kanjee and H. Zhu and T. Nguyen},
	Journal = {in 14th World Congress on Intelligent Transport Systems},
	Title = {Development of a prototype intersection collision avoidance system under VII},
	Year = {2007}}




@inproceedings{salamatian2013hide,
	title={How to hide the elephant-or the donkey-in the room: Practical privacy against statistical inference for large data.},
	author={Salamatian, Salman and Zhang, Amy and du Pin Calmon, Flavio and Bhamidipati, Sandilya and Fawaz, Nadia and Kveton, Branislav and Oliveira, Pedro and Taft, Nina},
	booktitle={GlobalSIP},
	pages={269--272},
	year={2013}
}

@article{sankar2013utility,
	title={Utility-privacy tradeoffs in databases: An information-theoretic approach},
	author={Sankar, Lalitha and Rajagopalan, S Raj and Poor, H Vincent},
	journal={Information Forensics and Security, IEEE Transactions on},
	volume={8},
	number={6},
	pages={838--852},
	year={2013},
	publisher={IEEE}
}
@inproceedings{ghinita2007prive,
	title={PRIVE: anonymous location-based queries in distributed mobile systems},
	author={Ghinita, Gabriel and Kalnis, Panos and Skiadopoulos, Spiros},
	booktitle={Proceedings of the 16th international conference on World Wide Web},
	pages={371--380},
	year={2007},
	organization={ACM}
}

@article{beresford2004mix,
	title={Mix zones: User privacy in location-aware services},
	author={Beresford, Alastair R and Stajano, Frank},
	year={2004},
	publisher={IEEE}
}

%@inproceedings{Mont1610Achieving,
	%  title={Achieving Perfect Location Privacy in Markov Models Using Anonymization},
	%  author={Montazeri, Zarrin and Houmansadr, Amir and H.Pishro-Nik},
	%  booktitle="2016 International Symposium on Information Theory and its Applications
	%  (ISITA2016)",
	%  address="Monterey, USA",
	%  days=30,
	%  month=oct,
	%  year=2016,
	%}

@article{csiszar1996almost,
	title={Almost independence and secrecy capacity},
	author={Csisz{\'a}r, Imre},
	journal={Problemy Peredachi Informatsii},
	volume={32},
	number={1},
	pages={48--57},
	year={1996},
	publisher={Russian Academy of Sciences, Branch of Informatics, Computer Equipment and Automatization}
}

@article{yamamoto1983source,
	title={A source coding problem for sources with additional outputs to keep secret from the receiver or wiretappers (corresp.)},
	author={Yamamoto, Hirosuke},
	journal={IEEE Transactions on Information Theory},
	volume={29},
	number={6},
	pages={918--923},
	year={1983},
	publisher={IEEE}
}


@inproceedings{calmon2015fundamental,
	title={Fundamental limits of perfect privacy},
	author={Calmon, Flavio P and Makhdoumi, Ali and M{\'e}dard, Muriel},
	booktitle={Information Theory (ISIT), 2015 IEEE International Symposium on},
	pages={1796--1800},
	year={2015},
	organization={IEEE}
}



@inproceedings{Lehman1999Large-Sample-Theory,
	title={Elements of Large Sample Theory},
	author={E. L. Lehman},
	organization={Springer},
	year={1999}
}


@inproceedings{Ferguson1999Large-Sample-Theory,
	title={A Course in Large Sample Theory},
	author={Thomas S. Ferguson},
	organization={CRC Press},
	year={1996}
}



@inproceedings{Dembo1999Large-Deviations,
	title={Large Deviation Techniques and Applications, Second Edition},
	author={A. Dembo and O. Zeitouni},
	organization={Springer},
	year={1998}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Hossein's Coding Journals
%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{myoptics,
	AUTHOR =       "H. Pishro-Nik and N. Rahnavard and J. Ha and F. Fekri and A. Adibi ",
	TITLE =        "Low-density parity-check codes for volume holographic memory systems",
	JOURNAL =      " Appl. Opt.",
	YEAR =         "2003",
	volume =       "42",
	pages =        "861-870  "
}






@ARTICLE{myit,
	AUTHOR =       "H. Pishro-Nik and F. Fekri  ",
	TITLE =        "On Decoding of Low-Density Parity-Check Codes on the Binary Erasure Channel",
	JOURNAL =      "IEEE Trans. Inform. Theory",
	YEAR =         "2004",
	volume =       "50",
	pages =        "439--454"
}




@ARTICLE{myitpuncture,
	AUTHOR =       "H. Pishro-Nik and F. Fekri  ",
	TITLE =        "Results on Punctured Low-Density Parity-Check Codes and Improved Iterative Decoding Techniques",
	JOURNAL =      "IEEE Trans. on Inform. Theory",
	YEAR =         "2007",
	volume =       "53",
	number=        "2",
	pages =        "599--614",
	month= "February"
}




@ARTICLE{myitlinmimdist,
	AUTHOR =       "H. Pishro-Nik and F. Fekri",
	TITLE =        "Performance of Low-Density Parity-Check Codes With Linear Minimum Distance",
	JOURNAL =         "IEEE Trans. Inform. Theory ",
	YEAR =         "2006",
	volume =       "52",
	number="1",
	pages =        "292 --300"
}






@ARTICLE{myitnonuni,
	AUTHOR =       "H. Pishro-Nik and N. Rahnavard and F. Fekri  ",
	TITLE =        "Non-uniform Error Correction Using Low-Density Parity-Check Codes",
	JOURNAL =      "IEEE Trans. Inform. Theory",
	YEAR =         "2005",
	volume =       "51",
	number=  "7",
	pages =        "2702--2714"
}





@article{eslamitcomhybrid10,
	author = {A. Eslami and S. Vangala and H. Pishro-Nik},
	title = {Hybrid channel codes for highly efficient FSO/RF communication systems},
	journal = {IEEE Transactions on Communications},
	volume = {58},
	number = {10},
	year = {2010},
	pages = {2926--2938},
}


@article{eslamitcompolar13,
	author = {A. Eslami and H. Pishro-Nik},
	title = {On Finite-Length Performance of Polar Codes: Stopping Sets, Error Floor, and Concatenated Design},
	journal = {IEEE Transactions on Communications},
	volume = {61},
	number = {13},
	year = {2013},
	pages = {919--929},
}



@article{saeeditcom11,
	author = {H. Saeedi and H. Pishro-Nik and  A. H. Banihashemi},
	title = {Successive maximization for the systematic design of universally capacity approaching rate-compatible
	sequences of LDPC code ensembles over binary-input output-symmetric memoryless channels},
	journal = {IEEE Transactions on Communications},
	year = {2011},
	volume={59},
	number = {7}
}


@article{rahnavard07,
	author = {Rahnavard, N. and Pishro-Nik, H. and Fekri, F.},
	title = {Unequal Error Protection Using Partially Regular LDPC Codes},
	journal = {IEEE Transactions on Communications},
	year = {2007},
	volume = {55},
	number = {3},
	pages = {387 -- 391}
}


@article{hosseinira04,
	author = {H. Pishro-Nik and F. Fekri},
	title = {Irregular repeat-accumulate codes for volume holographic memory systems},
	journal = {Journal of Applied Optics},
	year = {2004},
	volume = {43},
	number = {27},
	pages = {5222--5227},
}


@article{azadeh2015Ephemeralkey,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
	journal = {IEEE Transactions on Wireless Communications},
	year = {2015},
	volume = {14},
	number = {11},
	pages = {6072--6081},
}


@article{azadeh2014Everlasting,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Everlasting secrecy in disadvantaged wireless environments against sophisticated eavesdroppers},
	journal = {48th Asilomar Conference on Signals, Systems and Computers},
	year = {2014},
	pages = {1994--1998},
}


@article{azadeh2013ISIT,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Artificial intersymbol interference (ISI) to exploit receiver imperfections for secrecy},
	journal = {IEEE International Symposium on Information Theory (ISIT)},
	year = {2013},
}


@article{azadeh2013Jsac,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
	journal = {IEEE Journal on Selected Areas in Communications},
	year = {2013},
	volume = {31},
	number = {9},
	pages = {1828--1839},
}


@article{azadeh2012Allerton,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Exploiting the non-commutativity of nonlinear operators for information-theoretic security in disadvantaged wireless environments},
	journal = {50th Annual Allerton Conference on Communication, Control, and Computing},
	year = {2012},
	pages = {233--240},
}


@article{azadeh2012Infocom,
	author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
	title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
	journal = {IEEE INFOCOM},
	year = {2012},
	pages = {1179--1187},
}

@article{1corser2016evaluating,
	title={Evaluating Location Privacy in Vehicular Communications and Applications},
	author={Corser, George P and Fu, Huirong and Banihani, Abdelnasser},
	journal={IEEE Transactions on Intelligent Transportation Systems},
	volume={17},
	number={9},
	pages={2658-2667},
	year={2016},
	publisher={IEEE}
}
@article{2zhang2016designing,
	title={On Designing Satisfaction-Ratio-Aware Truthful Incentive Mechanisms for k-Anonymity Location Privacy},
	author={Zhang, Yuan and Tong, Wei and Zhong, Sheng},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={11},
	number={11},
	pages={2528--2541},
	year={2016},
	publisher={IEEE}
}
@article{3li2016privacy,
	title={Privacy-preserving Location Proof for Securing Large-scale Database-driven Cognitive Radio Networks},
	author={Li, Yi and Zhou, Lu and Zhu, Haojin and Sun, Limin},
	journal={IEEE Internet of Things Journal},
	volume={3},
	number={4},
	pages={563-571},
	year={2016},
	publisher={IEEE}
}
@article{4olteanu2016quantifying,
	title={Quantifying Interdependent Privacy Risks with Location Data},
	author={Olteanu, Alexandra-Mihaela and Huguenin, K{\'e}vin and Shokri, Reza and Humbert, Mathias and Hubaux, Jean-Pierre},
	journal={IEEE Transactions on Mobile Computing},
	year={2016},
	volume={PP},
	number={99},
	pages={1-1},
	publisher={IEEE}
}
@article{5yi2016practical,
	title={Practical Approximate k Nearest Neighbor Queries with Location and Query Privacy},
	author={Yi, Xun and Paulet, Russell and Bertino, Elisa and Varadharajan, Vijay},
	journal={IEEE Transactions on Knowledge and Data Engineering},
	volume={28},
	number={6},
	pages={1546--1559},
	year={2016},
	publisher={IEEE}
}
@article{6li2016privacy,
	title={Privacy Leakage of Location Sharing in Mobile Social Networks: Attacks and Defense},
	author={Li, Huaxin and Zhu, Haojin and Du, Suguo and Liang, Xiaohui and Shen, Xuemin},
	journal={IEEE Transactions on Dependable and Secure Computing},
	year={2016},
	volume={PP},
	number={99},
	publisher={IEEE}
}

@article{7murakami2016localization,
	title={Localization Attacks Using Matrix and Tensor Factorization},
	author={Murakami, Takao and Watanabe, Hajime},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={11},
	number={8},
	pages={1647--1660},
	year={2016},
	publisher={IEEE}
}
@article{8zurbaran2015near,
	title={Near-Rand: Noise-based Location Obfuscation Based on Random Neighboring Points},
	author={Zurbaran, Mayra Alejandra and Avila, Karen and Wightman, Pedro and Fernandez, Michael},
	journal={IEEE Latin America Transactions},
	volume={13},
	number={11},
	pages={3661--3667},
	year={2015},
	publisher={IEEE}
}

@article{9tan2014anti,
	title={An anti-tracking source-location privacy protection protocol in wsns based on path extension},
	author={Tan, Wei and Xu, Ke and Wang, Dan},
	journal={IEEE Internet of Things Journal},
	volume={1},
	number={5},
	pages={461--471},
	year={2014},
	publisher={IEEE}
}

@article{10peng2014enhanced,
	title={Enhanced Location Privacy Preserving Scheme in Location-Based Services},
	author={Peng, Tao and Liu, Qin and Wang, Guojun},
	journal={IEEE Systems Journal},
	year={2014},
	volume={PP},
	number={99},
	pages={1-12},
	publisher={IEEE}
}
@article{11dewri2014exploiting,
	title={Exploiting service similarity for privacy in location-based search queries},
	author={Dewri, Rinku and Thurimella, Ramakrisha},
	journal={IEEE Transactions on Parallel and Distributed Systems},
	volume={25},
	number={2},
	pages={374--383},
	year={2014},
	publisher={IEEE}
}

@article{12hwang2014novel,
	title={A novel time-obfuscated algorithm for trajectory privacy protection},
	author={Hwang, Ren-Hung and Hsueh, Yu-Ling and Chung, Hao-Wei},
	journal={IEEE Transactions on Services Computing},
	volume={7},
	number={2},
	pages={126--139},
	year={2014},
	publisher={IEEE}
}
@article{13puttaswamy2014preserving,
	title={Preserving location privacy in geosocial applications},
	author={Puttaswamy, Krishna PN and Wang, Shiyuan and Steinbauer, Troy and Agrawal, Divyakant and El Abbadi, Amr and Kruegel, Christopher and Zhao, Ben Y},
	journal={IEEE Transactions on Mobile Computing},
	volume={13},
	number={1},
	pages={159--173},
	year={2014},
	publisher={IEEE}
}

@article{14zhang2014privacy,
	title={Privacy quantification model based on the Bayes conditional risk in Location-Based Services},
	author={Zhang, Xuejun and Gui, Xiaolin and Tian, Feng and Yu, Si and An, Jian},
	journal={Tsinghua Science and Technology},
	volume={19},
	number={5},
	pages={452--462},
	year={2014},
	publisher={TUP}
}

@article{15bilogrevic2014privacy,
	title={Privacy-preserving optimal meeting location determination on mobile devices},
	author={Bilogrevic, Igor and Jadliwala, Murtuza and Joneja, Vishal and Kalkan, K{\"u}bra and Hubaux, Jean-Pierre and Aad, Imad},
	journal={IEEE transactions on information forensics and security},
	volume={9},
	number={7},
	pages={1141--1156},
	year={2014},
	publisher={IEEE}
}
@article{16haghnegahdar2014privacy,
	title={Privacy Risks in Publishing Mobile Device Trajectories},
	author={Haghnegahdar, Alireza and Khabbazian, Majid and Bhargava, Vijay K},
	journal={IEEE Wireless Communications Letters},
	volume={3},
	number={3},
	pages={241--244},
	year={2014},
	publisher={IEEE}
}
@article{17malandrino2014verification,
	title={Verification and inference of positions in vehicular networks through anonymous beaconing},
	author={Malandrino, Francesco and Borgiattino, Carlo and Casetti, Claudio and Chiasserini, Carla-Fabiana and Fiore, Marco and Sadao, Roberto},
	journal={IEEE Transactions on Mobile Computing},
	volume={13},
	number={10},
	pages={2415--2428},
	year={2014},
	publisher={IEEE}
}
@article{18shokri2014hiding,
	title={Hiding in the mobile crowd: Locationprivacy through collaboration},
	author={Shokri, Reza and Theodorakopoulos, George and Papadimitratos, Panos and Kazemi, Ehsan and Hubaux, Jean-Pierre},
	journal={IEEE transactions on dependable and secure computing},
	volume={11},
	number={3},
	pages={266--279},
	year={2014},
	publisher={IEEE}
}
@article{19freudiger2013non,
	title={Non-cooperative location privacy},
	author={Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
	journal={IEEE Transactions on Dependable and Secure Computing},
	volume={10},
	number={2},
	pages={84--98},
	year={2013},
	publisher={IEEE}
}
@article{20gao2013trpf,
	title={TrPF: A trajectory privacy-preserving framework for participatory sensing},
	author={Gao, Sheng and Ma, Jianfeng and Shi, Weisong and Zhan, Guoxing and Sun, Cong},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={8},
	number={6},
	pages={874--887},
	year={2013},
	publisher={IEEE}
}
@article{21ma2013privacy,
	title={Privacy vulnerability of published anonymous mobility traces},
	author={Ma, Chris YT and Yau, David KY and Yip, Nung Kwan and Rao, Nageswara SV},
	journal={IEEE/ACM Transactions on Networking},
	volume={21},
	number={3},
	pages={720--733},
	year={2013},
	publisher={IEEE}
}
@article{22niu2013pseudo,
	title={Pseudo-Location Updating System for privacy-preserving location-based services},
	author={Niu, Ben and Zhu, Xiaoyan and Chi, Haotian and Li, Hui},
	journal={China Communications},
	volume={10},
	number={9},
	pages={1--12},
	year={2013},
	publisher={IEEE}
}
@article{23dewri2013local,
	title={Local differential perturbations: Location privacy under approximate knowledge attackers},
	author={Dewri, Rinku},
	journal={IEEE Transactions on Mobile Computing},
	volume={12},
	number={12},
	pages={2360--2372},
	year={2013},
	publisher={IEEE}
}
@inproceedings{24kanoria2012tractable,
	title={Tractable bayesian social learning on trees},
	author={Kanoria, Yashodhan and Tamuz, Omer},
	booktitle={Information Theory Proceedings (ISIT), 2012 IEEE International Symposium on},
	pages={2721--2725},
	year={2012},
	organization={IEEE}
}
@inproceedings{25farias2005universal,
	title={A universal scheme for learning},
	author={Farias, Vivek F and Moallemi, Ciamac C and Van Roy, Benjamin and Weissman, Tsachy},
	booktitle={Proceedings. International Symposium on Information Theory, 2005. ISIT 2005.},
	pages={1158--1162},
	year={2005},
	organization={IEEE}
}
@inproceedings{26misra2013unsupervised,
	title={Unsupervised learning and universal communication},
	author={Misra, Vinith and Weissman, Tsachy},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={261--265},
	year={2013},
	organization={IEEE}
}
@inproceedings{27ryabko2013time,
	title={Time-series information and learning},
	author={Ryabko, Daniil},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={1392--1395},
	year={2013},
	organization={IEEE}
}
@inproceedings{28krzakala2013phase,
	title={Phase diagram and approximate message passing for blind calibration and dictionary learning},
	author={Krzakala, Florent and M{\'e}zard, Marc and Zdeborov{\'a}, Lenka},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={659--663},
	year={2013},
	organization={IEEE}
}
@inproceedings{29sakata2013sample,
	title={Sample complexity of Bayesian optimal dictionary learning},
	author={Sakata, Ayaka and Kabashima, Yoshiyuki},
	booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
	pages={669--673},
	year={2013},
	organization={IEEE}
}
@inproceedings{30predd2004consistency,
	title={Consistency in a model for distributed learning with specialists},
	author={Predd, Joel B and Kulkarni, Sanjeev R and Poor, H Vincent},
	booktitle={IEEE International Symposium on Information Theory},
	year={2004},
	organization={IEEE}
}
@inproceedings{31nokleby2016rate,
	title={Rate-Distortion Bounds on Bayes Risk in Supervised Learning},
	author={Nokleby, Matthew and Beirami, Ahmad and Calderbank, Robert},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={2099-2103},
	year={2016},
	organization={IEEE}
}

@inproceedings{32le2016imperfect,
	title={Are imperfect reviews helpful in social learning?},
	author={Le, Tho Ngoc and Subramanian, Vijay G and Berry, Randall A},
	booktitle={Information Theory (ISIT), 2016 IEEE International Symposium on},
	pages={2089--2093},
	year={2016},
	organization={IEEE}
}
@inproceedings{33gadde2016active,
	title={Active Learning for Community Detection in Stochastic Block Models},
	author={Gadde, Akshay and Gad, Eyal En and Avestimehr, Salman and Ortega, Antonio},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={1889-1893},
	year={2016}
}
@inproceedings{34shakeri2016minimax,
	title={Minimax Lower Bounds for Kronecker-Structured Dictionary Learning},
	author={Shakeri, Zahra and Bajwa, Waheed U and Sarwate, Anand D},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={1148-1152},
	year={2016}
}
@article{35lee2015speeding,
	title={Speeding up distributed machine learning using codes},
	author={Lee, Kangwook and Lam, Maximilian and Pedarsani, Ramtin and Papailiopoulos, Dimitris and Ramchandran, Kannan},
	booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
	pages={1143-1147},
	year={2016}
}
@article{36oneto2016statistical,
	title={Statistical Learning Theory and ELM for Big Social Data Analysis},
	author={Oneto, Luca and Bisio, Federica and Cambria, Erik and Anguita, Davide},
	journal={ieee CompUTATionAl inTelliGenCe mAGAzine},
	volume={11},
	number={3},
	pages={45--55},
	year={2016},
	publisher={IEEE}
}
@article{37lin2015probabilistic,
	title={Probabilistic approach to modeling and parameter learning of indirect drive robots from incomplete data},
	author={Lin, Chung-Yen and Tomizuka, Masayoshi},
	journal={IEEE/ASME Transactions on Mechatronics},
	volume={20},
	number={3},
	pages={1036--1045},
	year={2015},
	publisher={IEEE}
}
@article{38wang2016towards,
	title={Towards Bayesian Deep Learning: A Framework and Some Existing Methods},
	author={Wang, Hao and Yeung, Dit-Yan},
	journal={IEEE Transactions on Knowledge and Data Engineering},
	volume={PP},
	number={99},
	year={2016},
	publisher={IEEE}
}


%%%%%Informationtheoreticsecurity%%%%%%%%%%%%%%%%%%%%%%%




@inproceedings{Bloch2011PhysicalSecBook,
	title={Physical-Layer Security},
	author={M. Bloch and J. Barros},
	organization={Cambridge University Press},
	year={2011}
}



@inproceedings{Liang2009InfoSecBook,
	title={Information Theoretic Security},
	author={Y. Liang and H. V. Poor and S. Shamai (Shitz)},
	organization={Now Publishers Inc.},
	year={2009}
}


@inproceedings{Zhou2013PhysicalSecBook,
	title={Physical Layer Security in Wireless Communications},
	author={ X. Zhou and L. Song and Y. Zhang},
	organization={CRC Press},
	year={2013}
}

@article{Ni2012IEA,
	Author = {D. Ni and H. Liu and W. Ding and  Y. Xie and H. Wang and H. Pishro-Nik and Q. Yu},
	Journal = {IEA/AIE},
	Title = {Cyber-Physical Integration to Connect Vehicles for Transformed Transportation Safety and Efficiency},
	Year = {2012}}



@inproceedings{Ni2012Inproceedings,
	Author = {D. Ni, H. Liu, Y. Xie, W. Ding, H. Wang, H. Pishro-Nik, Q. Yu and M. Ferreira},
	Booktitle = {Spring Simulation Multiconference},
	Date-Added = {2016-09-04 14:18:42 +0000},
	Date-Modified = {2016-09-06 16:22:14 +0000},
	Title = {Virtual Lab of Connected Vehicle Technology},
	Year = {2012}}

@inproceedings{Ni2012Inproceedings,
	Author = {D. Ni, H. Liu, W. Ding, Y. Xie, H. Wang, H. Pishro-Nik and Q. Yu,},
	Booktitle = {IEA/AIE},
	Date-Added = {2016-09-04 09:11:02 +0000},
	Date-Modified = {2016-09-06 14:46:53 +0000},
	Title = {Cyber-Physical Integration to Connect Vehicles for Transformed Transportation Safety and Efficiency},
	Year = {2012}}


@article{Nekoui_IJIPT_2009,
	Author = {M. Nekoui and D. Ni and H. Pishro-Nik and R. Prasad and M. Kanjee and H. Zhu and T. Nguyen},
	Journal = {International Journal of Internet Protocol Technology (IJIPT)},
	Number = {3},
	Pages = {},
	Publisher = {},
	Title = {Development of a VII-Enabled Prototype Intersection Collision Warning System},
	Volume = {4},
	Year = {2009}}


@inproceedings{Pishro_Ganz_Ni,
	Author = {H. Pishro-Nik, A. Ganz, and Daiheng Ni},
	Booktitle = {Forty-Fifth Annual Allerton Conference on Communication, Control, and Computing. Allerton House, Monticello, IL},
	Date-Added = {},
	Date-Modified = {},
	Number = {},
	Pages = {},
	Title = {The capacity of vehicular ad hoc networks},
	Volume = {},
	Year = {September 26-28, 2007}}

@inproceedings{Leow_Pishro_Ni_1,
	Author = {W. L. Leow, H. Pishro-Nik and Daiheng Ni},
	Booktitle = {IEEE Global Telecommunications Conference, Washington, D.C.},
	Date-Added = {},
	Date-Modified = {},
	Number = {},
	Pages = {},
	Title = {Delay and Energy Tradeoff in Multi-state Wireless Sensor Networks},
	Volume = {},
	Year = {November 26-30, 2007}}


@misc{UMass-Trans,
	title = {{UMass Transportation Center}},
	note = {\url{http://www.umasstransportationcenter.org/}},
}


@inproceedings{Haenggi2013book,
	title={Stochastic geometry for wireless networks},
	author={M. Haenggi},
	organization={Cambridge Uinversity Press},
	year={2013}
}


%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Created for Zarrin Montazeri at 2015-11-09 18:45:31 -0500


%% Saved with string encoding Unicode (UTF-8)


%%%%%%%%%%%%%%%%personalization%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{osma2015,
	title={Impact of Time-to-Collision Information on Driving Behavior in Connected Vehicle Environments Using A Driving Simulator Test Bed},
	journal{Journal of Traffic and Logistics Engineering},
	author={Osama A. Osman, Julius Codjoe, and Sherif Ishak},
	volume={3},
	number={1},
	 pages={18--24},
	year={2015}
}


@article{charisma2010,
	title={Dynamic Latent Plan Models},
	author={Charisma F. Choudhurya, Moshe Ben-Akivab and Maya Abou-Zeid},
	journal={Journal of Choice Modelling},
	volume={3},
	number={2},
	pages={50--70},
	year={2010},
	publisher={Elsvier}
}


@misc{noble2014,
	author = {A. M. Noble, Shane B. McLaughlin, Zachary R. Doerzaph and Thomas A. Dingus},
	title = {Crowd-sourced Connected-vehicle Warning Algorithm using Naturalistic Driving Data},
	howpublished = {Downloaded from \url{http://hdl.handle.net/10919/53978}},

	month = August,
	year = 2014
}


@phdthesis{charisma2007,
	title    = {Modeling Driving Decisions with Latent Plans},
	school   = {Massachusetts Institute of Technology },
	author   = {Charisma Farheen Choudhury},
	year     = {2007}, %other attributes omitted
}


@article{chrysler2015,
	title={Cost of Warning of Unseen Threats:Unintended Consequences of Connected Vehicle Alerts},
	author={S. T. Chrysler, J. M. Cooper and D. C. Marshall},
	journal={Transportation Research Record: Journal of the Transportation Research Board},
	volume={2518},
	pages={79--85},
	year={2015},
}

@misc{nsf_cps,
        title = {Cyber-Physical Systems (CPS) PROGRAM SOLICITATION NSF 17-529},
        howpublished = {Downloaded from \url{https://www.nsf.gov/publications/pub_summ.jsp?WT.z_pims_id=503286&ods_key=nsf17529}},
}



%%%%%%%%%%%%%%IOT%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




@article{FTC2015,
  title={Internet of Things: Privacy and Security in a Connected World},
  author={FTC Staff Report},
  year={2015}
}



@article{0Quest2016,
  title={The Quest for Privacy in the Internet of Things},
  author={ Pawani Porambag and Mika Ylianttila and Corinna Schmitt and  Pardeep Kumar and  Andrei Gurtov and  Athanasios V. Vasilakos},
  journal={IEEE Cloud Computing},
  volum={3},
  number={2},
  year={2016},
  publisher={IEEE}
}

%% Saved with string encoding Unicode (UTF-8)
@inproceedings{1zhou2014security,
  title={Security/privacy of wearable fitness tracking {I}o{T} devices},
  author={Zhou, Wei and Piramuthu, Selwyn},
  booktitle={Information Systems and Technologies (CISTI), 2014 9th Iberian Conference on},
  pages={1--5},
  year={2014},
  organization={IEEE}
}


@inproceedings{3ukil2014iot,
  title={{I}o{T}-privacy: To be private or not to be private},
  author={Ukil, Arijit and Bandyopadhyay, Soma and Pal, Arpan},
  booktitle={Computer Communications Workshops (INFOCOM WKSHPS), IEEE Conference on},
  pages={123--124},
  year={2014},
  organization={IEEE}
}


@article{4arias2015privacy,
  title={Privacy and security in internet of things and wearable devices},
  author={Arias, Orlando and Wurm, Jacob and Hoang, Khoa and Jin, Yier},
  journal={IEEE Transactions on Multi-Scale Computing Systems},
  volume={1},
  number={2},
  pages={99--109},
  year={2015},
  publisher={IEEE}
}
@inproceedings{5ullah2016novel,
  title={A novel model for preserving Location Privacy in Internet of Things},
  author={Ullah, Ikram and Shah, Munam Ali},
  booktitle={Automation and Computing (ICAC), 2016 22nd International Conference on},
  pages={542--547},
  year={2016},
  organization={IEEE}
}
@inproceedings{6sathishkumar2016enhanced,
  title={Enhanced location privacy algorithm for wireless sensor network in Internet of Things},
  author={Sathishkumar, J and Patel, Dhiren R},
  booktitle={Internet of Things and Applications (IOTA), International Conference on},
  pages={208--212},
  year={2016},
  organization={IEEE}
}
@inproceedings{7zhou2012preserving,
  title={Preserving sensor location privacy in internet of things},
  author={Zhou, Liming and Wen, Qiaoyan and Zhang, Hua},
  booktitle={Computational and Information Sciences (ICCIS), 2012 Fourth International Conference on},
  pages={856--859},
  year={2012},
  organization={IEEE}
}

@inproceedings{8ukil2015privacy,
  title={Privacy for {I}o{T}: Involuntary privacy enablement for smart energy systems},
  author={Ukil, Arijit and Bandyopadhyay, Soma and Pal, Arpan},
  booktitle={Communications (ICC), 2015 IEEE International Conference on},
  pages={536--541},
  year={2015},
  organization={IEEE}
}

@inproceedings{9dalipi2016security,
  title={Security and Privacy Considerations for {I}o{T} Application on Smart Grids: Survey and Research Challenges},
  author={Dalipi, Fisnik and Yayilgan, Sule Yildirim},
  booktitle={Future Internet of Things and Cloud Workshops (FiCloudW), IEEE International Conference on},
  pages={63--68},
  year={2016},
  organization={IEEE}
}
@inproceedings{10harris2016security,
  title={Security and Privacy in Public {I}o{T} Spaces},
  author={Harris, Albert F and Sundaram, Hari and Kravets, Robin},
  booktitle={Computer Communication and Networks (ICCCN), 2016 25th International Conference on},
  pages={1--8},
  year={2016},
  organization={IEEE}
}

@inproceedings{11al2015security,
  title={Security and privacy framework for ubiquitous healthcare {I}o{T} devices},
  author={Al Alkeem, Ebrahim and Yeun, Chan Yeob and Zemerly, M Jamal},
  booktitle={Internet Technology and Secured Transactions (ICITST), 2015 10th International Conference for},
  pages={70--75},
  year={2015},
  organization={IEEE}
}
@inproceedings{12sivaraman2015network,
  title={Network-level security and privacy control for smart-home {I}o{T} devices},
  author={Sivaraman, Vijay and Gharakheili, Hassan Habibi and Vishwanath, Arun and Boreli, Roksana and Mehani, Olivier},
  booktitle={Wireless and Mobile Computing, Networking and Communications (WiMob), 2015 IEEE 11th International Conference on},
  pages={163--167},
  year={2015},
  organization={IEEE}
}

@inproceedings{13srinivasan2016privacy,
  title={Privacy conscious architecture for improving emergency response in smart cities},
  author={Srinivasan, Ramya and Mohan, Apurva and Srinivasan, Priyanka},
  booktitle={Smart City Security and Privacy Workshop (SCSP-W), 2016},
  pages={1--5},
  year={2016},
  organization={IEEE}
}
@inproceedings{14sadeghi2015security,
  title={Security and privacy challenges in industrial internet of things},
  author={Sadeghi, Ahmad-Reza and Wachsmann, Christian and Waidner, Michael},
  booktitle={Design Automation Conference (DAC), 2015 52nd ACM/EDAC/IEEE},
  pages={1--6},
  year={2015},
  organization={IEEE}
}
@inproceedings{15otgonbayar2016toward,
  title={Toward Anonymizing {I}o{T} Data Streams via Partitioning},
  author={Otgonbayar, Ankhbayar and Pervez, Zeeshan and Dahal, Keshav},
  booktitle={Mobile Ad Hoc and Sensor Systems (MASS), 2016 IEEE 13th International Conference on},
  pages={331--336},
  year={2016},
  organization={IEEE}
}
@inproceedings{16rutledge2016privacy,
  title={Privacy Impacts of {I}o{T} Devices: A SmartTV Case Study},
  author={Rutledge, Richard L and Massey, Aaron K and Ant{\'o}n, Annie I},
  booktitle={Requirements Engineering Conference Workshops (REW), IEEE International},
  pages={261--270},
  year={2016},
  organization={IEEE}
}

@inproceedings{17andrea2015internet,
  title={Internet of Things: Security vulnerabilities and challenges},
  author={Andrea, Ioannis and Chrysostomou, Chrysostomos and Hadjichristofi, George},
  booktitle={Computers and Communication (ISCC), 2015 IEEE Symposium on},
  pages={180--187},
  year={2015},
  organization={IEEE}
}






























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@misc{epfl-mobility-20090224,
    author = {Michal Piorkowski and Natasa Sarafijanovic-Djukic and Matthias Grossglauser},
    title = {{CRAWDAD} dataset epfl/mobility (v. 2009-02-24)},
    howpublished = {Downloaded from \url{http://crawdad.org/epfl/mobility/20090224}},
    doi = {10.15783/C7J010},
    month = feb,
    year = 2009
}

@misc{roma-taxi-20140717,
    author = {Lorenzo Bracciale and Marco Bonola and Pierpaolo Loreti and Giuseppe Bianchi and Raul Amici and Antonello Rabuffi},
    title = {{CRAWDAD} dataset roma/taxi (v. 2014-07-17)},
    howpublished = {Downloaded from \url{http://crawdad.org/roma/taxi/20140717}},
    doi = {10.15783/C7QC7M},
    month = jul,
    year = 2014
}

@misc{rice-ad_hoc_city-20030911,
    author = {Jorjeta G. Jetcheva and Yih-Chun Hu and Santashil PalChaudhuri and Amit Kumar Saha and David B. Johnson},
    title = {{CRAWDAD} dataset rice/ad\_hoc\_city (v. 2003-09-11)},
    howpublished = {Downloaded from \url{http://crawdad.org/rice/ad_hoc_city/20030911}},
    doi = {10.15783/C73K5B},
    month = sep,
    year = 2003
}

@misc{china:2012,
author = {Microsoft Research Asia},
title = {GeoLife GPS Trajectories},
year = {2012},
howpublished= {\url{https://www.microsoft.com/en-us/download/details.aspx?id=52367}},
}


@misc{china:2011,
ALTauthor = {Microsoft Research Asia)},
ALTeditor = {},
title = {GeoLife GPS Trajectories,
year = {2012},
url = {https://www.microsoft.com/en-us/download/details.aspx?id=52367},
}


@misc{longversion,
  author = {N. Takbiri and A. Houmansadr and D.L. Goeckel and H. Pishro-Nik},
  title = {{Limits of Location Privacy under Anonymization and Obfuscation}},
  howpublished = "\url{http://www.ecs.umass.edu/ece/pishro/Papers/ISIT_2017-2.pdf}",
  year = 2017,
month= "January",
  note = "Summarized version submitted to IEEE ISIT 2017"
}

@misc{isit_ke,
  author = {K. Li and D. Goeckel and H. Pishro-Nik},
  title = {{Bayesian Time Series Matching and Privacy}},
  note = "submitted to IEEE ISIT 2017"
}

@article{matching,
  title={Asymptotically Optimal Matching of Multiple Sequences to Source Distributions and Training Sequences},
  author={Jayakrishnan Unnikrishnan},
  journal={ IEEE Transactions on Information Theory},
  volume={61},
  number={1},
  pages={452-468},
  year={2015},
  publisher={IEEE}
}


@article{Naini2016,
	Author = {F. Naini and J. Unnikrishnan and P. Thiran and M. Vetterli},
	Journal = {IEEE Transactions on Information Forensics and Security},
	Publisher = {IEEE},
	Title = {Where You Are Is Who You Are: User Identification by Matching Statistics},
	 volume={11},
    number={2},
     pages={358--372},
    Year = {2016}
}



@inproceedings{holowczak2015cachebrowser,
  title={{CacheBrowser: Bypassing Chinese Censorship without Proxies Using Cached Content}},
  author={Holowczak, John and Houmansadr, Amir},
  booktitle={Proceedings of the 22nd ACM SIGSAC Conference on Computer and Communications Security},
  pages={70--83},
  year={2015},
  organization={ACM}
}
@misc{cb-website,
	Howpublished = {\url{https://cachebrowser.net/#/}},
	Title = {{CacheBrowser}},
	key={cachebrowser}
}

@inproceedings{GameOfDecoys,
 title={{GAME OF DECOYS: Optimal Decoy Routing Through Game Theory}},
 author={Milad Nasr and Amir Houmansadr},
 booktitle={The $23^{rd}$ ACM Conference on Computer and Communications Security (CCS)},
 year={2016}
}

@inproceedings{CDNReaper,
 title={{Practical Censorship Evasion Leveraging Content Delivery Networks}},
 author={Hadi Zolfaghari and Amir Houmansadr},
 booktitle={The $23^{rd}$ ACM Conference on Computer and Communications Security (CCS)},
 year={2016}
}

@misc{Leberknight2010,
	Author = {Leberknight, C. and Chiang, M. and Poor, H. and Wong, F.},
	Howpublished = {\url{http://www.princeton.edu/~chiangm/anticensorship.pdf}},
	Title = {{A Taxonomy of Internet Censorship and Anti-censorship}},
	Year = {2010}}

@techreport{ultrasurf-analysis,
	Author = {Appelbaum, Jacob},
	Institution = {The Tor Project},
	Title = {{Technical analysis of the Ultrasurf proxying software}},
	Url = {http://scholar.google.com/scholar?hl=en\&btnG=Search\&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software\#0},
	Year = {2012},
	Bdsk-Url-1 = {http://scholar.google.com/scholar?hl=en%5C&btnG=Search%5C&q=intitle:Technical+analysis+of+the+Ultrasurf+proxying+software%5C#0}}

@misc{gifc:07,
	Howpublished = {\url{http://www.internetfreedom.org/archive/Defeat\_Internet\_Censorship\_White\_Paper.pdf}},
	Key = {defeatcensorship},
	Publisher = {Global Internet Freedom Consortium (GIFC)},
	Title = {{Defeat Internet Censorship: Overview of Advanced Technologies and Products}},
	Type = {White Paper},
	Year = {2007}}

@article{pan2011survey,
	Author = {Pan, J. and Paul, S. and Jain, R.},
	Journal = {Communications Magazine, IEEE},
	Number = {7},
	Pages = {26--36},
	Publisher = {IEEE},
	Title = {{A Survey of the Research on Future Internet Architectures}},
	Volume = {49},
	Year = {2011}}

@misc{nsf-fia,
	Howpublished = {\url{http://www.nets-fia.net/}},
	Key = {FIA},
	Title = {{NSF Future Internet Architecture Project}}}

@misc{NDN,
	Howpublished = {\url{http://www.named- data.net}},
	Key = {NDN},
	Title = {{Named Data Networking Project}}}

@inproceedings{MobilityFirst,
	Author = {Seskar, I. and Nagaraja, K. and Nelson, S. and Raychaudhuri, D.},
	Booktitle = {Asian Internet Engineering Conference},
	Title = {{Mobilityfirst Future internet Architecture Project}},
	Year = {2011}}

@incollection{NEBULA,
	Author = {Anderson, T. and Birman, K. and Broberg, R. and Caesar, M. and Comer, D. and Cotton, C. and Freedman, M.~J. and Haeberlen, A. and Ives, Z.~G. and Krishnamurthy, A. and others},
	Booktitle = {The Future Internet},
	Pages = {16--26},
	Publisher = {Springer},
	Title = {{The NEBULA Future Internet Architecture}},
	Year = {2013}}

@inproceedings{XIA,
	Author = {Anand, A. and Dogar, F. and Han, D. and Li, B. and Lim, H. and Machado, M. and Wu, W. and Akella, A. and Andersen, D.~G. and Byers, J.~W. and others},
	Booktitle = {ACM Workshop on Hot Topics in Networks},
	Pages = {2},
	Title = {{XIA: An Architecture for an Evolvable and Trustworthy Internet}},
	Year = {2011}}

@inproceedings{ChoiceNet,
	Author = {Rouskas, G.~N. and Baldine, I. and Calvert, K.~L. and Dutta, R. and Griffioen, J. and Nagurney, A. and Wolf, T.},
	Booktitle = {ONDM},
	Title = {{ChoiceNet: Network Innovation Through Choice}},
	Year = {2013}}

@misc{nsf-find,
	Howpublished = {http://www.nets-find.net/},
	Title = {{NSF NeTS FIND Initiative}}}

@article{traid,
	Author = {Cheriton, D.~R. and Gritter, M.},
	Title = {{TRIAD: A New Next-Generation Internet Architecture}},
	Year = {2000}}

@inproceedings{dona,
	Author = {Koponen, T. and Chawla, M. and Chun, B-G. and Ermolinskiy, A. and Kim, K.~H. and Shenker, S. and Stoica, I.},
	Booktitle = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Organization = {ACM},
	Pages = {181--192},
	Title = {{A Data-Oriented (and Beyond) Network Architecture}},
	Volume = {37},
	Year = {2007}}

@misc{ultrasurf,
	Howpublished = {\url{http://www.ultrareach.com}},
	Key = {ultrasurf},
	Title = {{Ultrasurf}}}

@misc{tor-bridge,
	Author = {Dingledine, R. and Mathewson, N.},
	Howpublished = {\url{https://svn.torproject.org/svn/projects/design-paper/blocking.html}},
	Title = {{Design of a Blocking-Resistant Anonymity System}}}

@inproceedings{McLachlanH09,
	Author = {J. McLachlan and N. Hopper},
	Booktitle = {WPES},
	Title = {{On the Risks of Serving Whenever You Surf: Vulnerabilities in Tor's Blocking Resistance Design}},
	Year = {2009}}

@inproceedings{mahdian2010,
	Author = {Mahdian, M.},
	Booktitle = {{Fun with Algorithms}},
	Title = {{Fighting Censorship with Algorithms}},
	Year = {2010}}

@inproceedings{McCoy2011,
	Author = {McCoy, D. and Morales, J.~A. and Levchenko, K.},
	Booktitle = {FC},
	Title = {{Proximax: A Measurement Based System for Proxies Dissemination}},
	Year = {2011}}

@inproceedings{Sovran2008,
	Author = {Sovran, Y. and Libonati, A. and Li, J.},
	Booktitle = {IPTPS},
	Title = {{Pass it on: Social Networks Stymie Censors}},
	Year = {2008}}

@inproceedings{rbridge,
	Author = {Wang, Q. and Lin, Zi and Borisov, N. and Hopper, N.},
	Booktitle = {{NDSS}},
	Title = {{rBridge: User Reputation based Tor Bridge Distribution with Privacy Preservation}},
	Year = {2013}}

@inproceedings{telex,
	Author = {Wustrow, E. and Wolchok, S. and Goldberg, I. and Halderman, J.},
	Booktitle = {{USENIX Security}},
	Title = {{Telex: Anticensorship in the Network Infrastructure}},
	Year = {2011}}

@inproceedings{cirripede,
	Author = {Houmansadr, A. and Nguyen, G. and Caesar, M. and Borisov, N.},
	Booktitle = {CCS},
	Title = {{Cirripede: Circumvention Infrastructure Using Router Redirection with Plausible Deniability}},
	Year = {2011}}

@inproceedings{decoyrouting,
	Author = {Karlin, J. and Ellard, D. and Jackson, A. and Jones, C. and Lauer, G. and Mankins, D. and Strayer, W.},
	Booktitle = {{FOCI}},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = {2011}}

@inproceedings{routing-around-decoys,
	Author = {M.~Schuchard and J.~Geddes and C.~Thompson and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Routing Around Decoys}},
	Year = {2012}}

@inproceedings{parrot,
	Author = {A. Houmansadr and C. Brubaker and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{The Parrot is Dead: Observing Unobservable Network Communications}},
	Year = {2013}}

@misc{knock,
	Author = {T. Wilde},
	Howpublished = {\url{https://blog.torproject.org/blog/knock-knock-knockin-bridges-doors}},
	Title = {{Knock Knock Knockin' on Bridges' Doors}},
	Year = {2012}}

@inproceedings{china-tor,
	Author = {Winter, P. and Lindskog, S.},
	Booktitle = {{FOCI}},
	Title = {{How the Great Firewall of China Is Blocking Tor}},
	Year = {2012}}

@misc{discover-bridge,
	Howpublished = {\url{https://blog.torproject.org/blog/research-problems-ten-ways-discover-tor-bridges}},
	Key = {tenways},
	Title = {{Ten Ways to Discover Tor Bridges}}}

@inproceedings{freewave,
	Author = {A.~Houmansadr and T.~Riedl and N.~Borisov and A.~Singer},
	Booktitle = {{NDSS}},
	Title = {{I Want My Voice to Be Heard: IP over Voice-over-IP for Unobservable Censorship Circumvention}},
	Year = 2013}

@inproceedings{censorspoofer,
	Author = {Q. Wang and X. Gong and G. Nguyen and A. Houmansadr and N. Borisov},
	Booktitle = {CCS},
	Title = {{CensorSpoofer: Asymmetric Communication Using IP Spoofing for Censorship-Resistant Web Browsing}},
	Year = {2012}}

@inproceedings{skypemorph,
	Author = {H. Moghaddam and B. Li and M. Derakhshani and I. Goldberg},
	Booktitle = {CCS},
	Title = {{SkypeMorph: Protocol Obfuscation for Tor Bridges}},
	Year = {2012}}

@inproceedings{stegotorus,
	Author = {Weinberg, Z. and Wang, J. and Yegneswaran, V. and Briesemeister, L. and Cheung, S. and Wang, F. and Boneh, D.},
	Booktitle = {CCS},
	Title = {{StegoTorus: A Camouflage Proxy for the Tor Anonymity System}},
	Year = {2012}}

@techreport{dust,
	Author = {{B.~Wiley}},
	Howpublished = {\url{http://blanu.net/ Dust.pdf}},
	Institution = {School of Information, University of Texas at Austin},
	Title = {{Dust: A Blocking-Resistant Internet Transport Protocol}},
	Year = {2011}}

@inproceedings{FTE,
	Author = {K.~Dyer and S.~Coull and T.~Ristenpart and T.~Shrimpton},
	Booktitle = {CCS},
	Title = {{Protocol Misidentification Made Easy with Format-Transforming Encryption}},
	Year = {2013}}

@inproceedings{fp,
	Author = {Fifield, D. and Hardison, N. and Ellithrope, J. and Stark, E. and Dingledine, R. and Boneh, D. and Porras, P.},
	Booktitle = {PETS},
	Title = {{Evading Censorship with Browser-Based Proxies}},
	Year = {2012}}

@misc{obfsproxy,
	Howpublished = {\url{https://www.torproject.org/projects/obfsproxy.html.en}},
	Key = {obfsproxy},
	Publisher = {The Tor Project},
	Title = {{A Simple Obfuscating Proxy}}}

@inproceedings{Tor-instead-of-IP,
	Author = {Liu, V. and Han, S. and Krishnamurthy, A. and Anderson, T.},
	Booktitle = {HotNets},
	Title = {{Tor instead of IP}},
	Year = {2011}}

@misc{roger-slides,
	Howpublished = {\url{https://svn.torproject.org/svn/projects/presentations/slides-28c3.pdf}},
	Key = {torblocking},
	Title = {{How Governments Have Tried to Block Tor}}}

@inproceedings{infranet,
	Author = {Feamster, N. and Balazinska, M. and Harfst, G. and Balakrishnan, H. and Karger, D.},
	Booktitle = {USENIX Security},
	Title = {{Infranet: Circumventing Web Censorship and Surveillance}},
	Year = {2002}}

@inproceedings{collage,
	Author = {S.~Burnett and N.~Feamster and S.~Vempala},
	Booktitle = {USENIX Security},
	Title = {{Chipping Away at Censorship Firewalls with User-Generated Content}},
	Year = {2010}}

@article{anonymizer,
	Author = {Boyan, J.},
	Journal = {Computer-Mediated Communication Magazine},
	Month = sep,
	Number = {9},
	Title = {{The Anonymizer: Protecting User Privacy on the Web}},
	Volume = {4},
	Year = {1997}}

@article{schulze2009internet,
	Author = {Schulze, H. and Mochalski, K.},
	Journal = {IPOQUE Report},
	Pages = {351--362},
	Title = {Internet Study 2008/2009},
	Volume = {37},
	Year = {2009}}

@inproceedings{cya-ccs13,
	Author = {J.~Geddes and M.~Schuchard and N.~Hopper},
	Booktitle = {{CCS}},
	Title = {{Cover Your ACKs: Pitfalls of Covert Channel Censorship Circumvention}},
	Year = {2013}}

@inproceedings{andana,
	Author = {DiBenedetto, S. and Gasti, P. and Tsudik, G. and Uzun, E.},
	Booktitle = {{NDSS}},
	Title = {{ANDaNA: Anonymous Named Data Networking Application}},
	Year = {2012}}

@inproceedings{darkly,
	Author = {Jana, S. and Narayanan, A. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{A Scanner Darkly: Protecting User Privacy From Perceptual Applications}},
	Year = {2013}}

@inproceedings{NS08,
	Author = {A.~Narayanan and V.~Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {Robust de-anonymization of large sparse datasets},
	Year = {2008}}

@inproceedings{NS09,
	Author = {A.~Narayanan and V.~Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {De-anonymizing social networks},
	Year = {2009}}

@inproceedings{memento,
	Author = {Jana, S. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{Memento: Learning secrets from process footprints}},
	Year = {2012}}

@misc{plugtor,
	Howpublished = {\url{https://www.torproject.org/docs/pluggable-transports.html.en}},
	Key = {PluggableTransports},
	Publisher = {The Tor Project},
	Title = {{Tor: Pluggable transports}}}

@misc{psiphon,
	Author = {J.~Jia and P.~Smith},
	Howpublished = {\url{http://www.cdf.toronto.edu/~csc494h/reports/2004-fall/psiphon_ae.html}},
	Title = {{Psiphon: Analysis and Estimation}},
	Year = 2004}

@misc{china-github,
	Howpublished = {\url{http://mobile.informationweek.com/80269/show/72e30386728f45f56b343ddfd0fdb119/}},
	Key = {github},
	Title = {{China's GitHub Censorship Dilemma}}}

@inproceedings{txbox,
	Author = {Jana, S. and Porter, D. and Shmatikov, V.},
	Booktitle = {IEEE S\&P},
	Title = {{TxBox: Building Secure, Efficient Sandboxes with System Transactions}},
	Year = {2011}}

@inproceedings{airavat,
	Author = {I. Roy and S. Setty and A. Kilzer and V. Shmatikov and E. Witchel},
	Booktitle = {NSDI},
	Title = {{Airavat: Security and Privacy for MapReduce}},
	Year = {2010}}

@inproceedings{osdi12,
	Author = {A. Dunn and M. Lee and S. Jana and S. Kim and M. Silberstein and Y. Xu and V. Shmatikov and E. Witchel},
	Booktitle = {OSDI},
	Title = {{Eternal Sunshine of the Spotless Machine: Protecting Privacy with Ephemeral Channels}},
	Year = {2012}}

@inproceedings{ymal,
	Author = {J. Calandrino and A. Kilzer and A. Narayanan and E. Felten and V. Shmatikov},
	Booktitle = {IEEE S\&P},
	Title = {{``You Might Also Like:'' Privacy Risks of Collaborative Filtering}},
	Year = {2011}}

@inproceedings{srivastava11,
	Author = {V. Srivastava and M. Bond and K. McKinley and V. Shmatikov},
	Booktitle = {PLDI},
	Title = {{A Security Policy Oracle: Detecting Security Holes Using Multiple API Implementations}},
	Year = {2011}}

@inproceedings{chen-oakland10,
	Author = {Chen, S. and Wang, R. and Wang, X. and Zhang, K.},
	Booktitle = {IEEE S\&P},
	Title = {{Side-Channel Leaks in Web Applications: A Reality Today, a Challenge Tomorrow}},
	Year = {2010}}

@book{kerck,
	Author = {Kerckhoffs, A.},
	Publisher = {University Microfilms},
	Title = {{La cryptographie militaire}},
	Year = {1978}}

@inproceedings{foci11,
	Author = {J. Karlin and D. Ellard and A.~Jackson and C.~ Jones and G. Lauer and D. Mankins and W.~T.~Strayer},
	Booktitle = {FOCI},
	Title = {{Decoy Routing: Toward Unblockable Internet Communication}},
	Year = 2011}

@inproceedings{sun02,
	Author = {Sun, Q. and Simon, D.~R. and Wang, Y. and Russell, W. and Padmanabhan, V. and Qiu, L.},
	Booktitle = {IEEE S\&P},
	Title = {{Statistical Identification of Encrypted Web Browsing Traffic}},
	Year = {2002}}

@inproceedings{danezis,
	Author = {Murdoch, S.~J. and Danezis, G.},
	Booktitle = {IEEE S\&P},
	Title = {{Low-Cost Traffic Analysis of Tor}},
	Year = {2005}}

@inproceedings{pakicensorship,
	Author = {Z.~Nabi},
	Booktitle = {FOCI},
	Title = {The Anatomy of {Web} Censorship in {Pakistan}},
	Year = {2013}}

@inproceedings{irancensorship,
	Author = {S.~Aryan and H.~Aryan and A.~Halderman},
	Booktitle = {FOCI},
	Title = {Internet Censorship in {Iran}: {A} First Look},
	Year = {2013}}

@inproceedings{ford10efficient,
	Author = {Amittai Aviram and Shu-Chun Weng and Sen Hu and Bryan Ford},
	Booktitle = {\bibconf[9th]{OSDI}{USENIX Symposium on Operating Systems Design and Implementation}},
	Location = {Vancouver, BC, Canada},
	Month = oct,
	Title = {Efficient System-Enforced Deterministic Parallelism},
	Year = 2010}

@inproceedings{ford10determinating,
	Author = {Amittai Aviram and Sen Hu and Bryan Ford and Ramakrishna Gummadi},
	Booktitle = {\bibconf{CCSW}{ACM Cloud Computing Security Workshop}},
	Location = {Chicago, IL},
	Month = oct,
	Title = {Determinating Timing Channels in Compute Clouds},
	Year = 2010}

@inproceedings{ford12plugging,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Plugging Side-Channel Leaks with Timing Information Flow Control},
	Year = 2012}

@inproceedings{ford12icebergs,
	Author = {Bryan Ford},
	Booktitle = {\bibconf[4th]{HotCloud}{USENIX Workshop on Hot Topics in Cloud Computing}},
	Location = {Boston, MA},
	Month = jun,
	Title = {Icebergs in the Clouds: the {\em Other} Risks of Cloud Computing},
	Year = 2012}

@misc{mullenize,
	Author = {Washington Post},
	Howpublished = {\url{http://apps.washingtonpost.com/g/page/world/gchq-report-on-mullenize-program-to-stain-anonymous-electronic-traffic/502/}},
	Month = {oct},
	Title = {{GCHQ} report on {`MULLENIZE'} program to `stain' anonymous electronic traffic},
	Year = {2013}}

@inproceedings{shue13street,
	Author = {Craig A. Shue and Nathanael Paul and Curtis R. Taylor},
	Booktitle = {\bibbrev[7th]{WOOT}{USENIX Workshop on Offensive Technologies}},
	Month = aug,
	Title = {From an {IP} Address to a Street Address: Using Wireless Signals to Locate a Target},
	Year = 2013}

@inproceedings{knockel11three,
	Author = {Jeffrey Knockel and Jedidiah R. Crandall and Jared Saia},
	Booktitle = {\bibbrev{FOCI}{USENIX Workshop on Free and Open Communications on the Internet}},
	Location = {San Francisco, CA},
	Month = aug,
	Year = 2011}

@misc{rfc4960,
	Author = {R. {Stewart, ed.}},
	Month = sep,
	Note = {RFC 4960},
	Title = {Stream Control Transmission Protocol},
	Year = 2007}

@inproceedings{ford07structured,
	Author = {Bryan Ford},
	Booktitle = {\bibbrev{SIGCOMM}{ACM SIGCOMM}},
	Location = {Kyoto, Japan},
	Month = aug,
	Title = {Structured Streams: a New Transport Abstraction},
	Year = {2007}}

@misc{spdy,
	Author = {Google, Inc.},
	Note = {\url{http://www.chromium.org/spdy/spdy-whitepaper}},
	Title = {{SPDY}: An Experimental Protocol For a Faster {Web}}}

@misc{quic,
	Author = {Jim Roskind},
	Month = jun,
	Note = {\url{http://blog.chromium.org/2013/06/experimenting-with-quic.html}},
	Title = {Experimenting with {QUIC}},
	Year = 2013}

@misc{podjarny12not,
	Author = {G.~Podjarny},
	Month = jun,
	Note = {\url{http://www.guypo.com/technical/not-as-spdy-as-you-thought/}},
	Title = {{Not as SPDY as You Thought}},
	Year = 2012}

@inproceedings{cor,
	Author = {Jones, N.~A. and Arye, M. and Cesareo, J. and Freedman, M.~J.},
	Booktitle = {FOCI},
	Title = {{Hiding Amongst the Clouds: A Proposal for Cloud-based Onion Routing}},
	Year = {2011}}

@misc{torcloud,
	Howpublished = {\url{https://cloud.torproject.org/}},
	Key = {tor cloud},
	Title = {{The Tor Cloud Project}}}

@inproceedings{scramblesuit,
	Author = {Philipp Winter and Tobias Pulls and Juergen Fuss},
	Booktitle = {WPES},
	Title = {{ScrambleSuit: A Polymorphic Network Protocol to Circumvent Censorship}},
	Year = 2013}

@article{savage2000practical,
	Author = {Savage, S. and Wetherall, D. and Karlin, A. and Anderson, T.},
	Journal = {ACM SIGCOMM Computer Communication Review},
	Number = {4},
	Pages = {295--306},
	Publisher = {ACM},
	Title = {Practical network support for IP traceback},
	Volume = {30},
	Year = {2000}}

@inproceedings{ooni,
	Author = {Filast, A. and Appelbaum, J.},
	Booktitle = {{FOCI}},
	Title = {{OONI : Open Observatory of Network Interference}},
	Year = {2012}}

@misc{caida-rank,
	Howpublished = {\url{http://as-rank.caida.org/}},
	Key = {caida rank},
	Title = {{AS Rank: AS Ranking}}}

@inproceedings{usersrouted-ccs13,
	Author = {A.~Johnson and C.~Wacek and R.~Jansen and M.~Sherr and P.~Syverson},
	Booktitle = {CCS},
	Title = {{Users Get Routed: Traffic Correlation on Tor by Realistic Adversaries}},
	Year = {2013}}

@inproceedings{edman2009awareness,
	Author = {Edman, M. and Syverson, P.},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2009}}

@inproceedings{DecoyCosts,
	Author = {A.~Houmansadr and E.~L.~Wong and V.~Shmatikov},
	Booktitle = {NDSS},
	Title = {{No Direction Home: The True Cost of Routing Around Decoys}},
	Year = {2014}}

@article{cordon,
	Author = {Elahi, T. and Goldberg, I.},
	Journal = {University of Waterloo CACR},
	Title = {{CORDON--A Taxonomy of Internet Censorship Resistance Strategies}},
	Volume = {33},
	Year = {2012}}

@inproceedings{privex,
	Author = {T.~Elahi and G.~Danezis and I.~Goldberg	},
	Booktitle = {{CCS}},
	Title = {{AS-awareness in Tor path selection}},
	Year = {2014}}

@inproceedings{changeGuards,
	Author = {T.~Elahi and K.~Bauer and M.~AlSabah and R.~Dingledine and I.~Goldberg},
	Booktitle = {{WPES}},
	Title = {{ Changing of the Guards: Framework for Understanding and Improving Entry Guard Selection in Tor}},
	Year = {2012}}

@article{RAINBOW:Journal,
	Author = {A.~Houmansadr and N.~Kiyavash and N.~Borisov},
	Journal = {IEEE/ACM Transactions on Networking},
	Title = {{Non-Blind Watermarking of Network Flows}},
	Year = 2014}

@inproceedings{info-tod,
	Author = {A.~Houmansadr and S.~Gorantla and T.~Coleman and N.~Kiyavash and and N.~Borisov},
	Booktitle = {{CCS (poster session)}},
	Title = {{On the Channel Capacity of Network Flow Watermarking}},
	Year = {2009}}

@inproceedings{johnson2014game,
	Author = {Johnson, B. and Laszka, A. and Grossklags, J. and Vasek, M. and Moore, T.},
	Booktitle = {Workshop on Bitcoin Research},
	Title = {{Game-theoretic Analysis of DDoS Attacks Against Bitcoin Mining Pools}},
	Year = {2014}}

@incollection{laszka2013mitigation,
	Author = {Laszka, A. and Johnson, B. and Grossklags, J.},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {175--191},
	Publisher = {Springer},
	Title = {{Mitigation of Targeted and Non-targeted Covert Attacks as a Timing Game}},
	Year = {2013}}

@inproceedings{schottle2013game,
	Author = {Schottle, P. and Laszka, A. and Johnson, B. and Grossklags, J. and Bohme, R.},
	Booktitle = {EUSIPCO},
	Title = {{A Game-theoretic Analysis of Content-adaptive Steganography with Independent Embedding}},
	Year = {2013}}

@inproceedings{CloudTransport,
	Author = {C.~Brubaker and A.~Houmansadr and V.~Shmatikov},
	Booktitle = {PETS},
	Title = {{CloudTransport: Using Cloud Storage for Censorship-Resistant Networking}},
	Year = {2014}}

@inproceedings{sweet,
	Author = {W.~Zhou and A.~Houmansadr and M.~Caesar and N.~Borisov},
	Booktitle = {HotPETs},
	Title = {{SWEET: Serving the Web by Exploiting Email Tunnels}},
	Year = {2013}}

@inproceedings{ahsan2002practical,
	Author = {Ahsan, K. and Kundur, D.},
	Booktitle = {Workshop on Multimedia Security},
	Title = {{Practical data hiding in TCP/IP}},
	Year = {2002}}

@incollection{danezis2011covert,
	Author = {Danezis, G.},
	Booktitle = {Security Protocols XVI},
	Pages = {198--214},
	Publisher = {Springer},
	Title = {{Covert Communications Despite Traffic Data Retention}},
	Year = {2011}}

@inproceedings{liu2009hide,
	Author = {Liu, Y. and Ghosal, D. and Armknecht, F. and Sadeghi, A.-R. and Schulz, S. and Katzenbeisser, S.},
	Booktitle = {ESORICS},
	Title = {{Hide and Seek in Time---Robust Covert Timing Channels}},
	Year = {2009}}

@misc{image-watermark-fing,
	Author = {Jonathan Bailey},
	Howpublished = {\url{https://www.plagiarismtoday.com/2009/12/02/image-detection-watermarking-vs-fingerprinting/}},
	Title = {{Image Detection: Watermarking vs. Fingerprinting}},
	Year = {2009}}

@inproceedings{Servetto98,
	Author = {S. D. Servetto and C. I. Podilchuk and K. Ramchandran},
	Booktitle = {Int. Conf. Image Processing},
	Title = {Capacity issues in digital image watermarking},
	Year = {1998}}

@inproceedings{Chen01,
	Author = {B. Chen and G.W.Wornell},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1423--1443},
	Title = {Quantization index modulation: A class of provably good methods for digital watermarking and information embedding},
	Year = {2001}}

@inproceedings{Karakos00,
	Author = {D. Karakos and A. Papamarcou},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {47},
	Title = {Relationship between quantization and distribution rates of digitally watermarked data},
	Year = {2000}}

@inproceedings{Sullivan98,
	Author = {J. A. OSullivan and P. Moulin and J. M. Ettinger},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {297},
	Title = {Information theoretic analysis of steganography},
	Year = {1998}}

@inproceedings{Merhav00,
	Author = {N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {420--430},
	Title = {On random coding error exponents of watermarking systems},
	Year = {2000}}

@inproceedings{Somekh01,
	Author = {A. Somekh-Baruch and N. Merhav},
	Booktitle = {IEEE Int. Symp. Information Theory},
	Pages = {7},
	Title = {On the error exponent and capacity games of private watermarking systems},
	Year = {2001}}

@inproceedings{Steinberg01,
	Author = {Y. Steinberg and N. Merhav},
	Booktitle = {IEEE Trans. Inform. Theory},
	Pages = {1410--1422},
	Title = {Identification in the presence of side information with application to watermarking},
	Year = {2001}}

@article{Moulin03,
	Author = {P. Moulin and J.A. O'Sullivan},
	Journal = {IEEE Trans. Info. Theory},
	Number = {3},
	Title = {Information-theoretic analysis of information hiding},
	Volume = 49,
	Year = 2003}

@article{Gelfand80,
	Author = {S.I.~Gelfand and M.S.~Pinsker},
	Journal = {Problems of Control and Information Theory},
	Number = {1},
	Pages = {19-31},
	Title = {{Coding for channel with random parameters}},
	Url = {citeseer.ist.psu.edu/anantharam96bits.html},
	Volume = {9},
	Year = {1980},
	Bdsk-Url-1 = {citeseer.ist.psu.edu/anantharam96bits.html}}

@book{Wolfowitz78,
	Author = {J. Wolfowitz},
	Edition = {3rd},
	Location = {New York},
	Publisher = {Springer-Verlag},
	Title = {Coding Theorems of Information Theory},
	Year = 1978}

@article{caire99,
	Author = {G. Caire and S. Shamai},
	Journal = {IEEE Transactions on Information Theory},
	Number = {6},
	Pages = {2007--2019},
	Title = {On the Capacity of Some Channels with Channel State Information},
	Volume = {45},
	Year = {1999}}

@inproceedings{wright2007language,
	Author = {Wright, Charles V and Ballard, Lucas and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {USENIX Security},
	Title = {{Language identification of encrypted VoIP traffic: Alejandra y Roberto or Alice and Bob?}},
	Year = {2007}}

@inproceedings{backes2010speaker,
	Author = {Backes, Michael and Doychev, Goran and D{\"u}rmuth, Markus and K{\"o}pf, Boris},
	Booktitle = {{European Symposium on Research in Computer Security (ESORICS)}},
	Pages = {508--523},
	Publisher = {Springer},
	Title = {{Speaker Recognition in Encrypted Voice Streams}},
	Year = {2010}}

@phdthesis{lu2009traffic,
	Author = {Lu, Yuanchao},
	School = {Cleveland State University},
	Title = {{On Traffic Analysis Attacks to Encrypted VoIP Calls}},
	Year = {2009}}

@inproceedings{wright2008spot,
	Author = {Wright, Charles V and Ballard, Lucas and Coull, Scott E and Monrose, Fabian and Masson, Gerald M},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {35--49},
	Title = {Spot me if you can: Uncovering spoken phrases in encrypted VoIP conversations},
	Year = {2008}}

@inproceedings{white2011phonotactic,
	Author = {White, Andrew M and Matthews, Austin R and Snow, Kevin Z and Monrose, Fabian},
	Booktitle = {IEEE Symposium on Security and Privacy},
	Pages = {3--18},
	Title = {Phonotactic reconstruction of encrypted VoIP conversations: Hookt on fon-iks},
	Year = {2011}}

@inproceedings{fancy,
	Author = {Houmansadr, Amir and Borisov, Nikita},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {205--224},
	Title = {The Need for Flow Fingerprints to Link Correlated Network Flows},
	Year = {2013}}

@article{botmosaic,
	Author = {Amir Houmansadr and Nikita Borisov},
	Doi = {10.1016/j.jss.2012.11.005},
	Issn = {0164-1212},
	Journal = {Journal of Systems and Software},
	Keywords = {Network security},
	Number = {3},
	Pages = {707 - 715},
	Title = {BotMosaic: Collaborative network watermark for the detection of IRC-based botnets},
	Url = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Volume = {86},
	Year = {2013},
	Bdsk-Url-1 = {http://www.sciencedirect.com/science/article/pii/S0164121212003068},
	Bdsk-Url-2 = {http://dx.doi.org/10.1016/j.jss.2012.11.005}}

@inproceedings{ramsbrock2008first,
	Author = {Ramsbrock, Daniel and Wang, Xinyuan and Jiang, Xuxian},
	Booktitle = {Recent Advances in Intrusion Detection},
	Organization = {Springer},
	Pages = {59--77},
	Title = {A first step towards live botmaster traceback},
	Year = {2008}}

@inproceedings{potdar2005survey,
	Author = {Potdar, Vidyasagar M and Han, Song and Chang, Elizabeth},
	Booktitle = {Industrial Informatics, 2005. INDIN'05. 2005 3rd IEEE International Conference on},
	Organization = {IEEE},
	Pages = {709--716},
	Title = {A survey of digital image watermarking techniques},
	Year = {2005}}

@book{cole2003hiding,
	Author = {Cole, Eric and Krutz, Ronald D},
	Publisher = {John Wiley \& Sons, Inc.},
	Title = {Hiding in plain sight: Steganography and the art of covert communication},
	Year = {2003}}

@incollection{akaike1998information,
	Author = {Akaike, Hirotogu},
	Booktitle = {Selected Papers of Hirotugu Akaike},
	Pages = {199--213},
	Publisher = {Springer},
	Title = {Information theory and an extension of the maximum likelihood principle},
	Year = {1998}}

@misc{central-command-hack,
	Author = {Everett Rosenfeld},
	Howpublished = {\url{http://www.cnbc.com/id/102330338}},
	Title = {{FBI investigating Central Command Twitter hack}},
	Year = {2015}}

@misc{sony-psp-ddos,
	Howpublished = {\url{http://n4g.com/news/1644853/sony-and-microsoft-cant-do-much-ddos-attacks-explained}},
	Key = {sony},
	Month = {December},
	Title = {{Sony and Microsoft cant do much -- DDoS attacks explained}},
	Year = {2014}}

@misc{sony-hack,
	Author = {David Bloom},
	Howpublished = {\url{http://goo.gl/MwR4A7}},
	Title = {{Online Game Networks Hacked, Sony Unit President Threatened}},
	Year = {2014}}

@misc{home-depot,
	Author = {Dune Lawrence},
	Howpublished = {\url{http://www.businessweek.com/articles/2014-09-02/home-depots-credit-card-breach-looks-just-like-the-target-hack}},
	Title = {{Home Depot's Suspected Breach Looks Just Like the Target Hack}},
	Year = {2014}}

@misc{target,
	Author = {Julio Ojeda-Zapata},
	Howpublished = {\url{http://www.mercurynews.com/business/ci_24765398/how-did-hackers-pull-off-target-data-heist}},
	Title = {{Target hack: How did they do it?}},
	Year = {2014}}


@article{probabilitycourse,
	Author = {H. Pishro-Nik},
	note = {\url{http://www.probabilitycourse.com}},
	Title = {Introduction to probability, statistics, and random processes},
    Year = {2014}}



@inproceedings{shokri2011quantifying,
	Author = {Shokri, Reza and Theodorakopoulos, George and Le Boudec, Jean-Yves and Hubaux, Jean-Pierre},
	Booktitle = {Security and Privacy (SP), 2011 IEEE Symposium on},
	Organization = {IEEE},
	Pages = {247--262},
	Title = {Quantifying location privacy},
	Year = {2011}}

@inproceedings{hoh2007preserving,
	Author = {Hoh, Baik and Gruteser, Marco and Xiong, Hui and Alrabady, Ansaf},
	Booktitle = {Proceedings of the 14th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {161--171},
	Title = {Preserving privacy in gps traces via uncertainty-aware path cloaking},
	Year = {2007}}



@article{kafsi2013entropy,
	Author = {Kafsi, Mohamed and Grossglauser, Matthias and Thiran, Patrick},
	Journal = {Information Theory, IEEE Transactions on},
	Number = {9},
	Pages = {5577--5583},
	Publisher = {IEEE},
	Title = {The entropy of conditional Markov trajectories},
	Volume = {59},
	Year = {2013}}

@inproceedings{gruteser2003anonymous,
	Author = {Gruteser, Marco and Grunwald, Dirk},
	Booktitle = {Proceedings of the 1st international conference on Mobile systems, applications and services},
	Organization = {ACM},
	Pages = {31--42},
	Title = {Anonymous usage of location-based services through spatial and temporal cloaking},
	Year = {2003}}

@inproceedings{husted2010mobile,
	Author = {Husted, Nathaniel and Myers, Steven},
	Booktitle = {Proceedings of the 17th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {85--96},
	Title = {Mobile location tracking in metro areas: malnets and others},
	Year = {2010}}

@inproceedings{li2009tradeoff,
	Author = {Li, Tiancheng and Li, Ninghui},
	Booktitle = {Proceedings of the 15th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {517--526},
	Title = {On the tradeoff between privacy and utility in data publishing},
	Year = {2009}}

@inproceedings{ma2009location,
	Author = {Ma, Zhendong and Kargl, Frank and Weber, Michael},
	Booktitle = {Sarnoff Symposium, 2009. SARNOFF'09. IEEE},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {A location privacy metric for v2x communication systems},
	Year = {2009}}

@inproceedings{shokri2012protecting,
	Author = {Shokri, Reza and Theodorakopoulos, George and Troncoso, Carmela and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
	Booktitle = {Proceedings of the 2012 ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {617--627},
	Title = {Protecting location privacy: optimal strategy against localization attacks},
	Year = {2012}}

@inproceedings{freudiger2009non,
	Author = {Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
	Booktitle = {Proceedings of the 16th ACM conference on Computer and communications security},
	Organization = {ACM},
	Pages = {324--337},
	Title = {On non-cooperative location privacy: a game-theoretic analysis},
	Year = {2009}}

@incollection{humbert2010tracking,
	Author = {Humbert, Mathias and Manshaei, Mohammad Hossein and Freudiger, Julien and Hubaux, Jean-Pierre},
	Booktitle = {Decision and Game Theory for Security},
	Pages = {38--57},
	Publisher = {Springer},
	Title = {Tracking games in mobile networks},
	Year = {2010}}

@article{manshaei2013game,
	Author = {Manshaei, Mohammad Hossein and Zhu, Quanyan and Alpcan, Tansu and Bac{\c{s}}ar, Tamer and Hubaux, Jean-Pierre},
	Journal = {ACM Computing Surveys (CSUR)},
	Number = {3},
	Pages = {25},
	Publisher = {ACM},
	Title = {Game theory meets network security and privacy},
	Volume = {45},
	Year = {2013}}

@article{palamidessi2006probabilistic,
	Author = {Palamidessi, Catuscia},
	Journal = {Electronic Notes in Theoretical Computer Science},
	Pages = {33--42},
	Publisher = {Elsevier},
	Title = {Probabilistic and nondeterministic aspects of anonymity},
	Volume = {155},
	Year = {2006}}

@inproceedings{mokbel2006new,
	Author = {Mokbel, Mohamed F and Chow, Chi-Yin and Aref, Walid G},
	Booktitle = {Proceedings of the 32nd international conference on Very large data bases},
	Organization = {VLDB Endowment},
	Pages = {763--774},
	Title = {The new Casper: query processing for location services without compromising privacy},
	Year = {2006}}

@article{kalnis2007preventing,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {12},
	Pages = {1719--1733},
	Publisher = {IEEE},
	Title = {Preventing location-based identity inference in anonymous spatial queries},
	Volume = {19},
	Year = {2007}}
	
@article{freudiger2007mix,
  title={Mix-zones for location privacy in vehicular networks},
  author={Freudiger, Julien and Raya, Maxim and F{\'e}legyh{\'a}zi, M{\'a}rk and Papadimitratos, Panos and Hubaux, Jean-Pierre},
  year={2007}
}
@article{sweeney2002k,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {557--570},
	Publisher = {World Scientific},
	Title = {k-anonymity: A model for protecting privacy},
	Volume = {10},
	Year = {2002}}

@article{sweeney2002achieving,
	Author = {Sweeney, Latanya},
	Journal = {International Journal of Uncertainty, Fuzziness and Knowledge-Based Systems},
	Number = {05},
	Pages = {571--588},
	Publisher = {World Scientific},
	Title = {Achieving k-anonymity privacy protection using generalization and suppression},
	Volume = {10},
	Year = {2002}}

@inproceedings{niu2014achieving,
	Author = {Niu, Ben and Li, Qinghua and Zhu, Xiaoyan and Cao, Guohong and Li, Hui},
	Booktitle = {INFOCOM, 2014 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {754--762},
	Title = {Achieving k-anonymity in privacy-aware location-based services},
	Year = {2014}}

@inproceedings{liu2013game,
	Author = {Liu, Xinxin and Liu, Kaikai and Guo, Linke and Li, Xiaolin and Fang, Yuguang},
	Booktitle = {INFOCOM, 2013 Proceedings IEEE},
	Organization = {IEEE},
	Pages = {2985--2993},
	Title = {A game-theoretic approach for achieving k-anonymity in location based services},
	Year = {2013}}

@inproceedings{kido2005protection,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Data Engineering Workshops, 2005. 21st International Conference on},
	Organization = {IEEE},
	Pages = {1248--1248},
	Title = {Protection of location privacy using dummies for location-based services},
	Year = {2005}}

@inproceedings{gedik2005location,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Booktitle = {Distributed Computing Systems, 2005. ICDCS 2005. Proceedings. 25th IEEE International Conference on},
	Organization = {IEEE},
	Pages = {620--629},
	Title = {Location privacy in mobile systems: A personalized anonymization model},
	Year = {2005}}

@inproceedings{bordenabe2014optimal,
	Author = {Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2014 ACM SIGSAC Conference on Computer and Communications Security},
	Organization = {ACM},
	Pages = {251--262},
	Title = {Optimal geo-indistinguishable mechanisms for location privacy},
	Year = {2014}}

@incollection{duckham2005formal,
	Author = {Duckham, Matt and Kulik, Lars},
	Booktitle = {Pervasive computing},
	Pages = {152--170},
	Publisher = {Springer},
	Title = {A formal model of obfuscation and negotiation for location privacy},
	Year = {2005}}

@inproceedings{kido2005anonymous,
	Author = {Kido, Hidetoshi and Yanagisawa, Yutaka and Satoh, Tetsuji},
	Booktitle = {Pervasive Services, 2005. ICPS'05. Proceedings. International Conference on},
	Organization = {IEEE},
	Pages = {88--97},
	Title = {An anonymous communication technique using dummies for location-based services},
	Year = {2005}}

@incollection{duckham2006spatiotemporal,
	Author = {Duckham, Matt and Kulik, Lars and Birtley, Athol},
	Booktitle = {Geographic Information Science},
	Pages = {47--64},
	Publisher = {Springer},
	Title = {A spatiotemporal model of strategies and counter strategies for location privacy protection},
	Year = {2006}}

@inproceedings{shankar2009privately,
	Author = {Shankar, Pravin and Ganapathy, Vinod and Iftode, Liviu},
	Booktitle = {Proceedings of the 11th international conference on Ubiquitous computing},
	Organization = {ACM},
	Pages = {31--40},
	Title = {Privately querying location-based services with SybilQuery},
	Year = {2009}}

@inproceedings{chow2009faking,
	Author = {Chow, Richard and Golle, Philippe},
	Booktitle = {Proceedings of the 8th ACM workshop on Privacy in the electronic society},
	Organization = {ACM},
	Pages = {105--108},
	Title = {Faking contextual data for fun, profit, and privacy},
	Year = {2009}}

@incollection{xue2009location,
	Author = {Xue, Mingqiang and Kalnis, Panos and Pung, Hung Keng},
	Booktitle = {Location and Context Awareness},
	Pages = {70--87},
	Publisher = {Springer},
	Title = {Location diversity: Enhanced privacy protection in location based services},
	Year = {2009}}

@article{wernke2014classification,
	Author = {Wernke, Marius and Skvortsov, Pavel and D{\"u}rr, Frank and Rothermel, Kurt},
	Journal = {Personal and Ubiquitous Computing},
	Number = {1},
	Pages = {163--175},
	Publisher = {Springer-Verlag},
	Title = {A classification of location privacy attacks and approaches},
	Volume = {18},
	Year = {2014}}

@misc{cai2015cloaking,
	Author = {Cai, Y. and Xu, G.},
	Month = jan # {~1},
	Note = {US Patent App. 14/472,462},
	Publisher = {Google Patents},
	Title = {Cloaking with footprints to provide location privacy protection in location-based services},
	Url = {https://www.google.com/patents/US20150007341},
	Year = {2015},
	Bdsk-Url-1 = {https://www.google.com/patents/US20150007341}}

@article{gedik2008protecting,
	Author = {Gedik, Bu{\u{g}}ra and Liu, Ling},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {1},
	Pages = {1--18},
	Publisher = {IEEE},
	Title = {Protecting location privacy with personalized k-anonymity: Architecture and algorithms},
	Volume = {7},
	Year = {2008}}

@article{kalnis2006preserving,
	Author = {Kalnis, Panos and Ghinita, Gabriel and Mouratidis, Kyriakos and Papadias, Dimitris},
	Publisher = {TRB6/06},
	Title = {Preserving anonymity in location based services},
	Year = {2006}}

@inproceedings{hoh2005protecting,
	Author = {Hoh, Baik and Gruteser, Marco},
	Booktitle = {Security and Privacy for Emerging Areas in Communications Networks, 2005. SecureComm 2005. First International Conference on},
	Organization = {IEEE},
	Pages = {194--205},
	Title = {Protecting location privacy through path confusion},
	Year = {2005}}

@article{terrovitis2011privacy,
	Author = {Terrovitis, Manolis},
	Journal = {ACM SIGKDD Explorations Newsletter},
	Number = {1},
	Pages = {6--18},
	Publisher = {ACM},
	Title = {Privacy preservation in the dissemination of location data},
	Volume = {13},
	Year = {2011}}

@article{shin2012privacy,
	Author = {Shin, Kang G and Ju, Xiaoen and Chen, Zhigang and Hu, Xin},
	Journal = {Wireless Communications, IEEE},
	Number = {1},
	Pages = {30--39},
	Publisher = {IEEE},
	Title = {Privacy protection for users of location-based services},
	Volume = {19},
	Year = {2012}}

@article{khoshgozaran2011location,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus and Shirani-Mehr, Houtan},
	Journal = {Knowledge and Information Systems},
	Number = {3},
	Pages = {435--465},
	Publisher = {Springer},
	Title = {Location privacy: going beyond K-anonymity, cloaking and anonymizers},
	Volume = {26},
	Year = {2011}}

@incollection{chatzikokolakis2015geo,
	Author = {Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
	Booktitle = {Distributed Computing and Internet Technology},
	Pages = {49--72},
	Publisher = {Springer},
	Title = {Geo-indistinguishability: A Principled Approach to Location Privacy},
	Year = {2015}}

@inproceedings{ngo2015location,
	Author = {Ngo, Hoa and Kim, Jong},
	Booktitle = {Computer Security Foundations Symposium (CSF), 2015 IEEE 28th},
	Organization = {IEEE},
	Pages = {63--74},
	Title = {Location Privacy via Differential Private Perturbation of Cloaking Area},
	Year = {2015}}

@inproceedings{palanisamy2011mobimix,
	Author = {Palanisamy, Balaji and Liu, Ling},
	Booktitle = {Data Engineering (ICDE), 2011 IEEE 27th International Conference on},
	Organization = {IEEE},
	Pages = {494--505},
	Title = {Mobimix: Protecting location privacy with mix-zones over road networks},
	Year = {2011}}

@inproceedings{um2010advanced,
	Author = {Um, Jung-Ho and Kim, Hee-Dae and Chang, Jae-Woo},
	Booktitle = {Social Computing (SocialCom), 2010 IEEE Second International Conference on},
	Organization = {IEEE},
	Pages = {1093--1098},
	Title = {An advanced cloaking algorithm using Hilbert curves for anonymous location based service},
	Year = {2010}}

@inproceedings{bamba2008supporting,
	Author = {Bamba, Bhuvan and Liu, Ling and Pesti, Peter and Wang, Ting},
	Booktitle = {Proceedings of the 17th international conference on World Wide Web},
	Organization = {ACM},
	Pages = {237--246},
	Title = {Supporting anonymous location queries in mobile environments with privacygrid},
	Year = {2008}}

@inproceedings{zhangwei2010distributed,
	Author = {Zhangwei, Huang and Mingjun, Xin},
	Booktitle = {Networks Security Wireless Communications and Trusted Computing (NSWCTC), 2010 Second International Conference on},
	Organization = {IEEE},
	Pages = {468--471},
	Title = {A distributed spatial cloaking protocol for location privacy},
	Volume = {2},
	Year = {2010}}

@article{chow2011spatial,
	Author = {Chow, Chi-Yin and Mokbel, Mohamed F and Liu, Xuan},
	Journal = {GeoInformatica},
	Number = {2},
	Pages = {351--380},
	Publisher = {Springer},
	Title = {Spatial cloaking for anonymous location-based services in mobile peer-to-peer environments},
	Volume = {15},
	Year = {2011}}

@inproceedings{lu2008pad,
	Author = {Lu, Hua and Jensen, Christian S and Yiu, Man Lung},
	Booktitle = {Proceedings of the Seventh ACM International Workshop on Data Engineering for Wireless and Mobile Access},
	Organization = {ACM},
	Pages = {16--23},
	Title = {Pad: privacy-area aware, dummy-based location privacy in mobile services},
	Year = {2008}}

@incollection{khoshgozaran2007blind,
	Author = {Khoshgozaran, Ali and Shahabi, Cyrus},
	Booktitle = {Advances in Spatial and Temporal Databases},
	Pages = {239--257},
	Publisher = {Springer},
	Title = {Blind evaluation of nearest neighbor queries using space transformation to preserve location privacy},
	Year = {2007}}

@inproceedings{ghinita2008private,
	Author = {Ghinita, Gabriel and Kalnis, Panos and Khoshgozaran, Ali and Shahabi, Cyrus and Tan, Kian-Lee},
	Booktitle = {Proceedings of the 2008 ACM SIGMOD international conference on Management of data},
	Organization = {ACM},
	Pages = {121--132},
	Title = {Private queries in location based services: anonymizers are not necessary},
	Year = {2008}}

@article{paulet2014privacy,
	Author = {Paulet, Russell and Kaosar, Md Golam and Yi, Xun and Bertino, Elisa},
	Journal = {Knowledge and Data Engineering, IEEE Transactions on},
	Number = {5},
	Pages = {1200--1210},
	Publisher = {IEEE},
	Title = {Privacy-preserving and content-protecting location based queries},
	Volume = {26},
	Year = {2014}}

@article{nguyen2013differential,
	Author = {Nguyen, Hiep H and Kim, Jong and Kim, Yoonho},
	Journal = {Journal of Computing Science and Engineering},
	Number = {3},
	Pages = {177--186},
	Title = {Differential privacy in practice},
	Volume = {7},
	Year = {2013}}

@inproceedings{lee2012differential,
	Author = {Lee, Jaewoo and Clifton, Chris},
	Booktitle = {Proceedings of the 18th ACM SIGKDD international conference on Knowledge discovery and data mining},
	Organization = {ACM},
	Pages = {1041--1049},
	Title = {Differential identifiability},
	Year = {2012}}

@inproceedings{andres2013geo,
	Author = {Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s E and Chatzikokolakis, Konstantinos and Palamidessi, Catuscia},
	Booktitle = {Proceedings of the 2013 ACM SIGSAC conference on Computer \& communications security},
	Organization = {ACM},
	Pages = {901--914},
	Title = {Geo-indistinguishability: Differential privacy for location-based systems},
	Year = {2013}}

@inproceedings{machanavajjhala2008privacy,
	Author = {Machanavajjhala, Ashwin and Kifer, Daniel and Abowd, John and Gehrke, Johannes and Vilhuber, Lars},
	Booktitle = {Data Engineering, 2008. ICDE 2008. IEEE 24th International Conference on},
	Organization = {IEEE},
	Pages = {277--286},
	Title = {Privacy: Theory meets practice on the map},
	Year = {2008}}

@article{dewri2013local,
	Author = {Dewri, Rinku},
	Journal = {Mobile Computing, IEEE Transactions on},
	Number = {12},
	Pages = {2360--2372},
	Publisher = {IEEE},
	Title = {Local differential perturbations: Location privacy under approximate knowledge attackers},
	Volume = {12},
	Year = {2013}}

@inproceedings{chatzikokolakis2013broadening,
	Author = {Chatzikokolakis, Konstantinos and Andr{\'e}s, Miguel E and Bordenabe, Nicol{\'a}s Emilio and Palamidessi, Catuscia},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {82--102},
	Title = {Broadening the Scope of Differential Privacy Using Metrics.},
	Year = {2013}}

@inproceedings{zhong2009distributed,
	Author = {Zhong, Ge and Hengartner, Urs},
	Booktitle = {Pervasive Computing and Communications, 2009. PerCom 2009. IEEE International Conference on},
	Organization = {IEEE},
	Pages = {1--10},
	Title = {A distributed k-anonymity protocol for location privacy},
	Year = {2009}}

@inproceedings{ho2011differential,
	Author = {Ho, Shen-Shyang and Ruan, Shuhua},
	Booktitle = {Proceedings of the 4th ACM SIGSPATIAL International Workshop on Security and Privacy in GIS and LBS},
	Organization = {ACM},
	Pages = {17--24},
	Title = {Differential privacy for location pattern mining},
	Year = {2011}}

@inproceedings{cheng2006preserving,
	Author = {Cheng, Reynold and Zhang, Yu and Bertino, Elisa and Prabhakar, Sunil},
	Booktitle = {Privacy Enhancing Technologies},
	Organization = {Springer},
	Pages = {393--412},
	Title = {Preserving user location privacy in mobile data management infrastructures},
	Year = {2006}}

@article{beresford2003location,
	Author = {Beresford, Alastair R and Stajano, Frank},
	Journal = {IEEE Pervasive computing},
	Number = {1},
	Pages = {46--55},
	Publisher = {IEEE},
	Title = {Location privacy in pervasive computing},
	Year = {2003}}

@inproceedings{freudiger2009optimal,
	Author = {Freudiger, Julien and Shokri, Reza and Hubaux, Jean-Pierre},
	Booktitle = {Privacy enhancing technologies},
	Organization = {Springer},
	Pages = {216--234},
	Title = {On the optimal placement of mix zones},
	Year = {2009}}

@article{krumm2009survey,
	Author = {Krumm, John},
	Journal = {Personal and Ubiquitous Computing},
	Number = {6},
	Pages = {391--399},
	Publisher = {Springer},
	Title = {A survey of computational location privacy},
	Volume = {13},
	Year = {2009}}

@article{Rakhshan2016letter,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Wireless Communications Letter},
	Publisher = {IEEE},
	Title = {Interference Models for Vehicular Ad Hoc Networks},
	Year = {2016, submitted}}

@article{Rakhshan2015Journal,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Publisher = {IEEE},
	Title = {Improving Safety on Highways by Customizing Vehicular Ad Hoc Networks},
	Year = {to appear, 2017}}

@inproceedings{Rakhshan2015Cogsima,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Booktitle = {IEEE International Multi-Disciplinary Conference on Cognitive Methods in Situation Awareness and Decision Support},
	Organization = {IEEE},
	Title = {A New Approach to Customization of Accident Warning Systems to Individual Drivers},
	Year = {2015}}

@inproceedings{Rakhshan2015CISS,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Nekoui, Mohammad},
	Booktitle = {Conference on Information Sciences and Systems},
	Organization = {IEEE},
	Pages = {1--6},
	Title = {Driver-based adaptation of Vehicular Ad Hoc Networks for design of active safety systems},
	Year = {2015}}

@inproceedings{Rakhshan2014IV,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Ray, Evan},
	Booktitle = {Intelligent Vehicles Symposium},
	Organization = {IEEE},
	Pages = {1181--1186},
	Title = {Real-time estimation of the distribution of brake response times for an individual driver using Vehicular Ad Hoc Network.},
	Year = {2014}}

@inproceedings{Rakhshan2013Globecom,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein and Fisher, Donald and Nekoui, Mohammad},
	Booktitle = {IEEE Global Communications Conference},
	Organization = {IEEE},
	Pages = {1333--1337},
	Title = {Tuning collision warning algorithms to individual drivers for design of active safety systems.},
	Year = {2013}}

@article{Nekoui2012Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Wireless Communications},
	Number = {8},
	Pages = {2895--2905},
	Publisher = {IEEE},
	Title = {Throughput Scaling laws for Vehicular Ad Hoc Networks},
	Volume = {11},
	Year = {2012}}









@article{Nekoui2011Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein and Ni, Daiheng},
	Journal = {International Journal of Vehicular Technology},
	Pages = {1--11},
	Publisher = {Hindawi Publishing Corporation},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {2011},
	Year = {2011}}





	
@article{shokri2014optimal,
	  title={Optimal user-centric data obfuscation},
 	 author={Shokri, Reza},
 	 journal={arXiv preprint arXiv:1402.3426},
 	 year={2014}
	}
@article{chatzikokolakis2015location,
  title={Location privacy via geo-indistinguishability},
  author={Chatzikokolakis, Konstantinos and Palamidessi, Catuscia and Stronati, Marco},
  journal={ACM SIGLOG News},
  volume={2},
  number={3},
  pages={46--69},
  year={2015},
  publisher={ACM}

}
@inproceedings{shokri2011quantifying2,
  title={Quantifying location privacy: the case of sporadic location exposure},
  author={Shokri, Reza and Theodorakopoulos, George and Danezis, George and Hubaux, Jean-Pierre and Le Boudec, Jean-Yves},
  booktitle={Privacy Enhancing Technologies},
  pages={57--76},
  year={2011},
  organization={Springer}
}


@inproceedings{Mont1603:Defining,
AUTHOR="Zarrin Montazeri and Amir Houmansadr and Hossein Pishro-Nik",
TITLE="Defining Perfect Location Privacy Using Anonymization",
BOOKTITLE="2016 Annual Conference on Information Science and Systems (CISS) (CISS
2016)",
ADDRESS="Princeton, USA",
DAYS=16,
MONTH=mar,
YEAR=2016,
KEYWORDS="Information Theoretic Privacy; location-based services; Location Privacy;
Information Theory",
ABSTRACT="The popularity of mobile devices and location-based services (LBS) have
created great concerns regarding the location privacy of users of such
devices and services. Anonymization is a common technique that is often
being used to protect the location privacy of LBS users. In this paper, we
provide a general information theoretic definition for location privacy. In
particular, we define perfect location privacy. We show that under certain
conditions, perfect privacy is achieved if the pseudonyms of users is
changed after o(N^(2/r?1)) observations by the adversary, where N is the
number of users and r is the number of sub-regions or locations.
"
}
@article{our-isita-location,
	Author = {Zarrin Montazeri and Amir Houmansadr and Hossein Pishro-Nik},
	Journal = {IEEE International Symposium on Information Theory and Its Applications (ISITA)},
	Title = {Achieving Perfect Location Privacy in Markov Models Using Anonymization},
	Year = {2016}
	}
@article{our-TIFS,
	Author = {Zarrin Montazeri and Hossein Pishro-Nik and Amir Houmansadr},
	Journal = {IEEE Transactions on Information Forensics and Security, accepted with mandatory minor revisions},
	Title = {Perfect Location Privacy Using Anonymization in Mobile Networks},
	Year = {2017},
    note={Available on arxiv.org}
	}



@techreport{sampigethaya2005caravan,
  title={CARAVAN: Providing location privacy for VANET},
  author={Sampigethaya, Krishna and Huang, Leping and Li, Mingyan and Poovendran, Radha and Matsuura, Kanta and Sezaki, Kaoru},
  year={2005},
  institution={DTIC Document}
}
@incollection{buttyan2007effectiveness,
  title={On the effectiveness of changing pseudonyms to provide location privacy in VANETs},
  author={Butty{\'a}n, Levente and Holczer, Tam{\'a}s and Vajda, Istv{\'a}n},
  booktitle={Security and Privacy in Ad-hoc and Sensor Networks},
  pages={129--141},
  year={2007},
  publisher={Springer}
}
@article{sampigethaya2007amoeba,
  title={AMOEBA: Robust location privacy scheme for VANET},
  author={Sampigethaya, Krishna and Li, Mingyan and Huang, Leping and Poovendran, Radha},
  journal={Selected Areas in communications, IEEE Journal on},
  volume={25},
  number={8},
  pages={1569--1589},
  year={2007},
  publisher={IEEE}
}

@article{lu2012pseudonym,
  title={Pseudonym changing at social spots: An effective strategy for location privacy in vanets},
  author={Lu, Rongxing and Li, Xiaodong and Luan, Tom H and Liang, Xiaohui and Shen, Xuemin},
  journal={Vehicular Technology, IEEE Transactions on},
  volume={61},
  number={1},
  pages={86--96},
  year={2012},
  publisher={IEEE}
}
@inproceedings{lu2010sacrificing,
  title={Sacrificing the plum tree for the peach tree: A socialspot tactic for protecting receiver-location privacy in VANET},
  author={Lu, Rongxing and Lin, Xiaodong and Liang, Xiaohui and Shen, Xuemin},
  booktitle={Global Telecommunications Conference (GLOBECOM 2010), 2010 IEEE},
  pages={1--5},
  year={2010},
  organization={IEEE}
}
@inproceedings{lin2011stap,
  title={STAP: A social-tier-assisted packet forwarding protocol for achieving receiver-location privacy preservation in VANETs},
  author={Lin, Xiaodong and Lu, Rongxing and Liang, Xiaohui and Shen, Xuemin Sherman},
  booktitle={INFOCOM, 2011 Proceedings IEEE},
  pages={2147--2155},
  year={2011},
  organization={IEEE}
}
@inproceedings{gerlach2007privacy,
  title={Privacy in VANETs using changing pseudonyms-ideal and real},
  author={Gerlach, Matthias and Guttler, Felix},
  booktitle={Vehicular Technology Conference, 2007. VTC2007-Spring. IEEE 65th},
  pages={2521--2525},
  year={2007},
  organization={IEEE}
}
@inproceedings{el2002security,
  title={Security issues in a future vehicular network},
  author={El Zarki, Magda and Mehrotra, Sharad and Tsudik, Gene and Venkatasubramanian, Nalini},
  booktitle={European Wireless},
  volume={2},
  year={2002}
}

@article{hubaux2004security,
  title={The security and privacy of smart vehicles},
  author={Hubaux, Jean-Pierre and Capkun, Srdjan and Luo, Jun},
  journal={IEEE Security \& Privacy Magazine},
  volume={2},
  number={LCA-ARTICLE-2004-007},
  pages={49--55},
  year={2004}
}



@inproceedings{duri2002framework,
  title={Framework for security and privacy in automotive telematics},
  author={Duri, Sastry and Gruteser, Marco and Liu, Xuan and Moskowitz, Paul and Perez, Ronald and Singh, Moninder and Tang, Jung-Mu},
  booktitle={Proceedings of the 2nd international workshop on Mobile commerce},
  pages={25--32},
  year={2002},
  organization={ACM}
}
@misc{NS-3,
	Howpublished = {\url{https://www.nsnam.org/}}},
}
@misc{testbed,
	Howpublished = {\url{http://www.its.dot.gov/testbed/PDF/SE-MI-Resource-Guide-9-3-1.pdf}}},
@misc{NGSIM,
	Howpublished = {\url{http://ops.fhwa.dot.gov/trafficanalysistools/ngsim.htm}},
	}

@misc{National-a2013,
	Author = {National Highway Traffic Safety Administration},
	Howpublished = {\url{http://ops.fhwa.dot.gov/trafficanalysistools/ngsim.htm}},
	Title = {2013 Motor Vehicle Crashes: Overview. Traffic Safety Factors},
	Year = {2013}
	}

	@inproceedings{karnadi2007rapid,
	  title={Rapid generation of realistic mobility models for VANET},
	  author={Karnadi, Feliz Kristianto and Mo, Zhi Hai and Lan, Kun-chan},
	  booktitle={Wireless Communications and Networking Conference, 2007. WCNC 2007. IEEE},
	  pages={2506--2511},
	  year={2007},
	  organization={IEEE}
	}
	@inproceedings{saha2004modeling,
  title={Modeling mobility for vehicular ad-hoc networks},
  author={Saha, Amit Kumar and Johnson, David B},
  booktitle={Proceedings of the 1st ACM international workshop on Vehicular ad hoc networks},
  pages={91--92},
  year={2004},
  organization={ACM}
}
@inproceedings{lee2006modeling,
  title={Modeling steady-state and transient behaviors of user mobility: formulation, analysis, and application},
  author={Lee, Jong-Kwon and Hou, Jennifer C},
  booktitle={Proceedings of the 7th ACM international symposium on Mobile ad hoc networking and computing},
  pages={85--96},
  year={2006},
  organization={ACM}
}
@inproceedings{yoon2006building,
  title={Building realistic mobility models from coarse-grained traces},
  author={Yoon, Jungkeun and Noble, Brian D and Liu, Mingyan and Kim, Minkyong},
  booktitle={Proceedings of the 4th international conference on Mobile systems, applications and services},
  pages={177--190},
  year={2006},
  organization={ACM}
}

@inproceedings{choffnes2005integrated,
	title={An integrated mobility and traffic model for vehicular wireless networks},
	author={Choffnes, David R and Bustamante, Fabi{\'a}n E},
	booktitle={Proceedings of the 2nd ACM international workshop on Vehicular ad hoc networks},
	pages={69--78},
	year={2005},
	organization={ACM}
}

@inproceedings{Qian2008Globecom,
	title={CA Secure VANET MAC Protocol for DSRC Applications},
	author={Yi, Q. and Lu, K. and Moyeri, N.{\'a}n E},
	booktitle={Proceedings of IEEE GLOBECOM 2008},
	pages={1--5},
	year={2008},
	organization={IEEE}
}





	@inproceedings{naumov2006evaluation,
  title={An evaluation of inter-vehicle ad hoc networks based on realistic vehicular traces},
  author={Naumov, Valery and Baumann, Rainer and Gross, Thomas},
  booktitle={Proceedings of the 7th ACM international symposium on Mobile ad hoc networking and computing},
  pages={108--119},
  year={2006},
  organization={ACM}
}
	@article{sommer2008progressing,
  title={Progressing toward realistic mobility models in VANET simulations},
  author={Sommer, Christoph and Dressler, Falko},
  journal={Communications Magazine, IEEE},
  volume={46},
  number={11},
  pages={132--137},
  year={2008},
  publisher={IEEE}
}




	@inproceedings{mahajan2006urban,
  title={Urban mobility models for vanets},
  author={Mahajan, Atulya and Potnis, Niranjan and Gopalan, Kartik and Wang, Andy},
  booktitle={2nd IEEE International Workshop on Next Generation Wireless Networks},
  volume={33},
  year={2006}
}

@inproceedings{Rakhshan2016packet,
  title={Packet success probability derivation in a vehicular ad hoc network for a highway scenario},
  author={Rakhshan, Ali and Pishro-Nik, Hossein},
  booktitle={2016 Annual Conference on Information Science and Systems (CISS)},
  pages={210--215},
  year={2016},
  organization={IEEE}
}

@inproceedings{Rakhshan2016CISS,
	Author = {Rakhshan, Ali and Pishro-Nik, Hossein},
	Booktitle = {Conference on Information Sciences and Systems},
	Organization = {IEEE},
	Pages = {210--215},
	Title = {Packet Success Probability Derivation in a Vehicular Ad Hoc Network for a Highway Scenario},
	Year = {2016}}

@article{Nekoui2013Journal,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Journal = {Journal on Selected Areas in Communications, Special Issue on Emerging Technologies in Communications},
	Number = {9},
	Pages = {491--503},
	Publisher = {IEEE},
	Title = {Analytic Design of Active Safety Systems for Vehicular Ad hoc Networks},
	Volume = {31},
	Year = {2013}}


@inproceedings{Nekoui2011MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM workshop on VehiculAr InterNETworking},
	Organization = {ACM},
	Title = {Analytic Design of Active Vehicular Safety Systems in Sparse Traffic},
	Year = {2011}}

@inproceedings{Nekoui2011VTC,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Analytical Design of Inter-vehicular Communications for Collision Avoidance},
	Year = {2011}}

@inproceedings{Bovee2011VTC,
	Author = {Bovee, Ben Louis and Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {VTC-Fall},
	Organization = {IEEE},
	Title = {Evaluation of the Universal Geocast Scheme For VANETs},
	Year = {2011}}

@inproceedings{Nekoui2010MOBICOM,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {MOBICOM},
	Organization = {ACM},
	Title = {Fundamental Tradeoffs in Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2010IVCS,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IVCS},
	Organization = {IEEE},
	Title = {A Universal Geocast Scheme for Vehicular Ad Hoc Networks},
	Year = {2010}}

@inproceedings{Nekoui2009ITW,
	Author = {Nekoui, Mohammad and Pishro-Nik, Hossein},
	Booktitle = {IEEE Communications Society Conference on Sensor, Mesh and Ad Hoc Communications and Networks Workshops},
	Organization = {IEEE},
	Pages = {1--3},
	Title = {A Geometrical Analysis of Obstructed Wireless Networks},
	Year = {2009}}

@article{Eslami2013Journal,
	Author = {Eslami, Ali and Nekoui, Mohammad and Pishro-Nik, Hossein and Fekri, Faramarz},
	Journal = {ACM Transactions on Sensor Networks},
	Number = {4},
	Pages = {51},
	Publisher = {ACM},
	Title = {Results on finite wireless sensor networks: Connectivity and coverage},
	Volume = {9},
	Year = {2013}}


@article{Jiafu2014Journal,
	Author = {Jiafu, W. and Zhang, D. and Zhao, S. and Yang, L. and Lloret, J.},
	Journal = {Communications Magazine},
	Number = {8},
	Pages = {106-113},
	Publisher = {IEEE},
	Title = {Context-aware vehicular cyber-physical systems with cloud support: architecture, challenges, and solutions},
	Volume = {52},
	Year = {2014}}

@inproceedings{Haas2010ACM,
	Author = {Haas, J.J. and Hu, Y.},
	Booktitle = {international workshop on VehiculAr InterNETworking},
	Organization = {ACM},
	Title = {Communication requirements for crash avoidance.},
	Year = {2010}}

@inproceedings{Yi2008GLOBECOM,
	Author = {Yi, Q. and Lu, K. and Moayeri, N.},
	Booktitle = {GLOBECOM},
	Organization = {IEEE},
	Title = {CA Secure VANET MAC Protocol for DSRC Applications.},
	Year = {2008}}

@inproceedings{Mughal2010ITSim,
	Author = {Mughal, B.M. and Wagan, A. and Hasbullah, H.},
	Booktitle = {International Symposium on Information Technology (ITSim)},
	Organization = {IEEE},
	Title = {Efficient congestion control in VANET for safety messaging.},
	Year = {2010}}

@article{Chang2011Journal,
	Author = {Chang, Y. and Lee, C. and Copeland, J.},
	Journal = {Selected Areas in Communications},
	Pages = {236 –249},
	Publisher = {IEEE},
	Title = {Goodput enhancement of VANETs in noisy CSMA/CA channels},
	Volume = {29},
	Year = {2011}}

@article{Garcia-Costa2011Journal,
	Author = {Garcia-Costa, C. and Egea-Lopez, E. and Tomas-Gabarron, J. B. and Garcia-Haro, J. and Haas, Z. J.},
	Journal = {Transactions on Intelligent Transportation Systems},
	Pages = {1 –16},
	Publisher = {IEEE},
	Title = {A stochastic model for chain collisions of vehicles equipped with vehicular communications},
	Volume = {99},
	Year = {2011}}

@article{Carbaugh2011Journal,
	Author = {Carbaugh, J. and Godbole,  D. N. and Sengupta, R. and Garcia-Haro, J. and Haas, Z. J.},
	Publisher = {Transportation Research Part C (Emerging Technologies)},
	Title = {Safety and capacity analysis of automated and manual highway systems},
	Year = {1997}}

@article{Goh2004Journal,
	Author = {Goh, P. and Wong, Y.},
	Publisher = {Appl Health Econ Health Policy},
	Title = {Driver perception response time during the signal change interval},
	Year = {2004}}

@article{Chang1985Journal,
	Author = {Chang, M.S. and Santiago, A.J.},
	Pages = {20-30},
	Publisher = {Transportation Research Record},
	Title = {Timing traffic signal changes based on driver behavior},
	Volume = {1027},
	Year = {1985}}

@article{Green2000Journal,
	Author = {Green, M.},
	Pages = {195-216},
	Publisher = {Transportation Human Factors},
	Title = {How long does it take to stop? Methodological analysis of driver perception-brake times.},
	Year = {2000}}

@article{Koppa2005,
	Author = {Koppa, R.J.},
	Pages = {195-216},
	Publisher = {http://www.fhwa.dot.gov/publications/},
	Title = {Human Factors},
	Year = {2005}}

@inproceedings{Maxwell2010ETC,
	Author = {Maxwell, A. and Wood, K.},
	Booktitle = {Europian Transport Conference},
	Organization = {http://www.etcproceedings.org/paper/review-of-traffic-signals-on-high-speed-roads},
	Title = {Review of Traffic Signals on High Speed Road},
	Year = {2010}}

@article{Wortman1983,
	Author = {Wortman, R.H. and Matthias, J.S.},
	Publisher = {Arizona Department of Transportation},
	Title = {An Evaluation of Driver Behavior at Signalized Intersections},
	Year = {1983}}
@inproceedings{Zhang2007IASTED,
	Author = {Zhang, X. and Bham, G.H.},
	Booktitle = {18th IASTED International Conference: modeling and simulation},
	Title = {Estimation of driver reaction time from detailed vehicle trajectory data.},
	Year = {2007}}


@inproceedings{bai2003important,
  title={IMPORTANT: A framework to systematically analyze the Impact of Mobility on Performance of RouTing protocols for Adhoc NeTworks},
  author={Bai, Fan and Sadagopan, Narayanan and Helmy, Ahmed},
  booktitle={INFOCOM 2003. Twenty-second annual joint conference of the IEEE computer and communications. IEEE societies},
  volume={2},
  pages={825--835},
  year={2003},
  organization={IEEE}
}


@inproceedings{abedi2008enhancing,
	  title={Enhancing AODV routing protocol using mobility parameters in VANET},
	  author={Abedi, Omid and Fathy, Mahmood and Taghiloo, Jamshid},
	  booktitle={Computer Systems and Applications, 2008. AICCSA 2008. IEEE/ACS International Conference on},
	  pages={229--235},
	  year={2008},
	  organization={IEEE}
	}


@article{AlSultan2013Journal,
	Author = {Al-Sultan, Saif and Al-Bayatti, Ali H. and Zedan, Hussien},
	Journal = {IEEE Transactions on Vehicular Technology},
	Number = {9},
	Pages = {4264-4275},
	Publisher = {IEEE},
	Title = {Context Aware Driver Behaviour Detection System in Intelligent Transportation Systems},
	Volume = {62},
	Year = {2013}}






@article{Leow2008ITS,
	Author = {Leow, Woei Ling and Ni, Daiheng and Pishro-Nik, Hossein},
	Journal = {IEEE Transactions on Intelligent Transportation Systems},
	Number = {2},
	Pages = {369--374},
	Publisher = {IEEE},
	Title = {A Sampling Theorem Approach to Traffic Sensor Optimization},
	Volume = {9},
	Year = {2008}}



@article{REU2007,
	Author = {D. Ni and H. Pishro-Nik and R. Prasad and M. R. Kanjee and H. Zhu and T. Nguyen},
	Journal = {in 14th World Congress on Intelligent Transport Systems},
	Title = {Development of a prototype intersection collision avoidance system under VII},
	Year = {2007}}




@inproceedings{salamatian2013hide,
  title={How to hide the elephant-or the donkey-in the room: Practical privacy against statistical inference for large data.},
  author={Salamatian, Salman and Zhang, Amy and du Pin Calmon, Flavio and Bhamidipati, Sandilya and Fawaz, Nadia and Kveton, Branislav and Oliveira, Pedro and Taft, Nina},
  booktitle={GlobalSIP},
  pages={269--272},
  year={2013}
}

@article{sankar2013utility,
  title={Utility-privacy tradeoffs in databases: An information-theoretic approach},
  author={Sankar, Lalitha and Rajagopalan, S Raj and Poor, H Vincent},
  journal={Information Forensics and Security, IEEE Transactions on},
  volume={8},
  number={6},
  pages={838--852},
  year={2013},
  publisher={IEEE}
}
@inproceedings{ghinita2007prive,
  title={PRIVE: anonymous location-based queries in distributed mobile systems},
  author={Ghinita, Gabriel and Kalnis, Panos and Skiadopoulos, Spiros},
  booktitle={Proceedings of the 16th international conference on World Wide Web},
  pages={371--380},
  year={2007},
  organization={ACM}
}

@article{beresford2004mix,
  title={Mix zones: User privacy in location-aware services},
  author={Beresford, Alastair R and Stajano, Frank},
  year={2004},
  publisher={IEEE}
}

%@inproceedings{Mont1610Achieving,
%  title={Achieving Perfect Location Privacy in Markov Models Using Anonymization},
%  author={Montazeri, Zarrin and Houmansadr, Amir and H.Pishro-Nik},
%  booktitle="2016 International Symposium on Information Theory and its Applications
%  (ISITA2016)",
%  address="Monterey, USA",
%  days=30,
%  month=oct,
%  year=2016,
%}

@article{csiszar1996almost,
  title={Almost independence and secrecy capacity},
  author={Csisz{\'a}r, Imre},
  journal={Problemy Peredachi Informatsii},
  volume={32},
  number={1},
  pages={48--57},
  year={1996},
  publisher={Russian Academy of Sciences, Branch of Informatics, Computer Equipment and Automatization}
}

@article{yamamoto1983source,
  title={A source coding problem for sources with additional outputs to keep secret from the receiver or wiretappers (corresp.)},
  author={Yamamoto, Hirosuke},
  journal={IEEE Transactions on Information Theory},
  volume={29},
  number={6},
  pages={918--923},
  year={1983},
  publisher={IEEE}
}


@inproceedings{calmon2015fundamental,
  title={Fundamental limits of perfect privacy},
  author={Calmon, Flavio P and Makhdoumi, Ali and M{\'e}dard, Muriel},
  booktitle={Information Theory (ISIT), 2015 IEEE International Symposium on},
  pages={1796--1800},
  year={2015},
  organization={IEEE}
}



@inproceedings{Lehman1999Large-Sample-Theory,
	title={Elements of Large Sample Theory},
	author={E. L. Lehman},
	organization={Springer},
	year={1999}
}


@inproceedings{Ferguson1999Large-Sample-Theory,
	title={A Course in Large Sample Theory},
	author={Thomas S. Ferguson},
	organization={CRC Press},
	year={1996}
}



@inproceedings{Dembo1999Large-Deviations,
	title={Large Deviation Techniques and Applications, Second Edition},
	author={A. Dembo and O. Zeitouni},
	organization={Springer},
	year={1998}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Hossein's Coding Journals
%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{myoptics,
  AUTHOR =       "H. Pishro-Nik and N. Rahnavard and J. Ha and F. Fekri and A. Adibi ",
  TITLE =        "Low-density parity-check codes for volume holographic memory systems",
  JOURNAL =      " Appl. Opt.",
  YEAR =         "2003",
  volume =       "42",
  pages =        "861-870  "
 }






@ARTICLE{myit,
  AUTHOR =       "H. Pishro-Nik and F. Fekri  ",
  TITLE =        "On Decoding of Low-Density Parity-Check Codes on the Binary Erasure Channel",
  JOURNAL =      "IEEE Trans. Inform. Theory",
  YEAR =         "2004",
  volume =       "50",
  pages =        "439--454"
  }




@ARTICLE{myitpuncture,
  AUTHOR =       "H. Pishro-Nik and F. Fekri  ",
  TITLE =        "Results on Punctured Low-Density Parity-Check Codes and Improved Iterative Decoding Techniques",
  JOURNAL =      "IEEE Trans. on Inform. Theory",
  YEAR =         "2007",
  volume =       "53",
  number=        "2",
  pages =        "599--614",
  month= "February"
  }




@ARTICLE{myitlinmimdist,
  AUTHOR =       "H. Pishro-Nik and F. Fekri",
  TITLE =        "Performance of Low-Density Parity-Check Codes With Linear Minimum Distance",
  JOURNAL =         "IEEE Trans. Inform. Theory ",
  YEAR =         "2006",
  volume =       "52",
  number="1",
  pages =        "292 --300"
  }






@ARTICLE{myitnonuni,
  AUTHOR =       "H. Pishro-Nik and N. Rahnavard and F. Fekri  ",
  TITLE =        "Non-uniform Error Correction Using Low-Density Parity-Check Codes",
  JOURNAL =      "IEEE Trans. Inform. Theory",
  YEAR =         "2005",
  volume =       "51",
  number=  "7",
  pages =        "2702--2714"
 }





@article{eslamitcomhybrid10,
 author = {A. Eslami and S. Vangala and H. Pishro-Nik},
 title = {Hybrid channel codes for highly efficient FSO/RF communication systems},
 journal = {IEEE Transactions on Communications},
 volume = {58},
 number = {10},
 year = {2010},
 pages = {2926--2938},
 }


@article{eslamitcompolar13,
 author = {A. Eslami and H. Pishro-Nik},
 title = {On Finite-Length Performance of Polar Codes: Stopping Sets, Error Floor, and Concatenated Design},
 journal = {IEEE Transactions on Communications},
 volume = {61},
 number = {13},
 year = {2013},
 pages = {919--929},
 }



 @article{saeeditcom11,
 author = {H. Saeedi and H. Pishro-Nik and  A. H. Banihashemi},
 title = {Successive maximization for the systematic design of universally capacity approaching rate-compatible
 sequences of LDPC code ensembles over binary-input output-symmetric memoryless channels},
 journal = {IEEE Transactions on Communications},
 year = {2011},
 volume={59},
 number = {7}
 }


@article{rahnavard07,
 author = {Rahnavard, N. and Pishro-Nik, H. and Fekri, F.},
 title = {Unequal Error Protection Using Partially Regular LDPC Codes},
 journal = {IEEE Transactions on Communications},
 year = {2007},
 volume = {55},
 number = {3},
 pages = {387 -- 391}
 }


 @article{hosseinira04,
 author = {H. Pishro-Nik and F. Fekri},
 title = {Irregular repeat-accumulate codes for volume holographic memory systems},
 journal = {Journal of Applied Optics},
 year = {2004},
 volume = {43},
 number = {27},
 pages = {5222--5227},
 }


@article{azadeh2015Ephemeralkey,
 author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
 title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
 journal = {IEEE Transactions on Wireless Communications},
 year = {2015},
 volume = {14},
 number = {11},
 pages = {6072--6081},
}


@article{azadeh2014Everlasting,
 author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
 title = {Everlasting secrecy in disadvantaged wireless environments against sophisticated eavesdroppers},
 journal = {48th Asilomar Conference on Signals, Systems and Computers},
 year = {2014},
 pages = {1994--1998},
}


@article{azadeh2013ISIT,
 author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
 title = {Artificial intersymbol interference (ISI) to exploit receiver imperfections for secrecy},
 journal = {IEEE International Symposium on Information Theory (ISIT)},
 year = {2013},
}


@article{azadeh2013Jsac,
 author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
 title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
 journal = {IEEE Journal on Selected Areas in Communications},
 year = {2013},
 volume = {31},
 number = {9},
 pages = {1828--1839},
}


@article{azadeh2012Allerton,
 author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
 title = {Exploiting the non-commutativity of nonlinear operators for information-theoretic security in disadvantaged wireless environments},
 journal = {50th Annual Allerton Conference on Communication, Control, and Computing},
 year = {2012},
 pages = {233--240},
}


@article{azadeh2012Infocom,
 author = {A. Sheikholeslami and D. Goeckel and H. Pishro-Nik},
 title = {Jamming Based on an Ephemeral Key to Obtain Everlasting Security in Wireless Environments},
 journal = {IEEE INFOCOM},
 year = {2012},
 pages = {1179--1187},
}

@article{1corser2016evaluating,
  title={Evaluating Location Privacy in Vehicular Communications and Applications},
  author={Corser, George P and Fu, Huirong and Banihani, Abdelnasser},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={17},
  number={9},
  pages={2658-2667},
  year={2016},
  publisher={IEEE}
}
@article{2zhang2016designing,
  title={On Designing Satisfaction-Ratio-Aware Truthful Incentive Mechanisms for k-Anonymity Location Privacy},
  author={Zhang, Yuan and Tong, Wei and Zhong, Sheng},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={11},
  number={11},
  pages={2528--2541},
  year={2016},
  publisher={IEEE}
}
@article{3li2016privacy,
  title={Privacy-preserving Location Proof for Securing Large-scale Database-driven Cognitive Radio Networks},
  author={Li, Yi and Zhou, Lu and Zhu, Haojin and Sun, Limin},
  journal={IEEE Internet of Things Journal},
  volume={3},
  number={4},
  pages={563-571},
  year={2016},
  publisher={IEEE}
}
@article{4olteanu2016quantifying,
  title={Quantifying Interdependent Privacy Risks with Location Data},
  author={Olteanu, Alexandra-Mihaela and Huguenin, K{\'e}vin and Shokri, Reza and Humbert, Mathias and Hubaux, Jean-Pierre},
  journal={IEEE Transactions on Mobile Computing},
  year={2016},
  volume={PP},
  number={99},
  pages={1-1},
  publisher={IEEE}
}
@article{5yi2016practical,
  title={Practical Approximate k Nearest Neighbor Queries with Location and Query Privacy},
  author={Yi, Xun and Paulet, Russell and Bertino, Elisa and Varadharajan, Vijay},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={28},
  number={6},
  pages={1546--1559},
  year={2016},
  publisher={IEEE}
}
@article{6li2016privacy,
  title={Privacy Leakage of Location Sharing in Mobile Social Networks: Attacks and Defense},
  author={Li, Huaxin and Zhu, Haojin and Du, Suguo and Liang, Xiaohui and Shen, Xuemin},
  journal={IEEE Transactions on Dependable and Secure Computing},
  year={2016},
  volume={PP},
  number={99},
  publisher={IEEE}
}

@article{7murakami2016localization,
  title={Localization Attacks Using Matrix and Tensor Factorization},
  author={Murakami, Takao and Watanabe, Hajime},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={11},
  number={8},
  pages={1647--1660},
  year={2016},
  publisher={IEEE}
}
@article{8zurbaran2015near,
  title={Near-Rand: Noise-based Location Obfuscation Based on Random Neighboring Points},
  author={Zurbaran, Mayra Alejandra and Avila, Karen and Wightman, Pedro and Fernandez, Michael},
  journal={IEEE Latin America Transactions},
  volume={13},
  number={11},
  pages={3661--3667},
  year={2015},
  publisher={IEEE}
}

@article{9tan2014anti,
  title={An anti-tracking source-location privacy protection protocol in wsns based on path extension},
  author={Tan, Wei and Xu, Ke and Wang, Dan},
  journal={IEEE Internet of Things Journal},
  volume={1},
  number={5},
  pages={461--471},
  year={2014},
  publisher={IEEE}
}

@article{10peng2014enhanced,
  title={Enhanced Location Privacy Preserving Scheme in Location-Based Services},
  author={Peng, Tao and Liu, Qin and Wang, Guojun},
  journal={IEEE Systems Journal},
  year={2014},
  volume={PP},
  number={99},
  pages={1-12},
  publisher={IEEE}
}
@article{11dewri2014exploiting,
  title={Exploiting service similarity for privacy in location-based search queries},
  author={Dewri, Rinku and Thurimella, Ramakrisha},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={25},
  number={2},
  pages={374--383},
  year={2014},
  publisher={IEEE}
}

@article{12hwang2014novel,
  title={A novel time-obfuscated algorithm for trajectory privacy protection},
  author={Hwang, Ren-Hung and Hsueh, Yu-Ling and Chung, Hao-Wei},
  journal={IEEE Transactions on Services Computing},
  volume={7},
  number={2},
  pages={126--139},
  year={2014},
  publisher={IEEE}
}
@article{13puttaswamy2014preserving,
  title={Preserving location privacy in geosocial applications},
  author={Puttaswamy, Krishna PN and Wang, Shiyuan and Steinbauer, Troy and Agrawal, Divyakant and El Abbadi, Amr and Kruegel, Christopher and Zhao, Ben Y},
  journal={IEEE Transactions on Mobile Computing},
  volume={13},
  number={1},
  pages={159--173},
  year={2014},
  publisher={IEEE}
}

@article{14zhang2014privacy,
  title={Privacy quantification model based on the Bayes conditional risk in Location-Based Services},
  author={Zhang, Xuejun and Gui, Xiaolin and Tian, Feng and Yu, Si and An, Jian},
  journal={Tsinghua Science and Technology},
  volume={19},
  number={5},
  pages={452--462},
  year={2014},
  publisher={TUP}
}

@article{15bilogrevic2014privacy,
  title={Privacy-preserving optimal meeting location determination on mobile devices},
  author={Bilogrevic, Igor and Jadliwala, Murtuza and Joneja, Vishal and Kalkan, K{\"u}bra and Hubaux, Jean-Pierre and Aad, Imad},
  journal={IEEE transactions on information forensics and security},
  volume={9},
  number={7},
  pages={1141--1156},
  year={2014},
  publisher={IEEE}
}
@article{16haghnegahdar2014privacy,
  title={Privacy Risks in Publishing Mobile Device Trajectories},
  author={Haghnegahdar, Alireza and Khabbazian, Majid and Bhargava, Vijay K},
  journal={IEEE Wireless Communications Letters},
  volume={3},
  number={3},
  pages={241--244},
  year={2014},
  publisher={IEEE}
}
@article{17malandrino2014verification,
  title={Verification and inference of positions in vehicular networks through anonymous beaconing},
  author={Malandrino, Francesco and Borgiattino, Carlo and Casetti, Claudio and Chiasserini, Carla-Fabiana and Fiore, Marco and Sadao, Roberto},
  journal={IEEE Transactions on Mobile Computing},
  volume={13},
  number={10},
  pages={2415--2428},
  year={2014},
  publisher={IEEE}
}
@article{18shokri2014hiding,
  title={Hiding in the mobile crowd: Locationprivacy through collaboration},
  author={Shokri, Reza and Theodorakopoulos, George and Papadimitratos, Panos and Kazemi, Ehsan and Hubaux, Jean-Pierre},
  journal={IEEE transactions on dependable and secure computing},
  volume={11},
  number={3},
  pages={266--279},
  year={2014},
  publisher={IEEE}
}
@article{19freudiger2013non,
  title={Non-cooperative location privacy},
  author={Freudiger, Julien and Manshaei, Mohammad Hossein and Hubaux, Jean-Pierre and Parkes, David C},
  journal={IEEE Transactions on Dependable and Secure Computing},
  volume={10},
  number={2},
  pages={84--98},
  year={2013},
  publisher={IEEE}
}
@article{20gao2013trpf,
  title={TrPF: A trajectory privacy-preserving framework for participatory sensing},
  author={Gao, Sheng and Ma, Jianfeng and Shi, Weisong and Zhan, Guoxing and Sun, Cong},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={8},
  number={6},
  pages={874--887},
  year={2013},
  publisher={IEEE}
}
@article{21ma2013privacy,
  title={Privacy vulnerability of published anonymous mobility traces},
  author={Ma, Chris YT and Yau, David KY and Yip, Nung Kwan and Rao, Nageswara SV},
  journal={IEEE/ACM Transactions on Networking},
  volume={21},
  number={3},
  pages={720--733},
  year={2013},
  publisher={IEEE}
}
@article{22niu2013pseudo,
  title={Pseudo-Location Updating System for privacy-preserving location-based services},
  author={Niu, Ben and Zhu, Xiaoyan and Chi, Haotian and Li, Hui},
  journal={China Communications},
  volume={10},
  number={9},
  pages={1--12},
  year={2013},
  publisher={IEEE}
}
@article{23dewri2013local,
  title={Local differential perturbations: Location privacy under approximate knowledge attackers},
  author={Dewri, Rinku},
  journal={IEEE Transactions on Mobile Computing},
  volume={12},
  number={12},
  pages={2360--2372},
  year={2013},
  publisher={IEEE}
}
@inproceedings{24kanoria2012tractable,
  title={Tractable bayesian social learning on trees},
  author={Kanoria, Yashodhan and Tamuz, Omer},
  booktitle={Information Theory Proceedings (ISIT), 2012 IEEE International Symposium on},
  pages={2721--2725},
  year={2012},
  organization={IEEE}
}
@inproceedings{25farias2005universal,
  title={A universal scheme for learning},
  author={Farias, Vivek F and Moallemi, Ciamac C and Van Roy, Benjamin and Weissman, Tsachy},
  booktitle={Proceedings. International Symposium on Information Theory, 2005. ISIT 2005.},
  pages={1158--1162},
  year={2005},
  organization={IEEE}
}
@inproceedings{26misra2013unsupervised,
  title={Unsupervised learning and universal communication},
  author={Misra, Vinith and Weissman, Tsachy},
  booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
  pages={261--265},
  year={2013},
  organization={IEEE}
}
@inproceedings{27ryabko2013time,
  title={Time-series information and learning},
  author={Ryabko, Daniil},
  booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
  pages={1392--1395},
  year={2013},
  organization={IEEE}
}
@inproceedings{28krzakala2013phase,
  title={Phase diagram and approximate message passing for blind calibration and dictionary learning},
  author={Krzakala, Florent and M{\'e}zard, Marc and Zdeborov{\'a}, Lenka},
  booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
  pages={659--663},
  year={2013},
  organization={IEEE}
}
@inproceedings{29sakata2013sample,
  title={Sample complexity of Bayesian optimal dictionary learning},
  author={Sakata, Ayaka and Kabashima, Yoshiyuki},
  booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
  pages={669--673},
  year={2013},
  organization={IEEE}
}
@inproceedings{30predd2004consistency,
  title={Consistency in a model for distributed learning with specialists},
  author={Predd, Joel B and Kulkarni, Sanjeev R and Poor, H Vincent},
  booktitle={IEEE International Symposium on Information Theory},
  year={2004},
organization={IEEE}
}
@inproceedings{31nokleby2016rate,
  title={Rate-Distortion Bounds on Bayes Risk in Supervised Learning},
  author={Nokleby, Matthew and Beirami, Ahmad and Calderbank, Robert},
  booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
pages={2099-2103},
  year={2016},
organization={IEEE}
}

@inproceedings{32le2016imperfect,
  title={Are imperfect reviews helpful in social learning?},
  author={Le, Tho Ngoc and Subramanian, Vijay G and Berry, Randall A},
  booktitle={Information Theory (ISIT), 2016 IEEE International Symposium on},
  pages={2089--2093},
  year={2016},
  organization={IEEE}
}
@inproceedings{33gadde2016active,
  title={Active Learning for Community Detection in Stochastic Block Models},
  author={Gadde, Akshay and Gad, Eyal En and Avestimehr, Salman and Ortega, Antonio},
  booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
  pages={1889-1893},
  year={2016}
}
@inproceedings{34shakeri2016minimax,
  title={Minimax Lower Bounds for Kronecker-Structured Dictionary Learning},
  author={Shakeri, Zahra and Bajwa, Waheed U and Sarwate, Anand D},
  booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
  pages={1148-1152},
  year={2016}
}
@article{35lee2015speeding,
  title={Speeding up distributed machine learning using codes},
  author={Lee, Kangwook and Lam, Maximilian and Pedarsani, Ramtin and Papailiopoulos, Dimitris and Ramchandran, Kannan},
  booktitle={2016 IEEE International Symposium on Information Theory (ISIT)},
  pages={1143-1147},
  year={2016}
}
@article{36oneto2016statistical,
  title={Statistical Learning Theory and ELM for Big Social Data Analysis},
  author={Oneto, Luca and Bisio, Federica and Cambria, Erik and Anguita, Davide},
  journal={ieee CompUTATionAl inTelliGenCe mAGAzine},
  volume={11},
  number={3},
  pages={45--55},
  year={2016},
  publisher={IEEE}
}
@article{37lin2015probabilistic,
  title={Probabilistic approach to modeling and parameter learning of indirect drive robots from incomplete data},
  author={Lin, Chung-Yen and Tomizuka, Masayoshi},
  journal={IEEE/ASME Transactions on Mechatronics},
  volume={20},
  number={3},
  pages={1036--1045},
  year={2015},
  publisher={IEEE}
}
@article{38wang2016towards,
  title={Towards Bayesian Deep Learning: A Framework and Some Existing Methods},
  author={Wang, Hao and Yeung, Dit-Yan},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={PP},
  number={99},
  year={2016},
  publisher={IEEE}
}


%%%%%Informationtheoreticsecurity%%%%%%%%%%%%%%%%%%%%%%%




@inproceedings{Bloch2011PhysicalSecBook,
	title={Physical-Layer Security},
	author={M. Bloch and J. Barros},
	organization={Cambridge University Press},
	year={2011}
}



@inproceedings{Liang2009InfoSecBook,
	title={Information Theoretic Security},
	author={Y. Liang and H. V. Poor and S. Shamai (Shitz)},
	organization={Now Publishers Inc.},
	year={2009}
}


@inproceedings{Zhou2013PhysicalSecBook,
	title={Physical Layer Security in Wireless Communications},
	author={ X. Zhou and L. Song and Y. Zhang},
	organization={CRC Press},
	year={2013}
}

@article{Ni2012IEA,
	Author = {D. Ni and H. Liu and W. Ding and  Y. Xie and H. Wang and H. Pishro-Nik and Q. Yu},
	Journal = {IEA/AIE},
	Title = {Cyber-Physical Integration to Connect Vehicles for Transformed Transportation Safety and Efficiency},
	Year = {2012}}



@inproceedings{Ni2012Inproceedings,
	Author = {D. Ni, H. Liu, Y. Xie, W. Ding, H. Wang, H. Pishro-Nik, Q. Yu and M. Ferreira},
	Booktitle = {Spring Simulation Multiconference},
	Date-Added = {2016-09-04 14:18:42 +0000},
	Date-Modified = {2016-09-06 16:22:14 +0000},
	Title = {Virtual Lab of Connected Vehicle Technology},
	Year = {2012}}

@inproceedings{Ni2012Inproceedings,
	Author = {D. Ni, H. Liu, W. Ding, Y. Xie, H. Wang, H. Pishro-Nik and Q. Yu,},
	Booktitle = {IEA/AIE},
	Date-Added = {2016-09-04 09:11:02 +0000},
	Date-Modified = {2016-09-06 14:46:53 +0000},
	Title = {Cyber-Physical Integration to Connect Vehicles for Transformed Transportation Safety and Efficiency},
	Year = {2012}}


@article{Nekoui_IJIPT_2009,
	Author = {M. Nekoui and D. Ni and H. Pishro-Nik and R. Prasad and M. Kanjee and H. Zhu and T. Nguyen},
	Journal = {International Journal of Internet Protocol Technology (IJIPT)},
	Number = {3},
	Pages = {},
	Publisher = {},
	Title = {Development of a VII-Enabled Prototype Intersection Collision Warning System},
	Volume = {4},
	Year = {2009}}


@inproceedings{Pishro_Ganz_Ni,
	Author = {H. Pishro-Nik, A. Ganz, and Daiheng Ni},
	Booktitle = {Forty-Fifth Annual Allerton Conference on Communication, Control, and Computing. Allerton House, Monticello, IL},
	Date-Added = {},
	Date-Modified = {},
	Number = {},
	Pages = {},
	Title = {The capacity of vehicular ad hoc networks},
	Volume = {},
	Year = {September 26-28, 2007}}

@inproceedings{Leow_Pishro_Ni_1,
	Author = {W. L. Leow, H. Pishro-Nik and Daiheng Ni},
	Booktitle = {IEEE Global Telecommunications Conference, Washington, D.C.},
	Date-Added = {},
	Date-Modified = {},
	Number = {},
	Pages = {},
	Title = {Delay and Energy Tradeoff in Multi-state Wireless Sensor Networks},
	Volume = {},
	Year = {November 26-30, 2007}}


@misc{UMass-Trans,
title = {{UMass Transportation Center}},
note = {\url{http://www.umasstransportationcenter.org/}},
}


@inproceedings{Haenggi2013book,
	title={Stochastic geometry for wireless networks},
	author={M. Haenggi},
	organization={Cambridge Uinversity Press},
	year={2013}
}


==> relatedwork.tex <==
\section{Related Work}
\label{relatedwork}

Previously, mutual information has been used as a privacy metric in a number of settings,~\cite{salamatian2013hide, csiszar1996almost, calmon2015fundamental, sankar2013utility, sankarISIT,sankar, yamamoto1983source, hyposankar}. However, the framework and problem formulation for our setting (Internet of Things (IoT) privacy) is quite different from those encountered in previous work. More specifically, the IoT privacy problem we consider here is based on a large set of time-series data that belong to different users with different statistical patterns that has gone through a privacy-preserving mechanism, and the adversary is aiming at de-anonymizing and de-obfuscating the data.


Next, consider related works in smart-home/public environment Internet of Things (IoT) systems. The authors in \cite{8ukil2015privacy} investigate privacy for IoT smart energy metering where the concern results from the fact that any privacy breach can reveal in-house activity. A `Dynamic Privacy Analyzer' scheme is proposed as an attempt towards achieving a unique privacy metric that is derived from fundamental principles like robust statistics and information theory.
To deal with concerns in different smart-home IoT devices such as lights, smoke-alarms, power switches, baby monitors, and weighing scales, which again makes it possible for the entities to snoop and intrude into the family's activities, the authors in \cite{12sivaraman2015network} suggest that device-level protections be augmented with network-level security solutions. This can be achieved through software defined networking technology when used to dynamically block/quarantine suspicious devices. In \cite{10harris2016security}, the authors consider the privacy issues in public environments such as an IoT-enabled retail store. An IoT-enable retail store has the potential to provide rich, targeted information and services to users within the environment. However, to fully realize such potential, users must be willing to share certain data regarding their habits and preferences with the public IoT facility. To encourage users to share such information, the paper proposes a protocol to ensure the customers that their data will not be leaked to third parties.

As far as other applications of IoT is concerned, authors in \cite{9dalipi2016security} investigate privacy considerations for IoT applications on Smart Grids. In particular, the authors address three types of challenge domains: customer domain, information and communication domain, and the grid domain. In \cite{battery15}, the author tried to provide privacy for smart-metering systems with rechargeable batteries by obscuring the user's power demand.
In \cite{11al2015security}, the authors consider the privacy issue of wearable devices. These devices make it possible for health care services start a new phase in serving patients' needs and monitor their health remotely. Finally, authors in \cite{14sadeghi2015security}, overview the privacy challenges in  industrial IoT systems.

Among these applications, location privacy constitutes one of the most important aspects of IoT privacy. Location privacy preserving mechanisms (LPPMs) can be categorized into two main classes:
identity perturbation LPPMs (anonymization) ~\cite{1corser2016evaluating,hoh2005protecting,freudiger2007mix, ma2009location, shokri2011quantifying, Naini2016}
and location perturbation LPPMs (obfuscation)~\cite{shokri2012protecting, gruteser2003anonymous,  bordenabe2014optimal}.

There are various approaches suggested for identity perturbation LPPMs. Particularly,  k-anonymity approaches help to keep each user's identity indistinguishable within a group of $k-1$ other users ~\cite{1corser2016evaluating,2zhang2016designing,11dewri2014exploiting, gedik2005location, zhong2009distributed, mokbel2006new, sweeney2002k, bordenabe2014optimal, kalnis2007preventing,liu2013game}. Another proposal changes users' pseudonyms within areas called mix-zones~\cite{hoh2005protecting, beresford2003location, freudiger2009optimal, beresford2003location, palanisamy2011mobimix}. There are also various approaches used by location perturbation LPPMs.  For instance, cloaking replaces each user's location information with a larger region~\cite{18shokri2014hiding,8zurbaran2015near,hoh2007preserving, gruteser2003anonymous, gedik2005location, gedik2008protecting, bordenabe2014optimal, duckham2005formal, duckham2006spatiotemporal, xue2009location, wernke2014classification, cai2015cloaking, chow2011spatial, cheng2006preserving, mokbel2006new, kalnis2006preserving, khoshgozaran2011location, bamba2008supporting, um2010advanced, zhangwei2010distributed}, while an alternative direction is to use dummy locations in the set of possible locations of users~\cite{kido2005protection, krumm2009survey, shankar2009privately, chow2009faking, kido2005anonymous, lu2008pad}.
Some prior works combine techniques to achieve stronger location privacy. For instance, Freudiger et al.\ combine techniques from cryptography with mix-zones to improve location privacy~\cite{freudiger2007mix}.




Differential privacy, which aims at protecting queries on aggregated data, has also been applied to the problem of location privacy.
Particularly, several identity perturbation~\cite{lee2012differential, bordenabe2014optimal, chatzikokolakis2015geo, nguyen2013differential, machanavajjhala2008privacy} and location perturbation ~\cite{chatzikokolakis2013broadening,shokri2014optimal, chatzikokolakis2015location,andres2013geo,bordenabe2014optimal} LPPMs are based on differential privacy techniques.
Dewri~\cite{dewri2013local} combines k-anonymity and differential privacy to achieve higher location privacy. Alternatively, Andres et al.\ hide the exact location of a user in a region by adding Laplacian distributed noise  to achieve a desired level of geo-indistinguishability~\cite{andres2013geo}. In ~\cite{info2012}, it  is proved that differential privacy arises out of maximizing entropy principle which is equal to minimizing information leakage and is measured using the mutual information notion. ~\cite{yeb17} tries to reduce the expected estonimation loss by using differential privacy and constraining the privacy level.




Several studies aim at quantifying location privacy protection.  Shokri et al.~\cite{shokri2011quantifying, shokri2011quantifying2} define the expected estimation error of the adversary  as a metric to evaluate LPPM mechanisms.  Ma et al.~\cite{ma2009location}  use  uncertainty about users' location information to quantify user location privacy in vehicular networks.
To defeat localization attacks and achieve privacy at the same time, Shokri et al.~\cite{shokri2012protecting} proposed a method which finds optimal LPPM for an LBS given service quality constraints. Shokri et al.~\cite{shokri2012protecting} design LPPM mechanisms that will defeat localization attacks.
% To defeat localization attack and reach privacy at the same time, \cite{shokri2012protecting} proposed a method which finds optimal LPPM for LSB given service quality constraints.
In \cite{6li2016privacy} and \cite{4olteanu2016quantifying}, privacy leakage of location sharing and interdependent location privacy risks are quantified, respectively. A similar idea is proposed in \cite{14zhang2014privacy} where the quantification model is based on the Bayes conditional risk. Yu et al. \cite{diff2017} combine two complementary notations, geo-indstingushability and expected inference error, to achieve location privacy. The geo-indstingushability is derived from differential privacy but cannot adequately protect users' location against inference attacks of adversary by using prior information, and the expected inference error as privacy metric doesn't consider posterior information obtained from  pseudo-location. As a result, combining both notations gives users the opportunity to have location privacy. In addition, users are allowed to personalized error bound for different locations.

In \cite{5ullah2016novel}, the authors propose a novel model for preserving location privacy in IoT in which they propose the so-called Enhanced Semantic Obfuscation Technique (ESOT).
In \cite{7zhou2012preserving}, in the context of IoT based wireless sensor networks, the authors propose a flexible routing strategy, called Multi-routing Random Walk, which protects the sensor's location. Another approach has been proposed in \cite{6sathishkumar2016enhanced}.

The discussed studies demonstrate the growing importance of privacy. What is missing from the current literature is a solid theoretical framework for privacy that is general enough to encompass various privacy preserving methods in the literature. Such a framework will allow us to achieve provable privacy guarantees, obtain fundamental trade-offs between privacy and performance, and provide analytical tools to optimally achieve provable privacy.   The closest works to this paper are ~\cite{montazeri2016defining, Mont1610Achieving,tifs2016,sit2017,ciss2017}. As mentioned, these works only consider anonymization and only achiveability. In this paper, by considering obfuscation and anonymization, we characterize the limits of privacy in the entire $m(n)-a_n$ plane by considering both achievability and converse results.



























